Improved Code Summarization via a Graph Neural Network

Automatic source code summarization is the task of generating natural language descriptions for source code. Automatic code summarization is a rapidly expanding research area, especially as the community has taken greater advantage of advances in neural network and AI technologies. In general, source code summarization techniques use the source code as input and outputs a natural language description. Yet a strong consensus is developing that using structural information as input leads to improved performance. The first approaches to use structural information flattened the AST into a sequence. Recently, more complex approaches based on random AST paths or graph neural networks have improved on the models using flattened ASTs. However, the literature still does not describe the using a graph neural network together with source code sequence as separate inputs to a model. Therefore, in this paper, we present an approach that uses a graph-based neural architecture that better matches the default structure of the AST to generate these summaries. We evaluate our technique using a data set of 2.1 million Java method-comment pairs and show improvement over four baseline techniques, two from the software engineering literature, and two from machine learning literature.

==> main_bib_bak.tex <==
@inproceedings{chu2018survey,
	title={A Survey of Domain Adaptation for Neural Machine Translation},
	author={Chu, Chenhui and Wang, Rui},
	booktitle={Proceedings of the 27th International Conference on Computational Linguistics},
	pages={1304--1319},
	year={2018}
}

@article{weston2015towards,
	title={Towards ai-complete question answering: A set of prerequisite toy tasks},
	author={Weston, Jason and Bordes, Antoine and Chopra, Sumit and Rush, Alexander M and van Merri{\"e}nboer, Bart and Joulin, Armand and Mikolov, Tomas},
	journal={arXiv preprint arXiv:1502.05698},
	year={2015}
}

@article{liu2017survey,
	title={A survey of deep neural network architectures and their applications},
	author={Liu, Weibo and Wang, Zidong and Liu, Xiaohui and Zeng, Nianyin and Liu, Yurong and Alsaadi, Fuad E},
	journal={Neurocomputing},
	volume={234},
	pages={11--26},
	year={2017},
	publisher={Elsevier}
}

@article{chen2017survey,
	title={A survey on dialogue systems: Recent advances and new frontiers},
	author={Chen, Hongshen and Liu, Xiaorui and Yin, Dawei and Tang, Jiliang},
	journal={Acm Sigkdd Explorations Newsletter},
	volume={19},
	number={2},
	pages={25--35},
	year={2017},
	publisher={ACM}
}

@article{gao2019neural,
	title={Neural approaches to conversational AI},
	author={Gao, Jianfeng and Galley, Michel and Li, Lihong and others},
	journal={Foundations and Trends{\textregistered} in Information Retrieval},
	volume={13},
	number={2-3},
	pages={127--298},
	year={2019},
	publisher={Now Publishers, Inc.}
}

@inproceedings{malinowski2015ask,
	title={Ask your neurons: A neural-based approach to answering questions about images},
	author={Malinowski, Mateusz and Rohrbach, Marcus and Fritz, Mario},
	booktitle={Proceedings of the IEEE international conference on computer vision},
	pages={1--9},
	year={2015}
}

@inproceedings{yin2016neural,
	title={Neural generative question answering},
	author={Yin, Jun and Jiang, Xin and Lu, Zhengdong and Shang, Lifeng and Li, Hang and Li, Xiaoming},
	booktitle={Proceedings of the Twenty-Fifth International Joint Conference on Artificial Intelligence},
	pages={2972--2978},
	year={2016},
	organization={AAAI Press}
}

@inproceedings{ren2015faster,
	title={Faster r-cnn: Towards real-time object detection with region proposal networks},
	author={Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
	booktitle={Advances in neural information processing systems},
	pages={91--99},
	year={2015}
}

@article{young2018recent,
	title={Recent trends in deep learning based natural language processing},
	author={Young, Tom and Hazarika, Devamanyu and Poria, Soujanya and Cambria, Erik},
	journal={ieee Computational intelligenCe magazine},
	volume={13},
	number={3},
	pages={55--75},
	year={2018},
	publisher={IEEE}
}

@inproceedings{vaswani2017attention,
	title={Attention is all you need},
	author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
	booktitle={Advances in neural information processing systems},
	pages={5998--6008},
	year={2017}
}

@inproceedings{kuncoro2017recurrent,
	title={What Do Recurrent Neural Network Grammars Learn About Syntax?},
	author={Kuncoro, Adhiguna and Ballesteros, Miguel and Kong, Lingpeng and Dyer, Chris and Neubig, Graham and Smith, Noah A},
	booktitle={Proceedings of the 15th Conference of the European Chapter of the Association for Computational Linguistics: Volume 1, Long Papers},
	pages={1249--1258},
	year={2017}
}

@inproceedings{leclair2019neural,
	title={A neural model for generating natural language summaries of program subroutines},
	author={LeClair, Alexander and Jiang, Siyuan and McMillan, Collin},
	booktitle={Proceedings of the 41st International Conference on Software Engineering},
	pages={795--806},
	year={2019},
	organization={IEEE Press}
}

@incollection{ras2018explanation,
	title={Explanation methods in deep learning: Users, values, concerns and challenges},
	author={Ras, Gabri{\"e}lle and van Gerven, Marcel and Haselager, Pim},
	booktitle={Explainable and Interpretable Models in Computer Vision and Machine Learning},
	pages={19--36},
	year={2018},
	publisher={Springer}
}

@article{samek2017explainable,
	title={Explainable artificial intelligence: Understanding, visualizing and interpreting deep learning models},
	author={Samek, Wojciech and Wiegand, Thomas and M{\"u}ller, Klaus-Robert},
	journal={arXiv preprint arXiv:1708.08296},
	year={2017}
}

@inproceedings{hill2009automatically,
	title={Automatically capturing source code context of nl-queries for software maintenance and reuse},
	author={Hill, Emily and Pollock, Lori and Vijay-Shanker, K},
	booktitle={Proceedings of the 31st International Conference on Software Engineering},
	pages={232--242},
	year={2009},
	organization={IEEE Computer Society}
}

@inproceedings{doya1992bifurcations,
	title={Bifurcations in the learning of recurrent neural networks},
	author={Doya, Kenji},
	booktitle={[Proceedings] 1992 IEEE International Symposium on Circuits and Systems},
	volume={6},
	pages={2777--2780},
	year={1992},
	organization={IEEE}
}

@article{doya2003recurrent,
	title={Recurrent networks: learning algorithms},
	author={Doya, Kenji},
	journal={The Handbook of Brain Theory and Neural Networks,},
	pages={955--960},
	year={2003}
}

@article{xu2018graph2seq,
  title={Graph2seq: Graph to sequence learning with attention-based neural networks},
  author={Xu, Kun and Wu, Lingfei and Wang, Zhiguo and Feng, Yansong and Witbrock, Michael and Sheinin, Vadim},
  journal={arXiv preprint arXiv:1804.00823},
  year={2018}
}

@article{xu2018exploiting,
  title={Exploiting rich syntactic information for semantic parsing with graph-to-sequence model},
  author={Xu, Kun and Wu, Lingfei and Wang, Zhiguo and Yu, Mo and Chen, Liwei and Sheinin, Vadim},
 journal={Conference on Empirical Methods in Natural Language Processing},
year={2018}
}

@article{chen2019reinforcement,
  title={Reinforcement learning based graph-to-sequence model for natural question generation},
  author={Chen, Yu and Wu, Lingfei and Zaki, Mohammed J},
  journal={International Conference on Learning Representations},
  year={2020}
}

@inproceedings{leclair2019recommendations,
	title={Recommendations for Datasets for Source Code Summarization},
	author={LeClair, Alexander and McMillan, Collin},
	booktitle={Proceedings of the 2019 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)},
	pages={3931--3937},
	year={2019}
}

@inproceedings{nallapati2016abstractive,
	title={Abstractive Text Summarization using Sequence-to-sequence RNNs and Beyond},
	author={Nallapati, Ramesh and Zhou, Bowen and dos Santos, Cicero and Gulcehre, Caglar and Xiang, Bing},
	booktitle={Proceedings of The 20th SIGNLL Conference on Computational Natural Language Learning},
	pages={280--290},
	year={2016}
}

@inproceedings{Papineni:2002:BMA:1073083.1073135,
	author = {Papineni, Kishore and Roukos, Salim and Ward, Todd and Zhu, Wei-Jing},
	title = {BLEU: A Method for Automatic Evaluation of Machine Translation},
	booktitle = {Proceedings of the 40th Annual Meeting on Association for Computational Linguistics},
	series = {ACL '02},
	year = {2002},
	location = {Philadelphia, Pennsylvania},
	pages = {311--318},
	numpages = {8},
	url = {https://doi.org/10.3115/1073083.1073135},
	doi = {10.3115/1073083.1073135},
	acmid = {1073135},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
} 

@article{wu2019gnnsurvey,
  author    = {Zonghan Wu and
               Shirui Pan and
               Fengwen Chen and
               Guodong Long and
               Chengqi Zhang and
               Philip S. Yu},
  title     = {A Comprehensive Survey on Graph Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1901.00596},
  year      = {2019},
  url       = {http://arxiv.org/abs/1901.00596},
  archivePrefix = {arXiv},
  eprint    = {1901.00596},
  timestamp = {Thu, 31 Jan 2019 13:52:49 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1901-00596},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{alon2018code2seq,
	title={code2seq: Generating sequences from structured representations of code},
	author={Alon, Uri and Brody, Shaked and Levy, Omer and Yahav, Eran},
	journal={International Conference on Learning Representations},
	year={2019}
}

@article{allamanis2018learning,
	title={Learning to represent programs with graphs},
	author={Allamanis, Miltiadis and Brockschmidt, Marc and Khademi, Mahmoud},
	journal={International Conference on Learning Representations},
	year={2018}
}

@article{young2018recent,
	title={Recent trends in deep learning based natural language processing},
	author={Young, Tom and Hazarika, Devamanyu and Poria, Soujanya and Cambria, Erik},
	journal={ieee Computational intelligenCe magazine},
	volume={13},
	number={3},
	pages={55--75},
	year={2018},
	publisher={IEEE}
}

@article{shrestha2019review,
	title={Review of Deep Learning Algorithms and Architectures},
	author={Shrestha, Ajay and Mahmood, Ausif},
	journal={IEEE Access},
	volume={7},
	pages={53040--53065},
	year={2019},
	publisher={IEEE}
}

@article{pouyanfar2018survey,
	title={A survey on deep learning: Algorithms, techniques, and applications},
	author={Pouyanfar, Samira and Sadiq, Saad and Yan, Yilin and Tian, Haiman and Tao, Yudong and Reyes, Maria Presa and Shyu, Mei-Ling and Chen, Shu-Ching and Iyengar, SS},
	journal={ACM Computing Surveys (CSUR)},
	volume={51},
	number={5},
	pages={92},
	year={2018},
	publisher={ACM}
}

@article{mcburney2016automatic,
  title={Automatic source code summarization of context for java methods},
  author={McBurney, Paul W and McMillan, Collin},
  journal={IEEE Transactions on Software Engineering},
  volume={42},
  number={2},
  pages={103--119},
  year={2016},
  publisher={IEEE}
}

@article{Louis2018DeepLT,
	title={Deep Learning to Detect Redundant Method Comments},
	author={Annie Louis and Santanu Kumar Dash and Earl T. Barr and Charles A. Sutton},
	journal={CoRR},
	year={2018},
	volume={abs/1806.04616}
}

@inproceedings{papineni2002bleu,
	title={BLEU: a method for automatic evaluation of machine translation},
	author={Papineni, Kishore and Roukos, Salim and Ward, Todd and Zhu, Wei-Jing},
	booktitle={Proceedings of the 40th annual meeting on association for computational linguistics},
	pages={311--318},
	year={2002},
	organization={Association for Computational Linguistics}
}

@INPROCEEDINGS{6200082,
	author={S. H. Tan and D. Marinov and L. Tan and G. T. Leavens},
	booktitle={2012 IEEE Fifth International Conference on Software Testing, Verification and Validation},
	title={@tComment: Testing Javadoc Comments to Detect Comment-Code Inconsistencies},
	year={2012},
	volume={},
	number={},
	pages={260-269},
	keywords={application program interfaces;formal specification;Java;natural language processing;program testing;text analysis;@TCOMMENT;Javadoc comment testing;comment-code inconsistency detection;software artifact;API specification;English text analysis;Java;Contracts;Arrays;Libraries;Synchronization;Testing;Educational institutions;comment analysis;random testing;test generation},
	doi={10.1109/ICST.2012.106},
	ISSN={2159-4848},
	month={April}
}

@inproceedings{balog2017deepcoder,
	title={DeepCoder: Learning to Write Programs},
	author={Balog, M and Gaunt, AL and Brockschmidt, M and Nowozin, S and Tarlow, D},
	booktitle={International Conference on Learning Representations (ICLR 2017)},
	year={2017},
	organization={OpenReview. net}
}

@inproceedings{yu2019neural,
	title={Neural detection of semantic code clones via tree-based convolution},
	author={Yu, Hao and Lam, Wing and Chen, Long and Li, Ge and Xie, Tao and Wang, Qianxiang},
	booktitle={Proceedings of the 27th International Conference on Program Comprehension},
	pages={70--80},
	year={2019},
	organization={IEEE Press}
}

@inproceedings{zhang2019novel,
	title={A novel neural source code representation based on abstract syntax tree},
	author={Zhang, Jian and Wang, Xu and Zhang, Hongyu and Sun, Hailong and Wang, Kaixuan and Liu, Xudong},
	booktitle={Proceedings of the 41st International Conference on Software Engineering},
	pages={783--794},
	year={2019},
	organization={IEEE Press}
}

@article{hossain2019comprehensive,
	title={A comprehensive survey of deep learning for image captioning},
	author={Hossain, MD and Sohel, Ferdous and Shiratuddin, Mohd Fairuz and Laga, Hamid},
	journal={ACM Computing Surveys (CSUR)},
	volume={51},
	number={6},
	pages={118},
	year={2019},
	publisher={ACM}
}

@inproceedings{chen2017improved,
    title = "Improved Neural Machine Translation with a Syntax-Aware Encoder and Decoder",
    author = "Chen, Huadong  and
      Huang, Shujian  and
      Chiang, David  and
      Chen, Jiajun",
    booktitle = "Proceedings of the 55th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = jul,
    year = "2017",
    address = "Vancouver, Canada",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P17-1177",
    doi = "10.18653/v1/P17-1177",
    pages = "1936--1945",
    abstract = "Most neural machine translation (NMT) models are based on the sequential encoder-decoder framework, which makes no use of syntactic information. In this paper, we improve this model by explicitly incorporating source-side syntactic trees. More specifically, we propose (1) a bidirectional tree encoder which learns both sequential and tree structured representations; (2) a tree-coverage model that lets the attention depend on the source-side syntax. Experiments on Chinese-English translation demonstrate that our proposed models outperform the sequential attentional model as well as a stronger baseline with a bottom-up tree encoder and word coverage.",
}

@inproceedings{holmes2005using,
	title={Using structural context to recommend source code examples},
	author={Holmes, Reid and Murphy, Gail C},
	booktitle={Proceedings. 27th International Conference on Software Engineering, 2005. ICSE 2005.},
	pages={117--125},
	year={2005},
	organization={IEEE}
}

@inproceedings{collard2011lightweight,
	title={Lightweight transformation and fact extraction with the srcML toolkit},
	author={Collard, Michael L and Decker, Michael J and Maletic, Jonathan I},
	booktitle={Source Code Analysis and Manipulation (SCAM), 2011 11th IEEE International Working Conference on},
	pages={173--184},
	year={2011},
	organization={IEEE}
}

@inproceedings{shimonaka2016identifying,
	title={Identifying Auto-Generated Code by Using Machine Learning Techniques},
	author={Shimonaka, Kento and Sumi, Soichi and Higo, Yoshiki and Kusumoto, Shinji},
	booktitle={Empirical Software Engineering in Practice (IWESEP), 2016 7th International Workshop on},
	pages={18--23},
	year={2016},
	organization={IEEE}
}

@inproceedings{moreno2013automatic,
	title={Automatic generation of natural language summaries for java classes},
	author={Moreno, Laura and Aponte, Jairo and Sridhara, Giriprasad and Marcus, Andrian and Pollock, Lori and Vijay-Shanker, K},
	booktitle={Program Comprehension (ICPC), 2013 IEEE 21st International Conference on},
	pages={23--32},
	year={2013},
	organization={IEEE}
}

@inproceedings{kramer1999api,
	title={API documentation from source code comments: a case study of Javadoc},
	author={Kramer, Douglas},
	booktitle={Proceedings of the 17th annual international conference on Computer documentation},
	pages={147--153},
	year={1999},
	organization={ACM}
}

@article{ottenstein1984program,
	title={The program dependence graph in a software development environment},
	author={Ottenstein, Karl J and Ottenstein, Linda M},
	journal={ACM SIGSOFT Software Engineering Notes},
	volume={9},
	number={3},
	pages={177--184},
	year={1984},
	publisher={ACM}
}

@inproceedings{binkley2007source,
	title={Source code analysis: A road map},
	author={Binkley, David},
	booktitle={2007 Future of Software Engineering},
	pages={104--119},
	year={2007},
	organization={IEEE Computer Society}
}

@article{lin2004rouge,
	title={Rouge: A package for automatic evaluation of summaries},
	author={Lin, Chin-Yew},
	journal={Text Summarization Branches Out},
	year={2004}
}

@misc{Lopes+Bajracharya+Ossher+Baldi:2010 ,
	author = "C. Lopes and S. Bajracharya and J. Ossher and P. Baldi",
	year = "2010",
	title = "{UCI} Source Code Data Sets",
	url = "http://www.ics.uci.edu/$\sim$lopes/datasets/",
	institution = "University of California, Irvine, 
	Bren School of Information and Computer Sciences"
}

@inproceedings{hill2009automatically,
	title={Automatically capturing source code context of nl-queries for software maintenance and reuse},
	author={Hill, Emily and Pollock, Lori and Vijay-Shanker, K},
	booktitle={Proceedings of the 31st International Conference on Software Engineering},
	pages={232--242},
	year={2009},
	organization={IEEE Computer Society}
}

@article{yao2018staqc,
	title={StaQC: A Systematically Mined Question-Code Dataset from Stack Overflow},
	author={Yao, Ziyu and Weld, Daniel S and Chen, Wei-Peng and Sun, Huan},
	journal={arXiv preprint arXiv:1803.09371},
	year={2018}
}

@inproceedings{haiduc2010supporting,
	title={Supporting program comprehension with source code summarization},
	author={Haiduc, Sonia and Aponte, Jairo and Marcus, Andrian},
	booktitle={Proceedings of the 32Nd ACM/IEEE International Conference on Software Engineering-Volume 2},
	pages={223--226},
	year={2010},
	organization={ACM}
}

@inproceedings{bettenburg2010workshop,
	title={Workshop on Mining Unstructured Data (MUD) because" Mining Unstructured Data is Like Fishing in Muddy Waters"!},
	author={Bettenburg, Nicolas and Adams, Bram},
	booktitle={2010 17th Working Conference on Reverse Engineering},
	pages={277--278},
	year={2010},
	organization={IEEE}
}

@inproceedings{bavota2016mining,
	title={Mining unstructured data in software repositories: Current and future trends},
	author={Bavota, Gabriele},
	booktitle={2016 IEEE 23rd International Conference on Software Analysis, Evolution, and Reengineering (SANER)},
	volume={5},
	pages={1--12},
	year={2016},
	organization={IEEE}
}

@inproceedings{haiduc2010use,
	title={On the use of automated text summarization techniques for summarizing source code},
	author={Haiduc, Sonia and Aponte, Jairo and Moreno, Laura and Marcus, Andrian},
	booktitle={Reverse Engineering (WCRE), 2010 17th Working Conference on},
	pages={35--44},
	year={2010},
	organization={IEEE}
}

@article{bahdanau2014neural,
	title={Neural machine translation by jointly learning to align and translate},
	author={Bahdanau, Dzmitry and Cho, Kyunghyun and Bengio, Yoshua},
	journal={arXiv preprint arXiv:1409.0473},
	year={2014}
}

@inproceedings{gu2018deep,
	title={Deep code search},
	author={Gu, Xiaodong and Zhang, Hongyu and Kim, Sunghun},
	booktitle={Proceedings of the 40th International Conference on Software Engineering},
	pages={933--944},
	year={2018},
	organization={ACM}
}

@inproceedings{mcmillan2011portfolio,
	title={Portfolio: finding relevant functions and their usage},
	author={McMillan, Collin and Grechanik, Mark and Poshyvanyk, Denys and Xie, Qing and Fu, Chen},
	booktitle={Proceedings of the 33rd International Conference on Software Engineering},
	pages={111--120},
	year={2011},
	organization={ACM}
}

% @misc{Lopes+Bajracharya+Ossher+Baldi:2010 ,
% author = "C. Lopes and S. Bajracharya and J. Ossher and P. Baldi",
% year = "2010",
% title = "{UCI} Source Code Data Sets",
% url = "http://www.ics.uci.edu/$\sim$lopes/datasets/",
% institution = "University of California, Irvine, 
% Bren School of Information and Computer Sciences"
% }

@article{olden2002illuminating,
	title={Illuminating the “black box”: a randomization approach for understanding variable contributions in artificial neural networks},
	author={Olden, Julian D and Jackson, Donald A},
	journal={Ecological modelling},
	volume={154},
	number={1-2},
	pages={135--150},
	year={2002},
	publisher={Elsevier}
}

@misc{NL4SEAAAI:2018,
author = "Cohen, William and Devanbu, Prem",
year = "2018",
title = "Workshop on NLP for Software Engineering",
url = "https://nl4se.github.io/"
}

@inproceedings{xie2018intelligent,
	title={Intelligent Software Engineering: Synergy between AI and Software Engineering},
	author={Xie, Tao},
	booktitle={Proceedings of the 11th Innovations in Software Engineering Conference},
	pages={1},
	year={2018},
	organization={ACM}
}

@inproceedings{meng2017deep,
	title={Deep Keyphrase Generation},
	author={Meng, Rui and Zhao, Sanqiang and Han, Shuguang and He, Daqing and Brusilovsky, Peter and Chi, Yu},
	booktitle={Proceedings of the 55th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
	pages={582--592},
	year={2017}
}

@article{buhrmester2011amazon,
	title={Amazon's Mechanical Turk: A new source of inexpensive, yet high-quality, data?},
	author={Buhrmester, Michael and Kwang, Tracy and Gosling, Samuel D},
	journal={Perspectives on psychological science},
	volume={6},
	number={1},
	pages={3--5},
	year={2011},
	publisher={Sage Publications Sage CA: Los Angeles, CA}
}

@inproceedings{stol2014two,
	title={Two's company, three's a crowd: a case study of crowdsourcing software development},
	author={Stol, Klaas-Jan and Fitzgerald, Brian},
	booktitle={Proceedings of the 36th International Conference on Software Engineering},
	pages={187--198},
	year={2014},
	organization={ACM}
}

@inproceedings{zhang2016keyphrase,
	title={Keyphrase extraction using deep recurrent neural networks on Twitter},
	author={Zhang, Qi and Wang, Yang and Gong, Yeyun and Huang, Xuanjing},
	booktitle={Proceedings of the 2016 Conference on Empirical Methods in Natural Language Processing},
	pages={836--845},
	year={2016}
}

@inproceedings{hellendoorn2017deep,
	title={Are deep neural networks the best choice for modeling source code?},
	author={Hellendoorn, Vincent J and Devanbu, Premkumar},
	booktitle={Proceedings of the 2017 11th Joint Meeting on Foundations of Software Engineering},
	pages={763--773},
	year={2017},
	organization={ACM}
}

@inproceedings{walker1997evaluating,
	title={Evaluating interactive dialogue systems: Extending component evaluation to integrated system evaluation},
	author={Walker, Marilyn A and Litman, Diane J and Kamm, Candace A and Abella, Alicia},
	booktitle={Interactive Spoken Dialog Systems: Bringing Speech and NLP Together in Real Applications},
	year={1997}
}

@inproceedings{beringer2002promise,
	title={PROMISE: A procedure for multimodal interactive system evaluation},
	author={Beringer, Nicole and Kartal, Ute and Louka, Katerina and Schiel, Florian and T{\"u}rk, Uli and others},
	booktitle={Proceedings of the Workshop’Multimodal Resources and Multimodal Systems Evaluation},
	pages={90--95},
	year={2002},
	organization={Citeseer}
}

@inproceedings{he2018decoupling,
	title={Decoupling Strategy and Generation in Negotiation Dialogues},
	author={He, He and Chen, Derek and Balakrishnan, Anusha and Liang, Percy},
	booktitle={Proceedings of the 2018 Conference on Empirical Methods in Natural Language Processing},
	pages={2333--2343},
	year={2018}
}

@incollection{burger2000verbmobil,
	title={Verbmobil data collection and annotation},
	author={Burger, Susanne and Weilhammer, Karl and Schiel, Florian and Tillmann, Hans G},
	booktitle={Verbmobil: Foundations of speech-to-speech translation},
	pages={537--549},
	year={2000},
	publisher={Springer}
}

@inproceedings{blunsom2013recurrent,
	title={Recurrent convolutional neural networks for discourse compositionality},
	author={Blunsom, Phil and Kalchbrenner, Nal and Kalchbrenner, Nal},
	booktitle={Proceedings of the 2013 Workshop on Continuous Vector Space Models and their Compositionality},
	year={2013},
	organization={Proceedings of the 2013 Workshop on Continuous Vector Space Models and their Compositionality}
}

@inproceedings{chen2018dialogue,
	title={Dialogue Act Recognition via CRF-Attentive Structured Network},
	author={Chen, Zheqian and Yang, Rongqin and Zhao, Zhou and Cai, Deng and He, Xiaofei},
	booktitle={The 41st International ACM SIGIR Conference on Research \& Development in Information Retrieval},
	pages={225--234},
	year={2018},
	organization={ACM}
}

@article{kumar2017dialogue,
	title={Dialogue Act Sequence Labeling using Hierarchical encoder with CRF},
	author={Kumar, Harshit and Agarwal, Arvind and Dasgupta, Riddhiman and Joshi, Sachindra and Kumar, Arun},
	journal={AAAI},
	year={2018}
}

@inproceedings{wood2018detecting,
	title={Detecting speech act types in developer question/answer conversations during bug repair},
	author={Wood, Andrew and Rodeghero, Paige and Armaly, Ameer and McMillan, Collin},
	booktitle={Proceedings of the 2018 26th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering},
	pages={491--502},
	year={2018},
	organization={ACM}
}

@article{lemon2011learning,
	title={Learning what to say and how to say it: Joint optimisation of spoken dialogue management and natural language generation},
	author={Lemon, Oliver},
	journal={Computer Speech \& Language},
	volume={25},
	number={2},
	pages={210--221},
	year={2011},
	publisher={Elsevier}
}

@inproceedings{xiong2016dynamic,
	title={Dynamic memory networks for visual and textual question answering},
	author={Xiong, Caiming and Merity, Stephen and Socher, Richard},
	booktitle={International conference on machine learning},
	pages={2397--2406},
	year={2016}
}

@article{graves2016hybrid,
	title={Hybrid computing using a neural network with dynamic external memory},
	author={Graves, Alex and Wayne, Greg and Reynolds, Malcolm and Harley, Tim and Danihelka, Ivo and Grabska-Barwi{\'n}ska, Agnieszka and Colmenarejo, Sergio G{\'o}mez and Grefenstette, Edward and Ramalho, Tiago and Agapiou, John and others},
	journal={Nature},
	volume={538},
	number={7626},
	pages={471},
	year={2016},
	publisher={Nature Publishing Group}
}

@article{li2015gated,
	title={Gated graph sequence neural networks},
	author={Li, Yujia and Tarlow, Daniel and Brockschmidt, Marc and Zemel, Richard},
	journal={arXiv preprint arXiv:1511.05493},
	year={2015}
}

@book{rieser2011reinforcement,
	title={Reinforcement learning for adaptive dialogue systems: a data-driven methodology for dialogue management and natural language generation},
	author={Rieser, Verena and Lemon, Oliver},
	year={2011},
	publisher={Springer Science \& Business Media}
}

@inproceedings{jiang2017automatically,
	title={Automatically generating commit messages from diffs using neural machine translation},
	author={Jiang, Siyuan and Armaly, Ameer and McMillan, Collin},
	booktitle={Proceedings of the 32nd IEEE/ACM International Conference on Automated Software Engineering},
	pages={135--146},
	year={2017},
	organization={IEEE Press}
}

@article{ward2016challenges,
	title={Challenges in building highly-interactive dialog systems},
	author={Ward, Nigel G and DeVault, David},
	journal={AI Magazine},
	volume={37},
	number={4},
	pages={7--18},
	year={2016}
}

@article{johnson2019no,
	title={No AI Is an Island: The Case for Teaming Intelligence},
	author={Johnson, Matthew and Vera, Alonso},
	journal={AI Magazine},
	volume={40},
	number={1},
	pages={16--28},
	year={2019}
}

@inproceedings{robillard2017demand,
	title={On-demand developer documentation},
	author={Robillard, Martin P and Marcus, Andrian and Treude, Christoph and Bavota, Gabriele and Chaparro, Oscar and Ernst, Neil and Gerosa, Marco Aur{\'e}lio and Godfrey, Michael and Lanza, Michele and Linares-V{\'a}squez, Mario and others},
	booktitle={2017 IEEE International Conference on Software Maintenance and Evolution (ICSME)},
	pages={479--483},
	year={2017},
	organization={IEEE}
}

@inproceedings{iyer2016summarizing,
	title={Summarizing source code using a neural attention model},
	author={Iyer, Srinivasan and Konstas, Ioannis and Cheung, Alvin and Zettlemoyer, Luke},
	booktitle={Proceedings of the 54th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
	volume={1},
	pages={2073--2083},
	year={2016}
}

@inproceedings{eddy2013evaluating,
	title={Evaluating source code summarization techniques: Replication and expansion},
	author={Eddy, Brian P and Robinson, Jeffrey A and Kraft, Nicholas A and Carver, Jeffrey C},
	booktitle={Program Comprehension (ICPC), 2013 IEEE 21st International Conference on},
	pages={13--22},
	year={2013},
	organization={IEEE}
}

@article{loyola2017neural,
	title={A neural architecture for generating natural language descriptions from source code changes},
	author={Loyola, Pablo and Marrese-Taylor, Edison and Matsuo, Yutaka},
	journal={arXiv preprint arXiv:1704.04856},
	year={2017}
}

% @article{allamanis2018learning,
% 	title={Learning to represent programs with graphs},
% 	author={Allamanis, Miltiadis and Brockschmidt, Marc and Khademi, Mahmoud},
% 	journal={International Conference on Learning Representations},
% 	year={2018}
% }

@book{deng2018deep,
	title={Deep Learning in Natural Language Processing},
	author={Deng, Li and Liu, Yang},
	year={2018},
	publisher={Springer}
}

@book{Reiter:2000:BNL:331955,
	author = {Reiter, Ehud and Dale, Robert},
	title = {Building natural language generation systems},
	year = {2000},
	isbn = {0-521-62036-8},
	publisher = {Cambridge University Press},
	address = {New York, NY, USA},
} 

@InProceedings{sennrich-EtAl:2017:EACLDemo,
	author    = {Sennrich, Rico  and  Firat, Orhan  and  Cho, Kyunghyun  and  Birch, Alexandra  and  Haddow, Barry  and  Hitschler, Julian  and  Junczys-Dowmunt, Marcin  and  L\"{a}ubli, Samuel  and  Miceli Barone, Antonio Valerio  and  Mokry, Jozef  and  Nadejde, Maria},
	title     = {Nematus: a Toolkit for Neural Machine Translation},
	booktitle = {Proceedings of the Software Demonstrations of the 15th Conference of the European Chapter of the Association for Computational Linguistics},
	month     = {April},
	year      = {2017},
	address   = {Valencia, Spain},
	publisher = {Association for Computational Linguistics},
	pages     = {65--68},
	url       = {http://aclweb.org/anthology/E17-3017}
}

@article{richardson2017code2text,
	title={The Code2Text Challenge: Text Generation in Source Code Libraries},
	author={Richardson, Kyle and Zarrie{\ss}, Sina and Kuhn, Jonas},
	journal={arXiv preprint arXiv:1708.00098},
	year={2017}
}

@inproceedings{allamanis2015bimodal,
	title={Bimodal modelling of source code and natural language},
	author={Allamanis, Miltos and Tarlow, Daniel and Gordon, Andrew and Wei, Yi},
	booktitle={International Conference on Machine Learning},
	pages={2123--2132},
	year={2015}
}

@inproceedings{chen2018best,
	title={The Best of Both Worlds: Combining Recent Advances in Neural Machine Translation},
	author={Chen, Mia Xu and Firat, Orhan and Bapna, Ankur and Johnson, Melvin and Macherey, Wolfgang and Foster, George and Jones, Llion and Schuster, Mike and Shazeer, Noam and Parmar, Niki and others},
	booktitle={Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
	pages={76--86},
	year={2018}
}

@inproceedings{yin2018mining,
	author = {Yin, Pengcheng and Deng, Bowen and Chen, Edgar and Vasilescu, Bogdan and Neubig, Graham},
	title = {Learning to Mine Aligned Code and Natural Language Pairs from Stack Overflow},
	booktitle = {International Conference on Mining Software Repositories},
	series = {MSR},
	pages = {476--486},
	year = {2018},
	publisher = {ACM},
	doi = {https://doi.org/10.1145/3196398.3196408},
}

@inproceedings{hu2018summarizing,
	title={Summarizing Source Code with Transferred API Knowledge.},
	author={Hu, Xing and Li, Ge and Xia, Xin and Lo, David and Lu, Shuai and Jin, Zhi},
	booktitle={IJCAI},
	pages={2269--2275},
	year={2018}
}

@inproceedings{hu2018deep,
	title={Deep code comment generation},
	author={Hu, Xing and Li, Ge and Xia, Xin and Lo, David and Jin, Zhi},
	booktitle={Proceedings of the 26th International Conference on Program Comprehension},
	pages={200--210},
	year={2018},
	organization={ACM}
}

@article{chen2015abc,
	title={ABC-CNN: An attention based convolutional neural network for visual question answering},
	author={Chen, Kan and Wang, Jiang and Chen, Liang-Chieh and Gao, Haoyuan and Xu, Wei and Nevatia, Ram},
	journal={arXiv preprint arXiv:1511.05960},
	year={2015}
}

@inproceedings{yang2016stacked,
	title={Stacked attention networks for image question answering},
	author={Yang, Zichao and He, Xiaodong and Gao, Jianfeng and Deng, Li and Smola, Alex},
	booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
	pages={21--29},
	year={2016}
}

@inproceedings{marcus2003recovering,
	title={Recovering documentation-to-source-code traceability links using latent semantic indexing},
	author={Marcus, Andrian and Maletic, Jonathan I},
	booktitle={Proceedings of the 25th international conference on software engineering},
	pages={125--135},
	year={2003},
	organization={IEEE Computer Society}
}

@article{mao2014deep,
	title={Deep captioning with multimodal recurrent neural networks (m-rnn)},
	author={Mao, Junhua and Xu, Wei and Yang, Yi and Wang, Jiang and Huang, Zhiheng and Yuille, Alan},
	journal={arXiv preprint arXiv:1412.6632},
	year={2014}
}

@inproceedings{johnson2016densecap,
	title={Densecap: Fully convolutional localization networks for dense captioning},
	author={Johnson, Justin and Karpathy, Andrej and Fei-Fei, Li},
	booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
	pages={4565--4574},
	year={2016}
}

@article{luong2015effective,
	title={Effective approaches to attention-based neural machine translation},
	author={Luong, Minh-Thang and Pham, Hieu and Manning, Christopher D},
	journal={arXiv preprint arXiv:1508.04025},
	year={2015}
}

@article{allamanis2017survey,
	title={A survey of machine learning for big code and naturalness},
	author={Allamanis, Miltiadis and Barr, Earl T and Devanbu, Premkumar and Sutton, Charles},
	journal={arXiv preprint arXiv:1709.06182},
	year={2017}
}

@inproceedings{oda2015learning,
	title={Learning to generate pseudo-code from source code using statistical machine translation (t)},
	author={Oda, Yusuke and Fudaba, Hiroyuki and Neubig, Graham and Hata, Hideaki and Sakti, Sakriani and Toda, Tomoki and Nakamura, Satoshi},
	booktitle={Automated Software Engineering (ASE), 2015 30th IEEE/ACM International Conference on},
	pages={574--584},
	year={2015},
	organization={IEEE}
}

@inproceedings{allamanis2016convolutional,
	title={A convolutional attention network for extreme summarization of source code},
	author={Allamanis, Miltiadis and Peng, Hao and Sutton, Charles},
	booktitle={International Conference on Machine Learning},
	pages={2091--2100},
	year={2016}
}

@article{rodeghero2015eye,
	title={An eye-tracking study of java programmers and application to source code summarization},
	author={Rodeghero, Paige and Liu, Cheng and McBurney, Paul W and McMillan, Collin},
	journal={IEEE Transactions on Software Engineering},
	volume={41},
	number={11},
	pages={1038--1054},
	year={2015},
	publisher={IEEE}
}

@inproceedings{rastkar2011generating,
	title={Generating natural language summaries for crosscutting source code concerns},
	author={Rastkar, Sarah and Murphy, Gail C and Bradley, Alexander WJ},
	booktitle={Software Maintenance (ICSM), 2011 27th IEEE International Conference on},
	pages={103--112},
	year={2011},
	organization={IEEE}
}

@article{nazar2016summarizing,
	title={Summarizing software artifacts: A literature review},
	author={Nazar, Najam and Hu, Yan and Jiang, He},
	journal={Journal of Computer Science and Technology},
	volume={31},
	number={5},
	pages={883--909},
	year={2016},
	publisher={Springer}
}

@inproceedings{cortes2014automatically,
	title={On automatically generating commit messages via summarization of source code changes},
	author={Cort{\'e}s-Coy, Luis Fernando and Linares-V{\'a}squez, Mario and Aponte, Jairo and Poshyvanyk, Denys},
	booktitle={Source Code Analysis and Manipulation (SCAM), 2014 IEEE 14th International Working Conference on},
	pages={275--284},
	year={2014},
	organization={IEEE}
}

@inproceedings{kamimura2013towards,
	title={Towards generating human-oriented summaries of unit test cases},
	author={Kamimura, Manabu and Murphy, Gail C},
	booktitle={2013 IEEE 21st International Conference on Program Comprehension (ICPC)},
	pages={215--218},
	year={2013},
	organization={IEEE}
}

@article{johnson2017google,
	title={Google's Multilingual Neural Machine Translation System: Enabling Zero-Shot Translation},
	author={Johnson, Melvin and Schuster, Mike and Le, Quoc V and Krikun, Maxim and Wu, Yonghui and Chen, Zhifeng and Thorat, Nikhil and Vi{\'e}gas, Fernanda and Wattenberg, Martin and Corrado, Greg and others},
	journal={Transactions of the Association of Computational Linguistics},
	volume={5},
	number={1},
	pages={339--351},
	year={2017}
}

@inproceedings{vinyals2015show,
	title={Show and tell: A neural image caption generator},
	author={Vinyals, Oriol and Toshev, Alexander and Bengio, Samy and Erhan, Dumitru},
	booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
	pages={3156--3164},
	year={2015}
}

@inproceedings{vaswani2017attention,
	title={Attention is all you need},
	author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
	booktitle={Advances in Neural Information Processing Systems},
	pages={5998--6008},
	year={2017}
}

@book{goodfellow2016deep,
	title={Deep learning},
	author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron and Bengio, Yoshua},
	volume={1},
	year={2016},
	publisher={MIT press Cambridge}
}

@article{lecun2015deep,
	title={Deep learning},
	author={LeCun, Yann and Bengio, Yoshua and Hinton, Geoffrey},
	journal={nature},
	volume={521},
	number={7553},
	pages={436},
	year={2015},
	publisher={Nature Publishing Group}
}

@inproceedings{sutskever2014sequence,
	title={Sequence to sequence learning with neural networks},
	author={Sutskever, Ilya and Vinyals, Oriol and Le, Quoc V},
	booktitle={Advances in neural information processing systems},
	pages={3104--3112},
	year={2014}
}

@inproceedings{sutskever2011generating,
	title={Generating text with recurrent neural networks},
	author={Sutskever, Ilya and Martens, James and Hinton, Geoffrey E},
	booktitle={Proceedings of the 28th International Conference on Machine Learning (ICML-11)},
	pages={1017--1024},
	year={2011}
}

@inproceedings{sridhara2011automatically,
	title={Automatically detecting and describing high level actions within methods},
	author={Sridhara, Giriprasad and Pollock, Lori and Vijay-Shanker, K},
	booktitle={Proceedings of the 33rd International Conference on Software Engineering},
	pages={101--110},
	year={2011},
	organization={ACM}
}

@inproceedings{sridhara2010towards,
	title={Towards automatically generating summary comments for java methods},
	author={Sridhara, Giriprasad and Hill, Emily and Muppaneni, Divya and Pollock, Lori and Vijay-Shanker, K},
	booktitle={Proceedings of the IEEE/ACM international conference on Automated software engineering},
	pages={43--52},
	year={2010},
	organization={ACM}
}

@article{von1995program,
	title={Program comprehension during software maintenance and evolution},
	author={Von Mayrhauser, Anneliese and Vans, A Marie},
	journal={Computer},
	number={8},
	pages={44--55},
	year={1995},
	publisher={IEEE}
}

@article{letovsky1987cognitive,
	title={Cognitive processes in program comprehension},
	author={Letovsky, Stanley},
	journal={Journal of Systems and software},
	volume={7},
	number={4},
	pages={325--339},
	year={1987},
	publisher={Elsevier}
}

@article{cornelissen2009systematic,
	title={A systematic survey of program comprehension through dynamic analysis},
	author={Cornelissen, Bas and Zaidman, Andy and Van Deursen, Arie and Moonen, Leon and Koschke, Rainer},
	journal={IEEE Transactions on Software Engineering},
	volume={35},
	number={5},
	pages={684--702},
	year={2009},
	publisher={IEEE}
}

@inproceedings{maletic2001supporting,
	title={Supporting program comprehension using semantic and structural information},
	author={Maletic, Jonathan I and Marcus, Andrian},
	booktitle={Proceedings of the 23rd International Conference on Software Engineering},
	pages={103--112},
	year={2001},
	organization={IEEE Computer Society}
}

@inproceedings{de2005study,
	title={A study of the documentation essential to software maintenance},
	author={de Souza, Sergio Cozzetti B and Anquetil, Nicolas and de Oliveira, Kathia M},
	booktitle={Proceedings of the 23rd annual international conference on Design of communication: documenting \& designing for pervasive information},
	pages={68--75},
	year={2005},
	organization={ACM}
}

@article{barone2017parallel,
	title={A parallel corpus of Python functions and documentation strings for automated code documentation and code generation},
	author={Barone, Antonio Valerio Miceli and Sennrich, Rico},
	journal={arXiv preprint arXiv:1707.02275},
	year={2017}
}

@inproceedings{movshovitz2013natural,
	title={Natural language models for predicting programming comments},
	author={Movshovitz-Attias, Dana and Cohen, William W},
	booktitle={Proceedings of the 51st Annual Meeting of the Association for Computational Linguistics (Volume 2: Short Papers)},
	volume={2},
	pages={35--40},
	year={2013}
}

@inproceedings{fluri2007code,
	title={Do code and comments co-evolve? on the relation between source code and comment changes},
	author={Fluri, Beat and Wursch, Michael and Gall, Harald C},
	booktitle={Reverse Engineering, 2007. WCRE 2007. 14th Working Conference on},
	pages={70--79},
	year={2007},
	organization={IEEE}
}

@article{ibrahim2012relationship,
	title={On the relationship between comment update practices and software bugs},
	author={Ibrahim, Walid M and Bettenburg, Nicolas and Adams, Bram and Hassan, Ahmed E},
	journal={Journal of Systems and Software},
	volume={85},
	number={10},
	pages={2293--2304},
	year={2012},
	publisher={Elsevier}
}

@inproceedings{forward2002relevance,
	title={The relevance of software documentation, tools and technologies: a survey},
	author={Forward, Andrew and Lethbridge, Timothy C},
	booktitle={Proceedings of the 2002 ACM symposium on Document engineering},
	pages={26--33},
	year={2002},
	organization={ACM}
}

@article{song2019survey,
	title={A Survey of Automatic Generation of Source Code Comments: Algorithms and Techniques},
	author={Song, Xiaotao and Sun, Hailong and Wang, Xu and Yan, Jiafei},
	journal={IEEE Access},
	year={2019},
	publisher={IEEE}
}

@inproceedings{garmash2016ensemble,
	title={Ensemble learning for multi-source neural machine translation},
	author={Garmash, Ekaterina and Monz, Christof},
	booktitle={Proceedings of COLING 2016, the 26th International Conference on Computational Linguistics: Technical Papers},
	pages={1409--1418},
	year={2016}
}

@electronic{NLTKWebsite,
	author        = "Chin Yee Lee, Hengfeng Li, Ruxin Hou, Calvin Tanujaya Lim",
	title         = "NLTK Translate BLEU Score Calculator v3.3",
	url           = "https://www.nltk.org/modules/nltk/translate/bleuscore.html",
	year          = "2019"
}

@electronic{ml4codewebsite,
	author        = "Miltos Allamanis",
	title         = "Machine Learning for Big Code and Naturalness",
	url           = "https://ml4code.github.io/papers.html",
	year          = "2019"
}

@electronic{OpenNMTWebsite,
	author        = "Stig-Arne Grönroos",
	title         = "OpenNMT Ensemble Decoding",
	url           = "https://github.com/OpenNMT/OpenNMT-py/pull/732",
	year          = "2019"
}


@electronic{DoxygenWebsite,
	author        = "Dimitri van Heesch",
	title         = "Doxygen Website",
	url           = "http://www.doxygen.org/",
	year          = "2019"
}

@inproceedings{biggerstaff1993concept,
	title={The concept assignment problem in program understanding},
	author={Biggerstaff, Ted J and Mitbander, Bharat G and Webster, Dallas},
	booktitle={Proceedings of the 15th international conference on Software Engineering},
	pages={482--498},
	year={1993},
	organization={IEEE Computer Society Press}
}

@article{kajko2005survey,
	title={A survey of documentation practice within corrective maintenance},
	author={Kajko-Mattsson, Mira},
	journal={Empirical Software Engineering},
	volume={10},
	number={1},
	pages={31--55},
	year={2005},
	publisher={Springer}
}

@article{newell2011design,
	title={Design and the digital divide: insights from 40 years in computer support for older and disabled people},
	author={Newell, Alan F},
	journal={Synthesis Lectures on Assistive, Rehabilitative, and Health-Preserving Technologies},
	volume={1},
	number={1},
	pages={1--195},
	year={2011},
	publisher={Morgan \& Claypool Publishers}
}

@article{tintarev2016personal,
	title={Personal storytelling: Using Natural Language Generation for children with complex communication needs, in the wild…},
	author={Tintarev, Nava and Reiter, Ehud and Black, Rolf and Waller, Annalu and Reddington, Joe},
	journal={International Journal of Human-Computer Studies},
	volume={92},
	pages={1--16},
	year={2016},
	publisher={Academic Press}
}

@inproceedings{kohavi1995study,
	title={A study of cross-validation and bootstrap for accuracy estimation and model selection},
	author={Kohavi, Ron},
	booktitle={Ijcai},
	volume={14},
	number={2},
	pages={1137--1145},
	year={1995}
}

@article{cheng2016neural,
	title={Neural Summarization by Extracting Sentences and Words},
	author={Cheng, Jianpeng and Lapata, Mirella},
	journal={arXiv preprint arXiv:1603.07252},
	year={2016}
}

@inproceedings{iyersummarizing,
	title={Summarizing Source Code using a Neural Attention Model},
	author={Iyer, Srinivasan and Konstas, Ioannis and Cheung, Alvin and Zettlemoyer, Luke},
	booktitle={Proceedings of the 54th Annual Meeting of the Association for Computational Linguistics},
	year={2016}
}


@article{clark1986referring,
	title={Referring as a collaborative process},
	author={Clark, Herbert H and Wilkes-Gibbs, Deanna},
	journal={Cognition},
	volume={22},
	number={1},
	pages={1--39},
	year={1986},
	publisher={Elsevier}
}

@article{brennan1996conceptual,
	title={Conceptual pacts and lexical choice in conversation.},
	author={Brennan, Susan E and Clark, Herbert H},
	journal={Journal of Experimental Psychology: Learning, Memory, and Cognition},
	volume={22},
	number={6},
	pages={1482},
	year={1996},
	publisher={American Psychological Association}
}

@inproceedings{devault2007managing,
	title={Managing ambiguities across utterances in dialogue},
	author={DeVault, David and Stone, Matthew},
	booktitle={Proceedings of the 11th Workshop on the Semantics and Pragmatics of Dialogue (Decalog 2007)},
	pages={49--56},
	year={2007}
}

@article{perlow2002s,
	title={Who's helping whom? Layers of culture and workplace behavior},
	author={Perlow, Leslie and Weeks, John},
	journal={Journal of Organizational Behavior},
	volume={23},
	number={4},
	pages={345--361},
	year={2002},
	publisher={Wiley Online Library}
}

@article{vinyals2015neural,
	title={A neural conversational model},
	author={Vinyals, Oriol and Le, Quoc},
	journal={arXiv preprint arXiv:1506.05869},
	year={2015}
}

@inproceedings{henderson2013deep,
	title={Deep neural network approach for the dialog state tracking challenge},
	author={Henderson, Matthew and Thomson, Blaise and Young, Steve},
	booktitle={Proceedings of the SIGDIAL 2013 Conference},
	pages={467--471},
	year={2013}
}

@article{williams2007partially,
	title={Partially observable Markov decision processes for spoken dialog systems},
	author={Williams, Jason D and Young, Steve},
	journal={Computer Speech \& Language},
	volume={21},
	number={2},
	pages={393--422},
	year={2007},
	publisher={Elsevier}
}

@inproceedings{mcmillan2016collaborative,
	title={Collaborative software engineering education between college seniors and blind high school students},
	author={McMillan, Collin and Rodda-Tyler, Amanda},
	booktitle={Proceedings of the 38th International Conference on Software Engineering Companion},
	pages={360--363},
	year={2016},
	organization={ACM}
}

@inproceedings{ameer2016icsme,
	title={A Case Study of Automated Feature Location Techniques for Industrial Cost Estimation},
	author={Armaly, Ameer and Klaczynski, John and McMillan, Collin},
	booktitle={Proceedings of the 32nd IEEE International Conference on Software Maintenance and Evolution, Industry Track},
	year={2016},
	organization={IEEE}
}

@incollection{bateman2003natural,
	title={Natural language generation},
	author={Bateman, John and Zock, Michael},
	booktitle={The Oxford Handbook of Computational Linguistics 2nd edition},
	year={2003}
}

@inproceedings{boehm2006view,
	title={A view of 20th and 21st century software engineering},
	author={Boehm, Barry},
	booktitle={Proceedings of the 28th international conference on Software engineering},
	pages={12--29},
	year={2006},
	organization={ACM}
}

@book{robillard2014recommendation,
	title={Recommendation systems in software engineering},
	author={Robillard, Martin P and Maalej, Walid and Walker, Robert J and Zimmermann, Thomas},
	year={2014},
	publisher={Springer}
}

@misc{pinzger2016guest,
	title={Guest editorial: mining software repositories},
	author={Pinzger, Martin and Kim, Sunghun},
	year={2016},
	publisher={Springer}
}

@article{kagdi2007survey,
	title={A survey and taxonomy of approaches for mining software repositories in the context of software evolution},
	author={Kagdi, Huzefa and Collard, Michael L and Maletic, Jonathan I},
	journal={Journal of software maintenance and evolution: Research and practice},
	volume={19},
	number={2},
	pages={77--131},
	year={2007},
	publisher={Wiley Online Library}
}

@article{anderson1993problem,
	title={Problem solving and learning.},
	author={Anderson, John R},
	journal={American Psychologist},
	volume={48},
	number={1},
	pages={35},
	year={1993},
	publisher={American Psychological Association}
}

@article{harnad1990symbol,
	title={The symbol grounding problem},
	author={Harnad, Stevan},
	journal={Physica D: Nonlinear Phenomena},
	volume={42},
	number={1-3},
	pages={335--346},
	year={1990},
	publisher={Elsevier}
}

@book{stent2014natural,
	title={Natural language generation in interactive systems},
	author={Stent, Amanda and Bangalore, Srinivas},
	year={2014},
	publisher={Cambridge University Press}
}

@inproceedings{viethen2006algorithms,
	title={Algorithms for generating referring expressions: do they do what people do?},
	author={Viethen, Jette and Dale, Robert},
	booktitle={Proceedings of the Fourth International Natural Language Generation Conference},
	pages={63--70},
	year={2006},
	organization={Association for Computational Linguistics}
}

@inproceedings{bavota2016mining,
	title={Mining Unstructured Data in Software Repositories: Current and Future Trends},
	author={Bavota, Gabriele},
	booktitle={2016 IEEE 23rd International Conference on Software Analysis, Evolution, and Reengineering (SANER)},
	volume={5},
	pages={1--12},
	year={2016},
	organization={IEEE}
}

@inproceedings{ai2007comparing,
	title={Comparing user simulation models for dialog strategy learning},
	author={Ai, Hua and Tetreault, Joel R and Litman, Diane J},
	booktitle={Human Language Technologies 2007: The Conference of the North American Chapter of the Association for Computational Linguistics; Companion Volume, Short Papers},
	pages={1--4},
	year={2007},
	organization={Association for Computational Linguistics}
}

@inproceedings{schatzmann2007agenda,
	title={Agenda-based user simulation for bootstrapping a POMDP dialogue system},
	author={Schatzmann, Jost and Thomson, Blaise and Weilhammer, Karl and Ye, Hui and Young, Steve},
	booktitle={Human Language Technologies 2007: The Conference of the North American Chapter of the Association for Computational Linguistics; Companion Volume, Short Papers},
	pages={149--152},
	year={2007},
	organization={Association for Computational Linguistics}
}

@article{holton2007coding,
	title={The coding process and its challenges},
	author={Holton, Judith A},
	journal={The SAGE handbook of grounded theory},
	pages={265--289},
	year={2007},
	publisher={Sage Publications Los Angeles\^{} eCA CA}
}

@inproceedings{gabsdil2003clarification,
	title={Clarification in spoken dialogue systems},
	author={Gabsdil, Malte},
	booktitle={Proceedings of the 2003 AAAI Spring Symposium. Workshop on Natural Language Generation in Spoken and Written Dialogue},
	pages={28--35},
	year={2003}
}

@inproceedings{guhe2008adapting,
	title={Adapting referring expressions to the task environment},
	author={Guhe, Markus and Bard, Ellen Gurman},
	booktitle={Proceedings of the 30th Annual Conference of the Cognitive Science Society (CogSci)},
	pages={2404--2409},
	year={2008}
}

@inproceedings{foster2008roles,
	title={The roles of haptic-ostensive referring expressions in cooperative, task-based human-robot dialogue},
	author={Foster, Mary Ellen and Bard, Ellen Gurman and Guhe, Markus and Hill, Robin L and Oberlander, Jon and Knoll, Alois},
	booktitle={Proceedings of the 3rd ACM/IEEE international conference on Human robot interaction},
	pages={295--302},
	year={2008},
	organization={ACM}
}

@article{krahmer2003graph,
	title={Graph-based generation of referring expressions},
	author={Krahmer, Emiel and Van Erk, Sebastiaan and Verleg, Andr{\'e}},
	journal={Computational Linguistics},
	volume={29},
	number={1},
	pages={53--72},
	year={2003},
	publisher={MIT Press}
}

@article{neubigsurvey,
	title={Survey of Methods to Generate Natural Language from Source Code},
	author={Neubig, Graham},
	journal={http://www.languageandcode.org/nlse2015/neubig15nlse-survey.pdf},
	year={2015}
}

@inproceedings{goudbeek2010preferences,
	title={Preferences versus adaptation during referring expression generation},
	author={Goudbeek, Martijn and Krahmer, Emiel},
	booktitle={Proceedings of the ACL 2010 Conference Short Papers},
	pages={55--59},
	year={2010},
	organization={Association for Computational Linguistics}
}

@article{passonneau1996using,
	title={Using centering to relax Gricean informational constraints on discourse anaphoric noun phrases},
	author={Passonneau, Rebecca J},
	journal={Language and speech},
	volume={39},
	number={2-3},
	pages={229--264},
	year={1996},
	publisher={SAGE Publications}
}

@inproceedings{jordan2000learning,
	title={Learning attribute selections for non-pronominal expressions},
	author={Jordan, Pamela and Walker, Marilyn},
	booktitle={Proceedings of the 38th Annual Meeting on Association for Computational Linguistics},
	pages={181--190},
	year={2000},
	organization={Association for Computational Linguistics}
}



@article{krahmer2012computational,
	title={Computational generation of referring expressions: A survey},
	author={Krahmer, Emiel and Van Deemter, Kees},
	journal={Computational Linguistics},
	volume={38},
	number={1},
	pages={173--218},
	year={2012},
	publisher={MIT Press}
}

@article{Johnson:1997:IES:591952.591964,
	author = {Johnson, W. Lewis and Erdem, Ali},
	title = {Interactive Explanation of Software Systems},
	journal = {Automated Software Engg.},
	issue_date = {January 1997},
	volume = {4},
	number = {1},
	month = jan,
	year = {1997},
	issn = {0928-8910},
	pages = {53--75},
	numpages = {23},
	url = {http://dx.doi.org/10.1023/A:1008655629091},
	doi = {10.1023/A:1008655629091},
	acmid = {591964},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {World Wide Web, hypertext, software explanation, software understanding},
} 

@inproceedings{Mittal:1995:DGF:223904.223916,
	author = {Mittal, Vibhu O. and Moore, Johanna D.},
	title = {Dynamic Generation of Follow Up Question Menus: Facilitating Interactive Natural Language Dialogues},
	booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
	series = {CHI '95},
	year = {1995},
	isbn = {0-201-84705-1},
	location = {Denver, Colorado, USA},
	pages = {90--97},
	numpages = {8},
	url = {http://dx.doi.org/10.1145/223904.223916},
	doi = {10.1145/223904.223916},
	acmid = {223916},
	publisher = {ACM Press/Addison-Wesley Publishing Co.},
	address = {New York, NY, USA},
} 

@article{bohannon1988issue,
	title={The issue of negative evidence: Adult responses to children's language errors.},
	author={Bohannon, John N and Stanowicz, Laura B},
	journal={Developmental psychology},
	volume={24},
	number={5},
	pages={684},
	year={1988},
	publisher={American Psychological Association}
}

@article{demetras1986feedback,
	title={Feedback to first language learners: The role of repetitions and clarification questions},
	author={Demetras, Marty J and Post, Kathryn Nolan and Snow, Catherine E},
	journal={Journal of child language},
	volume={13},
	number={02},
	pages={275--292},
	year={1986},
	publisher={Cambridge Univ Press}
}

@inproceedings{devault2004interpreting,
	title={Interpreting vague utterances in context},
	author={DeVault, David and Stone, Matthew},
	booktitle={Proceedings of the 20th international conference on Computational Linguistics},
	pages={1247},
	year={2004},
	organization={Association for Computational Linguistics}
}

@inproceedings{devault2006societal,
	title={Societal grounding is essential to meaningful language use},
	author={DeVault, David and Oved, Iris and Stone, Matthew},
	booktitle={Proceedings of the National Conference on Artificial Intelligence},
	volume={21},
	number={1},
	pages={747},
	year={2006},
	organization={Menlo Park, CA; Cambridge, MA; London; AAAI Press; MIT Press; 1999}
}

@book{rieser2011reinforcement,
	title={Reinforcement learning for adaptive dialogue systems: a data-driven methodology for dialogue management and natural language generation},
	author={Rieser, Verena and Lemon, Oliver},
	year={2011},
	publisher={Springer Science \& Business Media}
}

@article{lemon2011learning,
	title={Learning what to say and how to say it: Joint optimisation of spoken dialogue management and natural language generation},
	author={Lemon, Oliver},
	journal={Computer Speech \& Language},
	volume={25},
	number={2},
	pages={210--221},
	year={2011},
	publisher={Elsevier}
}

@inproceedings{bos2003dipper,
	title={DIPPER: Description and formalisation of an information-state update dialogue system architecture},
	author={Bos, Johan and Klein, Ewan and Lemon, Oliver and Oka, Tetsushi},
	booktitle={4th SIGdial Workshop on Discourse and Dialogue},
	pages={115--124},
	year={2003}
}

@inproceedings{Walker:2001:QQE:1073012.1073078,
	author = {Walker, Marilyn A. and Passonneau, Rebecca and Boland, Julie E.},
	title = {Quantitative and Qualitative Evaluation of Darpa Communicator Spoken Dialogue Systems},
	booktitle = {Proceedings of the 39th Annual Meeting on Association for Computational Linguistics},
	series = {ACL '01},
	year = {2001},
	location = {Toulouse, France},
	pages = {515--522},
	numpages = {8},
	url = {http://dx.doi.org/10.3115/1073012.1073078},
	doi = {10.3115/1073012.1073078},
	acmid = {1073078},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
} 

@article{hirschman1998evaluating,
	title={Evaluating Spoken Language Interaction: Experiences from the DARPA Spoken Language Program 1988--1995},
	author={Hirschman, Lynette},
	journal={To appear. See http://www. research. att. com/\~{} walker/eval/hirschman-survey. ps},
	year={1998}
}

@inproceedings{Reithinger:1995:USD:981658.981674,
	author = {Reithinger, Norbert and Maier, Elisabeth},
	title = {Utilizing Statistical Dialogue Act Processing in VERBMOBIL},
	booktitle = {Proceedings of the 33rd Annual Meeting on Association for Computational Linguistics},
	series = {ACL '95},
	year = {1995},
	location = {Cambridge, Massachusetts},
	pages = {116--121},
	numpages = {6},
	url = {http://dx.doi.org/10.3115/981658.981674},
	doi = {10.3115/981658.981674},
	acmid = {981674},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
} 

@book{Moore:1994:PED:197236,
	author = {Moore, Johanna D.},
	title = {Participating in Explanatory Dialogues: Interpreting and Responding to Questions in Context},
	year = {1994},
	isbn = {0-262-13301-6},
	publisher = {MIT Press},
	address = {Cambridge, MA, USA},
} 

@inproceedings{Mittal:1995:DGF:223904.223916,
	author = {Mittal, Vibhu O. and Moore, Johanna D.},
	title = {Dynamic Generation of Follow Up Question Menus: Facilitating Interactive Natural Language Dialogues},
	booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
	series = {CHI '95},
	year = {1995},
	isbn = {0-201-84705-1},
	location = {Denver, Colorado, USA},
	pages = {90--97},
	numpages = {8},
	url = {http://dx.doi.org/10.1145/223904.223916},
	doi = {10.1145/223904.223916},
	acmid = {223916},
	publisher = {ACM Press/Addison-Wesley Publishing Co.},
	address = {New York, NY, USA},
} 

@article{D'mello:2013:AAA:2395123.2395128,
	author = {D'mello, Sidney and Graesser, Art},
	title = {AutoTutor and Affective Autotutor: Learning by Talking with Cognitively and Emotionally Intelligent Computers That Talk Back},
	journal = {ACM Trans. Interact. Intell. Syst.},
	issue_date = {December 2012},
	volume = {2},
	number = {4},
	month = jan,
	year = {2013},
	issn = {2160-6455},
	pages = {23:1--23:39},
	articleno = {23},
	numpages = {39},
	url = {http://doi.acm.org/10.1145/2395123.2395128},
	doi = {10.1145/2395123.2395128},
	acmid = {2395128},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Intelligent tutoring systems, affect detection and synthesis, affective computing, constructivism, deep learning, natural language understanding, student modeling, user modeling},
} 

@article{Forbes-Riley:2008:RIS:1341585.1341623,
	author = {Forbes-Riley, Kate and Rotaru, Mihai and Litman, Diane J.},
	title = {The Relative Impact of Student Affect on Performance Models in a Spoken Dialogue Tutoring System},
	journal = {User Modeling and User-Adapted Interaction},
	issue_date = {February  2008},
	volume = {18},
	number = {1-2},
	month = feb,
	year = {2008},
	issn = {0924-1868},
	pages = {11--43},
	numpages = {33},
	url = {http://dx.doi.org/10.1007/s11257-007-9038-5},
	doi = {10.1007/s11257-007-9038-5},
	acmid = {1341623},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Adaptive spoken dialogue systems, Affective user modeling, Discourse structure, Emotional speech, Multiple linear regression, System performance modeling, Tutorial dialogue systems},
} 

@misc{mud2016,
	howpublished = {\url{http://shonan.nii.ac.jp/shonan/blog/2015/04/04/mining-modeling-unstructured-data-in-software-\%E2\%80\%90-challenges-for-the-future-2/}},
	note = {Accessed October 25, 2016},
	title = {Mining \& Modeling Unstructured Data in Software ‐ Challenges for the Future},
	author = {Sonia Haiduc and Takashi Kobayashi and Michele Lanza and Andrian Marcus}
}

@misc{nlse2015,
	howpublished = {\url{http://www.languageandcode.org/nlse2015/}},
	note = {Accessed October 25, 2016},
	title = {NSF Interdisciplinary Workshop on Statistical NLP and Software Engineering},
	author = {Devanbu, Prem and Quirk, Chris}
}

@article{deemter2012generation,
	title={Generation of referring expressions: Assessing the incremental algorithm},
	author={Deemter, Kees van and Gatt, Albert and Sluis, Ielka van der and Power, Richard},
	journal={Cognitive science},
	volume={36},
	number={5},
	pages={799--836},
	year={2012},
	publisher={Wiley Online Library}
}

@article{paraboni2007generating,
	title={Generating referring expressions: Making referents easy to identify},
	author={Paraboni, Ivandr{\'e} and Van Deemter, Kees and Masthoff, Judith},
	journal={Computational Linguistics},
	volume={33},
	number={2},
	pages={229--254},
	year={2007},
	publisher={MIT Press}
}

@inproceedings{gonzalez2004constant,
	title={Constant, constant, multi-tasking craziness: managing multiple working spheres},
	author={Gonz{\'a}lez, Victor M and Mark, Gloria},
	booktitle={Proceedings of the SIGCHI conference on Human factors in computing systems},
	pages={113--120},
	year={2004},
	organization={ACM}
}

@inproceedings{latoza2006maintaining,
	title={Maintaining mental models: a study of developer work habits},
	author={LaToza, Thomas D and Venolia, Gina and DeLine, Robert},
	booktitle={Proceedings of the 28th international conference on Software engineering},
	pages={492--501},
	year={2006},
	organization={ACM}
}

@article{sillito2008asking,
	title={Asking and answering questions during a programming change task},
	author={Sillito, Jonathan and Murphy, Gail C and De Volder, Kris},
	journal={IEEE Transactions on Software Engineering},
	volume={34},
	number={4},
	pages={434--451},
	year={2008},
	publisher={IEEE}
}

@article{ko2006exploratory,
	title={An exploratory study of how developers seek, relate, and collect relevant information during software maintenance tasks},
	author={Ko, Andrew J and Myers, Brad A and Coblenz, Michael J and Aung, Htet Htet},
	journal={IEEE Transactions on software engineering},
	volume={32},
	number={12},
	pages={971--987},
	year={2006},
	publisher={IEEE}
}

@article{DBLP:journals/corr/ChoMGBSB14,
	author    = {Kyunghyun Cho and
	Bart van Merrienboer and
	{\c{C}}aglar G{\"{u}}l{\c{c}}ehre and
	Fethi Bougares and
	Holger Schwenk and
	Yoshua Bengio},
	title     = {Learning Phrase Representations using {RNN} Encoder-Decoder for Statistical
	Machine Translation},
	journal   = {CoRR},
	volume    = {abs/1406.1078},
	year      = {2014},
	url       = {http://arxiv.org/abs/1406.1078},
	timestamp = {Wed, 02 Jul 2014 08:24:58 +0200},
	biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/ChoMGBSB14},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/SutskeverVL14,
	author    = {Ilya Sutskever and
	Oriol Vinyals and
	Quoc V. Le},
	title     = {Sequence to Sequence Learning with Neural Networks},
	journal   = {CoRR},
	volume    = {abs/1409.3215},
	year      = {2014},
	url       = {http://arxiv.org/abs/1409.3215},
	timestamp = {Wed, 01 Oct 2014 15:00:04 +0200},
	biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/SutskeverVL14},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}



@inproceedings{manning2014stanford,
	title={The Stanford CoreNLP Natural Language Processing Toolkit.},
	author={Manning, Christopher D and Surdeanu, Mihai and Bauer, John and Finkel, Jenny Rose and Bethard, Steven and McClosky, David},
	booktitle={ACL (System Demonstrations)},
	pages={55--60},
	year={2014}
}

@inproceedings{ferreira2014classification,
	title={Classification-based referring expression generation},
	author={Ferreira, Thiago Castro and Paraboni, Ivandr{\'e}},
	booktitle={International Conference on Intelligent Text Processing and Computational Linguistics},
	pages={481--491},
	year={2014},
	organization={Springer}
}

@inproceedings{hou2005can,
	title={What can programmer questions tell us about frameworks?},
	author={Hou, Daqing and Wong, Kenny and Hoover, H James},
	booktitle={13th International Workshop on Program Comprehension (IWPC'05)},
	pages={87--96},
	year={2005},
	organization={IEEE}
}

@inproceedings{roehm2012professional,
	title={How do professional developers comprehend software?},
	author={Roehm, Tobias and Tiarks, Rebecca and Koschke, Rainer and Maalej, Walid},
	booktitle={Proceedings of the 34th International Conference on Software Engineering},
	pages={255--265},
	year={2012},
	organization={IEEE Press}
}

@article{robillard2004effective,
	title={How effective developers investigate source code: An exploratory study},
	author={Robillard, Martin P and Coelho, Wesley and Murphy, Gail C},
	journal={IEEE Transactions on Software Engineering},
	volume={30},
	number={12},
	pages={889--903},
	year={2004},
	publisher={IEEE}
}


biblio2.bib
@inproceedings{mcmillan2014teaching,
	title={Teaching students to understand large programs by understanding historical context},
	author={McMillan, Collin and Oosterhoff, Richard},
	booktitle={Companion Proceedings of the 36th International Conference on Software Engineering},
	pages={287--290},
	year={2014},
	organization={ACM}
}

@article{huo2014expert,
	title={An Empirical Study of the Effects of Expect Knowledge on Bug Reports},
	author={Huo, Da and Ding, Tao and McMillan, Collin and Gethers, Malcom},
	journal={International Conference on Software Maintenance and Evolution},
	year={2014},
	publisher={IEEE}
}

@article{lohse1997consumer,
	title={Consumer eye movement patterns on yellow pages advertising},
	author={Lohse, Gerald L},
	journal={Journal of Advertising},
	volume={26},
	number={1},
	pages={61--73},
	year={1997},
	publisher={Taylor \& Francis}
}

@article{mourant1970mapping,
	title={Mapping eye-movement patterns to the visual scene in driving: An exploratory study},
	author={Mourant, Ronald R and Rockwell, Thomas H},
	journal={Human Factors: The Journal of the Human Factors and Ergonomics Society},
	volume={12},
	number={1},
	pages={81--87},
	year={1970},
	publisher={Sage Publications}
}

@inproceedings{Siegmund:2014:UUS:2568225.2568252,
	author = {Siegmund, Janet and K\"{a}stner, Christian and Apel, Sven and Parnin, Chris and Bethmann, Anja and Leich, Thomas and Saake, Gunter and Brechmann, Andr{\'e}},
	title = {Understanding Understanding Source Code with Functional Magnetic Resonance Imaging},
	booktitle = {Proceedings of the 36th International Conference on Software Engineering},
	series = {ICSE 2014},
	year = {2014},
	isbn = {978-1-4503-2756-5},
	location = {Hyderabad, India},
	pages = {378--389},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/2568225.2568252},
	doi = {10.1145/2568225.2568252},
	acmid = {2568252},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Functional magnetic resonance imaging, program comprehension},
} 

@inproceedings{kanade2000comprehensive,
	title={Comprehensive database for facial expression analysis},
	author={Kanade, Takeo and Cohn, Jeffrey F and Tian, Yingli},
	booktitle={Automatic Face and Gesture Recognition, 2000. Proceedings. Fourth IEEE International Conference on},
	pages={46--53},
	year={2000},
	organization={IEEE}
}

@inproceedings{harman1997amorphous,
	title={Amorphous program slicing},
	author={Harman, Mark and Danicic, Sebastian},
	booktitle={Program Comprehension, 1997. IWPC'97. Proceedings., Fifth Iternational Workshop on},
	pages={70--79},
	year={1997},
	organization={IEEE}
}

@article{potter1989fragmented,
	title={Fragmented ideologies: Accounts of educational failure and positive discrimination},
	author={Potter, Jonathan and Wetherell, Margaret},
	journal={Text},
	volume={9},
	number={2},
	pages={175--90},
	year={1989},
	publisher={Mouton de Gruyter}
}

@article{giangreco1997attitudes,
	title={Attitudes about educational and related service provision for students with deaf-blindness and multiple disabilities},
	author={Giangreco, Michael F and Edelman, SUSAN W and MacFarland, Stephanie and Luiselli, Tracy Evans},
	journal={Exceptional Children},
	volume={63},
	pages={329--342},
	year={1997},
	publisher={Council for Exceptional Children}
}

@article{mangrubang2005issues,
	title={Issues and trends in science education: The shortage of qualified science teachers},
	author={Mangrubang, Fred R},
	journal={American annals of the deaf},
	volume={150},
	number={1},
	pages={42--46},
	year={2005},
	publisher={Gallaudet University Press}
}

@article{smith2002diversity,
	title={Diversity and disability: exploring the experiences of vision impaired people in the workplace},
	author={Smith, Theresa},
	journal={Equal Opportunities International},
	volume={21},
	number={8},
	pages={59--72},
	year={2002},
	publisher={MCB UP Ltd}
}

@article{o1999employment,
	title={Employment Barriers for People with Visual Impairments.},
	author={O'Day, Bonnie},
	journal={Journal of Visual Impairment \& Blindness},
	volume={93},
	number={10},
	year={1999}
}

@article{vanderheiden1998universal,
	title={Universal design and assistive technology in communication and information technologies: alternatives or complements?},
	author={Vanderheiden, Gregg C},
	journal={Assistive Technology},
	volume={10},
	number={1},
	pages={29--36},
	year={1998},
	publisher={Taylor \& Francis}
}

@inproceedings{Wilson:2001:CSI:364447.364581,
	author = {Wilson, Brenda Cantwell and Shrock, Sharon},
	title = {Contributing to Success in an Introductory Computer Science Course: A Study of Twelve Factors},
	booktitle = {Proceedings of the Thirty-second SIGCSE Technical Symposium on Computer Science Education},
	series = {SIGCSE '01},
	year = {2001},
	isbn = {1-58113-329-4},
	location = {Charlotte, North Carolina, USA},
	pages = {184--188},
	numpages = {5},
	url = {http://doi.acm.org/10.1145/364447.364581},
	doi = {10.1145/364447.364581},
	acmid = {364581},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{ellson2002graphviz,
	title={Graphviz—open source graph drawing tools},
	author={Ellson, John and Gansner, Emden and Koutsofios, Lefteris and North, Stephen C and Woodhull, Gordon},
	booktitle={Graph Drawing},
	pages={483--484},
	year={2002},
	organization={Springer}
}

@article{hayes2006computing,
	title={Computing Science: The Semicolon Wars},
	author={Hayes, Brian},
	journal={American Scientist},
	pages={299--303},
	year={2006},
	publisher={JSTOR}
}

@INPROCEEDINGS{175815,
	author={Johnson, B. and Shneiderman, B.},
	booktitle={Visualization, 1991. Visualization '91, Proceedings., IEEE Conference on},
	title={Tree-maps: a space-filling approach to the visualization of hierarchical information structures},
	year={1991},
	month={Oct},
	pages={284-291},
	keywords={computer graphics;data analysis;trees (mathematics);display space;hierarchical information structures;rectangular region;semantic information;space-filling approach;tree-map visualization technique;visualization;Computer displays;Computer science;Educational institutions;Feedback;Humans;Laboratories;Libraries;Marine vehicles;Two dimensional displays;Visualization},
	doi={10.1109/VISUAL.1991.175815}
}

@article{d2007raised,
	title={Raised-Line Pictures, Blindness, and Tactile" Beliefs": An Observational Case Study.},
	author={D'Angiulli, Amedeo},
	journal={Journal of Visual Impairment \& Blindness},
	volume={101},
	number={3},
	pages={172--177},
	year={2007},
	publisher={ERIC}
}

@inproceedings{bigham2008inspiring,
	title={Inspiring blind high school students to pursue computer science with instant messaging chatbots},
	author={Bigham, Jeffrey P and Aller, Maxwell B and Brudvik, Jeremy T and Leung, Jessica O and Yazzolino, Lindsay A and Ladner, Richard E},
	booktitle={ACM SIGCSE Bulletin},
	volume={40},
	number={1},
	pages={449--453},
	year={2008},
	organization={ACM}
}

@article{Griffith01081990,
	author = {Griffith, Doug}, 
	title = {Computer Access for Persons Who Are Blind or Visually Impaired: Human Factors Issues},
	volume = {32}, 
	number = {4}, 
	pages = {467-475}, 
	year = {1990}, 
	doi = {10.1177/001872089003200408}, 
	abstract ={Suitably adapted computers hold considerable potential for integrating people who are blind or visually impaired into the mainstream. The principal problems that preclude the achievement of this potential are human factors issues. These issues are discussed, and the problems presented by icon-based interfaces are reviewed. An argument is offered that these issues, which ostensibly pertain to the blind or visually impaired user, are fundamental issues confronting all users. There is reason to hope that the benefits of research into the human factors issues of people with vision impairments will also extend to the sighted user.}, 
	URL = {http://hfs.sagepub.com/content/32/4/467.abstract}, 
	eprint = {http://hfs.sagepub.com/content/32/4/467.full.pdf+html}, 
	journal = {Human Factors: The Journal of the Human Factors and Ergonomics Society} 
}

@article{Kennel:1996:WWW:231674.231675,
	author = {Kennel, Andrea and Perrochon, Louis and Darvishi, Alireza},
	title = {WAB: World Wide Web Access for Blind and Visually Impaired Computer Users},
	journal = {SIGCAPH Comput. Phys. Handicap.},
	issue_date = {June 1996},
	number = {55},
	month = jun,
	year = {1996},
	issn = {0163-5727},
	pages = {10--15},
	numpages = {6},
	url = {http://doi.acm.org/10.1145/231674.231675},
	doi = {10.1145/231674.231675},
	acmid = {231675},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {WWW, W3, blindness and visual impairment, document structure and formats, proxy Servers, screen reader, user interfaces},
}

@article{Stefik:2013:EIP:2543488.2534973,
	author = {Stefik, Andreas and Siebert, Susanna},
	title = {An Empirical Investigation into Programming Language Syntax},
	journal = {Trans. Comput. Educ.},
	issue_date = {November 2013},
	volume = {13},
	number = {4},
	month = nov,
	year = {2013},
	issn = {1946-6226},
	pages = {19:1--19:40},
	articleno = {19},
	numpages = {40},
	url = {http://doi.acm.org/10.1145/2534973},
	doi = {10.1145/2534973},
	acmid = {2534973},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Novice Programmers, Programming Languages, Syntax},
} 

@inproceedings{Stefik:2011:ECA:2089155.2089159,
	author = {Stefik, Andreas and Siebert, Susanna and Stefik, Melissa and Slattery, Kim},
	title = {An Empirical Comparison of the Accuracy Rates of Novices Using the Quorum, Perl, and Randomo Programming Languages},
	booktitle = {Proceedings of the 3rd ACM SIGPLAN Workshop on Evaluation and Usability of Programming Languages and Tools},
	series = {PLATEAU '11},
	year = {2011},
	isbn = {978-1-4503-1024-6},
	location = {Portland, Oregon, USA},
	pages = {3--8},
	numpages = {6},
	url = {http://doi.acm.org/10.1145/2089155.2089159},
	doi = {10.1145/2089155.2089159},
	acmid = {2089159},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {comprehension, intuitiveness, language reductionism, programming languages},
} 

@INPROCEEDINGS{5090064,
	author={Stefik, A. and Haywood, A. and Mansoor, S. and Dunda, B. and Garcia, D.},
	booktitle={Program Comprehension, 2009. ICPC '09. IEEE 17th International Conference on},
	title={SODBeans},
	year={2009},
	month={May},
	pages={293-294},
	keywords={program debugging;Netbeans;Sonified Omniscient Debugger;accessibility architecture;computer programs debugging;debugging environments;program audio-based representations;program execution;sighted programmers;visual information;Computer displays;Computer science;Debugging;Eyes;Humans;Program processors;Programming environments;Programming profession;Speech;User interfaces},
	doi={10.1109/ICPC.2009.5090064},
	ISSN={1092-8138}
}

@inproceedings{Stefik:2011:DEI:1953163.1953323,
	author = {Stefik, Andreas M. and Hundhausen, Christopher and Smith, Derrick},
	title = {On the Design of an Educational Infrastructure for the Blind and Visually Impaired in Computer Science},
	booktitle = {Proceedings of the 42Nd ACM Technical Symposium on Computer Science Education},
	series = {SIGCSE '11},
	year = {2011},
	isbn = {978-1-4503-0500-6},
	location = {Dallas, TX, USA},
	pages = {571--576},
	numpages = {6},
	url = {http://doi.acm.org/10.1145/1953163.1953323},
	doi = {10.1145/1953163.1953323},
	acmid = {1953323},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {accessibility, assistive technology, auditory debugging, visual impairments},
}

@incollection{textsumchap2011,
	year={2011},
	isbn={978-3-642-17088-1},
	booktitle={Knowledge in Formation},
	series={Cognitive Technologies},
	doi={10.1007/978-3-642-17089-8_9},
	title={Text summarization},
	url={http://dx.doi.org/10.1007/978-3-642-17089-8_9},
	publisher={Springer Berlin Heidelberg},
	author={Sarbo, JanosJ. and Farkas, JozsefI. and Breemen, AukeJ.J.},
	pages={151-164},
	language={English}
}

@INPROCEEDINGS{1181320,
	author={Fang Chen and Kesong Han and Guilin Chen},
	booktitle={TENCON '02. Proceedings. 2002 IEEE Region 10 Conference on Computers, Communications, Control and Power Engineering},
	title={An approach to sentence-selection-based text summarization},
	year={2002},
	volume={1},
	pages={489-493 vol.1},
	keywords={feature extraction;text analysis;word processing;Chinese processing;performance;sentence length feature;sentence level features;sentence selection;text summarization;topic sensitive word feature;word level features;Australia;Character generation;Costing;Costs;Kernel;Supervised learning;Tagging},
	doi={10.1109/TENCON.2002.1181320}
}

@article{Wang:2012:CDS:2362383.2362386,
	author = {Wang, Dingding and Zhu, Shenghuo and Li, Tao and Gong, Yihong},
	title = {Comparative Document Summarization via Discriminative Sentence Selection},
	journal = {ACM Trans. Knowl. Discov. Data},
	issue_date = {October 2012},
	volume = {6},
	number = {3},
	month = oct,
	year = {2012},
	issn = {1556-4681},
	pages = {12:1--12:18},
	articleno = {12},
	numpages = {18},
	url = {http://doi.acm.org/10.1145/2362383.2362386},
	doi = {10.1145/2362383.2362386},
	acmid = {2362386},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Comparative document summarization, discriminative sentence selection},
}

@inproceedings{Goldstein:1999:STD:312624.312665,
	author = {Goldstein, Jade and Kantrowitz, Mark and Mittal, Vibhu and Carbonell, Jaime},
	title = {Summarizing Text Documents: Sentence Selection and Evaluation Metrics},
	booktitle = {Proceedings of the 22Nd Annual International ACM SIGIR Conference on Research and Development in Information Retrieval},
	series = {SIGIR '99},
	year = {1999},
	isbn = {1-58113-096-1},
	location = {Berkeley, California, USA},
	pages = {121--128},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/312624.312665},
	doi = {10.1145/312624.312665},
	acmid = {312665},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Radev:2000:CSM:1567564.1567567,
	author = {Radev, Dragomir R. and Jing, Hongyan and Budzikowska, Malgorzata},
	title = {Centroid-based Summarization of Multiple Documents: Sentence Extraction, Utility-based Evaluation, and User Studies},
	booktitle = {Proceedings of the 2000 NAACL-ANLP Workshop on Automatic Summarization},
	series = {NAACL-ANLP-AutoSum '00},
	year = {2000},
	location = {Seattle, Washington},
	pages = {21--30},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=1567564.1567567},
	acmid = {1567567},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
} 

@article{SparckJones:2007:ASS:1284916.1285154,
	author = {Sp\"{a}rck Jones, Karen},
	title = {Automatic Summarising: The State of the Art},
	journal = {Inf. Process. Manage.},
	issue_date = {November, 2007},
	volume = {43},
	number = {6},
	month = nov,
	year = {2007},
	issn = {0306-4573},
	pages = {1449--1481},
	numpages = {33},
	url = {http://dx.doi.org/10.1016/j.ipm.2007.03.009},
	doi = {10.1016/j.ipm.2007.03.009},
	acmid = {1285154},
	publisher = {Pergamon Press, Inc.},
	address = {Tarrytown, NY, USA},
	keywords = {Abstraction natural language processing, Evaluation, Sentence extraction, Summarization},
}

@article{Luhn:1958:BIS:1662374.1662381,
	author = {Luhn, H. P.},
	title = {A Business Intelligence System},
	journal = {IBM J. Res. Dev.},
	issue_date = {October 1958},
	volume = {2},
	number = {4},
	month = oct,
	year = {1958},
	issn = {0018-8646},
	pages = {314--319},
	numpages = {6},
	url = {http://dx.doi.org/10.1147/rd.24.0314},
	doi = {10.1147/rd.24.0314},
	acmid = {1662381},
	publisher = {IBM Corp.},
	address = {Riverton, NJ, USA},
} 

@article{Corbi:1989:PUC:97118.97124,
	author = {Corbi, T. A.},
	title = {Program understanding: challenge for the 1990's},
	journal = {IBM Syst. J.},
	issue_date = {1989},
	volume = {28},
	number = {2},
	month = jun,
	year = {1989},
	issn = {0018-8670},
	pages = {294--306},
	numpages = {13},
	url = {http://dx.doi.org/10.1147/sj.282.0294},
	doi = {10.1147/sj.282.0294},
	acmid = {97124},
	publisher = {IBM Corp.},
	address = {Riverton, NJ, USA},
}

@misc{NSF-2013-GPG,
	author=	"National Science Foundation",
	howpublished=	"Published online",
	month=		"January",
	title=		"Grant Proposal Guide",
	year=		"2013"
}

@inproceedings{Cleland-Huang:2011:GCB:1987856.1987861,
	author = {Cleland-Huang, Jane and Czauderna, Adam and Dekhtyar, Alex and Gotel, Olly and Hayes, Jane Huffman and Keenan, Ed and Leach, Greg and Maletic, Jonathan and Poshyvanyk, Denys and Shin, Youghee and Zisman, Andrea and Antoniol, Giuliano and Berenbach, Brian and Egyed, Alexander and Maeder, Patrick},
	title = {Grand Challenges, Benchmarks, and TraceLab: Developing Infrastructure for the Software Traceability Research Community},
	booktitle = {Proceedings of the 6th International Workshop on Traceability in Emerging Forms of Software Engineering},
	series = {TEFSE '11},
	year = {2011},
	isbn = {978-1-4503-0589-1},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {17--23},
	numpages = {7},
	url = {http://doi.acm.org/10.1145/1987856.1987861},
	doi = {10.1145/1987856.1987861},
	acmid = {1987861},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {benchmarks, metrics, traceability, tracelab},
} 

@inproceedings{Papineni:2002:BMA:1073083.1073135,
	author = {Papineni, Kishore and Roukos, Salim and Ward, Todd and Zhu, Wei-Jing},
	title = {BLEU: A Method for Automatic Evaluation of Machine Translation},
	booktitle = {Proceedings of the 40th Annual Meeting on Association for Computational Linguistics},
	series = {ACL '02},
	year = {2002},
	location = {Philadelphia, Pennsylvania},
	pages = {311--318},
	numpages = {8},
	url = {http://dx.doi.org/10.3115/1073083.1073135},
	doi = {10.3115/1073083.1073135},
	acmid = {1073135},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
}

@inproceedings{Papineni:2002:BMA:1073083.1073135,
	author = {Papineni, Kishore and Roukos, Salim and Ward, Todd and Zhu, Wei-Jing},
	title = {BLEU: A Method for Automatic Evaluation of Machine Translation},
	booktitle = {Proceedings of the 40th Annual Meeting on Association for Computational Linguistics},
	series = {ACL '02},
	year = {2002},
	location = {Philadelphia, Pennsylvania},
	pages = {311--318},
	numpages = {8},
	url = {http://dx.doi.org/10.3115/1073083.1073135},
	doi = {10.3115/1073083.1073135},
	acmid = {1073135},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
}

@inproceedings{Koehn:2007:MOS:1557769.1557821,
	author = {Koehn, Philipp and Hoang, Hieu and Birch, Alexandra and Callison-Burch, Chris and Federico, Marcello and Bertoldi, Nicola and Cowan, Brooke and Shen, Wade and Moran, Christine and Zens, Richard and Dyer, Chris and Bojar, Ond\v{r}ej and Constantin, Alexandra and Herbst, Evan},
	title = {Moses: Open Source Toolkit for Statistical Machine Translation},
	booktitle = {Proceedings of the 45th Annual Meeting of the ACL on Interactive Poster and Demonstration Sessions},
	series = {ACL '07},
	year = {2007},
	location = {Prague, Czech Republic},
	pages = {177--180},
	numpages = {4},
	url = {http://dl.acm.org/citation.cfm?id=1557769.1557821},
	acmid = {1557821},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
}

@article{Brown:1990:SAM:92858.92860,
	author = {Brown, Peter F. and Cocke, John and Pietra, Stephen A. Della and Pietra, Vincent J. Della and Jelinek, Fredrick and Lafferty, John D. and Mercer, Robert L. and Roossin, Paul S.},
	title = {A Statistical Approach to Machine Translation},
	journal = {Comput. Linguist.},
	issue_date = {June 1990},
	volume = {16},
	number = {2},
	month = jun,
	year = {1990},
	issn = {0891-2017},
	pages = {79--85},
	numpages = {7},
	url = {http://dl.acm.org/citation.cfm?id=92858.92860},
	acmid = {92860},
	publisher = {MIT Press},
	address = {Cambridge, MA, USA},
} 

@inproceedings{DBLP:conf/interspeech/KombrinkMKB11,
	author    = {Stefan Kombrink and
	Tomas Mikolov and
	Martin Karafi{\'a}t and
	Luk{\'a}s Burget},
	title     = {Recurrent Neural Network Based Language Modeling in Meeting
	Recognition},
	booktitle = {INTERSPEECH},
	year      = {2011},
	pages     = {2877-2880},
	ee        = {http://www.isca-speech.org/archive/interspeech_2011/i11_2877.html},
	crossref  = {DBLP:conf/interspeech/2011},
	bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{DBLP:conf/emnlp/VaswaniZFC13,
	author    = {Ashish Vaswani and
	Yinggong Zhao and
	Victoria Fossum and
	David Chiang},
	title     = {Decoding with Large-Scale Neural Language Models Improves
	Translation},
	booktitle = {EMNLP},
	year      = {2013},
	pages     = {1387-1392},
	ee        = {http://aclweb.org/anthology//D/D13/D13-1140.pdf},
	crossref  = {DBLP:conf/emnlp/2013},
	bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{Hindle:2012:NS:2337223.2337322,
	author = {Hindle, Abram and Barr, Earl T. and Su, Zhendong and Gabel, Mark and Devanbu, Premkumar},
	title = {On the Naturalness of Software},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {837--847},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337322},
	acmid = {2337322},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@inproceedings{Allamanis:2013:MSC:2487085.2487127,
	author = {Allamanis, Miltiadis and Sutton, Charles},
	title = {Mining Source Code Repositories at Massive Scale Using Language Modeling},
	booktitle = {Proceedings of the 10th Working Conference on Mining Software Repositories},
	series = {MSR '13},
	year = {2013},
	isbn = {978-1-4673-2936-1},
	location = {San Francisco, CA, USA},
	pages = {207--216},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=2487085.2487127},
	acmid = {2487127},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@inproceedings{Zhong:2009:MMR:1615184.1615205,
	author = {Zhong, Hao and Xie, Tao and Zhang, Lu and Pei, Jian and Mei, Hong},
	title = {MAPO: Mining and Recommending API Usage Patterns},
	booktitle = {Proceedings of the 23rd European Conference on ECOOP 2009 --- Object-Oriented Programming},
	series = {Genoa},
	year = {2009},
	isbn = {978-3-642-03012-3},
	location = {Italy},
	pages = {318--343},
	numpages = {26},
	url = {http://dx.doi.org/10.1007/978-3-642-03013-0_15},
	doi = {10.1007/978-3-642-03013-0_15},
	acmid = {1615205},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
}

@inproceedings{LijieWang:2011:AEW:2190078.2190135,
	author = {Lijie Wang and Lu Fang and Leye Wang and Ge Li and Bing Xie and Fuqing Yang},
	title = {APIExample: An effective web search based usage example recommendation system for java APIs},
	booktitle = {Proceedings of the 2011 26th IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '11},
	year = {2011},
	isbn = {978-1-4577-1638-6},
	pages = {592--595},
	numpages = {4},
	url = {http://dx.doi.org/10.1109/ASE.2011.6100133},
	doi = {10.1109/ASE.2011.6100133},
	acmid = {2190135},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Brandt:2010:EPI:1753326.1753402,
	author = {Brandt, Joel and Dontcheva, Mira and Weskamp, Marcos and Klemmer, Scott R.},
	title = {Example-centric programming: integrating web search into the development environment},
	booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
	series = {CHI '10},
	year = {2010},
	isbn = {978-1-60558-929-9},
	location = {Atlanta, Georgia, USA},
	pages = {513--522},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1753326.1753402},
	doi = {10.1145/1753326.1753402},
	acmid = {1753402},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {example-centric development},
} 

@article{Mcmillan:2013:PSR:2522920.2522930,
	author = {McMillan, Collin and Poshyvanyk, Denys and Grechanik, Mark and Xie, Qing and Fu, Chen},
	title = {Portfolio: Searching for Relevant Functions and Their Usages in Millions of Lines of Code},
	journal = {ACM Trans. Softw. Eng. Methodol.},
	issue_date = {October 2013},
	volume = {22},
	number = {4},
	month = oct,
	year = {2013},
	issn = {1049-331X},
	pages = {37:1--37:30},
	articleno = {37},
	numpages = {30},
	url = {http://doi.acm.org/10.1145/2522920.2522930},
	doi = {10.1145/2522920.2522930},
	acmid = {2522930},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Pagerank, Source-code search, information retrieval, natural language processing, user studies},
} 

@article{moritzexport,
	title={ExPort: Detecting and Visualizing API Usages in Large Source Code Repositories},
	author={Moritz, Evan and Linares-V{\'a}squez, Mario and Poshyvanyk, Denys and Grechanik, Mark and McMillan, Collin and Gethers, Malcom}
}

@inproceedings{LSSPaper,
	author = {Croft, David and Coupland, Simon and Shell, Jethro and Brown, Stephen},
	title = {A Fast and Efficient Semantic Short Text Similarity Metric},
} 

@article{Yuhua.TKDE.2006.130,
	author = {Yuhua Li and David McLean and Zuhair A. Bandar and James D. O'Shea and Keeley Crockett},
	title = {Sentence Similarity Based on Semantic Nets and Corpus Statistics},
	journal ={IEEE Transactions on Knowledge and Data Engineering},
	volume = {18},
	number = {8},
	issn = {1041-4347},
	year = {2006},
	pages = {1138-1150},
	doi = {http://doi.ieeecomputersociety.org/10.1109/TKDE.2006.130},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{OShea:2008:CST:1787839.1787859,
	author = {O'Shea, James and Bandar, Zuhair and Crockett, Keeley and McLean, David},
	title = {A comparative study of two short text semantic similarity measures},
	booktitle = {Proceedings of the 2nd KES International conference on Agent and multi-agent systems: technologies and applications},
	series = {KES-AMSTA'08},
	year = {2008},
	isbn = {3-540-78581-7, 978-3-540-78581-1},
	location = {Incheon, Korea},
	pages = {172--181},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=1787839.1787859},
	acmid = {1787859},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
	keywords = {benchmark, dialogue management, natural language, semantic similarity, sentence, user modeling},
} 

@inproceedings{Biggerstaff:1993:CAP:257572.257679,
	author = {Biggerstaff, Ted J. and Mitbander, Bharat G. and Webster, Dallas},
	title = {The concept assignment problem in program understanding},
	booktitle = {Proceedings of the 15th international conference on Software Engineering},
	series = {ICSE '93},
	year = {1993},
	isbn = {0-89791-588-7},
	location = {Baltimore, Maryland, USA},
	pages = {482--498},
	numpages = {17},
	url = {http://dl.acm.org/citation.cfm?id=257572.257679},
	acmid = {257679},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
	keywords = {concept recognition, connectionist, domain, knowledge base, plausible reasoning, reverse engineering, slicing},
} 

@article{Morse:1999:Minsize2,
	author={David T. Morse},
	journal={Educational and Psychological Measurement},
	title={Minsize2: A computer program for determining effect size and minimum sample size for statistical significance for univariate, multivariate, and nonparametric tests},
	year={1999},
	month={June},
	volume={59},
	number={3},
	pages={518--531},
	doi={10.1109/64.294135},
	ISSN={0885-9000}
}

@inproceedings{Smucker:07,
	author = {Smucker, Mark D. and Allan, James and Carterette, Ben},
	title = {A comparison of statistical significance tests for information retrieval evaluation},
	booktitle = {CIKM},
	year = {2007},
	pages = {623--632}
}

@book{STAT:05,
	author = {R. Mark Sirkin},
	title = {Statistics for the Social Sciences},
	month = {August},
	year = {2005},
	edition = "Third",
	pages = {632},
	publisher = {Sage Publications}
}

@book{IR:08,
	author = {Manning, Christopher D. and Raghavan, Prabhakar and Schtze, Hinrich},
	title = {Introduction to Information Retrieval},
	year = {2008},
	isbn = {0521865719, 9780521865715},
	publisher = {Cambridge University Press},
	address = {New York, NY, USA}
}

@inproceedings{Moreno:2013:ICPC,
	author = {Moreno, Laura and Aponte, Jairo and Sridhara Giriprasad and Marcus, Andrian and Pollock, Lori and Vijay-Shanker, K.},
	title = {Automatic Generation of Natural Language Summaries for Java Classes},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	year = {2013},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@inproceedings{Eddy:2013:ICPC,
	author = {Eddy, Brian and Robinson, Jeffrey and Kraft, Nicholas and Carver, Jeffrey},
	title = {Evaluating Source Code Summarization Techniques: Replication and Expansion},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	year = {2013},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@conference {Javadocminer,
	title = {{Automatic Quality Assessment of Source Code Comments: The JavadocMiner}},
	booktitle = {15th International Conference on Applications of Natural Language to Information Systems (NLDB 2010)},
	series = {Lecture Notes in Computer Science (LNCS)},
	volume = {6177/2010},
	year = {2010},
	month = {June 23--25},
	pages = {68--79},
	publisher = {Springer},
	organization = {Springer},
	address = {Cardiff, UK},
	isbn = {978-3-642-13880-5},
	doi = {10.1007/978-3-642-13881-2_7},
	url = {http://www.springerlink.com/content/n67470n270mt61m1/fulltext.pdf},
	attachments = {http://www.semanticsoftware.info/system/files/nldb2010-javadocminer.pdf},
	author = {Ninus Khamis and Ren{\'e} Witte and Juergen Rilling},
	editor = {Christina J. Hopfe and Yacine Rezgui and Elisabeth M{\'e}tais and Alun D. Preece and Haijiang Li}
}

@inproceedings{Steidl:2013:ICPC,
	author = {Steidl, Daniela and Hummel, Benjamin and Juergens, Elmar},
	title = {Quality Analysis of Source Code Comments},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	year = {2013},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@inproceedings{Gatt:2009:SRE:1610195.1610208,
	author = {Gatt, Albert and Reiter, Ehud},
	title = {SimpleNLG: a realisation engine for practical applications},
	booktitle = {Proceedings of the 12th European Workshop on Natural Language Generation},
	series = {ENLG '09},
	year = {2009},
	location = {Athens, Greece},
	pages = {90--93},
	numpages = {4},
	url = {http://dl.acm.org/citation.cfm?id=1610195.1610208},
	acmid = {1610208},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
}

@inproceedings{McMillan:2012:RSC:2337223.2337323,
	author = {McMillan, Collin and Hariri, Negar and Poshyvanyk, Denys and Cleland-Huang, Jane and Mobasher, Bamshad},
	title = {Recommending source code for use in rapid software prototypes},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {848--858},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337323},
	acmid = {2337323},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@inproceedings{McMillan:2011:PFR:1985793.1985809,
	author = {McMillan, Collin and Grechanik, Mark and Poshyvanyk, Denys and Xie, Qing and Fu, Chen},
	title = {Portfolio: finding relevant functions and their usage},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {111--120},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985809},
	doi = {10.1145/1985793.1985809},
	acmid = {1985809},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {code search, function call graph, pagerank, portfolio, ranking},
}

@inproceedings{Puppin:2006:SNJ:1141277.1141605,
	author = {Puppin, Diego and Silvestri, Fabrizio},
	title = {The social network of Java classes},
	booktitle = {Proceedings of the 2006 ACM symposium on Applied computing},
	series = {SAC '06},
	year = {2006},
	isbn = {1-59593-108-2},
	location = {Dijon, France},
	pages = {1409--1413},
	numpages = {5},
	url = {http://doi.acm.org/10.1145/1141277.1141605},
	doi = {10.1145/1141277.1141605},
	acmid = {1141605},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Inoue:2003:CRR:776816.776819,
	author = {Inoue, Katsuro and Yokomori, Reishi and Fujiwara, Hikaru and Yamamoto, Tetsuo and Matsushita, Makoto and Kusumoto, Shinji},
	title = {Component rank: relative significance rank for software component search},
	booktitle = {Proceedings of the 25th International Conference on Software Engineering},
	series = {ICSE '03},
	year = {2003},
	isbn = {0-7695-1877-X},
	location = {Portland, Oregon},
	pages = {14--24},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=776816.776819},
	acmid = {776819},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Chan:2012:SCA:2393596.2393606,
	author = {Chan, Wing-Kwan and Cheng, Hong and Lo, David},
	title = {Searching connected API subgraph via text phrases},
	booktitle = {Proceedings of the ACM SIGSOFT 20th International Symposium on the Foundations of Software Engineering},
	series = {FSE '12},
	year = {2012},
	isbn = {978-1-4503-1614-9},
	location = {Cary, North Carolina},
	pages = {10:1--10:11},
	articleno = {10},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2393596.2393606},
	doi = {10.1145/2393596.2393606},
	acmid = {2393606},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {API graph, API recommendation, subgraph searching},
}

@book{Langville:2006:GPB:1146372,
	author = {Langville, Amy N. and Meyer, Carl D.},
	title = {Google's PageRank and Beyond: The Science of Search Engine Rankings},
	year = {2006},
	isbn = {0691122024},
	publisher = {Princeton University Press},
	address = {Princeton, NJ, USA},
}

@inproceedings{Liu:2009:ITV:1645953.1646023,
	author = {Liu, Shixia and Zhou, Michelle X. and Pan, Shimei and Qian, Weihong and Cai, Weijia and Lian, Xiaoxiao},
	title = {Interactive, Topic-based Visual Text Summarization and Analysis},
	booktitle = {Proceedings of the 18th ACM Conference on Information and Knowledge Management},
	series = {CIKM '09},
	year = {2009},
	isbn = {978-1-60558-512-3},
	location = {Hong Kong, China},
	pages = {543--552},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1645953.1646023},
	doi = {10.1145/1645953.1646023},
	acmid = {1646023},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {interactive text visualization, stacked graph, text summarization, topic model},
}

@inproceedings{Wang:2012:UTM:2392800.2392808,
	author = {Wang, Lu and Cardie, Claire},
	title = {Unsupervised Topic Modeling Approaches to Decision Summarization in Spoken Meetings},
	booktitle = {Proceedings of the 13th Annual Meeting of the Special Interest Group on Discourse and Dialogue},
	series = {SIGDIAL '12},
	year = {2012},
	location = {Seoul, South Korea},
	pages = {40--49},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=2392800.2392808},
	acmid = {2392808},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
}

@inproceedings{Haghighi:2009:ECM:1620754.1620807,
	author = {Haghighi, Aria and Vanderwende, Lucy},
	title = {Exploring Content Models for Multi-document Summarization},
	booktitle = {Proceedings of Human Language Technologies: The 2009 Annual Conference of the North American Chapter of the Association for Computational Linguistics},
	series = {NAACL '09},
	year = {2009},
	isbn = {978-1-932432-41-1},
	location = {Boulder, Colorado},
	pages = {362--370},
	numpages = {9},
	url = {http://dl.acm.org/citation.cfm?id=1620754.1620807},
	acmid = {1620807},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
}

@inproceedings{Marcu2001,
	author = {Daniel Marcu and Laurie Gerber},
	year = {2001},
	title = {An Inquiry into the Nature of Multidocument Abstracts, Extracts, and Their Evaluation},
	booktitle = {NAACL-2001 Workshop on Automatic Summarization},
	location = {Pittsburgh, PA},
	month = {June},
	day = {3}
}

@inproceedings{Panichella:2013:EUT:2486788.2486857,
	author = {Panichella, Annibale and Dit, Bogdan and Oliveto, Rocco and Di Penta, Massimiliano and Poshyvanyk, Denys and De Lucia, Andrea},
	title = {How to Effectively Use Topic Models for Software Engineering Tasks? An Approach Based on Genetic Algorithms},
	booktitle = {Proceedings of the 2013 International Conference on Software Engineering},
	series = {ICSE '13},
	year = {2013},
	isbn = {978-1-4673-3076-3},
	location = {San Francisco, CA, USA},
	pages = {522--531},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=2486788.2486857},
	acmid = {2486857},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@incollection{mdtsutmfl,
	year={2013},
	isbn={978-3-642-39711-0},
	booktitle={Machine Learning and Data Mining in Pattern Recognition},
	volume={7988},
	series={Lecture Notes in Computer Science},
	editor={Perner, Petra},
	doi={10.1007/978-3-642-39712-7_12},
	title={Multi-document Text Summarization Using Topic Model and Fuzzy Logic},
	url={http://dx.doi.org/10.1007/978-3-642-39712-7_12},
	publisher={Springer Berlin Heidelberg},
	keywords={Fuzzy Systems; Data mining; Text Analysis; Semantics},
	author={Lee, Sanghoon and Belkasim, Saeid and Zhang, Yanqing},
	pages={159-168}
}

@inproceedings{Ladner:2012:IAC:2157136.2157354,
	author = {Ladner, Richard and Alkoby, Karen and Bigham, Jeff and Ludi, Stephanie and Marghitu, Daniela and Stefik, Andreas},
	title = {Improving the Accessibility of Computing Enrichment Programs (Abstract Only)},
	booktitle = {Proceedings of the 43rd ACM Technical Symposium on Computer Science Education},
	series = {SIGCSE '12},
	year = {2012},
	isbn = {978-1-4503-1098-7},
	location = {Raleigh, North Carolina, USA},
	pages = {662--662},
	numpages = {1},
	url = {http://doi.acm.org/10.1145/2157136.2157354},
	doi = {10.1145/2157136.2157354},
	acmid = {2157354},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {computing enrichment, disability, programming},
} 

@inproceedings{Haiduc:2010:UAT:1919284.1919577,
	author = {Haiduc, Sonia and Aponte, Jairo and Moreno, Laura and Marcus, Andrian},
	title = {On the Use of Automated Text Summarization Techniques for Summarizing Source Code},
	booktitle = {Proceedings of the 2010 17th Working Conference on Reverse Engineering},
	series = {WCRE '10},
	year = {2010},
	isbn = {978-0-7695-4123-5},
	pages = {35--44},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/WCRE.2010.13},
	doi = {10.1109/WCRE.2010.13},
	acmid = {1919577},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {text summarization, program comprehension},
}

@inproceedings{Aponte:2011:ITL:1987856.1987867,
	author = {Aponte, Jairo and Marcus, Andrian},
	title = {Improving traceability link recovery methods through software artifact summarization},
	booktitle = {Proceedings of the 6th International Workshop on Traceability in Emerging Forms of Software Engineering},
	series = {TEFSE '11},
	year = {2011},
	isbn = {978-1-4503-0589-1},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {46--49},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1987856.1987867},
	doi = {10.1145/1987856.1987867},
	acmid = {1987867},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {information retrieval, program comprehension, summarization, traceability management},
}

@article{Goldberg:FOG,
	author={Goldberg, E. and Driedger, N. and Kittredge, R.I.},
	journal={IEEE Expert}, title={Using natural-language processing to produce weather forecasts},
	year={1994},
	month={April},
	volume={9},
	number={2},
	pages={45-53},
	doi={10.1109/64.294135},
	ISSN={0885-9000}
}

@article{mcdonald2010natural,
	title={Natural Language Generation.},
	author={McDonald, David D},
	journal={Handbook of natural language processing},
	volume={2},
	pages={121--144},
	year={2010}
}

@book{Reiter:2000:BNL:331955,
	author = {Reiter, Ehud and Dale, Robert},
	title = {Building natural language generation systems},
	year = {2000},
	isbn = {0-521-62036-8},
	publisher = {Cambridge University Press},
	address = {New York, NY, USA},
} 

@PhdThesis{MurphyPhd96,
	title = "{Lightweight structural summarization as an aid to software evolution}",
	author = "Gail C. Murphy",
	school = "University of Washington",
	month = "July",
	year = "1996",
}

@PhdThesis{SridharaPhd12,
	title = "{Automatic Generation of Descriptive Summary Comments for Methods in Object-oriented Programs}",
	author = "Giriprasad Sridhara",
	school = "University of Delaware",
	month = Jan,
	year = "2012",
}

@inproceedings{Buse:2008:ADI:1390630.1390664,
	author = {Buse, Raymond P.L. and Weimer, Westley R.},
	title = {Automatic documentation inference for exceptions},
	booktitle = {Proceedings of the 2008 international symposium on Software testing and analysis},
	series = {ISSTA '08},
	year = {2008},
	isbn = {978-1-60558-050-0},
	location = {Seattle, WA, USA},
	pages = {273--282},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1390630.1390664},
	doi = {10.1145/1390630.1390664},
	acmid = {1390664},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation inference, exception handling, software documentation},
}

@inproceedings{Buse:2010:ADP:1858996.1859005,
	author = {Buse, Raymond P.L. and Weimer, Westley R.},
	title = {Automatically documenting program changes},
	booktitle = {Proceedings of the IEEE/ACM international conference on Automated software engineering},
	series = {ASE '10},
	year = {2010},
	isbn = {978-1-4503-0116-9},
	location = {Antwerp, Belgium},
	pages = {33--42},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1858996.1859005},
	doi = {10.1145/1858996.1859005},
	acmid = {1859005},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {code summarization, commit messages, differencing},
}

@ARTICLE{6165314,
	author={Miryung Kim and Notkin, D. and Grossman, D. and Wilson, G.},
	journal={IEEE Transactions on Software Engineering},
	title={Identifying and Summarizing Systematic Code Changes via Rule Inference},
	year={2013},
	month={Jan. },
	volume={39},
	number={1},
	pages={45 -62},
	doi={10.1109/TSE.2012.16},
	ISSN={0098-5589},
}

@inproceedings{SaiZhang:2011:ADI:2190078.2190153,
	author = {Sai Zhang and Cheng Zhang and Ernst, Michael D.},
	title = {Automated documentation inference to explain failed tests},
	booktitle = {Proceedings of the 2011 26th IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '11},
	year = {2011},
	isbn = {978-1-4577-1638-6},
	pages = {63--72},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ASE.2011.6100145},
	doi = {10.1109/ASE.2011.6100145},
	acmid = {2190153},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Holmes:2005:USC:1062455.1062491,
	author = {Holmes, Reid and Murphy, Gail C.},
	title = {Using structural context to recommend source code examples},
	booktitle = {Proceedings of the 27th international conference on Software engineering},
	series = {ICSE '05},
	year = {2005},
	isbn = {1-58113-963-2},
	location = {St. Louis, MO, USA},
	pages = {117--125},
	numpages = {9},
	url = {http://doi.acm.org/10.1145/1062455.1062491},
	doi = {10.1145/1062455.1062491},
	acmid = {1062491},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {development environment framework, examples, recommender, software structure},
}

@article{Krinke:2006:ECP:1167771.1167775,
	author = {Krinke, Jens},
	title = {Effects of context on program slicing},
	journal = {J. Syst. Softw.},
	issue_date = {September 2006},
	volume = {79},
	number = {9},
	month = sep,
	year = {2006},
	issn = {0164-1212},
	pages = {1249--1260},
	numpages = {12},
	url = {http://dx.doi.org/10.1016/j.jss.2006.02.040},
	doi = {10.1016/j.jss.2006.02.040},
	acmid = {1167775},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {program analysis, program slicing},
}

@inproceedings{deSouza:2005:SDE:1085313.1085331,
	author = {de Souza, Sergio Cozzetti B. and Anquetil, Nicolas and de Oliveira, K\'{a}thia M.},
	title = {A study of the documentation essential to software maintenance},
	booktitle = {Proceedings of the 23rd annual international conference on Design of communication: documenting \& designing for pervasive information},
	series = {SIGDOC '05},
	year = {2005},
	isbn = {1-59593-175-9},
	location = {Coventry, United Kingdom},
	pages = {68--75},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1085313.1085331},
	doi = {10.1145/1085313.1085331},
	acmid = {1085331},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {empirical study, program understanding, software maintenance, software system documentation},
} 

@inproceedings{Shi:2011:ESE:1987434.1987473,
	author = {Shi, Lin and Zhong, Hao and Xie, Tao and Li, Mingshu},
	title = {An empirical study on evolution of API documentation},
	booktitle = {Proceedings of the 14th international conference on Fundamental approaches to software engineering: part of the joint European conferences on theory and practice of software},
	series = {FASE'11/ETAPS'11},
	year = {2011},
	isbn = {978-3-642-19810-6},
	location = {Saarbr\&\#252;cken, Germany},
	pages = {416--431},
	numpages = {16},
	url = {http://dl.acm.org/citation.cfm?id=1987434.1987473},
	acmid = {1987473},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
}

@article{Kajko-Mattsson:2005:SDP:1032622.1035374,
	author = {Kajko-Mattsson, Mira},
	title = {A Survey of Documentation Practice within Corrective Maintenance},
	journal = {Empirical Softw. Engg.},
	issue_date = {January 2005},
	volume = {10},
	number = {1},
	month = jan,
	year = {2005},
	issn = {1382-3256},
	pages = {31--55},
	numpages = {25},
	url = {http://dx.doi.org/10.1023/B:LIDA.0000048322.42751.ca},
	doi = {10.1023/B:LIDA.0000048322.42751.ca},
	acmid = {1035374},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Corrective maintenance, software process documentation, software system documentation},
}

@inproceedings{Dekel:2009:IAD:1555001.1555047,
	author = {Dekel, Uri and Herbsleb, James D.},
	title = {Improving API documentation usability with knowledge pushing},
	booktitle = {Proceedings of the 31st International Conference on Software Engineering},
	series = {ICSE '09},
	year = {2009},
	isbn = {978-1-4244-3453-4},
	pages = {320--330},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2009.5070532},
	doi = {10.1109/ICSE.2009.5070532},
	acmid = {1555047},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Storey05,
	author={Storey, M.},
	booktitle={Program Comprehension, 2005. IWPC 2005. Proceedings. 13th International Workshop on},
	title={Theories, methods and tools in program comprehension: past, present and future},
	year={2005},
	pages={181-191},
	doi={10.1109/WPC.2005.38},
	ISSN={1092-8138}
}

@inproceedings{Dekel09,
	author={Dekel, Uri and Herbsleb, J.D.},
	booktitle={Program Comprehension, 2009. ICPC '09. IEEE 17th International Conference on},
	title={Reading the documentation of invoked API functions in program comprehension},
	year={2009},
	pages={168-177},
	doi={10.1109/ICPC.2009.5090040},
	ISSN={1092-8138}
}

@inproceedings{Fluri:2007:CCC:1339262.1339530,
	author = {Fluri, Beat and Wursch, Michael and Gall, Harald C.},
	title = {Do Code and Comments Co-Evolve? On the Relation between Source Code and Comment Changes},
	booktitle = {Proceedings of the 14th Working Conference on Reverse Engineering},
	series = {WCRE '07},
	year = {2007},
	isbn = {0-7695-3034-6},
	pages = {70--79},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/WCRE.2007.21},
	doi = {10.1109/WCRE.2007.21},
	acmid = {1339530},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Fluri:2009:ACC:1613014.1613065,
	author = {Fluri, Beat and W\"{u}rsch, Michael and Giger, Emanuel and Gall, Harald C.},
	title = {Analyzing the co-evolution of comments and source code},
	journal = {Software Quality Control},
	issue_date = {December  2009},
	volume = {17},
	number = {4},
	month = dec,
	year = {2009},
	issn = {0963-9314},
	pages = {367--394},
	numpages = {28},
	url = {http://dx.doi.org/10.1007/s11219-009-9075-x},
	doi = {10.1007/s11219-009-9075-x},
	acmid = {1613065},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Comment changes, Comment quality, Software evolution analysis, Software maintenance, Software repositories, Source code changes},
} 

@article{Ibrahim:2012:CCR:2330373.2330435,
	author = {Ibrahim, Walid M. and Bettenburg, Nicolas and Adams, Bram and Hassan, Ahmed E.},
	title = {Controversy Corner: On the relationship between comment update practices and Software Bugs},
	journal = {J. Syst. Softw.},
	issue_date = {October, 2012},
	volume = {85},
	number = {10},
	month = oct,
	year = {2012},
	issn = {0164-1212},
	pages = {2293--2304},
	numpages = {12},
	url = {http://dx.doi.org/10.1016/j.jss.2011.09.019},
	doi = {10.1016/j.jss.2011.09.019},
	acmid = {2330435},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {Code quality, Empirical studies, Software bugs, Software evolution, Source code comments},
} 

@inproceedings{Forward:2002:RSD:585058.585065,
	author = {Forward, Andrew and Lethbridge, Timothy C.},
	title = {The relevance of software documentation, tools and technologies: a survey},
	booktitle = {Proceedings of the 2002 ACM symposium on Document engineering},
	series = {DocEng '02},
	year = {2002},
	isbn = {1-58113-594-7},
	location = {McLean, Virginia, USA},
	pages = {26--33},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/585058.585065},
	doi = {10.1145/585058.585065},
	acmid = {585065},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation relevance, documentation survey, documentation technologies, program comprehension, software documentation, software engineering, software maintenance},
}

@inproceedings{Roehm:2012:PDC:2337223.2337254,
	author = {Roehm, Tobias and Tiarks, Rebecca and Koschke, Rainer and Maalej, Walid},
	title = {How do professional developers comprehend software?},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {255--265},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337254},
	acmid = {2337254},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@inproceedings{Friendly95thedesign,
	author = {Lisa Friendly},
	title = {The Design of Distributed Hyperlinked Programming Documentation},
	booktitle = {Proceedings of the International Workshop on Hypermedia Design},
	series = {IWDH '95},
	pages = {151--173},
	year = {1995}
}

@inproceedings{Kramer:1999:ADS:318372.318577,
	author = {Kramer, Douglas},
	title = {API documentation from source code comments: a case study of Javadoc},
	booktitle = {Proceedings of the 17th annual international conference on Computer documentation},
	series = {SIGDOC '99},
	year = {1999},
	isbn = {1-58113-072-4},
	location = {New Orleans, Louisiana, USA},
	pages = {147--153},
	numpages = {7},
	url = {http://doi.acm.org/10.1145/318372.318577},
	doi = {10.1145/318372.318577},
	acmid = {318577},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {API documentation, Java platform, Javadoc, doc comments, doclets, documentation comments, generated documentation, source code comments},
} 

@article{Sillito:2008:AAQ:1446226.1446241,
	author = {Sillito, Jonathan and Murphy, Gail C. and De Volder, Kris},
	title = {Asking and Answering Questions during a Programming Change Task},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {July 2008},
	volume = {34},
	number = {4},
	month = jul,
	year = {2008},
	issn = {0098-5589},
	pages = {434--451},
	numpages = {18},
	url = {http://dx.doi.org/10.1109/TSE.2008.26},
	doi = {10.1109/TSE.2008.26},
	acmid = {1446241},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Enhancement, Programming Environments/Construction Tools, Software psychology, Software psychology, Programming Environments/Construction Tools, Enhancement},
} 

@inproceedings{Sim:1998:ASC:580914.858229,
	author = {Sim, S. E. and Clarke, C. L. A. and Holt, R. C.},
	title = {Archetypal Source Code Searches: A Survey of Software Developers and Maintainers},
	booktitle = {Proceedings of the 6th International Workshop on Program Comprehension},
	series = {IWPC '98},
	year = {1998},
	isbn = {0-8186-8560-3},
	pages = {180--},
	url = {http://dl.acm.org/citation.cfm?id=580914.858229},
	acmid = {858229},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Duala-Ekoko:2012:AAQ:2337223.2337255,
	author = {Duala-Ekoko, Ekwa and Robillard, Martin P.},
	title = {Asking and answering questions about unfamiliar APIs: an exploratory study},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {266--276},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337255},
	acmid = {2337255},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@article{Binkley:2007:ESS:1217295.1217297,
	author = {Binkley, David and Gold, Nicolas and Harman, Mark},
	title = {An empirical study of static program slice size},
	journal = {ACM Trans. Softw. Eng. Methodol.},
	issue_date = {April 2007},
	volume = {16},
	number = {2},
	month = apr,
	year = {2007},
	issn = {1049-331X},
	articleno = {8},
	url = {http://doi.acm.org/10.1145/1217295.1217297},
	doi = {10.1145/1217295.1217297},
	acmid = {1217297},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Program slicing, slice size},
} 

@techreport{
	yiji_2012_tr,
	author = "Yiji Zhang and Raul Santelices",
	institution = "University of Notre Dame Computer Science Department",
	title = "Predicting Runtime Data Dependences for Slice Inspection Prioritization",
	number = "2012-02",
	month = "July",
	year = "2012"
}

@article{Miller:1995:WLD:219717.219748,
	author = {Miller, George A.},
	title = {WordNet: A Lexical Database for English},
	journal = {Commun. ACM},
	issue_date = {Nov. 1995},
	volume = {38},
	number = {11},
	month = nov,
	year = {1995},
	issn = {0001-0782},
	pages = {39--41},
	numpages = {3},
	url = {http://doi.acm.org/10.1145/219717.219748},
	doi = {10.1145/219717.219748},
	acmid = {219748},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Hill:2009:ACS:1555001.1555039,
	author = {Hill, Emily and Pollock, Lori and Vijay-Shanker, K.},
	title = {Automatically capturing source code context of NL-queries for software maintenance and reuse},
	booktitle = {Proceedings of the 31st International Conference on Software Engineering},
	series = {ICSE '09},
	year = {2009},
	isbn = {978-1-4244-3453-4},
	pages = {232--242},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2009.5070524},
	doi = {10.1109/ICSE.2009.5070524},
	acmid = {1555039},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Sridhara:2010:TAG:1858996.1859006,
	author = {Sridhara, Giriprasad and Hill, Emily and Muppaneni, Divya and Pollock, Lori and Vijay-Shanker, K.},
	title = {Towards automatically generating summary comments for Java methods},
	booktitle = {Proceedings of the IEEE/ACM international conference on Automated software engineering},
	series = {ASE '10},
	year = {2010},
	isbn = {978-1-4503-0116-9},
	location = {Antwerp, Belgium},
	pages = {43--52},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1858996.1859006},
	doi = {10.1145/1858996.1859006},
	acmid = {1859006},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {comment generation, method summarization, natural language program analysis},
} 

@inproceedings{Mani:2012:AAU:2393596.2393607,
	author = {Mani, Senthil and Catherine, Rose and Sinha, Vibha Singhal and Dubey, Avinava},
	title = {AUSUM: approach for unsupervised bug report summarization},
	booktitle = {Proceedings of the ACM SIGSOFT 20th International Symposium on the Foundations of Software Engineering},
	series = {FSE '12},
	year = {2012},
	isbn = {978-1-4503-1614-9},
	location = {Cary, North Carolina},
	pages = {11:1--11:11},
	articleno = {11},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2393596.2393607},
	doi = {10.1145/2393596.2393607},
	acmid = {2393607},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug report, summarization, unsupervised},
} 

@inproceedings{Burden:2011:NLG:2095654.2095665,
	author = {Burden, H{\aa}kan and Heldal, Rogardt},
	title = {Natural language generation from class diagrams},
	booktitle = {Proceedings of the 8th International Workshop on Model-Driven Engineering, Verification and Validation},
	series = {MoDeVVa},
	year = {2011},
	isbn = {978-1-4503-0914-1},
	location = {Wellington, New Zealand},
	pages = {8:1--8:8},
	articleno = {8},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/2095654.2095665},
	doi = {10.1145/2095654.2095665},
	acmid = {2095665},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {model transformations, model-driven architecture},
} 

@inproceedings{Sridhara:2011:GPC:2057176.2057211,
	author = {Sridhara, Giriprasad and Pollock, Lori and Vijay-Shanker, K.},
	title = {Generating Parameter Comments and Integrating with Method Summaries},
	booktitle = {Proceedings of the 2011 IEEE 19th International Conference on Program Comprehension},
	series = {ICPC '11},
	year = {2011},
	isbn = {978-0-7695-4398-7},
	pages = {71--80},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICPC.2011.28},
	doi = {10.1109/ICPC.2011.28},
	acmid = {2057211},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {documentation, software maintenance},
} 

@electronic{DoxygenWebsite,
	author        = "Dimitri van Heesch",
	title         = "Doxygen Website",
	url           = "http://www.stack.nl/~dimitri/doxygen/",
	year          = "2013"
}

@article{Curtis1989167,
	title = "Experimental evaluation of software documentation formats",
	journal = "Journal of Systems and Software",
	volume = "9",
	number = "2",
	pages = "167 - 207",
	year = "1989",
	issn = "0164-1212",
	doi = "10.1016/0164-1212(89)90019-8",
	url = "http://www.sciencedirect.com/science/article/pii/0164121289900198",
	author = "Bill Curtis and Sylvia B. Sheppard and Elizabeth Kruesi-Bailey and John Bailey and Deborah A. Boehm-Davis"
}

@inproceedings{Sridhara:2011:ADD:1985793.1985808,
	author = {Sridhara, Giriprasad and Pollock, Lori and Vijay-Shanker, K.},
	title = {Automatically detecting and describing high level actions within methods},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {101--110},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985808},
	doi = {10.1145/1985793.1985808},
	acmid = {1985808},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation, program comprehension},
} 

@article{Takang96,
	author = {Takang, A. A. and Grubb, P. A. and Macredie, R. D.},
	citeulike-article-id = {8398723},
	journal = {Journal of Programming Languages},
	keywords = {paolos, references},
	number = {3},
	pages = {143--167},
	posted-at = {2010-12-09 10:57:36},
	priority = {3},
	title = {{The Effects of Comments and Identifier Names on Program Comprehensibility: An Experimental Study}},
	volume = {4},
	year = {1996}
}

@INPROCEEDINGS{Lawrie06whatsin,
	author = {Dawn Lawrie and Christopher Morrell and Henry Feild and David Binkley},
	title = {What's in a name? a study of identifiers},
	booktitle = {In 14th International Conference on Program Comprehension},
	year = {2006},
	pages = {3--12},
	publisher = {IEEE Computer Society}
}

@article{Lethbridge:2003:SEU:950628.950726,
	author = {Lethbridge, Timothy C. and Singer, Janice and Forward, Andrew},
	title = {How Software Engineers Use Documentation: The State of the Practice},
	journal = {IEEE Softw.},
	issue_date = {November 2003},
	volume = {20},
	number = {6},
	month = nov,
	year = {2003},
	issn = {0740-7459},
	pages = {35--39},
	numpages = {5},
	url = {http://dx.doi.org/10.1109/MS.2003.1241364},
	doi = {10.1109/MS.2003.1241364},
	acmid = {950726},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
	keywords = {D.210.b Design notations and documentation, D.2.7.c Documentation, D.2.17g Code documentation},
}

@inproceedings{Stylos:2006:MWT:1174509.1174678,
	author = {Stylos, Jeffrey and Myers, Brad A.},
	title = {Mica: A Web-Search Tool for Finding API Components and Examples},
	booktitle = {Proceedings of the Visual Languages and Human-Centric Computing},
	series = {VLHCC '06},
	year = {2006},
	isbn = {0-7695-2586-5},
	pages = {195--202},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/VLHCC.2006.32},
	doi = {10.1109/VLHCC.2006.32},
	acmid = {1174678},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Eisenberg:2010:ANI:1753326.1753525,
	author = {Eisenberg, Daniel S. and Stylos, Jeffrey and Myers, Brad A.},
	title = {Apatite: a new interface for exploring APIs},
	booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
	series = {CHI '10},
	year = {2010},
	isbn = {978-1-60558-929-9},
	location = {Atlanta, Georgia, USA},
	pages = {1331--1334},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1753326.1753525},
	doi = {10.1145/1753326.1753525},
	acmid = {1753525},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {api documentation, browsing, search tools, visualizations, web applications},
} 

@inproceedings{Karrer:2011:SCG:2047196.2047225,
	author = {Karrer, Thorsten and Kr\"{a}mer, Jan-Peter and Diehl, Jonathan and Hartmann, Bj\"{o}rn and Borchers, Jan},
	title = {Stacksplorer: call graph navigation helps increasing code maintenance efficiency},
	booktitle = {Proceedings of the 24th annual ACM symposium on User interface software and technology},
	series = {UIST '11},
	year = {2011},
	isbn = {978-1-4503-0716-1},
	location = {Santa Barbara, California, USA},
	pages = {217--224},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/2047196.2047225},
	doi = {10.1145/2047196.2047225},
	acmid = {2047225},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {development tools / toolkits / programming environments, visualization},
}

@inproceedings{Tao:2012:SEU:2393596.2393656,
	author = {Tao, Yida and Dang, Yingnong and Xie, Tao and Zhang, Dongmei and Kim, Sunghun},
	title = {How do software engineers understand code changes?: an exploratory study in industry},
	booktitle = {Proceedings of the ACM SIGSOFT 20th International Symposium on the Foundations of Software Engineering},
	series = {FSE '12},
	year = {2012},
	isbn = {978-1-4503-1614-9},
	location = {Cary, North Carolina},
	pages = {51:1--51:11},
	articleno = {51},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2393596.2393656},
	doi = {10.1145/2393596.2393656},
	acmid = {2393656},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {code change, code review, information needs, tool support},
} 

@inproceedings{LaToza:2010:DAR:1806799.1806829,
	author = {LaToza, Thomas D. and Myers, Brad A.},
	title = {Developers ask reachability questions},
	booktitle = {Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering - Volume 1},
	series = {ICSE '10},
	year = {2010},
	isbn = {978-1-60558-719-6},
	location = {Cape Town, South Africa},
	pages = {185--194},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1806799.1806829},
	doi = {10.1145/1806799.1806829},
	acmid = {1806829},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {code navigation, developer questions, empirical study, program comprehension, software maintenance},
} 

@inproceedings{Stylos:2009:JIA:1520340.1520678,
	author = {Stylos, Jeffrey and Myers, Brad A. and Yang, Zizhuang},
	title = {Jadeite: improving API documentation using usage information},
	booktitle = {CHI '09 Extended Abstracts on Human Factors in Computing Systems},
	series = {CHI EA '09},
	year = {2009},
	isbn = {978-1-60558-247-4},
	location = {Boston, MA, USA},
	pages = {4429--4434},
	numpages = {6},
	url = {http://doi.acm.org/10.1145/1520340.1520678},
	doi = {10.1145/1520340.1520678},
	acmid = {1520678},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {APIs, documentation, javadoc},
}

@inproceedings{Ko:2004:SLB:1032665.1034570,
	author = {Ko, Andrew J. and Myers, Brad A. and Aung, Htet Htet},
	title = {Six Learning Barriers in End-User Programming Systems},
	booktitle = {Proceedings of the 2004 IEEE Symposium on Visual Languages - Human Centric Computing},
	series = {VLHCC '04},
	year = {2004},
	isbn = {0-7803-8696-5},
	pages = {199--206},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/VLHCC.2004.47},
	doi = {10.1109/VLHCC.2004.47},
	acmid = {1034570},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Steidl:2013:ICPC,
	author = {Steidl, Daniela and Hummel, Benjamin and Juergens, Elmar},
	title = {Quality Analysis of Source Code Comments},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	year = {2013},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@inproceedings{Smucker:07,
	author = {Smucker, Mark D. and Allan, James and Carterette, Ben},
	title = {A comparison of statistical significance tests for information retrieval evaluation},
	booktitle = {CIKM},
	year = {2007},
	pages = {623--632}
}

@inproceedings{Fagin:2003:CTK:644108.644113,
	author = {Fagin, Ronald and Kumar, Ravi and Sivakumar, D.},
	title = {Comparing top k lists},
	booktitle = {Proceedings of the fourteenth annual ACM-SIAM symposium on Discrete algorithms},
	series = {SODA '03},
	year = {2003},
	isbn = {0-89871-538-5},
	location = {Baltimore, Maryland},
	pages = {28--36},
	numpages = {9},
	url = {http://dl.acm.org/citation.cfm?id=644108.644113},
	acmid = {644113},
	publisher = {Society for Industrial and Applied Mathematics},
	address = {Philadelphia, PA, USA},
}

@article{Bansal:2009:CDP:1480540.1480730,
	author = {Bansal, Mukul S. and Fern\'{a}ndez-Baca, David},
	title = {Computing distances between partial rankings},
	journal = {Inf. Process. Lett.},
	issue_date = {January, 2009},
	volume = {109},
	number = {4},
	month = jan,
	year = {2009},
	issn = {0020-0190},
	pages = {238--241},
	numpages = {4},
	url = {http://dx.doi.org/10.1016/j.ipl.2008.10.010},
	doi = {10.1016/j.ipl.2008.10.010},
	acmid = {1480730},
	publisher = {Elsevier North-Holland, Inc.},
	address = {Amsterdam, The Netherlands, The Netherlands},
	keywords = {Algorithms, Kendall tau distance, Partial rankings, Top-m lists, p-ratings},
}

@article{wolfe1973nonparametric,
	title={Nonparametric statistical methods},
	author={Wolfe, Douglas A and Hollander, Myles},
	journal={Nonparametric statistical methods},
	year={1973},
	publisher={John Wiley New York}
}

@article{BBS:209012,
	author = {Rayner,Keith and Pollatsek,Alexander and Reichle,Erik D.},
	title = {Eye movements in reading: Models and data},
	journal = {Behavioral and Brain Sciences},
	volume = {26},
	issue = {04},
	month = {7},
	year = {2003},
	issn = {1469-1825},
	pages = {507--518},
	numpages = {12},
	doi = {10.1017/S0140525X03520106},
	URL = {http://journals.cambridge.org/article_S0140525X03520106},
}

@inproceedings{SaiZhang:2011:ADI:2190078.2190153,
	author = {Sai Zhang and Cheng Zhang and Ernst, Michael D.},
	title = {Automated documentation inference to explain failed tests},
	booktitle = {Proceedings of the 2011 26th IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '11},
	year = {2011},
	isbn = {978-1-4577-1638-6},
	pages = {63--72},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ASE.2011.6100145},
	doi = {10.1109/ASE.2011.6100145},
	acmid = {2190153},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@PhdThesis{MurphyPhd96,
	title = "{Lightweight structural summarization as an aid to software evolution}",
	author = "Gail C. Murphy",
	school = "University of Washington",
	month = "July",
	year = "1996",
}

@inproceedings{Buse:2008:ADI:1390630.1390664,
	author = {Buse, Raymond P.L. and Weimer, Westley R.},
	title = {Automatic documentation inference for exceptions},
	booktitle = {Proceedings of the 2008 international symposium on Software testing and analysis},
	series = {ISSTA '08},
	year = {2008},
	isbn = {978-1-60558-050-0},
	location = {Seattle, WA, USA},
	pages = {273--282},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1390630.1390664},
	doi = {10.1145/1390630.1390664},
	acmid = {1390664},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation inference, exception handling, software documentation},
}

@inproceedings{Buse:2010:ADP:1858996.1859005,
	author = {Buse, Raymond P.L. and Weimer, Westley R.},
	title = {Automatically documenting program changes},
	booktitle = {Proceedings of the IEEE/ACM international conference on Automated software engineering},
	series = {ASE '10},
	year = {2010},
	isbn = {978-1-4503-0116-9},
	location = {Antwerp, Belgium},
	pages = {33--42},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1858996.1859005},
	doi = {10.1145/1858996.1859005},
	acmid = {1859005},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {code summarization, commit messages, differencing},
}

@ARTICLE{6165314,
	author={Miryung Kim and Notkin, D. and Grossman, D. and Wilson, G.},
	journal={IEEE Transactions on Software Engineering},
	title={Identifying and Summarizing Systematic Code Changes via Rule Inference},
	year={2013},
	month={Jan. },
	volume={39},
	number={1},
	pages={45 -62},
	doi={10.1109/TSE.2012.16},
	ISSN={0098-5589},
}

@inproceedings{Aponte:2011:ITL:1987856.1987867,
	author = {Aponte, Jairo and Marcus, Andrian},
	title = {Improving traceability link recovery methods through software artifact summarization},
	booktitle = {Proceedings of the 6th International Workshop on Traceability in Emerging Forms of Software Engineering},
	series = {TEFSE '11},
	year = {2011},
	isbn = {978-1-4503-0589-1},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {46--49},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1987856.1987867},
	doi = {10.1145/1987856.1987867},
	acmid = {1987867},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {information retrieval, program comprehension, summarization, traceability management},
}

@article{Crosby:1990:WRA:77577.77580,
	author = {Crosby, Martha E. and Stelovsky, Jan},
	title = {How Do We Read Algorithms? A Case Study},
	journal = {Computer},
	issue_date = {January 1990},
	volume = {23},
	number = {1},
	month = jan,
	year = {1990},
	issn = {0018-9162},
	pages = {24--35},
	numpages = {12},
	url = {http://dl.acm.org/citation.cfm?id=77577.77580},
	acmid = {77580},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{Bednarik:2006:EMC:1117309.1117356,
	author = {Bednarik, Roman and Tukiainen, Markku},
	title = {An eye-tracking methodology for characterizing program comprehension processes},
	booktitle = {Proceedings of the 2006 symposium on Eye tracking research \& applications},
	series = {ETRA '06},
	year = {2006},
	isbn = {1-59593-305-0},
	location = {San Diego, California},
	pages = {125--132},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1117309.1117356},
	doi = {10.1145/1117309.1117356},
	acmid = {1117356},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {eye-movement tracking methodology, program comprehension, program visualization, psychology of programming},
} 

@inproceedings{Sharif:2012:ESR:2168556.2168642,
	author = {Sharif, Bonita and Falcone, Michael and Maletic, Jonathan I.},
	title = {An eye-tracking study on the role of scan time in finding source code defects},
	booktitle = {Proceedings of the Symposium on Eye Tracking Research and Applications},
	series = {ETRA '12},
	year = {2012},
	isbn = {978-1-4503-1221-9},
	location = {Santa Barbara, California},
	pages = {381--384},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/2168556.2168642},
	doi = {10.1145/2168556.2168642},
	acmid = {2168642},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {eye-tracking study, software defects, source-code review},
} 

@inproceedings{Sharif:2011:EAU:2117694.2119672,
	author = {Sharif, Bonita},
	title = {Empirical assessment of UML class diagram layouts based on architectural importance},
	booktitle = {Proceedings of the 2011 27th IEEE International Conference on Software Maintenance},
	series = {ICSM '11},
	year = {2011},
	isbn = {978-1-4577-0663-9},
	pages = {544--549},
	numpages = {6},
	url = {http://dx.doi.org/10.1109/ICSM.2011.6080828},
	doi = {10.1109/ICSM.2011.6080828},
	acmid = {2119672},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Sharif:2010:ELD:1796177.1796642,
	author = {Sharif, Bonita and Maletic, Jonathan I.},
	title = {The Effects of Layout on Detecting the Role of Design Patterns},
	booktitle = {Proceedings of the 2010 23rd IEEE Conference on Software Engineering Education and Training},
	series = {CSEET '10},
	year = {2010},
	isbn = {978-0-7695-4054-2},
	pages = {41--48},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/CSEET.2010.23},
	acmid = {1796642},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Binkley:2013:IIS:2436118.2436136,
	author = {Binkley, Dave and Davis, Marcia and Lawrie, Dawn and Maletic, Jonathan I. and Morrell, Christopher and Sharif, Bonita},
	title = {The impact of identifier style on effort and comprehension},
	journal = {Empirical Softw. Engg.},
	issue_date = {April     2013},
	volume = {18},
	number = {2},
	month = apr,
	year = {2013},
	issn = {1382-3256},
	pages = {219--276},
	numpages = {58},
	url = {http://dx.doi.org/10.1007/s10664-012-9201-4},
	doi = {10.1007/s10664-012-9201-4},
	acmid = {2436136},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Code readability, Coding standards, Eye-tracking study, Identifier names, Identifier styles, Memory, Program comprehension, Text recognition},
} 

@inproceedings{Sharif:2010:ETS:1846454.1847968,
	author = {Sharif, Bonita and Maletic, Jonathan I.},
	title = {An Eye Tracking Study on camelCase and under\_score Identifier Styles},
	booktitle = {Proceedings of the 2010 IEEE 18th International Conference on Program Comprehension},
	series = {ICPC '10},
	year = {2010},
	isbn = {978-0-7695-4113-6},
	pages = {196--205},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICPC.2010.41},
	doi = {10.1109/ICPC.2010.41},
	acmid = {1847968},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {identifier styles, eye-tracking study, code readability},
} 

@inproceedings{Bednarik:2008:TED:1344471.1344497,
	author = {Bednarik, Roman and Tukiainen, Markku},
	title = {Temporal eye-tracking data: evolution of debugging strategies with multiple representations},
	booktitle = {Proceedings of the 2008 symposium on Eye tracking research \&\#38; applications},
	series = {ETRA '08},
	year = {2008},
	isbn = {978-1-59593-982-1},
	location = {Savannah, Georgia},
	pages = {99--102},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1344471.1344497},
	doi = {10.1145/1344471.1344497},
	acmid = {1344497},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Uwano:2006:AIP:1117309.1117357,
	author = {Uwano, Hidetake and Nakamura, Masahide and Monden, Akito and Matsumoto, Ken-ichi},
	title = {Analyzing individual performance of source code review using reviewers' eye movement},
	booktitle = {Proceedings of the 2006 symposium on Eye tracking research \& applications},
	series = {ETRA '06},
	year = {2006},
	isbn = {1-59593-305-0},
	location = {San Diego, California},
	pages = {133--140},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1117309.1117357},
	doi = {10.1145/1117309.1117357},
	acmid = {1117357},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {computer program, eye movement, human factor, source code review},
} 

@inproceedings{LaToza:2006:MMM:1134285.1134355,
	author = {LaToza, Thomas D. and Venolia, Gina and DeLine, Robert},
	title = {Maintaining mental models: a study of developer work habits},
	booktitle = {Proceedings of the 28th international conference on Software engineering},
	series = {ICSE '06},
	year = {2006},
	isbn = {1-59593-375-1},
	location = {Shanghai, China},
	pages = {492--501},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1134285.1134355},
	doi = {10.1145/1134285.1134355},
	acmid = {1134355},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {agile software development, code duplication, code ownership, communication, debugging, interruptions},
}

@inproceedings{Guzzi:2012:DSK:2337223.2337476,
	author = {Guzzi, Anja},
	title = {Documenting and sharing knowledge about code},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {1535--1538},
	numpages = {4},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337476},
	acmid = {2337476},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@inproceedings{Brandt:2010:EPI:1753326.1753402,
	author = {Brandt, Joel and Dontcheva, Mira and Weskamp, Marcos and Klemmer, Scott R.},
	title = {Example-centric programming: integrating web search into the development environment},
	booktitle = {Proceedings of the 28th international conference on Human factors in computing systems},
	series = {CHI '10},
	year = {2010},
	isbn = {978-1-60558-929-9},
	location = {Atlanta, Georgia, USA},
	pages = {513--522},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1753326.1753402},
	doi = {10.1145/1753326.1753402},
	acmid = {1753402},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {example-centric development},
}

@inproceedings{Kotonya:2008:ORL:1478087.1478113,
	author = {Kotonya, Gerald and Lock, Simon and Mariani, John},
	title = {Opportunistic Reuse: Lessons from Scrapheap Software Development},
	booktitle = {Proceedings of the 11th International Symposium on Component-Based Software Engineering},
	series = {CBSE '08},
	year = {2008},
	isbn = {978-3-540-87890-2},
	location = {Karlsruhe, Germany},
	pages = {302--309},
	numpages = {8},
	url = {http://dx.doi.org/10.1007/978-3-540-87891-9_20},
	doi = {10.1007/978-3-540-87891-9_20},
	acmid = {1478113},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
}

@ARTICLE{Davison00understandingand,
	author = {Joseph W. Davison and Dennis M. Mancl and William F. Opdyke},
	title = {Understanding and addressing the essential costs of evolving systems},
	journal = {Bell Labs Technical Journal},
	year = {2000},
	pages = {44--54}
}

@inproceedings{Mirghasemi:2011:QMB:2025113.2025184,
	author = {Mirghasemi, Salman and Barton, John J. and Petitpierre, Claude},
	title = {Querypoint: moving backwards on wrong values in the buggy execution},
	booktitle = {Proceedings of the 19th ACM SIGSOFT symposium and the 13th European conference on Foundations of software engineering},
	series = {ESEC/FSE '11},
	year = {2011},
	isbn = {978-1-4503-0443-6},
	location = {Szeged, Hungary},
	pages = {436--439},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/2025113.2025184},
	doi = {10.1145/2025113.2025184},
	acmid = {2025184},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {breakpoint, debugging, lastchange, locating defects, logging, querypoint, watchpoint},
}

@article{Douce91,
	author = {Douce, C.},
	title = {Long Term Comprehension of Software Systems: A Methodology for Study},
	journal = {Proc. Psychology of Programming Interest Group},
	year = {2001}
}

@inproceedings{Gonzalez:2004:CCM:985692.985707,
	author = {Gonz\'{a}lez, Victor M. and Mark, Gloria},
	title = {"Constant, constant, multi-tasking craziness": managing multiple working spheres},
	booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
	series = {CHI '04},
	year = {2004},
	isbn = {1-58113-702-8},
	location = {Vienna, Austria},
	pages = {113--120},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/985692.985707},
	doi = {10.1145/985692.985707},
	acmid = {985707},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {attention management, empirical study, information overload, interruptions, personal information management},
} 

@inproceedings{Kramer:2012:BLA:2337223.2337451,
	author = {Kr\"{a}mer, Jan-Peter and Kurz, Joachim and Karrer, Thorsten and Borchers, Jan},
	title = {Blaze},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {1457--1458},
	numpages = {2},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337451},
	acmid = {2337451},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@article{ALTMANN2001189,
	title = "Near-term memory in programming: a simulation-based analysis ",
	journal = "International Journal of Human-Computer Studies ",
	volume = "54",
	number = "2",
	pages = "189 - 210",
	year = "2001",
	note = "",
	issn = "1071-5819",
	doi = "http://dx.doi.org/10.1006/ijhc.2000.0407",
	url = "http://www.sciencedirect.com/science/article/pii/S1071581900904075",
	author = "Erik M. Altmann"
}

@inproceedings{Borodin:2010:MME:1805986.1806005,
	author = {Borodin, Yevgen and Bigham, Jeffrey P. and Dausch, Glenn and Ramakrishnan, I. V.},
	title = {More Than Meets the Eye: A Survey of Screen-reader Browsing Strategies},
	booktitle = {Proceedings of the 2010 International Cross Disciplinary Conference on Web Accessibility (W4A)},
	series = {W4A '10},
	year = {2010},
	isbn = {978-1-4503-0045-2},
	location = {Raleigh, North Carolina},
	pages = {13:1--13:10},
	articleno = {13},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1805986.1806005},
	doi = {10.1145/1805986.1806005},
	acmid = {1806005},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {accessibility, blind, browsing strategy, screen reader, usability},
} 

@article{Holmes:2013:SPS:2377656.2377657,
	author = {Holmes, Reid and Walker, Robert J.},
	title = {Systematizing pragmatic software reuse},
	journal = {ACM Trans. Softw. Eng. Methodol.},
	issue_date = {November 2012},
	volume = {21},
	number = {4},
	month = feb,
	year = {2013},
	issn = {1049-331X},
	pages = {20:1--20:44},
	articleno = {20},
	numpages = {44},
	url = {http://doi.acm.org/10.1145/2377656.2377657},
	doi = {10.1145/2377656.2377657},
	acmid = {2377657},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Gilligan, Software reuse, lightweight process and tooling, low commitment, planning, pragmatic software reuse, pragmatic-reuse plan enactment, pragmatic-reuse plans, source code investigation, white box reuse},
}

@article{Littman1987341,
	title = "Mental models and software maintenance ",
	journal = "Journal of Systems and Software ",
	volume = "7",
	number = "4",
	pages = "341 - 355",
	year = "1987",
	note = "",
	issn = "0164-1212",
	doi = "http://dx.doi.org/10.1016/0164-1212(87)90033-1",
	url = "http://www.sciencedirect.com/science/article/pii/0164121287900331",
	author = "David C. Littman and Jeannine Pinto and Stanley Letovsky and Elliot Soloway"
}

@article{Ko200541,
	title = "A framework and methodology for studying the causes of software errors in programming systems ",
	journal = "Journal of Visual Languages and Computing ",
	volume = "16",
	number = "1–2",
	pages = "41 - 84",
	year = "2005",
	issn = "1045-926X",
	doi = "http://dx.doi.org/10.1016/j.jvlc.2004.08.003",
	url = "http://www.sciencedirect.com/science/article/pii/S1045926X04000394",
	author = "Andrew J. Ko and Brad A. Myers"
}

@inproceedings{Dearman:2005:ACV:1058432.1059367,
	author = {Dearman, David and Cox, Anthony and Fisher, Maryanne},
	title = {Adding Control-Flow to a Visual Data-Flow Representation},
	booktitle = {Proceedings of the 13th International Workshop on Program Comprehension},
	series = {IWPC '05},
	year = {2005},
	isbn = {0-7695-2254-8},
	pages = {297--306},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/WPC.2005.5},
	doi = {10.1109/WPC.2005.5},
	acmid = {1059367},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Eddy:2013:ICPC,
	author = {Eddy, Brian and Robinson, Jeffrey and Kraft, Nicholas and Carver, Jeffrey},
	title = {Evaluating Source Code Summarization Techniques: Replication and Expansion},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	year = {2013},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@article{Freeman:2003:RDF:903893.903930,
	author = {Freeman, Lee A.},
	title = {A refresher in data flow diagramming: an effective aid for analysts},
	journal = {Commun. ACM},
	issue_date = {September 2003},
	volume = {46},
	number = {9},
	month = sep,
	year = {2003},
	issn = {0001-0782},
	pages = {147--151},
	numpages = {5},
	url = {http://doi.acm.org/10.1145/903893.903930},
	doi = {10.1145/903893.903930},
	acmid = {903930},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@incollection{Anderson:1992,
	year={1992},
	isbn={978-3-540-55606-0},
	booktitle={Intelligent Tutoring Systems},
	volume={608},
	series={Lecture Notes in Computer Science},
	editor={Frasson, Claude and Gauthier, Gilles and McCalla, GordonI.},
	doi={10.1007/3-540-55606-0_68},
	title={The advantages of data flow diagrams for beginning programming},
	url={http://dx.doi.org/10.1007/3-540-55606-0_68},
	publisher={Springer Berlin Heidelberg},
	author={Anjaneyulu, K.S.R. and Anderson, JohnR.},
	pages={585-592}
}

@article{Ko:2006:ESD:1248728.1248780,
	author = {Ko, Andrew J. and Myers, Brad A. and Coblenz, Michael J. and Aung, Htet Htet},
	title = {An Exploratory Study of How Developers Seek, Relate, and Collect Relevant Information during Software Maintenance Tasks},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {December 2006},
	volume = {32},
	number = {12},
	month = dec,
	year = {2006},
	issn = {0098-5589},
	pages = {971--987},
	numpages = {17},
	url = {http://dx.doi.org/10.1109/TSE.2006.116},
	doi = {10.1109/TSE.2006.116},
	acmid = {1248780},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Program investigation, Program investigation, program understanding, program comprehension, empirical software engineering, information foraging, information scent., empirical software engineering, information foraging, information scent., program comprehension, program understanding},
}

@inproceedings{Singer:1997:ESE:782010.782031,
	author = {Singer, Janice and Lethbridge, Timothy and Vinson, Norman and Anquetil, Nicolas},
	title = {An examination of software engineering work practices},
	booktitle = {Proceedings of the 1997 conference of the Centre for Advanced Studies on Collaborative research},
	series = {CASCON '97},
	year = {1997},
	location = {Toronto, Ontario, Canada},
	pages = {21--},
	url = {http://dl.acm.org/citation.cfm?id=782010.782031},
	acmid = {782031},
	publisher = {IBM Press},
}

@article{Lakhotia:1993:USE:177728.177735,
	author = {Lakhotia, Arun},
	title = {Understanding someone else's code: analysis of experiences},
	journal = {J. Syst. Softw.},
	issue_date = {Dec. 1993},
	volume = {23},
	number = {3},
	month = dec,
	year = {1993},
	issn = {0164-1212},
	pages = {269--275},
	numpages = {7},
	url = {http://dx.doi.org/10.1016/0164-1212(93)90101-3},
	doi = {10.1016/0164-1212(93)90101-3},
	acmid = {177735},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
}

@inproceedings{fjeldstadt83,
	author = {Fjeldstad, R. K. and Hamlen, W. T.},
	booktitle = {Proceedings GUIDE 48},
	citeulike-article-id = {6922207},
	keywords = {maintenance},
	location = {Philadelphia, PA},
	month = apr,
	posted-at = {2010-03-27 23:13:35},
	priority = {2},
	title = {{Application Program Maintenance Study: Report to Our Respondents}},
	year = {1983}
}

@inproceedings{Roehm:2012:PDC:2337223.2337254,
	author = {Roehm, Tobias and Tiarks, Rebecca and Koschke, Rainer and Maalej, Walid},
	title = {How do professional developers comprehend software?},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {255--265},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337254},
	acmid = {2337254},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@inproceedings{Stylos:2006:MWT:1174509.1174678,
	author = {Stylos, Jeffrey and Myers, Brad A.},
	title = {Mica: A Web-Search Tool for Finding API Components and Examples},
	booktitle = {Proceedings of the Visual Languages and Human-Centric Computing},
	series = {VLHCC '06},
	year = {2006},
	isbn = {0-7695-2586-5},
	pages = {195--202},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/VLHCC.2006.32},
	doi = {10.1109/VLHCC.2006.32},
	acmid = {1174678},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@ARTICLE{1241364,
	author={Lethbridge, T.C. and Singer, J. and Forward, A.},
	journal={Software, IEEE},
	title={How software engineers use documentation: the state of the practice},
	year={2003},
	volume={20},
	number={6},
	pages={35-39},
	keywords={software engineering;system documentation;decision making;documentation update;documentation use;software engineering;software engineers;software process managers;software process personnel;tool design;Data engineering;Documentation;Humans;Maintenance engineering;Power engineering and energy;Software engineering;Software maintenance;Software systems;Software testing;System testing},
	doi={10.1109/MS.2003.1241364},
	ISSN={0740-7459}
}

@inproceedings{Forward:2002:RSD:585058.585065,
	author = {Forward, Andrew and Lethbridge, Timothy C.},
	title = {The relevance of software documentation, tools and technologies: a survey},
	booktitle = {Proceedings of the 2002 ACM symposium on Document engineering},
	series = {DocEng '02},
	year = {2002},
	isbn = {1-58113-594-7},
	location = {McLean, Virginia, USA},
	pages = {26--33},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/585058.585065},
	doi = {10.1145/585058.585065},
	acmid = {585065},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation relevance, documentation survey, documentation technologies, program comprehension, software documentation, software engineering, software maintenance},
} 

@inproceedings{Gweon:2007:EAT:1308174.1308329,
	author = {Gweon, G. and Bergman, L. and Castelli, V. and Bellamy, R. K. E.},
	title = {Evaluating an Automated Tool to Assist Evolutionary Document Generation},
	booktitle = {Proceedings of the IEEE Symposium on Visual Languages and Human-Centric Computing},
	series = {VLHCC '07},
	year = {2007},
	isbn = {0-7695-2987-9},
	pages = {243--248},
	numpages = {6},
	url = {http://dx.doi.org/10.1109/VLHCC.2007.20},
	doi = {10.1109/VLHCC.2007.20},
	acmid = {1308329},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Bergman:2005:DSA:1095034.1095067,
	author = {Bergman, Lawrence and Castelli, Vittorio and Lau, Tessa and Oblinger, Daniel},
	title = {DocWizards: a system for authoring follow-me documentation wizards},
	booktitle = {Proceedings of the 18th annual ACM symposium on User interface software and technology},
	series = {UIST '05},
	year = {2005},
	isbn = {1-59593-271-2},
	location = {Seattle, WA, USA},
	pages = {191--200},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1095034.1095067},
	doi = {10.1145/1095034.1095067},
	acmid = {1095067},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation generation, programming-by-demonstration},
} 

@inproceedings{5306335,
	author={Starke, J. and Luce, C. and Sillito, J.},
	booktitle={Software Maintenance, 2009. ICSM 2009. IEEE International Conference on},
	title={Searching and skimming: An exploratory study},
	year={2009},
	pages={157-166},
	keywords={software engineering;program comprehension;software system;source code search tools;Concrete;Data analysis;Information analysis;Java;Laboratories;Navigation;Programming profession;Software design;Software systems;Software tools},
	doi={10.1109/ICSM.2009.5306335},
	ISSN={1063-6773}
}

@inproceedings{Kramer:1999:ADS:318372.318577,
	author = {Kramer, Douglas},
	title = {API documentation from source code comments: a case study of Javadoc},
	booktitle = {Proceedings of the 17th annual international conference on Computer documentation},
	series = {SIGDOC '99},
	year = {1999},
	isbn = {1-58113-072-4},
	location = {New Orleans, Louisiana, USA},
	pages = {147--153},
	numpages = {7},
	url = {http://doi.acm.org/10.1145/318372.318577},
	doi = {10.1145/318372.318577},
	acmid = {318577},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {API documentation, Java platform, Javadoc, doc comments, doclets, documentation comments, generated documentation, source code comments},
} 

@inproceedings{deSouza:2005:SDE:1085313.1085331,
	author = {de Souza, Sergio Cozzetti B. and Anquetil, Nicolas and de Oliveira, K\'{a}thia M.},
	title = {A study of the documentation essential to software maintenance},
	booktitle = {Proceedings of the 23rd annual international conference on Design of communication: documenting \& designing for pervasive information},
	series = {SIGDOC '05},
	year = {2005},
	isbn = {1-59593-175-9},
	location = {Coventry, United Kingdom},
	pages = {68--75},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1085313.1085331},
	doi = {10.1145/1085313.1085331},
	acmid = {1085331},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {empirical study, program understanding, software maintenance, software system documentation},
}

@article{Kajko-Mattsson:2005:SDP:1032622.1035374,
	author = {Kajko-Mattsson, Mira},
	title = {A Survey of Documentation Practice within Corrective Maintenance},
	journal = {Empirical Softw. Engg.},
	issue_date = {January 2005},
	volume = {10},
	number = {1},
	month = jan,
	year = {2005},
	issn = {1382-3256},
	pages = {31--55},
	numpages = {25},
	url = {http://dx.doi.org/10.1023/B:LIDA.0000048322.42751.ca},
	doi = {10.1023/B:LIDA.0000048322.42751.ca},
	acmid = {1035374},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Corrective maintenance, software process documentation, software system documentation},
}

@inproceedings{Fluri:2007:CCC:1339262.1339530,
	author = {Fluri, Beat and Wursch, Michael and Gall, Harald C.},
	title = {Do Code and Comments Co-Evolve? On the Relation between Source Code and Comment Changes},
	booktitle = {Proceedings of the 14th Working Conference on Reverse Engineering},
	series = {WCRE '07},
	year = {2007},
	isbn = {0-7695-3034-6},
	pages = {70--79},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/WCRE.2007.21},
	doi = {10.1109/WCRE.2007.21},
	acmid = {1339530},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Ibrahim:2012:CCR:2330373.2330435,
	author = {Ibrahim, Walid M. and Bettenburg, Nicolas and Adams, Bram and Hassan, Ahmed E.},
	title = {Controversy Corner: On the relationship between comment update practices and Software Bugs},
	journal = {J. Syst. Softw.},
	issue_date = {October, 2012},
	volume = {85},
	number = {10},
	month = oct,
	year = {2012},
	issn = {0164-1212},
	pages = {2293--2304},
	numpages = {12},
	url = {http://dx.doi.org/10.1016/j.jss.2011.09.019},
	doi = {10.1016/j.jss.2011.09.019},
	acmid = {2330435},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {Code quality, Empirical studies, Software bugs, Software evolution, Source code comments},
}

@inproceedings{Sim:1998:ASC:580914.858229,
	author = {Sim, S. E. and Clarke, C. L. A. and Holt, R. C.},
	title = {Archetypal Source Code Searches: A Survey of Software Developers and Maintainers},
	booktitle = {Proceedings of the 6th International Workshop on Program Comprehension},
	series = {IWPC '98},
	year = {1998},
	isbn = {0-8186-8560-3},
	pages = {180--},
	url = {http://dl.acm.org/citation.cfm?id=580914.858229},
	acmid = {858229},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Sillito:2008:AAQ:1446226.1446241,
	author = {Sillito, Jonathan and Murphy, Gail C. and De Volder, Kris},
	title = {Asking and Answering Questions during a Programming Change Task},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {July 2008},
	volume = {34},
	number = {4},
	month = jul,
	year = {2008},
	issn = {0098-5589},
	pages = {434--451},
	numpages = {18},
	url = {http://dx.doi.org/10.1109/TSE.2008.26},
	doi = {10.1109/TSE.2008.26},
	acmid = {1446241},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Enhancement, Programming Environments/Construction Tools, Software psychology, Software psychology, Programming Environments/Construction Tools, Enhancement},
} 

@inproceedings{Burden:2011:NLG:2095654.2095665,
	author = {Burden, H{\aa}kan and Heldal, Rogardt},
	title = {Natural language generation from class diagrams},
	booktitle = {Proceedings of the 8th International Workshop on Model-Driven Engineering, Verification and Validation},
	series = {MoDeVVa},
	year = {2011},
	isbn = {978-1-4503-0914-1},
	location = {Wellington, New Zealand},
	pages = {8:1--8:8},
	articleno = {8},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/2095654.2095665},
	doi = {10.1145/2095654.2095665},
	acmid = {2095665},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {model transformations, model-driven architecture},
} 

@inproceedings{Mani:2012:AAU:2393596.2393607,
	author = {Mani, Senthil and Catherine, Rose and Sinha, Vibha Singhal and Dubey, Avinava},
	title = {AUSUM: approach for unsupervised bug report summarization},
	booktitle = {Proceedings of the ACM SIGSOFT 20th International Symposium on the Foundations of Software Engineering},
	series = {FSE '12},
	year = {2012},
	isbn = {978-1-4503-1614-9},
	location = {Cary, North Carolina},
	pages = {11:1--11:11},
	articleno = {11},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2393596.2393607},
	doi = {10.1145/2393596.2393607},
	acmid = {2393607},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug report, summarization, unsupervised},
} 

@inproceedings{Moreno:2013:ICPC,
	author = {Moreno, Laura and Aponte, Jairo and Sridhara Giriprasad and Marcus, Andrian and Pollock, Lori and Vijay-Shanker, K.},
	title = {Automatic Generation of Natural Language Summaries for Java Classes},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	year = {2013},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@inproceedings{Sridhara:2011:ADD:1985793.1985808,
	author = {Sridhara, Giriprasad and Pollock, Lori and Vijay-Shanker, K.},
	title = {Automatically detecting and describing high level actions within methods},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {101--110},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985808},
	doi = {10.1145/1985793.1985808},
	acmid = {1985808},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation, program comprehension},
}

@inproceedings{Sridhara:2010:TAG:1858996.1859006,
	author = {Sridhara, Giriprasad and Hill, Emily and Muppaneni, Divya and Pollock, Lori and Vijay-Shanker, K.},
	title = {Towards automatically generating summary comments for Java methods},
	booktitle = {Proceedings of the IEEE/ACM international conference on Automated software engineering},
	series = {ASE '10},
	year = {2010},
	isbn = {978-1-4503-0116-9},
	location = {Antwerp, Belgium},
	pages = {43--52},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1858996.1859006},
	doi = {10.1145/1858996.1859006},
	acmid = {1859006},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {comment generation, method summarization, natural language program analysis},
} 

@inproceedings{Zhong:2009:IRS:1747491.1747528,
	author = {Zhong, Hao and Zhang, Lu and Xie, Tao and Mei, Hong},
	title = {Inferring Resource Specifications from Natural Language API Documentation},
	booktitle = {Proceedings of the 2009 IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '09},
	year = {2009},
	isbn = {978-0-7695-3891-4},
	pages = {307--318},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/ASE.2009.94},
	doi = {10.1109/ASE.2009.94},
	acmid = {1747528},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}



@inproceedings{McMillan:2011:PFR:1985793.1985809,
	author = {McMillan, Collin and Grechanik, Mark and Poshyvanyk, Denys and Xie, Qing and Fu, Chen},
	title = {Portfolio: finding relevant functions and their usage},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {111--120},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985809},
	doi = {10.1145/1985793.1985809},
	acmid = {1985809},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {code search, function call graph, pagerank, portfolio, ranking},
} 

@PhdThesis{SridharaPhd12,
	title = "{Automatic Generation of Descriptive Summary Comments for Methods in Object-oriented Programs}",
	author = "Giriprasad Sridhara",
	school = "University of Delaware",
	month = Jan,
	year = "2012",
}

@inproceedings{Sridhara:2011:GPC:2057176.2057211,
	author = {Sridhara, Giriprasad and Pollock, Lori and Vijay-Shanker, K.},
	title = {Generating Parameter Comments and Integrating with Method Summaries},
	booktitle = {Proceedings of the 2011 IEEE 19th International Conference on Program Comprehension},
	series = {ICPC '11},
	year = {2011},
	isbn = {978-0-7695-4398-7},
	pages = {71--80},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICPC.2011.28},
	doi = {10.1109/ICPC.2011.28},
	acmid = {2057211},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {documentation, software maintenance},
}

@article{Lininger:2008:UCB:1409763.1409808,
	author = {Lininger, Joseph},
	title = {Use of Computers by Blind Computer Science Students},
	journal = {J. Comput. Sci. Coll.},
	issue_date = {October 2008},
	volume = {24},
	number = {1},
	month = oct,
	year = {2008},
	issn = {1937-4771},
	pages = {182--187},
	numpages = {6},
	url = {http://dl.acm.org/citation.cfm?id=1409763.1409808},
	acmid = {1409808},
	publisher = {Consortium for Computing Sciences in Colleges},
	address = {USA},
}

@inproceedings{Haiduc:2010:UAT:1919284.1919577,
	author = {Haiduc, Sonia and Aponte, Jairo and Moreno, Laura and Marcus, Andrian},
	title = {On the Use of Automated Text Summarization Techniques for Summarizing Source Code},
	booktitle = {Proceedings of the 2010 17th Working Conference on Reverse Engineering},
	series = {WCRE '10},
	year = {2010},
	isbn = {978-0-7695-4123-5},
	pages = {35--44},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/WCRE.2010.13},
	doi = {10.1109/WCRE.2010.13},
	acmid = {1919577},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {text summarization, program comprehension},
}

@article{Herbsleb:2003:ESS:1435631.859041,
	author = {Herbsleb, James D. and Mockus, Audris},
	title = {An Empirical Study of Speed and Communication in Globally Distributed Software Development},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {June 2003},
	volume = {29},
	number = {6},
	month = jun,
	year = {2003},
	issn = {0098-5589},
	pages = {481--494},
	numpages = {14},
	url = {http://dx.doi.org/10.1109/TSE.2003.1205177},
	doi = {10.1109/TSE.2003.1205177},
	acmid = {859041},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Global development, collaboration, delay, speed, awareness, informal communication.},
}

@inproceedings{Aranda:2009:SLB:1555001.1555045,
	author = {Aranda, Jorge and Venolia, Gina},
	title = {The secret life of bugs: Going past the errors and omissions in software repositories},
	booktitle = {Proceedings of the 31st International Conference on Software Engineering},
	series = {ICSE '09},
	year = {2009},
	isbn = {978-1-4244-3453-4},
	pages = {298--308},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2009.5070530},
	doi = {10.1109/ICSE.2009.5070530},
	acmid = {1555045},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Cataldo:2006:ICR:1180875.1180929,
	author = {Cataldo, Marcelo and Wagstrom, Patrick A. and Herbsleb, James D. and Carley, Kathleen M.},
	title = {Identification of coordination requirements: implications for the Design of collaboration and awareness tools},
	booktitle = {Proceedings of the 2006 20th anniversary conference on Computer supported cooperative work},
	series = {CSCW '06},
	year = {2006},
	isbn = {1-59593-249-6},
	location = {Banff, Alberta, Canada},
	pages = {353--362},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1180875.1180929},
	doi = {10.1145/1180875.1180929},
	acmid = {1180929},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {collaboration tools, coordination, dynamic network analysis, task awareness tools},
}

@article{Curtis:1988:FSS:50087.50089,
	author = {Curtis, Bill and Krasner, Herb and Iscoe, Neil},
	title = {A field study of the software design process for large systems},
	journal = {Commun. ACM},
	issue_date = {Nov. 1988},
	volume = {31},
	number = {11},
	month = nov,
	year = {1988},
	issn = {0001-0782},
	pages = {1268--1287},
	numpages = {20},
	url = {http://doi.acm.org/10.1145/50087.50089},
	doi = {10.1145/50087.50089},
	acmid = {50089},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{deSouza:2008:ESS:1368088.1368122,
	author = {de Souza, Cleidson R. B. and Redmiles, David F.},
	title = {An empirical study of software developers' management of dependencies and changes},
	booktitle = {Proceedings of the 30th international conference on Software engineering},
	series = {ICSE '08},
	year = {2008},
	isbn = {978-1-60558-079-1},
	location = {Leipzig, Germany},
	pages = {241--250},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1368088.1368122},
	doi = {10.1145/1368088.1368122},
	acmid = {1368122},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {change impact analysis, collaborative software development, empirical studies, socio-technical aspects},
} 

@inproceedings{Leszak:2000:CSR:337180.337232,
	author = {Leszak, Marek and Perry, Dewayne E. and Stoll, Dieter},
	title = {A case study in root cause defect analysis},
	booktitle = {Proceedings of the 22nd international conference on Software engineering},
	series = {ICSE '00},
	year = {2000},
	isbn = {1-58113-206-9},
	location = {Limerick, Ireland},
	pages = {428--437},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/337180.337232},
	doi = {10.1145/337180.337232},
	acmid = {337232},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {defect prevention, modification management, process improvement, quality assurance, root cause analyis},
} 

@article {BLTJ:BLTJ2101,
	author = {Yu, Weider D.},
	title = {A software fault prevention approach in coding and root cause analysis},
	journal = {Bell Labs Technical Journal},
	volume = {3},
	number = {2},
	publisher = {Wiley Subscription Services, Inc., A Wiley Company},
	issn = {1538-7305},
	url = {http://dx.doi.org/10.1002/bltj.2101},
	doi = {10.1002/bltj.2101},
	pages = {3--21},
	year = {1998},
}

@inproceedings{Valetto:2007:USR:1268983.1269039,
	author = {Valetto, Giuseppe and Helander, Mary and Ehrlich, Kate and Chulani, Sunita and Wegman, Mark and Williams, Clay},
	title = {Using Software Repositories to Investigate Socio-technical Congruence in Development Projects},
	booktitle = {Proceedings of the Fourth International Workshop on Mining Software Repositories},
	series = {MSR '07},
	year = {2007},
	isbn = {0-7695-2950-X},
	pages = {25--},
	url = {http://dx.doi.org/10.1109/MSR.2007.33},
	doi = {10.1109/MSR.2007.33},
	acmid = {1269039},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{dell2012yours,
	title={Yours is better!: participant response bias in HCI},
	author={Dell, Nicola and Vaidyanathan, Vidya and Medhi, Indrani and Cutrell, Edward and Thies, William},
	booktitle={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
	pages={1321--1330},
	year={2012},
	organization={ACM}
}

@inproceedings{Bugde:2008:GSS:1471606.1472247,
	author = {Bugde, Shilpa and Nagappan, Nachiappan and Rajamani, Sriram and Ramalingam, G.},
	title = {Global Software Servicing: Observational Experiences at Microsoft},
	booktitle = {Proceedings of the 2008 IEEE International Conference on Global Software Engineering},
	series = {ICGSE '08},
	year = {2008},
	isbn = {978-0-7695-3280-6},
	pages = {182--191},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICGSE.2008.18},
	doi = {10.1109/ICGSE.2008.18},
	acmid = {1472247},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Ashok:2009:DRS:1595696.1595766,
	author = {Ashok, B. and Joy, Joseph and Liang, Hongkang and Rajamani, Sriram K. and Srinivasa, Gopal and Vangala, Vipindeep},
	title = {DebugAdvisor: a recommender system for debugging},
	booktitle = {Proceedings of the the 7th joint meeting of the European software engineering conference and the ACM SIGSOFT symposium on The foundations of software engineering},
	series = {ESEC/FSE '09},
	year = {2009},
	isbn = {978-1-60558-001-2},
	location = {Amsterdam, The Netherlands},
	pages = {373--382},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1595696.1595766},
	doi = {10.1145/1595696.1595766},
	acmid = {1595766},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, recommendation systems, search},
}

@techreport{NIST_bugs_cost:2002,
	author = {Tassey, Gregory},
	title = {The Economic Impacts of Inadequate Infrastructure for Software Testing},
	institution = {National Institute of Standards \& Technology},
	month = {May},
	year = {2002}
}

@inproceedings{Weiss:2007:LTF:1268983.1269017,
	author = {Weiss, Cathrin and Premraj, Rahul and Zimmermann, Thomas and Zeller, Andreas},
	title = {How Long Will It Take to Fix This Bug?},
	booktitle = {Proceedings of the Fourth International Workshop on Mining Software Repositories},
	series = {MSR '07},
	year = {2007},
	isbn = {0-7695-2950-X},
	pages = {1--},
	url = {http://dx.doi.org/10.1109/MSR.2007.13},
	doi = {10.1109/MSR.2007.13},
	acmid = {1269017},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Guo:2010:CPB:1806799.1806871,
	author = {Guo, Philip J. and Zimmermann, Thomas and Nagappan, Nachiappan and Murphy, Brendan},
	title = {Characterizing and predicting which bugs get fixed: an empirical study of Microsoft Windows},
	booktitle = {Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering - Volume 1},
	series = {ICSE '10},
	year = {2010},
	isbn = {978-1-60558-719-6},
	location = {Cape Town, South Africa},
	pages = {495--504},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1806799.1806871},
	doi = {10.1145/1806799.1806871},
	acmid = {1806871},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Bettenburg:2007:QBR:1328279.1328284,
	author = {Bettenburg, Nicolas and Just, Sascha and Schr\"{o}ter, Adrian and Wei\ss, Cathrin and Premraj, Rahul and Zimmermann, Thomas},
	title = {Quality of bug reports in Eclipse},
	booktitle = {Proceedings of the 2007 OOPSLA workshop on eclipse technology eXchange},
	series = {eclipse '07},
	year = {2007},
	isbn = {978-1-60558-015-9},
	location = {Montreal, Quebec, Canada},
	pages = {21--25},
	numpages = {5},
	url = {http://doi.acm.org/10.1145/1328279.1328284},
	doi = {10.1145/1328279.1328284},
	acmid = {1328284},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@article{Treude:2012:WIT:2122269.2122542,
	author = {Treude, Christoph and Storey, Margaret-Anne},
	title = {Work Item Tagging: Communicating Concerns in Collaborative Software Development},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {January 2012},
	volume = {38},
	number = {1},
	month = jan,
	year = {2012},
	issn = {0098-5589},
	pages = {19--34},
	numpages = {16},
	url = {http://dx.doi.org/10.1109/TSE.2010.91},
	doi = {10.1109/TSE.2010.91},
	acmid = {2122542},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Tagging, collaboration, software development, task management, articulation work, work items.},
} 

@inproceedings{Bettenburg:2008:4658082,
	author={Bettenburg, N. and Premraj, R. and Zimmermann, T. and Sunghun Kim},
	booktitle={Software Maintenance, 2008. ICSM 2008. IEEE International Conference on},
	title={Duplicate bug reports considered harmful ... really?},
	year={2008},
	month={28 2008-oct. 4},
	volume={},
	number={},
	pages={337 -345},
	keywords={duplicate bug;open source projects;software maintenance;program debugging;public domain software;software maintenance;},
	doi={10.1109/ICSM.2008.4658082},
	ISSN={1063-6773}
}

@inproceedings{Bettenburg:2008:MGB:1453101.1453146,
	author = {Bettenburg, Nicolas and Just, Sascha and Schr\"{o}ter, Adrian and Wei\ss, Cathrin and Premraj, Rahul and Zimmermann, Thomas},
	title = {What makes a good bug report?},
	booktitle = {Proceedings of the 16th ACM SIGSOFT International Symposium on Foundations of software engineering},
	series = {SIGSOFT '08/FSE-16},
	year = {2008},
	isbn = {978-1-59593-995-1},
	location = {Atlanta, Georgia},
	pages = {308--318},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1453101.1453146},
	doi = {10.1145/1453101.1453146},
	acmid = {1453146},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Herbsleb:2001:GEI:624642.626244,
	author = {Herbsleb, James D. and Moitra, Deependra},
	title = {Guest Editors' Introduction: Global Software Development},
	journal = {IEEE Softw.},
	issue_date = {March 2001},
	volume = {18},
	number = {2},
	month = mar,
	year = {2001},
	issn = {0740-7459},
	pages = {16--20},
	numpages = {5},
	url = {http://dx.doi.org/10.1109/52.914732},
	doi = {10.1109/52.914732},
	acmid = {626244},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
}

@article{Grinter:1996:SAW:259640.259651,
	author = {Grinter, Rebecca E.},
	title = {Supporting articulation work using software configuration management systems},
	journal = {Comput. Supported Coop. Work},
	issue_date = {1996},
	volume = {5},
	number = {4},
	month = dec,
	year = {1996},
	issn = {0925-9724},
	pages = {447--465},
	numpages = {19},
	url = {http://dx.doi.org/10.1007/BF00136714},
	doi = {10.1007/BF00136714},
	acmid = {259651},
	publisher = {Kluwer Academic Publishers},
	address = {Norwell, MA, USA},
	keywords = {articulation work, computer-supported cooperated work, configuration management, coordination mechanisms, empirical studies},
} 

@inproceedings{Storey:2008:TBE:1368088.1368123,
	author = {Storey, Margaret-Anne and Ryall, Jody and Bull, R. Ian and Myers, Del and Singer, Janice},
	title = {TODO or to bug: exploring how task annotations play a role in the work practices of software developers},
	booktitle = {Proceedings of the 30th international conference on Software engineering},
	series = {ICSE '08},
	year = {2008},
	isbn = {978-1-60558-079-1},
	location = {Leipzig, Germany},
	pages = {251--260},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1368088.1368123},
	doi = {10.1145/1368088.1368123},
	acmid = {1368123},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {source code comments, task annotations, work practices},
}

@inproceedings{Ko:2006:LAP:1174509.1174667,
	author = {Ko, Andrew J. and Myers, Brad A. and Chau, Duen Horng},
	title = {A Linguistic Analysis of How People Describe Software Problems},
	booktitle = {Proceedings of the Visual Languages and Human-Centric Computing},
	series = {VLHCC '06},
	year = {2006},
	isbn = {0-7695-2586-5},
	pages = {127--134},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/VLHCC.2006.3},
	doi = {10.1109/VLHCC.2006.3},
	acmid = {1174667},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{deSouza:2205:SIGGROUP,
	author = {de Souza, C. and Froehlich, J. and Dourish, P.},
	title = {Seeking the Source: Software Source Code as a Social and Technical Artifact},
	booktitle = {Proceedings of the 2005 international ACM SIGGROUP conference on Supporting group work},
	series = {GROUP '05},
	year = {2005},
	isbn = {1-59593-223-2},
	location = {Sanibel Island, Florida, USA},
	pages = {107--206},
	numpages = {10},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Sandusky:2005:NCI:1099203.1099238,
	author = {Sandusky, Robert J. and Gasser, Les},
	title = {Negotiation and the coordination of information and activity in distributed software problem management},
	booktitle = {Proceedings of the 2005 international ACM SIGGROUP conference on Supporting group work},
	series = {GROUP '05},
	year = {2005},
	isbn = {1-59593-223-2},
	location = {Sanibel Island, Florida, USA},
	pages = {187--196},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1099203.1099238},
	doi = {10.1145/1099203.1099238},
	acmid = {1099238},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {coordination mechanisms, coordination theory, distributed collective practices, negotiation, software problem management},
}

@inproceedings{Kagdi:2007:MSR:1270394.1271355,
	author = {Kagdi, Huzefa and Maletic, Jonathan I. and Sharif, Bonita},
	title = {Mining Software Repositories for Traceability Links},
	booktitle = {Proceedings of the 15th IEEE International Conference on Program Comprehension},
	series = {ICPC '07},
	year = {2007},
	isbn = {0-7695-2860-0},
	pages = {145--154},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICPC.2007.28},
	doi = {10.1109/ICPC.2007.28},
	acmid = {1271355},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Murphy:1995:SRM:222124.222136,
	author = {Murphy, Gail C. and Notkin, David and Sullivan, Kevin},
	title = {Software reflexion models: bridging the gap between source and high-level models},
	booktitle = {Proceedings of the 3rd ACM SIGSOFT symposium on Foundations of software engineering},
	series = {SIGSOFT '95},
	year = {1995},
	isbn = {0-89791-716-2},
	location = {Washington, D.C., United States},
	pages = {18--28},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/222124.222136},
	doi = {10.1145/222124.222136},
	acmid = {222136},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@article{McMillan:10.1109/TSE.2011.84,
	author = {Collin McMillan and Mark Grechanik and Denys Poshyvanyk and Chen Fu and Qing Xie},
	title = {Exemplar: A Source Code Search Engine For Finding Highly Relevant Applications},
	journal ={IEEE Transactions on Software Engineering},
	volume = {99},
	number = {PrePrints},
	issn = {0098-5589},
	year = {2011},
	doi = {http://doi.ieeecomputersociety.org/10.1109/TSE.2011.84},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{McMillan:C:ICSE:2011,
	Author = {McMillan, C. and Grechanik, M. and Poshyvanyk, D. and Xie, Q. and Fu, C.},
	Title = {Portfolio: Finding Relevant Functions And Their Usages},
	BookTitle = {33rd IEEE/ACM International Conference on Software Engineering (ICSE'11)},
	Address= {Honolulu, Hawaii, USA},
	Pages = {111-120},
	Year = {2011} }

@inproceedings{Panis:5636546,
	author={Panis, M.C.},
	booktitle={Requirements Engineering Conference (RE), 2010 18th IEEE International}, title={Successful Deployment of Requirements Traceability in a Commercial Engineering Organization...Really},
	year={2010},
	month={27 2010-oct. 1},
	volume={},
	number={},
	pages={303 -307},
	keywords={commercial engineering organization;foregone conclusion;product development process;requirements engineering;requirements traceability;successful deployment;systems analysis;},
	doi={10.1109/RE.2010.43},
	ISSN={1090-705X}
}

@article{Binkley:2008:ESR:1454787.1454982,
	author = {Binkley, David and Gold, Nicolas and Harman, Mark and Li, Zheng and Mahdavi, Kiarash},
	title = {An empirical study of the relationship between the concepts expressed in source code and dependence},
	journal = {J. Syst. Softw.},
	issue_date = {December, 2008},
	volume = {81},
	number = {12},
	month = dec,
	year = {2008},
	issn = {0164-1212},
	pages = {2287--2298},
	numpages = {12},
	url = {http://dx.doi.org/10.1016/j.jss.2008.04.007},
	doi = {10.1016/j.jss.2008.04.007},
	acmid = {1454982},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {Concept assignment, Program comprehension, Program slicing, Software engineering},
}

@article{Zou:2010:IAR:1743628.1743653,
	author = {Zou, Xuchang and Settimi, Raffaella and Cleland-Huang, Jane},
	title = {Improving automated requirements trace retrieval: a study of term-based enhancement methods},
	journal = {Empirical Softw. Engg.},
	issue_date = {April     2010},
	volume = {15},
	number = {2},
	month = apr,
	year = {2010},
	issn = {1382-3256},
	pages = {119--146},
	numpages = {28},
	url = {http://dx.doi.org/10.1007/s10664-009-9114-z},
	doi = {10.1007/s10664-009-9114-z},
	acmid = {1743653},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Information retrieval models., Requirements management, Requirements traceability},
}

@article{Linstead2009,
	Author = {Linstead, Erik and Bajracharya, Sushil and Ngo, Trung and Rigor, Paul and Lopes, Cristina and Baldi, Pierre},
	Date-Modified = {2012-04-22 14:01:25 +0000},
	Journal = {Data Mining and Knowledge Discovery},
	Pages = {300-336},
	Title = {Sourcerer: mining and searching internet-scale software repositories},
	Volume = {18},
	Year = {2009},
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s10618-008-0118-x}
}

@inproceedings{Bajracharya:2010:LUS:1882291.1882316,
	author = {Bajracharya, Sushil K. and Ossher, Joel and Lopes, Cristina V.},
	title = {Leveraging usage similarity for effective retrieval of examples in code repositories},
	booktitle = {Proceedings of the eighteenth ACM SIGSOFT international symposium on Foundations of software engineering},
	series = {FSE '10},
	year = {2010},
	isbn = {978-1-60558-791-2},
	location = {Santa Fe, New Mexico, USA},
	pages = {157--166},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1882291.1882316},
	doi = {10.1145/1882291.1882316},
	acmid = {1882316},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {api usage, code search, software information retrieval, ssi, structural semantic indexing},
}

@inproceedings{Chan:2012:SCA:2393596.2393606,
	author = {Chan, Wing-Kwan and Cheng, Hong and Lo, David},
	title = {Searching connected API subgraph via text phrases},
	booktitle = {Proceedings of the ACM SIGSOFT 20th International Symposium on the Foundations of Software Engineering},
	series = {FSE '12},
	year = {2012},
	isbn = {978-1-4503-1614-9},
	location = {Cary, North Carolina},
	pages = {10:1--10:11},
	articleno = {10},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2393596.2393606},
	doi = {10.1145/2393596.2393606},
	acmid = {2393606},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {API graph, API recommendation, subgraph searching},
}

@inproceedings{McMillan:2012:RSC:2337223.2337323,
	author = {McMillan, Collin and Hariri, Negar and Poshyvanyk, Denys and Cleland-Huang, Jane and Mobasher, Bamshad},
	title = {Recommending source code for use in rapid software prototypes},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {848--858},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337323},
	acmid = {2337323},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@inproceedings{McMillan:2012:DSS:2337223.2337267,
	author = {McMillan, Collin and Grechanik, Mark and Poshyvanyk, Denys},
	title = {Detecting similar software applications},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {364--374},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337267},
	acmid = {2337267},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@INPROCEEDINGS{McMillan:5069582,
	author={McMillan, C. and Poshyvanyk, D. and Revelle, M.},
	booktitle={Traceability in Emerging Forms of Software Engineering, 2009. TEFSE '09. ICSE Workshop on},
	title={Combining textual and structural analysis of software artifacts for traceability link recovery},
	year={2009},
	month={may},
	volume={},
	number={},
	pages={41 -48},
	keywords={requirements documentation;software documentation artifacts;source code elements;structural analysis;textual analysis;traceability link recovery;information retrieval;software engineering;system documentation;},
	doi={10.1109/TEFSE.2009.5069582},
	ISSN={}
}

@inproceedings{Shepherd:2007:UNL:1218563.1218587,
	author = {Shepherd, David and Fry, Zachary P. and Hill, Emily and Pollock, Lori and Vijay-Shanker, K.},
	title = {Using natural language program analysis to locate and understand action-oriented concerns},
	booktitle = {Proceedings of the 6th international conference on Aspect-oriented software development},
	series = {AOSD '07},
	year = {2007},
	isbn = {1-59593-615-7},
	location = {Vancouver, British Columbia, Canada},
	pages = {212--224},
	numpages = {13},
	url = {http://doi.acm.org/10.1145/1218563.1218587},
	doi = {10.1145/1218563.1218587},
	acmid = {1218587},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {feature location, program analysis, remodularization, reverse engineering},
}

@inproceedings{Hill:2011:IEC:1985429.1985439,
	author = {Hill, Emily and Pollock, Lori and Vijay-Shanker, K.},
	title = {Investigating how to effectively combine static concern location techniques},
	booktitle = {Proceedings of the 3rd International Workshop on Search-Driven Development: Users, Infrastructure, Tools, and Evaluation},
	series = {SUITE '11},
	year = {2011},
	isbn = {978-1-4503-0597-6},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {37--40},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1985429.1985439},
	doi = {10.1145/1985429.1985439},
	acmid = {1985439},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {concern location, software maintenance, source code exploration, source code search},
} 

@inproceedings{Bettenburg:2010:SIS:1846454.1847957,
	author = {Bettenburg, Nicolas and Hassan, Ahmed E.},
	title = {Studying the Impact of Social Structures on Software Quality},
	booktitle = {Proceedings of the 2010 IEEE 18th International Conference on Program Comprehension},
	series = {ICPC '10},
	year = {2010},
	isbn = {978-0-7695-4113-6},
	pages = {124--133},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICPC.2010.46},
	doi = {10.1109/ICPC.2010.46},
	acmid = {1847957},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {Human Factors, Software Evolution, Metrics/Measurement, Software Quality Assurance},
} 

@inproceedings{Bettenburg:2011:MDR:2025113.2025165,
	author = {Bettenburg, Nicolas},
	title = {Mining development repositories to study the impact of collaboration on software systems},
	booktitle = {Proceedings of the 19th ACM SIGSOFT symposium and the 13th European conference on Foundations of software engineering},
	series = {ESEC/FSE '11},
	year = {2011},
	isbn = {978-1-4503-0443-6},
	location = {Szeged, Hungary},
	pages = {376--379},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/2025113.2025165},
	doi = {10.1145/2025113.2025165},
	acmid = {2025165},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {collaboration, empirical studies, socio-technical congruence, software repositories, unstructured data},
}

@article {M:Harrold:STVR:2000,
	author = {Harrold, Mary Jean and Rothermel, Gregg and Sayre, Kent and Wu, Rui
	and Yi, Liu},
	title = {An empirical investigation of the relationship between spectra
	differences and regression faults},
	journal = {Software Testing, Verification and Reliability},
	volume = {10},
	number = {3},
	publisher = {John Wiley & Sons, Ltd.},
	year = {2000}
}

@inproceedings{T:Reps:ESEC:1997,
	author = {Reps, Thomas and Ball, Thomas and Das, Manuvir and Larus, James},
	title = {The use of program profiling for software maintenance with
	applications to the year 2000 problem},
	booktitle = {Proceedings of the 6th European SOFTWARE ENGINEERING conference
	held jointly with the 5th ACM SIGSOFT international symposium on Foundations of
	software engineering},
	series = {ESEC '97/FSE-5},
	year = {1997},
	pages = {432--449}
} 

@inproceedings{M:Renierses:ASE:2003,
	author={Renieres, M. and Reiss, S.P.},
	booktitle={Automated Software Engineering, 2003. Proceedings. 18th IEEE
	International Conference on}, 
	title={Fault localization with nearest neighbor
	queries},
	year={2003},
	pages={ 30 - 39}
}

@inproceedings{Santelices:2009:LFU:1555001.1555021,
	author = {Santelices, Raul and Jones, James A. and Yanbing Yu and Harrold, Mary Jean},
	title = {Lightweight fault-localization using multiple coverage types},
	booktitle = {Proceedings of the 31st International Conference on Software Engineering},
	series = {ICSE '09},
	year = {2009},
	isbn = {978-1-4244-3453-4},
	pages = {56--66},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2009.5070508},
	doi = {10.1109/ICSE.2009.5070508},
	acmid = {1555021},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@article{Ficco:2011:BLT:1992516.2043292,
	author = {Ficco, Massimo and Pietrantuono, Roberto and Russo, Stefano},
	title = {Bug localization in test-driven development},
	journal = {Adv. Soft. Eng.},
	issue_date = {January 2011},
	volume = {2011},
	month = jan,
	year = {2011},
	issn = {1687-8655},
	pages = {2:1--2:18},
	articleno = {2},
	numpages = {18},
	url = {http://dx.doi.org/10.1155/2011/492757},
	doi = {10.1155/2011/492757},
	acmid = {2043292},
	publisher = {Hindawi Publishing Corp.},
	address = {New York, NY, United States},
} 

@article{Ball:2003:SCL:640128.604140,
	author = {Ball, Thomas and Naik, Mayur and Rajamani, Sriram K.},
	title = {From symptom to cause: localizing errors in counterexample traces},
	journal = {SIGPLAN Not.},
	issue_date = {January 2003},
	volume = {38},
	number = {1},
	month = jan,
	year = {2003},
	issn = {0362-1340},
	pages = {97--105},
	numpages = {9},
	url = {http://doi.acm.org/10.1145/640128.604140},
	doi = {10.1145/640128.604140},
	acmid = {604140},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, software model checking},
}

@inproceedings{Park:2010:FFL:1806799.1806838,
	author = {Park, Sangmin and Vuduc, Richard W. and Harrold, Mary Jean},
	title = {Falcon: fault localization in concurrent programs},
	booktitle = {Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering - Volume 1},
	series = {ICSE '10},
	year = {2010},
	isbn = {978-1-60558-719-6},
	location = {Cape Town, South Africa},
	pages = {245--254},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1806799.1806838},
	doi = {10.1145/1806799.1806838},
	acmid = {1806838},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {atomicity violation, concurrency, debugging, fault localization, order violation},
} 

@inproceedings{Yilmaz:2008:TTF:1368088.1368100,
	author = {Yilmaz, Cemal and Paradkar, Amit and Williams, Clay},
	title = {Time will tell: fault localization using time spectra},
	booktitle = {Proceedings of the 30th international conference on Software engineering},
	series = {ICSE '08},
	year = {2008},
	isbn = {978-1-60558-079-1},
	location = {Leipzig, Germany},
	pages = {81--90},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1368088.1368100},
	doi = {10.1145/1368088.1368100},
	acmid = {1368100},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {automated debugging, fault localization},
}

@inproceedings{Hangal:2002:TDS:581339.581377,
	author = {Hangal, Sudheendra and Lam, Monica S.},
	title = {Tracking down software bugs using automatic anomaly detection},
	booktitle = {Proceedings of the 24th International Conference on Software Engineering},
	series = {ICSE '02},
	year = {2002},
	isbn = {1-58113-472-X},
	location = {Orlando, Florida},
	pages = {291--301},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/581339.581377},
	doi = {10.1145/581339.581377},
	acmid = {581377},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Bhat:2006:EET:1159733.1159787,
	author = {Bhat, Thirumalesh and Nagappan, Nachiappan},
	title = {Evaluating the efficacy of test-driven development: industrial case studies},
	booktitle = {Proceedings of the 2006 ACM/IEEE international symposium on Empirical software engineering},
	series = {ISESE '06},
	year = {2006},
	isbn = {1-59593-218-6},
	location = {Rio de Janeiro, Brazil},
	pages = {356--363},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1159733.1159787},
	doi = {10.1145/1159733.1159787},
	acmid = {1159787},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {software quality, test-driven development},
}

@inproceedings{Chilimbi:2009:HES:1555001.1555020,
	author = {Chilimbi, Trishul M. and Liblit, Ben and Mehra, Krishna and Nori, Aditya V. and Vaswani, Kapil},
	title = {HOLMES: Effective statistical debugging via efficient path profiling},
	booktitle = {Proceedings of the 31st International Conference on Software Engineering},
	series = {ICSE '09},
	year = {2009},
	isbn = {978-1-4244-3453-4},
	pages = {34--44},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2009.5070506},
	doi = {10.1109/ICSE.2009.5070506},
	acmid = {1555020},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{10.1109/ICECCS.2005.25,
	author = {Leonardo Mariani and Mauro Pezza},
	title = {Behavior Capture and Test: Automated Analysis of Component Integration},
	journal ={Engineering of Complex Computer Systems, IEEE International Conference on},
	volume = {0},
	isbn = {0-7695-2284-X},
	year = {2005},
	pages = {292-301},
	doi = {http://doi.ieeecomputersociety.org/10.1109/ICECCS.2005.25},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{Lorenzoli:2008:AGS:1368088.1368157,
	author = {Lorenzoli, Davide and Mariani, Leonardo and Pezz\`{e}, Mauro},
	title = {Automatic generation of software behavioral models},
	booktitle = {Proceedings of the 30th international conference on Software engineering},
	series = {ICSE '08},
	year = {2008},
	isbn = {978-1-60558-079-1},
	location = {Leipzig, Germany},
	pages = {501--510},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1368088.1368157},
	doi = {10.1145/1368088.1368157},
	acmid = {1368157},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {dynamic analysis, gk-tail, model synthesis},
} 

@inproceedings{Cleve:2005:LCP:1062455.1062522,
	author = {Cleve, Holger and Zeller, Andreas},
	title = {Locating causes of program failures},
	booktitle = {Proceedings of the 27th international conference on Software engineering},
	series = {ICSE '05},
	year = {2005},
	isbn = {1-58113-963-2},
	location = {St. Louis, MO, USA},
	pages = {342--351},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1062455.1062522},
	doi = {10.1145/1062455.1062522},
	acmid = {1062522},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {adaptive testing, automated debugging, program analysis, tracing},
} 

@inproceedings{J:Jones:ASE:2005,
	author = {Jones, James A. and Harrold, Mary Jean},
	title = {Empirical evaluation of the tarantula automatic fault-localization
	technique},
	booktitle = {Proceedings of the 20th IEEE/ACM international Conference on
	Automated software engineering},
	year = {2005},
	pages = {273--282},
	numpages = {10}
}

@inproceedings{J:Jone:ICSE:2002,
	author = {Jones, James A. and Harrold, Mary Jean and Stasko, John},
	title = {Visualization of test information to assist fault localization},
	booktitle = {Proceedings of the 24th International Conference on Software
	Engineering},
	series = {ICSE '02},
	year = {2002},
	pages = {467--477},
	numpages = {11}
} 

@techreport{H:Pan:1992,
	title={Heuristics for automatic localization of software faults},
	author={Pan, H. and Spafford, E.H.},
	journal={World Wide Web},
	year={1992}
}

@inproceedings{H:Agrawal:ISSRE:1995,
	author={Agrawal, H. and Horgan, J.R. and London, S. and Wong, W.E.},
	booktitle={Software Reliability Engineering, 1995. Proceedings., Sixth
	International Symposium on}, title={Fault localization using execution slices
	and dataflow tests},
	year={1995},
	pages={143 -151}}

@inproceedings{T:Gyimothy:ESEC:1999,
	author = {Gyim\'{o}thy, Tibor and Besz{\'e}des, \'{A}rp\'{a}d and Forg\'{a}cs,
	Ist\'{a}n},
	title = {An efficient relevant slicing method for debugging},
	booktitle = {Proceedings of the 7th European software engineering conference
	held jointly with the 7th ACM SIGSOFT international symposium on Foundations of
	software engineering},
	series = {ESEC/FSE-7},
	year = {1999},
	pages = {303--321}
} 

@inproceedings{F:Servant:ICSE:2012,
	author = {Servant, Francisco and Jones, James A.},
	title = {WhoseFault: automatic developer-to-fault assignment through fault localization},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	pages = {36--46}
} 

@inproceedings{A:Mockus:ICSE:2002,
	author = {Mockus, Audris and Herbsleb, James D.},
	title = {Expertise browser: a quantitative approach to identifying expertise},
	booktitle = {Proceedings of the 24th International Conference on Software Engineering},
	series = {ICSE '02},
	year = {2002},
	pages = {503--512}
} 

@inproceedings{S:Minto:MSR:2007,
	author = {Minto, Shawn and Murphy, Gail C.},
	title = {Recommending Emergent Teams},
	booktitle = {Proceedings of the Fourth International Workshop on Mining Software Repositories},
	series = {MSR '07},
	year = {2007},
	pages = {5--}
} 

@inproceedings{D:Ma:ICSM:2009,
	author = {David Ma and David Schuler and Thomas Zimmermann and Jonathan Sillito},
	title = {Expert recommendation with usage expertise},
	journal ={Software Maintenance, IEEE International Conference on},
	volume = {0},
	isbn = {978-1-4244-4897-5},
	year = {2009},
	pages = {535-538},
	doi = {http://doi.ieeecomputersociety.org/10.1109/ICSM.2009.5306386},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{G:Jeong:ESEC:2009,
	author = {Jeong, Gaeul and Kim, Sunghun and Zimmermann, Thomas},
	title = {Improving bug triage with bug tossing graphs},
	booktitle = {Proceedings of the the 7th joint meeting of the European software engineering conference and the ACM SIGSOFT symposium on The foundations of software engineering},
	series = {ESEC/FSE '09},
	year = {2009},
	pages = {111--120},
	numpages = {10}
} 

@inproceedings{J:Anvik:ICSE:2006,
	author = {Anvik, John and Hiew, Lyndon and Murphy, Gail C.},
	title = {Who should fix this bug?},
	booktitle = {Proceedings of the 28th international conference on Software engineering},
	series = {ICSE '06},
	year = {2006},
	isbn = {1-59593-375-1},
	location = {Shanghai, China},
	pages = {361--370},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1134285.1134336},
	doi = {10.1145/1134285.1134336},
	acmid = {1134336},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug report assignment, bug triage, issue tracking, machine learning, problem tracking},
} 

@inproceedings{Abadi:A:ICPC:08,
	Author={Abadi, A. and Nisenson, M. and Simionovici, Y. },
	Title = {A Traceability Technique for Specifications},
	BookTitle = {16th IEEE International Conference on Program Comprehension (ICPC'08)},
	Address= {Amsterdam, The Netherlands},
	Pages = {103-112},
	Year = {2008} }

@inproceedings{Abebe:S:CSMR:2009,
	Author = {Abebe, S. L. and Haiduc, S. and Marcus, A. and Tonella, P. and Antoniol, G.},
	Title = {Analyzing the Evolution of the Source Code Vocabulary},
	BookTitle = {13th IEEE European Conference on Software Maintenance and Reengineering (CSMR'09)},
	Address= {Kaiserslautern, Germany},
	Pages = {189-198},
	Year = {2009} }

@inproceedings{Antoniol:G:CSMR:2000,
	Author = {Antoniol, G. and Canfora, G. and Casazza, G. and De Lucia, A.},
	Title = {Identifying the Starting Impact  Set of a Maintenance and Reengineering},
	BookTitle = {4th European Conference on Software Maintenance (CSMR2000)},
	Address= {Zurich, Switzerland},
	Publisher = {CS Press},
	Pages = {227-230},
	Year = {2000} }

@inproceedings{Antoniol:G:ICSM:2000,
	Author = {Antoniol, Giuliano and Canfora, Gerardo and Casazza, Gerardo and De Lucia, Andrea},
	Title = {Information Retrieval Models for Recovering Traceability Links between Code and Documentation},
	BookTitle = {IEEE International Conference on Software Maintenance (ICSM'00)},
	Address= {San Jose, CA},
	Publisher = {IEEE COmputer Society},
	Pages = {40-51},
	Year = {2000} }

@article{Antoniol:G:TSE:2002,
	Author = {Antoniol, Giuliano and Canfora, Gerardo and Casazza, Gerardo and De Lucia, Andrea and Merlo, Ettore},
	Title = {Recovering Traceability Links between Code and Documentation},
	Journal = {IEEE Transactions on Software Engineering},
	Volume = {28},
	Number = {10},
	Pages = {970 - 983},
	Year = {2002} }

@article{Antoniol:G:TSE:2006,
	Author = {Antoniol, G. and Guéhéneuc, Y.G.},
	Title = {Feature Identification: An Epidemiological Metaphor},
	Journal = {IEEE Transactions on Software Engineering},
	Volume = {32},
	Number = {9},
	Pages = {627-641},
	Year = {2006} }

@inproceedings{Antoniol:G:ICSM:2008,
	Author = {Antoniol, G. and Hayes, J. H. and Gueheneuc, Y.. and Di Penta, M. },
	Title = {Reuse or rewrite: Combining textual, static, and dynamic analyses to assess the cost of keeping a system up-to-date},
	BookTitle = {IEEE International Conference on Software Maintenance (ICSM'08)},
	Pages = {147-156},
	Year = {2008} }

@inproceedings{Asuncion:H:ICSE:2010,
	Author = {Asuncion, H.  and Asuncion, A.  and Taylor, R.},
	Title = {Software Traceability with Topic Modeling},
	BookTitle = {32nd International Conference on Software Engineering (ICSE'10)},
	Year = {2010} }

@inproceedings{Baldi:P:OOPSLA:2008,
	Author = {Baldi, P. and Linstead, E. and Lopes, C. and Bajracharya, S.},
	Title = {A Theory of Aspects as Latent Topics},
	BookTitle = {ACM SIGPLAN Conference on Object-Oriented Programming, Systems, Languages and Applications (OOPSLA'08)},
	Address= {Nashville, Tennessee},
	Pages = {543-562},
	Year = {2008} }

@article{Binkley:D:JSS:2008,
	Author = {Binkley, D. and Gold, G. and Harman, M. and Li, Z. and Mahdavi, K.},
	Title = {An empirical study of the relationship between the concepts expressed in source code and dependence},
	Journal = {The Journal of Systems and Software},
	Volume = {81},
	Pages = {2287–2298},
	Year = {2008} }

@misc{Binkley:D:2009,
	Author = {Binkley, D. and Lawrie, D.},
	Title = {Information Retrieval Applications in Software Maintenance and Evolution},
	Publisher = {Taylor & Francis LLC},
	Year = {2009} }

@article{Boyd:N:JOOP:1999,
	Author = {Boyd, N.},
	Title = {Using Natural Language in Software Development},
	Journal = {Journal of Object-Oriented Programming},
	Volume = {11},
	Number = {9},
	Pages = {45-55},
	Year = {1999} }

@inproceedings{Capobianco:G:ICPC:2009,
	Author = {Capobianco, Giovanni and De Lucia, Andrea and Oliveto, Rocco and Panichella, Annibale and Panichella, Sebastiano},
	Title = {On the role of the nouns in IR-based traceability recovery},
	BookTitle = {17th IEEE International Conference on Program Comprehension (ICPC'09)},
	Address= {Vancouver, British Columbia, Canada},
	Pages = {148 - 157},
	Year = {2009} }

@inproceedings{Caprile:B:ICSM:2000,
	Author = {Caprile, B. and Tonella, P.},
	Title = {Restructuring Program Identifier Names},
	BookTitle = {16th IEEE Internation Conference on Software Maintenance (ICSM'00)},
	Address= {San Jose, California, USA},
	Pages = {97-107},
	Year = {2000} }

@article{Cleary:B:EMSE:2009,
	Author = {Cleary, B. and Exton, C. and Buckley, J. and English, M.},
	Title = {An empirical analysis of information retrieval based concept location techniques in software comprehension},
	Journal = {Empirical Software Engineering},
	Volume = {14},
	Number = {1},
	Pages = {93-130},
	Year = {2009} }

@article{DeLucia:A:TSE:2011,
	Author = {De Lucia, A. and Di Penta, M. and Oliveto, R.},
	Title = {Improving Source Code Lexicon via Traceability and Information Retrieval},
	Journal = {IEEE Transactions on Software Engineering},
	volume = {37},
	number = {2},
	year = {2011},
	pages = {205--227} }

@article{DeLucia:A:TOSEM:2007,
	Author = {De Lucia, A. and Fasano, F. and Oliveto, R. and Tortora, G.},
	Title = {Recovering Traceability Links in Software Artefact Management Systems},
	Journal = {ACM Transactions on Software Engineering and Methodology},
	Volume = {16},
	Number = {4},
	Year = {2007} }

@inproceedings{DeLucia:A:ICSM:2009,
	Author = {De Lucia, Andrea and Oliveto, Rocco and Tortora, Genoveffa},
	Title = {The role of the coverage analysis during IR-based traceability recovery: A controlled experiment},
	BookTitle = {25th IEEE International Conference on Software Maintenance (ICSM'09)},
	Address= {Edmonton, Alberta, Canada},
	Pages = {371-380},
	Year = {2009} }

@inproceedings{Dit:B:ICPC:2011,
	Author = {Dit, Bogdan and Guerrouj, Latifa  and Poshyvanyk, Denys and Antoniol, Giulio},
	Title = {Can Better Identifier Splitting Techniques Help Feature Location?},
	BookTitle = {19th IEEE International Conference on Program Comprehension (ICPC'11)},
	Address= {Kingston, Ontario},
	Pages = {11-20},
	Year = {2011} }

@inproceedings{Haiduc:S:ICPC:2008,
	Author = {Haiduc, S. and Marcus, A.},
	Title = {On the Use of Domain Terms in Source Code},
	BookTitle = {16th IEEE International Conference on Program Comprehension (ICPC'08)},
	Address= {Amsterdam, The Netherlands},
	Pages = {113-122},
	Year = {2008} }

@inproceedings{Helm:R:OOPSLA:1991,
	Author = {Helm, Richard  	  and Maarek, Yoelle S.  	 },
	Title = {Integrating information retrieval and domain specific approaches for browsing and retrieval in object-oriented class libraries},
	BookTitle = {Conference proceedings on Object-oriented programming systems, languages, and applications},
	Address= {Phoenix, Arizona, United States},
	Publisher = {ACM Press   New York, NY, USA},
	Pages = {47-61},
	Year = {1991} }

@inproceedings{Hindle:A:ICSM:2009,
	Author = {Hindle, A. J. and Godfrey, M. W. and Holt, R. C.},
	Title = {What’s Hot and What’s Not: Windowing Developer Topic Analysis},
	BookTitle = {IEEE International Conference on Software Maintenance (ICSM'09)},
	Address= {Edmonton, Alberta},
	Year = {2009} }

@article{Kagdi:H:JSME:2011,
	Author = {Kagdi, H. and Gethers, M. and Poshyvanyk, D. and Hammad, M.},
	Title = {Assigning Change Requests to Software Developers},
	Journal = {Journal of Software Maintenance and Evolution: Research and Practice (JSME)},
	Year = {2011} }

@inproceedings{Lawrie:D:ICPC:2006,
	Author = {Lawrie, D. and Morrell, C. and Feild, H. and Binkley, D.},
	Title = {What's in a Name? A Study of Identifiers},
	BookTitle = {14th IEEE International Conference on Program Comprehension (ICPC'06)},
	Address= {Athens, Greece},
	Pages = {3-12},
	Year = {2006} }

@inproceedings{Lo:K:OOPSLA:2006,
	Author = {Lo, K. K.  and Chan, M. K.  and Baniassad, E. },
	Title = {Isolating and Relating Concerns in Requirements using Latent Semantic Analysis},
	BookTitle = {ACM SIGPLAN International Conference on Object-Oriented Programming, Systems, Languages and Applications (OOPSLA'06)},
	Pages = {383 - 396 },
	Year = {2006} }

@article{Lukings:S:IST:2010,
	Author = {Lukins, S. K. and Kraft, N. A. and Etzkorn, L. H.},
	Title = {Bug localization using Latent Dirichlet Allocation},
	Journal = {Information and Software Technology},
	Volume = {52},
	Number = {9},
	Pages = {972-990},
	Year = {2010} }

@article{Maarek:Y:TSE:1991,
	Author = {Maarek, Y. S. and Berry, D. M. and Kaiser, G. E.},
	Title = {An Information Retrieval Approach for Automatically Constructing Software Libraries},
	Journal = {IEEE Transactions on Software Engineering},
	Volume = {17},
	Number = {8},
	Pages = {800-813},
	Year = {1991} }

@inproceedings{Maletic:J:ASE:1999,
	Author = {Maletic, Jonathan I. and Valluri, N.},
	Title = {Automatic Software Clustering via Latent Semantic Analysis},
	BookTitle = {14th IEEE International Conference on Automated Software Engineering (ASE'99)},
	Address= {Cocoa Beach Florida},
	Pages = {251-254},
	Note  = {hard copy - .pdf},
	Year = {1999} }

@inproceedings{Marcus:A:ICSE:2003,
	Author = {Marcus, Andrian and Maletic, Jonathan I.},
	Title = {Recovering Documentation-to-Source-Code Traceability Links using Latent Semantic Indexing},
	BookTitle = {25th IEEE/ACM International Conference on Software Engineering (ICSE'03)},
	Address= {Portland, OR},
	Pages = {125-137},
	Keywords = {reverse_engineering
	traceability},
	Year = {2003} }

@inproceedings{Marcus:A:ICSM:2005,
	Author = {Marcus, Andrian and Poshyvanyk, Denys},
	Title = {The Conceptual Cohesion of Classes},
	BookTitle = {21st IEEE International Conference on Software Maintenance (ICSM'05)},
	Address= {Budapest, Hungary},
	Pages = {133-142},
	Year = {2005} }

@article{Marcus:A:TSE:2008,
	Author = {Marcus, A. and Poshyvanyk, D. and Ferenc, R.},
	Title = {Using the Conceptual Cohesion of Classes for Fault Prediction in Object Oriented Systems},
	Journal = {IEEE Transactions on Software Engineering},
	Volume = {34},
	Number = {2},
	Pages = {287-300},
	Year = {2008} }

@article{Yadla:Hayes:NASE:2005,
	Author = {Yadla, S. and Hayes, J. and Dekhtyar, A.},
	Title = {Tracing Requirements to Defect Reports:  An Application of Information Retrieval Techniques},
	Journal = {Innovations in Systems and Software Engineering:  A NASA Journal},
	Volume = {1},
	Number = {2},
	Pages = {116-124},
	Year = {2005}
}

@article{Poshyvanyk:D:TOSEM:2012,
	Author = {Poshyvanyk, D. and Gethers, M. and Marcus, A.},
	Title = {Concept Location using Formal Concept Analysis and Information Retrieval},
	Journal = {ACM Transactions on Software Engineering and Methodology},
	Year = {2012} }

@article{Poshyvanyk:D:TSE:07,
	Author = {Poshyvanyk, D. and Guéhéneuc, Y.G. and Marcus, A. and Antoniol, G. and Rajlich, V.},
	Title = {Feature Location using Probabilistic Ranking of Methods based on Execution Scenarios and Information Retrieval},
	Journal = {IEEE Transactions on Software Engineering},
	Volume = {33},
	Number = {6},
	Pages = {420-432},
	Year = {2007} }

@article{Poshyvanyk:D:EMSE:2009,
	Author = {Poshyvanyk, D. and Marcus, A. and Ferenc, R. and Gyimóthy, T.},
	Title = {Using Information Retrieval based Coupling Measures for Impact Analysis},
	Journal = {Empirical Software Engineering},
	Volume = {14},
	Number = {1},
	Pages = {5-32},
	Year = {2009} }

@article{Blei:D:JMLR:2003,
	Author = {Blei, D. M. and Ng, A. Y. and Jordan, M. I.},
	Title = {Latent Dirichlet Allocation},
	Journal = {Journal of Machine Learning Research},
	Volume = {3},
	Pages = {993-1022},
	Year = {2003} }

@book{Salton:G:1986,
	Author = {Salton, G. and McGill, M.},
	Title = {Introduction to Modern Information Retrieval},
	Publisher = {McGraw-Hill},
	Year = {1986} }

@book{Baeza-Yates:R:1999,
	Author = {Baeza-Yates, Ricardo A. and Ribeiro-Neto, Berthier},
	Title = {Modern Information Retrieval},
	Publisher = {Addison-Wesley},
	Year = {1999} }

@article{Deerwester:S:JASIS:1990,
	Author = {Deerwester, Scott and Dumais, Susan T. and Furnas, G. W. and Landauer, Thomas K. and Harshman, R.},
	Title = {Indexing by Latent Semantic Analysis},
	Journal = {Journal of the American Society for Information Science},
	Volume = {41},
	Pages = {391-407},
	Year = {1990} }

@inproceedings{Gethers:M:ASE:2011,
	Author = {Gethers, M. and Kagdi, H. and Dit, B. and Poshyvanyk, D.},
	Title = {An Adaptive Approach to Impact Analysis from Change Requests to Source Code},
	BookTitle = {26th IEEE/ACM International Conference on Automated Software Engineering (ASE'11)},
	Address= {Lawrence, Kansas},
	Year = {2011} }

@inproceedings{Gethers:M:ICSM:2011,
	Author = {Gethers, M. and Oliveto, R. and Poshyvanyk, D. and De Lucia, A.},
	Title = {On Integrating Orthogonal Information Retrieval Methods to Improve Traceability Link Recovery},
	BookTitle = {27th IEEE International Conference on Software Maintenance (ICSM'11)},
	Address= {Williamsburg, Virginia, USA},
	Pages = {to appear},
	Year = {2011} }

@inproceedings{Gethers:M:ICSM:2010,
	Author = {Gethers, M.  and Poshyvanyk, D.},
	Title = {Using Relational Topic Models to Capture Coupling among Classes in Object-Oriented Software Systems},
	BookTitle = {26th IEEE International Conference on Software Maintenance (ICSM'10)},
	Address= {Timişoara, Romania},
	Pages = {1-10},
	Year = {2010} }

@inproceedings{Gethers:M:ICSE-T:2011,
	Author = {Gethers, M. and Savage, T. and Di Penta, M. and Oliveto, R. and Poshyvanyk, D. and De Lucia, A.},
	Title = {CodeTopics: Which Topic Am I Coding Now?},
	BookTitle = {33rd IEEE/ACM International Conference on Software Engineering (ICSE'11), Formal Research Tool Demonstration},
	Address= {Honolulu, Hawaii, USA},
	Pages = {1034-1036},
	Year = {2011} }

@inproceedings{Oliveto:R:ICSE-NIER:2011,
	Author = {Oliveto, R. and Gethers, M. and Bavota, G. and Poshyvanyk, D. and De Lucia, A.},
	Title = {Identifying Method Friendships to Remove the Feature Envy Bad Smell},
	BookTitle = {33rd IEEE/ACM International Conference on Software Engineering (ICSE'11)},
	Address= {Honolulu, Hawaii, USA},
	Pages = {820-823},
	Year = {2011} }

@article{Lukins:2010:BLU:1824820.1824850,
	author = {Lukins, Stacy K. and Kraft, Nicholas A. and Etzkorn, Letha H.},
	title = {Bug localization using latent Dirichlet allocation},
	journal = {Inf. Softw. Technol.},
	issue_date = {September, 2010},
	volume = {52},
	number = {9},
	month = sep,
	year = {2010},
	issn = {0950-5849},
	pages = {972--990},
	numpages = {19},
	url = {http://dx.doi.org/10.1016/j.infsof.2010.04.002},
	doi = {10.1016/j.infsof.2010.04.002},
	acmid = {1824850},
	publisher = {Butterworth-Heinemann},
	address = {Newton, MA, USA},
	keywords = {Bug localization, Information retrieval, Latent Dirichlet allocation, Program comprehension},
}

@inproceedings{Linares-Vasquez:M:ICSM:2012,
	Author = {Linares-Vasquez, M. and Dang, H. and Hossen, K. and Kagdi, H. and Gethers, M. and Poshyvanyk, D.},
	Title = {Triaging Incoming Change Requests: Bug or Commit History, or Code Authorship?},
	BookTitle = {28th IEEE International Conference on Software Maintenance (ICSM'12)},
	Address = {Riva del Garda, Italy},
	Year = {2012} }

@inproceedings{Oliveto:R:ICPC:2010,
	Author = {Oliveto, R. and Gethers, M. and Poshyvanyk, D. and De Lucia, A.},
	Title = {On the Equivalence of Information Retrieval Methods for Automated Traceability Link Recovery},
	BookTitle = {18th IEEE International Conference on Program Comprehension (ICPC'10)},
	Address= {Braga, Portugal},
	Pages = {68-71},
	Year = {2010} }

@inproceedings{Klock:S:TEFSE:2011,
	Author = {Klock, S. and Gethers, M. and Dit, B. and Poshyvanyk, D.},
	Title = {Traceclipse: An Eclipse Plug-in for Traceability Link Recovery and Management},
	BookTitle = {6th International Workshop on Traceability in Emerging Forms of Software Engineering (TEFSE'11)},
	Address= {Honolulu, Hawaii, HI},
	Year = {2011} }


@article{Dit:B:JSME:2011,
	Author = {Dit, B. and Revelle, M. and Gethers, M. and Poshyvanyk, D.},
	Title = {Feature Location in Source Code: A Taxonomy and Survey},
	Journal = {Journal of Software Maintenance and Evolution: Research and Practice},
	Year = {2011} }

@inproceedings{Gethers:2012:IIA:2337223.2337274,
	author = {Gethers, Malcom and Dit, Bogdan and Kagdi, Huzefa and Poshyvanyk, Denys},
	title = {Integrated impact analysis for managing software changes},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {430--440},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337274},
	acmid = {2337274},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA}
}

@inproceedings{Dickinson:2001:FFC:381473.381509,
	author = {Dickinson, William and Leon, David and Podgurski, Andy},
	title = {Finding failures by cluster analysis of execution profiles},
	booktitle = {Proceedings of the 23rd International Conference on Software Engineering},
	series = {ICSE '01},
	year = {2001},
	isbn = {0-7695-1050-7},
	location = {Toronto, Ontario, Canada},
	pages = {339--348},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=381473.381509},
	acmid = {381509},
	publisher = {IEEE Computer Society}
} 


@inproceedings{McDonald:D:CSCW:2000,
	author = {McDonald, David W. and Ackerman, Mark S.},
	title = {Expertise recommender: a flexible recommendation system and architecture},
	booktitle = {Proceedings of the 2000 ACM conference on Computer supported cooperative work},
	series = {CSCW '00},
	year = {2000},
	isbn = {1-58113-222-0},
	location = {Philadelphia, Pennsylvania, United States},
	pages = {231--240},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/358916.358994},
	doi = {10.1145/358916.358994},
	acmid = {358994},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {CSCW, collaborative filtering, computer-supported cooperative work, expert locators, expertise finding, expertise location, information seeking, recommendation systems}
} 

@inproceedings{Anvik:J:MSR:2007,
	author = {Anvik, John and Murphy, Gail C.},
	title = {Determining Implementation Expertise from Bug Reports},
	booktitle = {Proceedings of the Fourth International Workshop on Mining Software Repositories},
	series = {MSR '07},
	year = {2007},
	isbn = {0-7695-2950-X},
	pages = {2--},
	url = {http://dx.doi.org/10.1109/MSR.2007.7},
	doi = {10.1109/MSR.2007.7},
	acmid = {1269018},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA}
}

@inproceedings{Tamrawi:A:FSE:2011,
	author = {Tamrawi, Ahmed and Nguyen, Tung Thanh and Al-Kofahi, Jafar M. and Nguyen, Tien N.},
	title = {Fuzzy set and cache-based approach for bug triaging},
	booktitle = {Proceedings of the 19th ACM SIGSOFT symposium and the 13th European conference on Foundations of software engineering},
	series = {ESEC/FSE '11},
	year = {2011},
	isbn = {978-1-4503-0443-6},
	location = {Szeged, Hungary},
	pages = {365--375},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2025113.2025163},
	doi = {10.1145/2025113.2025163},
	acmid = {2025163},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug triaging, developers' expertise, fuzzy set}
} 

@incollection{Song:X:UM:2005,
	year={2005},
	isbn={978-3-540-27885-6},
	booktitle={User Modeling 2005},
	volume={3538},
	series={Lecture Notes in Computer Science},
	editor={Ardissono, Liliana and Brna, Paul and Mitrovic, Antonija},
	doi={10.1007/11527886_14},
	title={ExpertiseNet: Relational and Evolutionary Expert Modeling},
	url={http://dx.doi.org/10.1007/11527886_14},
	publisher={Springer Berlin Heidelberg},
	author={Song, Xiaodan and Tseng, BelleL. and Lin, Ching-Yung and Sun, Ming-Ting},
	pages={99-108}
}

@inproceedings{Matter:D:MSR:2009,
	author = {Matter, Dominique and Kuhn, Adrian and Nierstrasz, Oscar},
	title = {Assigning bug reports using a vocabulary-based expertise model of developers},
	booktitle = {Proceedings of the 2009 6th IEEE International Working Conference on Mining Software Repositories},
	series = {MSR '09},
	year = {2009},
	isbn = {978-1-4244-3493-0},
	pages = {131--140},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/MSR.2009.5069491},
	doi = {10.1109/MSR.2009.5069491},
	acmid = {1591148},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA}
} 

@inproceedings{Rahman:F:ICSE:2011,
	author = {Rahman, Foyzur and Devanbu, Premkumar},
	title = {Ownership, experience and defects: a fine-grained study of authorship},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {491--500},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985860},
	doi = {10.1145/1985793.1985860},
	acmid = {1985860},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {collaboration, experience, ownership, software quality}
} 

@inproceedings{Bird:C:FSE:2011,
	author = {Bird, Christian and Nagappan, Nachiappan and Murphy, Brendan and Gall, Harald and Devanbu, Premkumar},
	title = {Don't touch my code!: examining the effects of ownership on software quality},
	booktitle = {Proceedings of the 19th ACM SIGSOFT symposium and the 13th European conference on Foundations of software engineering},
	series = {ESEC/FSE '11},
	year = {2011},
	isbn = {978-1-4503-0443-6},
	location = {Szeged, Hungary},
	pages = {4--14},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2025113.2025119},
	doi = {10.1145/2025113.2025119},
	acmid = {2025119},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {emprical software engineering, expertise, ownership, quality}
} 

@inproceedings{German:D:MSR:2006,
	author = {German, Daniel M.},
	title = {A study of the contributors of PostgreSQL},
	booktitle = {Proceedings of the 2006 international workshop on Mining software repositories},
	series = {MSR '06},
	year = {2006},
	isbn = {1-59593-397-2},
	location = {Shanghai, China},
	pages = {163--164},
	numpages = {2},
	url = {http://doi.acm.org/10.1145/1137983.1138022},
	doi = {10.1145/1137983.1138022},
	acmid = {1138022},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {mining software repositories, software evolution}
} 

@inproceedings{Tsunoda:M:MSR:2006,
	author = {Tsunoda, Masateru and Monden, Akito and Kakimoto, Takeshi and Kamei, Yasutaka and Matsumoto, Ken-ichi},
	title = {Analyzing OSS developers' working time using mailing lists archives},
	booktitle = {Proceedings of the 2006 international workshop on Mining software repositories},
	series = {MSR '06},
	year = {2006},
	isbn = {1-59593-397-2},
	location = {Shanghai, China},
	pages = {181--182},
	numpages = {2},
	url = {http://doi.acm.org/10.1145/1137983.1138031},
	doi = {10.1145/1137983.1138031},
	acmid = {1138031},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {overtime work, workload}
} 

@inproceedings{Bird:C:MSR:2006,
	author = {Bird, Christian and Gourley, Alex and Devanbu, Prem and Gertz, Michael and Swaminathan, Anand},
	title = {Mining email social networks},
	booktitle = {Proceedings of the 2006 international workshop on Mining software repositories},
	series = {MSR '06},
	year = {2006},
	isbn = {1-59593-397-2},
	location = {Shanghai, China},
	pages = {137--143},
	numpages = {7},
	url = {http://doi.acm.org/10.1145/1137983.1138016},
	doi = {10.1145/1137983.1138016},
	acmid = {1138016},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {open source, social networks}
} 

@article{DelRosso:C:JSME:2009,
	author = {Del Rosso, Christian},
	title = {Comprehend and analyze knowledge networks to improve software evolution},
	journal = {J. Softw. Maint. Evol.},
	issue_date = {May 2009},
	volume = {21},
	number = {3},
	month = may,
	year = {2009},
	issn = {1532-060X},
	pages = {189--215},
	numpages = {27},
	url = {http://dx.doi.org/10.1002/smr.v21:3},
	doi = {10.1002/smr.v21:3},
	acmid = {1552147},
	publisher = {John Wiley \& Sons, Inc.},
	address = {New York, NY, USA},
	keywords = {global software engineering, knowledge management, social network analysis, software development}
} 

@inproceedings{Weissgerber:P:MSR:2007,
	author = {Weissgerber, Peter and Pohl, Mathias and Burch, Michael},
	title = {Visual Data Mining in Software Archives to Detect How Developers Work Together},
	booktitle = {Proceedings of the Fourth International Workshop on Mining Software Repositories},
	series = {MSR '07},
	year = {2007},
	isbn = {0-7695-2950-X},
	pages = {9--},
	url = {http://dx.doi.org/10.1109/MSR.2007.34},
	doi = {10.1109/MSR.2007.34},
	acmid = {1269024},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA}
} 

@article{German:D:EMSE:2006,
	author = {German, Daniel M.},
	title = {An empirical study of fine-grained software modifications},
	journal = {Empirical Softw. Engg.},
	issue_date = {September 2006},
	volume = {11},
	number = {3},
	month = sep,
	year = {2006},
	issn = {1382-3256},
	pages = {369--393},
	numpages = {25},
	url = {http://dx.doi.org/10.1007/s10664-006-9004-6},
	doi = {10.1007/s10664-006-9004-6},
	acmid = {1146486},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Software artifacts, Software evolution, Software visualization, Version control}
} 

@inproceedings{Fischer:M:ICSM:2003,
	author = {Fischer, Michael and Pinzger, Martin and Gall, Harald},
	title = {Populating a Release History Database from Version Control and Bug Tracking Systems},
	booktitle = {Proceedings of the International Conference on Software Maintenance},
	series = {ICSM '03},
	year = {2003},
	isbn = {0-7695-1905-9},
	pages = {23--},
	url = {http://dl.acm.org/citation.cfm?id=942800.943568},
	acmid = {943568},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA}
} 

@inproceedings{Runeson:P:ICSE:2007,
	author = {Runeson, Per and Alexandersson, Magnus and Nyholm, Oskar},
	title = {Detection of Duplicate Defect Reports Using Natural Language Processing},
	booktitle = {Proceedings of the 29th international conference on Software Engineering},
	series = {ICSE '07},
	year = {2007},
	isbn = {0-7695-2828-7},
	pages = {499--510},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/ICSE.2007.32},
	doi = {10.1109/ICSE.2007.32},
	acmid = {1248882},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@phdthesis{Hiew:L:Thesis,
	title={Assisted detection of duplicate bug reports},
	author={Hiew, L.},
	year={2006},
	school={The University Of British Columbia}
}

@inproceedings{Wang:X:ICSE:2008,
	author = {Wang, Xiaoyin and Zhang, Lu and Xie, Tao and Anvik, John and Sun, Jiasu},
	title = {An approach to detecting duplicate bug reports using natural language and execution information},
	booktitle = {Proceedings of the 30th international conference on Software engineering},
	series = {ICSE '08},
	year = {2008},
	isbn = {978-1-60558-079-1},
	location = {Leipzig, Germany},
	pages = {461--470},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1368088.1368151},
	doi = {10.1145/1368088.1368151},
	acmid = {1368151},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {duplicate bug report, execution information, information retrieval},
} 

@inproceedings{Sun:C:ICSE:2010,
	author = {Sun, Chengnian and Lo, David and Wang, Xiaoyin and Jiang, Jing and Khoo, Siau-Cheng},
	title = {A discriminative model approach for accurate duplicate bug report retrieval},
	booktitle = {Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering - Volume 1},
	series = {ICSE '10},
	year = {2010},
	isbn = {978-1-60558-719-6},
	location = {Cape Town, South Africa},
	pages = {45--54},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1806799.1806811},
	doi = {10.1145/1806799.1806811},
	acmid = {1806811},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Jalbert:N:DSN:2008,
	title={Automated duplicate detection for bug tracking systems},
	author={Jalbert, N. and Weimer, W.},
	booktitle={Dependable Systems and Networks With FTCS and DCC, 2008. DSN 2008. IEEE International Conference on},
	pages={52--61},
	year={2008},
	organization={IEEE}
}

@inproceedings{Sun:C:ASE:2011,
	author = {Sun, Chengnian and Lo, David and Khoo, Siau-Cheng and Jiang, Jing},
	title = {Towards more accurate retrieval of duplicate bug reports},
	booktitle = {Proceedings of the 2011 26th IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '11},
	year = {2011},
	isbn = {978-1-4577-1638-6},
	pages = {253--262},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ASE.2011.6100061},
	doi = {10.1109/ASE.2011.6100061},
	acmid = {2190180},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Bettenburg:N:FSE:2008,
	author = {Bettenburg, Nicolas and Just, Sascha and Schr\"{o}ter, Adrian and Weiss, Cathrin and Premraj, Rahul and Zimmermann, Thomas},
	title = {What makes a good bug report?},
	booktitle = {Proceedings of the 16th ACM SIGSOFT International Symposium on Foundations of software engineering},
	series = {SIGSOFT '08/FSE-16},
	year = {2008},
	isbn = {978-1-59593-995-1},
	location = {Atlanta, Georgia},
	pages = {308--318},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1453101.1453146},
	doi = {10.1145/1453101.1453146},
	acmid = {1453146},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Bettenburg:N:MSR:2008,
	author = {Bettenburg, Nicolas and Premraj, Rahul and Zimmermann, Thomas and Kim, Sunghun},
	title = {Extracting structural information from bug reports},
	booktitle = {Proceedings of the 2008 international working conference on Mining software repositories},
	series = {MSR '08},
	year = {2008},
	isbn = {978-1-60558-024-1},
	location = {Leipzig, Germany},
	pages = {27--30},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1370750.1370757},
	doi = {10.1145/1370750.1370757},
	acmid = {1370757},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug reports, patches, source code, stack traces, structural information},
} 

@inproceedings{Kim:S:MSR:2006,
	author = {Kim, Sunghun and Whitehead,Jr., E. James},
	title = {How long did it take to fix bugs?},
	booktitle = {Proceedings of the 2006 international workshop on Mining software repositories},
	series = {MSR '06},
	year = {2006},
	isbn = {1-59593-397-2},
	location = {Shanghai, China},
	pages = {173--174},
	numpages = {2},
	url = {http://doi.acm.org/10.1145/1137983.1138027},
	doi = {10.1145/1137983.1138027},
	acmid = {1138027},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Canfora:G:SAC:2006,
	author = {Canfora, Gerardo and Cerulo, Luigi},
	title = {Supporting change request assignment in open source development},
	booktitle = {Proceedings of the 2006 ACM symposium on Applied computing},
	series = {SAC '06},
	year = {2006},
	isbn = {1-59593-108-2},
	location = {Dijon, France},
	pages = {1767--1772},
	numpages = {6},
	url = {http://doi.acm.org/10.1145/1141277.1141693},
	doi = {10.1145/1141277.1141693},
	acmid = {1141693},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {information retrieval, maintenance task assignment, mining software repositories},
} 

@inproceedings{Hooimeijer:P:ASE:2007,
	author = {Hooimeijer, Pieter and Weimer, Westley},
	title = {Modeling bug report quality},
	booktitle = {Proceedings of the twenty-second IEEE/ACM international conference on Automated software engineering},
	series = {ASE '07},
	year = {2007},
	isbn = {978-1-59593-882-4},
	location = {Atlanta, Georgia, USA},
	pages = {34--43},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1321631.1321639},
	doi = {10.1145/1321631.1321639},
	acmid = {1321639},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug report triage, information retrieval, issue tracking, statistical model},
} 

@inproceedings{Podgurski:A:ICSE:2003,
	author = {Podgurski, Andy and Leon, David and Francis, Patrick and Masri, Wes and Minch, Melinda and Sun, Jiayang and Wang, Bin},
	title = {Automated support for classifying software failure reports},
	booktitle = {Proceedings of the 25th International Conference on Software Engineering},
	series = {ICSE '03},
	year = {2003},
	isbn = {0-7695-1877-X},
	location = {Portland, Oregon},
	pages = {465--475},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=776816.776872},
	acmid = {776872},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Cubrani:D:SEKE:2004,
	title={Automatic bug triage using text categorization},
	author={{\v{C}}ubrani{\'c}, D. and Murphy, G.},
	booktitle={In SEKE 2004: Proceedings of the Sixteenth International Conference on Software Engineering \& Knowledge Engineering},
	year={2004},
	organization={Citeseer}
}

@INPROCEEDINGS{Menzies:T:ICSM:2008,
	author={Menzies, T. and Marcus, A.},
	booktitle={Software Maintenance, 2008. ICSM 2008. IEEE International Conference on}, title={Automated severity assessment of software defect reports},
	year={2008},
	month={28 2008-oct. 4},
	volume={},
	number={},
	pages={346 -355},
	keywords={NASA;automated severity assessment;machine learning techniques;mission critical systems;resource allocation;severity issue assessment;software defect reports;text mining;data mining;learning (artificial intelligence);resource allocation;software engineering;},
	doi={10.1109/ICSM.2008.4658083},
	ISSN={1063-6773},}

@inproceedings{Bettenburg:N:ETX:2007,
	author = {Bettenburg, Nicolas and Just, Sascha and Schr\"{o}ter, Adrian and Wei\ss, Cathrin and Premraj, Rahul and Zimmermann, Thomas},
	title = {Quality of bug reports in Eclipse},
	booktitle = {Proceedings of the 2007 OOPSLA workshop on eclipse technology eXchange},
	series = {eclipse '07},
	year = {2007},
	isbn = {978-1-60558-015-9},
	location = {Montreal, Quebec, Canada},
	pages = {21--25},
	numpages = {5},
	url = {http://doi.acm.org/10.1145/1328279.1328284},
	doi = {10.1145/1328279.1328284},
	acmid = {1328284},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@article{Basili:V:TSE:1996,
	author = {Basili, Victor R. and Briand, Lionel C. and Melo, Walc{\'e}lio L.},
	title = {A Validation of Object-Oriented Design Metrics as Quality Indicators},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {October 1996},
	volume = {22},
	number = {10},
	month = oct,
	year = {1996},
	issn = {0098-5589},
	pages = {751--761},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/32.544352},
	doi = {10.1109/32.544352},
	acmid = {239308},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Object-oriented design metrics, error prediction model, object-oriented software development, C++ programming language.},
} 

@article{Briand:L:TSE:1999,
	author = {Briand, Lionel C. and Daly, John W. and W\"{u}st, J\"{u}rgen K.},
	title = {A Unified Framework for Coupling Measurement in Object-Oriented Systems},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {January 1999},
	volume = {25},
	number = {1},
	month = jan,
	year = {1999},
	issn = {0098-5589},
	pages = {91--121},
	numpages = {31},
	url = {http://dx.doi.org/10.1109/32.748920},
	doi = {10.1109/32.748920},
	acmid = {297728},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Coupling, object-oriented, measurement.},
} 

@article{Emam:K:JSS:2001,
	author = {Emam, Khaled El and Melo, Walcelio and Machado, Javam C.},
	title = {The prediction of faulty classes using object-oriented design metrics},
	journal = {J. Syst. Softw.},
	issue_date = {Feb 1,2001},
	volume = {56},
	number = {1},
	month = feb,
	year = {2001},
	issn = {0164-1212},
	pages = {63--75},
	numpages = {13},
	url = {http://dx.doi.org/10.1016/S0164-1212(00)00086-8},
	doi = {10.1016/S0164-1212(00)00086-8},
	acmid = {371306},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {Java metrics, Java quality, Object-oriented metrics, Software metrics, Software quality},
} 

@article{Gyimothy:T:TSE:2005,
	author = {Gyimothy, Tibor and Ferenc, Rudolf and Siket, Istvan},
	title = {Empirical Validation of Object-Oriented Metrics on Open Source Software for Fault Prediction},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {October 2005},
	volume = {31},
	number = {10},
	month = oct,
	year = {2005},
	issn = {0098-5589},
	pages = {897--910},
	numpages = {14},
	url = {http://dx.doi.org/10.1109/TSE.2005.112},
	doi = {10.1109/TSE.2005.112},
	acmid = {1100985},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Bugzilla, C++, Columbus., Index Terms- Fact extraction, Index Terms- Fact extraction, metrics validation, reverse engineering, open source software, fault-proneness detection, Mozilla, Bugzilla, C++, compiler wrapping, Columbus., Mozilla, compiler wrapping, fault-proneness detection, metrics validation, open source software, reverse engineering},
} 

@inproceedings{Nagappan:N:ICSE:2005,
	author = {Nagappan, Nachiappan and Ball, Thomas},
	title = {Static analysis tools as early indicators of pre-release defect density},
	booktitle = {Proceedings of the 27th international conference on Software engineering},
	series = {ICSE '05},
	year = {2005},
	isbn = {1-58113-963-2},
	location = {St. Louis, MO, USA},
	pages = {580--586},
	numpages = {7},
	url = {http://doi.acm.org/10.1145/1062455.1062558},
	doi = {10.1145/1062455.1062558},
	acmid = {1062558},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {defect density, fault-proneness, static analysis tools, statistical methods},
} 

@inproceedings{Nagappan:N:ICSE:2006,
	author = {Nagappan, Nachiappan and Ball, Thomas and Zeller, Andreas},
	title = {Mining metrics to predict component failures},
	booktitle = {Proceedings of the 28th international conference on Software engineering},
	series = {ICSE '06},
	year = {2006},
	isbn = {1-59593-375-1},
	location = {Shanghai, China},
	pages = {452--461},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1134285.1134349},
	doi = {10.1145/1134285.1134349},
	acmid = {1134349},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug database, complexity metrics, empirical study, principal component analysis, regression model},
} 

@article{Ohlsson:N:TSE:1996,
	author = {Ohlsson, Niclas and Alberg, Hans},
	title = {Predicting Fault-Prone Software Modules in Telephone Switches},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {December 1996},
	volume = {22},
	number = {12},
	month = dec,
	year = {1996},
	issn = {0098-5589},
	pages = {886--894},
	numpages = {9},
	url = {http://dx.doi.org/10.1109/32.553637},
	doi = {10.1109/32.553637},
	acmid = {246143},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Complexity, empirical study, fault-prone modules, metrics, prediction, software measurement, regression analysis, software reliability, statistical analysis.},
} 

@article{Subramanyam:R:TSE:2003,
	author = {Subramanyam, Ramanath and Krishnan, M. S.},
	title = {Empirical Analysis of CK Metrics for Object-Oriented Design Complexity: Implications for Software Defects},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {April 2003},
	volume = {29},
	number = {4},
	month = apr,
	year = {2003},
	issn = {0098-5589},
	pages = {297--310},
	numpages = {14},
	url = {http://dx.doi.org/10.1109/TSE.2003.1191795},
	doi = {10.1109/TSE.2003.1191795},
	acmid = {766682},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Object-oriented design, software metrics validation, object-oriented languages, C++, Java.},
}

@inproceedings{Nagappan:2005:URC:1062455.1062514,
	author = {Nagappan, Nachiappan and Ball, Thomas},
	title = {Use of relative code churn measures to predict system defect density},
	booktitle = {Proceedings of the 27th international conference on Software engineering},
	series = {ICSE '05},
	year = {2005},
	isbn = {1-58113-963-2},
	location = {St. Louis, MO, USA},
	pages = {284--292},
	numpages = {9},
	url = {http://doi.acm.org/10.1145/1062455.1062514},
	doi = {10.1145/1062455.1062514},
	acmid = {1062514},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {defect density, fault-proneness, multiple regression, principal component analysis, relative code churn},
} 

@inproceedings{Hassan:2009:PFU:1555001.1555024,
	author = {Hassan, Ahmed E.},
	title = {Predicting faults using the complexity of code changes},
	booktitle = {Proceedings of the 31st International Conference on Software Engineering},
	series = {ICSE '09},
	year = {2009},
	isbn = {978-1-4244-3453-4},
	pages = {78--88},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2009.5070510},
	doi = {10.1109/ICSE.2009.5070510},
	acmid = {1555024},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Moser:2008:CAE:1368088.1368114,
	author = {Moser, Raimund and Pedrycz, Witold and Succi, Giancarlo},
	title = {A comparative analysis of the efficiency of change metrics and static code attributes for defect prediction},
	booktitle = {Proceedings of the 30th international conference on Software engineering},
	series = {ICSE '08},
	year = {2008},
	isbn = {978-1-60558-079-1},
	location = {Leipzig, Germany},
	pages = {181--190},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1368088.1368114},
	doi = {10.1145/1368088.1368114},
	acmid = {1368114},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {cost-sensitive classification, defect prediction, software metrics},
} 

@article{DAmbros:2012:EDP:2318097.2318149,
	author = {D'Ambros, Marco and Lanza, Michele and Robbes, Romain},
	title = {Evaluating defect prediction approaches: a benchmark and an extensive comparison},
	journal = {Empirical Softw. Engg.},
	issue_date = {August    2012},
	volume = {17},
	number = {4-5},
	month = aug,
	year = {2012},
	issn = {1382-3256},
	pages = {531--577},
	numpages = {47},
	url = {http://dx.doi.org/10.1007/s10664-011-9173-9},
	doi = {10.1007/s10664-011-9173-9},
	acmid = {2318149},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Change metrics, Defect prediction, Source code metrics},
} 



@inproceedings{Bernstein:2007:IDP:1294948.1294953,
	author = {Bernstein, Abraham and Ekanayake, Jayalath and Pinzger, Martin},
	title = {Improving defect prediction using temporal features and non linear models},
	booktitle = {Ninth international workshop on Principles of software evolution: in conjunction with the 6th ESEC/FSE joint meeting},
	series = {IWPSE '07},
	year = {2007},
	isbn = {978-1-59593-722-3},
	location = {Dubrovnik, Croatia},
	pages = {11--18},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1294948.1294953},
	doi = {10.1145/1294948.1294953},
	acmid = {1294953},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {decision tree learner, defect prediction, mining software repository},
} 


@inproceedings{Kim:2007:PFC:1248820.1248881,
	author = {Kim, Sunghun and Zimmermann, Thomas and Whitehead Jr., E. James and Zeller, Andreas},
	title = {Predicting Faults from Cached History},
	booktitle = {Proceedings of the 29th international conference on Software Engineering},
	series = {ICSE '07},
	year = {2007},
	isbn = {0-7695-2828-7},
	pages = {489--498},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICSE.2007.66},
	doi = {10.1109/ICSE.2007.66},
	acmid = {1248881},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Hassan:2005:TTL:1090952.1091858,
	author = {Hassan, Ahmed E. and Holt, Richard C.},
	title = {The Top Ten List: Dynamic Fault Prediction},
	booktitle = {Proceedings of the 21st IEEE International Conference on Software Maintenance},
	series = {ICSM '05},
	year = {2005},
	isbn = {0-7695-2368-4},
	pages = {263--272},
	numpages = {10},
	publisher = {IEEE Computer Society}
} 

@article{Arisholm:2010:SCI:1663656.1663909,
	author = {Arisholm, Erik and Briand, Lionel C. and Johannessen, Eivind B.},
	title = {A systematic and comprehensive investigation of methods to build and evaluate fault prediction models},
	journal = {J. Syst. Softw.},
	issue_date = {January, 2010},
	volume = {83},
	number = {1},
	month = jan,
	year = {2010},
	issn = {0164-1212},
	pages = {2--17},
	numpages = {16},
	url = {http://dx.doi.org/10.1016/j.jss.2009.06.055},
	doi = {10.1016/j.jss.2009.06.055},
	acmid = {1663909},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {Cost-effectiveness, Fault prediction models, Verification},
} 

@inproceedings{Binkley:1998:VCD:302163.302212,
	author = {Binkley, Aaron B. and Schach, Stephen R.},
	title = {Validation of the coupling dependency metric as a predictor of run-time failures and maintenance measures},
	booktitle = {Proceedings of the 20th international conference on Software engineering},
	series = {ICSE '98},
	year = {1998},
	isbn = {0-8186-8368-6},
	location = {Kyoto, Japan},
	pages = {452--455},
	numpages = {4},
	url = {http://dl.acm.org/citation.cfm?id=302163.302212},
	acmid = {302212},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Fenton:2000:QAF:630824.631250,
	author = {Fenton, Norman E. and Ohlsson, Niclas},
	title = {Quantitative Analysis of Faults and Failures in a Complex Software System},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {August 2000},
	volume = {26},
	number = {8},
	month = aug,
	year = {2000},
	issn = {0098-5589},
	pages = {797--814},
	numpages = {18},
	url = {http://dx.doi.org/10.1109/32.879815},
	doi = {10.1109/32.879815},
	acmid = {631250},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Software faults and failures, software metrics, empirical studies.},
} 

@Article{Jiang2016,
	author="Jiang, Siyuan
	and McMillan, Collin
	and Santelices, Raul",
	title="Do Programmers do Change Impact Analysis in Debugging?",
	journal="Empirical Software Engineering",
	year="2016",
	pages="1--39",
	abstract="``Change Impact Analysis'' is the process of determining the consequences of a modification to software. In theory, change impact analysis should be done during software maintenance, to make sure changes do not introduce new bugs. Many approaches and techniques are proposed to help programmers do change impact analysis automatically. However, it is still an open question whether and how programmers do change impact analysis. In this paper, we conducted two studies, one in-depth study and one breadth study. For the in-depth study, we recorded videos of nine professional programmers repairing two bugs for two hours. For the breadth study, we surveyed 35 professional programmers using an online system. We found that the programmers in our studies did static change impact analysis before they made changes by using IDE navigational functionalities, and they did dynamic change impact analysis after they made changes by running the programs. We also found that they did not use any change impact analysis tools.",
	issn="1573-7616",
	doi="10.1007/s10664-016-9441-9",
	url="http://dx.doi.org/10.1007/s10664-016-9441-9"
}

@article{armaly2016pragmatic,
	title={Pragmatic source code reuse via execution record and replay},
	author={Armaly, Ameer and McMillan, Collin},
	journal={Journal of Software: Evolution and Process},
	year={2016},
	publisher={Wiley Online Library}
}

@article{rodeghero2016empirical,
	title={An empirical study on how expert knowledge affects bug reports},
	author={Rodeghero, Paige and Huo, Da and Ding, Tao and McMillan, Collin and Gethers, Malcom},
	journal={Journal of Software: Evolution and Process},
	year={2016},
	publisher={Wiley Online Library}
}

@article{mcburney2016automated,
	title={Automated feature discovery via sentence selection and source code summarization},
	author={McBurney, Paul W and Liu, Cheng and McMillan, Collin},
	journal={Journal of Software: Evolution and Process},
	volume={28},
	number={2},
	pages={120--145},
	year={2016},
	publisher={Wiley Online Library}
}


@article{Jiang:2008:TEF:1416830.1416836,
	author = {Jiang, Yue and Cukic, Bojan and Ma, Yan},
	title = {Techniques for evaluating fault prediction models},
	journal = {Empirical Softw. Engg.},
	issue_date = {October   2008},
	volume = {13},
	number = {5},
	month = oct,
	year = {2008},
	issn = {1382-3256},
	pages = {561--595},
	numpages = {35},
	url = {http://dx.doi.org/10.1007/s10664-008-9079-3},
	doi = {10.1007/s10664-008-9079-3},
	acmid = {1416836},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Empirical studies, Fault-prediction models, Model evaluation, Predictive models in software engineering},
}

@article{Khoshgoftaar:1999:CSO:594380.594449,
	author = {Khoshgoftaar, Taghi M. and Allen, Edward B.},
	title = {A Comparative Study of Ordering and Classification of Fault-ProneSoftware Modules},
	journal = {Empirical Softw. Engg.},
	issue_date = {June 1999},
	volume = {4},
	number = {2},
	month = jun,
	year = {1999},
	issn = {1382-3256},
	pages = {159--186},
	numpages = {28},
	url = {http://dx.doi.org/10.1023/A:1009876418873},
	doi = {10.1023/A:1009876418873},
	acmid = {594449},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Software reliability, fault-prone modules, module-order models, multiple linear regression, nonparametric discriminant analysis, principal components analysis, software quality models},
}

@inproceedings{Koru:2007:MES:1268984.1269058,
	author = {Koru, A. Gunes and Zhang, Dongsong and Liu, Hongfang},
	title = {Modeling the Effect of Size on Defect Proneness for Open-Source Software},
	booktitle = {Proceedings of the Third International Workshop on Predictor Models in Software Engineering},
	series = {PROMISE '07},
	year = {2007},
	isbn = {0-7695-2954-2},
	pages = {10--},
	url = {http://dx.doi.org/10.1109/PROMISE.2007.9},
	doi = {10.1109/PROMISE.2007.9},
	acmid = {1269058},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Koru:2008:TRD:1416830.1416834,
	author = {Koru, A. G\"{u}ne\c{s} and Emam, Khaled El and Zhang, Dongsong and Liu, Hongfang and Mathew, Divya},
	title = {Theory of relative defect proneness},
	journal = {Empirical Softw. Engg.},
	issue_date = {October   2008},
	volume = {13},
	number = {5},
	month = oct,
	year = {2008},
	issn = {1382-3256},
	pages = {473--498},
	numpages = {26},
	url = {http://dx.doi.org/10.1007/s10664-008-9080-x},
	doi = {10.1007/s10664-008-9080-x},
	acmid = {1416834},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Open---source software, Planning for software quality assurance, Size---defect relationship, Software inspections, Software metrics, Software reviews, Software science, Software testing},
} 

@article{Lessmann:2008:BCM:1446226.1446245,
	author = {Lessmann, Stefan and Baesens, Bart and Mues, Christophe and Pietsch, Swantje},
	title = {Benchmarking Classification Models for Software Defect Prediction: A Proposed Framework and Novel Findings},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {July 2008},
	volume = {34},
	number = {4},
	month = jul,
	year = {2008},
	issn = {0098-5589},
	pages = {485--496},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/TSE.2008.35},
	doi = {10.1109/TSE.2008.35},
	acmid = {1446245},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Complexity measures, Complexity measures, Data mining, Formal methods, Statistical methods, Data mining, Formal methods, Statistical methods},
} 

@inproceedings{Mende:2010:RDP:1868328.1868336,
	author = {Mende, Thilo},
	title = {Replication of defect prediction studies: problems, pitfalls and recommendations},
	booktitle = {Proceedings of the 6th International Conference on Predictive Models in Software Engineering},
	series = {PROMISE '10},
	year = {2010},
	isbn = {978-1-4503-0404-7},
	location = {Timi\şoara, Romania},
	pages = {5:1--5:10},
	articleno = {5},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1868328.1868336},
	doi = {10.1145/1868328.1868336},
	acmid = {1868336},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {defect prediction model, replication},
} 

@inproceedings{Mende:2009:RED:1540438.1540448,
	author = {Mende, Thilo and Koschke, Rainer},
	title = {Revisiting the evaluation of defect prediction models},
	booktitle = {Proceedings of the 5th International Conference on Predictor Models in Software Engineering},
	series = {PROMISE '09},
	year = {2009},
	isbn = {978-1-60558-634-2},
	location = {Vancouver, British Columbia, Canada},
	pages = {7:1--7:10},
	articleno = {7},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1540438.1540448},
	doi = {10.1145/1540438.1540448},
	acmid = {1540448},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {cost-sensitive performance measures, defect prediction},
} 

@article{Myrtveit:2005:RVC:1069599.1069771,
	author = {Myrtveit, Ingunn and Stensrud, Erik and Shepperd, Martin},
	title = {Reliability and Validity in Comparative Studies of Software Prediction Models},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {May 2005},
	volume = {31},
	number = {5},
	month = may,
	year = {2005},
	issn = {0098-5589},
	pages = {380--391},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/TSE.2005.58},
	doi = {10.1109/TSE.2005.58},
	acmid = {1069771},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Index Terms- Software metrics, Index Terms- Software metrics, cost estimation, cross-validation, empirical methods, arbitrary function approximators, machine learning, estimation by analogy, regression analysis, simulation, reliability, validity, accuracy indicators., accuracy indicators., arbitrary function approximators, cost estimation, cross-validation, empirical methods, estimation by analogy, machine learning, regression analysis, reliability, simulation, validity},
} 

@inproceedings{Ostrand:2002:DFL:566172.566181,
	author = {Ostrand, Thomas J. and Weyuker, Elaine J.},
	title = {The distribution of faults in a large industrial software system},
	booktitle = {Proceedings of the 2002 ACM SIGSOFT international symposium on Software testing and analysis},
	series = {ISSTA '02},
	year = {2002},
	isbn = {1-58113-562-9},
	location = {Roma, Italy},
	pages = {55--64},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/566172.566181},
	doi = {10.1145/566172.566181},
	acmid = {566181},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {empirical study, fault-prone, pareto, software faults, software testing},
}

@article{Subramanyam:2003:EAC:766665.766682,
	author = {Subramanyam, Ramanath and Krishnan, M. S.},
	title = {Empirical Analysis of CK Metrics for Object-Oriented Design Complexity: Implications for Software Defects},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {April 2003},
	volume = {29},
	number = {4},
	month = apr,
	year = {2003},
	issn = {0098-5589},
	pages = {297--310},
	numpages = {14},
	url = {http://dx.doi.org/10.1109/TSE.2003.1191795},
	doi = {10.1109/TSE.2003.1191795},
	acmid = {766682},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Object-oriented design, software metrics validation, object-oriented languages, C++, Java.},
} 


@inproceedings{Zimmermann:2009:CDP:1595696.1595713,
	author = {Zimmermann, Thomas and Nagappan, Nachiappan and Gall, Harald and Giger, Emanuel and Murphy, Brendan},
	title = {Cross-project defect prediction: a large scale experiment on data vs. domain vs. process},
	booktitle = {Proceedings of the the 7th joint meeting of the European software engineering conference and the ACM SIGSOFT symposium on The foundations of software engineering},
	series = {ESEC/FSE '09},
	year = {2009},
	isbn = {978-1-60558-001-2},
	location = {Amsterdam, The Netherlands},
	pages = {91--100},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1595696.1595713},
	doi = {10.1145/1595696.1595713},
	acmid = {1595713},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {churn, cross-project, decision trees, defect prediction, logistic regression, prediction quality},
}

@inproceedings{Zimmermann:2007:PDE:1268984.1269057,
	author = {Zimmermann, Thomas and Premraj, Rahul and Zeller, Andreas},
	title = {Predicting Defects for Eclipse},
	booktitle = {Proceedings of the Third International Workshop on Predictor Models in Software Engineering},
	series = {PROMISE '07},
	year = {2007},
	isbn = {0-7695-2954-2},
	pages = {9--},
	url = {http://dx.doi.org/10.1109/PROMISE.2007.10},
	doi = {10.1109/PROMISE.2007.10},
	acmid = {1269057},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Zimmermann:2008:PDU:1368088.1368161,
	author = {Zimmermann, Thomas and Nagappan, Nachiappan},
	title = {Predicting defects using network analysis on dependency graphs},
	booktitle = {Proceedings of the 30th international conference on Software engineering},
	series = {ICSE '08},
	year = {2008},
	isbn = {978-1-60558-079-1},
	location = {Leipzig, Germany},
	pages = {531--540},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1368088.1368161},
	doi = {10.1145/1368088.1368161},
	acmid = {1368161},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {defect prediction, dependency graph, network analysis, windows server 2003},
} 

@inproceedings{Wolf:2009:PBF:1555001.1555017,
	author = {Wolf, Timo and Schroter, Adrian and Damian, Daniela and Nguyen, Thanh},
	title = {Predicting build failures using social network analysis on developer communication},
	booktitle = {Proceedings of the 31st International Conference on Software Engineering},
	series = {ICSE '09},
	year = {2009},
	isbn = {978-1-4244-3453-4},
	pages = {1--11},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2009.5070503},
	doi = {10.1109/ICSE.2009.5070503},
	acmid = {1555017},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Turhan:2009:RVC:1612763.1612782,
	author = {Turhan, Burak and Menzies, Tim and Bener, Ay\c{s}e B. and Di Stefano, Justin},
	title = {On the relative value of cross-company and within-company data for defect prediction},
	journal = {Empirical Softw. Engg.},
	issue_date = {October   2009},
	volume = {14},
	number = {5},
	month = oct,
	year = {2009},
	issn = {1382-3256},
	pages = {540--578},
	numpages = {39},
	url = {http://dx.doi.org/10.1007/s10664-008-9103-7},
	doi = {10.1007/s10664-008-9103-7},
	acmid = {1612782},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Cross-company, Defect prediction, Learning, Metrics (product metrics), Nearest-neighbor filtering, Within-company},
} 

@inproceedings{Shin:2009:CSI:1590955.1591138,
	author = {Shin, Yonghee and Bell, Robert and Ostrand, Thomas and Weyuker, Elaine},
	title = {Does calling structure information improve the accuracy of fault prediction?},
	booktitle = {Proceedings of the 2009 6th IEEE International Working Conference on Mining Software Repositories},
	series = {MSR '09},
	year = {2009},
	isbn = {978-1-4244-3493-0},
	pages = {61--70},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/MSR.2009.5069481},
	doi = {10.1109/MSR.2009.5069481},
	acmid = {1591138},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Pinzger:2008:DNP:1453101.1453105,
	author = {Pinzger, Martin and Nagappan, Nachiappan and Murphy, Brendan},
	title = {Can developer-module networks predict failures?},
	booktitle = {Proceedings of the 16th ACM SIGSOFT International Symposium on Foundations of software engineering},
	series = {SIGSOFT '08/FSE-16},
	year = {2008},
	isbn = {978-1-59593-995-1},
	location = {Atlanta, Georgia},
	pages = {2--12},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1453101.1453105},
	doi = {10.1145/1453101.1453105},
	acmid = {1453105},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {developer contribution network, failure prediction, network centrality measures, social network analysis},
} 

@inproceedings{Ostrand:2007:AAI:1273463.1273493,
	author = {Ostrand, Thomas J. and Weyuker, Elaine J. and Bell, Robert M.},
	title = {Automating algorithms for the identification of fault-prone files},
	booktitle = {Proceedings of the 2007 international symposium on Software testing and analysis},
	series = {ISSTA '07},
	year = {2007},
	isbn = {978-1-59593-734-6},
	location = {London, United Kingdom},
	pages = {219--227},
	numpages = {9},
	url = {http://doi.acm.org/10.1145/1273463.1273493},
	doi = {10.1145/1273463.1273493},
	acmid = {1273493},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {empirical study, fault-prone, prediction, regression model, software faults, software testing},
} 

@article{Ostrand:2005:PLN:1069598.1069769,
	author = {Ostrand, Thomas J. and Weyuker, Elaine J. and Bell, Robert M.},
	title = {Predicting the Location and Number of Faults in Large Software Systems},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {April 2005},
	volume = {31},
	number = {4},
	month = apr,
	year = {2005},
	issn = {0098-5589},
	pages = {340--355},
	numpages = {16},
	url = {http://dx.doi.org/10.1109/TSE.2005.49},
	doi = {10.1109/TSE.2005.49},
	acmid = {1069769},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Index Terms- Software faults, Index Terms- Software faults, fault-prone, prediction, regression model, empirical study, software testing., empirical study, fault-prone, prediction, regression model, software testing.},
} 

@inproceedings{Ostrand:2004:BUG:1007512.1007524,
	author = {Ostrand, Thomas J. and Weyuker, Elaine J. and Bell, Robert M.},
	title = {Where the bugs are},
	booktitle = {Proceedings of the 2004 ACM SIGSOFT international symposium on Software testing and analysis},
	series = {ISSTA '04},
	year = {2004},
	isbn = {1-58113-820-2},
	location = {Boston, Massachusetts, USA},
	pages = {86--96},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1007512.1007524},
	doi = {10.1145/1007512.1007524},
	acmid = {1007524},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {empirical study, fault-prone, prediction, regression model, software faults, software testing},
} 

@inproceedings{Neuhaus:2007:PVS:1315245.1315311,
	author = {Neuhaus, Stephan and Zimmermann, Thomas and Holler, Christian and Zeller, Andreas},
	title = {Predicting vulnerable software components},
	booktitle = {Proceedings of the 14th ACM conference on Computer and communications security},
	series = {CCS '07},
	year = {2007},
	isbn = {978-1-59593-703-2},
	location = {Alexandria, Virginia, USA},
	pages = {529--540},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1315245.1315311},
	doi = {10.1145/1315245.1315311},
	acmid = {1315311},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {prediction, software security},
} 


@inproceedings{Nikora:2003:DFP:942804.943747,
	author = {Nikora, Allen P. and Munson, John C.},
	title = {Developing Fault Predictors for Evolving Software Systems},
	booktitle = {Proceedings of the 9th International Symposium on Software Metrics},
	series = {METRICS '03},
	year = {2003},
	isbn = {0-7695-1987-3},
	pages = {338--},
	url = {http://dl.acm.org/citation.cfm?id=942804.943747},
	acmid = {943747},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {defect content estimation techniques, fault prediction, software metrics, software measurement frameworks, software quality models},
}

@article{Menzies:2010:DPS:1842512.1842517,
	author = {Menzies, Tim and Milton, Zach and Turhan, Burak and Cukic, Bojan and Jiang, Yue and Bener, Ay\c{s}e},
	title = {Defect prediction from static code features: current results, limitations, new approaches},
	journal = {Automated Software Engg.},
	issue_date = {December  2010},
	volume = {17},
	number = {4},
	month = dec,
	year = {2010},
	issn = {0928-8910},
	pages = {375--407},
	numpages = {33},
	url = {http://dx.doi.org/10.1007/s10515-010-0069-5},
	doi = {10.1007/s10515-010-0069-5},
	acmid = {1842517},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Defect prediction, Static code features, WHICH},
}

@article{Menzies:2007:DMS:1248721.1248734,
	author = {Menzies, Tim and Greenwald, Jeremy and Frank, Art},
	title = {Data Mining Static Code Attributes to Learn Defect Predictors},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {January 2007},
	volume = {33},
	number = {1},
	month = jan,
	year = {2007},
	issn = {0098-5589},
	pages = {2--13},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/TSE.2007.10},
	doi = {10.1109/TSE.2007.10},
	acmid = {1248734},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Data mining detect prediction, Data mining detect prediction, McCabe, Halstead, artifical intelligence, empirical, naive Bayes., Halstead, McCabe, artifical intelligence, empirical, naive Bayes.},
} 

@inproceedings{Mende:2010:EDP:1955601.1955974,
	author = {Mende, Thilo and Koschke, Rainer},
	title = {Effort-Aware Defect Prediction Models},
	booktitle = {Proceedings of the 2010 14th European Conference on Software Maintenance and Reengineering},
	series = {CSMR '10},
	year = {2010},
	isbn = {978-0-7695-4321-5},
	pages = {107--116},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/CSMR.2010.18},
	doi = {10.1109/CSMR.2010.18},
	acmid = {1955974},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {Defect Prediction Models, Evaluation, Cost-Benefits},
} 

@inproceedings{Khoshgoftaar:1996:DSM:851006.856044,
	author = {Khoshgoftaar, T. M. and Allen, E. B. and Goel, N. and Nandi, A. and McMullan, J.},
	title = {Detection of software modules with high debug code churn in a very large legacy system},
	booktitle = {Proceedings of the The Seventh International Symposium on Software Reliability Engineering},
	series = {ISSRE '96},
	year = {1996},
	isbn = {0-8186-7707-4},
	pages = {364--},
	url = {http://dl.acm.org/citation.cfm?id=851006.856044},
	acmid = {856044},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {bug fixes, consecutive releases, discriminant analysis, fault counts, fault prone modules, fit data set, high debug code churn, realistic simulation, reliable telecommunications, reuse history, software module detection, static software product metrics, telecommunication computing, telecommunications software, test data set, unexpected problems, very large legacy system},
}

@inproceedings{Kamei:2010:RCB:1912607.1913298,
	author = {Kamei, Yasutaka and Matsumoto, Shinsuke and Monden, Akito and Matsumoto, Ken-ichi and Adams, Bram and Hassan, Ahmed E.},
	title = {Revisiting common bug prediction findings using effort-aware models},
	booktitle = {Proceedings of the 2010 IEEE International Conference on Software Maintenance},
	series = {ICSM '10},
	year = {2010},
	isbn = {978-1-4244-8630-4},
	pages = {1--10},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICSM.2010.5609530},
	doi = {10.1109/ICSM.2010.5609530},
	acmid = {1913298},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Graves:2000:PFI:347489.347496,
	author = {Graves, Todd L. and Karr, Alan F. and Marron, J. S. and Siy, Harvey},
	title = {Predicting Fault Incidence Using Software Change History},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {July 2000},
	volume = {26},
	number = {7},
	month = jul,
	year = {2000},
	issn = {0098-5589},
	pages = {653--661},
	numpages = {9},
	url = {http://dx.doi.org/10.1109/32.859533},
	doi = {10.1109/32.859533},
	acmid = {347496},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Fault potential, code decay, change management data, metrics, statistical analysis, generalized linear models.},
} 

@inproceedings{Bacchelli:2010:PCM:2128562.2128570,
	author = {Bacchelli, Alberto and D'Ambros, Marco and Lanza, Michele},
	title = {Are popular classes more defect prone?},
	booktitle = {Proceedings of the 13th international conference on Fundamental Approaches to Software Engineering},
	series = {FASE'10},
	year = {2010},
	isbn = {3-642-12028-8, 978-3-642-12028-2},
	location = {Paphos, Cyprus},
	pages = {59--73},
	numpages = {15},
	url = {http://dx.doi.org/10.1007/978-3-642-12029-9_5},
	doi = {10.1007/978-3-642-12029-9_5},
	acmid = {2128570},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
} 

@inproceedings{Arnaoudova:2010:PCI:1912607.1913343,
	author = {Arnaoudova, Venera and Eshkevari, Laleh and Oliveto, Rocco and Gueheneuc, Yann-Gael and Antoniol, Giuliano},
	title = {Physical and conceptual identifier dispersion: Measures and relation to fault proneness},
	booktitle = {Proceedings of the 2010 IEEE International Conference on Software Maintenance},
	series = {ICSM '10},
	year = {2010},
	isbn = {978-1-4244-8630-4},
	pages = {1--5},
	numpages = {5},
	url = {http://dx.doi.org/10.1109/ICSM.2010.5609748},
	doi = {10.1109/ICSM.2010.5609748},
	acmid = {1913343},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Arisholm:2006:PFC:1159733.1159738,
	author = {Arisholm, Erik and Briand, Lionel C.},
	title = {Predicting fault-prone components in a java legacy system},
	booktitle = {Proceedings of the 2006 ACM/IEEE international symposium on Empirical software engineering},
	series = {ISESE '06},
	year = {2006},
	isbn = {1-59593-218-6},
	location = {Rio de Janeiro, Brazil},
	pages = {8--17},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1159733.1159738},
	doi = {10.1145/1159733.1159738},
	acmid = {1159738},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Marks:2011:SFB:2020390.2020401,
	author = {Marks, Lionel and Zou, Ying and Hassan, Ahmed E.},
	title = {Studying the fix-time for bugs in large open source projects},
	booktitle = {Proceedings of the 7th International Conference on Predictive Models in Software Engineering},
	series = {Promise '11},
	year = {2011},
	isbn = {978-1-4503-0709-3},
	location = {Banff, Alberta, Canada},
	pages = {11:1--11:8},
	articleno = {11},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/2020390.2020401},
	doi = {10.1145/2020390.2020401},
	acmid = {2020401},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug fix-time, empirical software engineering, mining software repositories},
} 

@article{Anvik:J:TOSEM:2011,
	title={Reducing the effort of bug report triage: Recommenders for development-oriented decisions},
	author={Anvik, J. and Murphy, G.C.},
	journal={ACM Transactions on Software Engineering and Methodology (TOSEM)},
	volume={20},
	number={3},
	pages={10},
	year={2011},
	publisher={ACM}
}

@article{Hofman:2011:BES:1968922.1968960,
	author = {Hofman, Rados\law},
	title = {Behavioral economics in software quality engineering},
	journal = {Empirical Softw. Engg.},
	issue_date = {April     2011},
	volume = {16},
	number = {2},
	month = apr,
	year = {2011},
	issn = {1382-3256},
	pages = {278--293},
	numpages = {16},
	url = {http://dx.doi.org/10.1007/s10664-010-9140-x},
	doi = {10.1007/s10664-010-9140-x},
	acmid = {1968960},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Behavioral economics, Cognitive psychology, Quality perception, Software},
} 

@inproceedings{Ko:2012:MWS:2212776.2212797,
	author = {Ko, Andrew},
	title = {Mining whining in support forums with frictionary},
	booktitle = {CHI '12 Extended Abstracts on Human Factors in Computing Systems},
	series = {CHI EA '12},
	year = {2012},
	isbn = {978-1-4503-1016-1},
	location = {Austin, Texas, USA},
	pages = {191--200},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/2212776.2212797},
	doi = {10.1145/2212776.2212797},
	acmid = {2212797},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bugs, software problems, support, topic extraction},
} 

@article{Stavrinoudis:2005:EEU:1059832.1059836,
	author = {Stavrinoudis, Dimitris and Xenos, Michalis and Peppas, Pavlos and Christodoulakis, Dimitris},
	title = {Early Estimation of Users' Perception of Software Quality},
	journal = {Software Quality Control},
	issue_date = {June 2005},
	volume = {13},
	number = {2},
	month = jun,
	year = {2005},
	issn = {0963-9314},
	pages = {155--175},
	numpages = {21},
	url = {http://dx.doi.org/10.1007/s11219-005-6215-9},
	doi = {10.1007/s11219-005-6215-9},
	acmid = {1059836},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Grove's System of Spheres, ISO9126, belief revision, quality characteristics, software quality measurements, users' opinion},
} 

@inproceedings{Xenos:1994:SQU:646294.687542,
	author = {Xenos, Michalis Nik and Christodoulakis, D.},
	title = {Software Quality: The User's Point of View},
	booktitle = {Software Quality and Productivity: Theory, practice and training},
	year = {1995},
	isbn = {0-412-62960-7},
	pages = {266--272},
	numpages = {7},
	url = {http://dl.acm.org/citation.cfm?id=646294.687542},
	acmid = {687542},
	publisher = {Chapman \& Hall, Ltd.},
	address = {London, UK, UK},
} 

@inproceedings{Mockus:2005:PCP:1062455.1062506,
	author = {Mockus, Audris and Zhang, Ping and Li, Paul Luo},
	title = {Predictors of customer perceived software quality},
	booktitle = {Proceedings of the 27th international conference on Software engineering},
	series = {ICSE '05},
	year = {2005},
	isbn = {1-58113-963-2},
	location = {St. Louis, MO, USA},
	pages = {225--233},
	numpages = {9},
	url = {http://doi.acm.org/10.1145/1062455.1062506},
	doi = {10.1145/1062455.1062506},
	acmid = {1062506},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {metrics, modeling, quality},
} 

@article{Morris:1997:UPI:624620.625741,
	author = {Morris, Michael G. and Dillon, Andrew},
	title = {How User Perceptions Influence Software Use},
	journal = {IEEE Softw.},
	issue_date = {July 1997},
	volume = {14},
	number = {4},
	month = jul,
	year = {1997},
	issn = {0740-7459},
	pages = {58--65},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/52.595956},
	doi = {10.1109/52.595956},
	acmid = {625741},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{Chilana:2010:UEU:1915084.1916371,
	author = {Chilana, Parmit K. and Ko, Andrew J. and Wobbrock, Jacob O.},
	title = {Understanding Expressions of Unwanted Behaviors in Open Bug Reporting},
	booktitle = {Proceedings of the 2010 IEEE Symposium on Visual Languages and Human-Centric Computing},
	series = {VLHCC '10},
	year = {2010},
	isbn = {978-0-7695-4206-5},
	pages = {203--206},
	numpages = {4},
	url = {http://dx.doi.org/10.1109/VLHCC.2010.35},
	doi = {10.1109/VLHCC.2010.35},
	acmid = {1916371},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {open bug reporting, user expectations, software behavior},
} 

@book{langville2009google,
	title={Google's PageRank and beyond: The science of search engine rankings},
	author={Langville, A.N. and Meyer, C.D.},
	year={2009},
	publisher={Princeton University Press}
}

@article{chang2010hierarchical,
	title={Hierarchical relational models for document networks},
	author={Chang, J. and Blei, D.M.},
	journal={The Annals of Applied Statistics},
	volume={4},
	number={1},
	pages={124--150},
	year={2010},
	publisher={Institute of Mathematical Statistics}
}

@inproceedings{Nagappan:2010:CBD:1913797.1914387,
	author = {Nagappan, Nachiappan and Zeller, Andreas and Zimmermann, Thomas and Herzig, Kim and Murphy, Brendan},
	title = {Change Bursts as Defect Predictors},
	booktitle = {Proceedings of the 2010 IEEE 21st International Symposium on Software Reliability Engineering},
	series = {ISSRE '10},
	year = {2010},
	isbn = {978-0-7695-4255-3},
	pages = {309--318},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ISSRE.2010.25},
	doi = {10.1109/ISSRE.2010.25},
	acmid = {1914387},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {Process metrics, product metrics, software quality assurance, version control, change history, defects, developers, software mining, empirical studies},
} 

@inproceedings{Zhang:2011:CSD:2001420.2001463,
	author = {Zhang, Sai and Saff, David and Bu, Yingyi and Ernst, Michael D.},
	title = {Combined static and dynamic automated test generation},
	booktitle = {Proceedings of the 2011 International Symposium on Software Testing and Analysis},
	series = {ISSTA '11},
	year = {2011},
	isbn = {978-1-4503-0562-4},
	location = {Toronto, Ontario, Canada},
	pages = {353--363},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2001420.2001463},
	doi = {10.1145/2001420.2001463},
	acmid = {2001463},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {automated test generation, dynamic analyses, static},
} 

@article{Sebastiani:2002:MLA:505282.505283,
	author = {Sebastiani, Fabrizio},
	title = {Machine learning in automated text categorization},
	journal = {ACM Comput. Surv.},
	issue_date = {March 2002},
	volume = {34},
	number = {1},
	month = mar,
	year = {2002},
	issn = {0360-0300},
	pages = {1--47},
	numpages = {47},
	url = {http://doi.acm.org/10.1145/505282.505283},
	doi = {10.1145/505282.505283},
	acmid = {505283},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Machine learning, text categorization, text classification},
} 

@article{Jain:2010:DCY:1755267.1755654,
	author = {Jain, Anil K.},
	title = {Data clustering: 50 years beyond K-means},
	journal = {Pattern Recogn. Lett.},
	issue_date = {June, 2010},
	volume = {31},
	number = {8},
	month = jun,
	year = {2010},
	issn = {0167-8655},
	pages = {651--666},
	numpages = {16},
	url = {http://dx.doi.org/10.1016/j.patrec.2009.09.011},
	doi = {10.1016/j.patrec.2009.09.011},
	acmid = {1755654},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {Data clustering, Historical developments, King-Sun Fu prize, Perspectives on clustering, User's dilemma},
} 

@inproceedings{McMillan:2011:CSA:2117694.2119646,
	author = {McMillan, Collin and Linares-Vasquez, Mario and Poshyvanyk, Denys and Grechanik, Mark},
	title = {Categorizing software applications for maintenance},
	booktitle = {Proceedings of the 2011 27th IEEE International Conference on Software Maintenance},
	series = {ICSM '11},
	year = {2011},
	isbn = {978-1-4577-0663-9},
	pages = {343--352},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICSM.2011.6080801},
	doi = {10.1109/ICSM.2011.6080801},
	acmid = {2119646},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Luhn:1958:ACL:1662353.1662360,
	author = {Luhn, H. P.},
	title = {The automatic creation of literature abstracts},
	journal = {IBM J. Res. Dev.},
	issue_date = {April 1958},
	volume = {2},
	number = {2},
	month = apr,
	year = {1958},
	issn = {0018-8646},
	pages = {159--165},
	numpages = {7},
	url = {http://dx.doi.org/10.1147/rd.22.0159},
	doi = {10.1147/rd.22.0159},
	acmid = {1662360},
	publisher = {IBM Corp.},
	address = {Riverton, NJ, USA},
} 

@inproceedings{Goldstein:2000:MSS:1117575.1117580,
	author = {Goldstein, Jade and Mittal, Vibhu and Carbonell, Jaime and Kantrowitz, Mark},
	title = {Multi-document summarization by sentence extraction},
	booktitle = {Proceedings of the 2000 NAACL-ANLPWorkshop on Automatic summarization - Volume 4},
	series = {NAACL-ANLP-AutoSum '00},
	year = {2000},
	location = {Seattle, Washington},
	pages = {40--48},
	numpages = {9},
	url = {http://dx.doi.org/10.3115/1117575.1117580},
	doi = {10.3115/1117575.1117580},
	acmid = {1117580},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
} 

@article{Knight200291,
	title = "Summarization beyond sentence extraction: A probabilistic approach to sentence compression",
	journal = "Artificial Intelligence",
	volume = "139",
	number = "1",
	pages = "91 - 107",
	year = "2002",
	note = "",
	issn = "0004-3702",
	doi = "10.1016/S0004-3702(02)00222-9",
	url = "http://www.sciencedirect.com/science/article/pii/S0004370202002229",
	author = "Kevin Knight and Daniel Marcu",
	keywords = "Summarization",
	keywords = "Compression",
	keywords = "Noisy-channel model"
}

@inproceedings{Sridhara:2010:TAG:1858996.1859006,
	author = {Sridhara, Giriprasad and Hill, Emily and Muppaneni, Divya and Pollock, Lori and Vijay-Shanker, K.},
	title = {Towards automatically generating summary comments for Java methods},
	booktitle = {Proceedings of the IEEE/ACM international conference on Automated software engineering},
	series = {ASE '10},
	year = {2010},
	isbn = {978-1-4503-0116-9},
	location = {Antwerp, Belgium},
	pages = {43--52},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1858996.1859006},
	doi = {10.1145/1858996.1859006},
	acmid = {1859006},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {comment generation, method summarization, natural language program analysis},
}

@inproceedings{Aponte:2011:ITL:1987856.1987867,
	author = {Aponte, Jairo and Marcus, Andrian},
	title = {Improving traceability link recovery methods through software artifact summarization},
	booktitle = {Proceedings of the 6th International Workshop on Traceability in Emerging Forms of Software Engineering},
	series = {TEFSE '11},
	year = {2011},
	isbn = {978-1-4503-0589-1},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {46--49},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1987856.1987867},
	doi = {10.1145/1987856.1987867},
	acmid = {1987867},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {information retrieval, program comprehension, summarization, traceability management},
} 

@article{Powers_2011, 
	title={EVALUATION : FROM PRECISION , RECALL AND F-MEASURE TO ROC , INFORMEDNESS , MARKEDNESS \& CORRELATION}, 
	volume={2}, 
	number={1}, 
	journal={Journal of Machine Learning Technologies}, 
	author={Powers, David M W}, 
	year={2011}, 
	pages={37--63}}

@inproceedings{Grechanik:2010:SEF:1806799.1806868,
	author = {Grechanik, Mark and Fu, Chen and Xie, Qing and McMillan, Collin and Poshyvanyk, Denys and Cumby, Chad},
	title = {A search engine for finding highly relevant applications},
	booktitle = {Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering},
	series = {ICSE '10},
	year = {2010},
	isbn = {978-1-60558-719-6},
	location = {Cape Town, South Africa},
	pages = {475--484},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1806799.1806868},
	doi = {10.1145/1806799.1806868},
	acmid = {1806868},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Grechanik:2010:EIL:1852786.1852801,
	author = {Grechanik, Mark and McMillan, Collin and DeFerrari, Luca and Comi, Marco and Crespi, Stefano and Poshyvanyk, Denys and Fu, Chen and Xie, Qing and Ghezzi, Carlo},
	title = {An empirical investigation into a large-scale Java open source code repository},
	booktitle = {Proceedings of the 2010 ACM-IEEE International Symposium on Empirical Software Engineering and Measurement},
	series = {ESEM '10},
	year = {2010},
	isbn = {978-1-4503-0039-1},
	location = {Bolzano-Bozen, Italy},
	pages = {11:1--11:10},
	articleno = {11},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1852786.1852801},
	doi = {10.1145/1852786.1852801},
	acmid = {1852801},
	publisher = {ACM},
	address = {New York, NY, USA}
} 

@inproceedings{Dagenais:2010:MNS:1806799.1806842,
	author = {Dagenais, Barth{\'e}l{\'e}my and Ossher, Harold and Bellamy, Rachel K. E. and Robillard, Martin P. and de Vries, Jacqueline P.},
	title = {Moving into a new software project landscape},
	booktitle = {Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering - Volume 1},
	series = {ICSE '10},
	year = {2010},
	isbn = {978-1-60558-719-6},
	location = {Cape Town, South Africa},
	pages = {275--284},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1806799.1806842},
	doi = {10.1145/1806799.1806842},
	acmid = {1806842},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@article{vonKrogh20031217,
	title = "Community, joining, and specialization in open source software innovation: a case study",
	journal = "Research Policy",
	volume = "32",
	number = "7",
	pages = "1217 - 1241",
	year = "2003",
	note = "<ce:title>Open Source Software Development</ce:title>",
	issn = "0048-7333",
	doi = "10.1016/S0048-7333(03)00050-7",
	url = "http://www.sciencedirect.com/science/article/pii/S0048733303000507",
	author = "Georg von Krogh and Sebastian Spaeth and Karim R Lakhani",
	keywords = "Open source software",
	keywords = "Innovation",
	keywords = "Community",
	keywords = "Collective action",
	keywords = "Virtual teams"
}
@inproceedings{5306335,
	author={Starke, J. and Luce, C. and Sillito, J.},
	booktitle={Software Maintenance, 2009. ICSM 2009. IEEE International Conference on},
	title={Searching and skimming: An exploratory study},
	year={2009},
	pages={157-166},
	keywords={software engineering;program comprehension;software system;source code search tools;Concrete;Data analysis;Information analysis;Java;Laboratories;Navigation;Programming profession;Software design;Software systems;Software tools},
	doi={10.1109/ICSM.2009.5306335},
	ISSN={1063-6773}
}

@inproceedings{Clause:2007:DGD:1273463.1273490,
	author = {Clause, James and Li, Wanchun and Orso, Alessandro},
	title = {Dytan: a generic dynamic taint analysis framework},
	booktitle = {Proceedings of the 2007 international symposium on Software testing and analysis},
	series = {ISSTA '07},
	year = {2007},
	isbn = {978-1-59593-734-6},
	location = {London, United Kingdom},
	pages = {196--206},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1273463.1273490},
	doi = {10.1145/1273463.1273490},
	acmid = {1273490},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {dynamic tainting, general framework, information flow},
} 

@inproceedings{Chan:2012:SCA:2393596.2393606,
	author = {Chan, Wing-Kwan and Cheng, Hong and Lo, David},
	title = {Searching connected API subgraph via text phrases},
	booktitle = {Proceedings of the ACM SIGSOFT 20th International Symposium on the Foundations of Software Engineering},
	series = {FSE '12},
	year = {2012},
	isbn = {978-1-4503-1614-9},
	location = {Cary, North Carolina},
	pages = {10:1--10:11},
	articleno = {10},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2393596.2393606},
	doi = {10.1145/2393596.2393606},
	acmid = {2393606},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {API graph, API recommendation, subgraph searching},
} 

@article{Shackelford:2006:CCO:1124706.1121482,
	author = {Shackelford, Russell and McGettrick, Andrew and Sloan, Robert and Topi, Heikki and Davies, Gordon and Kamali, Reza and Cross, James and Impagliazzo, John and LeBlanc, Richard and Lunt, Barry},
	title = {Computing Curricula 2005: The Overview Report},
	journal = {SIGCSE Bull.},
	issue_date = {March 2006},
	volume = {38},
	number = {1},
	month = mar,
	year = {2006},
	issn = {0097-8418},
	pages = {456--457},
	numpages = {2},
	url = {http://doi.acm.org/10.1145/1124706.1121482},
	doi = {10.1145/1124706.1121482},
	acmid = {1121482},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {comparison of curriculum, computer engineering curriculum, computer science curriculum, computing curricula, information systems curriculum, information technology curriculum, software engineering curriculum},
} 

@book{Rajlich:2011:SEC:2077657,
	author = {Rajlich, Vaclav},
	title = {Software Engineering: The Current Practice},
	year = {2011},
	isbn = {1439841225, 9781439841228},
	edition = {1st},
	publisher = {Chapman \& Hall/CRC},
}

@article{10.1109/HICSS.2005.378,
	author = {Georg von Krogh and Sebastian Spaeth and Stefan Haefliger},
	title = {Knowledge Reuse in Open Source Software: An Exploratory Study of 15 Open Source Projects},
	journal ={Hawaii International Conference on System Sciences},
	volume = {7},
	issn = {1530-1605},
	year = {2005},
	pages = {198b},
	doi = {http://doi.ieeecomputersociety.org/10.1109/HICSS.2005.378},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{McMillan:2011:CSA:2117694.2119646,
	author = {McMillan, Collin and Linares-Vasquez, Mario and Poshyvanyk, Denys and Grechanik, Mark},
	title = {Categorizing software applications for maintenance},
	booktitle = {Proceedings of the 2011 27th IEEE International Conference on Software Maintenance},
	series = {ICSM '11},
	year = {2011},
	isbn = {978-1-4577-0663-9},
	pages = {343--352},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICSM.2011.6080801},
	doi = {10.1109/ICSM.2011.6080801},
	acmid = {2119646},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Grechanik:2010:EIL:1852786.1852801,
	author = {Grechanik, Mark and McMillan, Collin and DeFerrari, Luca and Comi, Marco and Crespi, Stefano and Poshyvanyk, Denys and Fu, Chen and Xie, Qing and Ghezzi, Carlo},
	title = {An empirical investigation into a large-scale Java open source code repository},
	booktitle = {Proceedings of the 2010 ACM-IEEE International Symposium on Empirical Software Engineering and Measurement},
	series = {ESEM '10},
	year = {2010},
	isbn = {978-1-4503-0039-1},
	location = {Bolzano-Bozen, Italy},
	pages = {11:1--11:10},
	articleno = {11},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1852786.1852801},
	doi = {10.1145/1852786.1852801},
	acmid = {1852801},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {empirical study, large-scale software, mining software repositories, open source, patterns, practice, software repository},
}

@inproceedings{Agichtein:2006:LUI:1148170.1148175,
	author = {Agichtein, Eugene and Brill, Eric and Dumais, Susan and Ragno, Robert},
	title = {Learning user interaction models for predicting web search result preferences},
	booktitle = {Proceedings of the 29th annual international ACM SIGIR conference on Research and development in information retrieval},
	series = {SIGIR '06},
	year = {2006},
	isbn = {1-59593-369-7},
	location = {Seattle, Washington, USA},
	pages = {3--10},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1148170.1148175},
	doi = {10.1145/1148170.1148175},
	acmid = {1148175},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {interpreting implicit relevance feedback, predicting relevance preferences, user behavior modeling},
} 

@article{Claypool:2001:IUI:613351.613651,
	author = {Claypool, Mark and Brown, David and Le, Phong and Waseda, Makoto},
	title = {Inferring User Interest},
	journal = {IEEE Internet Computing},
	issue_date = {November 2001},
	volume = {5},
	number = {6},
	month = nov,
	year = {2001},
	issn = {1089-7801},
	pages = {32--39},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/4236.968829},
	doi = {10.1109/4236.968829},
	acmid = {613651},
	publisher = {IEEE Educational Activities Department},
	address = {Piscataway, NJ, USA},
} 

@book{IR:08,
	author = {Manning, Christopher D. and Raghavan, Prabhakar and Schtze, Hinrich},
	title = {Introduction to Information Retrieval},
	year = {2008},
	isbn = {0521865719, 9780521865715},
	publisher = {Cambridge University Press},
	address = {New York, NY, USA}
}

@article{Likert1932,
	author = {Likert, R.A.},
	title= {A technique for the measurement of attitudes},
	year = {1932},
	journal = {Archives of Psychology},
	volume = {22},
	number = {140},
	pages = {5-55},
}

@inproceedings{Antoniol:2000:IRM:850948.853428,
	author = {Antoniol, G. and Canfora, G. and de Lucia, A. and Casazza, G.},
	title = {Information Retrieval Models for Recovering Traceability Links Between Code and Documentation},
	booktitle = {Proceedings of the International Conference on Software Maintenance (ICSM'00)},
	series = {ICSM '00},
	year = {2000},
	isbn = {0-7695-0753-0},
	pages = {40--},
	url = {http://dl.acm.org/citation.cfm?id=850948.853428},
	acmid = {853428},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@article{Deerwester:jasis1990,
	Author = {S. Deerwester and S. T. Dumais and G. W. Furnas and T. K. Landauer and R. Harshman},
	Date-Added = {2007-08-31 12:57:51 +0200},
	Date-Modified = {2007-08-31 12:57:51 +0200},
	Journal = {Journal of the American Society for Information Science},
	Number = {6},
	Pages = {391-407},
	Title = {Indexing by Latent Semantic Analysis},
	Volume = {41},
	Year = {1990}
}

@inproceedings{Marcus:icse2003,
	Author = {A. Marcus and J. I. Maletic},
	Booktitle = {Proceedings of 25th International Conference on Software Engineering},
	Date-Added = {2007-08-31 12:57:51 +0200},
	Date-Modified = {2010-02-19 22:36:39 +0100},
	Pages = {125-135},
	Title = {Recovering Documentation-to-Source-Code Traceability Links using Latent Semantic Indexing},
	Year = {2003}
}

@book{Baeza-Yates:1999,
	Author = {R. Baeza-Yates and B. Ribeiro-Neto},
	Date-Added = {2007-08-31 12:57:51 +0200},
	Date-Modified = {2007-08-31 12:57:51 +0200},
	Publisher = {Addison-Wesley},
	Title = {Modern Information Retrieval},
	Year = {1999}
}

@article{Landi:1992:USA:161494.161501,
	author = {Landi, William},
	title = {Undecidability of static analysis},
	journal = {ACM Lett. Program. Lang. Syst.},
	issue_date = {Dec. 1992},
	volume = {1},
	number = {4},
	month = dec,
	year = {1992},
	issn = {1057-4514},
	pages = {323--337},
	numpages = {15},
	url = {http://doi.acm.org/10.1145/161494.161501},
	doi = {10.1145/161494.161501},
	acmid = {161501},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {abstract interpretation, alias analysis, data flow analysis, halting problem, static analysis},
}

@inproceedings{Biggerstaff:1993:CAP:257572.257679,
	author = {Biggerstaff, Ted J. and Mitbander, Bharat G. and Webster, Dallas},
	title = {The concept assignment problem in program understanding},
	booktitle = {Proceedings of the 15th international conference on Software Engineering},
	series = {ICSE '93},
	year = {1993},
	isbn = {0-89791-588-7},
	location = {Baltimore, Maryland, United States},
	pages = {482--498},
	numpages = {17},
	url = {http://dl.acm.org/citation.cfm?id=257572.257679},
	acmid = {257679},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
	keywords = {concept recognition, connectionist, domain, knowledge base, plausible reasoning, reverse engineering, slicing},
}

@article{Knight:1998:SQT:590631.590635,
	author = {Knight, John C. and Dunn, Michael F.},
	title = {Software quality through domain-driven certification},
	journal = {Ann. Softw. Eng.},
	issue_date = {1998},
	volume = {5},
	month = jan,
	year = {1998},
	issn = {1022-7091},
	pages = {293--315},
	numpages = {23},
	url = {http://dl.acm.org/citation.cfm?id=590631.590635},
	acmid = {590635},
	publisher = {J. C. Baltzer AG, Science Publishers},
	address = {Red Bank, NJ, USA},
}

@ARTICLE{62928,
	author={Barns, B.H. and Bollinger, T.B.},
	journal={Software, IEEE}, title={Making reuse cost-effective},
	year={1991},
	month={jan. },
	volume={8},
	number={1},
	pages={13 -24},
	keywords={consumer reuse;human problem solving;management;quality-of-investment;reuse investments;software reuse;DP management;software reusability;},
	doi={10.1109/52.62928},
	ISSN={0740-7459},}

@article{Banker:1991:RPI:120901.120908,
	author = {Banker, Rajiv D. and Kauffman, Robert J.},
	title = {Reuse and productivity in integrated computer-aided software engineering: an empirical study},
	journal = {MIS Q.},
	issue_date = {Sept. 1991},
	volume = {15},
	number = {3},
	month = oct,
	year = {1991},
	issn = {0276-7783},
	pages = {375--401},
	numpages = {27},
	url = {http://dx.doi.org/10.2307/249649},
	doi = {10.2307/249649},
	acmid = {120908},
	publisher = {Society for Information Management and The Management Information Systems Research Center},
	address = {Minneapolis, MN, USA},
	keywords = {CASE, ICASE, productivity measurement, reuse, software development, software economics, software engineering},
}

@article{10.1109/TSE.2011.84,
	author = {Collin McMillan and Mark Grechanik and Denys Poshyvanyk and Chen Fu and Qing Xie},
	title = {Exemplar: A Source Code Search Engine For Finding Highly Relevant Applications},
	journal ={IEEE Transactions on Software Engineering},
	volume = {99},
	number = {PrePrints},
	issn = {0098-5589},
	year = {2011},
	doi = {http://doi.ieeecomputersociety.org/10.1109/TSE.2011.84},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{Grechanik:2010:SEF:1806799.1806868,
	author = {Grechanik, Mark and Fu, Chen and Xie, Qing and McMillan, Collin and Poshyvanyk, Denys and Cumby, Chad},
	title = {A search engine for finding highly relevant applications},
	booktitle = {Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering - Volume 1},
	series = {ICSE '10},
	year = {2010},
	isbn = {978-1-60558-719-6},
	location = {Cape Town, South Africa},
	pages = {475--484},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1806799.1806868},
	doi = {10.1145/1806799.1806868},
	acmid = {1806868},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{McMillan:2011:PFR:1985793.1985809,
	author = {McMillan, Collin and Grechanik, Mark and Poshyvanyk, Denys and Xie, Qing and Fu, Chen},
	title = {Portfolio: finding relevant functions and their usage},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {111--120},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985809},
	doi = {10.1145/1985793.1985809},
	acmid = {1985809},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {code search, function call graph, pagerank, portfolio, ranking},
} 

@article{McMillan:Portfolio:TOSEM,
	author = {Collin McMillan and Mark Grechanik and Denys Poshyvanyk and Qing Xie and Chen Fu},
	title = {Searching for Relevant Functions and Their Usages in Millions of Lines of Code},
	journal ={ACM Transactions on Software Engineering and Methodology},
	year = {2012},
	doi = {http://doi.ieeecomputersociety.org/10.1109/TSE.2011.84},
	publisher = {ACM},
	note = {To appear},
}

@article {springerlink:10.1007/s10618-008-0118-x,
	author = {Linstead, Erik and Bajracharya, Sushil and Ngo, Trung and Rigor, Paul and Lopes, Cristina and Baldi, Pierre},
	affiliation = {University of California Donald Bren School of Information and Computer Sciences Irvine USA},
	title = {Sourcerer: mining and searching internet-scale software repositories},
	journal = {Data Mining and Knowledge Discovery},
	publisher = {Springer Netherlands},
	issn = {1384-5810},
	keyword = {Computer Science},
	pages = {300-336},
	volume = {18},
	issue = {2},
	url = {http://dx.doi.org/10.1007/s10618-008-0118-x},
	note = {10.1007/s10618-008-0118-x},
	year = {2009}
}

@inproceedings{CODEFINDER:96,
	author    = {Scott Henninger},
	title     = {Supporting the Construction and Evolution of Component Repositories.},
	booktitle = {ICSE},
	year      = {1996},
	pages     = {279-288},
	ee        = {http://portal.acm.org/citation.cfm?id=227726.227776},
}

@inproceedings{MICA:06,
	author    = {Jeffrey Stylos and
	Brad A. Myers},
	title     = {A Web-Search Tool for Finding \textsc{API} Components and Examples.},
	booktitle = {IEEE Symposium on VL and HCC},
	year      = {2006},
	pages     = {195-202},
}

@inproceedings{CODEBROKER:02,
	author    = {Yunwen Ye and
	Gerhard Fischer},
	title     = {Supporting reuse by delivering task-relevant and personalized
	information.},
	booktitle = {ICSE},
	year      = {2002},
	pages     = {513-523},
	ee        = {http://doi.acm.org/10.1145/581339.581402},
}

@article{HIPIKAT:05,
	author    = {Davor Cubranic and
	Gail C. Murphy and
	Janice Singer and
	Kellogg S. Booth},
	title     = {Hipikat: A Project Memory for Software Development.},
	journal   = {IEEE Trans. Software Eng.},
	volume    = {31},
	number    = {6},
	year      = {2005},
	pages     = {446-465},
	ee        = {http://dx.doi.org/10.1109/TSE.2005.71},
}

@inproceedings{Holmes:2007:SIP:1248820.1248877,
	author = {Holmes, Reid and Walker, Robert J.},
	title = {Supporting the Investigation and Planning of Pragmatic Reuse Tasks},
	booktitle = {Proceedings of the 29th international conference on Software Engineering},
	series = {ICSE '07},
	year = {2007},
	isbn = {0-7695-2828-7},
	pages = {447--457},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2007.83},
	doi = {10.1109/ICSE.2007.83},
	acmid = {1248877},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{STRATHCONA:05,
	author    = {Reid Holmes and
	Robert J. Walker and
	Gail C. Murphy},
	title     = {Strathcona example recommendation tool.},
	booktitle = {ESEC/FSE},
	year      = {2005},
	pages     = {237-240},
	ee        = {http://doi.acm.org/10.1145/1081706.1081744},
}

@article{SPARSJ:05,
	author = {Inoue, Katsuro and Yokomori, Reishi and Yamamoto, Tetsuo and Matsushita, Makoto and Kusumoto, Shinji},
	title = {Ranking Significance of Software Components Based on Use Relations},
	journal = {IEEE Trans. Softw. Eng.},
	volume = {31},
	number = {3},
	year = {2005},
	issn = {0098-5589},
	pages = {213--225},
	doi = {http://dx.doi.org/10.1109/TSE.2005.38},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@inproceedings{McMillan:2012:DSS:2337223.2337267,
	author = {McMillan, Collin and Grechanik, Mark and Poshyvanyk, Denys},
	title = {Detecting similar software applications},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {364--374},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337267},
	acmid = {2337267},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@inproceedings{SPOTWEB:08,
	author = {Thummalapenta, S. and Tao Xie},
	title = {SpotWeb: Detecting Framework Hotspots and Coldspots via Mining Open Source Code on the Web},
	booktitle = {ASE '08},
	year = {2008},
	isbn = {978-1-4244-2187-9},
	pages = {327--336},
	doi = {http://dx.doi.org/10.1109/ASE.2008.43},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{PROSPECTOR:05,
	author    = {David Mandelin and
	Lin Xu and
	Rastislav Bod\'{\i}k and
	Doug Kimelman},
	title     = {Jungloid mining: helping to navigate the \textsc{API} jungle.},
	booktitle = {PLDI},
	year      = {2005},
	pages     = {48-61},
	ee        = {http://doi.acm.org/10.1145/1065010.1065018},
}

@inproceedings{XSNIPPET:06,
	author    = {Naiyana Sahavechaphan and
	Kajal T. Claypool},
	title     = {\textsc{XS}nippet: mining For sample code.},
	booktitle = {OOPSLA},
	year      = {2006},
	pages     = {413-430},
	ee        = {http://doi.acm.org/10.1145/1167473.1167508},
}

@inproceedings{PARSEWEB:07,
	author = {Thummalapenta, Suresh and Xie, Tao},
	title = {Parseweb: a programmer assistant for reusing open source code on the web},
	booktitle = {ASE '07},
	year = {2007},
	isbn = {978-1-59593-882-4},
	pages = {204--213},
	location = {Atlanta, Georgia, USA},
	doi = {http://doi.acm.org/10.1145/1321631.1321663},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{MURPHY:05,
	author    = {Reid Holmes and
	Gail C. Murphy},
	title     = {Using structural context to recommend source code examples.},
	booktitle = {ICSE},
	year      = {2005},
	pages     = {117-125},
	ee        = {http://doi.acm.org/10.1145/1062455.1062491},
}

@inproceedings{S6:09,
	author    = {Steven P. Reiss},
	title     = {Semantics-based code search},
	booktitle = {ICSE},
	year      = {2009},
	pages     = {243-253},
	ee        = {http://dx.doi.org/10.1109/ICSE.2009.5070525},
}

@article{Hummel:2008:CCP:1439186.1439224,
	author = {Hummel, Oliver and Janjic, Werner and Atkinson, Colin},
	title = {Code Conjurer: Pulling Reusable Software out of Thin Air},
	journal = {IEEE Softw.},
	issue_date = {September 2008},
	volume = {25},
	number = {5},
	month = sep,
	year = {2008},
	issn = {0740-7459},
	pages = {45--52},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/MS.2008.110},
	doi = {10.1109/MS.2008.110},
	acmid = {1439224},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
} 

@article{Frakes:2005:SRR:1083823.1083997,
	author = {Frakes, William B. and Kang, Kyo},
	title = {Software Reuse Research: Status and Future},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {July 2005},
	volume = {31},
	number = {7},
	month = jul,
	year = {2005},
	issn = {0098-5589},
	pages = {529--536},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/TSE.2005.85},
	doi = {10.1109/TSE.2005.85},
	acmid = {1083997},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@BOOK{Arango:DomainAnalysis,
	AUTHOR = "G. Arango and R. Prieto-Diaz",
	TITLE = "Domain Analysis: Acquisition of Reusable Information for Software Construction",
	PUBLISHER ="IEEE Comp. Society Press",
	MONTH = "May",
	YEAR = {1989}
}
@ARTICLE{Frakes:DARE,
	AUTHOR = "W.B. Frakes and R. Prieto-Diaz and C.J. Fox",
	TITLE = "Dare: Domain Analysis and Reuse Environment",
	JOURNAL = "Annals of Software Eng.",
	PUBLISHER ="IEEE Computer Society Press",
	VOLUME = {5},
	YEAR = {1998}
}

@book{Weiss:1999:SPE:317887,
	author = {Weiss, David M. and Lai, Chi Tau Robert},
	title = {Software product-line engineering: a family-based software development process},
	year = {1999},
	isbn = {0-201-69438-7},
	publisher = {Addison-Wesley Longman Publishing Co., Inc.},
	address = {Boston, MA, USA},
}

@ARTICLE{1020288,
	author={Kang, K.C. and Jaejoon Lee and Donohoe, P.},
	journal={Software, IEEE}, title={Feature-oriented product line engineering},
	year={2002},
	month={jul/aug},
	volume={19},
	number={4},
	pages={ 58 - 65},
	keywords={ FORM; commonalities; differences; feature-oriented product line engineering; feature-oriented reuse method; home integration system; software development management; software reusability;},
	doi={10.1109/MS.2002.1020288},
	ISSN={0740-7459},
}

@article{Bajracharya:2012:AMC:2318097.2318150,
	author = {Bajracharya, Sushil Krishna and Lopes, Cristina Videira},
	title = {Analyzing and mining a code search engine usage log},
	journal = {Empirical Softw. Engg.},
	issue_date = {August 2012},
	volume = {17},
	number = {4-5},
	month = aug,
	year = {2012},
	issn = {1382-3256},
	pages = {424--466},
	numpages = {43},
	url = {http://dx.doi.org/10.1007/s10664-010-9144-6},
	doi = {10.1007/s10664-010-9144-6},
	acmid = {2318150},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Code search engine, Mining topics, Usage log analysis},
} 

@inproceedings{Linstead:2007:MCC:1321631.1321709,
	author = {Linstead, Erik and Rigor, Paul and Bajracharya, Sushil and Lopes, Cristina and Baldi, Pierre},
	title = {Mining concepts from code with probabilistic topic models},
	booktitle = {Proceedings of the twenty-second IEEE/ACM international conference on Automated software engineering},
	series = {ASE '07},
	year = {2007},
	isbn = {978-1-59593-882-4},
	location = {Atlanta, Georgia, USA},
	pages = {461--464},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1321631.1321709},
	doi = {10.1145/1321631.1321709},
	acmid = {1321709},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {mining software, program understanding, topic models},
} 

@inproceedings{McMillan:2012:RSC:2337223.2337323,
	author = {McMillan, Collin and Hariri, Negar and Poshyvanyk, Denys and Cleland-Huang, Jane and Mobasher, Bamshad},
	title = {Recommending source code for use in rapid software prototypes},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {848--858},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337323},
	acmid = {2337323},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@book{Gomaa:2004:DSP:983234,
	author = {Gomaa, Hassan},
	title = {Designing Software Product Lines with UML: From Use Cases to Pattern-Based Software Architectures},
	year = {2004},
	isbn = {0201775956},
	publisher = {Addison Wesley Longman Publishing Co., Inc.},
	address = {Redwood City, CA, USA},
}

@ARTICLE{Niu:Features2,
	AUTHOR="N.Niu and S.Easterbrook",
	TITLE="Extracting and Modeling Product Line Functional Requirements",
	JOURNAL="RE",
	LOCATION="Washington DC",
	YEAR ={2008},
}

@ARTICLE{Moon:Features3,
	AUTHOR="M.Moon and K.Yeom and H.S.Chae",
	TITLE="An approach to developing domain requirements as a core asset based on commonality and variability analysis in a product line",
	JOURNAL="TSE",
	VOLUME={31},
	ISSUE={7},
	YEAR={2005},
}

@inproceedings{Dumitru:11,
	author = {Dumitru, Horatiu and Gibiec, Marek and Hariri, Negar and Cleland-Huang, Jane and Mobasher, Bamshad and Castro-Herrera, Carlos and Mirakhorli, Mehdi},
	title = {On-demand feature recommendations derived from mining public product descriptions},
	booktitle = {ICSE},
	year = {2011},
	pages = {181--190},
}

@article{Holmes:Pragmatic:TOSEM,
	author = {Reid Holmes and Robert J. Walker},
	title = {Systematizing Pragmatic Software Reuse},
	journal ={ACM Transactions on Software Engineering and Methodology},
	year = {2012},
	publisher = {ACM},
	note = {To appear},
}

@inproceedings{Holmes:2009:ART:1747491.1747534,
	author = {Holmes, Reid and Ratchford, Tristan and Robillard, Martin P. and Walker, Robert J.},
	title = {Automatically Recommending Triage Decisions for Pragmatic Reuse Tasks},
	booktitle = {Proceedings of the 2009 IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '09},
	year = {2009},
	isbn = {978-0-7695-3891-4},
	pages = {397--408},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/ASE.2009.65},
	doi = {10.1109/ASE.2009.65},
	acmid = {1747534},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {pragmatic software reuse tasks, triage decisions, recommendation systems, structural relevance, cost, source code analysis, retroactive evaluation},
}

@inproceedings{Kotonya:2008:ORL:1478087.1478113,
	author = {Kotonya, Gerald and Lock, Simon and Mariani, John},
	title = {Opportunistic Reuse: Lessons from Scrapheap Software Development},
	booktitle = {Proceedings of the 11th International Symposium on Component-Based Software Engineering},
	series = {CBSE '08},
	year = {2008},
	isbn = {978-3-540-87890-2},
	location = {Karlsruhe, Germany},
	pages = {302--309},
	numpages = {8},
	url = {http://dx.doi.org/10.1007/978-3-540-87891-9_20},
	doi = {10.1007/978-3-540-87891-9_20},
	acmid = {1478113},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
}

@inproceedings{Brandt:2010:EPI:1753326.1753402,
	author = {Brandt, Joel and Dontcheva, Mira and Weskamp, Marcos and Klemmer, Scott R.},
	title = {Example-centric programming: integrating web search into the development environment},
	booktitle = {Proceedings of the 28th international conference on Human factors in computing systems},
	series = {CHI '10},
	year = {2010},
	isbn = {978-1-60558-929-9},
	location = {Atlanta, Georgia, USA},
	pages = {513--522},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1753326.1753402},
	doi = {10.1145/1753326.1753402},
	acmid = {1753402},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {example-centric development},
}

@inproceedings{Hartmann:2010:OPS:1753326.1753478,
	author = {Hartmann, Bj\"{o}rn and MacDougall, Daniel and Brandt, Joel and Klemmer, Scott R.},
	title = {What would other programmers do: suggesting solutions to error messages},
	booktitle = {Proceedings of the 28th international conference on Human factors in computing systems},
	series = {CHI '10},
	year = {2010},
	isbn = {978-1-60558-929-9},
	location = {Atlanta, Georgia, USA},
	pages = {1019--1028},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1753326.1753478},
	doi = {10.1145/1753326.1753478},
	acmid = {1753478},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, recommender systems},
}

@inproceedings{Weiser:1981:PS:800078.802557,
	author = {Weiser, Mark},
	title = {Program slicing},
	booktitle = {Proceedings of the 5th international conference on Software engineering},
	series = {ICSE '81},
	year = {1981},
	isbn = {0-89791-146-6},
	location = {San Diego, California, United States},
	pages = {439--449},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=800078.802557},
	acmid = {802557},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Data flow analysis, Debugging, Human factors, Program maintenance, Program metrics, Software tools},
}

@article{DBLP:journals/tse/Weiser84,
	author    = {Mark Weiser},
	title     = {Program Slicing},
	journal   = {IEEE Trans. Software Eng.},
	volume    = {10},
	number    = {4},
	year      = {1984},
	pages     = {352-357},
	ee        = {http://doi.ieeecomputersociety.org/10.1109/TSE.1984.5010248},
	bibsource = {DBLP, http://dblp.uni-trier.de}
} 

@article{Horwitz:1988:ISU:960116.53994,
	author = {Horwitz, S. and Reps, T. and Binkley, D.},
	title = {Interprocedural slicing using dependence graphs},
	journal = {SIGPLAN Not.},
	issue_date = {July 1988},
	volume = {23},
	number = {7},
	month = jun,
	year = {1988},
	issn = {0362-1340},
	pages = {35--46},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/960116.53994},
	doi = {10.1145/960116.53994},
	acmid = {53994},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Horwitz:1988:ISU:53990.53994,
	author = {Horwitz, S. and Reps, T. and Binkley, D.},
	title = {Interprocedural slicing using dependence graphs},
	booktitle = {Proceedings of the ACM SIGPLAN 1988 conference on Programming Language design and Implementation},
	series = {PLDI '88},
	year = {1988},
	isbn = {0-89791-269-1},
	location = {Atlanta, Georgia, United States},
	pages = {35--46},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/53990.53994},
	doi = {10.1145/53990.53994},
	acmid = {53994},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Malenfant:2001:FAD:846228.848706,
	author = {Malenfant, Bruno},
	title = {Flow Analysis to Detect Blocked Statements},
	booktitle = {Proceedings of the IEEE International Conference on Software Maintenance (ICSM'01)},
	series = {ICSM '01},
	year = {2001},
	isbn = {0-7695-1189-9},
	pages = {62--},
	url = {http://dx.doi.org/10.1109/ICSM.2001.972712},
	doi = {10.1109/ICSM.2001.972712},
	acmid = {848706},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {Blocking analysis, inter-procedural flow analysis, software evaluation},
}

@article{Horwitz:1990:ISU:77606.77608,
	author = {Horwitz, Susan and Reps, Thomas and Binkley, David},
	title = {Interprocedural slicing using dependence graphs},
	journal = {ACM Trans. Program. Lang. Syst.},
	issue_date = {Jan. 1990},
	volume = {12},
	number = {1},
	month = jan,
	year = {1990},
	issn = {0164-0925},
	pages = {26--60},
	numpages = {35},
	url = {http://doi.acm.org/10.1145/77606.77608},
	doi = {10.1145/77606.77608},
	acmid = {77608},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Mock:2005:PSD:1083824.1084006,
	author = {Mock, Markus and Atkinson, Darren C. and Chambers, Craig and Eggers, Susan J.},
	title = {Program Slicing with Dynamic Points-To Sets},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {August 2005},
	volume = {31},
	number = {8},
	month = aug,
	year = {2005},
	issn = {0098-5589},
	pages = {657--678},
	numpages = {22},
	url = {http://dx.doi.org/10.1109/TSE.2005.94},
	doi = {10.1109/TSE.2005.94},
	acmid = {1084006},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Index Terms- Dynamic analysis, Index Terms- Dynamic analysis, points-to analysis, program slicing., points-to analysis, program slicing.},
} 

@inproceedings{Venkatesh:1991:SAP:113445.113455,
	author = {Venkatesh, G. A.},
	title = {The semantic approach to program slicing},
	booktitle = {Proceedings of the ACM SIGPLAN 1991 conference on Programming language design and implementation},
	series = {PLDI '91},
	year = {1991},
	isbn = {0-89791-428-7},
	location = {Toronto, Ontario, Canada},
	pages = {107--119},
	numpages = {13},
	url = {http://doi.acm.org/10.1145/113445.113455},
	doi = {10.1145/113445.113455},
	acmid = {113455},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Krinke:1998:SST:277631.277638,
	author = {Krinke, Jens},
	title = {Static slicing of threaded programs},
	booktitle = {Proceedings of the 1998 ACM SIGPLAN-SIGSOFT workshop on Program analysis for software tools and engineering},
	series = {PASTE '98},
	year = {1998},
	isbn = {1-58113-055-4},
	location = {Montreal, Quebec, Canada},
	pages = {35--42},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/277631.277638},
	doi = {10.1145/277631.277638},
	acmid = {277638},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Giffhorn:2009:PSC:1530080.1530094,
	author = {Giffhorn, Dennis and Hammer, Christian},
	title = {Precise slicing of concurrent programs},
	journal = {Automated Software Engg.},
	issue_date = {June      2009},
	volume = {16},
	number = {2},
	month = jun,
	year = {2009},
	issn = {0928-8910},
	pages = {197--234},
	numpages = {38},
	url = {http://dx.doi.org/10.1007/s10515-009-0048-x},
	doi = {10.1007/s10515-009-0048-x},
	acmid = {1530094},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Concurrency, Program analysis, Slicing, Threads},
}

@article{Binkley:2007:ESS:1217295.1217297,
	author = {Binkley, David and Gold, Nicolas and Harman, Mark},
	title = {An empirical study of static program slice size},
	journal = {ACM Trans. Softw. Eng. Methodol.},
	issue_date = {April 2007},
	volume = {16},
	number = {2},
	month = apr,
	year = {2007},
	issn = {1049-331X},
	articleno = {8},
	url = {http://doi.acm.org/10.1145/1217295.1217297},
	doi = {10.1145/1217295.1217297},
	acmid = {1217297},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Program slicing, slice size},
} 

@article{Agrawal:1990:DPS:93548.93576,
	author = {Agrawal, Hiralal and Horgan, Joseph R.},
	title = {Dynamic program slicing},
	journal = {SIGPLAN Not.},
	issue_date = {Jun. 1990},
	volume = {25},
	number = {6},
	month = jun,
	year = {1990},
	issn = {0362-1340},
	pages = {246--256},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/93548.93576},
	doi = {10.1145/93548.93576},
	acmid = {93576},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Binkley:2007:ESO:1290520.1290523,
	author = {Binkley, David and Harman, Mark and Krinke, Jens},
	title = {Empirical study of optimization techniques for massive slicing},
	journal = {ACM Trans. Program. Lang. Syst.},
	issue_date = {November 2007},
	volume = {30},
	number = {1},
	month = nov,
	year = {2007},
	issn = {0164-0925},
	articleno = {3},
	url = {http://doi.acm.org/10.1145/1290520.1290523},
	doi = {10.1145/1290520.1290523},
	acmid = {1290523},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Slicing, empirical study, internal representation, performance enhancement},
}

@article{Krinke:2006:ECP:1167771.1167775,
	author = {Krinke, Jens},
	title = {Effects of context on program slicing},
	journal = {J. Syst. Softw.},
	issue_date = {September 2006},
	volume = {79},
	number = {9},
	month = sep,
	year = {2006},
	issn = {0164-1212},
	pages = {1249--1260},
	numpages = {12},
	url = {http://dx.doi.org/10.1016/j.jss.2006.02.040},
	doi = {10.1016/j.jss.2006.02.040},
	acmid = {1167775},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {program analysis, program slicing},
}

@article{Canfora1998595,
	title = "Conditioned program slicing",
	journal = "Information and Software Technology",
	volume = "40",
	number = "11–12",
	pages = "595 - 607",
	year = "1998",
	note = "",
	issn = "0950-5849",
	doi = "10.1016/S0950-5849(98)00086-X",
	url = "http://www.sciencedirect.com/science/article/pii/S095058499800086X",
	author = "Gerardo Canfora and Aniello Cimitile and Andrea De Lucia",
}

@article{Korel:1997:CDP:249578.249587,
	author = {Korel, Bogdan},
	title = {Computation of Dynamic Program Slices for Unstructured Programs},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {January 1997},
	volume = {23},
	number = {1},
	month = jan,
	year = {1997},
	issn = {0098-5589},
	pages = {17--34},
	numpages = {18},
	url = {http://dx.doi.org/10.1109/32.581327},
	doi = {10.1109/32.581327},
	acmid = {249587},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Program slicing, dynamic program slicing, removable block, control dependence, data dependence, execution trace, unstructured program, debugging.},
} 

@article{DBLP:journals/infsof/KorelR98,
	author    = {Bogdan Korel and
	Juergen Rilling},
	title     = {Dynamic program slicing methods},
	journal   = {Information {\&} Software Technology},
	volume    = {40},
	number    = {11-12},
	year      = {1998},
	pages     = {647-659},
	ee        = {http://dx.doi.org/10.1016/S0950-5849(98)00089-5},
	bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{Xu:2005:BSP:1050849.1050865,
	author = {Xu, Baowen and Qian, Ju and Zhang, Xiaofang and Wu, Zhongqiang and Chen, Lin},
	title = {A brief survey of program slicing},
	journal = {SIGSOFT Softw. Eng. Notes},
	issue_date = {March 2005},
	volume = {30},
	number = {2},
	month = mar,
	year = {2005},
	issn = {0163-5948},
	pages = {1--36},
	numpages = {36},
	url = {http://doi.acm.org/10.1145/1050849.1050865},
	doi = {10.1145/1050849.1050865},
	acmid = {1050865},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, dependence analysis, pointer analysis, program analysis, program slicing},
}

@techreport{
	yiji_2012_tr,
	author = "Yiji Zhang and Raul Santelices",
	institution = "University of Notre Dame Computer Science Department",
	title = "Predicting Runtime Data Dependences for Slice Inspection Prioritization",
	number = "2012-02",
	month = "July",
	year = "2012"
}

@inproceedings{Zhang:2006:PDS:1133981.1134002,
	author = {Zhang, Xiangyu and Gupta, Neelam and Gupta, Rajiv},
	title = {Pruning dynamic slices with confidence},
	booktitle = {Proceedings of the 2006 ACM SIGPLAN conference on Programming language design and implementation},
	series = {PLDI '06},
	year = {2006},
	isbn = {1-59593-320-4},
	location = {Ottawa, Ontario, Canada},
	pages = {169--180},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1133981.1134002},
	doi = {10.1145/1133981.1134002},
	acmid = {1134002},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {data and control dependences, debugging, dynamic slicing},
}

@inproceedings{Sridharan:2007:TS:1250734.1250748,
	author = {Sridharan, Manu and Fink, Stephen J. and Bodik, Rastislav},
	title = {Thin slicing},
	booktitle = {Proceedings of the 2007 ACM SIGPLAN conference on Programming language design and implementation},
	series = {PLDI '07},
	year = {2007},
	isbn = {978-1-59593-633-2},
	location = {San Diego, California, USA},
	pages = {112--122},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1250734.1250748},
	doi = {10.1145/1250734.1250748},
	acmid = {1250748},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, program understanding, slicing},
}

@article{Gallagher:1991:UPS:126244.126248,
	author = {Gallagher, Keith Brian and Lyle, James R.},
	title = {Using Program Slicing in Software Maintenance},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {August 1991},
	volume = {17},
	number = {8},
	month = aug,
	year = {1991},
	issn = {0098-5589},
	pages = {751--761},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/32.83912},
	doi = {10.1109/32.83912},
	acmid = {126248},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {line number, linear time, program slice, program slicing, program testing, semantically consistent changes, set inclusion, single variable decomposition slices, slice-based decomposition, software maintenance, software maintenance problem, unmodified components},
}

@inproceedings{Robillard:2002:CGF:581339.581390,
	author = {Robillard, Martin P. and Murphy, Gail C.},
	title = {Concern graphs: finding and describing concerns using structural program dependencies},
	booktitle = {Proceedings of the 24th International Conference on Software Engineering},
	series = {ICSE '02},
	year = {2002},
	isbn = {1-58113-472-X},
	location = {Orlando, Florida},
	pages = {406--416},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/581339.581390},
	doi = {10.1145/581339.581390},
	acmid = {581390},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Mund:2006:EID:1150566.1150570,
	author = {Mund, G. B. and Mall, Rajib},
	title = {An efficient interprocedural dynamic slicing method},
	journal = {J. Syst. Softw.},
	issue_date = {June 2006},
	volume = {79},
	number = {6},
	month = jun,
	year = {2006},
	issn = {0164-1212},
	pages = {791--806},
	numpages = {16},
	url = {http://dx.doi.org/10.1016/j.jss.2005.07.024},
	doi = {10.1016/j.jss.2005.07.024},
	acmid = {1150570},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {Control dependence graph, Control flow graph, Dynamic slicing, Program debugging, Program dependence graph, Program slicing, Static slicing},
}

@inproceedings{Dunn:1993:ADR:257572.257660,
	author = {Dunn, Michael F. and Knight, John C.},
	title = {Automating the detection of reusable parts in existing software},
	booktitle = {Proceedings of the 15th international conference on Software Engineering},
	series = {ICSE '93},
	year = {1993},
	isbn = {0-89791-588-7},
	location = {Baltimore, Maryland, United States},
	pages = {381--390},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=257572.257660},
	acmid = {257660},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
	keywords = {Prolog, expert system, reengineering, reusable components, software reuse},
}

@article{Zhang:2010:BAH:1944279.1944280,
	author = {Zhang, Lu and Luo, Jing and Li, He and Sun, Jiasu and Mei, Hong},
	title = {A biting-down approach to hierarchical decomposition of object-oriented systems based on structure analysis},
	journal = {J. Softw. Maint. Evol.},
	issue_date = {December 2010},
	volume = {22},
	number = {8},
	month = dec,
	year = {2010},
	issn = {1532-060X},
	pages = {567--596},
	numpages = {30},
	url = {http://dx.doi.org/10.1002/smr.417},
	doi = {10.1002/smr.417},
	acmid = {1944280},
	publisher = {John Wiley \& Sons, Inc.},
	address = {New York, NY, USA},
	keywords = {architecture recovery, hierarchical system decomposition, software clustering},
}

@article{Caldiera:1991:IQR:103293.103294,
	author = {Caldiera, Gianluigi and Basili, Victor R.},
	title = {Identifying and Qualifying Reusable Software Components},
	journal = {Computer},
	issue_date = {February 1991},
	volume = {24},
	number = {2},
	month = feb,
	year = {1991},
	issn = {0018-9162},
	pages = {61--70},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/2.67210},
	doi = {10.1109/2.67210},
	acmid = {103294},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{Schach:1995:MTC:315891.316024,
	author = {Schach, Stephen R. and Yang, Xuefeng},
	title = {Metrics for targeting candidates for reuse: an experimental approach},
	booktitle = {Proceedings of the 1995 ACM symposium on Applied computing},
	series = {SAC '95},
	year = {1995},
	isbn = {0-89791-658-1},
	location = {Nashville, Tennessee, United States},
	pages = {379--383},
	numpages = {5},
	url = {http://doi.acm.org/10.1145/315891.316024},
	doi = {10.1145/315891.316024},
	acmid = {316024},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {accidental reuse, experimentation, reusability, software metrics},
}

@article{Roemer:2012:RPS:2133375.2133377,
	author = {Roemer, Ryan and Buchanan, Erik and Shacham, Hovav and Savage, Stefan},
	title = {Return-Oriented Programming: Systems, Languages, and Applications},
	journal = {ACM Trans. Inf. Syst. Secur.},
	issue_date = {March 2012},
	volume = {15},
	number = {1},
	month = mar,
	year = {2012},
	issn = {1094-9224},
	pages = {2:1--2:34},
	articleno = {2},
	numpages = {34},
	url = {http://doi.acm.org/10.1145/2133375.2133377},
	doi = {10.1145/2133375.2133377},
	acmid = {2133377},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {NX, RISC, Return-oriented programming, SPARC, W-xor-X, attacks, control flow integrity, memory safety, return-into-libc, x86},
}

@inproceedings{Checkoway:2010:RPW:1866307.1866370,
	author = {Checkoway, Stephen and Davi, Lucas and Dmitrienko, Alexandra and Sadeghi, Ahmad-Reza and Shacham, Hovav and Winandy, Marcel},
	title = {Return-oriented programming without returns},
	booktitle = {Proceedings of the 17th ACM conference on Computer and communications security},
	series = {CCS '10},
	year = {2010},
	isbn = {978-1-4503-0245-6},
	location = {Chicago, Illinois, USA},
	pages = {559--572},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/1866307.1866370},
	doi = {10.1145/1866307.1866370},
	acmid = {1866370},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {arm, return-oriented programming, x86},
}

@inproceedings{Chen:2010:EDR:1940366.1940380,
	author = {Chen, Ping and Xing, Xiao and Han, Hao and Mao, Bing and Xie, Li},
	title = {Efficient detection of the return-oriented programming malicious code},
	booktitle = {Proceedings of the 6th international conference on Information systems security},
	series = {ICISS'10},
	year = {2010},
	isbn = {3-642-17713-1, 978-3-642-17713-2},
	location = {Gandhinagar, India},
	pages = {140--155},
	numpages = {16},
	url = {http://dl.acm.org/citation.cfm?id=1940366.1940380},
	acmid = {1940380},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
}

@inproceedings{Bletsch:2011:JPN:1966913.1966919,
	author = {Bletsch, Tyler and Jiang, Xuxian and Freeh, Vince W. and Liang, Zhenkai},
	title = {Jump-oriented programming: a new class of code-reuse attack},
	booktitle = {Proceedings of the 6th ACM Symposium on Information, Computer and Communications Security},
	series = {ASIACCS '11},
	year = {2011},
	isbn = {978-1-4503-0564-8},
	location = {Hong Kong, China},
	pages = {30--40},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1966913.1966919},
	doi = {10.1145/1966913.1966919},
	acmid = {1966919},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@INPROCEEDINGS{mohan12woot,
	author = "Vishwath Mohan and Kevin W. Hamlen",
	title = "{Frankenstein}: Stitching Malware from Benign Binaries",
	booktitle = "Proceedings of the 6th USENIX Workshop on Offensive Technologies (WOOT)",
	address = "Bellevue, Washington",
	month = "August",
	year = 2012,
}

@article{Il68,
	added-at = {2006-11-21T05:45:44.000+0100},
	author = {McIlroy, M. D.},
	biburl = {http://www.bibsonomy.org/bibtex/2bdd8dc73582a1061c5353c143b85bb9e/berger},
	chapter = 14,
	interhash = {f27eb07f75ede5abc8af427c9d186453},
	intrahash = {bdd8dc73582a1061c5353c143b85bb9e},
	journal = {Proc. NATO Conf. on Software Engineering, Garmisch, Germany},
	keywords = {Software-Engineering},
	publisher = {Springer-Verlag},
	timestamp = {2006-11-21T05:45:44.000+0100},
	title = {Mass-produced software components},
	year = 1968
}

@INPROCEEDINGS{Howison04theperils,
	author = {James Howison and Kevin Crowston},
	title = {The perils and pitfalls of mining SourceForge},
	booktitle = {In Proceedings of the International Workshop on Mining Software Repositories (MSR 2004},
	year = {2004},
	pages = {7--11}
}

@article{Dunlap:2002:REI:844128.844148,
	author = {Dunlap, George W. and King, Samuel T. and Cinar, Sukru and Basrai, Murtaza A. and Chen, Peter M.},
	title = {ReVirt: enabling intrusion analysis through virtual-machine logging and replay},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {Winter 2002},
	volume = {36},
	number = {SI},
	month = dec,
	year = {2002},
	issn = {0163-5980},
	pages = {211--224},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/844128.844148},
	doi = {10.1145/844128.844148},
	acmid = {844148},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@misc{CRAW,
	author = {Computing Research Association},
	title = {Committee on the Status of Women in Computing Research},
	month = Jan,
	year = {2013},
	note = {http://www.cra-w.org/}
}

@misc{GDB:Website,
	author = {GNU},
	title = {The GNU Project Debugger},
	month = sep,
	year = {2012},
	note = {http://www.gnu.org/software/gdb/}
}

@article{LeBlanc:1987:DPP:32387.32396,
	author = {LeBlanc, T. J. and Mellor-Crummey, J. M.},
	title = {Debugging Parallel Programs with Instant Replay},
	journal = {IEEE Trans. Comput.},
	issue_date = {April 1987},
	volume = {36},
	number = {4},
	month = apr,
	year = {1987},
	issn = {0018-9340},
	pages = {471--482},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/TC.1987.1676929},
	doi = {10.1109/TC.1987.1676929},
	acmid = {32396},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {CREW protocols, distributed debugging, execution replay, parallel programming, program instrumentation, shared objects, shared objects, CREW protocols, distributed debugging, execution replay, parallel programming, program instrumentation},
}

@inproceedings{Balzer:1969:EED:1476793.1476881,
	author = {Balzer, R. M.},
	title = {EXDAMS: extendable debugging and monitoring system},
	booktitle = {Proceedings of the May 14-16, 1969, spring joint computer conference},
	series = {AFIPS '69 (Spring)},
	year = {1969},
	location = {Boston, Massachusetts},
	pages = {567--580},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/1476793.1476881},
	doi = {10.1145/1476793.1476881},
	acmid = {1476881},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Bacon:1991:HRM:122759.122777,
	author = {Bacon, David F. and Goldstein, Seth Copen},
	title = {Hardware-assisted replay of multiprocessor programs},
	booktitle = {Proceedings of the 1991 ACM/ONR workshop on Parallel and distributed debugging},
	series = {PADD '91},
	year = {1991},
	isbn = {0-89791-457-0},
	location = {Santa Cruz, California, United States},
	pages = {194--206},
	numpages = {13},
	url = {http://doi.acm.org/10.1145/122759.122777},
	doi = {10.1145/122759.122777},
	acmid = {122777},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Devietti:2009:DDS:1508244.1508255,
	author = {Devietti, Joseph and Lucia, Brandon and Ceze, Luis and Oskin, Mark},
	title = {DMP: deterministic shared memory multiprocessing},
	booktitle = {Proceedings of the 14th international conference on Architectural support for programming languages and operating systems},
	series = {ASPLOS '09},
	year = {2009},
	isbn = {978-1-60558-406-5},
	location = {Washington, DC, USA},
	pages = {85--96},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1508244.1508255},
	doi = {10.1145/1508244.1508255},
	acmid = {1508255},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, determinism, multicores, parallel programming},
}

@inproceedings{Hower:2008:REE:1381306.1382144,
	author = {Hower, Derek R. and Hill, Mark D.},
	title = {Rerun: Exploiting Episodes for Lightweight Memory Race Recording},
	booktitle = {Proceedings of the 35th Annual International Symposium on Computer Architecture},
	series = {ISCA '08},
	year = {2008},
	isbn = {978-0-7695-3174-8},
	pages = {265--276},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/ISCA.2008.26},
	doi = {10.1109/ISCA.2008.26},
	acmid = {1382144},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {Multicore, Determinism, Race Recording},
}

@inproceedings{Montesinos:2008:DRD:1381306.1382146,
	author = {Montesinos, Pablo and Ceze, Luis and Torrellas, Josep},
	title = {DeLorean: Recording and Deterministically Replaying Shared-Memory Multiprocessor Execution Ef?ciently},
	booktitle = {Proceedings of the 35th Annual International Symposium on Computer Architecture},
	series = {ISCA '08},
	year = {2008},
	isbn = {978-0-7695-3174-8},
	pages = {289--300},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/ISCA.2008.36},
	doi = {10.1109/ISCA.2008.36},
	acmid = {1382146},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Montesinos:2009:CSI:1508244.1508254,
	author = {Montesinos, Pablo and Hicks, Matthew and King, Samuel T. and Torrellas, Josep},
	title = {Capo: a software-hardware interface for practical deterministic multiprocessor replay},
	booktitle = {Proceedings of the 14th international conference on Architectural support for programming languages and operating systems},
	series = {ASPLOS '09},
	year = {2009},
	isbn = {978-1-60558-406-5},
	location = {Washington, DC, USA},
	pages = {73--84},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1508244.1508254},
	doi = {10.1145/1508244.1508254},
	acmid = {1508254},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {capo, capoone, deterministic replay, replay sphere},
}

@article{Narayanasamy:2006:RSM:1168917.1168886,
	author = {Narayanasamy, Satish and Pereira, Cristiano and Calder, Brad},
	title = {Recording shared memory dependencies using strata},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {December 2006},
	volume = {40},
	number = {5},
	month = oct,
	year = {2006},
	issn = {0163-5980},
	pages = {229--240},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1168917.1168886},
	doi = {10.1145/1168917.1168886},
	acmid = {1168886},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, dependencies, logging, replay, shared memory, strata},
}

@article{Narayanasamy:2005:BCR:1080695.1069994,
	author = {Narayanasamy, Satish and Pokam, Gilles and Calder, Brad},
	title = {BugNet: Continuously Recording Program Execution for Deterministic Replay Debugging},
	journal = {SIGARCH Comput. Archit. News},
	issue_date = {May 2005},
	volume = {33},
	number = {2},
	month = may,
	year = {2005},
	issn = {0163-5964},
	pages = {284--295},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1080695.1069994},
	doi = {10.1145/1080695.1069994},
	acmid = {1069994},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Olszewski:2009:KED:1508284.1508256,
	author = {Olszewski, Marek and Ansel, Jason and Amarasinghe, Saman},
	title = {Kendo: efficient deterministic multithreading in software},
	journal = {SIGPLAN Not.},
	issue_date = {March 2009},
	volume = {44},
	number = {3},
	month = mar,
	year = {2009},
	issn = {0362-1340},
	pages = {97--108},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1508284.1508256},
	doi = {10.1145/1508284.1508256},
	acmid = {1508256},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, determinism, deterministic multithreading, multicore, parallel programming},
}

@article{Bressoud:1996:HFT:225535.225538,
	author = {Bressoud, Thomas C. and Schneider, Fred B.},
	title = {Hypervisor-based fault tolerance},
	journal = {ACM Trans. Comput. Syst.},
	issue_date = {Feb. 1996},
	volume = {14},
	number = {1},
	month = feb,
	year = {1996},
	issn = {0734-2071},
	pages = {80--107},
	numpages = {28},
	url = {http://doi.acm.org/10.1145/225535.225538},
	doi = {10.1145/225535.225538},
	acmid = {225538},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {fault-tolerant computing system, primary/backup approach, virtual-machine manager},
}

@inproceedings{Dunlap:2008:ERM:1346256.1346273,
	author = {Dunlap, George W. and Lucchetti, Dominic G. and Fetterman, Michael A. and Chen, Peter M.},
	title = {Execution replay of multiprocessor virtual machines},
	booktitle = {Proceedings of the fourth ACM SIGPLAN/SIGOPS international conference on Virtual execution environments},
	series = {VEE '08},
	year = {2008},
	isbn = {978-1-59593-796-4},
	location = {Seattle, WA, USA},
	pages = {121--130},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1346256.1346273},
	doi = {10.1145/1346256.1346273},
	acmid = {1346273},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {ReVirt, Xen, determinism, direct memory access, execution replay, hardware page protections, multiprocessors, multithreading, virtual machines},
}

@article{Chow:2010:MRC:1837854.1736002,
	author = {Chow, Jim and Lucchetti, Dominic and Garfinkel, Tal and Lefebvre, Geoffrey and Gardner, Ryan and Mason, Joshua and Small, Sam and Chen, Peter M.},
	title = {Multi-stage replay with crosscut},
	journal = {SIGPLAN Not.},
	issue_date = {July 2010},
	volume = {45},
	number = {7},
	month = mar,
	year = {2010},
	issn = {0362-1340},
	pages = {13--24},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1837854.1736002},
	doi = {10.1145/1837854.1736002},
	acmid = {1736002},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {design, experimentation, performance, replay, security, virtual machines},
}

@inproceedings{Geels:2006:RDD:1267359.1267386,
	author = {Geels, Dennis and Altekar, Gautam and Shenker, Scott and Stoica, Ion},
	title = {Replay debugging for distributed applications},
	booktitle = {Proceedings of the annual conference on USENIX '06 Annual Technical Conference},
	series = {ATEC '06},
	year = {2006},
	location = {Boston, MA},
	pages = {27--27},
	numpages = {1},
	url = {http://dl.acm.org/citation.cfm?id=1267359.1267386},
	acmid = {1267386},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
}

@inproceedings{Guo:2008:RAK:1855741.1855755,
	author = {Guo, Zhenyu and Wang, Xi and Tang, Jian and Liu, Xuezheng and Xu, Zhilei and Wu, Ming and Kaashoek, M. Frans and Zhang, Zheng},
	title = {R2: an application-level kernel for record and replay},
	booktitle = {Proceedings of the 8th USENIX conference on Operating systems design and implementation},
	series = {OSDI'08},
	year = {2008},
	location = {San Diego, California},
	pages = {193--208},
	numpages = {16},
	url = {http://dl.acm.org/citation.cfm?id=1855741.1855755},
	acmid = {1855755},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
}

@inproceedings{Saito:2005:JUL:1085130.1085139,
	author = {Saito, Yasushi},
	title = {Jockey: a user-space library for record-replay debugging},
	booktitle = {Proceedings of the sixth international symposium on Automated analysis-driven debugging},
	series = {AADEBUG'05},
	year = {2005},
	isbn = {1-59593-050-7},
	location = {Monterey, California, USA},
	pages = {69--76},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1085130.1085139},
	doi = {10.1145/1085130.1085139},
	acmid = {1085139},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Linux, checkpointing, debugging, execution record and replay, jockey, keywords, x86},
}

@inproceedings{Choi:1998:DRJ:281035.281041,
	author = {Choi, Jong-Deok and Srinivasan, Harini},
	title = {Deterministic replay of Java multithreaded applications},
	booktitle = {Proceedings of the SIGMETRICS symposium on Parallel and distributed tools},
	series = {SPDT '98},
	year = {1998},
	isbn = {1-58113-001-5},
	location = {Welches, Oregon, United States},
	pages = {48--59},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/281035.281041},
	doi = {10.1145/281035.281041},
	acmid = {281041},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Russinovich:1996:RCN:249069.231432,
	author = {Russinovich, Mark and Cogswell, Bryce},
	title = {Replay for concurrent non-deterministic shared-memory applications},
	journal = {SIGPLAN Not.},
	issue_date = {May 1996},
	volume = {31},
	number = {5},
	month = may,
	year = {1996},
	issn = {0362-1340},
	pages = {258--266},
	numpages = {9},
	url = {http://doi.acm.org/10.1145/249069.231432},
	doi = {10.1145/249069.231432},
	acmid = {231432},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {instruction counter, non-determinism, repeatable execution, shared memory},
}

@inproceedings{Bergheaud:2007:FTM:1270387.1270855,
	author = {Bergheaud, Philippe and Subhraveti, Dinesh and Vertes, Marc},
	title = {Fault Tolerance in Multiprocessor Systems Via Application Cloning},
	booktitle = {Proceedings of the 27th International Conference on Distributed Computing Systems},
	series = {ICDCS '07},
	year = {2007},
	isbn = {0-7695-2837-3},
	pages = {21--},
	url = {http://dx.doi.org/10.1109/ICDCS.2007.111},
	doi = {10.1109/ICDCS.2007.111},
	acmid = {1270855},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Bressoud:1998:TSS:795671.796914,
	author = {Bressoud, T. C.},
	title = {TFT: A Software System for Application-Transparent Fault Tolerance},
	booktitle = {Proceedings of the The Twenty-Eighth Annual International Symposium on Fault-Tolerant Computing},
	series = {FTCS '98},
	year = {1998},
	isbn = {0-8186-8470-4},
	pages = {128--},
	url = {http://dl.acm.org/citation.cfm?id=795671.796914},
	acmid = {796914},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Bressoud:1998:TSS:795671.796914,
	author = {Bressoud, T. C.},
	title = {TFT: A Software System for Application-Transparent Fault Tolerance},
	booktitle = {Proceedings of the The Twenty-Eighth Annual International Symposium on Fault-Tolerant Computing},
	series = {FTCS '98},
	year = {1998},
	isbn = {0-8186-8470-4},
	pages = {128--},
	url = {http://dl.acm.org/citation.cfm?id=795671.796914},
	acmid = {796914},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Srinivasan:2004:FLE:1247415.1247418,
	author = {Srinivasan, Sudarshan M. and Kandula, Srikanth and Andrews, Christopher R. and Zhou, Yuanyuan},
	title = {Flashback: a lightweight extension for rollback and deterministic replay for software debugging},
	booktitle = {Proceedings of the annual conference on USENIX Annual Technical Conference},
	series = {ATEC '04},
	year = {2004},
	location = {Boston, MA},
	pages = {3--3},
	numpages = {1},
	url = {http://dl.acm.org/citation.cfm?id=1247415.1247418},
	acmid = {1247418},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
}

@inproceedings{Thane:2000:UDR:1947412.1947455,
	author = {Thane, Henrik and Hansson, Hans},
	title = {Using deterministic replay for debugging of distributed real-time systems},
	booktitle = {Proceedings of the 12th Euromicro conference on Real-time systems},
	series = {Euromicro-RTS'00},
	year = {2000},
	isbn = {0-7695-0734-4},
	location = {Stockholm, Sweden},
	pages = {265--272},
	numpages = {8},
	url = {http://dl.acm.org/citation.cfm?id=1947412.1947455},
	acmid = {1947455},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {debugging, determinism, distributed real-time systems, monitoring, probe-effect, replay, testing},
} 

@article{Laadan:2010:TLA:1811099.1811057,
	author = {Laadan, Oren and Viennot, Nicolas and Nieh, Jason},
	title = {Transparent, lightweight application execution replay on commodity multiprocessor operating systems},
	journal = {SIGMETRICS Perform. Eval. Rev.},
	issue_date = {June 2010},
	volume = {38},
	number = {1},
	month = jun,
	year = {2010},
	issn = {0163-5999},
	pages = {155--166},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1811099.1811057},
	doi = {10.1145/1811099.1811057},
	acmid = {1811057},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, fault-tolerance, record-replay, virtualization},
}

@inproceedings{Xu:2003:FDR:859618.859633,
	author = {Xu, Min and Bodik, Rastislav and Hill, Mark D.},
	title = {A "flight data recorder" for enabling full-system multiprocessor deterministic replay},
	booktitle = {Proceedings of the 30th annual international symposium on Computer architecture},
	series = {ISCA '03},
	year = {2003},
	isbn = {0-7695-1945-8},
	location = {San Diego, California},
	pages = {122--135},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/859618.859633},
	doi = {10.1145/859618.859633},
	acmid = {859633},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Subhraveti:2011:RTP:1993744.1993757,
	author = {Subhraveti, Dinesh and Nieh, Jason},
	title = {Record and transplay: partial checkpointing for replay debugging across heterogeneous systems},
	booktitle = {Proceedings of the ACM SIGMETRICS joint international conference on Measurement and modeling of computer systems},
	series = {SIGMETRICS '11},
	year = {2011},
	isbn = {978-1-4503-0814-4},
	location = {San Jose, California, USA},
	pages = {109--120},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1993744.1993757},
	doi = {10.1145/1993744.1993757},
	acmid = {1993757},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {checkpoint-restart, record-replay, virtualization},
}

@article{Min:1991:ECA:106974.106996,
	author = {Min, Sang L. and Choi, Jong-Deok},
	title = {An efficient cache-based access anomaly detection scheme},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {Apr. 1991},
	volume = {25},
	number = {Special Issue},
	month = apr,
	year = {1991},
	issn = {0163-5980},
	pages = {235--244},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/106974.106996},
	doi = {10.1145/106974.106996},
	acmid = {106996},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Pan:1988:SRE:68210.69227,
	author = {Pan, Douglas Z. and Linton, Mark A.},
	title = {Supporting reverse execution for parallel programs},
	booktitle = {Proceedings of the 1988 ACM SIGPLAN and SIGOPS workshop on Parallel and distributed debugging},
	series = {PADD '88},
	year = {1988},
	isbn = {0-89791-296-9},
	location = {Madison, Wisconsin, United States},
	pages = {124--129},
	numpages = {6},
	url = {http://doi.acm.org/10.1145/68210.69227},
	doi = {10.1145/68210.69227},
	acmid = {69227},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Netzer:1993:OTR:174266.174268,
	author = {Netzer, Robert H. B.},
	title = {Optimal tracing and replay for debugging shared-memory parallel programs},
	booktitle = {Proceedings of the 1993 ACM/ONR workshop on Parallel and distributed debugging},
	series = {PADD '93},
	year = {1993},
	isbn = {0-89791-633-6},
	location = {San Diego, California, United States},
	pages = {1--11},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/174266.174268},
	doi = {10.1145/174266.174268},
	acmid = {174268},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Savage:1997:EDD:269005.266641,
	author = {Savage, Stefan and Burrows, Michael and Nelson, Greg and Sobalvarro, Patrick and Anderson, Thomas},
	title = {Eraser: a dynamic data race detector for multi-threaded programs},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {Dec. 1997},
	volume = {31},
	number = {5},
	month = oct,
	year = {1997},
	issn = {0163-5980},
	pages = {27--37},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/269005.266641},
	doi = {10.1145/269005.266641},
	acmid = {266641},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Laadan:2007:DPV:1323293.1294289,
	author = {Laadan, Oren and Baratto, Ricardo A. and Phung, Dan B. and Potter, Shaya and Nieh, Jason},
	title = {DejaView: a personal virtual computer recorder},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {December 2007},
	volume = {41},
	number = {6},
	month = oct,
	year = {2007},
	issn = {0163-5980},
	pages = {279--292},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/1323293.1294289},
	doi = {10.1145/1323293.1294289},
	acmid = {1294289},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {desktop search, virtualization},
}

@inproceedings{Tsankov:2011:EHI:1989760.1990086,
	author = {Tsankov, Petar and Jin, Wei and Orso, Alessandro and Sinha, Saurabh},
	title = {Execution Hijacking: Improving Dynamic Analysis by Flying off Course},
	booktitle = {Proceedings of the 2011 Fourth IEEE International Conference on Software Testing, Verification and Validation},
	series = {ICST '11},
	year = {2011},
	isbn = {978-0-7695-4342-0},
	pages = {200--209},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICST.2011.45},
	doi = {10.1109/ICST.2011.45},
	acmid = {1990086},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@article{Silva:2012:VPS:2187671.2187674,
	author = {Silva, Josep},
	title = {A vocabulary of program slicing-based techniques},
	journal = {ACM Comput. Surv.},
	issue_date = {June 2012},
	volume = {44},
	number = {3},
	month = jun,
	year = {2012},
	issn = {0360-0300},
	pages = {12:1--12:41},
	articleno = {12},
	numpages = {41},
	url = {http://doi.acm.org/10.1145/2187671.2187674},
	doi = {10.1145/2187671.2187674},
	acmid = {2187674},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Program slicing, software engineering},
}

@inproceedings{LeVasseur:2004:SAR:1133572.1133617,
	author = {LeVasseur, Joshua and Uhlig, Volkmar},
	title = {A sledgehammer approach to reuse of legacy device drivers},
	booktitle = {Proceedings of the 11th workshop on ACM SIGOPS European workshop},
	series = {EW 11},
	year = {2004},
	location = {Leuven, Belgium},
	articleno = {24},
	url = {http://doi.acm.org/10.1145/1133572.1133617},
	doi = {10.1145/1133572.1133617},
	acmid = {1133617},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Jamrozik:2012:ADS:2351676.2351716,
	author = {Jamrozik, Konrad and Fraser, Gordon and Tillmann, Nikolai and De Halleux, Jonathan},
	title = {Augmented dynamic symbolic execution},
	booktitle = {Proceedings of the 27th IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE 2012},
	year = {2012},
	isbn = {978-1-4503-1204-2},
	location = {Essen, Germany},
	pages = {254--257},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/2351676.2351716},
	doi = {10.1145/2351676.2351716},
	acmid = {2351716},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Test generation, boundary values, dynamic symbolic execution, mutation testing},
}

@inproceedings{Zhang:2010:TGV:1912607.1913317,
	author = {Zhang, Lingming and Xie, Tao and Zhang, Lu and Tillmann, Nikolai and de Halleux, Jonathan and Mei, Hong},
	title = {Test generation via Dynamic Symbolic Execution for mutation testing},
	booktitle = {Proceedings of the 2010 IEEE International Conference on Software Maintenance},
	series = {ICSM '10},
	year = {2010},
	isbn = {978-1-4244-8630-4},
	pages = {1--10},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICSM.2010.5609672},
	doi = {10.1109/ICSM.2010.5609672},
	acmid = {1913317},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Anand:2011:HCE:2190078.2190144,
	author = {Anand, Saswat and Harrold, Mary Jean},
	title = {Heap cloning: Enabling dynamic symbolic execution of java programs},
	booktitle = {Proceedings of the 2011 26th IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '11},
	year = {2011},
	isbn = {978-1-4577-1638-6},
	pages = {33--42},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ASE.2011.6100071},
	doi = {10.1109/ASE.2011.6100071},
	acmid = {2190144},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Sen:2005:CCU:1081706.1081750,
	author = {Sen, Koushik and Marinov, Darko and Agha, Gul},
	title = {CUTE: a concolic unit testing engine for C},
	booktitle = {Proceedings of the 10th European software engineering conference held jointly with 13th ACM SIGSOFT international symposium on Foundations of software engineering},
	series = {ESEC/FSE-13},
	year = {2005},
	isbn = {1-59593-014-0},
	location = {Lisbon, Portugal},
	pages = {263--272},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1081706.1081750},
	doi = {10.1145/1081706.1081750},
	acmid = {1081750},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {concolic testing, data structure testing, explicit path model-checking, random testing, testing C programs, unit testing},
} 

@inproceedings{Godefroid:2005:DDA:1065010.1065036,
	author = {Godefroid, Patrice and Klarlund, Nils and Sen, Koushik},
	title = {DART: directed automated random testing},
	booktitle = {Proceedings of the 2005 ACM SIGPLAN conference on Programming language design and implementation},
	series = {PLDI '05},
	year = {2005},
	isbn = {1-59593-056-6},
	location = {Chicago, IL, USA},
	pages = {213--223},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1065010.1065036},
	doi = {10.1145/1065010.1065036},
	acmid = {1065036},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {automated test generation, interfaces, program verification, random testing, software testing},
} 

@inproceedings{Rubinov:2012:ATS:2337223.2337438,
	author = {Rubinov, Konstantin and Wuttke, Jochen},
	title = {Augmenting test suites automatically},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {1433--1434},
	numpages = {2},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337438},
	acmid = {2337438},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@article{Thummalapenta:2011:SMS:2076021.2048083,
	author = {Thummalapenta, Suresh and Xie, Tao and Tillmann, Nikolai and de Halleux, Jonathan and Su, Zhendong},
	title = {Synthesizing method sequences for high-coverage testing},
	journal = {SIGPLAN Not.},
	issue_date = {October 2011},
	volume = {46},
	number = {10},
	month = oct,
	year = {2011},
	issn = {0362-1340},
	pages = {189--206},
	numpages = {18},
	url = {http://doi.acm.org/10.1145/2076021.2048083},
	doi = {10.1145/2076021.2048083},
	acmid = {2048083},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {object-oriented testing, symbolic execution},
}

@inproceedings{Fraser:2011:ECO:1989760.1990074,
	author = {Fraser, Gordon and Zeller, Andreas},
	title = {Exploiting Common Object Usage in Test Case Generation},
	booktitle = {Proceedings of the 2011 Fourth IEEE International Conference on Software Testing, Verification and Validation},
	series = {ICST '11},
	year = {2011},
	isbn = {978-0-7695-4342-0},
	pages = {80--89},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICST.2011.53},
	doi = {10.1109/ICST.2011.53},
	acmid = {1990074},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {test case generation, specification mining, readability},
}

@inproceedings{Zhang:2011:CSD:2001420.2001463,
	author = {Zhang, Sai and Saff, David and Bu, Yingyi and Ernst, Michael D.},
	title = {Combined static and dynamic automated test generation},
	booktitle = {Proceedings of the 2011 International Symposium on Software Testing and Analysis},
	series = {ISSTA '11},
	year = {2011},
	isbn = {978-1-4503-0562-4},
	location = {Toronto, Ontario, Canada},
	pages = {353--363},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2001420.2001463},
	doi = {10.1145/2001420.2001463},
	acmid = {2001463},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {automated test generation, dynamic analyses, static},
}



@misc{libdwarf,
	author = {Michael Eager},
	title = {The DWARF Debugging Standard},
	month = apr,
	year = {2012},
	note = {http://www.dwarfstd.org/}
}

@inproceedings{Mockus:2007:LCR:1270231.1270273,
	author = {Mockus, Audris},
	title = {Large-Scale Code Reuse in Open Source Software},
	booktitle = {Proceedings of the First International Workshop on Emerging Trends in FLOSS Research and Development},
	series = {FLOSS '07},
	year = {2007},
	isbn = {0-7695-2961-5},
	pages = {7--},
	url = {http://dx.doi.org/10.1109/FLOSS.2007.10},
	acmid = {1270273},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Krueger:1992:SR:130844.130856,
	author = {Krueger, Charles W.},
	title = {Software reuse},
	journal = {ACM Comput. Surv.},
	issue_date = {June 1992},
	volume = {24},
	number = {2},
	month = jun,
	year = {1992},
	issn = {0360-0300},
	pages = {131--183},
	numpages = {53},
	url = {http://doi.acm.org/10.1145/130844.130856},
	doi = {10.1145/130844.130856},
	acmid = {130856},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {abstraction, cognitive distance, software reuse},
}

@ARTICLE{Johnson88designingreuseable,
	author = {Ralph E. Johnson and Brian Foote},
	title = {Designing reuseable classes},
	journal = {Journal of Object-Oriented Programming},
	year = {1988}
}

@article{Rosson:1996:RUS:234526.234530,
	author = {Rosson, Mary Beth and Carroll, John M.},
	title = {The reuse of uses in Smalltalk programming},
	journal = {ACM Trans. Comput.-Hum. Interact.},
	issue_date = {Sept. 1996},
	volume = {3},
	number = {3},
	month = sep,
	year = {1996},
	issn = {1073-0516},
	pages = {219--253},
	numpages = {35},
	url = {http://doi.acm.org/10.1145/234526.234530},
	doi = {10.1145/234526.234530},
	acmid = {234530},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Smalltalk, debugging into existence, example-based learning, reuse of uses, usage context},
}

@inproceedings{Ko:2004:SLB:1032665.1034570,
	author = {Ko, Andrew J. and Myers, Brad A. and Aung, Htet Htet},
	title = {Six Learning Barriers in End-User Programming Systems},
	booktitle = {Proceedings of the 2004 IEEE Symposium on Visual Languages - Human Centric Computing},
	series = {VLHCC '04},
	year = {2004},
	isbn = {0-7803-8696-5},
	pages = {199--206},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/VLHCC.2004.47},
	doi = {10.1109/VLHCC.2004.47},
	acmid = {1034570},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Corbi:1989:PUC:97118.97124,
	author = {Corbi, T. A.},
	title = {Program understanding: challenge for the 1990's},
	journal = {IBM Syst. J.},
	issue_date = {1989},
	volume = {28},
	number = {2},
	month = jun,
	year = {1989},
	issn = {0018-8670},
	pages = {294--306},
	numpages = {13},
	url = {http://dx.doi.org/10.1147/sj.282.0294},
	doi = {10.1147/sj.282.0294},
	acmid = {97124},
	publisher = {IBM Corp.},
	address = {Riverton, NJ, USA},
} 

@article{Sillito:2008:AAQ:1446226.1446241,
	author = {Sillito, Jonathan and Murphy, Gail C. and De Volder, Kris},
	title = {Asking and Answering Questions during a Programming Change Task},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {July 2008},
	volume = {34},
	number = {4},
	month = jul,
	year = {2008},
	issn = {0098-5589},
	pages = {434--451},
	numpages = {18},
	url = {http://dx.doi.org/10.1109/TSE.2008.26},
	doi = {10.1109/TSE.2008.26},
	acmid = {1446241},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Enhancement, Programming Environments/Construction Tools, Software psychology, Software psychology, Programming Environments/Construction Tools, Enhancement},
}

@inproceedings{Sim:1998:ASC:580914.858229,
	author = {Sim, S. E. and Clarke, C. L. A. and Holt, R. C.},
	title = {Archetypal Source Code Searches: A Survey of Software Developers and Maintainers},
	booktitle = {Proceedings of the 6th International Workshop on Program Comprehension},
	series = {IWPC '98},
	year = {1998},
	isbn = {0-8186-8560-3},
	pages = {180--},
	url = {http://dl.acm.org/citation.cfm?id=580914.858229},
	acmid = {858229},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@ARTICLE{Davison00understandingand,
	author = {Joseph W. Davison and Dennis M. Mancl and William F. Opdyke},
	title = {Understanding and addressing the essential costs of evolving systems},
	journal = {Bell Labs Technical Journal},
	year = {2000},
	pages = {44--54}
}

@inproceedings{Kapser:2006:CCH:1174510.1174714,
	author = {Kapser, Cory and Godfrey, Michael W.},
	title = {``Cloning Considered Harmful'' Considered Harmful},
	booktitle = {Proceedings of the 13th Working Conference on Reverse Engineering},
	series = {WCRE '06},
	year = {2006},
	isbn = {0-7695-2719-1},
	pages = {19--28},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/WCRE.2006.1},
	doi = {10.1109/WCRE.2006.1},
	acmid = {1174714},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Juergens:2009:CCM:1555001.1555062,
	author = {Juergens, Elmar and Deissenboeck, Florian and Hummel, Benjamin and Wagner, Stefan},
	title = {Do code clones matter?},
	booktitle = {Proceedings of the 31st International Conference on Software Engineering},
	series = {ICSE '09},
	year = {2009},
	isbn = {978-1-4244-3453-4},
	pages = {485--495},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2009.5070547},
	doi = {10.1109/ICSE.2009.5070547},
	acmid = {1555062},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Kagdi:2007:STA:1345056.1345057,
	author = {Kagdi, Huzefa and Collard, Michael L. and Maletic, Jonathan I.},
	title = {A survey and taxonomy of approaches for mining software repositories in the context of software evolution},
	journal = {J. Softw. Maint. Evol.},
	issue_date = {March 2007},
	volume = {19},
	number = {2},
	month = mar,
	year = {2007},
	issn = {1532-060X},
	pages = {77--131},
	numpages = {55},
	url = {http://dx.doi.org/10.1002/smr.344},
	doi = {10.1002/smr.344},
	acmid = {1345057},
	publisher = {John Wiley \& Sons, Inc.},
	address = {New York, NY, USA},
	keywords = {mining software repositories, multi-version analysis, software evolution},
} 

@inproceedings{Clause:2007:DGD:1273463.1273490,
	author = {Clause, James and Li, Wanchun and Orso, Alessandro},
	title = {Dytan: a generic dynamic taint analysis framework},
	booktitle = {Proceedings of the 2007 international symposium on Software testing and analysis},
	series = {ISSTA '07},
	year = {2007},
	isbn = {978-1-59593-734-6},
	location = {London, United Kingdom},
	pages = {196--206},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1273463.1273490},
	doi = {10.1145/1273463.1273490},
	acmid = {1273490},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {dynamic tainting, general framework, information flow},
} 

@inproceedings{Chan:2012:SCA:2393596.2393606,
	author = {Chan, Wing-Kwan and Cheng, Hong and Lo, David},
	title = {Searching connected API subgraph via text phrases},
	booktitle = {Proceedings of the ACM SIGSOFT 20th International Symposium on the Foundations of Software Engineering},
	series = {FSE '12},
	year = {2012},
	isbn = {978-1-4503-1614-9},
	location = {Cary, North Carolina},
	pages = {10:1--10:11},
	articleno = {10},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2393596.2393606},
	doi = {10.1145/2393596.2393606},
	acmid = {2393606},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {API graph, API recommendation, subgraph searching},
} 

@article{Shackelford:2006:CCO:1124706.1121482,
	author = {Shackelford, Russell and McGettrick, Andrew and Sloan, Robert and Topi, Heikki and Davies, Gordon and Kamali, Reza and Cross, James and Impagliazzo, John and LeBlanc, Richard and Lunt, Barry},
	title = {Computing Curricula 2005: The Overview Report},
	journal = {SIGCSE Bull.},
	issue_date = {March 2006},
	volume = {38},
	number = {1},
	month = mar,
	year = {2006},
	issn = {0097-8418},
	pages = {456--457},
	numpages = {2},
	url = {http://doi.acm.org/10.1145/1124706.1121482},
	doi = {10.1145/1124706.1121482},
	acmid = {1121482},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {comparison of curriculum, computer engineering curriculum, computer science curriculum, computing curricula, information systems curriculum, information technology curriculum, software engineering curriculum},
} 

@book{Rajlich:2011:SEC:2077657,
	author = {Rajlich, Vaclav},
	title = {Software Engineering: The Current Practice},
	year = {2011},
	isbn = {1439841225, 9781439841228},
	edition = {1st},
	publisher = {Chapman \& Hall/CRC},
}

@article{10.1109/HICSS.2005.378,
	author = {Georg von Krogh and Sebastian Spaeth and Stefan Haefliger},
	title = {Knowledge Reuse in Open Source Software: An Exploratory Study of 15 Open Source Projects},
	journal ={Hawaii International Conference on System Sciences},
	volume = {7},
	issn = {1530-1605},
	year = {2005},
	pages = {198b},
	doi = {http://doi.ieeecomputersociety.org/10.1109/HICSS.2005.378},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{McMillan:2011:CSA:2117694.2119646,
	author = {McMillan, Collin and Linares-Vasquez, Mario and Poshyvanyk, Denys and Grechanik, Mark},
	title = {Categorizing software applications for maintenance},
	booktitle = {Proceedings of the 2011 27th IEEE International Conference on Software Maintenance},
	series = {ICSM '11},
	year = {2011},
	isbn = {978-1-4577-0663-9},
	pages = {343--352},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICSM.2011.6080801},
	doi = {10.1109/ICSM.2011.6080801},
	acmid = {2119646},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Grechanik:2010:EIL:1852786.1852801,
	author = {Grechanik, Mark and McMillan, Collin and DeFerrari, Luca and Comi, Marco and Crespi, Stefano and Poshyvanyk, Denys and Fu, Chen and Xie, Qing and Ghezzi, Carlo},
	title = {An empirical investigation into a large-scale Java open source code repository},
	booktitle = {Proceedings of the 2010 ACM-IEEE International Symposium on Empirical Software Engineering and Measurement},
	series = {ESEM '10},
	year = {2010},
	isbn = {978-1-4503-0039-1},
	location = {Bolzano-Bozen, Italy},
	pages = {11:1--11:10},
	articleno = {11},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1852786.1852801},
	doi = {10.1145/1852786.1852801},
	acmid = {1852801},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {empirical study, large-scale software, mining software repositories, open source, patterns, practice, software repository},
}

@inproceedings{Agichtein:2006:LUI:1148170.1148175,
	author = {Agichtein, Eugene and Brill, Eric and Dumais, Susan and Ragno, Robert},
	title = {Learning user interaction models for predicting web search result preferences},
	booktitle = {Proceedings of the 29th annual international ACM SIGIR conference on Research and development in information retrieval},
	series = {SIGIR '06},
	year = {2006},
	isbn = {1-59593-369-7},
	location = {Seattle, Washington, USA},
	pages = {3--10},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1148170.1148175},
	doi = {10.1145/1148170.1148175},
	acmid = {1148175},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {interpreting implicit relevance feedback, predicting relevance preferences, user behavior modeling},
} 

@article{Claypool:2001:IUI:613351.613651,
	author = {Claypool, Mark and Brown, David and Le, Phong and Waseda, Makoto},
	title = {Inferring User Interest},
	journal = {IEEE Internet Computing},
	issue_date = {November 2001},
	volume = {5},
	number = {6},
	month = nov,
	year = {2001},
	issn = {1089-7801},
	pages = {32--39},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/4236.968829},
	doi = {10.1109/4236.968829},
	acmid = {613651},
	publisher = {IEEE Educational Activities Department},
	address = {Piscataway, NJ, USA},
} 

@book{IR:08,
	author = {Manning, Christopher D. and Raghavan, Prabhakar and Schtze, Hinrich},
	title = {Introduction to Information Retrieval},
	year = {2008},
	isbn = {0521865719, 9780521865715},
	publisher = {Cambridge University Press},
	address = {New York, NY, USA}
}

@article{Likert1932,
	author = {Likert, R.A.},
	title= {A technique for the measurement of attitudes},
	year = {1932},
	journal = {Archives of Psychology},
	volume = {22},
	number = {140},
	pages = {5-55},
}

@article{Deerwester:jasis1990,
	Author = {S. Deerwester and S. T. Dumais and G. W. Furnas and T. K. Landauer and R. Harshman},
	Date-Added = {2007-08-31 12:57:51 +0200},
	Date-Modified = {2007-08-31 12:57:51 +0200},
	Journal = {Journal of the American Society for Information Science},
	Number = {6},
	Pages = {391-407},
	Title = {Indexing by Latent Semantic Analysis},
	Volume = {41},
	Year = {1990}
}

@inproceedings{Marcus:icse2003,
	Author = {A. Marcus and J. I. Maletic},
	Booktitle = {Proceedings of 25th International Conference on Software Engineering},
	Date-Added = {2007-08-31 12:57:51 +0200},
	Date-Modified = {2010-02-19 22:36:39 +0100},
	Pages = {125-135},
	Title = {Recovering Documentation-to-Source-Code Traceability Links using Latent Semantic Indexing},
	Year = {2003}
}

@book{Baeza-Yates:1999,
	Author = {R. Baeza-Yates and B. Ribeiro-Neto},
	Date-Added = {2007-08-31 12:57:51 +0200},
	Date-Modified = {2007-08-31 12:57:51 +0200},
	Publisher = {Addison-Wesley},
	Title = {Modern Information Retrieval},
	Year = {1999}
}

@article{Landi:1992:USA:161494.161501,
	author = {Landi, William},
	title = {Undecidability of static analysis},
	journal = {ACM Lett. Program. Lang. Syst.},
	issue_date = {Dec. 1992},
	volume = {1},
	number = {4},
	month = dec,
	year = {1992},
	issn = {1057-4514},
	pages = {323--337},
	numpages = {15},
	url = {http://doi.acm.org/10.1145/161494.161501},
	doi = {10.1145/161494.161501},
	acmid = {161501},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {abstract interpretation, alias analysis, data flow analysis, halting problem, static analysis},
}

@inproceedings{Biggerstaff:1993:CAP:257572.257679,
	author = {Biggerstaff, Ted J. and Mitbander, Bharat G. and Webster, Dallas},
	title = {The concept assignment problem in program understanding},
	booktitle = {Proceedings of the 15th international conference on Software Engineering},
	series = {ICSE '93},
	year = {1993},
	isbn = {0-89791-588-7},
	location = {Baltimore, Maryland, United States},
	pages = {482--498},
	numpages = {17},
	url = {http://dl.acm.org/citation.cfm?id=257572.257679},
	acmid = {257679},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
	keywords = {concept recognition, connectionist, domain, knowledge base, plausible reasoning, reverse engineering, slicing},
}

@article{Knight:1998:SQT:590631.590635,
	author = {Knight, John C. and Dunn, Michael F.},
	title = {Software quality through domain-driven certification},
	journal = {Ann. Softw. Eng.},
	issue_date = {1998},
	volume = {5},
	month = jan,
	year = {1998},
	issn = {1022-7091},
	pages = {293--315},
	numpages = {23},
	url = {http://dl.acm.org/citation.cfm?id=590631.590635},
	acmid = {590635},
	publisher = {J. C. Baltzer AG, Science Publishers},
	address = {Red Bank, NJ, USA},
}

@ARTICLE{62928,
	author={Barns, B.H. and Bollinger, T.B.},
	journal={Software, IEEE}, title={Making reuse cost-effective},
	year={1991},
	month={jan. },
	volume={8},
	number={1},
	pages={13 -24},
	keywords={consumer reuse;human problem solving;management;quality-of-investment;reuse investments;software reuse;DP management;software reusability;},
	doi={10.1109/52.62928},
	ISSN={0740-7459},}

@article{Banker:1991:RPI:120901.120908,
	author = {Banker, Rajiv D. and Kauffman, Robert J.},
	title = {Reuse and productivity in integrated computer-aided software engineering: an empirical study},
	journal = {MIS Q.},
	issue_date = {Sept. 1991},
	volume = {15},
	number = {3},
	month = oct,
	year = {1991},
	issn = {0276-7783},
	pages = {375--401},
	numpages = {27},
	url = {http://dx.doi.org/10.2307/249649},
	doi = {10.2307/249649},
	acmid = {120908},
	publisher = {Society for Information Management and The Management Information Systems Research Center},
	address = {Minneapolis, MN, USA},
	keywords = {CASE, ICASE, productivity measurement, reuse, software development, software economics, software engineering},
}

@article{10.1109/TSE.2011.84,
	author = {Collin McMillan and Mark Grechanik and Denys Poshyvanyk and Chen Fu and Qing Xie},
	title = {Exemplar: A Source Code Search Engine For Finding Highly Relevant Applications},
	journal ={IEEE Transactions on Software Engineering},
	volume = {99},
	number = {PrePrints},
	issn = {0098-5589},
	year = {2011},
	doi = {http://doi.ieeecomputersociety.org/10.1109/TSE.2011.84},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{Grechanik:2010:SEF:1806799.1806868,
	author = {Grechanik, Mark and Fu, Chen and Xie, Qing and McMillan, Collin and Poshyvanyk, Denys and Cumby, Chad},
	title = {A search engine for finding highly relevant applications},
	booktitle = {Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering - Volume 1},
	series = {ICSE '10},
	year = {2010},
	isbn = {978-1-60558-719-6},
	location = {Cape Town, South Africa},
	pages = {475--484},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1806799.1806868},
	doi = {10.1145/1806799.1806868},
	acmid = {1806868},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{McMillan:2011:PFR:1985793.1985809,
	author = {McMillan, Collin and Grechanik, Mark and Poshyvanyk, Denys and Xie, Qing and Fu, Chen},
	title = {Portfolio: finding relevant functions and their usage},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {111--120},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985809},
	doi = {10.1145/1985793.1985809},
	acmid = {1985809},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {code search, function call graph, pagerank, portfolio, ranking},
} 

@article{Mario:EMSE:13,
	author = {Mario Linares-Vasquez and Collin McMillan and Denys Poshyvanyk and Mark Grechanik},
	title = {On Using Machine Learning to Automatically Classify Software Applications into Domain Categories},
	journal ={Empirical Software Engineering},
	year = {2013},
	publisher = {EMSE},
	note = {To appear},
}

@electronic{BlinuxWebsite,
	author        = "Karl Dahlke",
	title         = "Blinux Website",
	url           = "http://leb.net/blinux/",
	year          = "2014"
}

@article{McMillan:Portfolio:TOSEM,
	author = {Collin McMillan and Mark Grechanik and Denys Poshyvanyk and Qing Xie and Chen Fu},
	title = {Searching for Relevant Functions and Their Usages in Millions of Lines of Code},
	journal ={ACM Transactions on Software Engineering and Methodology},
	year = {2012},
	doi = {http://doi.ieeecomputersociety.org/10.1109/TSE.2011.84},
	publisher = {ACM},
	note = {To appear},
}

@article {springerlink:10.1007/s10618-008-0118-x,
	author = {Linstead, Erik and Bajracharya, Sushil and Ngo, Trung and Rigor, Paul and Lopes, Cristina and Baldi, Pierre},
	affiliation = {University of California Donald Bren School of Information and Computer Sciences Irvine USA},
	title = {Sourcerer: mining and searching internet-scale software repositories},
	journal = {Data Mining and Knowledge Discovery},
	publisher = {Springer Netherlands},
	issn = {1384-5810},
	keyword = {Computer Science},
	pages = {300-336},
	volume = {18},
	issue = {2},
	url = {http://dx.doi.org/10.1007/s10618-008-0118-x},
	note = {10.1007/s10618-008-0118-x},
	year = {2009}
}

@inproceedings{CODEFINDER:96,
	author    = {Scott Henninger},
	title     = {Supporting the Construction and Evolution of Component Repositories.},
	booktitle = {ICSE},
	year      = {1996},
	pages     = {279-288},
	ee        = {http://portal.acm.org/citation.cfm?id=227726.227776},
}

@inproceedings{MICA:06,
	author    = {Jeffrey Stylos and
	Brad A. Myers},
	title     = {A Web-Search Tool for Finding \textsc{API} Components and Examples.},
	booktitle = {IEEE Symposium on VL and HCC},
	year      = {2006},
	pages     = {195-202},
}

@inproceedings{CODEBROKER:02,
	author    = {Yunwen Ye and
	Gerhard Fischer},
	title     = {Supporting reuse by delivering task-relevant and personalized
	information.},
	booktitle = {ICSE},
	year      = {2002},
	pages     = {513-523},
	ee        = {http://doi.acm.org/10.1145/581339.581402},
}

@article{HIPIKAT:05,
	author    = {Davor Cubranic and
	Gail C. Murphy and
	Janice Singer and
	Kellogg S. Booth},
	title     = {Hipikat: A Project Memory for Software Development.},
	journal   = {IEEE Trans. Software Eng.},
	volume    = {31},
	number    = {6},
	year      = {2005},
	pages     = {446-465},
	ee        = {http://dx.doi.org/10.1109/TSE.2005.71},
}

@inproceedings{Holmes:2007:SIP:1248820.1248877,
	author = {Holmes, Reid and Walker, Robert J.},
	title = {Supporting the Investigation and Planning of Pragmatic Reuse Tasks},
	booktitle = {Proceedings of the 29th international conference on Software Engineering},
	series = {ICSE '07},
	year = {2007},
	isbn = {0-7695-2828-7},
	pages = {447--457},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2007.83},
	doi = {10.1109/ICSE.2007.83},
	acmid = {1248877},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{STRATHCONA:05,
	author    = {Reid Holmes and
	Robert J. Walker and
	Gail C. Murphy},
	title     = {Strathcona example recommendation tool.},
	booktitle = {ESEC/FSE},
	year      = {2005},
	pages     = {237-240},
	ee        = {http://doi.acm.org/10.1145/1081706.1081744},
}

@article{SPARSJ:05,
	author = {Inoue, Katsuro and Yokomori, Reishi and Yamamoto, Tetsuo and Matsushita, Makoto and Kusumoto, Shinji},
	title = {Ranking Significance of Software Components Based on Use Relations},
	journal = {IEEE Trans. Softw. Eng.},
	volume = {31},
	number = {3},
	year = {2005},
	issn = {0098-5589},
	pages = {213--225},
	doi = {http://dx.doi.org/10.1109/TSE.2005.38},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@inproceedings{McMillan:2012:DSS:2337223.2337267,
	author = {McMillan, Collin and Grechanik, Mark and Poshyvanyk, Denys},
	title = {Detecting similar software applications},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {364--374},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337267},
	acmid = {2337267},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@inproceedings{SPOTWEB:08,
	author = {Thummalapenta, S. and Tao Xie},
	title = {SpotWeb: Detecting Framework Hotspots and Coldspots via Mining Open Source Code on the Web},
	booktitle = {ASE '08},
	year = {2008},
	isbn = {978-1-4244-2187-9},
	pages = {327--336},
	doi = {http://dx.doi.org/10.1109/ASE.2008.43},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{PROSPECTOR:05,
	author    = {David Mandelin and
	Lin Xu and
	Rastislav Bod\'{\i}k and
	Doug Kimelman},
	title     = {Jungloid mining: helping to navigate the \textsc{API} jungle.},
	booktitle = {PLDI},
	year      = {2005},
	pages     = {48-61},
	ee        = {http://doi.acm.org/10.1145/1065010.1065018},
}

@inproceedings{XSNIPPET:06,
	author    = {Naiyana Sahavechaphan and
	Kajal T. Claypool},
	title     = {\textsc{XS}nippet: mining For sample code.},
	booktitle = {OOPSLA},
	year      = {2006},
	pages     = {413-430},
	ee        = {http://doi.acm.org/10.1145/1167473.1167508},
}

@inproceedings{PARSEWEB:07,
	author = {Thummalapenta, Suresh and Xie, Tao},
	title = {Parseweb: a programmer assistant for reusing open source code on the web},
	booktitle = {ASE '07},
	year = {2007},
	isbn = {978-1-59593-882-4},
	pages = {204--213},
	location = {Atlanta, Georgia, USA},
	doi = {http://doi.acm.org/10.1145/1321631.1321663},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{MURPHY:05,
	author    = {Reid Holmes and
	Gail C. Murphy},
	title     = {Using structural context to recommend source code examples.},
	booktitle = {ICSE},
	year      = {2005},
	pages     = {117-125},
	ee        = {http://doi.acm.org/10.1145/1062455.1062491},
}

@inproceedings{S6:09,
	author    = {Steven P. Reiss},
	title     = {Semantics-based code search},
	booktitle = {ICSE},
	year      = {2009},
	pages     = {243-253},
	ee        = {http://dx.doi.org/10.1109/ICSE.2009.5070525},
}

@article{Hummel:2008:CCP:1439186.1439224,
	author = {Hummel, Oliver and Janjic, Werner and Atkinson, Colin},
	title = {Code Conjurer: Pulling Reusable Software out of Thin Air},
	journal = {IEEE Softw.},
	issue_date = {September 2008},
	volume = {25},
	number = {5},
	month = sep,
	year = {2008},
	issn = {0740-7459},
	pages = {45--52},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/MS.2008.110},
	doi = {10.1109/MS.2008.110},
	acmid = {1439224},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
} 

@article{Frakes:2005:SRR:1083823.1083997,
	author = {Frakes, William B. and Kang, Kyo},
	title = {Software Reuse Research: Status and Future},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {July 2005},
	volume = {31},
	number = {7},
	month = jul,
	year = {2005},
	issn = {0098-5589},
	pages = {529--536},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/TSE.2005.85},
	doi = {10.1109/TSE.2005.85},
	acmid = {1083997},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@BOOK{Arango:DomainAnalysis,
	AUTHOR = "G. Arango and R. Prieto-Diaz",
	TITLE = "Domain Analysis: Acquisition of Reusable Information for Software Construction",
	PUBLISHER ="IEEE Comp. Society Press",
	MONTH = "May",
	YEAR = {1989}
}
@ARTICLE{Frakes:DARE,
	AUTHOR = "W.B. Frakes and R. Prieto-Diaz and C.J. Fox",
	TITLE = "Dare: Domain Analysis and Reuse Environment",
	JOURNAL = "Annals of Software Eng.",
	PUBLISHER ="IEEE Computer Society Press",
	VOLUME = {5},
	YEAR = {1998}
}

@book{Weiss:1999:SPE:317887,
	author = {Weiss, David M. and Lai, Chi Tau Robert},
	title = {Software product-line engineering: a family-based software development process},
	year = {1999},
	isbn = {0-201-69438-7},
	publisher = {Addison-Wesley Longman Publishing Co., Inc.},
	address = {Boston, MA, USA},
}

@ARTICLE{1020288,
	author={Kang, K.C. and Jaejoon Lee and Donohoe, P.},
	journal={Software, IEEE}, title={Feature-oriented product line engineering},
	year={2002},
	month={jul/aug},
	volume={19},
	number={4},
	pages={ 58 - 65},
	keywords={ FORM; commonalities; differences; feature-oriented product line engineering; feature-oriented reuse method; home integration system; software development management; software reusability;},
	doi={10.1109/MS.2002.1020288},
	ISSN={0740-7459},
}

@article{Bajracharya:2012:AMC:2318097.2318150,
	author = {Bajracharya, Sushil Krishna and Lopes, Cristina Videira},
	title = {Analyzing and mining a code search engine usage log},
	journal = {Empirical Softw. Engg.},
	issue_date = {August 2012},
	volume = {17},
	number = {4-5},
	month = aug,
	year = {2012},
	issn = {1382-3256},
	pages = {424--466},
	numpages = {43},
	url = {http://dx.doi.org/10.1007/s10664-010-9144-6},
	doi = {10.1007/s10664-010-9144-6},
	acmid = {2318150},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Code search engine, Mining topics, Usage log analysis},
} 

@inproceedings{Linstead:2007:MCC:1321631.1321709,
	author = {Linstead, Erik and Rigor, Paul and Bajracharya, Sushil and Lopes, Cristina and Baldi, Pierre},
	title = {Mining concepts from code with probabilistic topic models},
	booktitle = {Proceedings of the twenty-second IEEE/ACM international conference on Automated software engineering},
	series = {ASE '07},
	year = {2007},
	isbn = {978-1-59593-882-4},
	location = {Atlanta, Georgia, USA},
	pages = {461--464},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1321631.1321709},
	doi = {10.1145/1321631.1321709},
	acmid = {1321709},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {mining software, program understanding, topic models},
} 

@inproceedings{McMillan:2012:RSC:2337223.2337323,
	author = {McMillan, Collin and Hariri, Negar and Poshyvanyk, Denys and Cleland-Huang, Jane and Mobasher, Bamshad},
	title = {Recommending source code for use in rapid software prototypes},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {848--858},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337323},
	acmid = {2337323},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@book{Gomaa:2004:DSP:983234,
	author = {Gomaa, Hassan},
	title = {Designing Software Product Lines with UML: From Use Cases to Pattern-Based Software Architectures},
	year = {2004},
	isbn = {0201775956},
	publisher = {Addison Wesley Longman Publishing Co., Inc.},
	address = {Redwood City, CA, USA},
}

@ARTICLE{Niu:Features2,
	AUTHOR="N.Niu and S.Easterbrook",
	TITLE="Extracting and Modeling Product Line Functional Requirements",
	JOURNAL="RE",
	LOCATION="Washington DC",
	YEAR ={2008},
}

@ARTICLE{Moon:Features3,
	AUTHOR="M.Moon and K.Yeom and H.S.Chae",
	TITLE="An approach to developing domain requirements as a core asset based on commonality and variability analysis in a product line",
	JOURNAL="TSE",
	VOLUME={31},
	ISSUE={7},
	YEAR={2005},
}

@inproceedings{Dumitru:11,
	author = {Dumitru, Horatiu and Gibiec, Marek and Hariri, Negar and Cleland-Huang, Jane and Mobasher, Bamshad and Castro-Herrera, Carlos and Mirakhorli, Mehdi},
	title = {On-demand feature recommendations derived from mining public product descriptions},
	booktitle = {ICSE},
	year = {2011},
	pages = {181--190},
}

@article{Holmes:2013:SPS:2377656.2377657,
	author = {Holmes, Reid and Walker, Robert J.},
	title = {Systematizing pragmatic software reuse},
	journal = {ACM Trans. Softw. Eng. Methodol.},
	issue_date = {November 2012},
	volume = {21},
	number = {4},
	month = feb,
	year = {2013},
	issn = {1049-331X},
	pages = {20:1--20:44},
	articleno = {20},
	numpages = {44},
	url = {http://doi.acm.org/10.1145/2377656.2377657},
	doi = {10.1145/2377656.2377657},
	acmid = {2377657},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Gilligan, Software reuse, lightweight process and tooling, low commitment, planning, pragmatic software reuse, pragmatic-reuse plan enactment, pragmatic-reuse plans, source code investigation, white box reuse},
} 

@inproceedings{Holmes:2009:ART:1747491.1747534,
	author = {Holmes, Reid and Ratchford, Tristan and Robillard, Martin P. and Walker, Robert J.},
	title = {Automatically Recommending Triage Decisions for Pragmatic Reuse Tasks},
	booktitle = {Proceedings of the 2009 IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '09},
	year = {2009},
	isbn = {978-0-7695-3891-4},
	pages = {397--408},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/ASE.2009.65},
	doi = {10.1109/ASE.2009.65},
	acmid = {1747534},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {pragmatic software reuse tasks, triage decisions, recommendation systems, structural relevance, cost, source code analysis, retroactive evaluation},
}

@inproceedings{Kotonya:2008:ORL:1478087.1478113,
	author = {Kotonya, Gerald and Lock, Simon and Mariani, John},
	title = {Opportunistic Reuse: Lessons from Scrapheap Software Development},
	booktitle = {Proceedings of the 11th International Symposium on Component-Based Software Engineering},
	series = {CBSE '08},
	year = {2008},
	isbn = {978-3-540-87890-2},
	location = {Karlsruhe, Germany},
	pages = {302--309},
	numpages = {8},
	url = {http://dx.doi.org/10.1007/978-3-540-87891-9_20},
	doi = {10.1007/978-3-540-87891-9_20},
	acmid = {1478113},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
}

@inproceedings{Brandt:2010:EPI:1753326.1753402,
	author = {Brandt, Joel and Dontcheva, Mira and Weskamp, Marcos and Klemmer, Scott R.},
	title = {Example-centric programming: integrating web search into the development environment},
	booktitle = {Proceedings of the 28th international conference on Human factors in computing systems},
	series = {CHI '10},
	year = {2010},
	isbn = {978-1-60558-929-9},
	location = {Atlanta, Georgia, USA},
	pages = {513--522},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1753326.1753402},
	doi = {10.1145/1753326.1753402},
	acmid = {1753402},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {example-centric development},
}

@inproceedings{Hartmann:2010:OPS:1753326.1753478,
	author = {Hartmann, Bj\"{o}rn and MacDougall, Daniel and Brandt, Joel and Klemmer, Scott R.},
	title = {What would other programmers do: suggesting solutions to error messages},
	booktitle = {Proceedings of the 28th international conference on Human factors in computing systems},
	series = {CHI '10},
	year = {2010},
	isbn = {978-1-60558-929-9},
	location = {Atlanta, Georgia, USA},
	pages = {1019--1028},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1753326.1753478},
	doi = {10.1145/1753326.1753478},
	acmid = {1753478},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, recommender systems},
}

@inproceedings{Weiser:1981:PS:800078.802557,
	author = {Weiser, Mark},
	title = {Program slicing},
	booktitle = {Proceedings of the 5th international conference on Software engineering},
	series = {ICSE '81},
	year = {1981},
	isbn = {0-89791-146-6},
	location = {San Diego, California, United States},
	pages = {439--449},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=800078.802557},
	acmid = {802557},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Data flow analysis, Debugging, Human factors, Program maintenance, Program metrics, Software tools},
}

@article{DBLP:journals/tse/Weiser84,
	author    = {Mark Weiser},
	title     = {Program Slicing},
	journal   = {IEEE Trans. Software Eng.},
	volume    = {10},
	number    = {4},
	year      = {1984},
	pages     = {352-357},
	ee        = {http://doi.ieeecomputersociety.org/10.1109/TSE.1984.5010248},
	bibsource = {DBLP, http://dblp.uni-trier.de}
} 

@article{Horwitz:1988:ISU:960116.53994,
	author = {Horwitz, S. and Reps, T. and Binkley, D.},
	title = {Interprocedural slicing using dependence graphs},
	journal = {SIGPLAN Not.},
	issue_date = {July 1988},
	volume = {23},
	number = {7},
	month = jun,
	year = {1988},
	issn = {0362-1340},
	pages = {35--46},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/960116.53994},
	doi = {10.1145/960116.53994},
	acmid = {53994},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Horwitz:1988:ISU:53990.53994,
	author = {Horwitz, S. and Reps, T. and Binkley, D.},
	title = {Interprocedural slicing using dependence graphs},
	booktitle = {Proceedings of the ACM SIGPLAN 1988 conference on Programming Language design and Implementation},
	series = {PLDI '88},
	year = {1988},
	isbn = {0-89791-269-1},
	location = {Atlanta, Georgia, United States},
	pages = {35--46},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/53990.53994},
	doi = {10.1145/53990.53994},
	acmid = {53994},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Malenfant:2001:FAD:846228.848706,
	author = {Malenfant, Bruno},
	title = {Flow Analysis to Detect Blocked Statements},
	booktitle = {Proceedings of the IEEE International Conference on Software Maintenance (ICSM'01)},
	series = {ICSM '01},
	year = {2001},
	isbn = {0-7695-1189-9},
	pages = {62--},
	url = {http://dx.doi.org/10.1109/ICSM.2001.972712},
	doi = {10.1109/ICSM.2001.972712},
	acmid = {848706},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {Blocking analysis, inter-procedural flow analysis, software evaluation},
}

@article{Horwitz:1990:ISU:77606.77608,
	author = {Horwitz, Susan and Reps, Thomas and Binkley, David},
	title = {Interprocedural slicing using dependence graphs},
	journal = {ACM Trans. Program. Lang. Syst.},
	issue_date = {Jan. 1990},
	volume = {12},
	number = {1},
	month = jan,
	year = {1990},
	issn = {0164-0925},
	pages = {26--60},
	numpages = {35},
	url = {http://doi.acm.org/10.1145/77606.77608},
	doi = {10.1145/77606.77608},
	acmid = {77608},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Mock:2005:PSD:1083824.1084006,
	author = {Mock, Markus and Atkinson, Darren C. and Chambers, Craig and Eggers, Susan J.},
	title = {Program Slicing with Dynamic Points-To Sets},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {August 2005},
	volume = {31},
	number = {8},
	month = aug,
	year = {2005},
	issn = {0098-5589},
	pages = {657--678},
	numpages = {22},
	url = {http://dx.doi.org/10.1109/TSE.2005.94},
	doi = {10.1109/TSE.2005.94},
	acmid = {1084006},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Index Terms- Dynamic analysis, Index Terms- Dynamic analysis, points-to analysis, program slicing., points-to analysis, program slicing.},
} 

@inproceedings{Venkatesh:1991:SAP:113445.113455,
	author = {Venkatesh, G. A.},
	title = {The semantic approach to program slicing},
	booktitle = {Proceedings of the ACM SIGPLAN 1991 conference on Programming language design and implementation},
	series = {PLDI '91},
	year = {1991},
	isbn = {0-89791-428-7},
	location = {Toronto, Ontario, Canada},
	pages = {107--119},
	numpages = {13},
	url = {http://doi.acm.org/10.1145/113445.113455},
	doi = {10.1145/113445.113455},
	acmid = {113455},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Krinke:1998:SST:277631.277638,
	author = {Krinke, Jens},
	title = {Static slicing of threaded programs},
	booktitle = {Proceedings of the 1998 ACM SIGPLAN-SIGSOFT workshop on Program analysis for software tools and engineering},
	series = {PASTE '98},
	year = {1998},
	isbn = {1-58113-055-4},
	location = {Montreal, Quebec, Canada},
	pages = {35--42},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/277631.277638},
	doi = {10.1145/277631.277638},
	acmid = {277638},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Giffhorn:2009:PSC:1530080.1530094,
	author = {Giffhorn, Dennis and Hammer, Christian},
	title = {Precise slicing of concurrent programs},
	journal = {Automated Software Engg.},
	issue_date = {June      2009},
	volume = {16},
	number = {2},
	month = jun,
	year = {2009},
	issn = {0928-8910},
	pages = {197--234},
	numpages = {38},
	url = {http://dx.doi.org/10.1007/s10515-009-0048-x},
	doi = {10.1007/s10515-009-0048-x},
	acmid = {1530094},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Concurrency, Program analysis, Slicing, Threads},
}

@article{Binkley:2007:ESS:1217295.1217297,
	author = {Binkley, David and Gold, Nicolas and Harman, Mark},
	title = {An empirical study of static program slice size},
	journal = {ACM Trans. Softw. Eng. Methodol.},
	issue_date = {April 2007},
	volume = {16},
	number = {2},
	month = apr,
	year = {2007},
	issn = {1049-331X},
	articleno = {8},
	url = {http://doi.acm.org/10.1145/1217295.1217297},
	doi = {10.1145/1217295.1217297},
	acmid = {1217297},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Program slicing, slice size},
} 

@article{Agrawal:1990:DPS:93548.93576,
	author = {Agrawal, Hiralal and Horgan, Joseph R.},
	title = {Dynamic program slicing},
	journal = {SIGPLAN Not.},
	issue_date = {Jun. 1990},
	volume = {25},
	number = {6},
	month = jun,
	year = {1990},
	issn = {0362-1340},
	pages = {246--256},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/93548.93576},
	doi = {10.1145/93548.93576},
	acmid = {93576},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Binkley:2007:ESO:1290520.1290523,
	author = {Binkley, David and Harman, Mark and Krinke, Jens},
	title = {Empirical study of optimization techniques for massive slicing},
	journal = {ACM Trans. Program. Lang. Syst.},
	issue_date = {November 2007},
	volume = {30},
	number = {1},
	month = nov,
	year = {2007},
	issn = {0164-0925},
	articleno = {3},
	url = {http://doi.acm.org/10.1145/1290520.1290523},
	doi = {10.1145/1290520.1290523},
	acmid = {1290523},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Slicing, empirical study, internal representation, performance enhancement},
}

@article{Krinke:2006:ECP:1167771.1167775,
	author = {Krinke, Jens},
	title = {Effects of context on program slicing},
	journal = {J. Syst. Softw.},
	issue_date = {September 2006},
	volume = {79},
	number = {9},
	month = sep,
	year = {2006},
	issn = {0164-1212},
	pages = {1249--1260},
	numpages = {12},
	url = {http://dx.doi.org/10.1016/j.jss.2006.02.040},
	doi = {10.1016/j.jss.2006.02.040},
	acmid = {1167775},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {program analysis, program slicing},
}

@article{Canfora1998595,
	title = "Conditioned program slicing",
	journal = "Information and Software Technology",
	volume = "40",
	number = "11–12",
	pages = "595 - 607",
	year = "1998",
	note = "",
	issn = "0950-5849",
	doi = "10.1016/S0950-5849(98)00086-X",
	url = "http://www.sciencedirect.com/science/article/pii/S095058499800086X",
	author = "Gerardo Canfora and Aniello Cimitile and Andrea De Lucia",
}

@article{Korel:1997:CDP:249578.249587,
	author = {Korel, Bogdan},
	title = {Computation of Dynamic Program Slices for Unstructured Programs},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {January 1997},
	volume = {23},
	number = {1},
	month = jan,
	year = {1997},
	issn = {0098-5589},
	pages = {17--34},
	numpages = {18},
	url = {http://dx.doi.org/10.1109/32.581327},
	doi = {10.1109/32.581327},
	acmid = {249587},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Program slicing, dynamic program slicing, removable block, control dependence, data dependence, execution trace, unstructured program, debugging.},
} 

@article{DBLP:journals/infsof/KorelR98,
	author    = {Bogdan Korel and
	Juergen Rilling},
	title     = {Dynamic program slicing methods},
	journal   = {Information {\&} Software Technology},
	volume    = {40},
	number    = {11-12},
	year      = {1998},
	pages     = {647-659},
	ee        = {http://dx.doi.org/10.1016/S0950-5849(98)00089-5},
	bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{Xu:2005:BSP:1050849.1050865,
	author = {Xu, Baowen and Qian, Ju and Zhang, Xiaofang and Wu, Zhongqiang and Chen, Lin},
	title = {A brief survey of program slicing},
	journal = {SIGSOFT Softw. Eng. Notes},
	issue_date = {March 2005},
	volume = {30},
	number = {2},
	month = mar,
	year = {2005},
	issn = {0163-5948},
	pages = {1--36},
	numpages = {36},
	url = {http://doi.acm.org/10.1145/1050849.1050865},
	doi = {10.1145/1050849.1050865},
	acmid = {1050865},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, dependence analysis, pointer analysis, program analysis, program slicing},
}

@techreport{
	yiji_2012_tr,
	author = "Yiji Zhang and Raul Santelices",
	institution = "University of Notre Dame Computer Science Department",
	title = "Predicting Runtime Data Dependences for Slice Inspection Prioritization",
	number = "2012-02",
	month = "July",
	year = "2012"
}

@inproceedings{Zhang:2006:PDS:1133981.1134002,
	author = {Zhang, Xiangyu and Gupta, Neelam and Gupta, Rajiv},
	title = {Pruning dynamic slices with confidence},
	booktitle = {Proceedings of the 2006 ACM SIGPLAN conference on Programming language design and implementation},
	series = {PLDI '06},
	year = {2006},
	isbn = {1-59593-320-4},
	location = {Ottawa, Ontario, Canada},
	pages = {169--180},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1133981.1134002},
	doi = {10.1145/1133981.1134002},
	acmid = {1134002},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {data and control dependences, debugging, dynamic slicing},
}

@inproceedings{Sridharan:2007:TS:1250734.1250748,
	author = {Sridharan, Manu and Fink, Stephen J. and Bodik, Rastislav},
	title = {Thin slicing},
	booktitle = {Proceedings of the 2007 ACM SIGPLAN conference on Programming language design and implementation},
	series = {PLDI '07},
	year = {2007},
	isbn = {978-1-59593-633-2},
	location = {San Diego, California, USA},
	pages = {112--122},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1250734.1250748},
	doi = {10.1145/1250734.1250748},
	acmid = {1250748},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, program understanding, slicing},
}

@article{Gallagher:1991:UPS:126244.126248,
	author = {Gallagher, Keith Brian and Lyle, James R.},
	title = {Using Program Slicing in Software Maintenance},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {August 1991},
	volume = {17},
	number = {8},
	month = aug,
	year = {1991},
	issn = {0098-5589},
	pages = {751--761},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/32.83912},
	doi = {10.1109/32.83912},
	acmid = {126248},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {line number, linear time, program slice, program slicing, program testing, semantically consistent changes, set inclusion, single variable decomposition slices, slice-based decomposition, software maintenance, software maintenance problem, unmodified components},
}

@inproceedings{Robillard:2002:CGF:581339.581390,
	author = {Robillard, Martin P. and Murphy, Gail C.},
	title = {Concern graphs: finding and describing concerns using structural program dependencies},
	booktitle = {Proceedings of the 24th International Conference on Software Engineering},
	series = {ICSE '02},
	year = {2002},
	isbn = {1-58113-472-X},
	location = {Orlando, Florida},
	pages = {406--416},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/581339.581390},
	doi = {10.1145/581339.581390},
	acmid = {581390},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Mund:2006:EID:1150566.1150570,
	author = {Mund, G. B. and Mall, Rajib},
	title = {An efficient interprocedural dynamic slicing method},
	journal = {J. Syst. Softw.},
	issue_date = {June 2006},
	volume = {79},
	number = {6},
	month = jun,
	year = {2006},
	issn = {0164-1212},
	pages = {791--806},
	numpages = {16},
	url = {http://dx.doi.org/10.1016/j.jss.2005.07.024},
	doi = {10.1016/j.jss.2005.07.024},
	acmid = {1150570},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {Control dependence graph, Control flow graph, Dynamic slicing, Program debugging, Program dependence graph, Program slicing, Static slicing},
}

@inproceedings{Dunn:1993:ADR:257572.257660,
	author = {Dunn, Michael F. and Knight, John C.},
	title = {Automating the detection of reusable parts in existing software},
	booktitle = {Proceedings of the 15th international conference on Software Engineering},
	series = {ICSE '93},
	year = {1993},
	isbn = {0-89791-588-7},
	location = {Baltimore, Maryland, United States},
	pages = {381--390},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=257572.257660},
	acmid = {257660},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
	keywords = {Prolog, expert system, reengineering, reusable components, software reuse},
}

@article{Zhang:2010:BAH:1944279.1944280,
	author = {Zhang, Lu and Luo, Jing and Li, He and Sun, Jiasu and Mei, Hong},
	title = {A biting-down approach to hierarchical decomposition of object-oriented systems based on structure analysis},
	journal = {J. Softw. Maint. Evol.},
	issue_date = {December 2010},
	volume = {22},
	number = {8},
	month = dec,
	year = {2010},
	issn = {1532-060X},
	pages = {567--596},
	numpages = {30},
	url = {http://dx.doi.org/10.1002/smr.417},
	doi = {10.1002/smr.417},
	acmid = {1944280},
	publisher = {John Wiley \& Sons, Inc.},
	address = {New York, NY, USA},
	keywords = {architecture recovery, hierarchical system decomposition, software clustering},
}

@article{Caldiera:1991:IQR:103293.103294,
	author = {Caldiera, Gianluigi and Basili, Victor R.},
	title = {Identifying and Qualifying Reusable Software Components},
	journal = {Computer},
	issue_date = {February 1991},
	volume = {24},
	number = {2},
	month = feb,
	year = {1991},
	issn = {0018-9162},
	pages = {61--70},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/2.67210},
	doi = {10.1109/2.67210},
	acmid = {103294},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{Schach:1995:MTC:315891.316024,
	author = {Schach, Stephen R. and Yang, Xuefeng},
	title = {Metrics for targeting candidates for reuse: an experimental approach},
	booktitle = {Proceedings of the 1995 ACM symposium on Applied computing},
	series = {SAC '95},
	year = {1995},
	isbn = {0-89791-658-1},
	location = {Nashville, Tennessee, United States},
	pages = {379--383},
	numpages = {5},
	url = {http://doi.acm.org/10.1145/315891.316024},
	doi = {10.1145/315891.316024},
	acmid = {316024},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {accidental reuse, experimentation, reusability, software metrics},
}

@article{Roemer:2012:RPS:2133375.2133377,
	author = {Roemer, Ryan and Buchanan, Erik and Shacham, Hovav and Savage, Stefan},
	title = {Return-Oriented Programming: Systems, Languages, and Applications},
	journal = {ACM Trans. Inf. Syst. Secur.},
	issue_date = {March 2012},
	volume = {15},
	number = {1},
	month = mar,
	year = {2012},
	issn = {1094-9224},
	pages = {2:1--2:34},
	articleno = {2},
	numpages = {34},
	url = {http://doi.acm.org/10.1145/2133375.2133377},
	doi = {10.1145/2133375.2133377},
	acmid = {2133377},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {NX, RISC, Return-oriented programming, SPARC, W-xor-X, attacks, control flow integrity, memory safety, return-into-libc, x86},
}

@inproceedings{Checkoway:2010:RPW:1866307.1866370,
	author = {Checkoway, Stephen and Davi, Lucas and Dmitrienko, Alexandra and Sadeghi, Ahmad-Reza and Shacham, Hovav and Winandy, Marcel},
	title = {Return-oriented programming without returns},
	booktitle = {Proceedings of the 17th ACM conference on Computer and communications security},
	series = {CCS '10},
	year = {2010},
	isbn = {978-1-4503-0245-6},
	location = {Chicago, Illinois, USA},
	pages = {559--572},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/1866307.1866370},
	doi = {10.1145/1866307.1866370},
	acmid = {1866370},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {arm, return-oriented programming, x86},
}

@inproceedings{Chen:2010:EDR:1940366.1940380,
	author = {Chen, Ping and Xing, Xiao and Han, Hao and Mao, Bing and Xie, Li},
	title = {Efficient detection of the return-oriented programming malicious code},
	booktitle = {Proceedings of the 6th international conference on Information systems security},
	series = {ICISS'10},
	year = {2010},
	isbn = {3-642-17713-1, 978-3-642-17713-2},
	location = {Gandhinagar, India},
	pages = {140--155},
	numpages = {16},
	url = {http://dl.acm.org/citation.cfm?id=1940366.1940380},
	acmid = {1940380},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
}

@inproceedings{Bletsch:2011:JPN:1966913.1966919,
	author = {Bletsch, Tyler and Jiang, Xuxian and Freeh, Vince W. and Liang, Zhenkai},
	title = {Jump-oriented programming: a new class of code-reuse attack},
	booktitle = {Proceedings of the 6th ACM Symposium on Information, Computer and Communications Security},
	series = {ASIACCS '11},
	year = {2011},
	isbn = {978-1-4503-0564-8},
	location = {Hong Kong, China},
	pages = {30--40},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1966913.1966919},
	doi = {10.1145/1966913.1966919},
	acmid = {1966919},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@INPROCEEDINGS{mohan12woot,
	author = "Vishwath Mohan and Kevin W. Hamlen",
	title = "{Frankenstein}: Stitching Malware from Benign Binaries",
	booktitle = "Proceedings of the 6th USENIX Workshop on Offensive Technologies (WOOT)",
	address = "Bellevue, Washington",
	month = "August",
	year = 2012,
}

@article{Il68,
	added-at = {2006-11-21T05:45:44.000+0100},
	author = {McIlroy, M. D.},
	biburl = {http://www.bibsonomy.org/bibtex/2bdd8dc73582a1061c5353c143b85bb9e/berger},
	chapter = 14,
	interhash = {f27eb07f75ede5abc8af427c9d186453},
	intrahash = {bdd8dc73582a1061c5353c143b85bb9e},
	journal = {Proc. NATO Conf. on Software Engineering, Garmisch, Germany},
	keywords = {Software-Engineering},
	publisher = {Springer-Verlag},
	timestamp = {2006-11-21T05:45:44.000+0100},
	title = {Mass-produced software components},
	year = 1968
}

@INPROCEEDINGS{Howison04theperils,
	author = {James Howison and Kevin Crowston},
	title = {The perils and pitfalls of mining SourceForge},
	booktitle = {In Proceedings of the International Workshop on Mining Software Repositories (MSR 2004},
	year = {2004},
	pages = {7--11}
}

@article{Dunlap:2002:REI:844128.844148,
	author = {Dunlap, George W. and King, Samuel T. and Cinar, Sukru and Basrai, Murtaza A. and Chen, Peter M.},
	title = {ReVirt: enabling intrusion analysis through virtual-machine logging and replay},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {Winter 2002},
	volume = {36},
	number = {SI},
	month = dec,
	year = {2002},
	issn = {0163-5980},
	pages = {211--224},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/844128.844148},
	doi = {10.1145/844128.844148},
	acmid = {844148},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@misc{GDB:Website,
	author = {GNU},
	title = {The GNU Project Debugger},
	month = sep,
	year = {2012},
	note = {http://www.gnu.org/software/gdb/}
}

@article{LeBlanc:1987:DPP:32387.32396,
	author = {LeBlanc, T. J. and Mellor-Crummey, J. M.},
	title = {Debugging Parallel Programs with Instant Replay},
	journal = {IEEE Trans. Comput.},
	issue_date = {April 1987},
	volume = {36},
	number = {4},
	month = apr,
	year = {1987},
	issn = {0018-9340},
	pages = {471--482},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/TC.1987.1676929},
	doi = {10.1109/TC.1987.1676929},
	acmid = {32396},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {CREW protocols, distributed debugging, execution replay, parallel programming, program instrumentation, shared objects, shared objects, CREW protocols, distributed debugging, execution replay, parallel programming, program instrumentation},
}

@inproceedings{Balzer:1969:EED:1476793.1476881,
	author = {Balzer, R. M.},
	title = {EXDAMS: extendable debugging and monitoring system},
	booktitle = {Proceedings of the May 14-16, 1969, spring joint computer conference},
	series = {AFIPS '69 (Spring)},
	year = {1969},
	location = {Boston, Massachusetts},
	pages = {567--580},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/1476793.1476881},
	doi = {10.1145/1476793.1476881},
	acmid = {1476881},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Bacon:1991:HRM:122759.122777,
	author = {Bacon, David F. and Goldstein, Seth Copen},
	title = {Hardware-assisted replay of multiprocessor programs},
	booktitle = {Proceedings of the 1991 ACM/ONR workshop on Parallel and distributed debugging},
	series = {PADD '91},
	year = {1991},
	isbn = {0-89791-457-0},
	location = {Santa Cruz, California, United States},
	pages = {194--206},
	numpages = {13},
	url = {http://doi.acm.org/10.1145/122759.122777},
	doi = {10.1145/122759.122777},
	acmid = {122777},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Devietti:2009:DDS:1508244.1508255,
	author = {Devietti, Joseph and Lucia, Brandon and Ceze, Luis and Oskin, Mark},
	title = {DMP: deterministic shared memory multiprocessing},
	booktitle = {Proceedings of the 14th international conference on Architectural support for programming languages and operating systems},
	series = {ASPLOS '09},
	year = {2009},
	isbn = {978-1-60558-406-5},
	location = {Washington, DC, USA},
	pages = {85--96},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1508244.1508255},
	doi = {10.1145/1508244.1508255},
	acmid = {1508255},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, determinism, multicores, parallel programming},
}

@inproceedings{Hower:2008:REE:1381306.1382144,
	author = {Hower, Derek R. and Hill, Mark D.},
	title = {Rerun: Exploiting Episodes for Lightweight Memory Race Recording},
	booktitle = {Proceedings of the 35th Annual International Symposium on Computer Architecture},
	series = {ISCA '08},
	year = {2008},
	isbn = {978-0-7695-3174-8},
	pages = {265--276},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/ISCA.2008.26},
	doi = {10.1109/ISCA.2008.26},
	acmid = {1382144},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {Multicore, Determinism, Race Recording},
}

@inproceedings{Montesinos:2008:DRD:1381306.1382146,
	author = {Montesinos, Pablo and Ceze, Luis and Torrellas, Josep},
	title = {DeLorean: Recording and Deterministically Replaying Shared-Memory Multiprocessor Execution Ef?ciently},
	booktitle = {Proceedings of the 35th Annual International Symposium on Computer Architecture},
	series = {ISCA '08},
	year = {2008},
	isbn = {978-0-7695-3174-8},
	pages = {289--300},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/ISCA.2008.36},
	doi = {10.1109/ISCA.2008.36},
	acmid = {1382146},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Montesinos:2009:CSI:1508244.1508254,
	author = {Montesinos, Pablo and Hicks, Matthew and King, Samuel T. and Torrellas, Josep},
	title = {Capo: a software-hardware interface for practical deterministic multiprocessor replay},
	booktitle = {Proceedings of the 14th international conference on Architectural support for programming languages and operating systems},
	series = {ASPLOS '09},
	year = {2009},
	isbn = {978-1-60558-406-5},
	location = {Washington, DC, USA},
	pages = {73--84},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1508244.1508254},
	doi = {10.1145/1508244.1508254},
	acmid = {1508254},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {capo, capoone, deterministic replay, replay sphere},
}

@article{Narayanasamy:2006:RSM:1168917.1168886,
	author = {Narayanasamy, Satish and Pereira, Cristiano and Calder, Brad},
	title = {Recording shared memory dependencies using strata},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {December 2006},
	volume = {40},
	number = {5},
	month = oct,
	year = {2006},
	issn = {0163-5980},
	pages = {229--240},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1168917.1168886},
	doi = {10.1145/1168917.1168886},
	acmid = {1168886},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, dependencies, logging, replay, shared memory, strata},
}

@article{Narayanasamy:2005:BCR:1080695.1069994,
	author = {Narayanasamy, Satish and Pokam, Gilles and Calder, Brad},
	title = {BugNet: Continuously Recording Program Execution for Deterministic Replay Debugging},
	journal = {SIGARCH Comput. Archit. News},
	issue_date = {May 2005},
	volume = {33},
	number = {2},
	month = may,
	year = {2005},
	issn = {0163-5964},
	pages = {284--295},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1080695.1069994},
	doi = {10.1145/1080695.1069994},
	acmid = {1069994},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Olszewski:2009:KED:1508284.1508256,
	author = {Olszewski, Marek and Ansel, Jason and Amarasinghe, Saman},
	title = {Kendo: efficient deterministic multithreading in software},
	journal = {SIGPLAN Not.},
	issue_date = {March 2009},
	volume = {44},
	number = {3},
	month = mar,
	year = {2009},
	issn = {0362-1340},
	pages = {97--108},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1508284.1508256},
	doi = {10.1145/1508284.1508256},
	acmid = {1508256},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, determinism, deterministic multithreading, multicore, parallel programming},
}

@article{Bressoud:1996:HFT:225535.225538,
	author = {Bressoud, Thomas C. and Schneider, Fred B.},
	title = {Hypervisor-based fault tolerance},
	journal = {ACM Trans. Comput. Syst.},
	issue_date = {Feb. 1996},
	volume = {14},
	number = {1},
	month = feb,
	year = {1996},
	issn = {0734-2071},
	pages = {80--107},
	numpages = {28},
	url = {http://doi.acm.org/10.1145/225535.225538},
	doi = {10.1145/225535.225538},
	acmid = {225538},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {fault-tolerant computing system, primary/backup approach, virtual-machine manager},
}

@inproceedings{Dunlap:2008:ERM:1346256.1346273,
	author = {Dunlap, George W. and Lucchetti, Dominic G. and Fetterman, Michael A. and Chen, Peter M.},
	title = {Execution replay of multiprocessor virtual machines},
	booktitle = {Proceedings of the fourth ACM SIGPLAN/SIGOPS international conference on Virtual execution environments},
	series = {VEE '08},
	year = {2008},
	isbn = {978-1-59593-796-4},
	location = {Seattle, WA, USA},
	pages = {121--130},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1346256.1346273},
	doi = {10.1145/1346256.1346273},
	acmid = {1346273},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {ReVirt, Xen, determinism, direct memory access, execution replay, hardware page protections, multiprocessors, multithreading, virtual machines},
}

@article{Chow:2010:MRC:1837854.1736002,
	author = {Chow, Jim and Lucchetti, Dominic and Garfinkel, Tal and Lefebvre, Geoffrey and Gardner, Ryan and Mason, Joshua and Small, Sam and Chen, Peter M.},
	title = {Multi-stage replay with crosscut},
	journal = {SIGPLAN Not.},
	issue_date = {July 2010},
	volume = {45},
	number = {7},
	month = mar,
	year = {2010},
	issn = {0362-1340},
	pages = {13--24},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1837854.1736002},
	doi = {10.1145/1837854.1736002},
	acmid = {1736002},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {design, experimentation, performance, replay, security, virtual machines},
}

@inproceedings{Geels:2006:RDD:1267359.1267386,
	author = {Geels, Dennis and Altekar, Gautam and Shenker, Scott and Stoica, Ion},
	title = {Replay debugging for distributed applications},
	booktitle = {Proceedings of the annual conference on USENIX '06 Annual Technical Conference},
	series = {ATEC '06},
	year = {2006},
	location = {Boston, MA},
	pages = {27--27},
	numpages = {1},
	url = {http://dl.acm.org/citation.cfm?id=1267359.1267386},
	acmid = {1267386},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
}

@inproceedings{Guo:2008:RAK:1855741.1855755,
	author = {Guo, Zhenyu and Wang, Xi and Tang, Jian and Liu, Xuezheng and Xu, Zhilei and Wu, Ming and Kaashoek, M. Frans and Zhang, Zheng},
	title = {R2: an application-level kernel for record and replay},
	booktitle = {Proceedings of the 8th USENIX conference on Operating systems design and implementation},
	series = {OSDI'08},
	year = {2008},
	location = {San Diego, California},
	pages = {193--208},
	numpages = {16},
	url = {http://dl.acm.org/citation.cfm?id=1855741.1855755},
	acmid = {1855755},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
}

@inproceedings{Saito:2005:JUL:1085130.1085139,
	author = {Saito, Yasushi},
	title = {Jockey: a user-space library for record-replay debugging},
	booktitle = {Proceedings of the sixth international symposium on Automated analysis-driven debugging},
	series = {AADEBUG'05},
	year = {2005},
	isbn = {1-59593-050-7},
	location = {Monterey, California, USA},
	pages = {69--76},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1085130.1085139},
	doi = {10.1145/1085130.1085139},
	acmid = {1085139},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Linux, checkpointing, debugging, execution record and replay, jockey, keywords, x86},
}

@inproceedings{Choi:1998:DRJ:281035.281041,
	author = {Choi, Jong-Deok and Srinivasan, Harini},
	title = {Deterministic replay of Java multithreaded applications},
	booktitle = {Proceedings of the SIGMETRICS symposium on Parallel and distributed tools},
	series = {SPDT '98},
	year = {1998},
	isbn = {1-58113-001-5},
	location = {Welches, Oregon, United States},
	pages = {48--59},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/281035.281041},
	doi = {10.1145/281035.281041},
	acmid = {281041},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Russinovich:1996:RCN:249069.231432,
	author = {Russinovich, Mark and Cogswell, Bryce},
	title = {Replay for concurrent non-deterministic shared-memory applications},
	journal = {SIGPLAN Not.},
	issue_date = {May 1996},
	volume = {31},
	number = {5},
	month = may,
	year = {1996},
	issn = {0362-1340},
	pages = {258--266},
	numpages = {9},
	url = {http://doi.acm.org/10.1145/249069.231432},
	doi = {10.1145/249069.231432},
	acmid = {231432},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {instruction counter, non-determinism, repeatable execution, shared memory},
}

@inproceedings{Bergheaud:2007:FTM:1270387.1270855,
	author = {Bergheaud, Philippe and Subhraveti, Dinesh and Vertes, Marc},
	title = {Fault Tolerance in Multiprocessor Systems Via Application Cloning},
	booktitle = {Proceedings of the 27th International Conference on Distributed Computing Systems},
	series = {ICDCS '07},
	year = {2007},
	isbn = {0-7695-2837-3},
	pages = {21--},
	url = {http://dx.doi.org/10.1109/ICDCS.2007.111},
	doi = {10.1109/ICDCS.2007.111},
	acmid = {1270855},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Bressoud:1998:TSS:795671.796914,
	author = {Bressoud, T. C.},
	title = {TFT: A Software System for Application-Transparent Fault Tolerance},
	booktitle = {Proceedings of the The Twenty-Eighth Annual International Symposium on Fault-Tolerant Computing},
	series = {FTCS '98},
	year = {1998},
	isbn = {0-8186-8470-4},
	pages = {128--},
	url = {http://dl.acm.org/citation.cfm?id=795671.796914},
	acmid = {796914},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Bressoud:1998:TSS:795671.796914,
	author = {Bressoud, T. C.},
	title = {TFT: A Software System for Application-Transparent Fault Tolerance},
	booktitle = {Proceedings of the The Twenty-Eighth Annual International Symposium on Fault-Tolerant Computing},
	series = {FTCS '98},
	year = {1998},
	isbn = {0-8186-8470-4},
	pages = {128--},
	url = {http://dl.acm.org/citation.cfm?id=795671.796914},
	acmid = {796914},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Srinivasan:2004:FLE:1247415.1247418,
	author = {Srinivasan, Sudarshan M. and Kandula, Srikanth and Andrews, Christopher R. and Zhou, Yuanyuan},
	title = {Flashback: a lightweight extension for rollback and deterministic replay for software debugging},
	booktitle = {Proceedings of the annual conference on USENIX Annual Technical Conference},
	series = {ATEC '04},
	year = {2004},
	location = {Boston, MA},
	pages = {3--3},
	numpages = {1},
	url = {http://dl.acm.org/citation.cfm?id=1247415.1247418},
	acmid = {1247418},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
}

@inproceedings{Thane:2000:UDR:1947412.1947455,
	author = {Thane, Henrik and Hansson, Hans},
	title = {Using deterministic replay for debugging of distributed real-time systems},
	booktitle = {Proceedings of the 12th Euromicro conference on Real-time systems},
	series = {Euromicro-RTS'00},
	year = {2000},
	isbn = {0-7695-0734-4},
	location = {Stockholm, Sweden},
	pages = {265--272},
	numpages = {8},
	url = {http://dl.acm.org/citation.cfm?id=1947412.1947455},
	acmid = {1947455},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {debugging, determinism, distributed real-time systems, monitoring, probe-effect, replay, testing},
} 

@article{Laadan:2010:TLA:1811099.1811057,
	author = {Laadan, Oren and Viennot, Nicolas and Nieh, Jason},
	title = {Transparent, lightweight application execution replay on commodity multiprocessor operating systems},
	journal = {SIGMETRICS Perform. Eval. Rev.},
	issue_date = {June 2010},
	volume = {38},
	number = {1},
	month = jun,
	year = {2010},
	issn = {0163-5999},
	pages = {155--166},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1811099.1811057},
	doi = {10.1145/1811099.1811057},
	acmid = {1811057},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, fault-tolerance, record-replay, virtualization},
}

@inproceedings{Xu:2003:FDR:859618.859633,
	author = {Xu, Min and Bodik, Rastislav and Hill, Mark D.},
	title = {A "flight data recorder" for enabling full-system multiprocessor deterministic replay},
	booktitle = {Proceedings of the 30th annual international symposium on Computer architecture},
	series = {ISCA '03},
	year = {2003},
	isbn = {0-7695-1945-8},
	location = {San Diego, California},
	pages = {122--135},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/859618.859633},
	doi = {10.1145/859618.859633},
	acmid = {859633},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Subhraveti:2011:RTP:1993744.1993757,
	author = {Subhraveti, Dinesh and Nieh, Jason},
	title = {Record and transplay: partial checkpointing for replay debugging across heterogeneous systems},
	booktitle = {Proceedings of the ACM SIGMETRICS joint international conference on Measurement and modeling of computer systems},
	series = {SIGMETRICS '11},
	year = {2011},
	isbn = {978-1-4503-0814-4},
	location = {San Jose, California, USA},
	pages = {109--120},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1993744.1993757},
	doi = {10.1145/1993744.1993757},
	acmid = {1993757},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {checkpoint-restart, record-replay, virtualization},
}

@article{Min:1991:ECA:106974.106996,
	author = {Min, Sang L. and Choi, Jong-Deok},
	title = {An efficient cache-based access anomaly detection scheme},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {Apr. 1991},
	volume = {25},
	number = {Special Issue},
	month = apr,
	year = {1991},
	issn = {0163-5980},
	pages = {235--244},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/106974.106996},
	doi = {10.1145/106974.106996},
	acmid = {106996},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Pan:1988:SRE:68210.69227,
	author = {Pan, Douglas Z. and Linton, Mark A.},
	title = {Supporting reverse execution for parallel programs},
	booktitle = {Proceedings of the 1988 ACM SIGPLAN and SIGOPS workshop on Parallel and distributed debugging},
	series = {PADD '88},
	year = {1988},
	isbn = {0-89791-296-9},
	location = {Madison, Wisconsin, United States},
	pages = {124--129},
	numpages = {6},
	url = {http://doi.acm.org/10.1145/68210.69227},
	doi = {10.1145/68210.69227},
	acmid = {69227},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Netzer:1993:OTR:174266.174268,
	author = {Netzer, Robert H. B.},
	title = {Optimal tracing and replay for debugging shared-memory parallel programs},
	booktitle = {Proceedings of the 1993 ACM/ONR workshop on Parallel and distributed debugging},
	series = {PADD '93},
	year = {1993},
	isbn = {0-89791-633-6},
	location = {San Diego, California, United States},
	pages = {1--11},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/174266.174268},
	doi = {10.1145/174266.174268},
	acmid = {174268},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Savage:1997:EDD:269005.266641,
	author = {Savage, Stefan and Burrows, Michael and Nelson, Greg and Sobalvarro, Patrick and Anderson, Thomas},
	title = {Eraser: a dynamic data race detector for multi-threaded programs},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {Dec. 1997},
	volume = {31},
	number = {5},
	month = oct,
	year = {1997},
	issn = {0163-5980},
	pages = {27--37},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/269005.266641},
	doi = {10.1145/269005.266641},
	acmid = {266641},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Laadan:2007:DPV:1323293.1294289,
	author = {Laadan, Oren and Baratto, Ricardo A. and Phung, Dan B. and Potter, Shaya and Nieh, Jason},
	title = {DejaView: a personal virtual computer recorder},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {December 2007},
	volume = {41},
	number = {6},
	month = oct,
	year = {2007},
	issn = {0163-5980},
	pages = {279--292},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/1323293.1294289},
	doi = {10.1145/1323293.1294289},
	acmid = {1294289},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {desktop search, virtualization},
}

@inproceedings{Tsankov:2011:EHI:1989760.1990086,
	author = {Tsankov, Petar and Jin, Wei and Orso, Alessandro and Sinha, Saurabh},
	title = {Execution Hijacking: Improving Dynamic Analysis by Flying off Course},
	booktitle = {Proceedings of the 2011 Fourth IEEE International Conference on Software Testing, Verification and Validation},
	series = {ICST '11},
	year = {2011},
	isbn = {978-0-7695-4342-0},
	pages = {200--209},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICST.2011.45},
	doi = {10.1109/ICST.2011.45},
	acmid = {1990086},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@article{Silva:2012:VPS:2187671.2187674,
	author = {Silva, Josep},
	title = {A vocabulary of program slicing-based techniques},
	journal = {ACM Comput. Surv.},
	issue_date = {June 2012},
	volume = {44},
	number = {3},
	month = jun,
	year = {2012},
	issn = {0360-0300},
	pages = {12:1--12:41},
	articleno = {12},
	numpages = {41},
	url = {http://doi.acm.org/10.1145/2187671.2187674},
	doi = {10.1145/2187671.2187674},
	acmid = {2187674},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Program slicing, software engineering},
}

@inproceedings{LeVasseur:2004:SAR:1133572.1133617,
	author = {LeVasseur, Joshua and Uhlig, Volkmar},
	title = {A sledgehammer approach to reuse of legacy device drivers},
	booktitle = {Proceedings of the 11th workshop on ACM SIGOPS European workshop},
	series = {EW 11},
	year = {2004},
	location = {Leuven, Belgium},
	articleno = {24},
	url = {http://doi.acm.org/10.1145/1133572.1133617},
	doi = {10.1145/1133572.1133617},
	acmid = {1133617},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Jamrozik:2012:ADS:2351676.2351716,
	author = {Jamrozik, Konrad and Fraser, Gordon and Tillmann, Nikolai and De Halleux, Jonathan},
	title = {Augmented dynamic symbolic execution},
	booktitle = {Proceedings of the 27th IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE 2012},
	year = {2012},
	isbn = {978-1-4503-1204-2},
	location = {Essen, Germany},
	pages = {254--257},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/2351676.2351716},
	doi = {10.1145/2351676.2351716},
	acmid = {2351716},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Test generation, boundary values, dynamic symbolic execution, mutation testing},
}

@inproceedings{Zhang:2010:TGV:1912607.1913317,
	author = {Zhang, Lingming and Xie, Tao and Zhang, Lu and Tillmann, Nikolai and de Halleux, Jonathan and Mei, Hong},
	title = {Test generation via Dynamic Symbolic Execution for mutation testing},
	booktitle = {Proceedings of the 2010 IEEE International Conference on Software Maintenance},
	series = {ICSM '10},
	year = {2010},
	isbn = {978-1-4244-8630-4},
	pages = {1--10},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICSM.2010.5609672},
	doi = {10.1109/ICSM.2010.5609672},
	acmid = {1913317},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Anand:2011:HCE:2190078.2190144,
	author = {Anand, Saswat and Harrold, Mary Jean},
	title = {Heap cloning: Enabling dynamic symbolic execution of java programs},
	booktitle = {Proceedings of the 2011 26th IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '11},
	year = {2011},
	isbn = {978-1-4577-1638-6},
	pages = {33--42},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ASE.2011.6100071},
	doi = {10.1109/ASE.2011.6100071},
	acmid = {2190144},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Sen:2005:CCU:1081706.1081750,
	author = {Sen, Koushik and Marinov, Darko and Agha, Gul},
	title = {CUTE: a concolic unit testing engine for C},
	booktitle = {Proceedings of the 10th European software engineering conference held jointly with 13th ACM SIGSOFT international symposium on Foundations of software engineering},
	series = {ESEC/FSE-13},
	year = {2005},
	isbn = {1-59593-014-0},
	location = {Lisbon, Portugal},
	pages = {263--272},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1081706.1081750},
	doi = {10.1145/1081706.1081750},
	acmid = {1081750},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {concolic testing, data structure testing, explicit path model-checking, random testing, testing C programs, unit testing},
} 

@inproceedings{Godefroid:2005:DDA:1065010.1065036,
	author = {Godefroid, Patrice and Klarlund, Nils and Sen, Koushik},
	title = {DART: directed automated random testing},
	booktitle = {Proceedings of the 2005 ACM SIGPLAN conference on Programming language design and implementation},
	series = {PLDI '05},
	year = {2005},
	isbn = {1-59593-056-6},
	location = {Chicago, IL, USA},
	pages = {213--223},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1065010.1065036},
	doi = {10.1145/1065010.1065036},
	acmid = {1065036},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {automated test generation, interfaces, program verification, random testing, software testing},
} 

@inproceedings{Rubinov:2012:ATS:2337223.2337438,
	author = {Rubinov, Konstantin and Wuttke, Jochen},
	title = {Augmenting test suites automatically},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {1433--1434},
	numpages = {2},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337438},
	acmid = {2337438},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@article{Thummalapenta:2011:SMS:2076021.2048083,
	author = {Thummalapenta, Suresh and Xie, Tao and Tillmann, Nikolai and de Halleux, Jonathan and Su, Zhendong},
	title = {Synthesizing method sequences for high-coverage testing},
	journal = {SIGPLAN Not.},
	issue_date = {October 2011},
	volume = {46},
	number = {10},
	month = oct,
	year = {2011},
	issn = {0362-1340},
	pages = {189--206},
	numpages = {18},
	url = {http://doi.acm.org/10.1145/2076021.2048083},
	doi = {10.1145/2076021.2048083},
	acmid = {2048083},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {object-oriented testing, symbolic execution},
}

@inproceedings{Fraser:2011:ECO:1989760.1990074,
	author = {Fraser, Gordon and Zeller, Andreas},
	title = {Exploiting Common Object Usage in Test Case Generation},
	booktitle = {Proceedings of the 2011 Fourth IEEE International Conference on Software Testing, Verification and Validation},
	series = {ICST '11},
	year = {2011},
	isbn = {978-0-7695-4342-0},
	pages = {80--89},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICST.2011.53},
	doi = {10.1109/ICST.2011.53},
	acmid = {1990074},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {test case generation, specification mining, readability},
}

@inproceedings{Zhang:2011:CSD:2001420.2001463,
	author = {Zhang, Sai and Saff, David and Bu, Yingyi and Ernst, Michael D.},
	title = {Combined static and dynamic automated test generation},
	booktitle = {Proceedings of the 2011 International Symposium on Software Testing and Analysis},
	series = {ISSTA '11},
	year = {2011},
	isbn = {978-1-4503-0562-4},
	location = {Toronto, Ontario, Canada},
	pages = {353--363},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2001420.2001463},
	doi = {10.1145/2001420.2001463},
	acmid = {2001463},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {automated test generation, dynamic analyses, static},
}



@incollection{textsumchap2011,
	year={2011},
	isbn={978-3-642-17088-1},
	booktitle={Knowledge in Formation},
	series={Cognitive Technologies},
	doi={10.1007/978-3-642-17089-8_9},
	title={Text summarization},
	url={http://dx.doi.org/10.1007/978-3-642-17089-8_9},
	publisher={Springer Berlin Heidelberg},
	author={Sarbo, JanosJ. and Farkas, JozsefI. and Breemen, AukeJ.J.},
	pages={151-164},
	language={English}
}

@INPROCEEDINGS{1181320,
	author={Fang Chen and Kesong Han and Guilin Chen},
	booktitle={TENCON '02. Proceedings. 2002 IEEE Region 10 Conference on Computers, Communications, Control and Power Engineering},
	title={An approach to sentence-selection-based text summarization},
	year={2002},
	volume={1},
	pages={489-493 vol.1},
	keywords={feature extraction;text analysis;word processing;Chinese processing;performance;sentence length feature;sentence level features;sentence selection;text summarization;topic sensitive word feature;word level features;Australia;Character generation;Costing;Costs;Kernel;Supervised learning;Tagging},
	doi={10.1109/TENCON.2002.1181320}
}

@article{Wang:2012:CDS:2362383.2362386,
	author = {Wang, Dingding and Zhu, Shenghuo and Li, Tao and Gong, Yihong},
	title = {Comparative Document Summarization via Discriminative Sentence Selection},
	journal = {ACM Trans. Knowl. Discov. Data},
	issue_date = {October 2012},
	volume = {6},
	number = {3},
	month = oct,
	year = {2012},
	issn = {1556-4681},
	pages = {12:1--12:18},
	articleno = {12},
	numpages = {18},
	url = {http://doi.acm.org/10.1145/2362383.2362386},
	doi = {10.1145/2362383.2362386},
	acmid = {2362386},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Comparative document summarization, discriminative sentence selection},
}

@inproceedings{Goldstein:1999:STD:312624.312665,
	author = {Goldstein, Jade and Kantrowitz, Mark and Mittal, Vibhu and Carbonell, Jaime},
	title = {Summarizing Text Documents: Sentence Selection and Evaluation Metrics},
	booktitle = {Proceedings of the 22Nd Annual International ACM SIGIR Conference on Research and Development in Information Retrieval},
	series = {SIGIR '99},
	year = {1999},
	isbn = {1-58113-096-1},
	location = {Berkeley, California, USA},
	pages = {121--128},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/312624.312665},
	doi = {10.1145/312624.312665},
	acmid = {312665},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Radev:2000:CSM:1567564.1567567,
	author = {Radev, Dragomir R. and Jing, Hongyan and Budzikowska, Malgorzata},
	title = {Centroid-based Summarization of Multiple Documents: Sentence Extraction, Utility-based Evaluation, and User Studies},
	booktitle = {Proceedings of the 2000 NAACL-ANLP Workshop on Automatic Summarization},
	series = {NAACL-ANLP-AutoSum '00},
	year = {2000},
	location = {Seattle, Washington},
	pages = {21--30},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=1567564.1567567},
	acmid = {1567567},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
} 

@article{SparckJones:2007:ASS:1284916.1285154,
	author = {Sp\"{a}rck Jones, Karen},
	title = {Automatic Summarising: The State of the Art},
	journal = {Inf. Process. Manage.},
	issue_date = {November, 2007},
	volume = {43},
	number = {6},
	month = nov,
	year = {2007},
	issn = {0306-4573},
	pages = {1449--1481},
	numpages = {33},
	url = {http://dx.doi.org/10.1016/j.ipm.2007.03.009},
	doi = {10.1016/j.ipm.2007.03.009},
	acmid = {1285154},
	publisher = {Pergamon Press, Inc.},
	address = {Tarrytown, NY, USA},
	keywords = {Abstraction natural language processing, Evaluation, Sentence extraction, Summarization},
}

@article{Luhn:1958:BIS:1662374.1662381,
	author = {Luhn, H. P.},
	title = {A Business Intelligence System},
	journal = {IBM J. Res. Dev.},
	issue_date = {October 1958},
	volume = {2},
	number = {4},
	month = oct,
	year = {1958},
	issn = {0018-8646},
	pages = {314--319},
	numpages = {6},
	url = {http://dx.doi.org/10.1147/rd.24.0314},
	doi = {10.1147/rd.24.0314},
	acmid = {1662381},
	publisher = {IBM Corp.},
	address = {Riverton, NJ, USA},
} 

@article{Corbi:1989:PUC:97118.97124,
	author = {Corbi, T. A.},
	title = {Program understanding: challenge for the 1990's},
	journal = {IBM Syst. J.},
	issue_date = {1989},
	volume = {28},
	number = {2},
	month = jun,
	year = {1989},
	issn = {0018-8670},
	pages = {294--306},
	numpages = {13},
	url = {http://dx.doi.org/10.1147/sj.282.0294},
	doi = {10.1147/sj.282.0294},
	acmid = {97124},
	publisher = {IBM Corp.},
	address = {Riverton, NJ, USA},
}

@misc{NSF-2013-GPG,
	author=	"National Science Foundation",
	howpublished=	"Published online",
	month=		"January",
	title=		"Grant Proposal Guide",
	year=		"2013"
}

@inproceedings{Cleland-Huang:2011:GCB:1987856.1987861,
	author = {Cleland-Huang, Jane and Czauderna, Adam and Dekhtyar, Alex and Gotel, Olly and Hayes, Jane Huffman and Keenan, Ed and Leach, Greg and Maletic, Jonathan and Poshyvanyk, Denys and Shin, Youghee and Zisman, Andrea and Antoniol, Giuliano and Berenbach, Brian and Egyed, Alexander and Maeder, Patrick},
	title = {Grand Challenges, Benchmarks, and TraceLab: Developing Infrastructure for the Software Traceability Research Community},
	booktitle = {Proceedings of the 6th International Workshop on Traceability in Emerging Forms of Software Engineering},
	series = {TEFSE '11},
	year = {2011},
	isbn = {978-1-4503-0589-1},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {17--23},
	numpages = {7},
	url = {http://doi.acm.org/10.1145/1987856.1987861},
	doi = {10.1145/1987856.1987861},
	acmid = {1987861},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {benchmarks, metrics, traceability, tracelab},
} 

@inproceedings{Papineni:2002:BMA:1073083.1073135,
	author = {Papineni, Kishore and Roukos, Salim and Ward, Todd and Zhu, Wei-Jing},
	title = {BLEU: A Method for Automatic Evaluation of Machine Translation},
	booktitle = {Proceedings of the 40th Annual Meeting on Association for Computational Linguistics},
	series = {ACL '02},
	year = {2002},
	location = {Philadelphia, Pennsylvania},
	pages = {311--318},
	numpages = {8},
	url = {http://dx.doi.org/10.3115/1073083.1073135},
	doi = {10.3115/1073083.1073135},
	acmid = {1073135},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
}

@inproceedings{Papineni:2002:BMA:1073083.1073135,
	author = {Papineni, Kishore and Roukos, Salim and Ward, Todd and Zhu, Wei-Jing},
	title = {BLEU: A Method for Automatic Evaluation of Machine Translation},
	booktitle = {Proceedings of the 40th Annual Meeting on Association for Computational Linguistics},
	series = {ACL '02},
	year = {2002},
	location = {Philadelphia, Pennsylvania},
	pages = {311--318},
	numpages = {8},
	url = {http://dx.doi.org/10.3115/1073083.1073135},
	doi = {10.3115/1073083.1073135},
	acmid = {1073135},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
}

@inproceedings{Koehn:2007:MOS:1557769.1557821,
	author = {Koehn, Philipp and Hoang, Hieu and Birch, Alexandra and Callison-Burch, Chris and Federico, Marcello and Bertoldi, Nicola and Cowan, Brooke and Shen, Wade and Moran, Christine and Zens, Richard and Dyer, Chris and Bojar, Ond\v{r}ej and Constantin, Alexandra and Herbst, Evan},
	title = {Moses: Open Source Toolkit for Statistical Machine Translation},
	booktitle = {Proceedings of the 45th Annual Meeting of the ACL on Interactive Poster and Demonstration Sessions},
	series = {ACL '07},
	year = {2007},
	location = {Prague, Czech Republic},
	pages = {177--180},
	numpages = {4},
	url = {http://dl.acm.org/citation.cfm?id=1557769.1557821},
	acmid = {1557821},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
}

@article{Brown:1990:SAM:92858.92860,
	author = {Brown, Peter F. and Cocke, John and Pietra, Stephen A. Della and Pietra, Vincent J. Della and Jelinek, Fredrick and Lafferty, John D. and Mercer, Robert L. and Roossin, Paul S.},
	title = {A Statistical Approach to Machine Translation},
	journal = {Comput. Linguist.},
	issue_date = {June 1990},
	volume = {16},
	number = {2},
	month = jun,
	year = {1990},
	issn = {0891-2017},
	pages = {79--85},
	numpages = {7},
	url = {http://dl.acm.org/citation.cfm?id=92858.92860},
	acmid = {92860},
	publisher = {MIT Press},
	address = {Cambridge, MA, USA},
} 

@inproceedings{DBLP:conf/interspeech/KombrinkMKB11,
	author    = {Stefan Kombrink and
	Tomas Mikolov and
	Martin Karafi{\'a}t and
	Luk{\'a}s Burget},
	title     = {Recurrent Neural Network Based Language Modeling in Meeting
	Recognition},
	booktitle = {INTERSPEECH},
	year      = {2011},
	pages     = {2877-2880},
	ee        = {http://www.isca-speech.org/archive/interspeech_2011/i11_2877.html},
	crossref  = {DBLP:conf/interspeech/2011},
	bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{DBLP:conf/emnlp/VaswaniZFC13,
	author    = {Ashish Vaswani and
	Yinggong Zhao and
	Victoria Fossum and
	David Chiang},
	title     = {Decoding with Large-Scale Neural Language Models Improves
	Translation},
	booktitle = {EMNLP},
	year      = {2013},
	pages     = {1387-1392},
	ee        = {http://aclweb.org/anthology//D/D13/D13-1140.pdf},
	crossref  = {DBLP:conf/emnlp/2013},
	bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{hindle2016naturalness,
	title={On the naturalness of software},
	author={Hindle, Abram and Barr, Earl T and Gabel, Mark and Su, Zhendong and Devanbu, Premkumar},
	journal={Communications of the ACM},
	volume={59},
	number={5},
	pages={122--131},
	year={2016},
	publisher={ACM}
}

@inproceedings{Hindle:2012:NS:2337223.2337322,
	author = {Hindle, Abram and Barr, Earl T. and Su, Zhendong and Gabel, Mark and Devanbu, Premkumar},
	title = {On the Naturalness of Software},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {837--847},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337322},
	acmid = {2337322},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@inproceedings{Allamanis:2013:MSC:2487085.2487127,
	author = {Allamanis, Miltiadis and Sutton, Charles},
	title = {Mining Source Code Repositories at Massive Scale Using Language Modeling},
	booktitle = {Proceedings of the 10th Working Conference on Mining Software Repositories},
	series = {MSR '13},
	year = {2013},
	isbn = {978-1-4673-2936-1},
	location = {San Francisco, CA, USA},
	pages = {207--216},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=2487085.2487127},
	acmid = {2487127},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@inproceedings{Zhong:2009:MMR:1615184.1615205,
	author = {Zhong, Hao and Xie, Tao and Zhang, Lu and Pei, Jian and Mei, Hong},
	title = {MAPO: Mining and Recommending API Usage Patterns},
	booktitle = {Proceedings of the 23rd European Conference on ECOOP 2009 --- Object-Oriented Programming},
	series = {Genoa},
	year = {2009},
	isbn = {978-3-642-03012-3},
	location = {Italy},
	pages = {318--343},
	numpages = {26},
	url = {http://dx.doi.org/10.1007/978-3-642-03013-0_15},
	doi = {10.1007/978-3-642-03013-0_15},
	acmid = {1615205},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
}

@inproceedings{LijieWang:2011:AEW:2190078.2190135,
	author = {Lijie Wang and Lu Fang and Leye Wang and Ge Li and Bing Xie and Fuqing Yang},
	title = {APIExample: An effective web search based usage example recommendation system for java APIs},
	booktitle = {Proceedings of the 2011 26th IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '11},
	year = {2011},
	isbn = {978-1-4577-1638-6},
	pages = {592--595},
	numpages = {4},
	url = {http://dx.doi.org/10.1109/ASE.2011.6100133},
	doi = {10.1109/ASE.2011.6100133},
	acmid = {2190135},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Brandt:2010:EPI:1753326.1753402,
	author = {Brandt, Joel and Dontcheva, Mira and Weskamp, Marcos and Klemmer, Scott R.},
	title = {Example-centric programming: integrating web search into the development environment},
	booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
	series = {CHI '10},
	year = {2010},
	isbn = {978-1-60558-929-9},
	location = {Atlanta, Georgia, USA},
	pages = {513--522},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1753326.1753402},
	doi = {10.1145/1753326.1753402},
	acmid = {1753402},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {example-centric development},
} 

@article{Mcmillan:2013:PSR:2522920.2522930,
	author = {McMillan, Collin and Poshyvanyk, Denys and Grechanik, Mark and Xie, Qing and Fu, Chen},
	title = {Portfolio: Searching for Relevant Functions and Their Usages in Millions of Lines of Code},
	journal = {ACM Trans. Softw. Eng. Methodol.},
	issue_date = {October 2013},
	volume = {22},
	number = {4},
	month = oct,
	year = {2013},
	issn = {1049-331X},
	pages = {37:1--37:30},
	articleno = {37},
	numpages = {30},
	url = {http://doi.acm.org/10.1145/2522920.2522930},
	doi = {10.1145/2522920.2522930},
	acmid = {2522930},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Pagerank, Source-code search, information retrieval, natural language processing, user studies},
} 

@article{moritzexport,
	title={ExPort: Detecting and Visualizing API Usages in Large Source Code Repositories},
	author={Moritz, Evan and Linares-V{\'a}squez, Mario and Poshyvanyk, Denys and Grechanik, Mark and McMillan, Collin and Gethers, Malcom}
	
}

@INPROCEEDINGS{moritzexport,
	author={Moritz, E. and Linares-Vasquez, M. and Poshyvanyk, D. and Grechanik, M. and McMillan, C. and Gethers, M.},
	booktitle={Automated Software Engineering (ASE), 2013 IEEE/ACM 28th International Conference on},
	title={ExPort: Detecting and visualizing API usages in large source code repositories},
	year={2013},
	month={Nov},
	pages={646-651},
	doi={10.1109/ASE.2013.6693127}
}

@inproceedings{LSSPaper,
	author = {Croft, David and Coupland, Simon and Shell, Jethro and Brown, Stephen},
	title = {A Fast and Efficient Semantic Short Text Similarity Metric},
} 

@article{Yuhua.TKDE.2006.130,
	author = {Yuhua Li and David McLean and Zuhair A. Bandar and James D. O'Shea and Keeley Crockett},
	title = {Sentence Similarity Based on Semantic Nets and Corpus Statistics},
	journal ={IEEE Transactions on Knowledge and Data Engineering},
	volume = {18},
	number = {8},
	issn = {1041-4347},
	year = {2006},
	pages = {1138-1150},
	doi = {http://doi.ieeecomputersociety.org/10.1109/TKDE.2006.130},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{OShea:2008:CST:1787839.1787859,
	author = {O'Shea, James and Bandar, Zuhair and Crockett, Keeley and McLean, David},
	title = {A comparative study of two short text semantic similarity measures},
	booktitle = {Proceedings of the 2nd KES International conference on Agent and multi-agent systems: technologies and applications},
	series = {KES-AMSTA'08},
	year = {2008},
	isbn = {3-540-78581-7, 978-3-540-78581-1},
	location = {Incheon, Korea},
	pages = {172--181},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=1787839.1787859},
	acmid = {1787859},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
	keywords = {benchmark, dialogue management, natural language, semantic similarity, sentence, user modeling},
} 

@inproceedings{Biggerstaff:1993:CAP:257572.257679,
	author = {Biggerstaff, Ted J. and Mitbander, Bharat G. and Webster, Dallas},
	title = {The concept assignment problem in program understanding},
	booktitle = {Proceedings of the 15th international conference on Software Engineering},
	series = {ICSE '93},
	year = {1993},
	isbn = {0-89791-588-7},
	location = {Baltimore, Maryland, USA},
	pages = {482--498},
	numpages = {17},
	url = {http://dl.acm.org/citation.cfm?id=257572.257679},
	acmid = {257679},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
	keywords = {concept recognition, connectionist, domain, knowledge base, plausible reasoning, reverse engineering, slicing},
} 

@article{Morse:1999:Minsize2,
	author={David T. Morse},
	journal={Educational and Psychological Measurement},
	title={Minsize2: A computer program for determining effect size and minimum sample size for statistical significance for univariate, multivariate, and nonparametric tests},
	year={1999},
	month={June},
	volume={59},
	number={3},
	pages={518--531},
	doi={10.1109/64.294135},
	ISSN={0885-9000}
}

@inproceedings{Smucker:07,
	author = {Smucker, Mark D. and Allan, James and Carterette, Ben},
	title = {A comparison of statistical significance tests for information retrieval evaluation},
	booktitle = {CIKM},
	year = {2007},
	pages = {623--632}
}

@book{STAT:05,
	author = {R. Mark Sirkin},
	title = {Statistics for the Social Sciences},
	month = {August},
	year = {2005},
	edition = "Third",
	pages = {632},
	publisher = {Sage Publications}
}

@book{IR:08,
	author = {Manning, Christopher D. and Raghavan, Prabhakar and Schtze, Hinrich},
	title = {Introduction to Information Retrieval},
	year = {2008},
	isbn = {0521865719, 9780521865715},
	publisher = {Cambridge University Press},
	address = {New York, NY, USA}
}

@inproceedings{Moreno:2013:ICPC,
	author = {Moreno, Laura and Aponte, Jairo and Sridhara Giriprasad and Marcus, Andrian and Pollock, Lori and Vijay-Shanker, K.},
	title = {Automatic Generation of Natural Language Summaries for Java Classes},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	year = {2013},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@inproceedings{Eddy:2013:ICPC,
	author = {Eddy, Brian and Robinson, Jeffrey and Kraft, Nicholas and Carver, Jeffrey},
	title = {Evaluating Source Code Summarization Techniques: Replication and Expansion},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	year = {2013},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@conference {Javadocminer,
	title = {{Automatic Quality Assessment of Source Code Comments: The JavadocMiner}},
	booktitle = {15th International Conference on Applications of Natural Language to Information Systems (NLDB 2010)},
	series = {Lecture Notes in Computer Science (LNCS)},
	volume = {6177/2010},
	year = {2010},
	month = {June 23--25},
	pages = {68--79},
	publisher = {Springer},
	organization = {Springer},
	address = {Cardiff, UK},
	isbn = {978-3-642-13880-5},
	doi = {10.1007/978-3-642-13881-2_7},
	url = {http://www.springerlink.com/content/n67470n270mt61m1/fulltext.pdf},
	attachments = {http://www.semanticsoftware.info/system/files/nldb2010-javadocminer.pdf},
	author = {Ninus Khamis and Ren{\'e} Witte and Juergen Rilling},
	editor = {Christina J. Hopfe and Yacine Rezgui and Elisabeth M{\'e}tais and Alun D. Preece and Haijiang Li}
}

@inproceedings{Steidl:2013:ICPC,
	author = {Steidl, Daniela and Hummel, Benjamin and Juergens, Elmar},
	title = {Quality Analysis of Source Code Comments},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	year = {2013},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@inproceedings{Gatt:2009:SRE:1610195.1610208,
	author = {Gatt, Albert and Reiter, Ehud},
	title = {SimpleNLG: a realisation engine for practical applications},
	booktitle = {Proceedings of the 12th European Workshop on Natural Language Generation},
	series = {ENLG '09},
	year = {2009},
	location = {Athens, Greece},
	pages = {90--93},
	numpages = {4},
	url = {http://dl.acm.org/citation.cfm?id=1610195.1610208},
	acmid = {1610208},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
}

@inproceedings{McMillan:2012:RSC:2337223.2337323,
	author = {McMillan, Collin and Hariri, Negar and Poshyvanyk, Denys and Cleland-Huang, Jane and Mobasher, Bamshad},
	title = {Recommending source code for use in rapid software prototypes},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {848--858},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337323},
	acmid = {2337323},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@inproceedings{McMillan:2011:PFR:1985793.1985809,
	author = {McMillan, Collin and Grechanik, Mark and Poshyvanyk, Denys and Xie, Qing and Fu, Chen},
	title = {Portfolio: finding relevant functions and their usage},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {111--120},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985809},
	doi = {10.1145/1985793.1985809},
	acmid = {1985809},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {code search, function call graph, pagerank, portfolio, ranking},
}

@inproceedings{Puppin:2006:SNJ:1141277.1141605,
	author = {Puppin, Diego and Silvestri, Fabrizio},
	title = {The social network of Java classes},
	booktitle = {Proceedings of the 2006 ACM symposium on Applied computing},
	series = {SAC '06},
	year = {2006},
	isbn = {1-59593-108-2},
	location = {Dijon, France},
	pages = {1409--1413},
	numpages = {5},
	url = {http://doi.acm.org/10.1145/1141277.1141605},
	doi = {10.1145/1141277.1141605},
	acmid = {1141605},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Inoue:2003:CRR:776816.776819,
	author = {Inoue, Katsuro and Yokomori, Reishi and Fujiwara, Hikaru and Yamamoto, Tetsuo and Matsushita, Makoto and Kusumoto, Shinji},
	title = {Component rank: relative significance rank for software component search},
	booktitle = {Proceedings of the 25th International Conference on Software Engineering},
	series = {ICSE '03},
	year = {2003},
	isbn = {0-7695-1877-X},
	location = {Portland, Oregon},
	pages = {14--24},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=776816.776819},
	acmid = {776819},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Chan:2012:SCA:2393596.2393606,
	author = {Chan, Wing-Kwan and Cheng, Hong and Lo, David},
	title = {Searching connected API subgraph via text phrases},
	booktitle = {Proceedings of the ACM SIGSOFT 20th International Symposium on the Foundations of Software Engineering},
	series = {FSE '12},
	year = {2012},
	isbn = {978-1-4503-1614-9},
	location = {Cary, North Carolina},
	pages = {10:1--10:11},
	articleno = {10},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2393596.2393606},
	doi = {10.1145/2393596.2393606},
	acmid = {2393606},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {API graph, API recommendation, subgraph searching},
}

@book{Langville:2006:GPB:1146372,
	author = {Langville, Amy N. and Meyer, Carl D.},
	title = {Google's PageRank and Beyond: The Science of Search Engine Rankings},
	year = {2006},
	isbn = {0691122024},
	publisher = {Princeton University Press},
	address = {Princeton, NJ, USA},
}

@inproceedings{Liu:2009:ITV:1645953.1646023,
	author = {Liu, Shixia and Zhou, Michelle X. and Pan, Shimei and Qian, Weihong and Cai, Weijia and Lian, Xiaoxiao},
	title = {Interactive, Topic-based Visual Text Summarization and Analysis},
	booktitle = {Proceedings of the 18th ACM Conference on Information and Knowledge Management},
	series = {CIKM '09},
	year = {2009},
	isbn = {978-1-60558-512-3},
	location = {Hong Kong, China},
	pages = {543--552},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1645953.1646023},
	doi = {10.1145/1645953.1646023},
	acmid = {1646023},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {interactive text visualization, stacked graph, text summarization, topic model},
}

@inproceedings{Wang:2012:UTM:2392800.2392808,
	author = {Wang, Lu and Cardie, Claire},
	title = {Unsupervised Topic Modeling Approaches to Decision Summarization in Spoken Meetings},
	booktitle = {Proceedings of the 13th Annual Meeting of the Special Interest Group on Discourse and Dialogue},
	series = {SIGDIAL '12},
	year = {2012},
	location = {Seoul, South Korea},
	pages = {40--49},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=2392800.2392808},
	acmid = {2392808},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
}

@inproceedings{Haghighi:2009:ECM:1620754.1620807,
	author = {Haghighi, Aria and Vanderwende, Lucy},
	title = {Exploring Content Models for Multi-document Summarization},
	booktitle = {Proceedings of Human Language Technologies: The 2009 Annual Conference of the North American Chapter of the Association for Computational Linguistics},
	series = {NAACL '09},
	year = {2009},
	isbn = {978-1-932432-41-1},
	location = {Boulder, Colorado},
	pages = {362--370},
	numpages = {9},
	url = {http://dl.acm.org/citation.cfm?id=1620754.1620807},
	acmid = {1620807},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
}

@inproceedings{Marcu2001,
	author = {Daniel Marcu and Laurie Gerber},
	year = {2001},
	title = {An Inquiry into the Nature of Multidocument Abstracts, Extracts, and Their Evaluation},
	booktitle = {NAACL-2001 Workshop on Automatic Summarization},
	location = {Pittsburgh, PA},
	month = {June},
	day = {3}
}

@inproceedings{Panichella:2013:EUT:2486788.2486857,
	author = {Panichella, Annibale and Dit, Bogdan and Oliveto, Rocco and Di Penta, Massimiliano and Poshyvanyk, Denys and De Lucia, Andrea},
	title = {How to Effectively Use Topic Models for Software Engineering Tasks? An Approach Based on Genetic Algorithms},
	booktitle = {Proceedings of the 2013 International Conference on Software Engineering},
	series = {ICSE '13},
	year = {2013},
	isbn = {978-1-4673-3076-3},
	location = {San Francisco, CA, USA},
	pages = {522--531},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=2486788.2486857},
	acmid = {2486857},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@incollection{mdtsutmfl,
	year={2013},
	isbn={978-3-642-39711-0},
	booktitle={Machine Learning and Data Mining in Pattern Recognition},
	volume={7988},
	series={Lecture Notes in Computer Science},
	editor={Perner, Petra},
	doi={10.1007/978-3-642-39712-7_12},
	title={Multi-document Text Summarization Using Topic Model and Fuzzy Logic},
	url={http://dx.doi.org/10.1007/978-3-642-39712-7_12},
	publisher={Springer Berlin Heidelberg},
	keywords={Fuzzy Systems; Data mining; Text Analysis; Semantics},
	author={Lee, Sanghoon and Belkasim, Saeid and Zhang, Yanqing},
	pages={159-168}
}

@inproceedings{Haiduc:2010:UAT:1919284.1919577,
	author = {Haiduc, Sonia and Aponte, Jairo and Moreno, Laura and Marcus, Andrian},
	title = {On the Use of Automated Text Summarization Techniques for Summarizing Source Code},
	booktitle = {Proceedings of the 2010 17th Working Conference on Reverse Engineering},
	series = {WCRE '10},
	year = {2010},
	isbn = {978-0-7695-4123-5},
	pages = {35--44},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/WCRE.2010.13},
	doi = {10.1109/WCRE.2010.13},
	acmid = {1919577},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {text summarization, program comprehension},
}

@inproceedings{Aponte:2011:ITL:1987856.1987867,
	author = {Aponte, Jairo and Marcus, Andrian},
	title = {Improving traceability link recovery methods through software artifact summarization},
	booktitle = {Proceedings of the 6th International Workshop on Traceability in Emerging Forms of Software Engineering},
	series = {TEFSE '11},
	year = {2011},
	isbn = {978-1-4503-0589-1},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {46--49},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1987856.1987867},
	doi = {10.1145/1987856.1987867},
	acmid = {1987867},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {information retrieval, program comprehension, summarization, traceability management},
}

@article{Goldberg:FOG,
	author={Goldberg, E. and Driedger, N. and Kittredge, R.I.},
	journal={IEEE Expert}, title={Using natural-language processing to produce weather forecasts},
	year={1994},
	month={April},
	volume={9},
	number={2},
	pages={45-53},
	doi={10.1109/64.294135},
	ISSN={0885-9000}
}

@book{Reiter:2000:BNL:331955,
	author = {Reiter, Ehud and Dale, Robert},
	title = {Building natural language generation systems},
	year = {2000},
	isbn = {0-521-62036-8},
	publisher = {Cambridge University Press},
	address = {New York, NY, USA},
} 

@PhdThesis{MurphyPhd96,
	title = "{Lightweight structural summarization as an aid to software evolution}",
	author = "Gail C. Murphy",
	school = "University of Washington",
	month = "July",
	year = "1996",
}

@PhdThesis{SridharaPhd12,
	title = "{Automatic Generation of Descriptive Summary Comments for Methods in Object-oriented Programs}",
	author = "Giriprasad Sridhara",
	school = "University of Delaware",
	month = Jan,
	year = "2012",
}

@inproceedings{Buse:2008:ADI:1390630.1390664,
	author = {Buse, Raymond P.L. and Weimer, Westley R.},
	title = {Automatic documentation inference for exceptions},
	booktitle = {Proceedings of the 2008 international symposium on Software testing and analysis},
	series = {ISSTA '08},
	year = {2008},
	isbn = {978-1-60558-050-0},
	location = {Seattle, WA, USA},
	pages = {273--282},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1390630.1390664},
	doi = {10.1145/1390630.1390664},
	acmid = {1390664},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation inference, exception handling, software documentation},
}

@inproceedings{Buse:2010:ADP:1858996.1859005,
	author = {Buse, Raymond P.L. and Weimer, Westley R.},
	title = {Automatically documenting program changes},
	booktitle = {Proceedings of the IEEE/ACM international conference on Automated software engineering},
	series = {ASE '10},
	year = {2010},
	isbn = {978-1-4503-0116-9},
	location = {Antwerp, Belgium},
	pages = {33--42},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1858996.1859005},
	doi = {10.1145/1858996.1859005},
	acmid = {1859005},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {code summarization, commit messages, differencing},
}

@ARTICLE{6165314,
	author={Miryung Kim and Notkin, D. and Grossman, D. and Wilson, G.},
	journal={IEEE Transactions on Software Engineering},
	title={Identifying and Summarizing Systematic Code Changes via Rule Inference},
	year={2013},
	month={Jan. },
	volume={39},
	number={1},
	pages={45 -62},
	doi={10.1109/TSE.2012.16},
	ISSN={0098-5589},
}

@inproceedings{SaiZhang:2011:ADI:2190078.2190153,
	author = {Sai Zhang and Cheng Zhang and Ernst, Michael D.},
	title = {Automated documentation inference to explain failed tests},
	booktitle = {Proceedings of the 2011 26th IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '11},
	year = {2011},
	isbn = {978-1-4577-1638-6},
	pages = {63--72},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ASE.2011.6100145},
	doi = {10.1109/ASE.2011.6100145},
	acmid = {2190153},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Holmes:2005:USC:1062455.1062491,
	author = {Holmes, Reid and Murphy, Gail C.},
	title = {Using structural context to recommend source code examples},
	booktitle = {Proceedings of the 27th international conference on Software engineering},
	series = {ICSE '05},
	year = {2005},
	isbn = {1-58113-963-2},
	location = {St. Louis, MO, USA},
	pages = {117--125},
	numpages = {9},
	url = {http://doi.acm.org/10.1145/1062455.1062491},
	doi = {10.1145/1062455.1062491},
	acmid = {1062491},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {development environment framework, examples, recommender, software structure},
}

@article{Krinke:2006:ECP:1167771.1167775,
	author = {Krinke, Jens},
	title = {Effects of context on program slicing},
	journal = {J. Syst. Softw.},
	issue_date = {September 2006},
	volume = {79},
	number = {9},
	month = sep,
	year = {2006},
	issn = {0164-1212},
	pages = {1249--1260},
	numpages = {12},
	url = {http://dx.doi.org/10.1016/j.jss.2006.02.040},
	doi = {10.1016/j.jss.2006.02.040},
	acmid = {1167775},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {program analysis, program slicing},
}

@inproceedings{deSouza:2005:SDE:1085313.1085331,
	author = {de Souza, Sergio Cozzetti B. and Anquetil, Nicolas and de Oliveira, K\'{a}thia M.},
	title = {A study of the documentation essential to software maintenance},
	booktitle = {Proceedings of the 23rd annual international conference on Design of communication: documenting \& designing for pervasive information},
	series = {SIGDOC '05},
	year = {2005},
	isbn = {1-59593-175-9},
	location = {Coventry, United Kingdom},
	pages = {68--75},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1085313.1085331},
	doi = {10.1145/1085313.1085331},
	acmid = {1085331},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {empirical study, program understanding, software maintenance, software system documentation},
} 

@inproceedings{Shi:2011:ESE:1987434.1987473,
	author = {Shi, Lin and Zhong, Hao and Xie, Tao and Li, Mingshu},
	title = {An empirical study on evolution of API documentation},
	booktitle = {Proceedings of the 14th international conference on Fundamental approaches to software engineering: part of the joint European conferences on theory and practice of software},
	series = {FASE'11/ETAPS'11},
	year = {2011},
	isbn = {978-3-642-19810-6},
	location = {Saarbr\&\#252;cken, Germany},
	pages = {416--431},
	numpages = {16},
	url = {http://dl.acm.org/citation.cfm?id=1987434.1987473},
	acmid = {1987473},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
}

@article{Kajko-Mattsson:2005:SDP:1032622.1035374,
	author = {Kajko-Mattsson, Mira},
	title = {A Survey of Documentation Practice within Corrective Maintenance},
	journal = {Empirical Softw. Engg.},
	issue_date = {January 2005},
	volume = {10},
	number = {1},
	month = jan,
	year = {2005},
	issn = {1382-3256},
	pages = {31--55},
	numpages = {25},
	url = {http://dx.doi.org/10.1023/B:LIDA.0000048322.42751.ca},
	doi = {10.1023/B:LIDA.0000048322.42751.ca},
	acmid = {1035374},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Corrective maintenance, software process documentation, software system documentation},
}

@inproceedings{Dekel:2009:IAD:1555001.1555047,
	author = {Dekel, Uri and Herbsleb, James D.},
	title = {Improving API documentation usability with knowledge pushing},
	booktitle = {Proceedings of the 31st International Conference on Software Engineering},
	series = {ICSE '09},
	year = {2009},
	isbn = {978-1-4244-3453-4},
	pages = {320--330},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2009.5070532},
	doi = {10.1109/ICSE.2009.5070532},
	acmid = {1555047},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Storey05,
	author={Storey, M.},
	booktitle={Program Comprehension, 2005. IWPC 2005. Proceedings. 13th International Workshop on},
	title={Theories, methods and tools in program comprehension: past, present and future},
	year={2005},
	pages={181-191},
	doi={10.1109/WPC.2005.38},
	ISSN={1092-8138}
}

@inproceedings{Dekel09,
	author={Dekel, Uri and Herbsleb, J.D.},
	booktitle={Program Comprehension, 2009. ICPC '09. IEEE 17th International Conference on},
	title={Reading the documentation of invoked API functions in program comprehension},
	year={2009},
	pages={168-177},
	doi={10.1109/ICPC.2009.5090040},
	ISSN={1092-8138}
}

@inproceedings{Fluri:2007:CCC:1339262.1339530,
	author = {Fluri, Beat and Wursch, Michael and Gall, Harald C.},
	title = {Do Code and Comments Co-Evolve? On the Relation between Source Code and Comment Changes},
	booktitle = {Proceedings of the 14th Working Conference on Reverse Engineering},
	series = {WCRE '07},
	year = {2007},
	isbn = {0-7695-3034-6},
	pages = {70--79},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/WCRE.2007.21},
	doi = {10.1109/WCRE.2007.21},
	acmid = {1339530},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Fluri:2009:ACC:1613014.1613065,
	author = {Fluri, Beat and W\"{u}rsch, Michael and Giger, Emanuel and Gall, Harald C.},
	title = {Analyzing the co-evolution of comments and source code},
	journal = {Software Quality Control},
	issue_date = {December  2009},
	volume = {17},
	number = {4},
	month = dec,
	year = {2009},
	issn = {0963-9314},
	pages = {367--394},
	numpages = {28},
	url = {http://dx.doi.org/10.1007/s11219-009-9075-x},
	doi = {10.1007/s11219-009-9075-x},
	acmid = {1613065},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Comment changes, Comment quality, Software evolution analysis, Software maintenance, Software repositories, Source code changes},
} 

@article{Ibrahim:2012:CCR:2330373.2330435,
	author = {Ibrahim, Walid M. and Bettenburg, Nicolas and Adams, Bram and Hassan, Ahmed E.},
	title = {Controversy Corner: On the relationship between comment update practices and Software Bugs},
	journal = {J. Syst. Softw.},
	issue_date = {October, 2012},
	volume = {85},
	number = {10},
	month = oct,
	year = {2012},
	issn = {0164-1212},
	pages = {2293--2304},
	numpages = {12},
	url = {http://dx.doi.org/10.1016/j.jss.2011.09.019},
	doi = {10.1016/j.jss.2011.09.019},
	acmid = {2330435},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {Code quality, Empirical studies, Software bugs, Software evolution, Source code comments},
} 

@inproceedings{Forward:2002:RSD:585058.585065,
	author = {Forward, Andrew and Lethbridge, Timothy C.},
	title = {The relevance of software documentation, tools and technologies: a survey},
	booktitle = {Proceedings of the 2002 ACM symposium on Document engineering},
	series = {DocEng '02},
	year = {2002},
	isbn = {1-58113-594-7},
	location = {McLean, Virginia, USA},
	pages = {26--33},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/585058.585065},
	doi = {10.1145/585058.585065},
	acmid = {585065},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation relevance, documentation survey, documentation technologies, program comprehension, software documentation, software engineering, software maintenance},
}

@inproceedings{Roehm:2012:PDC:2337223.2337254,
	author = {Roehm, Tobias and Tiarks, Rebecca and Koschke, Rainer and Maalej, Walid},
	title = {How do professional developers comprehend software?},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {255--265},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337254},
	acmid = {2337254},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@inproceedings{Friendly95thedesign,
	author = {Lisa Friendly},
	title = {The Design of Distributed Hyperlinked Programming Documentation},
	booktitle = {Proceedings of the International Workshop on Hypermedia Design},
	series = {IWDH '95},
	pages = {151--173},
	year = {1995}
}

@inproceedings{Kramer:1999:ADS:318372.318577,
	author = {Kramer, Douglas},
	title = {API documentation from source code comments: a case study of Javadoc},
	booktitle = {Proceedings of the 17th annual international conference on Computer documentation},
	series = {SIGDOC '99},
	year = {1999},
	isbn = {1-58113-072-4},
	location = {New Orleans, Louisiana, USA},
	pages = {147--153},
	numpages = {7},
	url = {http://doi.acm.org/10.1145/318372.318577},
	doi = {10.1145/318372.318577},
	acmid = {318577},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {API documentation, Java platform, Javadoc, doc comments, doclets, documentation comments, generated documentation, source code comments},
} 

@article{Sillito:2008:AAQ:1446226.1446241,
	author = {Sillito, Jonathan and Murphy, Gail C. and De Volder, Kris},
	title = {Asking and Answering Questions during a Programming Change Task},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {July 2008},
	volume = {34},
	number = {4},
	month = jul,
	year = {2008},
	issn = {0098-5589},
	pages = {434--451},
	numpages = {18},
	url = {http://dx.doi.org/10.1109/TSE.2008.26},
	doi = {10.1109/TSE.2008.26},
	acmid = {1446241},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Enhancement, Programming Environments/Construction Tools, Software psychology, Software psychology, Programming Environments/Construction Tools, Enhancement},
} 

@inproceedings{Sim:1998:ASC:580914.858229,
	author = {Sim, S. E. and Clarke, C. L. A. and Holt, R. C.},
	title = {Archetypal Source Code Searches: A Survey of Software Developers and Maintainers},
	booktitle = {Proceedings of the 6th International Workshop on Program Comprehension},
	series = {IWPC '98},
	year = {1998},
	isbn = {0-8186-8560-3},
	pages = {180--},
	url = {http://dl.acm.org/citation.cfm?id=580914.858229},
	acmid = {858229},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Duala-Ekoko:2012:AAQ:2337223.2337255,
	author = {Duala-Ekoko, Ekwa and Robillard, Martin P.},
	title = {Asking and answering questions about unfamiliar APIs: an exploratory study},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {266--276},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337255},
	acmid = {2337255},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@article{Binkley:2007:ESS:1217295.1217297,
	author = {Binkley, David and Gold, Nicolas and Harman, Mark},
	title = {An empirical study of static program slice size},
	journal = {ACM Trans. Softw. Eng. Methodol.},
	issue_date = {April 2007},
	volume = {16},
	number = {2},
	month = apr,
	year = {2007},
	issn = {1049-331X},
	articleno = {8},
	url = {http://doi.acm.org/10.1145/1217295.1217297},
	doi = {10.1145/1217295.1217297},
	acmid = {1217297},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Program slicing, slice size},
} 

@techreport{
	yiji_2012_tr,
	author = "Yiji Zhang and Raul Santelices",
	institution = "University of Notre Dame Computer Science Department",
	title = "Predicting Runtime Data Dependences for Slice Inspection Prioritization",
	number = "2012-02",
	month = "July",
	year = "2012"
}

@article{Miller:1995:WLD:219717.219748,
	author = {Miller, George A.},
	title = {WordNet: A Lexical Database for English},
	journal = {Commun. ACM},
	issue_date = {Nov. 1995},
	volume = {38},
	number = {11},
	month = nov,
	year = {1995},
	issn = {0001-0782},
	pages = {39--41},
	numpages = {3},
	url = {http://doi.acm.org/10.1145/219717.219748},
	doi = {10.1145/219717.219748},
	acmid = {219748},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Hill:2009:ACS:1555001.1555039,
	author = {Hill, Emily and Pollock, Lori and Vijay-Shanker, K.},
	title = {Automatically capturing source code context of NL-queries for software maintenance and reuse},
	booktitle = {Proceedings of the 31st International Conference on Software Engineering},
	series = {ICSE '09},
	year = {2009},
	isbn = {978-1-4244-3453-4},
	pages = {232--242},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2009.5070524},
	doi = {10.1109/ICSE.2009.5070524},
	acmid = {1555039},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Sridhara:2010:TAG:1858996.1859006,
	author = {Sridhara, Giriprasad and Hill, Emily and Muppaneni, Divya and Pollock, Lori and Vijay-Shanker, K.},
	title = {Towards automatically generating summary comments for Java methods},
	booktitle = {Proceedings of the IEEE/ACM international conference on Automated software engineering},
	series = {ASE '10},
	year = {2010},
	isbn = {978-1-4503-0116-9},
	location = {Antwerp, Belgium},
	pages = {43--52},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1858996.1859006},
	doi = {10.1145/1858996.1859006},
	acmid = {1859006},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {comment generation, method summarization, natural language program analysis},
} 

@inproceedings{Mani:2012:AAU:2393596.2393607,
	author = {Mani, Senthil and Catherine, Rose and Sinha, Vibha Singhal and Dubey, Avinava},
	title = {AUSUM: approach for unsupervised bug report summarization},
	booktitle = {Proceedings of the ACM SIGSOFT 20th International Symposium on the Foundations of Software Engineering},
	series = {FSE '12},
	year = {2012},
	isbn = {978-1-4503-1614-9},
	location = {Cary, North Carolina},
	pages = {11:1--11:11},
	articleno = {11},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2393596.2393607},
	doi = {10.1145/2393596.2393607},
	acmid = {2393607},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug report, summarization, unsupervised},
} 

@inproceedings{Burden:2011:NLG:2095654.2095665,
	author = {Burden, H{\aa}kan and Heldal, Rogardt},
	title = {Natural language generation from class diagrams},
	booktitle = {Proceedings of the 8th International Workshop on Model-Driven Engineering, Verification and Validation},
	series = {MoDeVVa},
	year = {2011},
	isbn = {978-1-4503-0914-1},
	location = {Wellington, New Zealand},
	pages = {8:1--8:8},
	articleno = {8},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/2095654.2095665},
	doi = {10.1145/2095654.2095665},
	acmid = {2095665},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {model transformations, model-driven architecture},
} 

@inproceedings{Sridhara:2011:GPC:2057176.2057211,
	author = {Sridhara, Giriprasad and Pollock, Lori and Vijay-Shanker, K.},
	title = {Generating Parameter Comments and Integrating with Method Summaries},
	booktitle = {Proceedings of the 2011 IEEE 19th International Conference on Program Comprehension},
	series = {ICPC '11},
	year = {2011},
	isbn = {978-0-7695-4398-7},
	pages = {71--80},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICPC.2011.28},
	doi = {10.1109/ICPC.2011.28},
	acmid = {2057211},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {documentation, software maintenance},
} 

@electronic{DoxygenWebsite,
	author        = "Dimitri van Heesch",
	title         = "Doxygen Website",
	url           = "http://www.stack.nl/~dimitri/doxygen/",
	year          = "2013"
}

@article{Curtis1989167,
	title = "Experimental evaluation of software documentation formats",
	journal = "Journal of Systems and Software",
	volume = "9",
	number = "2",
	pages = "167 - 207",
	year = "1989",
	issn = "0164-1212",
	doi = "10.1016/0164-1212(89)90019-8",
	url = "http://www.sciencedirect.com/science/article/pii/0164121289900198",
	author = "Bill Curtis and Sylvia B. Sheppard and Elizabeth Kruesi-Bailey and John Bailey and Deborah A. Boehm-Davis"
}

@inproceedings{Sridhara:2011:ADD:1985793.1985808,
	author = {Sridhara, Giriprasad and Pollock, Lori and Vijay-Shanker, K.},
	title = {Automatically detecting and describing high level actions within methods},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {101--110},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985808},
	doi = {10.1145/1985793.1985808},
	acmid = {1985808},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation, program comprehension},
} 

@article{Takang96,
	author = {Takang, A. A. and Grubb, P. A. and Macredie, R. D.},
	citeulike-article-id = {8398723},
	journal = {Journal of Programming Languages},
	keywords = {paolos, references},
	number = {3},
	pages = {143--167},
	posted-at = {2010-12-09 10:57:36},
	priority = {3},
	title = {{The Effects of Comments and Identifier Names on Program Comprehensibility: An Experimental Study}},
	volume = {4},
	year = {1996}
}

@INPROCEEDINGS{Lawrie06whatsin,
	author = {Dawn Lawrie and Christopher Morrell and Henry Feild and David Binkley},
	title = {What's in a name? a study of identifiers},
	booktitle = {In 14th International Conference on Program Comprehension},
	year = {2006},
	pages = {3--12},
	publisher = {IEEE Computer Society}
}

@article{Lethbridge:2003:SEU:950628.950726,
	author = {Lethbridge, Timothy C. and Singer, Janice and Forward, Andrew},
	title = {How Software Engineers Use Documentation: The State of the Practice},
	journal = {IEEE Softw.},
	issue_date = {November 2003},
	volume = {20},
	number = {6},
	month = nov,
	year = {2003},
	issn = {0740-7459},
	pages = {35--39},
	numpages = {5},
	url = {http://dx.doi.org/10.1109/MS.2003.1241364},
	doi = {10.1109/MS.2003.1241364},
	acmid = {950726},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
	keywords = {D.210.b Design notations and documentation, D.2.7.c Documentation, D.2.17g Code documentation},
}

@inproceedings{Stylos:2006:MWT:1174509.1174678,
	author = {Stylos, Jeffrey and Myers, Brad A.},
	title = {Mica: A Web-Search Tool for Finding API Components and Examples},
	booktitle = {Proceedings of the Visual Languages and Human-Centric Computing},
	series = {VLHCC '06},
	year = {2006},
	isbn = {0-7695-2586-5},
	pages = {195--202},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/VLHCC.2006.32},
	doi = {10.1109/VLHCC.2006.32},
	acmid = {1174678},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Eisenberg:2010:ANI:1753326.1753525,
	author = {Eisenberg, Daniel S. and Stylos, Jeffrey and Myers, Brad A.},
	title = {Apatite: a new interface for exploring APIs},
	booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
	series = {CHI '10},
	year = {2010},
	isbn = {978-1-60558-929-9},
	location = {Atlanta, Georgia, USA},
	pages = {1331--1334},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1753326.1753525},
	doi = {10.1145/1753326.1753525},
	acmid = {1753525},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {api documentation, browsing, search tools, visualizations, web applications},
} 

@inproceedings{Karrer:2011:SCG:2047196.2047225,
	author = {Karrer, Thorsten and Kr\"{a}mer, Jan-Peter and Diehl, Jonathan and Hartmann, Bj\"{o}rn and Borchers, Jan},
	title = {Stacksplorer: call graph navigation helps increasing code maintenance efficiency},
	booktitle = {Proceedings of the 24th annual ACM symposium on User interface software and technology},
	series = {UIST '11},
	year = {2011},
	isbn = {978-1-4503-0716-1},
	location = {Santa Barbara, California, USA},
	pages = {217--224},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/2047196.2047225},
	doi = {10.1145/2047196.2047225},
	acmid = {2047225},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {development tools / toolkits / programming environments, visualization},
}

@inproceedings{Tao:2012:SEU:2393596.2393656,
	author = {Tao, Yida and Dang, Yingnong and Xie, Tao and Zhang, Dongmei and Kim, Sunghun},
	title = {How do software engineers understand code changes?: an exploratory study in industry},
	booktitle = {Proceedings of the ACM SIGSOFT 20th International Symposium on the Foundations of Software Engineering},
	series = {FSE '12},
	year = {2012},
	isbn = {978-1-4503-1614-9},
	location = {Cary, North Carolina},
	pages = {51:1--51:11},
	articleno = {51},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2393596.2393656},
	doi = {10.1145/2393596.2393656},
	acmid = {2393656},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {code change, code review, information needs, tool support},
} 

@inproceedings{LaToza:2010:DAR:1806799.1806829,
	author = {LaToza, Thomas D. and Myers, Brad A.},
	title = {Developers ask reachability questions},
	booktitle = {Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering - Volume 1},
	series = {ICSE '10},
	year = {2010},
	isbn = {978-1-60558-719-6},
	location = {Cape Town, South Africa},
	pages = {185--194},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1806799.1806829},
	doi = {10.1145/1806799.1806829},
	acmid = {1806829},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {code navigation, developer questions, empirical study, program comprehension, software maintenance},
} 

@inproceedings{Stylos:2009:JIA:1520340.1520678,
	author = {Stylos, Jeffrey and Myers, Brad A. and Yang, Zizhuang},
	title = {Jadeite: improving API documentation using usage information},
	booktitle = {CHI '09 Extended Abstracts on Human Factors in Computing Systems},
	series = {CHI EA '09},
	year = {2009},
	isbn = {978-1-60558-247-4},
	location = {Boston, MA, USA},
	pages = {4429--4434},
	numpages = {6},
	url = {http://doi.acm.org/10.1145/1520340.1520678},
	doi = {10.1145/1520340.1520678},
	acmid = {1520678},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {APIs, documentation, javadoc},
}

@inproceedings{Ko:2004:SLB:1032665.1034570,
	author = {Ko, Andrew J. and Myers, Brad A. and Aung, Htet Htet},
	title = {Six Learning Barriers in End-User Programming Systems},
	booktitle = {Proceedings of the 2004 IEEE Symposium on Visual Languages - Human Centric Computing},
	series = {VLHCC '04},
	year = {2004},
	isbn = {0-7803-8696-5},
	pages = {199--206},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/VLHCC.2004.47},
	doi = {10.1109/VLHCC.2004.47},
	acmid = {1034570},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Steidl:2013:ICPC,
	author = {Steidl, Daniela and Hummel, Benjamin and Juergens, Elmar},
	title = {Quality Analysis of Source Code Comments},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	year = {2013},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@inproceedings{Smucker:07,
	author = {Smucker, Mark D. and Allan, James and Carterette, Ben},
	title = {A comparison of statistical significance tests for information retrieval evaluation},
	booktitle = {CIKM},
	year = {2007},
	pages = {623--632}
}

@inproceedings{Fagin:2003:CTK:644108.644113,
	author = {Fagin, Ronald and Kumar, Ravi and Sivakumar, D.},
	title = {Comparing top k lists},
	booktitle = {Proceedings of the fourteenth annual ACM-SIAM symposium on Discrete algorithms},
	series = {SODA '03},
	year = {2003},
	isbn = {0-89871-538-5},
	location = {Baltimore, Maryland},
	pages = {28--36},
	numpages = {9},
	url = {http://dl.acm.org/citation.cfm?id=644108.644113},
	acmid = {644113},
	publisher = {Society for Industrial and Applied Mathematics},
	address = {Philadelphia, PA, USA},
}

@article{Bansal:2009:CDP:1480540.1480730,
	author = {Bansal, Mukul S. and Fern\'{a}ndez-Baca, David},
	title = {Computing distances between partial rankings},
	journal = {Inf. Process. Lett.},
	issue_date = {January, 2009},
	volume = {109},
	number = {4},
	month = jan,
	year = {2009},
	issn = {0020-0190},
	pages = {238--241},
	numpages = {4},
	url = {http://dx.doi.org/10.1016/j.ipl.2008.10.010},
	doi = {10.1016/j.ipl.2008.10.010},
	acmid = {1480730},
	publisher = {Elsevier North-Holland, Inc.},
	address = {Amsterdam, The Netherlands, The Netherlands},
	keywords = {Algorithms, Kendall tau distance, Partial rankings, Top-m lists, p-ratings},
}

@article{wolfe1973nonparametric,
	title={Nonparametric statistical methods},
	author={Wolfe, Douglas A and Hollander, Myles},
	journal={Nonparametric statistical methods},
	year={1973},
	publisher={John Wiley New York}
}

@article{BBS:209012,
	author = {Rayner,Keith and Pollatsek,Alexander and Reichle,Erik D.},
	title = {Eye movements in reading: Models and data},
	journal = {Behavioral and Brain Sciences},
	volume = {26},
	issue = {04},
	month = {7},
	year = {2003},
	issn = {1469-1825},
	pages = {507--518},
	numpages = {12},
	doi = {10.1017/S0140525X03520106},
	URL = {http://journals.cambridge.org/article_S0140525X03520106},
}

@inproceedings{SaiZhang:2011:ADI:2190078.2190153,
	author = {Sai Zhang and Cheng Zhang and Ernst, Michael D.},
	title = {Automated documentation inference to explain failed tests},
	booktitle = {Proceedings of the 2011 26th IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '11},
	year = {2011},
	isbn = {978-1-4577-1638-6},
	pages = {63--72},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ASE.2011.6100145},
	doi = {10.1109/ASE.2011.6100145},
	acmid = {2190153},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@PhdThesis{MurphyPhd96,
	title = "{Lightweight structural summarization as an aid to software evolution}",
	author = "Gail C. Murphy",
	school = "University of Washington",
	month = "July",
	year = "1996",
}

@inproceedings{Buse:2008:ADI:1390630.1390664,
	author = {Buse, Raymond P.L. and Weimer, Westley R.},
	title = {Automatic documentation inference for exceptions},
	booktitle = {Proceedings of the 2008 international symposium on Software testing and analysis},
	series = {ISSTA '08},
	year = {2008},
	isbn = {978-1-60558-050-0},
	location = {Seattle, WA, USA},
	pages = {273--282},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1390630.1390664},
	doi = {10.1145/1390630.1390664},
	acmid = {1390664},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation inference, exception handling, software documentation},
}

@inproceedings{Buse:2010:ADP:1858996.1859005,
	author = {Buse, Raymond P.L. and Weimer, Westley R.},
	title = {Automatically documenting program changes},
	booktitle = {Proceedings of the IEEE/ACM international conference on Automated software engineering},
	series = {ASE '10},
	year = {2010},
	isbn = {978-1-4503-0116-9},
	location = {Antwerp, Belgium},
	pages = {33--42},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1858996.1859005},
	doi = {10.1145/1858996.1859005},
	acmid = {1859005},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {code summarization, commit messages, differencing},
}

@ARTICLE{6165314,
	author={Miryung Kim and Notkin, D. and Grossman, D. and Wilson, G.},
	journal={IEEE Transactions on Software Engineering},
	title={Identifying and Summarizing Systematic Code Changes via Rule Inference},
	year={2013},
	month={Jan. },
	volume={39},
	number={1},
	pages={45 -62},
	doi={10.1109/TSE.2012.16},
	ISSN={0098-5589},
}

@inproceedings{Aponte:2011:ITL:1987856.1987867,
	author = {Aponte, Jairo and Marcus, Andrian},
	title = {Improving traceability link recovery methods through software artifact summarization},
	booktitle = {Proceedings of the 6th International Workshop on Traceability in Emerging Forms of Software Engineering},
	series = {TEFSE '11},
	year = {2011},
	isbn = {978-1-4503-0589-1},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {46--49},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1987856.1987867},
	doi = {10.1145/1987856.1987867},
	acmid = {1987867},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {information retrieval, program comprehension, summarization, traceability management},
}

@article{Connelly:2010:LTT:1791129.1791137,
	author = {Connelly, Richard},
	title = {Lessons and Tools from Teaching a Blind Student},
	journal = {J. Comput. Sci. Coll.},
	issue_date = {June 2010},
	volume = {25},
	number = {6},
	month = jun,
	year = {2010},
	issn = {1937-4771},
	pages = {34--39},
	numpages = {6},
	url = {http://dl.acm.org/citation.cfm?id=1791129.1791137},
	acmid = {1791137},
	publisher = {Consortium for Computing Sciences in Colleges},
	address = {USA},
}

@article{Crosby:1990:WRA:77577.77580,
	author = {Crosby, Martha E. and Stelovsky, Jan},
	title = {How Do We Read Algorithms? A Case Study},
	journal = {Computer},
	issue_date = {January 1990},
	volume = {23},
	number = {1},
	month = jan,
	year = {1990},
	issn = {0018-9162},
	pages = {24--35},
	numpages = {12},
	url = {http://dl.acm.org/citation.cfm?id=77577.77580},
	acmid = {77580},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{Bednarik:2006:EMC:1117309.1117356,
	author = {Bednarik, Roman and Tukiainen, Markku},
	title = {An eye-tracking methodology for characterizing program comprehension processes},
	booktitle = {Proceedings of the 2006 symposium on Eye tracking research \& applications},
	series = {ETRA '06},
	year = {2006},
	isbn = {1-59593-305-0},
	location = {San Diego, California},
	pages = {125--132},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1117309.1117356},
	doi = {10.1145/1117309.1117356},
	acmid = {1117356},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {eye-movement tracking methodology, program comprehension, program visualization, psychology of programming},
} 

@inproceedings{Sharif:2012:ESR:2168556.2168642,
	author = {Sharif, Bonita and Falcone, Michael and Maletic, Jonathan I.},
	title = {An eye-tracking study on the role of scan time in finding source code defects},
	booktitle = {Proceedings of the Symposium on Eye Tracking Research and Applications},
	series = {ETRA '12},
	year = {2012},
	isbn = {978-1-4503-1221-9},
	location = {Santa Barbara, California},
	pages = {381--384},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/2168556.2168642},
	doi = {10.1145/2168556.2168642},
	acmid = {2168642},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {eye-tracking study, software defects, source-code review},
} 

@inproceedings{Sharif:2011:EAU:2117694.2119672,
	author = {Sharif, Bonita},
	title = {Empirical assessment of UML class diagram layouts based on architectural importance},
	booktitle = {Proceedings of the 2011 27th IEEE International Conference on Software Maintenance},
	series = {ICSM '11},
	year = {2011},
	isbn = {978-1-4577-0663-9},
	pages = {544--549},
	numpages = {6},
	url = {http://dx.doi.org/10.1109/ICSM.2011.6080828},
	doi = {10.1109/ICSM.2011.6080828},
	acmid = {2119672},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Sharif:2010:ELD:1796177.1796642,
	author = {Sharif, Bonita and Maletic, Jonathan I.},
	title = {The Effects of Layout on Detecting the Role of Design Patterns},
	booktitle = {Proceedings of the 2010 23rd IEEE Conference on Software Engineering Education and Training},
	series = {CSEET '10},
	year = {2010},
	isbn = {978-0-7695-4054-2},
	pages = {41--48},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/CSEET.2010.23},
	acmid = {1796642},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Binkley:2013:IIS:2436118.2436136,
	author = {Binkley, Dave and Davis, Marcia and Lawrie, Dawn and Maletic, Jonathan I. and Morrell, Christopher and Sharif, Bonita},
	title = {The impact of identifier style on effort and comprehension},
	journal = {Empirical Softw. Engg.},
	issue_date = {April     2013},
	volume = {18},
	number = {2},
	month = apr,
	year = {2013},
	issn = {1382-3256},
	pages = {219--276},
	numpages = {58},
	url = {http://dx.doi.org/10.1007/s10664-012-9201-4},
	doi = {10.1007/s10664-012-9201-4},
	acmid = {2436136},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Code readability, Coding standards, Eye-tracking study, Identifier names, Identifier styles, Memory, Program comprehension, Text recognition},
} 

@inproceedings{Sharif:2010:ETS:1846454.1847968,
	author = {Sharif, Bonita and Maletic, Jonathan I.},
	title = {An Eye Tracking Study on camelCase and under\_score Identifier Styles},
	booktitle = {Proceedings of the 2010 IEEE 18th International Conference on Program Comprehension},
	series = {ICPC '10},
	year = {2010},
	isbn = {978-0-7695-4113-6},
	pages = {196--205},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICPC.2010.41},
	doi = {10.1109/ICPC.2010.41},
	acmid = {1847968},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {identifier styles, eye-tracking study, code readability},
} 

@inproceedings{Bednarik:2008:TED:1344471.1344497,
	author = {Bednarik, Roman and Tukiainen, Markku},
	title = {Temporal eye-tracking data: evolution of debugging strategies with multiple representations},
	booktitle = {Proceedings of the 2008 symposium on Eye tracking research \&\#38; applications},
	series = {ETRA '08},
	year = {2008},
	isbn = {978-1-59593-982-1},
	location = {Savannah, Georgia},
	pages = {99--102},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1344471.1344497},
	doi = {10.1145/1344471.1344497},
	acmid = {1344497},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Uwano:2006:AIP:1117309.1117357,
	author = {Uwano, Hidetake and Nakamura, Masahide and Monden, Akito and Matsumoto, Ken-ichi},
	title = {Analyzing individual performance of source code review using reviewers' eye movement},
	booktitle = {Proceedings of the 2006 symposium on Eye tracking research \& applications},
	series = {ETRA '06},
	year = {2006},
	isbn = {1-59593-305-0},
	location = {San Diego, California},
	pages = {133--140},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1117309.1117357},
	doi = {10.1145/1117309.1117357},
	acmid = {1117357},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {computer program, eye movement, human factor, source code review},
} 

@inproceedings{LaToza:2006:MMM:1134285.1134355,
	author = {LaToza, Thomas D. and Venolia, Gina and DeLine, Robert},
	title = {Maintaining mental models: a study of developer work habits},
	booktitle = {Proceedings of the 28th international conference on Software engineering},
	series = {ICSE '06},
	year = {2006},
	isbn = {1-59593-375-1},
	location = {Shanghai, China},
	pages = {492--501},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1134285.1134355},
	doi = {10.1145/1134285.1134355},
	acmid = {1134355},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {agile software development, code duplication, code ownership, communication, debugging, interruptions},
}

@inproceedings{Guzzi:2012:DSK:2337223.2337476,
	author = {Guzzi, Anja},
	title = {Documenting and sharing knowledge about code},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {1535--1538},
	numpages = {4},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337476},
	acmid = {2337476},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@inproceedings{Brandt:2010:EPI:1753326.1753402,
	author = {Brandt, Joel and Dontcheva, Mira and Weskamp, Marcos and Klemmer, Scott R.},
	title = {Example-centric programming: integrating web search into the development environment},
	booktitle = {Proceedings of the 28th international conference on Human factors in computing systems},
	series = {CHI '10},
	year = {2010},
	isbn = {978-1-60558-929-9},
	location = {Atlanta, Georgia, USA},
	pages = {513--522},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1753326.1753402},
	doi = {10.1145/1753326.1753402},
	acmid = {1753402},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {example-centric development},
}

@inproceedings{Kotonya:2008:ORL:1478087.1478113,
	author = {Kotonya, Gerald and Lock, Simon and Mariani, John},
	title = {Opportunistic Reuse: Lessons from Scrapheap Software Development},
	booktitle = {Proceedings of the 11th International Symposium on Component-Based Software Engineering},
	series = {CBSE '08},
	year = {2008},
	isbn = {978-3-540-87890-2},
	location = {Karlsruhe, Germany},
	pages = {302--309},
	numpages = {8},
	url = {http://dx.doi.org/10.1007/978-3-540-87891-9_20},
	doi = {10.1007/978-3-540-87891-9_20},
	acmid = {1478113},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
}

@ARTICLE{Davison00understandingand,
	author = {Joseph W. Davison and Dennis M. Mancl and William F. Opdyke},
	title = {Understanding and addressing the essential costs of evolving systems},
	journal = {Bell Labs Technical Journal},
	year = {2000},
	pages = {44--54}
}

@inproceedings{Mirghasemi:2011:QMB:2025113.2025184,
	author = {Mirghasemi, Salman and Barton, John J. and Petitpierre, Claude},
	title = {Querypoint: moving backwards on wrong values in the buggy execution},
	booktitle = {Proceedings of the 19th ACM SIGSOFT symposium and the 13th European conference on Foundations of software engineering},
	series = {ESEC/FSE '11},
	year = {2011},
	isbn = {978-1-4503-0443-6},
	location = {Szeged, Hungary},
	pages = {436--439},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/2025113.2025184},
	doi = {10.1145/2025113.2025184},
	acmid = {2025184},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {breakpoint, debugging, lastchange, locating defects, logging, querypoint, watchpoint},
}

@article{Douce91,
	author = {Douce, C.},
	title = {Long Term Comprehension of Software Systems: A Methodology for Study},
	journal = {Proc. Psychology of Programming Interest Group},
	year = {2001}
}

@inproceedings{Gonzalez:2004:CCM:985692.985707,
	author = {Gonz\'{a}lez, Victor M. and Mark, Gloria},
	title = {"Constant, constant, multi-tasking craziness": managing multiple working spheres},
	booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
	series = {CHI '04},
	year = {2004},
	isbn = {1-58113-702-8},
	location = {Vienna, Austria},
	pages = {113--120},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/985692.985707},
	doi = {10.1145/985692.985707},
	acmid = {985707},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {attention management, empirical study, information overload, interruptions, personal information management},
} 

@inproceedings{Kramer:2012:BLA:2337223.2337451,
	author = {Kr\"{a}mer, Jan-Peter and Kurz, Joachim and Karrer, Thorsten and Borchers, Jan},
	title = {Blaze},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {1457--1458},
	numpages = {2},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337451},
	acmid = {2337451},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@article{ALTMANN2001189,
	title = "Near-term memory in programming: a simulation-based analysis ",
	journal = "International Journal of Human-Computer Studies ",
	volume = "54",
	number = "2",
	pages = "189 - 210",
	year = "2001",
	note = "",
	issn = "1071-5819",
	doi = "http://dx.doi.org/10.1006/ijhc.2000.0407",
	url = "http://www.sciencedirect.com/science/article/pii/S1071581900904075",
	author = "Erik M. Altmann"
}

@article{Holmes:2013:SPS:2377656.2377657,
	author = {Holmes, Reid and Walker, Robert J.},
	title = {Systematizing pragmatic software reuse},
	journal = {ACM Trans. Softw. Eng. Methodol.},
	issue_date = {November 2012},
	volume = {21},
	number = {4},
	month = feb,
	year = {2013},
	issn = {1049-331X},
	pages = {20:1--20:44},
	articleno = {20},
	numpages = {44},
	url = {http://doi.acm.org/10.1145/2377656.2377657},
	doi = {10.1145/2377656.2377657},
	acmid = {2377657},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Gilligan, Software reuse, lightweight process and tooling, low commitment, planning, pragmatic software reuse, pragmatic-reuse plan enactment, pragmatic-reuse plans, source code investigation, white box reuse},
}

@article{Littman1987341,
	title = "Mental models and software maintenance ",
	journal = "Journal of Systems and Software ",
	volume = "7",
	number = "4",
	pages = "341 - 355",
	year = "1987",
	note = "",
	issn = "0164-1212",
	doi = "http://dx.doi.org/10.1016/0164-1212(87)90033-1",
	url = "http://www.sciencedirect.com/science/article/pii/0164121287900331",
	author = "David C. Littman and Jeannine Pinto and Stanley Letovsky and Elliot Soloway"
}

@inproceedings{Loyola2017ANA,
  title={A Neural Architecture for Generating Natural Language Descriptions from Source Code Changes},
  author={Pablo Loyola and Edison Marrese-Taylor and Yutaka Matsuo},
  booktitle={ACL},
  year={2017}
}

@inproceedings{neubig19naacl,
    title = {compare-mt: A Tool for Holistic Comparison of Language Generation Systems},
    author = {Graham Neubig and Zi-Yi Dou and Junjie Hu and Paul Michel and Danish Pruthi and Xinyi Wang},
    booktitle = {Meeting of the North American Chapter of the Association for Computational Linguistics (NAACL) Demo Track},
    address = {Minneapolis, USA},
    month = {June},
    url = {http://arxiv.org/abs/1903.07926},
    year = {2019}
}

@InProceedings{lu2017learning,
author="Lu, Yangyang
and Zhao, Zelong
and Li, Ge
and Jin, Zhi",
editor="Li, Zheng
and Jiang, He
and Li, Ge
and Zhou, Minghui
and Li, Ming",
title="Learning to Generate Comments for API-Based Code Snippets",
booktitle="Software Engineering and Methodology for Emerging Domains",
year="2019",
publisher="Springer Singapore",
address="Singapore",
pages="3--14",
isbn="978-981-15-0310-8"
}



@article{liang2018automatic,
  author    = {Yuding Liang and
               Kenny Q. Zhu},
  title     = {Automatic Generation of Text Descriptive Comments for Code Blocks},
  journal   = {CoRR},
  volume    = {abs/1808.06880},
  year      = {2018},
  url       = {http://arxiv.org/abs/1808.06880},
  archivePrefix = {arXiv},
  eprint    = {1808.06880},
  timestamp = {Sun, 02 Sep 2018 15:01:54 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1808-06880},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

  @inproceedings{nie2019framework,
 author = {Nie, Pengyu and Rai, Rishabh and Li, Junyi Jessy and Khurshid, Sarfraz and Mooney, Raymond J. and Gligoric, Milos},
 title = {A Framework for Writing Trigger-Action Todo Comments in Executable Format},
 year = {2019},
 isbn = {9781450355728},
 publisher = {Association for Computing Machinery},
 address = {New York, NY, USA},
 url = {https://doi.org/10.1145/3338906.3338965},
 doi = {10.1145/3338906.3338965},
 booktitle = {Proceedings of the 2019 27th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering},
 pages = {385–396},
 numpages = {12},
 keywords = {Todo comments, domain specific languages, trigger-action},
 location = {Tallinn, Estonia},
 series = {ESEC/FSE 2019}
}


@article{Ko200541,
	title = "A framework and methodology for studying the causes of software errors in programming systems ",
	journal = "Journal of Visual Languages and Computing ",
	volume = "16",
	number = "1–2",
	pages = "41 - 84",
	year = "2005",
	issn = "1045-926X",
	doi = "http://dx.doi.org/10.1016/j.jvlc.2004.08.003",
	url = "http://www.sciencedirect.com/science/article/pii/S1045926X04000394",
	author = "Andrew J. Ko and Brad A. Myers"
}

@inproceedings{Dearman:2005:ACV:1058432.1059367,
	author = {Dearman, David and Cox, Anthony and Fisher, Maryanne},
	title = {Adding Control-Flow to a Visual Data-Flow Representation},
	booktitle = {Proceedings of the 13th International Workshop on Program Comprehension},
	series = {IWPC '05},
	year = {2005},
	isbn = {0-7695-2254-8},
	pages = {297--306},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/WPC.2005.5},
	doi = {10.1109/WPC.2005.5},
	acmid = {1059367},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Eddy:2013:ICPC,
	author = {Eddy, Brian and Robinson, Jeffrey and Kraft, Nicholas and Carver, Jeffrey},
	title = {Evaluating Source Code Summarization Techniques: Replication and Expansion},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	year = {2013},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@article{Freeman:2003:RDF:903893.903930,
	author = {Freeman, Lee A.},
	title = {A refresher in data flow diagramming: an effective aid for analysts},
	journal = {Commun. ACM},
	issue_date = {September 2003},
	volume = {46},
	number = {9},
	month = sep,
	year = {2003},
	issn = {0001-0782},
	pages = {147--151},
	numpages = {5},
	url = {http://doi.acm.org/10.1145/903893.903930},
	doi = {10.1145/903893.903930},
	acmid = {903930},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@incollection{Anderson:1992,
	year={1992},
	isbn={978-3-540-55606-0},
	booktitle={Intelligent Tutoring Systems},
	volume={608},
	series={Lecture Notes in Computer Science},
	editor={Frasson, Claude and Gauthier, Gilles and McCalla, GordonI.},
	doi={10.1007/3-540-55606-0_68},
	title={The advantages of data flow diagrams for beginning programming},
	url={http://dx.doi.org/10.1007/3-540-55606-0_68},
	publisher={Springer Berlin Heidelberg},
	author={Anjaneyulu, K.S.R. and Anderson, JohnR.},
	pages={585-592}
}

@article{Ko:2006:ESD:1248728.1248780,
	author = {Ko, Andrew J. and Myers, Brad A. and Coblenz, Michael J. and Aung, Htet Htet},
	title = {An Exploratory Study of How Developers Seek, Relate, and Collect Relevant Information during Software Maintenance Tasks},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {December 2006},
	volume = {32},
	number = {12},
	month = dec,
	year = {2006},
	issn = {0098-5589},
	pages = {971--987},
	numpages = {17},
	url = {http://dx.doi.org/10.1109/TSE.2006.116},
	doi = {10.1109/TSE.2006.116},
	acmid = {1248780},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Program investigation, Program investigation, program understanding, program comprehension, empirical software engineering, information foraging, information scent., empirical software engineering, information foraging, information scent., program comprehension, program understanding},
}

@inproceedings{Singer:1997:ESE:782010.782031,
	author = {Singer, Janice and Lethbridge, Timothy and Vinson, Norman and Anquetil, Nicolas},
	title = {An examination of software engineering work practices},
	booktitle = {Proceedings of the 1997 conference of the Centre for Advanced Studies on Collaborative research},
	series = {CASCON '97},
	year = {1997},
	location = {Toronto, Ontario, Canada},
	pages = {21--},
	url = {http://dl.acm.org/citation.cfm?id=782010.782031},
	acmid = {782031},
	publisher = {IBM Press},
}

@article{Lakhotia:1993:USE:177728.177735,
	author = {Lakhotia, Arun},
	title = {Understanding someone else's code: analysis of experiences},
	journal = {J. Syst. Softw.},
	issue_date = {Dec. 1993},
	volume = {23},
	number = {3},
	month = dec,
	year = {1993},
	issn = {0164-1212},
	pages = {269--275},
	numpages = {7},
	url = {http://dx.doi.org/10.1016/0164-1212(93)90101-3},
	doi = {10.1016/0164-1212(93)90101-3},
	acmid = {177735},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
}

@inproceedings{fjeldstadt83,
	author = {Fjeldstad, R. K. and Hamlen, W. T.},
	booktitle = {Proceedings GUIDE 48},
	citeulike-article-id = {6922207},
	keywords = {maintenance},
	location = {Philadelphia, PA},
	month = apr,
	posted-at = {2010-03-27 23:13:35},
	priority = {2},
	title = {{Application Program Maintenance Study: Report to Our Respondents}},
	year = {1983}
}

@inproceedings{Roehm:2012:PDC:2337223.2337254,
	author = {Roehm, Tobias and Tiarks, Rebecca and Koschke, Rainer and Maalej, Walid},
	title = {How do professional developers comprehend software?},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {255--265},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337254},
	acmid = {2337254},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@inproceedings{Stylos:2006:MWT:1174509.1174678,
	author = {Stylos, Jeffrey and Myers, Brad A.},
	title = {Mica: A Web-Search Tool for Finding API Components and Examples},
	booktitle = {Proceedings of the Visual Languages and Human-Centric Computing},
	series = {VLHCC '06},
	year = {2006},
	isbn = {0-7695-2586-5},
	pages = {195--202},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/VLHCC.2006.32},
	doi = {10.1109/VLHCC.2006.32},
	acmid = {1174678},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@ARTICLE{1241364,
	author={Lethbridge, T.C. and Singer, J. and Forward, A.},
	journal={Software, IEEE},
	title={How software engineers use documentation: the state of the practice},
	year={2003},
	volume={20},
	number={6},
	pages={35-39},
	keywords={software engineering;system documentation;decision making;documentation update;documentation use;software engineering;software engineers;software process managers;software process personnel;tool design;Data engineering;Documentation;Humans;Maintenance engineering;Power engineering and energy;Software engineering;Software maintenance;Software systems;Software testing;System testing},
	doi={10.1109/MS.2003.1241364},
	ISSN={0740-7459}
}

@inproceedings{Forward:2002:RSD:585058.585065,
	author = {Forward, Andrew and Lethbridge, Timothy C.},
	title = {The relevance of software documentation, tools and technologies: a survey},
	booktitle = {Proceedings of the 2002 ACM symposium on Document engineering},
	series = {DocEng '02},
	year = {2002},
	isbn = {1-58113-594-7},
	location = {McLean, Virginia, USA},
	pages = {26--33},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/585058.585065},
	doi = {10.1145/585058.585065},
	acmid = {585065},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation relevance, documentation survey, documentation technologies, program comprehension, software documentation, software engineering, software maintenance},
} 

@inproceedings{Gweon:2007:EAT:1308174.1308329,
	author = {Gweon, G. and Bergman, L. and Castelli, V. and Bellamy, R. K. E.},
	title = {Evaluating an Automated Tool to Assist Evolutionary Document Generation},
	booktitle = {Proceedings of the IEEE Symposium on Visual Languages and Human-Centric Computing},
	series = {VLHCC '07},
	year = {2007},
	isbn = {0-7695-2987-9},
	pages = {243--248},
	numpages = {6},
	url = {http://dx.doi.org/10.1109/VLHCC.2007.20},
	doi = {10.1109/VLHCC.2007.20},
	acmid = {1308329},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Bergman:2005:DSA:1095034.1095067,
	author = {Bergman, Lawrence and Castelli, Vittorio and Lau, Tessa and Oblinger, Daniel},
	title = {DocWizards: a system for authoring follow-me documentation wizards},
	booktitle = {Proceedings of the 18th annual ACM symposium on User interface software and technology},
	series = {UIST '05},
	year = {2005},
	isbn = {1-59593-271-2},
	location = {Seattle, WA, USA},
	pages = {191--200},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1095034.1095067},
	doi = {10.1145/1095034.1095067},
	acmid = {1095067},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation generation, programming-by-demonstration},
} 

@inproceedings{5306335,
	author={Starke, J. and Luce, C. and Sillito, J.},
	booktitle={Software Maintenance, 2009. ICSM 2009. IEEE International Conference on},
	title={Searching and skimming: An exploratory study},
	year={2009},
	pages={157-166},
	keywords={software engineering;program comprehension;software system;source code search tools;Concrete;Data analysis;Information analysis;Java;Laboratories;Navigation;Programming profession;Software design;Software systems;Software tools},
	doi={10.1109/ICSM.2009.5306335},
	ISSN={1063-6773}
}

@inproceedings{Kramer:1999:ADS:318372.318577,
	author = {Kramer, Douglas},
	title = {API documentation from source code comments: a case study of Javadoc},
	booktitle = {Proceedings of the 17th annual international conference on Computer documentation},
	series = {SIGDOC '99},
	year = {1999},
	isbn = {1-58113-072-4},
	location = {New Orleans, Louisiana, USA},
	pages = {147--153},
	numpages = {7},
	url = {http://doi.acm.org/10.1145/318372.318577},
	doi = {10.1145/318372.318577},
	acmid = {318577},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {API documentation, Java platform, Javadoc, doc comments, doclets, documentation comments, generated documentation, source code comments},
} 

@inproceedings{deSouza:2005:SDE:1085313.1085331,
	author = {de Souza, Sergio Cozzetti B. and Anquetil, Nicolas and de Oliveira, K\'{a}thia M.},
	title = {A study of the documentation essential to software maintenance},
	booktitle = {Proceedings of the 23rd annual international conference on Design of communication: documenting \& designing for pervasive information},
	series = {SIGDOC '05},
	year = {2005},
	isbn = {1-59593-175-9},
	location = {Coventry, United Kingdom},
	pages = {68--75},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1085313.1085331},
	doi = {10.1145/1085313.1085331},
	acmid = {1085331},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {empirical study, program understanding, software maintenance, software system documentation},
}

@article{Kajko-Mattsson:2005:SDP:1032622.1035374,
	author = {Kajko-Mattsson, Mira},
	title = {A Survey of Documentation Practice within Corrective Maintenance},
	journal = {Empirical Softw. Engg.},
	issue_date = {January 2005},
	volume = {10},
	number = {1},
	month = jan,
	year = {2005},
	issn = {1382-3256},
	pages = {31--55},
	numpages = {25},
	url = {http://dx.doi.org/10.1023/B:LIDA.0000048322.42751.ca},
	doi = {10.1023/B:LIDA.0000048322.42751.ca},
	acmid = {1035374},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Corrective maintenance, software process documentation, software system documentation},
}

@inproceedings{Fluri:2007:CCC:1339262.1339530,
	author = {Fluri, Beat and Wursch, Michael and Gall, Harald C.},
	title = {Do Code and Comments Co-Evolve? On the Relation between Source Code and Comment Changes},
	booktitle = {Proceedings of the 14th Working Conference on Reverse Engineering},
	series = {WCRE '07},
	year = {2007},
	isbn = {0-7695-3034-6},
	pages = {70--79},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/WCRE.2007.21},
	doi = {10.1109/WCRE.2007.21},
	acmid = {1339530},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Ibrahim:2012:CCR:2330373.2330435,
	author = {Ibrahim, Walid M. and Bettenburg, Nicolas and Adams, Bram and Hassan, Ahmed E.},
	title = {Controversy Corner: On the relationship between comment update practices and Software Bugs},
	journal = {J. Syst. Softw.},
	issue_date = {October, 2012},
	volume = {85},
	number = {10},
	month = oct,
	year = {2012},
	issn = {0164-1212},
	pages = {2293--2304},
	numpages = {12},
	url = {http://dx.doi.org/10.1016/j.jss.2011.09.019},
	doi = {10.1016/j.jss.2011.09.019},
	acmid = {2330435},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {Code quality, Empirical studies, Software bugs, Software evolution, Source code comments},
}

@inproceedings{Sim:1998:ASC:580914.858229,
	author = {Sim, S. E. and Clarke, C. L. A. and Holt, R. C.},
	title = {Archetypal Source Code Searches: A Survey of Software Developers and Maintainers},
	booktitle = {Proceedings of the 6th International Workshop on Program Comprehension},
	series = {IWPC '98},
	year = {1998},
	isbn = {0-8186-8560-3},
	pages = {180--},
	url = {http://dl.acm.org/citation.cfm?id=580914.858229},
	acmid = {858229},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Sillito:2008:AAQ:1446226.1446241,
	author = {Sillito, Jonathan and Murphy, Gail C. and De Volder, Kris},
	title = {Asking and Answering Questions during a Programming Change Task},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {July 2008},
	volume = {34},
	number = {4},
	month = jul,
	year = {2008},
	issn = {0098-5589},
	pages = {434--451},
	numpages = {18},
	url = {http://dx.doi.org/10.1109/TSE.2008.26},
	doi = {10.1109/TSE.2008.26},
	acmid = {1446241},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Enhancement, Programming Environments/Construction Tools, Software psychology, Software psychology, Programming Environments/Construction Tools, Enhancement},
} 

@inproceedings{Burden:2011:NLG:2095654.2095665,
	author = {Burden, H{\aa}kan and Heldal, Rogardt},
	title = {Natural language generation from class diagrams},
	booktitle = {Proceedings of the 8th International Workshop on Model-Driven Engineering, Verification and Validation},
	series = {MoDeVVa},
	year = {2011},
	isbn = {978-1-4503-0914-1},
	location = {Wellington, New Zealand},
	pages = {8:1--8:8},
	articleno = {8},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/2095654.2095665},
	doi = {10.1145/2095654.2095665},
	acmid = {2095665},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {model transformations, model-driven architecture},
} 

@inproceedings{Mani:2012:AAU:2393596.2393607,
	author = {Mani, Senthil and Catherine, Rose and Sinha, Vibha Singhal and Dubey, Avinava},
	title = {AUSUM: approach for unsupervised bug report summarization},
	booktitle = {Proceedings of the ACM SIGSOFT 20th International Symposium on the Foundations of Software Engineering},
	series = {FSE '12},
	year = {2012},
	isbn = {978-1-4503-1614-9},
	location = {Cary, North Carolina},
	pages = {11:1--11:11},
	articleno = {11},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2393596.2393607},
	doi = {10.1145/2393596.2393607},
	acmid = {2393607},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug report, summarization, unsupervised},
} 

@inproceedings{Moreno:2013:ICPC,
	author = {Moreno, Laura and Aponte, Jairo and Sridhara Giriprasad and Marcus, Andrian and Pollock, Lori and Vijay-Shanker, K.},
	title = {Automatic Generation of Natural Language Summaries for Java Classes},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	year = {2013},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@inproceedings{Sridhara:2011:ADD:1985793.1985808,
	author = {Sridhara, Giriprasad and Pollock, Lori and Vijay-Shanker, K.},
	title = {Automatically detecting and describing high level actions within methods},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {101--110},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985808},
	doi = {10.1145/1985793.1985808},
	acmid = {1985808},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation, program comprehension},
}

@inproceedings{Sridhara:2010:TAG:1858996.1859006,
	author = {Sridhara, Giriprasad and Hill, Emily and Muppaneni, Divya and Pollock, Lori and Vijay-Shanker, K.},
	title = {Towards automatically generating summary comments for Java methods},
	booktitle = {Proceedings of the IEEE/ACM international conference on Automated software engineering},
	series = {ASE '10},
	year = {2010},
	isbn = {978-1-4503-0116-9},
	location = {Antwerp, Belgium},
	pages = {43--52},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1858996.1859006},
	doi = {10.1145/1858996.1859006},
	acmid = {1859006},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {comment generation, method summarization, natural language program analysis},
} 

@inproceedings{Zhong:2009:IRS:1747491.1747528,
	author = {Zhong, Hao and Zhang, Lu and Xie, Tao and Mei, Hong},
	title = {Inferring Resource Specifications from Natural Language API Documentation},
	booktitle = {Proceedings of the 2009 IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '09},
	year = {2009},
	isbn = {978-0-7695-3891-4},
	pages = {307--318},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/ASE.2009.94},
	doi = {10.1109/ASE.2009.94},
	acmid = {1747528},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}



@inproceedings{McMillan:2011:PFR:1985793.1985809,
	author = {McMillan, Collin and Grechanik, Mark and Poshyvanyk, Denys and Xie, Qing and Fu, Chen},
	title = {Portfolio: finding relevant functions and their usage},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {111--120},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985809},
	doi = {10.1145/1985793.1985809},
	acmid = {1985809},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {code search, function call graph, pagerank, portfolio, ranking},
} 

@PhdThesis{SridharaPhd12,
	title = "{Automatic Generation of Descriptive Summary Comments for Methods in Object-oriented Programs}",
	author = "Giriprasad Sridhara",
	school = "University of Delaware",
	month = Jan,
	year = "2012",
}

@inproceedings{Sridhara:2011:GPC:2057176.2057211,
	author = {Sridhara, Giriprasad and Pollock, Lori and Vijay-Shanker, K.},
	title = {Generating Parameter Comments and Integrating with Method Summaries},
	booktitle = {Proceedings of the 2011 IEEE 19th International Conference on Program Comprehension},
	series = {ICPC '11},
	year = {2011},
	isbn = {978-0-7695-4398-7},
	pages = {71--80},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICPC.2011.28},
	doi = {10.1109/ICPC.2011.28},
	acmid = {2057211},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {documentation, software maintenance},
}

@inproceedings{Haiduc:2010:UAT:1919284.1919577,
	author = {Haiduc, Sonia and Aponte, Jairo and Moreno, Laura and Marcus, Andrian},
	title = {On the Use of Automated Text Summarization Techniques for Summarizing Source Code},
	booktitle = {Proceedings of the 2010 17th Working Conference on Reverse Engineering},
	series = {WCRE '10},
	year = {2010},
	isbn = {978-0-7695-4123-5},
	pages = {35--44},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/WCRE.2010.13},
	doi = {10.1109/WCRE.2010.13},
	acmid = {1919577},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {text summarization, program comprehension},
}

@article{Herbsleb:2003:ESS:1435631.859041,
	author = {Herbsleb, James D. and Mockus, Audris},
	title = {An Empirical Study of Speed and Communication in Globally Distributed Software Development},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {June 2003},
	volume = {29},
	number = {6},
	month = jun,
	year = {2003},
	issn = {0098-5589},
	pages = {481--494},
	numpages = {14},
	url = {http://dx.doi.org/10.1109/TSE.2003.1205177},
	doi = {10.1109/TSE.2003.1205177},
	acmid = {859041},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Global development, collaboration, delay, speed, awareness, informal communication.},
}

@inproceedings{Aranda:2009:SLB:1555001.1555045,
	author = {Aranda, Jorge and Venolia, Gina},
	title = {The secret life of bugs: Going past the errors and omissions in software repositories},
	booktitle = {Proceedings of the 31st International Conference on Software Engineering},
	series = {ICSE '09},
	year = {2009},
	isbn = {978-1-4244-3453-4},
	pages = {298--308},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2009.5070530},
	doi = {10.1109/ICSE.2009.5070530},
	acmid = {1555045},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Cataldo:2006:ICR:1180875.1180929,
	author = {Cataldo, Marcelo and Wagstrom, Patrick A. and Herbsleb, James D. and Carley, Kathleen M.},
	title = {Identification of coordination requirements: implications for the Design of collaboration and awareness tools},
	booktitle = {Proceedings of the 2006 20th anniversary conference on Computer supported cooperative work},
	series = {CSCW '06},
	year = {2006},
	isbn = {1-59593-249-6},
	location = {Banff, Alberta, Canada},
	pages = {353--362},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1180875.1180929},
	doi = {10.1145/1180875.1180929},
	acmid = {1180929},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {collaboration tools, coordination, dynamic network analysis, task awareness tools},
}

@article{Curtis:1988:FSS:50087.50089,
	author = {Curtis, Bill and Krasner, Herb and Iscoe, Neil},
	title = {A field study of the software design process for large systems},
	journal = {Commun. ACM},
	issue_date = {Nov. 1988},
	volume = {31},
	number = {11},
	month = nov,
	year = {1988},
	issn = {0001-0782},
	pages = {1268--1287},
	numpages = {20},
	url = {http://doi.acm.org/10.1145/50087.50089},
	doi = {10.1145/50087.50089},
	acmid = {50089},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{deSouza:2008:ESS:1368088.1368122,
	author = {de Souza, Cleidson R. B. and Redmiles, David F.},
	title = {An empirical study of software developers' management of dependencies and changes},
	booktitle = {Proceedings of the 30th international conference on Software engineering},
	series = {ICSE '08},
	year = {2008},
	isbn = {978-1-60558-079-1},
	location = {Leipzig, Germany},
	pages = {241--250},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1368088.1368122},
	doi = {10.1145/1368088.1368122},
	acmid = {1368122},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {change impact analysis, collaborative software development, empirical studies, socio-technical aspects},
} 

@inproceedings{Leszak:2000:CSR:337180.337232,
	author = {Leszak, Marek and Perry, Dewayne E. and Stoll, Dieter},
	title = {A case study in root cause defect analysis},
	booktitle = {Proceedings of the 22nd international conference on Software engineering},
	series = {ICSE '00},
	year = {2000},
	isbn = {1-58113-206-9},
	location = {Limerick, Ireland},
	pages = {428--437},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/337180.337232},
	doi = {10.1145/337180.337232},
	acmid = {337232},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {defect prevention, modification management, process improvement, quality assurance, root cause analyis},
} 

@article {BLTJ:BLTJ2101,
	author = {Yu, Weider D.},
	title = {A software fault prevention approach in coding and root cause analysis},
	journal = {Bell Labs Technical Journal},
	volume = {3},
	number = {2},
	publisher = {Wiley Subscription Services, Inc., A Wiley Company},
	issn = {1538-7305},
	url = {http://dx.doi.org/10.1002/bltj.2101},
	doi = {10.1002/bltj.2101},
	pages = {3--21},
	year = {1998},
}

@inproceedings{Valetto:2007:USR:1268983.1269039,
	author = {Valetto, Giuseppe and Helander, Mary and Ehrlich, Kate and Chulani, Sunita and Wegman, Mark and Williams, Clay},
	title = {Using Software Repositories to Investigate Socio-technical Congruence in Development Projects},
	booktitle = {Proceedings of the Fourth International Workshop on Mining Software Repositories},
	series = {MSR '07},
	year = {2007},
	isbn = {0-7695-2950-X},
	pages = {25--},
	url = {http://dx.doi.org/10.1109/MSR.2007.33},
	doi = {10.1109/MSR.2007.33},
	acmid = {1269039},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Bugde:2008:GSS:1471606.1472247,
	author = {Bugde, Shilpa and Nagappan, Nachiappan and Rajamani, Sriram and Ramalingam, G.},
	title = {Global Software Servicing: Observational Experiences at Microsoft},
	booktitle = {Proceedings of the 2008 IEEE International Conference on Global Software Engineering},
	series = {ICGSE '08},
	year = {2008},
	isbn = {978-0-7695-3280-6},
	pages = {182--191},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICGSE.2008.18},
	doi = {10.1109/ICGSE.2008.18},
	acmid = {1472247},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Ashok:2009:DRS:1595696.1595766,
	author = {Ashok, B. and Joy, Joseph and Liang, Hongkang and Rajamani, Sriram K. and Srinivasa, Gopal and Vangala, Vipindeep},
	title = {DebugAdvisor: a recommender system for debugging},
	booktitle = {Proceedings of the the 7th joint meeting of the European software engineering conference and the ACM SIGSOFT symposium on The foundations of software engineering},
	series = {ESEC/FSE '09},
	year = {2009},
	isbn = {978-1-60558-001-2},
	location = {Amsterdam, The Netherlands},
	pages = {373--382},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1595696.1595766},
	doi = {10.1145/1595696.1595766},
	acmid = {1595766},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, recommendation systems, search},
}

@techreport{NIST_bugs_cost:2002,
	author = {Tassey, Gregory},
	title = {The Economic Impacts of Inadequate Infrastructure for Software Testing},
	institution = {National Institute of Standards \& Technology},
	month = {May},
	year = {2002}
}

@inproceedings{Weiss:2007:LTF:1268983.1269017,
	author = {Weiss, Cathrin and Premraj, Rahul and Zimmermann, Thomas and Zeller, Andreas},
	title = {How Long Will It Take to Fix This Bug?},
	booktitle = {Proceedings of the Fourth International Workshop on Mining Software Repositories},
	series = {MSR '07},
	year = {2007},
	isbn = {0-7695-2950-X},
	pages = {1--},
	url = {http://dx.doi.org/10.1109/MSR.2007.13},
	doi = {10.1109/MSR.2007.13},
	acmid = {1269017},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Guo:2010:CPB:1806799.1806871,
	author = {Guo, Philip J. and Zimmermann, Thomas and Nagappan, Nachiappan and Murphy, Brendan},
	title = {Characterizing and predicting which bugs get fixed: an empirical study of Microsoft Windows},
	booktitle = {Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering - Volume 1},
	series = {ICSE '10},
	year = {2010},
	isbn = {978-1-60558-719-6},
	location = {Cape Town, South Africa},
	pages = {495--504},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1806799.1806871},
	doi = {10.1145/1806799.1806871},
	acmid = {1806871},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Bettenburg:2007:QBR:1328279.1328284,
	author = {Bettenburg, Nicolas and Just, Sascha and Schr\"{o}ter, Adrian and Wei\ss, Cathrin and Premraj, Rahul and Zimmermann, Thomas},
	title = {Quality of bug reports in Eclipse},
	booktitle = {Proceedings of the 2007 OOPSLA workshop on eclipse technology eXchange},
	series = {eclipse '07},
	year = {2007},
	isbn = {978-1-60558-015-9},
	location = {Montreal, Quebec, Canada},
	pages = {21--25},
	numpages = {5},
	url = {http://doi.acm.org/10.1145/1328279.1328284},
	doi = {10.1145/1328279.1328284},
	acmid = {1328284},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@article{Treude:2012:WIT:2122269.2122542,
	author = {Treude, Christoph and Storey, Margaret-Anne},
	title = {Work Item Tagging: Communicating Concerns in Collaborative Software Development},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {January 2012},
	volume = {38},
	number = {1},
	month = jan,
	year = {2012},
	issn = {0098-5589},
	pages = {19--34},
	numpages = {16},
	url = {http://dx.doi.org/10.1109/TSE.2010.91},
	doi = {10.1109/TSE.2010.91},
	acmid = {2122542},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Tagging, collaboration, software development, task management, articulation work, work items.},
} 

@inproceedings{Bettenburg:2008:4658082,
	author={Bettenburg, N. and Premraj, R. and Zimmermann, T. and Sunghun Kim},
	booktitle={Software Maintenance, 2008. ICSM 2008. IEEE International Conference on},
	title={Duplicate bug reports considered harmful ... really?},
	year={2008},
	month={28 2008-oct. 4},
	volume={},
	number={},
	pages={337 -345},
	keywords={duplicate bug;open source projects;software maintenance;program debugging;public domain software;software maintenance;},
	doi={10.1109/ICSM.2008.4658082},
	ISSN={1063-6773}
}

@inproceedings{Bettenburg:2008:MGB:1453101.1453146,
	author = {Bettenburg, Nicolas and Just, Sascha and Schr\"{o}ter, Adrian and Wei\ss, Cathrin and Premraj, Rahul and Zimmermann, Thomas},
	title = {What makes a good bug report?},
	booktitle = {Proceedings of the 16th ACM SIGSOFT International Symposium on Foundations of software engineering},
	series = {SIGSOFT '08/FSE-16},
	year = {2008},
	isbn = {978-1-59593-995-1},
	location = {Atlanta, Georgia},
	pages = {308--318},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1453101.1453146},
	doi = {10.1145/1453101.1453146},
	acmid = {1453146},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Herbsleb:2001:GEI:624642.626244,
	author = {Herbsleb, James D. and Moitra, Deependra},
	title = {Guest Editors' Introduction: Global Software Development},
	journal = {IEEE Softw.},
	issue_date = {March 2001},
	volume = {18},
	number = {2},
	month = mar,
	year = {2001},
	issn = {0740-7459},
	pages = {16--20},
	numpages = {5},
	url = {http://dx.doi.org/10.1109/52.914732},
	doi = {10.1109/52.914732},
	acmid = {626244},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
}

@article{Grinter:1996:SAW:259640.259651,
	author = {Grinter, Rebecca E.},
	title = {Supporting articulation work using software configuration management systems},
	journal = {Comput. Supported Coop. Work},
	issue_date = {1996},
	volume = {5},
	number = {4},
	month = dec,
	year = {1996},
	issn = {0925-9724},
	pages = {447--465},
	numpages = {19},
	url = {http://dx.doi.org/10.1007/BF00136714},
	doi = {10.1007/BF00136714},
	acmid = {259651},
	publisher = {Kluwer Academic Publishers},
	address = {Norwell, MA, USA},
	keywords = {articulation work, computer-supported cooperated work, configuration management, coordination mechanisms, empirical studies},
} 

@inproceedings{Storey:2008:TBE:1368088.1368123,
	author = {Storey, Margaret-Anne and Ryall, Jody and Bull, R. Ian and Myers, Del and Singer, Janice},
	title = {TODO or to bug: exploring how task annotations play a role in the work practices of software developers},
	booktitle = {Proceedings of the 30th international conference on Software engineering},
	series = {ICSE '08},
	year = {2008},
	isbn = {978-1-60558-079-1},
	location = {Leipzig, Germany},
	pages = {251--260},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1368088.1368123},
	doi = {10.1145/1368088.1368123},
	acmid = {1368123},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {source code comments, task annotations, work practices},
}

@inproceedings{Ko:2006:LAP:1174509.1174667,
	author = {Ko, Andrew J. and Myers, Brad A. and Chau, Duen Horng},
	title = {A Linguistic Analysis of How People Describe Software Problems},
	booktitle = {Proceedings of the Visual Languages and Human-Centric Computing},
	series = {VLHCC '06},
	year = {2006},
	isbn = {0-7695-2586-5},
	pages = {127--134},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/VLHCC.2006.3},
	doi = {10.1109/VLHCC.2006.3},
	acmid = {1174667},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{deSouza:2205:SIGGROUP,
	author = {de Souza, C. and Froehlich, J. and Dourish, P.},
	title = {Seeking the Source: Software Source Code as a Social and Technical Artifact},
	booktitle = {Proceedings of the 2005 international ACM SIGGROUP conference on Supporting group work},
	series = {GROUP '05},
	year = {2005},
	isbn = {1-59593-223-2},
	location = {Sanibel Island, Florida, USA},
	pages = {107--206},
	numpages = {10},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Sandusky:2005:NCI:1099203.1099238,
	author = {Sandusky, Robert J. and Gasser, Les},
	title = {Negotiation and the coordination of information and activity in distributed software problem management},
	booktitle = {Proceedings of the 2005 international ACM SIGGROUP conference on Supporting group work},
	series = {GROUP '05},
	year = {2005},
	isbn = {1-59593-223-2},
	location = {Sanibel Island, Florida, USA},
	pages = {187--196},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1099203.1099238},
	doi = {10.1145/1099203.1099238},
	acmid = {1099238},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {coordination mechanisms, coordination theory, distributed collective practices, negotiation, software problem management},
}

@inproceedings{Kagdi:2007:MSR:1270394.1271355,
	author = {Kagdi, Huzefa and Maletic, Jonathan I. and Sharif, Bonita},
	title = {Mining Software Repositories for Traceability Links},
	booktitle = {Proceedings of the 15th IEEE International Conference on Program Comprehension},
	series = {ICPC '07},
	year = {2007},
	isbn = {0-7695-2860-0},
	pages = {145--154},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICPC.2007.28},
	doi = {10.1109/ICPC.2007.28},
	acmid = {1271355},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Murphy:1995:SRM:222124.222136,
	author = {Murphy, Gail C. and Notkin, David and Sullivan, Kevin},
	title = {Software reflexion models: bridging the gap between source and high-level models},
	booktitle = {Proceedings of the 3rd ACM SIGSOFT symposium on Foundations of software engineering},
	series = {SIGSOFT '95},
	year = {1995},
	isbn = {0-89791-716-2},
	location = {Washington, D.C., United States},
	pages = {18--28},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/222124.222136},
	doi = {10.1145/222124.222136},
	acmid = {222136},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@article{McMillan:10.1109/TSE.2011.84,
	author = {Collin McMillan and Mark Grechanik and Denys Poshyvanyk and Chen Fu and Qing Xie},
	title = {Exemplar: A Source Code Search Engine For Finding Highly Relevant Applications},
	journal ={IEEE Transactions on Software Engineering},
	volume = {99},
	number = {PrePrints},
	issn = {0098-5589},
	year = {2011},
	doi = {http://doi.ieeecomputersociety.org/10.1109/TSE.2011.84},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{McMillan:C:ICSE:2011,
	Author = {McMillan, C. and Grechanik, M. and Poshyvanyk, D. and Xie, Q. and Fu, C.},
	Title = {Portfolio: Finding Relevant Functions And Their Usages},
	BookTitle = {33rd IEEE/ACM International Conference on Software Engineering (ICSE'11)},
	Address= {Honolulu, Hawaii, USA},
	Pages = {111-120},
	Year = {2011} }

@inproceedings{Panis:5636546,
	author={Panis, M.C.},
	booktitle={Requirements Engineering Conference (RE), 2010 18th IEEE International}, title={Successful Deployment of Requirements Traceability in a Commercial Engineering Organization...Really},
	year={2010},
	month={27 2010-oct. 1},
	volume={},
	number={},
	pages={303 -307},
	keywords={commercial engineering organization;foregone conclusion;product development process;requirements engineering;requirements traceability;successful deployment;systems analysis;},
	doi={10.1109/RE.2010.43},
	ISSN={1090-705X}
}

@article{Binkley:2008:ESR:1454787.1454982,
	author = {Binkley, David and Gold, Nicolas and Harman, Mark and Li, Zheng and Mahdavi, Kiarash},
	title = {An empirical study of the relationship between the concepts expressed in source code and dependence},
	journal = {J. Syst. Softw.},
	issue_date = {December, 2008},
	volume = {81},
	number = {12},
	month = dec,
	year = {2008},
	issn = {0164-1212},
	pages = {2287--2298},
	numpages = {12},
	url = {http://dx.doi.org/10.1016/j.jss.2008.04.007},
	doi = {10.1016/j.jss.2008.04.007},
	acmid = {1454982},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {Concept assignment, Program comprehension, Program slicing, Software engineering},
}

@article{Zou:2010:IAR:1743628.1743653,
	author = {Zou, Xuchang and Settimi, Raffaella and Cleland-Huang, Jane},
	title = {Improving automated requirements trace retrieval: a study of term-based enhancement methods},
	journal = {Empirical Softw. Engg.},
	issue_date = {April     2010},
	volume = {15},
	number = {2},
	month = apr,
	year = {2010},
	issn = {1382-3256},
	pages = {119--146},
	numpages = {28},
	url = {http://dx.doi.org/10.1007/s10664-009-9114-z},
	doi = {10.1007/s10664-009-9114-z},
	acmid = {1743653},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Information retrieval models., Requirements management, Requirements traceability},
}

@article{Linstead2009,
	Author = {Linstead, Erik and Bajracharya, Sushil and Ngo, Trung and Rigor, Paul and Lopes, Cristina and Baldi, Pierre},
	Date-Modified = {2012-04-22 14:01:25 +0000},
	Journal = {Data Mining and Knowledge Discovery},
	Pages = {300-336},
	Title = {Sourcerer: mining and searching internet-scale software repositories},
	Volume = {18},
	Year = {2009},
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s10618-008-0118-x}
}

@inproceedings{Bajracharya:2010:LUS:1882291.1882316,
	author = {Bajracharya, Sushil K. and Ossher, Joel and Lopes, Cristina V.},
	title = {Leveraging usage similarity for effective retrieval of examples in code repositories},
	booktitle = {Proceedings of the eighteenth ACM SIGSOFT international symposium on Foundations of software engineering},
	series = {FSE '10},
	year = {2010},
	isbn = {978-1-60558-791-2},
	location = {Santa Fe, New Mexico, USA},
	pages = {157--166},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1882291.1882316},
	doi = {10.1145/1882291.1882316},
	acmid = {1882316},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {api usage, code search, software information retrieval, ssi, structural semantic indexing},
}

@inproceedings{Chan:2012:SCA:2393596.2393606,
	author = {Chan, Wing-Kwan and Cheng, Hong and Lo, David},
	title = {Searching connected API subgraph via text phrases},
	booktitle = {Proceedings of the ACM SIGSOFT 20th International Symposium on the Foundations of Software Engineering},
	series = {FSE '12},
	year = {2012},
	isbn = {978-1-4503-1614-9},
	location = {Cary, North Carolina},
	pages = {10:1--10:11},
	articleno = {10},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2393596.2393606},
	doi = {10.1145/2393596.2393606},
	acmid = {2393606},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {API graph, API recommendation, subgraph searching},
}

@inproceedings{McMillan:2012:RSC:2337223.2337323,
	author = {McMillan, Collin and Hariri, Negar and Poshyvanyk, Denys and Cleland-Huang, Jane and Mobasher, Bamshad},
	title = {Recommending source code for use in rapid software prototypes},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {848--858},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337323},
	acmid = {2337323},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@inproceedings{McMillan:2012:DSS:2337223.2337267,
	author = {McMillan, Collin and Grechanik, Mark and Poshyvanyk, Denys},
	title = {Detecting similar software applications},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {364--374},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337267},
	acmid = {2337267},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@INPROCEEDINGS{McMillan:5069582,
	author={McMillan, C. and Poshyvanyk, D. and Revelle, M.},
	booktitle={Traceability in Emerging Forms of Software Engineering, 2009. TEFSE '09. ICSE Workshop on},
	title={Combining textual and structural analysis of software artifacts for traceability link recovery},
	year={2009},
	month={may},
	volume={},
	number={},
	pages={41 -48},
	keywords={requirements documentation;software documentation artifacts;source code elements;structural analysis;textual analysis;traceability link recovery;information retrieval;software engineering;system documentation;},
	doi={10.1109/TEFSE.2009.5069582},
	ISSN={}
}

@inproceedings{Shepherd:2007:UNL:1218563.1218587,
	author = {Shepherd, David and Fry, Zachary P. and Hill, Emily and Pollock, Lori and Vijay-Shanker, K.},
	title = {Using natural language program analysis to locate and understand action-oriented concerns},
	booktitle = {Proceedings of the 6th international conference on Aspect-oriented software development},
	series = {AOSD '07},
	year = {2007},
	isbn = {1-59593-615-7},
	location = {Vancouver, British Columbia, Canada},
	pages = {212--224},
	numpages = {13},
	url = {http://doi.acm.org/10.1145/1218563.1218587},
	doi = {10.1145/1218563.1218587},
	acmid = {1218587},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {feature location, program analysis, remodularization, reverse engineering},
}

@inproceedings{Hill:2011:IEC:1985429.1985439,
	author = {Hill, Emily and Pollock, Lori and Vijay-Shanker, K.},
	title = {Investigating how to effectively combine static concern location techniques},
	booktitle = {Proceedings of the 3rd International Workshop on Search-Driven Development: Users, Infrastructure, Tools, and Evaluation},
	series = {SUITE '11},
	year = {2011},
	isbn = {978-1-4503-0597-6},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {37--40},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1985429.1985439},
	doi = {10.1145/1985429.1985439},
	acmid = {1985439},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {concern location, software maintenance, source code exploration, source code search},
} 

@inproceedings{Bettenburg:2010:SIS:1846454.1847957,
	author = {Bettenburg, Nicolas and Hassan, Ahmed E.},
	title = {Studying the Impact of Social Structures on Software Quality},
	booktitle = {Proceedings of the 2010 IEEE 18th International Conference on Program Comprehension},
	series = {ICPC '10},
	year = {2010},
	isbn = {978-0-7695-4113-6},
	pages = {124--133},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICPC.2010.46},
	doi = {10.1109/ICPC.2010.46},
	acmid = {1847957},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {Human Factors, Software Evolution, Metrics/Measurement, Software Quality Assurance},
} 

@inproceedings{Bettenburg:2011:MDR:2025113.2025165,
	author = {Bettenburg, Nicolas},
	title = {Mining development repositories to study the impact of collaboration on software systems},
	booktitle = {Proceedings of the 19th ACM SIGSOFT symposium and the 13th European conference on Foundations of software engineering},
	series = {ESEC/FSE '11},
	year = {2011},
	isbn = {978-1-4503-0443-6},
	location = {Szeged, Hungary},
	pages = {376--379},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/2025113.2025165},
	doi = {10.1145/2025113.2025165},
	acmid = {2025165},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {collaboration, empirical studies, socio-technical congruence, software repositories, unstructured data},
}

@article {M:Harrold:STVR:2000,
	author = {Harrold, Mary Jean and Rothermel, Gregg and Sayre, Kent and Wu, Rui
	and Yi, Liu},
	title = {An empirical investigation of the relationship between spectra
	differences and regression faults},
	journal = {Software Testing, Verification and Reliability},
	volume = {10},
	number = {3},
	publisher = {John Wiley & Sons, Ltd.},
	year = {2000}
}

@inproceedings{T:Reps:ESEC:1997,
	author = {Reps, Thomas and Ball, Thomas and Das, Manuvir and Larus, James},
	title = {The use of program profiling for software maintenance with
	applications to the year 2000 problem},
	booktitle = {Proceedings of the 6th European SOFTWARE ENGINEERING conference
	held jointly with the 5th ACM SIGSOFT international symposium on Foundations of
	software engineering},
	series = {ESEC '97/FSE-5},
	year = {1997},
	pages = {432--449}
} 

@inproceedings{M:Renierses:ASE:2003,
	author={Renieres, M. and Reiss, S.P.},
	booktitle={Automated Software Engineering, 2003. Proceedings. 18th IEEE
	International Conference on}, 
	title={Fault localization with nearest neighbor
	queries},
	year={2003},
	pages={ 30 - 39}
}

@inproceedings{Santelices:2009:LFU:1555001.1555021,
	author = {Santelices, Raul and Jones, James A. and Yanbing Yu and Harrold, Mary Jean},
	title = {Lightweight fault-localization using multiple coverage types},
	booktitle = {Proceedings of the 31st International Conference on Software Engineering},
	series = {ICSE '09},
	year = {2009},
	isbn = {978-1-4244-3453-4},
	pages = {56--66},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2009.5070508},
	doi = {10.1109/ICSE.2009.5070508},
	acmid = {1555021},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@article{Ficco:2011:BLT:1992516.2043292,
	author = {Ficco, Massimo and Pietrantuono, Roberto and Russo, Stefano},
	title = {Bug localization in test-driven development},
	journal = {Adv. Soft. Eng.},
	issue_date = {January 2011},
	volume = {2011},
	month = jan,
	year = {2011},
	issn = {1687-8655},
	pages = {2:1--2:18},
	articleno = {2},
	numpages = {18},
	url = {http://dx.doi.org/10.1155/2011/492757},
	doi = {10.1155/2011/492757},
	acmid = {2043292},
	publisher = {Hindawi Publishing Corp.},
	address = {New York, NY, United States},
} 

@article{Ball:2003:SCL:640128.604140,
	author = {Ball, Thomas and Naik, Mayur and Rajamani, Sriram K.},
	title = {From symptom to cause: localizing errors in counterexample traces},
	journal = {SIGPLAN Not.},
	issue_date = {January 2003},
	volume = {38},
	number = {1},
	month = jan,
	year = {2003},
	issn = {0362-1340},
	pages = {97--105},
	numpages = {9},
	url = {http://doi.acm.org/10.1145/640128.604140},
	doi = {10.1145/640128.604140},
	acmid = {604140},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, software model checking},
}

@inproceedings{Park:2010:FFL:1806799.1806838,
	author = {Park, Sangmin and Vuduc, Richard W. and Harrold, Mary Jean},
	title = {Falcon: fault localization in concurrent programs},
	booktitle = {Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering - Volume 1},
	series = {ICSE '10},
	year = {2010},
	isbn = {978-1-60558-719-6},
	location = {Cape Town, South Africa},
	pages = {245--254},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1806799.1806838},
	doi = {10.1145/1806799.1806838},
	acmid = {1806838},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {atomicity violation, concurrency, debugging, fault localization, order violation},
} 

@inproceedings{Yilmaz:2008:TTF:1368088.1368100,
	author = {Yilmaz, Cemal and Paradkar, Amit and Williams, Clay},
	title = {Time will tell: fault localization using time spectra},
	booktitle = {Proceedings of the 30th international conference on Software engineering},
	series = {ICSE '08},
	year = {2008},
	isbn = {978-1-60558-079-1},
	location = {Leipzig, Germany},
	pages = {81--90},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1368088.1368100},
	doi = {10.1145/1368088.1368100},
	acmid = {1368100},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {automated debugging, fault localization},
}

@inproceedings{Hangal:2002:TDS:581339.581377,
	author = {Hangal, Sudheendra and Lam, Monica S.},
	title = {Tracking down software bugs using automatic anomaly detection},
	booktitle = {Proceedings of the 24th International Conference on Software Engineering},
	series = {ICSE '02},
	year = {2002},
	isbn = {1-58113-472-X},
	location = {Orlando, Florida},
	pages = {291--301},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/581339.581377},
	doi = {10.1145/581339.581377},
	acmid = {581377},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Bhat:2006:EET:1159733.1159787,
	author = {Bhat, Thirumalesh and Nagappan, Nachiappan},
	title = {Evaluating the efficacy of test-driven development: industrial case studies},
	booktitle = {Proceedings of the 2006 ACM/IEEE international symposium on Empirical software engineering},
	series = {ISESE '06},
	year = {2006},
	isbn = {1-59593-218-6},
	location = {Rio de Janeiro, Brazil},
	pages = {356--363},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1159733.1159787},
	doi = {10.1145/1159733.1159787},
	acmid = {1159787},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {software quality, test-driven development},
}

@inproceedings{Chilimbi:2009:HES:1555001.1555020,
	author = {Chilimbi, Trishul M. and Liblit, Ben and Mehra, Krishna and Nori, Aditya V. and Vaswani, Kapil},
	title = {HOLMES: Effective statistical debugging via efficient path profiling},
	booktitle = {Proceedings of the 31st International Conference on Software Engineering},
	series = {ICSE '09},
	year = {2009},
	isbn = {978-1-4244-3453-4},
	pages = {34--44},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2009.5070506},
	doi = {10.1109/ICSE.2009.5070506},
	acmid = {1555020},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{10.1109/ICECCS.2005.25,
	author = {Leonardo Mariani and Mauro Pezza},
	title = {Behavior Capture and Test: Automated Analysis of Component Integration},
	journal ={Engineering of Complex Computer Systems, IEEE International Conference on},
	volume = {0},
	isbn = {0-7695-2284-X},
	year = {2005},
	pages = {292-301},
	doi = {http://doi.ieeecomputersociety.org/10.1109/ICECCS.2005.25},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{Lorenzoli:2008:AGS:1368088.1368157,
	author = {Lorenzoli, Davide and Mariani, Leonardo and Pezz\`{e}, Mauro},
	title = {Automatic generation of software behavioral models},
	booktitle = {Proceedings of the 30th international conference on Software engineering},
	series = {ICSE '08},
	year = {2008},
	isbn = {978-1-60558-079-1},
	location = {Leipzig, Germany},
	pages = {501--510},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1368088.1368157},
	doi = {10.1145/1368088.1368157},
	acmid = {1368157},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {dynamic analysis, gk-tail, model synthesis},
} 

@inproceedings{Cleve:2005:LCP:1062455.1062522,
	author = {Cleve, Holger and Zeller, Andreas},
	title = {Locating causes of program failures},
	booktitle = {Proceedings of the 27th international conference on Software engineering},
	series = {ICSE '05},
	year = {2005},
	isbn = {1-58113-963-2},
	location = {St. Louis, MO, USA},
	pages = {342--351},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1062455.1062522},
	doi = {10.1145/1062455.1062522},
	acmid = {1062522},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {adaptive testing, automated debugging, program analysis, tracing},
} 

@inproceedings{J:Jones:ASE:2005,
	author = {Jones, James A. and Harrold, Mary Jean},
	title = {Empirical evaluation of the tarantula automatic fault-localization
	technique},
	booktitle = {Proceedings of the 20th IEEE/ACM international Conference on
	Automated software engineering},
	year = {2005},
	pages = {273--282},
	numpages = {10}
}

@inproceedings{J:Jone:ICSE:2002,
	author = {Jones, James A. and Harrold, Mary Jean and Stasko, John},
	title = {Visualization of test information to assist fault localization},
	booktitle = {Proceedings of the 24th International Conference on Software
	Engineering},
	series = {ICSE '02},
	year = {2002},
	pages = {467--477},
	numpages = {11}
} 

@techreport{H:Pan:1992,
	title={Heuristics for automatic localization of software faults},
	author={Pan, H. and Spafford, E.H.},
	journal={World Wide Web},
	year={1992}
}

@inproceedings{H:Agrawal:ISSRE:1995,
	author={Agrawal, H. and Horgan, J.R. and London, S. and Wong, W.E.},
	booktitle={Software Reliability Engineering, 1995. Proceedings., Sixth
	International Symposium on}, title={Fault localization using execution slices
	and dataflow tests},
	year={1995},
	pages={143 -151}}

@inproceedings{T:Gyimothy:ESEC:1999,
	author = {Gyim\'{o}thy, Tibor and Besz{\'e}des, \'{A}rp\'{a}d and Forg\'{a}cs,
	Ist\'{a}n},
	title = {An efficient relevant slicing method for debugging},
	booktitle = {Proceedings of the 7th European software engineering conference
	held jointly with the 7th ACM SIGSOFT international symposium on Foundations of
	software engineering},
	series = {ESEC/FSE-7},
	year = {1999},
	pages = {303--321}
} 

@inproceedings{F:Servant:ICSE:2012,
	author = {Servant, Francisco and Jones, James A.},
	title = {WhoseFault: automatic developer-to-fault assignment through fault localization},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	pages = {36--46}
} 

@inproceedings{A:Mockus:ICSE:2002,
	author = {Mockus, Audris and Herbsleb, James D.},
	title = {Expertise browser: a quantitative approach to identifying expertise},
	booktitle = {Proceedings of the 24th International Conference on Software Engineering},
	series = {ICSE '02},
	year = {2002},
	pages = {503--512}
} 

@inproceedings{S:Minto:MSR:2007,
	author = {Minto, Shawn and Murphy, Gail C.},
	title = {Recommending Emergent Teams},
	booktitle = {Proceedings of the Fourth International Workshop on Mining Software Repositories},
	series = {MSR '07},
	year = {2007},
	pages = {5--}
} 

@inproceedings{D:Ma:ICSM:2009,
	author = {David Ma and David Schuler and Thomas Zimmermann and Jonathan Sillito},
	title = {Expert recommendation with usage expertise},
	journal ={Software Maintenance, IEEE International Conference on},
	volume = {0},
	isbn = {978-1-4244-4897-5},
	year = {2009},
	pages = {535-538},
	doi = {http://doi.ieeecomputersociety.org/10.1109/ICSM.2009.5306386},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{G:Jeong:ESEC:2009,
	author = {Jeong, Gaeul and Kim, Sunghun and Zimmermann, Thomas},
	title = {Improving bug triage with bug tossing graphs},
	booktitle = {Proceedings of the the 7th joint meeting of the European software engineering conference and the ACM SIGSOFT symposium on The foundations of software engineering},
	series = {ESEC/FSE '09},
	year = {2009},
	pages = {111--120},
	numpages = {10}
} 

@inproceedings{J:Anvik:ICSE:2006,
	author = {Anvik, John and Hiew, Lyndon and Murphy, Gail C.},
	title = {Who should fix this bug?},
	booktitle = {Proceedings of the 28th international conference on Software engineering},
	series = {ICSE '06},
	year = {2006},
	isbn = {1-59593-375-1},
	location = {Shanghai, China},
	pages = {361--370},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1134285.1134336},
	doi = {10.1145/1134285.1134336},
	acmid = {1134336},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug report assignment, bug triage, issue tracking, machine learning, problem tracking},
} 

@inproceedings{Abadi:A:ICPC:08,
	Author={Abadi, A. and Nisenson, M. and Simionovici, Y. },
	Title = {A Traceability Technique for Specifications},
	BookTitle = {16th IEEE International Conference on Program Comprehension (ICPC'08)},
	Address= {Amsterdam, The Netherlands},
	Pages = {103-112},
	Year = {2008} }

@inproceedings{finkel2005incorporating,
	title={Incorporating non-local information into information extraction systems by gibbs sampling},
	author={Finkel, Jenny Rose and Grenager, Trond and Manning, Christopher},
	booktitle={Proceedings of the 43rd Annual Meeting on Association for Computational Linguistics},
	pages={363--370},
	year={2005},
	organization={Association for Computational Linguistics}
}

@article{cowie1996information,
	title={Information extraction},
	author={Cowie, Jim and Lehnert, Wendy},
	journal={Communications of the ACM},
	volume={39},
	number={1},
	pages={80--91},
	year={1996},
	publisher={ACM}
}

@inproceedings{guarino1998formal,
	title={Formal ontology and information systems},
	author={Guarino, Nicola},
	booktitle={Proceedings of FOIS},
	volume={98},
	number={1998},
	pages={81--97},
	year={1998}
}

@book{buitelaar2005ontology,
	title={Ontology learning from text: methods, evaluation and applications},
	author={Buitelaar, Paul and Cimiano, Philipp and Magnini, Bernardo},
	volume={123},
	year={2005},
	publisher={IOS press}
}

@article{chen1990c,
	title={The C information abstraction system},
	author={Chen, Yih-Farn and Nishimoto, Michael Y. and Ramamoorthy, CV},
	journal={IEEE Transactions on software Engineering},
	volume={16},
	number={3},
	pages={325},
	year={1990},
	publisher={IEEE Computer Society}
}

@book{jones1997readings,
	title={Readings in information retrieval},
	author={Jones, Karen Sparck},
	year={1997},
	publisher={Morgan Kaufmann}
}

@article{lucia2007recovering,
	title={Recovering traceability links in software artifact management systems using information retrieval methods},
	author={Lucia, Andrea De and Fasano, Fausto and Oliveto, Rocco and Tortora, Genoveffa},
	journal={ACM Transactions on Software Engineering and Methodology (TOSEM)},
	volume={16},
	number={4},
	pages={13},
	year={2007},
	publisher={ACM}
}

@inproceedings{hayes2003improving,
	title={Improving requirements tracing via information retrieval},
	author={Hayes, Jane Huffman and Dekhtyar, Alex and Osborne, James},
	booktitle={Requirements Engineering Conference, 2003. Proceedings. 11th IEEE International},
	pages={138--147},
	year={2003},
	organization={IEEE}
}

@article{Wood:1988:IRS:54347.54349,
	author = {Wood, M. and Sommerville, I.},
	title = {An Information Retrieval System for Software Components},
	journal = {SIGIR Forum},
	issue_date = {Spring/Summer 1988},
	volume = {22},
	number = {3-4},
	month = may,
	year = {1988},
	issn = {0163-5840},
	pages = {11--28},
	numpages = {18},
	url = {http://doi.acm.org/10.1145/54347.54349},
	doi = {10.1145/54347.54349},
	acmid = {54349},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Abebe:S:CSMR:2009,
	Author = {Abebe, S. L. and Haiduc, S. and Marcus, A. and Tonella, P. and Antoniol, G.},
	Title = {Analyzing the Evolution of the Source Code Vocabulary},
	BookTitle = {13th IEEE European Conference on Software Maintenance and Reengineering (CSMR'09)},
	Address= {Kaiserslautern, Germany},
	Pages = {189-198},
	Year = {2009} }

@inproceedings{Antoniol:G:CSMR:2000,
	Author = {Antoniol, G. and Canfora, G. and Casazza, G. and De Lucia, A.},
	Title = {Identifying the Starting Impact  Set of a Maintenance and Reengineering},
	BookTitle = {4th European Conference on Software Maintenance (CSMR2000)},
	Address= {Zurich, Switzerland},
	Publisher = {CS Press},
	Pages = {227-230},
	Year = {2000} }

@inproceedings{Antoniol:G:ICSM:2000,
	Author = {Antoniol, Giuliano and Canfora, Gerardo and Casazza, Gerardo and De Lucia, Andrea},
	Title = {Information Retrieval Models for Recovering Traceability Links between Code and Documentation},
	BookTitle = {IEEE International Conference on Software Maintenance (ICSM'00)},
	Address= {San Jose, CA},
	Publisher = {IEEE COmputer Society},
	Pages = {40-51},
	Year = {2000} }

@article{Antoniol:G:TSE:2002,
	Author = {Antoniol, Giuliano and Canfora, Gerardo and Casazza, Gerardo and De Lucia, Andrea and Merlo, Ettore},
	Title = {Recovering Traceability Links between Code and Documentation},
	Journal = {IEEE Transactions on Software Engineering},
	Volume = {28},
	Number = {10},
	Pages = {970 - 983},
	Year = {2002} }

@article{Antoniol:G:TSE:2006,
	Author = {Antoniol, G. and Guéhéneuc, Y.G.},
	Title = {Feature Identification: An Epidemiological Metaphor},
	Journal = {IEEE Transactions on Software Engineering},
	Volume = {32},
	Number = {9},
	Pages = {627-641},
	Year = {2006} }

@inproceedings{Antoniol:G:ICSM:2008,
	Author = {Antoniol, G. and Hayes, J. H. and Gueheneuc, Y.. and Di Penta, M. },
	Title = {Reuse or rewrite: Combining textual, static, and dynamic analyses to assess the cost of keeping a system up-to-date},
	BookTitle = {IEEE International Conference on Software Maintenance (ICSM'08)},
	Pages = {147-156},
	Year = {2008} }

@inproceedings{Asuncion:H:ICSE:2010,
	Author = {Asuncion, H.  and Asuncion, A.  and Taylor, R.},
	Title = {Software Traceability with Topic Modeling},
	BookTitle = {32nd International Conference on Software Engineering (ICSE'10)},
	Year = {2010} }

@inproceedings{Baldi:P:OOPSLA:2008,
	Author = {Baldi, P. and Linstead, E. and Lopes, C. and Bajracharya, S.},
	Title = {A Theory of Aspects as Latent Topics},
	BookTitle = {ACM SIGPLAN Conference on Object-Oriented Programming, Systems, Languages and Applications (OOPSLA'08)},
	Address= {Nashville, Tennessee},
	Pages = {543-562},
	Year = {2008} }

@article{Binkley:D:JSS:2008,
	Author = {Binkley, D. and Gold, G. and Harman, M. and Li, Z. and Mahdavi, K.},
	Title = {An empirical study of the relationship between the concepts expressed in source code and dependence},
	Journal = {The Journal of Systems and Software},
	Volume = {81},
	Pages = {2287–2298},
	Year = {2008} }

@misc{Binkley:D:2009,
	Author = {Binkley, D. and Lawrie, D.},
	Title = {Information Retrieval Applications in Software Maintenance and Evolution},
	Publisher = {Taylor & Francis LLC},
	Year = {2009} }

@book{zelkowitz1979principles,
	title={Principles of software engineering and design},
	author={Zelkowitz, Marvin V and Shaw, Alan C and Gannon, John D},
	year={1979},
	publisher={Prentice-Hall Englewood Cliffs}
}

@article{schmidt2006model,
	title={Model-driven engineering},
	author={Schmidt, Douglas C},
	journal={COMPUTER-IEEE COMPUTER SOCIETY-},
	volume={39},
	number={2},
	pages={25},
	year={2006},
	publisher={Citeseer}
}

@inproceedings{kieburtz1996software,
	title={A software engineering experiment in software component generation},
	author={Kieburtz, Richard B and McKinney, Laura and Bell, Jeffrey M and Hook, James and Kotov, Alex and Lewis, Jeffrey and Oliva, Dino P and Sheard, Tim and Smith, Ira and Walton, Lisa},
	booktitle={Proceedings of the 18th international conference on Software engineering},
	pages={542--552},
	year={1996},
	organization={IEEE Computer Society}
}

@inproceedings{nickel2000fujaba,
	title={The FUJABA environment},
	author={Nickel, Ulrich and Niere, J{\"o}rg and Z{\"u}ndorf, Albert},
	booktitle={Proceedings of the 22nd international conference on Software engineering},
	pages={742--745},
	year={2000},
	organization={ACM}
}

@article{Boyd:N:JOOP:1999,
	Author = {Boyd, N.},
	Title = {Using Natural Language in Software Development},
	Journal = {Journal of Object-Oriented Programming},
	Volume = {11},
	Number = {9},
	Pages = {45-55},
	Year = {1999} }

@inproceedings{Capobianco:G:ICPC:2009,
	Author = {Capobianco, Giovanni and De Lucia, Andrea and Oliveto, Rocco and Panichella, Annibale and Panichella, Sebastiano},
	Title = {On the role of the nouns in IR-based traceability recovery},
	BookTitle = {17th IEEE International Conference on Program Comprehension (ICPC'09)},
	Address= {Vancouver, British Columbia, Canada},
	Pages = {148 - 157},
	Year = {2009} }

@inproceedings{Caprile:B:ICSM:2000,
	Author = {Caprile, B. and Tonella, P.},
	Title = {Restructuring Program Identifier Names},
	BookTitle = {16th IEEE Internation Conference on Software Maintenance (ICSM'00)},
	Address= {San Jose, California, USA},
	Pages = {97-107},
	Year = {2000} }

@article{Cleary:B:EMSE:2009,
	Author = {Cleary, B. and Exton, C. and Buckley, J. and English, M.},
	Title = {An empirical analysis of information retrieval based concept location techniques in software comprehension},
	Journal = {Empirical Software Engineering},
	Volume = {14},
	Number = {1},
	Pages = {93-130},
	Year = {2009} }

@article{DeLucia:A:TSE:2011,
	Author = {De Lucia, A. and Di Penta, M. and Oliveto, R.},
	Title = {Improving Source Code Lexicon via Traceability and Information Retrieval},
	Journal = {IEEE Transactions on Software Engineering},
	volume = {37},
	number = {2},
	year = {2011},
	pages = {205--227} }

@article{DeLucia:A:TOSEM:2007,
	Author = {De Lucia, A. and Fasano, F. and Oliveto, R. and Tortora, G.},
	Title = {Recovering Traceability Links in Software Artefact Management Systems},
	Journal = {ACM Transactions on Software Engineering and Methodology},
	Volume = {16},
	Number = {4},
	Year = {2007} }

@inproceedings{DeLucia:A:ICSM:2009,
	Author = {De Lucia, Andrea and Oliveto, Rocco and Tortora, Genoveffa},
	Title = {The role of the coverage analysis during IR-based traceability recovery: A controlled experiment},
	BookTitle = {25th IEEE International Conference on Software Maintenance (ICSM'09)},
	Address= {Edmonton, Alberta, Canada},
	Pages = {371-380},
	Year = {2009} }

@inproceedings{Dit:B:ICPC:2011,
	Author = {Dit, Bogdan and Guerrouj, Latifa  and Poshyvanyk, Denys and Antoniol, Giulio},
	Title = {Can Better Identifier Splitting Techniques Help Feature Location?},
	BookTitle = {19th IEEE International Conference on Program Comprehension (ICPC'11)},
	Address= {Kingston, Ontario},
	Pages = {11-20},
	Year = {2011} }

@inproceedings{Haiduc:S:ICPC:2008,
	Author = {Haiduc, S. and Marcus, A.},
	Title = {On the Use of Domain Terms in Source Code},
	BookTitle = {16th IEEE International Conference on Program Comprehension (ICPC'08)},
	Address= {Amsterdam, The Netherlands},
	Pages = {113-122},
	Year = {2008} }

@inproceedings{Helm:R:OOPSLA:1991,
	Author = {Helm, Richard  	  and Maarek, Yoelle S.  	 },
	Title = {Integrating information retrieval and domain specific approaches for browsing and retrieval in object-oriented class libraries},
	BookTitle = {Conference proceedings on Object-oriented programming systems, languages, and applications},
	Address= {Phoenix, Arizona, United States},
	Publisher = {ACM Press   New York, NY, USA},
	Pages = {47-61},
	Year = {1991} }

@inproceedings{Hindle:A:ICSM:2009,
	Author = {Hindle, A. J. and Godfrey, M. W. and Holt, R. C.},
	Title = {What’s Hot and What’s Not: Windowing Developer Topic Analysis},
	BookTitle = {IEEE International Conference on Software Maintenance (ICSM'09)},
	Address= {Edmonton, Alberta},
	Year = {2009} }

@article{Kagdi:H:JSME:2011,
	Author = {Kagdi, H. and Gethers, M. and Poshyvanyk, D. and Hammad, M.},
	Title = {Assigning Change Requests to Software Developers},
	Journal = {Journal of Software Maintenance and Evolution: Research and Practice (JSME)},
	Year = {2011} }

@inproceedings{Lawrie:D:ICPC:2006,
	Author = {Lawrie, D. and Morrell, C. and Feild, H. and Binkley, D.},
	Title = {What's in a Name? A Study of Identifiers},
	BookTitle = {14th IEEE International Conference on Program Comprehension (ICPC'06)},
	Address= {Athens, Greece},
	Pages = {3-12},
	Year = {2006} }

@inproceedings{Lo:K:OOPSLA:2006,
	Author = {Lo, K. K.  and Chan, M. K.  and Baniassad, E. },
	Title = {Isolating and Relating Concerns in Requirements using Latent Semantic Analysis},
	BookTitle = {ACM SIGPLAN International Conference on Object-Oriented Programming, Systems, Languages and Applications (OOPSLA'06)},
	Pages = {383 - 396 },
	Year = {2006} }

@article{Lukings:S:IST:2010,
	Author = {Lukins, S. K. and Kraft, N. A. and Etzkorn, L. H.},
	Title = {Bug localization using Latent Dirichlet Allocation},
	Journal = {Information and Software Technology},
	Volume = {52},
	Number = {9},
	Pages = {972-990},
	Year = {2010} }

@article{Maarek:Y:TSE:1991,
	Author = {Maarek, Y. S. and Berry, D. M. and Kaiser, G. E.},
	Title = {An Information Retrieval Approach for Automatically Constructing Software Libraries},
	Journal = {IEEE Transactions on Software Engineering},
	Volume = {17},
	Number = {8},
	Pages = {800-813},
	Year = {1991} }

@inproceedings{Maletic:J:ASE:1999,
	Author = {Maletic, Jonathan I. and Valluri, N.},
	Title = {Automatic Software Clustering via Latent Semantic Analysis},
	BookTitle = {14th IEEE International Conference on Automated Software Engineering (ASE'99)},
	Address= {Cocoa Beach Florida},
	Pages = {251-254},
	Note  = {hard copy - .pdf},
	Year = {1999} }

@inproceedings{Marcus:A:ICSE:2003,
	Author = {Marcus, Andrian and Maletic, Jonathan I.},
	Title = {Recovering Documentation-to-Source-Code Traceability Links using Latent Semantic Indexing},
	BookTitle = {25th IEEE/ACM International Conference on Software Engineering (ICSE'03)},
	Address= {Portland, OR},
	Pages = {125-137},
	Keywords = {reverse_engineering
	traceability},
	Year = {2003} }

@inproceedings{Marcus:A:ICSM:2005,
	Author = {Marcus, Andrian and Poshyvanyk, Denys},
	Title = {The Conceptual Cohesion of Classes},
	BookTitle = {21st IEEE International Conference on Software Maintenance (ICSM'05)},
	Address= {Budapest, Hungary},
	Pages = {133-142},
	Year = {2005} }

@article{Marcus:A:TSE:2008,
	Author = {Marcus, A. and Poshyvanyk, D. and Ferenc, R.},
	Title = {Using the Conceptual Cohesion of Classes for Fault Prediction in Object Oriented Systems},
	Journal = {IEEE Transactions on Software Engineering},
	Volume = {34},
	Number = {2},
	Pages = {287-300},
	Year = {2008} }

@article{Yadla:Hayes:NASE:2005,
	Author = {Yadla, S. and Hayes, J. and Dekhtyar, A.},
	Title = {Tracing Requirements to Defect Reports:  An Application of Information Retrieval Techniques},
	Journal = {Innovations in Systems and Software Engineering:  A NASA Journal},
	Volume = {1},
	Number = {2},
	Pages = {116-124},
	Year = {2005}
}

@article{Poshyvanyk:D:TOSEM:2012,
	Author = {Poshyvanyk, D. and Gethers, M. and Marcus, A.},
	Title = {Concept Location using Formal Concept Analysis and Information Retrieval},
	Journal = {ACM Transactions on Software Engineering and Methodology},
	Year = {2012} }

@article{Poshyvanyk:D:TSE:07,
	Author = {Poshyvanyk, D. and Guéhéneuc, Y.G. and Marcus, A. and Antoniol, G. and Rajlich, V.},
	Title = {Feature Location using Probabilistic Ranking of Methods based on Execution Scenarios and Information Retrieval},
	Journal = {IEEE Transactions on Software Engineering},
	Volume = {33},
	Number = {6},
	Pages = {420-432},
	Year = {2007} }

@article{Poshyvanyk:D:EMSE:2009,
	Author = {Poshyvanyk, D. and Marcus, A. and Ferenc, R. and Gyimóthy, T.},
	Title = {Using Information Retrieval based Coupling Measures for Impact Analysis},
	Journal = {Empirical Software Engineering},
	Volume = {14},
	Number = {1},
	Pages = {5-32},
	Year = {2009} }

@article{Blei:D:JMLR:2003,
	Author = {Blei, D. M. and Ng, A. Y. and Jordan, M. I.},
	Title = {Latent Dirichlet Allocation},
	Journal = {Journal of Machine Learning Research},
	Volume = {3},
	Pages = {993-1022},
	Year = {2003} }

@book{Salton:G:1986,
	Author = {Salton, G. and McGill, M.},
	Title = {Introduction to Modern Information Retrieval},
	Publisher = {McGraw-Hill},
	Year = {1986} }

@book{Baeza-Yates:R:1999,
	Author = {Baeza-Yates, Ricardo A. and Ribeiro-Neto, Berthier},
	Title = {Modern Information Retrieval},
	Publisher = {Addison-Wesley},
	Year = {1999} }

@article{Deerwester:S:JASIS:1990,
	Author = {Deerwester, Scott and Dumais, Susan T. and Furnas, G. W. and Landauer, Thomas K. and Harshman, R.},
	Title = {Indexing by Latent Semantic Analysis},
	Journal = {Journal of the American Society for Information Science},
	Volume = {41},
	Pages = {391-407},
	Year = {1990} }

@inproceedings{Gethers:M:ASE:2011,
	Author = {Gethers, M. and Kagdi, H. and Dit, B. and Poshyvanyk, D.},
	Title = {An Adaptive Approach to Impact Analysis from Change Requests to Source Code},
	BookTitle = {26th IEEE/ACM International Conference on Automated Software Engineering (ASE'11)},
	Address= {Lawrence, Kansas},
	Year = {2011} }

@inproceedings{Gethers:M:ICSM:2011,
	Author = {Gethers, M. and Oliveto, R. and Poshyvanyk, D. and De Lucia, A.},
	Title = {On Integrating Orthogonal Information Retrieval Methods to Improve Traceability Link Recovery},
	BookTitle = {27th IEEE International Conference on Software Maintenance (ICSM'11)},
	Address= {Williamsburg, Virginia, USA},
	Pages = {to appear},
	Year = {2011} }

@inproceedings{Gethers:M:ICSM:2010,
	Author = {Gethers, M.  and Poshyvanyk, D.},
	Title = {Using Relational Topic Models to Capture Coupling among Classes in Object-Oriented Software Systems},
	BookTitle = {26th IEEE International Conference on Software Maintenance (ICSM'10)},
	Address= {Timişoara, Romania},
	Pages = {1-10},
	Year = {2010} }

@inproceedings{Gethers:M:ICSE-T:2011,
	Author = {Gethers, M. and Savage, T. and Di Penta, M. and Oliveto, R. and Poshyvanyk, D. and De Lucia, A.},
	Title = {CodeTopics: Which Topic Am I Coding Now?},
	BookTitle = {33rd IEEE/ACM International Conference on Software Engineering (ICSE'11), Formal Research Tool Demonstration},
	Address= {Honolulu, Hawaii, USA},
	Pages = {1034-1036},
	Year = {2011} }

@inproceedings{Oliveto:R:ICSE-NIER:2011,
	Author = {Oliveto, R. and Gethers, M. and Bavota, G. and Poshyvanyk, D. and De Lucia, A.},
	Title = {Identifying Method Friendships to Remove the Feature Envy Bad Smell},
	BookTitle = {33rd IEEE/ACM International Conference on Software Engineering (ICSE'11)},
	Address= {Honolulu, Hawaii, USA},
	Pages = {820-823},
	Year = {2011} }

@article{Lukins:2010:BLU:1824820.1824850,
	author = {Lukins, Stacy K. and Kraft, Nicholas A. and Etzkorn, Letha H.},
	title = {Bug localization using latent Dirichlet allocation},
	journal = {Inf. Softw. Technol.},
	issue_date = {September, 2010},
	volume = {52},
	number = {9},
	month = sep,
	year = {2010},
	issn = {0950-5849},
	pages = {972--990},
	numpages = {19},
	url = {http://dx.doi.org/10.1016/j.infsof.2010.04.002},
	doi = {10.1016/j.infsof.2010.04.002},
	acmid = {1824850},
	publisher = {Butterworth-Heinemann},
	address = {Newton, MA, USA},
	keywords = {Bug localization, Information retrieval, Latent Dirichlet allocation, Program comprehension},
}

@inproceedings{Linares-Vasquez:M:ICSM:2012,
	Author = {Linares-Vasquez, M. and Dang, H. and Hossen, K. and Kagdi, H. and Gethers, M. and Poshyvanyk, D.},
	Title = {Triaging Incoming Change Requests: Bug or Commit History, or Code Authorship?},
	BookTitle = {28th IEEE International Conference on Software Maintenance (ICSM'12)},
	Address = {Riva del Garda, Italy},
	Year = {2012} }

@inproceedings{Oliveto:R:ICPC:2010,
	Author = {Oliveto, R. and Gethers, M. and Poshyvanyk, D. and De Lucia, A.},
	Title = {On the Equivalence of Information Retrieval Methods for Automated Traceability Link Recovery},
	BookTitle = {18th IEEE International Conference on Program Comprehension (ICPC'10)},
	Address= {Braga, Portugal},
	Pages = {68-71},
	Year = {2010} }

@inproceedings{Klock:S:TEFSE:2011,
	Author = {Klock, S. and Gethers, M. and Dit, B. and Poshyvanyk, D.},
	Title = {Traceclipse: An Eclipse Plug-in for Traceability Link Recovery and Management},
	BookTitle = {6th International Workshop on Traceability in Emerging Forms of Software Engineering (TEFSE'11)},
	Address= {Honolulu, Hawaii, HI},
	Year = {2011} }


@article{Dit:B:JSME:2011,
	Author = {Dit, B. and Revelle, M. and Gethers, M. and Poshyvanyk, D.},
	Title = {Feature Location in Source Code: A Taxonomy and Survey},
	Journal = {Journal of Software Maintenance and Evolution: Research and Practice},
	Year = {2011} }

@inproceedings{Gethers:2012:IIA:2337223.2337274,
	author = {Gethers, Malcom and Dit, Bogdan and Kagdi, Huzefa and Poshyvanyk, Denys},
	title = {Integrated impact analysis for managing software changes},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {430--440},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337274},
	acmid = {2337274},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA}
}

@inproceedings{Dickinson:2001:FFC:381473.381509,
	author = {Dickinson, William and Leon, David and Podgurski, Andy},
	title = {Finding failures by cluster analysis of execution profiles},
	booktitle = {Proceedings of the 23rd International Conference on Software Engineering},
	series = {ICSE '01},
	year = {2001},
	isbn = {0-7695-1050-7},
	location = {Toronto, Ontario, Canada},
	pages = {339--348},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=381473.381509},
	acmid = {381509},
	publisher = {IEEE Computer Society}
} 


@inproceedings{McDonald:D:CSCW:2000,
	author = {McDonald, David W. and Ackerman, Mark S.},
	title = {Expertise recommender: a flexible recommendation system and architecture},
	booktitle = {Proceedings of the 2000 ACM conference on Computer supported cooperative work},
	series = {CSCW '00},
	year = {2000},
	isbn = {1-58113-222-0},
	location = {Philadelphia, Pennsylvania, United States},
	pages = {231--240},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/358916.358994},
	doi = {10.1145/358916.358994},
	acmid = {358994},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {CSCW, collaborative filtering, computer-supported cooperative work, expert locators, expertise finding, expertise location, information seeking, recommendation systems}
} 

@inproceedings{Anvik:J:MSR:2007,
	author = {Anvik, John and Murphy, Gail C.},
	title = {Determining Implementation Expertise from Bug Reports},
	booktitle = {Proceedings of the Fourth International Workshop on Mining Software Repositories},
	series = {MSR '07},
	year = {2007},
	isbn = {0-7695-2950-X},
	pages = {2--},
	url = {http://dx.doi.org/10.1109/MSR.2007.7},
	doi = {10.1109/MSR.2007.7},
	acmid = {1269018},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA}
}

@inproceedings{Tamrawi:A:FSE:2011,
	author = {Tamrawi, Ahmed and Nguyen, Tung Thanh and Al-Kofahi, Jafar M. and Nguyen, Tien N.},
	title = {Fuzzy set and cache-based approach for bug triaging},
	booktitle = {Proceedings of the 19th ACM SIGSOFT symposium and the 13th European conference on Foundations of software engineering},
	series = {ESEC/FSE '11},
	year = {2011},
	isbn = {978-1-4503-0443-6},
	location = {Szeged, Hungary},
	pages = {365--375},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2025113.2025163},
	doi = {10.1145/2025113.2025163},
	acmid = {2025163},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug triaging, developers' expertise, fuzzy set}
} 

@incollection{Song:X:UM:2005,
	year={2005},
	isbn={978-3-540-27885-6},
	booktitle={User Modeling 2005},
	volume={3538},
	series={Lecture Notes in Computer Science},
	editor={Ardissono, Liliana and Brna, Paul and Mitrovic, Antonija},
	doi={10.1007/11527886_14},
	title={ExpertiseNet: Relational and Evolutionary Expert Modeling},
	url={http://dx.doi.org/10.1007/11527886_14},
	publisher={Springer Berlin Heidelberg},
	author={Song, Xiaodan and Tseng, BelleL. and Lin, Ching-Yung and Sun, Ming-Ting},
	pages={99-108}
}

@inproceedings{Matter:D:MSR:2009,
	author = {Matter, Dominique and Kuhn, Adrian and Nierstrasz, Oscar},
	title = {Assigning bug reports using a vocabulary-based expertise model of developers},
	booktitle = {Proceedings of the 2009 6th IEEE International Working Conference on Mining Software Repositories},
	series = {MSR '09},
	year = {2009},
	isbn = {978-1-4244-3493-0},
	pages = {131--140},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/MSR.2009.5069491},
	doi = {10.1109/MSR.2009.5069491},
	acmid = {1591148},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA}
} 

@inproceedings{Rahman:F:ICSE:2011,
	author = {Rahman, Foyzur and Devanbu, Premkumar},
	title = {Ownership, experience and defects: a fine-grained study of authorship},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {491--500},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985860},
	doi = {10.1145/1985793.1985860},
	acmid = {1985860},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {collaboration, experience, ownership, software quality}
} 

@inproceedings{Bird:C:FSE:2011,
	author = {Bird, Christian and Nagappan, Nachiappan and Murphy, Brendan and Gall, Harald and Devanbu, Premkumar},
	title = {Don't touch my code!: examining the effects of ownership on software quality},
	booktitle = {Proceedings of the 19th ACM SIGSOFT symposium and the 13th European conference on Foundations of software engineering},
	series = {ESEC/FSE '11},
	year = {2011},
	isbn = {978-1-4503-0443-6},
	location = {Szeged, Hungary},
	pages = {4--14},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2025113.2025119},
	doi = {10.1145/2025113.2025119},
	acmid = {2025119},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {emprical software engineering, expertise, ownership, quality}
} 

@inproceedings{German:D:MSR:2006,
	author = {German, Daniel M.},
	title = {A study of the contributors of PostgreSQL},
	booktitle = {Proceedings of the 2006 international workshop on Mining software repositories},
	series = {MSR '06},
	year = {2006},
	isbn = {1-59593-397-2},
	location = {Shanghai, China},
	pages = {163--164},
	numpages = {2},
	url = {http://doi.acm.org/10.1145/1137983.1138022},
	doi = {10.1145/1137983.1138022},
	acmid = {1138022},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {mining software repositories, software evolution}
} 

@inproceedings{Tsunoda:M:MSR:2006,
	author = {Tsunoda, Masateru and Monden, Akito and Kakimoto, Takeshi and Kamei, Yasutaka and Matsumoto, Ken-ichi},
	title = {Analyzing OSS developers' working time using mailing lists archives},
	booktitle = {Proceedings of the 2006 international workshop on Mining software repositories},
	series = {MSR '06},
	year = {2006},
	isbn = {1-59593-397-2},
	location = {Shanghai, China},
	pages = {181--182},
	numpages = {2},
	url = {http://doi.acm.org/10.1145/1137983.1138031},
	doi = {10.1145/1137983.1138031},
	acmid = {1138031},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {overtime work, workload}
} 

@inproceedings{Bird:C:MSR:2006,
	author = {Bird, Christian and Gourley, Alex and Devanbu, Prem and Gertz, Michael and Swaminathan, Anand},
	title = {Mining email social networks},
	booktitle = {Proceedings of the 2006 international workshop on Mining software repositories},
	series = {MSR '06},
	year = {2006},
	isbn = {1-59593-397-2},
	location = {Shanghai, China},
	pages = {137--143},
	numpages = {7},
	url = {http://doi.acm.org/10.1145/1137983.1138016},
	doi = {10.1145/1137983.1138016},
	acmid = {1138016},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {open source, social networks}
} 

@article{DelRosso:C:JSME:2009,
	author = {Del Rosso, Christian},
	title = {Comprehend and analyze knowledge networks to improve software evolution},
	journal = {J. Softw. Maint. Evol.},
	issue_date = {May 2009},
	volume = {21},
	number = {3},
	month = may,
	year = {2009},
	issn = {1532-060X},
	pages = {189--215},
	numpages = {27},
	url = {http://dx.doi.org/10.1002/smr.v21:3},
	doi = {10.1002/smr.v21:3},
	acmid = {1552147},
	publisher = {John Wiley \& Sons, Inc.},
	address = {New York, NY, USA},
	keywords = {global software engineering, knowledge management, social network analysis, software development}
} 

@inproceedings{Weissgerber:P:MSR:2007,
	author = {Weissgerber, Peter and Pohl, Mathias and Burch, Michael},
	title = {Visual Data Mining in Software Archives to Detect How Developers Work Together},
	booktitle = {Proceedings of the Fourth International Workshop on Mining Software Repositories},
	series = {MSR '07},
	year = {2007},
	isbn = {0-7695-2950-X},
	pages = {9--},
	url = {http://dx.doi.org/10.1109/MSR.2007.34},
	doi = {10.1109/MSR.2007.34},
	acmid = {1269024},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA}
} 

@article{German:D:EMSE:2006,
	author = {German, Daniel M.},
	title = {An empirical study of fine-grained software modifications},
	journal = {Empirical Softw. Engg.},
	issue_date = {September 2006},
	volume = {11},
	number = {3},
	month = sep,
	year = {2006},
	issn = {1382-3256},
	pages = {369--393},
	numpages = {25},
	url = {http://dx.doi.org/10.1007/s10664-006-9004-6},
	doi = {10.1007/s10664-006-9004-6},
	acmid = {1146486},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Software artifacts, Software evolution, Software visualization, Version control}
} 

@inproceedings{Fischer:M:ICSM:2003,
	author = {Fischer, Michael and Pinzger, Martin and Gall, Harald},
	title = {Populating a Release History Database from Version Control and Bug Tracking Systems},
	booktitle = {Proceedings of the International Conference on Software Maintenance},
	series = {ICSM '03},
	year = {2003},
	isbn = {0-7695-1905-9},
	pages = {23--},
	url = {http://dl.acm.org/citation.cfm?id=942800.943568},
	acmid = {943568},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA}
} 

@inproceedings{Runeson:P:ICSE:2007,
	author = {Runeson, Per and Alexandersson, Magnus and Nyholm, Oskar},
	title = {Detection of Duplicate Defect Reports Using Natural Language Processing},
	booktitle = {Proceedings of the 29th international conference on Software Engineering},
	series = {ICSE '07},
	year = {2007},
	isbn = {0-7695-2828-7},
	pages = {499--510},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/ICSE.2007.32},
	doi = {10.1109/ICSE.2007.32},
	acmid = {1248882},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@phdthesis{Hiew:L:Thesis,
	title={Assisted detection of duplicate bug reports},
	author={Hiew, L.},
	year={2006},
	school={The University Of British Columbia}
}

@inproceedings{Wang:X:ICSE:2008,
	author = {Wang, Xiaoyin and Zhang, Lu and Xie, Tao and Anvik, John and Sun, Jiasu},
	title = {An approach to detecting duplicate bug reports using natural language and execution information},
	booktitle = {Proceedings of the 30th international conference on Software engineering},
	series = {ICSE '08},
	year = {2008},
	isbn = {978-1-60558-079-1},
	location = {Leipzig, Germany},
	pages = {461--470},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1368088.1368151},
	doi = {10.1145/1368088.1368151},
	acmid = {1368151},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {duplicate bug report, execution information, information retrieval},
} 

@inproceedings{Sun:C:ICSE:2010,
	author = {Sun, Chengnian and Lo, David and Wang, Xiaoyin and Jiang, Jing and Khoo, Siau-Cheng},
	title = {A discriminative model approach for accurate duplicate bug report retrieval},
	booktitle = {Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering - Volume 1},
	series = {ICSE '10},
	year = {2010},
	isbn = {978-1-60558-719-6},
	location = {Cape Town, South Africa},
	pages = {45--54},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1806799.1806811},
	doi = {10.1145/1806799.1806811},
	acmid = {1806811},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Jalbert:N:DSN:2008,
	title={Automated duplicate detection for bug tracking systems},
	author={Jalbert, N. and Weimer, W.},
	booktitle={Dependable Systems and Networks With FTCS and DCC, 2008. DSN 2008. IEEE International Conference on},
	pages={52--61},
	year={2008},
	organization={IEEE}
}

@inproceedings{Sun:C:ASE:2011,
	author = {Sun, Chengnian and Lo, David and Khoo, Siau-Cheng and Jiang, Jing},
	title = {Towards more accurate retrieval of duplicate bug reports},
	booktitle = {Proceedings of the 2011 26th IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '11},
	year = {2011},
	isbn = {978-1-4577-1638-6},
	pages = {253--262},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ASE.2011.6100061},
	doi = {10.1109/ASE.2011.6100061},
	acmid = {2190180},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Bettenburg:N:FSE:2008,
	author = {Bettenburg, Nicolas and Just, Sascha and Schr\"{o}ter, Adrian and Weiss, Cathrin and Premraj, Rahul and Zimmermann, Thomas},
	title = {What makes a good bug report?},
	booktitle = {Proceedings of the 16th ACM SIGSOFT International Symposium on Foundations of software engineering},
	series = {SIGSOFT '08/FSE-16},
	year = {2008},
	isbn = {978-1-59593-995-1},
	location = {Atlanta, Georgia},
	pages = {308--318},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1453101.1453146},
	doi = {10.1145/1453101.1453146},
	acmid = {1453146},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Bettenburg:N:MSR:2008,
	author = {Bettenburg, Nicolas and Premraj, Rahul and Zimmermann, Thomas and Kim, Sunghun},
	title = {Extracting structural information from bug reports},
	booktitle = {Proceedings of the 2008 international working conference on Mining software repositories},
	series = {MSR '08},
	year = {2008},
	isbn = {978-1-60558-024-1},
	location = {Leipzig, Germany},
	pages = {27--30},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1370750.1370757},
	doi = {10.1145/1370750.1370757},
	acmid = {1370757},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug reports, patches, source code, stack traces, structural information},
} 

@inproceedings{Kim:S:MSR:2006,
	author = {Kim, Sunghun and Whitehead,Jr., E. James},
	title = {How long did it take to fix bugs?},
	booktitle = {Proceedings of the 2006 international workshop on Mining software repositories},
	series = {MSR '06},
	year = {2006},
	isbn = {1-59593-397-2},
	location = {Shanghai, China},
	pages = {173--174},
	numpages = {2},
	url = {http://doi.acm.org/10.1145/1137983.1138027},
	doi = {10.1145/1137983.1138027},
	acmid = {1138027},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Canfora:G:SAC:2006,
	author = {Canfora, Gerardo and Cerulo, Luigi},
	title = {Supporting change request assignment in open source development},
	booktitle = {Proceedings of the 2006 ACM symposium on Applied computing},
	series = {SAC '06},
	year = {2006},
	isbn = {1-59593-108-2},
	location = {Dijon, France},
	pages = {1767--1772},
	numpages = {6},
	url = {http://doi.acm.org/10.1145/1141277.1141693},
	doi = {10.1145/1141277.1141693},
	acmid = {1141693},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {information retrieval, maintenance task assignment, mining software repositories},
} 

@inproceedings{Hooimeijer:P:ASE:2007,
	author = {Hooimeijer, Pieter and Weimer, Westley},
	title = {Modeling bug report quality},
	booktitle = {Proceedings of the twenty-second IEEE/ACM international conference on Automated software engineering},
	series = {ASE '07},
	year = {2007},
	isbn = {978-1-59593-882-4},
	location = {Atlanta, Georgia, USA},
	pages = {34--43},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1321631.1321639},
	doi = {10.1145/1321631.1321639},
	acmid = {1321639},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug report triage, information retrieval, issue tracking, statistical model},
} 

@inproceedings{Podgurski:A:ICSE:2003,
	author = {Podgurski, Andy and Leon, David and Francis, Patrick and Masri, Wes and Minch, Melinda and Sun, Jiayang and Wang, Bin},
	title = {Automated support for classifying software failure reports},
	booktitle = {Proceedings of the 25th International Conference on Software Engineering},
	series = {ICSE '03},
	year = {2003},
	isbn = {0-7695-1877-X},
	location = {Portland, Oregon},
	pages = {465--475},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=776816.776872},
	acmid = {776872},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Cubrani:D:SEKE:2004,
	title={Automatic bug triage using text categorization},
	author={{\v{C}}ubrani{\'c}, D. and Murphy, G.},
	booktitle={In SEKE 2004: Proceedings of the Sixteenth International Conference on Software Engineering \& Knowledge Engineering},
	year={2004},
	organization={Citeseer}
}

@INPROCEEDINGS{Menzies:T:ICSM:2008,
	author={Menzies, T. and Marcus, A.},
	booktitle={Software Maintenance, 2008. ICSM 2008. IEEE International Conference on}, title={Automated severity assessment of software defect reports},
	year={2008},
	month={28 2008-oct. 4},
	volume={},
	number={},
	pages={346 -355},
	keywords={NASA;automated severity assessment;machine learning techniques;mission critical systems;resource allocation;severity issue assessment;software defect reports;text mining;data mining;learning (artificial intelligence);resource allocation;software engineering;},
	doi={10.1109/ICSM.2008.4658083},
	ISSN={1063-6773},}

@inproceedings{Bettenburg:N:ETX:2007,
	author = {Bettenburg, Nicolas and Just, Sascha and Schr\"{o}ter, Adrian and Wei\ss, Cathrin and Premraj, Rahul and Zimmermann, Thomas},
	title = {Quality of bug reports in Eclipse},
	booktitle = {Proceedings of the 2007 OOPSLA workshop on eclipse technology eXchange},
	series = {eclipse '07},
	year = {2007},
	isbn = {978-1-60558-015-9},
	location = {Montreal, Quebec, Canada},
	pages = {21--25},
	numpages = {5},
	url = {http://doi.acm.org/10.1145/1328279.1328284},
	doi = {10.1145/1328279.1328284},
	acmid = {1328284},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@article{Basili:V:TSE:1996,
	author = {Basili, Victor R. and Briand, Lionel C. and Melo, Walc{\'e}lio L.},
	title = {A Validation of Object-Oriented Design Metrics as Quality Indicators},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {October 1996},
	volume = {22},
	number = {10},
	month = oct,
	year = {1996},
	issn = {0098-5589},
	pages = {751--761},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/32.544352},
	doi = {10.1109/32.544352},
	acmid = {239308},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Object-oriented design metrics, error prediction model, object-oriented software development, C++ programming language.},
} 

@article{Briand:L:TSE:1999,
	author = {Briand, Lionel C. and Daly, John W. and W\"{u}st, J\"{u}rgen K.},
	title = {A Unified Framework for Coupling Measurement in Object-Oriented Systems},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {January 1999},
	volume = {25},
	number = {1},
	month = jan,
	year = {1999},
	issn = {0098-5589},
	pages = {91--121},
	numpages = {31},
	url = {http://dx.doi.org/10.1109/32.748920},
	doi = {10.1109/32.748920},
	acmid = {297728},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Coupling, object-oriented, measurement.},
} 

@article{Emam:K:JSS:2001,
	author = {Emam, Khaled El and Melo, Walcelio and Machado, Javam C.},
	title = {The prediction of faulty classes using object-oriented design metrics},
	journal = {J. Syst. Softw.},
	issue_date = {Feb 1,2001},
	volume = {56},
	number = {1},
	month = feb,
	year = {2001},
	issn = {0164-1212},
	pages = {63--75},
	numpages = {13},
	url = {http://dx.doi.org/10.1016/S0164-1212(00)00086-8},
	doi = {10.1016/S0164-1212(00)00086-8},
	acmid = {371306},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {Java metrics, Java quality, Object-oriented metrics, Software metrics, Software quality},
} 

@article{Gyimothy:T:TSE:2005,
	author = {Gyimothy, Tibor and Ferenc, Rudolf and Siket, Istvan},
	title = {Empirical Validation of Object-Oriented Metrics on Open Source Software for Fault Prediction},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {October 2005},
	volume = {31},
	number = {10},
	month = oct,
	year = {2005},
	issn = {0098-5589},
	pages = {897--910},
	numpages = {14},
	url = {http://dx.doi.org/10.1109/TSE.2005.112},
	doi = {10.1109/TSE.2005.112},
	acmid = {1100985},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Bugzilla, C++, Columbus., Index Terms- Fact extraction, Index Terms- Fact extraction, metrics validation, reverse engineering, open source software, fault-proneness detection, Mozilla, Bugzilla, C++, compiler wrapping, Columbus., Mozilla, compiler wrapping, fault-proneness detection, metrics validation, open source software, reverse engineering},
} 

@inproceedings{Nagappan:N:ICSE:2005,
	author = {Nagappan, Nachiappan and Ball, Thomas},
	title = {Static analysis tools as early indicators of pre-release defect density},
	booktitle = {Proceedings of the 27th international conference on Software engineering},
	series = {ICSE '05},
	year = {2005},
	isbn = {1-58113-963-2},
	location = {St. Louis, MO, USA},
	pages = {580--586},
	numpages = {7},
	url = {http://doi.acm.org/10.1145/1062455.1062558},
	doi = {10.1145/1062455.1062558},
	acmid = {1062558},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {defect density, fault-proneness, static analysis tools, statistical methods},
} 

@inproceedings{Nagappan:N:ICSE:2006,
	author = {Nagappan, Nachiappan and Ball, Thomas and Zeller, Andreas},
	title = {Mining metrics to predict component failures},
	booktitle = {Proceedings of the 28th international conference on Software engineering},
	series = {ICSE '06},
	year = {2006},
	isbn = {1-59593-375-1},
	location = {Shanghai, China},
	pages = {452--461},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1134285.1134349},
	doi = {10.1145/1134285.1134349},
	acmid = {1134349},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug database, complexity metrics, empirical study, principal component analysis, regression model},
} 

@article{Ohlsson:N:TSE:1996,
	author = {Ohlsson, Niclas and Alberg, Hans},
	title = {Predicting Fault-Prone Software Modules in Telephone Switches},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {December 1996},
	volume = {22},
	number = {12},
	month = dec,
	year = {1996},
	issn = {0098-5589},
	pages = {886--894},
	numpages = {9},
	url = {http://dx.doi.org/10.1109/32.553637},
	doi = {10.1109/32.553637},
	acmid = {246143},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Complexity, empirical study, fault-prone modules, metrics, prediction, software measurement, regression analysis, software reliability, statistical analysis.},
} 

@article{Subramanyam:R:TSE:2003,
	author = {Subramanyam, Ramanath and Krishnan, M. S.},
	title = {Empirical Analysis of CK Metrics for Object-Oriented Design Complexity: Implications for Software Defects},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {April 2003},
	volume = {29},
	number = {4},
	month = apr,
	year = {2003},
	issn = {0098-5589},
	pages = {297--310},
	numpages = {14},
	url = {http://dx.doi.org/10.1109/TSE.2003.1191795},
	doi = {10.1109/TSE.2003.1191795},
	acmid = {766682},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Object-oriented design, software metrics validation, object-oriented languages, C++, Java.},
}

@inproceedings{Nagappan:2005:URC:1062455.1062514,
	author = {Nagappan, Nachiappan and Ball, Thomas},
	title = {Use of relative code churn measures to predict system defect density},
	booktitle = {Proceedings of the 27th international conference on Software engineering},
	series = {ICSE '05},
	year = {2005},
	isbn = {1-58113-963-2},
	location = {St. Louis, MO, USA},
	pages = {284--292},
	numpages = {9},
	url = {http://doi.acm.org/10.1145/1062455.1062514},
	doi = {10.1145/1062455.1062514},
	acmid = {1062514},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {defect density, fault-proneness, multiple regression, principal component analysis, relative code churn},
} 

@inproceedings{Hassan:2009:PFU:1555001.1555024,
	author = {Hassan, Ahmed E.},
	title = {Predicting faults using the complexity of code changes},
	booktitle = {Proceedings of the 31st International Conference on Software Engineering},
	series = {ICSE '09},
	year = {2009},
	isbn = {978-1-4244-3453-4},
	pages = {78--88},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2009.5070510},
	doi = {10.1109/ICSE.2009.5070510},
	acmid = {1555024},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Moser:2008:CAE:1368088.1368114,
	author = {Moser, Raimund and Pedrycz, Witold and Succi, Giancarlo},
	title = {A comparative analysis of the efficiency of change metrics and static code attributes for defect prediction},
	booktitle = {Proceedings of the 30th international conference on Software engineering},
	series = {ICSE '08},
	year = {2008},
	isbn = {978-1-60558-079-1},
	location = {Leipzig, Germany},
	pages = {181--190},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1368088.1368114},
	doi = {10.1145/1368088.1368114},
	acmid = {1368114},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {cost-sensitive classification, defect prediction, software metrics},
} 

@article{DAmbros:2012:EDP:2318097.2318149,
	author = {D'Ambros, Marco and Lanza, Michele and Robbes, Romain},
	title = {Evaluating defect prediction approaches: a benchmark and an extensive comparison},
	journal = {Empirical Softw. Engg.},
	issue_date = {August    2012},
	volume = {17},
	number = {4-5},
	month = aug,
	year = {2012},
	issn = {1382-3256},
	pages = {531--577},
	numpages = {47},
	url = {http://dx.doi.org/10.1007/s10664-011-9173-9},
	doi = {10.1007/s10664-011-9173-9},
	acmid = {2318149},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Change metrics, Defect prediction, Source code metrics},
} 



@inproceedings{Bernstein:2007:IDP:1294948.1294953,
	author = {Bernstein, Abraham and Ekanayake, Jayalath and Pinzger, Martin},
	title = {Improving defect prediction using temporal features and non linear models},
	booktitle = {Ninth international workshop on Principles of software evolution: in conjunction with the 6th ESEC/FSE joint meeting},
	series = {IWPSE '07},
	year = {2007},
	isbn = {978-1-59593-722-3},
	location = {Dubrovnik, Croatia},
	pages = {11--18},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1294948.1294953},
	doi = {10.1145/1294948.1294953},
	acmid = {1294953},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {decision tree learner, defect prediction, mining software repository},
} 


@inproceedings{Kim:2007:PFC:1248820.1248881,
	author = {Kim, Sunghun and Zimmermann, Thomas and Whitehead Jr., E. James and Zeller, Andreas},
	title = {Predicting Faults from Cached History},
	booktitle = {Proceedings of the 29th international conference on Software Engineering},
	series = {ICSE '07},
	year = {2007},
	isbn = {0-7695-2828-7},
	pages = {489--498},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICSE.2007.66},
	doi = {10.1109/ICSE.2007.66},
	acmid = {1248881},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Hassan:2005:TTL:1090952.1091858,
	author = {Hassan, Ahmed E. and Holt, Richard C.},
	title = {The Top Ten List: Dynamic Fault Prediction},
	booktitle = {Proceedings of the 21st IEEE International Conference on Software Maintenance},
	series = {ICSM '05},
	year = {2005},
	isbn = {0-7695-2368-4},
	pages = {263--272},
	numpages = {10},
	publisher = {IEEE Computer Society}
} 

@article{Arisholm:2010:SCI:1663656.1663909,
	author = {Arisholm, Erik and Briand, Lionel C. and Johannessen, Eivind B.},
	title = {A systematic and comprehensive investigation of methods to build and evaluate fault prediction models},
	journal = {J. Syst. Softw.},
	issue_date = {January, 2010},
	volume = {83},
	number = {1},
	month = jan,
	year = {2010},
	issn = {0164-1212},
	pages = {2--17},
	numpages = {16},
	url = {http://dx.doi.org/10.1016/j.jss.2009.06.055},
	doi = {10.1016/j.jss.2009.06.055},
	acmid = {1663909},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {Cost-effectiveness, Fault prediction models, Verification},
} 

@inproceedings{Binkley:1998:VCD:302163.302212,
	author = {Binkley, Aaron B. and Schach, Stephen R.},
	title = {Validation of the coupling dependency metric as a predictor of run-time failures and maintenance measures},
	booktitle = {Proceedings of the 20th international conference on Software engineering},
	series = {ICSE '98},
	year = {1998},
	isbn = {0-8186-8368-6},
	location = {Kyoto, Japan},
	pages = {452--455},
	numpages = {4},
	url = {http://dl.acm.org/citation.cfm?id=302163.302212},
	acmid = {302212},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Fenton:2000:QAF:630824.631250,
	author = {Fenton, Norman E. and Ohlsson, Niclas},
	title = {Quantitative Analysis of Faults and Failures in a Complex Software System},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {August 2000},
	volume = {26},
	number = {8},
	month = aug,
	year = {2000},
	issn = {0098-5589},
	pages = {797--814},
	numpages = {18},
	url = {http://dx.doi.org/10.1109/32.879815},
	doi = {10.1109/32.879815},
	acmid = {631250},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Software faults and failures, software metrics, empirical studies.},
} 

@article{Jiang:2008:TEF:1416830.1416836,
	author = {Jiang, Yue and Cukic, Bojan and Ma, Yan},
	title = {Techniques for evaluating fault prediction models},
	journal = {Empirical Softw. Engg.},
	issue_date = {October   2008},
	volume = {13},
	number = {5},
	month = oct,
	year = {2008},
	issn = {1382-3256},
	pages = {561--595},
	numpages = {35},
	url = {http://dx.doi.org/10.1007/s10664-008-9079-3},
	doi = {10.1007/s10664-008-9079-3},
	acmid = {1416836},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Empirical studies, Fault-prediction models, Model evaluation, Predictive models in software engineering},
}

@article{Khoshgoftaar:1999:CSO:594380.594449,
	author = {Khoshgoftaar, Taghi M. and Allen, Edward B.},
	title = {A Comparative Study of Ordering and Classification of Fault-ProneSoftware Modules},
	journal = {Empirical Softw. Engg.},
	issue_date = {June 1999},
	volume = {4},
	number = {2},
	month = jun,
	year = {1999},
	issn = {1382-3256},
	pages = {159--186},
	numpages = {28},
	url = {http://dx.doi.org/10.1023/A:1009876418873},
	doi = {10.1023/A:1009876418873},
	acmid = {594449},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Software reliability, fault-prone modules, module-order models, multiple linear regression, nonparametric discriminant analysis, principal components analysis, software quality models},
}

@inproceedings{Koru:2007:MES:1268984.1269058,
	author = {Koru, A. Gunes and Zhang, Dongsong and Liu, Hongfang},
	title = {Modeling the Effect of Size on Defect Proneness for Open-Source Software},
	booktitle = {Proceedings of the Third International Workshop on Predictor Models in Software Engineering},
	series = {PROMISE '07},
	year = {2007},
	isbn = {0-7695-2954-2},
	pages = {10--},
	url = {http://dx.doi.org/10.1109/PROMISE.2007.9},
	doi = {10.1109/PROMISE.2007.9},
	acmid = {1269058},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Koru:2008:TRD:1416830.1416834,
	author = {Koru, A. G\"{u}ne\c{s} and Emam, Khaled El and Zhang, Dongsong and Liu, Hongfang and Mathew, Divya},
	title = {Theory of relative defect proneness},
	journal = {Empirical Softw. Engg.},
	issue_date = {October   2008},
	volume = {13},
	number = {5},
	month = oct,
	year = {2008},
	issn = {1382-3256},
	pages = {473--498},
	numpages = {26},
	url = {http://dx.doi.org/10.1007/s10664-008-9080-x},
	doi = {10.1007/s10664-008-9080-x},
	acmid = {1416834},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Open---source software, Planning for software quality assurance, Size---defect relationship, Software inspections, Software metrics, Software reviews, Software science, Software testing},
} 

@article{Lessmann:2008:BCM:1446226.1446245,
	author = {Lessmann, Stefan and Baesens, Bart and Mues, Christophe and Pietsch, Swantje},
	title = {Benchmarking Classification Models for Software Defect Prediction: A Proposed Framework and Novel Findings},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {July 2008},
	volume = {34},
	number = {4},
	month = jul,
	year = {2008},
	issn = {0098-5589},
	pages = {485--496},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/TSE.2008.35},
	doi = {10.1109/TSE.2008.35},
	acmid = {1446245},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Complexity measures, Complexity measures, Data mining, Formal methods, Statistical methods, Data mining, Formal methods, Statistical methods},
} 

@inproceedings{Mende:2010:RDP:1868328.1868336,
	author = {Mende, Thilo},
	title = {Replication of defect prediction studies: problems, pitfalls and recommendations},
	booktitle = {Proceedings of the 6th International Conference on Predictive Models in Software Engineering},
	series = {PROMISE '10},
	year = {2010},
	isbn = {978-1-4503-0404-7},
	location = {Timi\şoara, Romania},
	pages = {5:1--5:10},
	articleno = {5},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1868328.1868336},
	doi = {10.1145/1868328.1868336},
	acmid = {1868336},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {defect prediction model, replication},
} 

@inproceedings{Mende:2009:RED:1540438.1540448,
	author = {Mende, Thilo and Koschke, Rainer},
	title = {Revisiting the evaluation of defect prediction models},
	booktitle = {Proceedings of the 5th International Conference on Predictor Models in Software Engineering},
	series = {PROMISE '09},
	year = {2009},
	isbn = {978-1-60558-634-2},
	location = {Vancouver, British Columbia, Canada},
	pages = {7:1--7:10},
	articleno = {7},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1540438.1540448},
	doi = {10.1145/1540438.1540448},
	acmid = {1540448},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {cost-sensitive performance measures, defect prediction},
} 

@article{Myrtveit:2005:RVC:1069599.1069771,
	author = {Myrtveit, Ingunn and Stensrud, Erik and Shepperd, Martin},
	title = {Reliability and Validity in Comparative Studies of Software Prediction Models},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {May 2005},
	volume = {31},
	number = {5},
	month = may,
	year = {2005},
	issn = {0098-5589},
	pages = {380--391},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/TSE.2005.58},
	doi = {10.1109/TSE.2005.58},
	acmid = {1069771},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Index Terms- Software metrics, Index Terms- Software metrics, cost estimation, cross-validation, empirical methods, arbitrary function approximators, machine learning, estimation by analogy, regression analysis, simulation, reliability, validity, accuracy indicators., accuracy indicators., arbitrary function approximators, cost estimation, cross-validation, empirical methods, estimation by analogy, machine learning, regression analysis, reliability, simulation, validity},
} 

@inproceedings{Ostrand:2002:DFL:566172.566181,
	author = {Ostrand, Thomas J. and Weyuker, Elaine J.},
	title = {The distribution of faults in a large industrial software system},
	booktitle = {Proceedings of the 2002 ACM SIGSOFT international symposium on Software testing and analysis},
	series = {ISSTA '02},
	year = {2002},
	isbn = {1-58113-562-9},
	location = {Roma, Italy},
	pages = {55--64},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/566172.566181},
	doi = {10.1145/566172.566181},
	acmid = {566181},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {empirical study, fault-prone, pareto, software faults, software testing},
}

@article{Subramanyam:2003:EAC:766665.766682,
	author = {Subramanyam, Ramanath and Krishnan, M. S.},
	title = {Empirical Analysis of CK Metrics for Object-Oriented Design Complexity: Implications for Software Defects},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {April 2003},
	volume = {29},
	number = {4},
	month = apr,
	year = {2003},
	issn = {0098-5589},
	pages = {297--310},
	numpages = {14},
	url = {http://dx.doi.org/10.1109/TSE.2003.1191795},
	doi = {10.1109/TSE.2003.1191795},
	acmid = {766682},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Object-oriented design, software metrics validation, object-oriented languages, C++, Java.},
} 


@inproceedings{Zimmermann:2009:CDP:1595696.1595713,
	author = {Zimmermann, Thomas and Nagappan, Nachiappan and Gall, Harald and Giger, Emanuel and Murphy, Brendan},
	title = {Cross-project defect prediction: a large scale experiment on data vs. domain vs. process},
	booktitle = {Proceedings of the the 7th joint meeting of the European software engineering conference and the ACM SIGSOFT symposium on The foundations of software engineering},
	series = {ESEC/FSE '09},
	year = {2009},
	isbn = {978-1-60558-001-2},
	location = {Amsterdam, The Netherlands},
	pages = {91--100},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1595696.1595713},
	doi = {10.1145/1595696.1595713},
	acmid = {1595713},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {churn, cross-project, decision trees, defect prediction, logistic regression, prediction quality},
}

@inproceedings{Zimmermann:2007:PDE:1268984.1269057,
	author = {Zimmermann, Thomas and Premraj, Rahul and Zeller, Andreas},
	title = {Predicting Defects for Eclipse},
	booktitle = {Proceedings of the Third International Workshop on Predictor Models in Software Engineering},
	series = {PROMISE '07},
	year = {2007},
	isbn = {0-7695-2954-2},
	pages = {9--},
	url = {http://dx.doi.org/10.1109/PROMISE.2007.10},
	doi = {10.1109/PROMISE.2007.10},
	acmid = {1269057},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Zimmermann:2008:PDU:1368088.1368161,
	author = {Zimmermann, Thomas and Nagappan, Nachiappan},
	title = {Predicting defects using network analysis on dependency graphs},
	booktitle = {Proceedings of the 30th international conference on Software engineering},
	series = {ICSE '08},
	year = {2008},
	isbn = {978-1-60558-079-1},
	location = {Leipzig, Germany},
	pages = {531--540},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1368088.1368161},
	doi = {10.1145/1368088.1368161},
	acmid = {1368161},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {defect prediction, dependency graph, network analysis, windows server 2003},
} 

@inproceedings{Wolf:2009:PBF:1555001.1555017,
	author = {Wolf, Timo and Schroter, Adrian and Damian, Daniela and Nguyen, Thanh},
	title = {Predicting build failures using social network analysis on developer communication},
	booktitle = {Proceedings of the 31st International Conference on Software Engineering},
	series = {ICSE '09},
	year = {2009},
	isbn = {978-1-4244-3453-4},
	pages = {1--11},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2009.5070503},
	doi = {10.1109/ICSE.2009.5070503},
	acmid = {1555017},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Turhan:2009:RVC:1612763.1612782,
	author = {Turhan, Burak and Menzies, Tim and Bener, Ay\c{s}e B. and Di Stefano, Justin},
	title = {On the relative value of cross-company and within-company data for defect prediction},
	journal = {Empirical Softw. Engg.},
	issue_date = {October   2009},
	volume = {14},
	number = {5},
	month = oct,
	year = {2009},
	issn = {1382-3256},
	pages = {540--578},
	numpages = {39},
	url = {http://dx.doi.org/10.1007/s10664-008-9103-7},
	doi = {10.1007/s10664-008-9103-7},
	acmid = {1612782},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Cross-company, Defect prediction, Learning, Metrics (product metrics), Nearest-neighbor filtering, Within-company},
} 

@inproceedings{Shin:2009:CSI:1590955.1591138,
	author = {Shin, Yonghee and Bell, Robert and Ostrand, Thomas and Weyuker, Elaine},
	title = {Does calling structure information improve the accuracy of fault prediction?},
	booktitle = {Proceedings of the 2009 6th IEEE International Working Conference on Mining Software Repositories},
	series = {MSR '09},
	year = {2009},
	isbn = {978-1-4244-3493-0},
	pages = {61--70},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/MSR.2009.5069481},
	doi = {10.1109/MSR.2009.5069481},
	acmid = {1591138},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Pinzger:2008:DNP:1453101.1453105,
	author = {Pinzger, Martin and Nagappan, Nachiappan and Murphy, Brendan},
	title = {Can developer-module networks predict failures?},
	booktitle = {Proceedings of the 16th ACM SIGSOFT International Symposium on Foundations of software engineering},
	series = {SIGSOFT '08/FSE-16},
	year = {2008},
	isbn = {978-1-59593-995-1},
	location = {Atlanta, Georgia},
	pages = {2--12},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1453101.1453105},
	doi = {10.1145/1453101.1453105},
	acmid = {1453105},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {developer contribution network, failure prediction, network centrality measures, social network analysis},
} 

@inproceedings{Ostrand:2007:AAI:1273463.1273493,
	author = {Ostrand, Thomas J. and Weyuker, Elaine J. and Bell, Robert M.},
	title = {Automating algorithms for the identification of fault-prone files},
	booktitle = {Proceedings of the 2007 international symposium on Software testing and analysis},
	series = {ISSTA '07},
	year = {2007},
	isbn = {978-1-59593-734-6},
	location = {London, United Kingdom},
	pages = {219--227},
	numpages = {9},
	url = {http://doi.acm.org/10.1145/1273463.1273493},
	doi = {10.1145/1273463.1273493},
	acmid = {1273493},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {empirical study, fault-prone, prediction, regression model, software faults, software testing},
} 

@article{Ostrand:2005:PLN:1069598.1069769,
	author = {Ostrand, Thomas J. and Weyuker, Elaine J. and Bell, Robert M.},
	title = {Predicting the Location and Number of Faults in Large Software Systems},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {April 2005},
	volume = {31},
	number = {4},
	month = apr,
	year = {2005},
	issn = {0098-5589},
	pages = {340--355},
	numpages = {16},
	url = {http://dx.doi.org/10.1109/TSE.2005.49},
	doi = {10.1109/TSE.2005.49},
	acmid = {1069769},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Index Terms- Software faults, Index Terms- Software faults, fault-prone, prediction, regression model, empirical study, software testing., empirical study, fault-prone, prediction, regression model, software testing.},
} 

@inproceedings{Ostrand:2004:BUG:1007512.1007524,
	author = {Ostrand, Thomas J. and Weyuker, Elaine J. and Bell, Robert M.},
	title = {Where the bugs are},
	booktitle = {Proceedings of the 2004 ACM SIGSOFT international symposium on Software testing and analysis},
	series = {ISSTA '04},
	year = {2004},
	isbn = {1-58113-820-2},
	location = {Boston, Massachusetts, USA},
	pages = {86--96},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1007512.1007524},
	doi = {10.1145/1007512.1007524},
	acmid = {1007524},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {empirical study, fault-prone, prediction, regression model, software faults, software testing},
} 

@inproceedings{Neuhaus:2007:PVS:1315245.1315311,
	author = {Neuhaus, Stephan and Zimmermann, Thomas and Holler, Christian and Zeller, Andreas},
	title = {Predicting vulnerable software components},
	booktitle = {Proceedings of the 14th ACM conference on Computer and communications security},
	series = {CCS '07},
	year = {2007},
	isbn = {978-1-59593-703-2},
	location = {Alexandria, Virginia, USA},
	pages = {529--540},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1315245.1315311},
	doi = {10.1145/1315245.1315311},
	acmid = {1315311},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {prediction, software security},
} 


@inproceedings{Nikora:2003:DFP:942804.943747,
	author = {Nikora, Allen P. and Munson, John C.},
	title = {Developing Fault Predictors for Evolving Software Systems},
	booktitle = {Proceedings of the 9th International Symposium on Software Metrics},
	series = {METRICS '03},
	year = {2003},
	isbn = {0-7695-1987-3},
	pages = {338--},
	url = {http://dl.acm.org/citation.cfm?id=942804.943747},
	acmid = {943747},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {defect content estimation techniques, fault prediction, software metrics, software measurement frameworks, software quality models},
}

@article{Menzies:2010:DPS:1842512.1842517,
	author = {Menzies, Tim and Milton, Zach and Turhan, Burak and Cukic, Bojan and Jiang, Yue and Bener, Ay\c{s}e},
	title = {Defect prediction from static code features: current results, limitations, new approaches},
	journal = {Automated Software Engg.},
	issue_date = {December  2010},
	volume = {17},
	number = {4},
	month = dec,
	year = {2010},
	issn = {0928-8910},
	pages = {375--407},
	numpages = {33},
	url = {http://dx.doi.org/10.1007/s10515-010-0069-5},
	doi = {10.1007/s10515-010-0069-5},
	acmid = {1842517},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Defect prediction, Static code features, WHICH},
}

@article{Menzies:2007:DMS:1248721.1248734,
	author = {Menzies, Tim and Greenwald, Jeremy and Frank, Art},
	title = {Data Mining Static Code Attributes to Learn Defect Predictors},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {January 2007},
	volume = {33},
	number = {1},
	month = jan,
	year = {2007},
	issn = {0098-5589},
	pages = {2--13},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/TSE.2007.10},
	doi = {10.1109/TSE.2007.10},
	acmid = {1248734},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Data mining detect prediction, Data mining detect prediction, McCabe, Halstead, artifical intelligence, empirical, naive Bayes., Halstead, McCabe, artifical intelligence, empirical, naive Bayes.},
} 

@inproceedings{Mende:2010:EDP:1955601.1955974,
	author = {Mende, Thilo and Koschke, Rainer},
	title = {Effort-Aware Defect Prediction Models},
	booktitle = {Proceedings of the 2010 14th European Conference on Software Maintenance and Reengineering},
	series = {CSMR '10},
	year = {2010},
	isbn = {978-0-7695-4321-5},
	pages = {107--116},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/CSMR.2010.18},
	doi = {10.1109/CSMR.2010.18},
	acmid = {1955974},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {Defect Prediction Models, Evaluation, Cost-Benefits},
} 

@inproceedings{Khoshgoftaar:1996:DSM:851006.856044,
	author = {Khoshgoftaar, T. M. and Allen, E. B. and Goel, N. and Nandi, A. and McMullan, J.},
	title = {Detection of software modules with high debug code churn in a very large legacy system},
	booktitle = {Proceedings of the The Seventh International Symposium on Software Reliability Engineering},
	series = {ISSRE '96},
	year = {1996},
	isbn = {0-8186-7707-4},
	pages = {364--},
	url = {http://dl.acm.org/citation.cfm?id=851006.856044},
	acmid = {856044},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {bug fixes, consecutive releases, discriminant analysis, fault counts, fault prone modules, fit data set, high debug code churn, realistic simulation, reliable telecommunications, reuse history, software module detection, static software product metrics, telecommunication computing, telecommunications software, test data set, unexpected problems, very large legacy system},
}

@inproceedings{Kamei:2010:RCB:1912607.1913298,
	author = {Kamei, Yasutaka and Matsumoto, Shinsuke and Monden, Akito and Matsumoto, Ken-ichi and Adams, Bram and Hassan, Ahmed E.},
	title = {Revisiting common bug prediction findings using effort-aware models},
	booktitle = {Proceedings of the 2010 IEEE International Conference on Software Maintenance},
	series = {ICSM '10},
	year = {2010},
	isbn = {978-1-4244-8630-4},
	pages = {1--10},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICSM.2010.5609530},
	doi = {10.1109/ICSM.2010.5609530},
	acmid = {1913298},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Graves:2000:PFI:347489.347496,
	author = {Graves, Todd L. and Karr, Alan F. and Marron, J. S. and Siy, Harvey},
	title = {Predicting Fault Incidence Using Software Change History},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {July 2000},
	volume = {26},
	number = {7},
	month = jul,
	year = {2000},
	issn = {0098-5589},
	pages = {653--661},
	numpages = {9},
	url = {http://dx.doi.org/10.1109/32.859533},
	doi = {10.1109/32.859533},
	acmid = {347496},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Fault potential, code decay, change management data, metrics, statistical analysis, generalized linear models.},
} 

@inproceedings{Bacchelli:2010:PCM:2128562.2128570,
	author = {Bacchelli, Alberto and D'Ambros, Marco and Lanza, Michele},
	title = {Are popular classes more defect prone?},
	booktitle = {Proceedings of the 13th international conference on Fundamental Approaches to Software Engineering},
	series = {FASE'10},
	year = {2010},
	isbn = {3-642-12028-8, 978-3-642-12028-2},
	location = {Paphos, Cyprus},
	pages = {59--73},
	numpages = {15},
	url = {http://dx.doi.org/10.1007/978-3-642-12029-9_5},
	doi = {10.1007/978-3-642-12029-9_5},
	acmid = {2128570},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
} 

@inproceedings{Arnaoudova:2010:PCI:1912607.1913343,
	author = {Arnaoudova, Venera and Eshkevari, Laleh and Oliveto, Rocco and Gueheneuc, Yann-Gael and Antoniol, Giuliano},
	title = {Physical and conceptual identifier dispersion: Measures and relation to fault proneness},
	booktitle = {Proceedings of the 2010 IEEE International Conference on Software Maintenance},
	series = {ICSM '10},
	year = {2010},
	isbn = {978-1-4244-8630-4},
	pages = {1--5},
	numpages = {5},
	url = {http://dx.doi.org/10.1109/ICSM.2010.5609748},
	doi = {10.1109/ICSM.2010.5609748},
	acmid = {1913343},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Arisholm:2006:PFC:1159733.1159738,
	author = {Arisholm, Erik and Briand, Lionel C.},
	title = {Predicting fault-prone components in a java legacy system},
	booktitle = {Proceedings of the 2006 ACM/IEEE international symposium on Empirical software engineering},
	series = {ISESE '06},
	year = {2006},
	isbn = {1-59593-218-6},
	location = {Rio de Janeiro, Brazil},
	pages = {8--17},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1159733.1159738},
	doi = {10.1145/1159733.1159738},
	acmid = {1159738},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Marks:2011:SFB:2020390.2020401,
	author = {Marks, Lionel and Zou, Ying and Hassan, Ahmed E.},
	title = {Studying the fix-time for bugs in large open source projects},
	booktitle = {Proceedings of the 7th International Conference on Predictive Models in Software Engineering},
	series = {Promise '11},
	year = {2011},
	isbn = {978-1-4503-0709-3},
	location = {Banff, Alberta, Canada},
	pages = {11:1--11:8},
	articleno = {11},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/2020390.2020401},
	doi = {10.1145/2020390.2020401},
	acmid = {2020401},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug fix-time, empirical software engineering, mining software repositories},
} 

@article{Anvik:J:TOSEM:2011,
	title={Reducing the effort of bug report triage: Recommenders for development-oriented decisions},
	author={Anvik, J. and Murphy, G.C.},
	journal={ACM Transactions on Software Engineering and Methodology (TOSEM)},
	volume={20},
	number={3},
	pages={10},
	year={2011},
	publisher={ACM}
}

@article{Hofman:2011:BES:1968922.1968960,
	author = {Hofman, Rados\law},
	title = {Behavioral economics in software quality engineering},
	journal = {Empirical Softw. Engg.},
	issue_date = {April     2011},
	volume = {16},
	number = {2},
	month = apr,
	year = {2011},
	issn = {1382-3256},
	pages = {278--293},
	numpages = {16},
	url = {http://dx.doi.org/10.1007/s10664-010-9140-x},
	doi = {10.1007/s10664-010-9140-x},
	acmid = {1968960},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Behavioral economics, Cognitive psychology, Quality perception, Software},
} 

@inproceedings{Ko:2012:MWS:2212776.2212797,
	author = {Ko, Andrew},
	title = {Mining whining in support forums with frictionary},
	booktitle = {CHI '12 Extended Abstracts on Human Factors in Computing Systems},
	series = {CHI EA '12},
	year = {2012},
	isbn = {978-1-4503-1016-1},
	location = {Austin, Texas, USA},
	pages = {191--200},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/2212776.2212797},
	doi = {10.1145/2212776.2212797},
	acmid = {2212797},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bugs, software problems, support, topic extraction},
} 

@article{Stavrinoudis:2005:EEU:1059832.1059836,
	author = {Stavrinoudis, Dimitris and Xenos, Michalis and Peppas, Pavlos and Christodoulakis, Dimitris},
	title = {Early Estimation of Users' Perception of Software Quality},
	journal = {Software Quality Control},
	issue_date = {June 2005},
	volume = {13},
	number = {2},
	month = jun,
	year = {2005},
	issn = {0963-9314},
	pages = {155--175},
	numpages = {21},
	url = {http://dx.doi.org/10.1007/s11219-005-6215-9},
	doi = {10.1007/s11219-005-6215-9},
	acmid = {1059836},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Grove's System of Spheres, ISO9126, belief revision, quality characteristics, software quality measurements, users' opinion},
} 

@inproceedings{Xenos:1994:SQU:646294.687542,
	author = {Xenos, Michalis Nik and Christodoulakis, D.},
	title = {Software Quality: The User's Point of View},
	booktitle = {Software Quality and Productivity: Theory, practice and training},
	year = {1995},
	isbn = {0-412-62960-7},
	pages = {266--272},
	numpages = {7},
	url = {http://dl.acm.org/citation.cfm?id=646294.687542},
	acmid = {687542},
	publisher = {Chapman \& Hall, Ltd.},
	address = {London, UK, UK},
} 

@inproceedings{Mockus:2005:PCP:1062455.1062506,
	author = {Mockus, Audris and Zhang, Ping and Li, Paul Luo},
	title = {Predictors of customer perceived software quality},
	booktitle = {Proceedings of the 27th international conference on Software engineering},
	series = {ICSE '05},
	year = {2005},
	isbn = {1-58113-963-2},
	location = {St. Louis, MO, USA},
	pages = {225--233},
	numpages = {9},
	url = {http://doi.acm.org/10.1145/1062455.1062506},
	doi = {10.1145/1062455.1062506},
	acmid = {1062506},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {metrics, modeling, quality},
} 

@article{Morris:1997:UPI:624620.625741,
	author = {Morris, Michael G. and Dillon, Andrew},
	title = {How User Perceptions Influence Software Use},
	journal = {IEEE Softw.},
	issue_date = {July 1997},
	volume = {14},
	number = {4},
	month = jul,
	year = {1997},
	issn = {0740-7459},
	pages = {58--65},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/52.595956},
	doi = {10.1109/52.595956},
	acmid = {625741},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{Chilana:2010:UEU:1915084.1916371,
	author = {Chilana, Parmit K. and Ko, Andrew J. and Wobbrock, Jacob O.},
	title = {Understanding Expressions of Unwanted Behaviors in Open Bug Reporting},
	booktitle = {Proceedings of the 2010 IEEE Symposium on Visual Languages and Human-Centric Computing},
	series = {VLHCC '10},
	year = {2010},
	isbn = {978-0-7695-4206-5},
	pages = {203--206},
	numpages = {4},
	url = {http://dx.doi.org/10.1109/VLHCC.2010.35},
	doi = {10.1109/VLHCC.2010.35},
	acmid = {1916371},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {open bug reporting, user expectations, software behavior},
} 

@book{langville2009google,
	title={Google's PageRank and beyond: The science of search engine rankings},
	author={Langville, A.N. and Meyer, C.D.},
	year={2009},
	publisher={Princeton University Press}
}

@article{chang2010hierarchical,
	title={Hierarchical relational models for document networks},
	author={Chang, J. and Blei, D.M.},
	journal={The Annals of Applied Statistics},
	volume={4},
	number={1},
	pages={124--150},
	year={2010},
	publisher={Institute of Mathematical Statistics}
}

@inproceedings{Nagappan:2010:CBD:1913797.1914387,
	author = {Nagappan, Nachiappan and Zeller, Andreas and Zimmermann, Thomas and Herzig, Kim and Murphy, Brendan},
	title = {Change Bursts as Defect Predictors},
	booktitle = {Proceedings of the 2010 IEEE 21st International Symposium on Software Reliability Engineering},
	series = {ISSRE '10},
	year = {2010},
	isbn = {978-0-7695-4255-3},
	pages = {309--318},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ISSRE.2010.25},
	doi = {10.1109/ISSRE.2010.25},
	acmid = {1914387},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {Process metrics, product metrics, software quality assurance, version control, change history, defects, developers, software mining, empirical studies},
} 

@inproceedings{Zhang:2011:CSD:2001420.2001463,
	author = {Zhang, Sai and Saff, David and Bu, Yingyi and Ernst, Michael D.},
	title = {Combined static and dynamic automated test generation},
	booktitle = {Proceedings of the 2011 International Symposium on Software Testing and Analysis},
	series = {ISSTA '11},
	year = {2011},
	isbn = {978-1-4503-0562-4},
	location = {Toronto, Ontario, Canada},
	pages = {353--363},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2001420.2001463},
	doi = {10.1145/2001420.2001463},
	acmid = {2001463},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {automated test generation, dynamic analyses, static},
} 

@article{Sebastiani:2002:MLA:505282.505283,
	author = {Sebastiani, Fabrizio},
	title = {Machine learning in automated text categorization},
	journal = {ACM Comput. Surv.},
	issue_date = {March 2002},
	volume = {34},
	number = {1},
	month = mar,
	year = {2002},
	issn = {0360-0300},
	pages = {1--47},
	numpages = {47},
	url = {http://doi.acm.org/10.1145/505282.505283},
	doi = {10.1145/505282.505283},
	acmid = {505283},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Machine learning, text categorization, text classification},
} 

@article{Jain:2010:DCY:1755267.1755654,
	author = {Jain, Anil K.},
	title = {Data clustering: 50 years beyond K-means},
	journal = {Pattern Recogn. Lett.},
	issue_date = {June, 2010},
	volume = {31},
	number = {8},
	month = jun,
	year = {2010},
	issn = {0167-8655},
	pages = {651--666},
	numpages = {16},
	url = {http://dx.doi.org/10.1016/j.patrec.2009.09.011},
	doi = {10.1016/j.patrec.2009.09.011},
	acmid = {1755654},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {Data clustering, Historical developments, King-Sun Fu prize, Perspectives on clustering, User's dilemma},
} 

@inproceedings{McMillan:2011:CSA:2117694.2119646,
	author = {McMillan, Collin and Linares-Vasquez, Mario and Poshyvanyk, Denys and Grechanik, Mark},
	title = {Categorizing software applications for maintenance},
	booktitle = {Proceedings of the 2011 27th IEEE International Conference on Software Maintenance},
	series = {ICSM '11},
	year = {2011},
	isbn = {978-1-4577-0663-9},
	pages = {343--352},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICSM.2011.6080801},
	doi = {10.1109/ICSM.2011.6080801},
	acmid = {2119646},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Luhn:1958:ACL:1662353.1662360,
	author = {Luhn, H. P.},
	title = {The automatic creation of literature abstracts},
	journal = {IBM J. Res. Dev.},
	issue_date = {April 1958},
	volume = {2},
	number = {2},
	month = apr,
	year = {1958},
	issn = {0018-8646},
	pages = {159--165},
	numpages = {7},
	url = {http://dx.doi.org/10.1147/rd.22.0159},
	doi = {10.1147/rd.22.0159},
	acmid = {1662360},
	publisher = {IBM Corp.},
	address = {Riverton, NJ, USA},
} 

@inproceedings{Goldstein:2000:MSS:1117575.1117580,
	author = {Goldstein, Jade and Mittal, Vibhu and Carbonell, Jaime and Kantrowitz, Mark},
	title = {Multi-document summarization by sentence extraction},
	booktitle = {Proceedings of the 2000 NAACL-ANLPWorkshop on Automatic summarization - Volume 4},
	series = {NAACL-ANLP-AutoSum '00},
	year = {2000},
	location = {Seattle, Washington},
	pages = {40--48},
	numpages = {9},
	url = {http://dx.doi.org/10.3115/1117575.1117580},
	doi = {10.3115/1117575.1117580},
	acmid = {1117580},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
} 

@article{Knight200291,
	title = "Summarization beyond sentence extraction: A probabilistic approach to sentence compression",
	journal = "Artificial Intelligence",
	volume = "139",
	number = "1",
	pages = "91 - 107",
	year = "2002",
	note = "",
	issn = "0004-3702",
	doi = "10.1016/S0004-3702(02)00222-9",
	url = "http://www.sciencedirect.com/science/article/pii/S0004370202002229",
	author = "Kevin Knight and Daniel Marcu",
	keywords = "Summarization",
	keywords = "Compression",
	keywords = "Noisy-channel model"
}

@inproceedings{Sridhara:2010:TAG:1858996.1859006,
	author = {Sridhara, Giriprasad and Hill, Emily and Muppaneni, Divya and Pollock, Lori and Vijay-Shanker, K.},
	title = {Towards automatically generating summary comments for Java methods},
	booktitle = {Proceedings of the IEEE/ACM international conference on Automated software engineering},
	series = {ASE '10},
	year = {2010},
	isbn = {978-1-4503-0116-9},
	location = {Antwerp, Belgium},
	pages = {43--52},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1858996.1859006},
	doi = {10.1145/1858996.1859006},
	acmid = {1859006},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {comment generation, method summarization, natural language program analysis},
}

@inproceedings{Aponte:2011:ITL:1987856.1987867,
	author = {Aponte, Jairo and Marcus, Andrian},
	title = {Improving traceability link recovery methods through software artifact summarization},
	booktitle = {Proceedings of the 6th International Workshop on Traceability in Emerging Forms of Software Engineering},
	series = {TEFSE '11},
	year = {2011},
	isbn = {978-1-4503-0589-1},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {46--49},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1987856.1987867},
	doi = {10.1145/1987856.1987867},
	acmid = {1987867},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {information retrieval, program comprehension, summarization, traceability management},
} 

@article{Powers_2011, 
	title={EVALUATION : FROM PRECISION , RECALL AND F-MEASURE TO ROC , INFORMEDNESS , MARKEDNESS \& CORRELATION}, 
	volume={2}, 
	number={1}, 
	journal={Journal of Machine Learning Technologies}, 
	author={Powers, David M W}, 
	year={2011}, 
	pages={37--63}}

@inproceedings{Grechanik:2010:SEF:1806799.1806868,
	author = {Grechanik, Mark and Fu, Chen and Xie, Qing and McMillan, Collin and Poshyvanyk, Denys and Cumby, Chad},
	title = {A search engine for finding highly relevant applications},
	booktitle = {Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering},
	series = {ICSE '10},
	year = {2010},
	isbn = {978-1-60558-719-6},
	location = {Cape Town, South Africa},
	pages = {475--484},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1806799.1806868},
	doi = {10.1145/1806799.1806868},
	acmid = {1806868},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Grechanik:2010:EIL:1852786.1852801,
	author = {Grechanik, Mark and McMillan, Collin and DeFerrari, Luca and Comi, Marco and Crespi, Stefano and Poshyvanyk, Denys and Fu, Chen and Xie, Qing and Ghezzi, Carlo},
	title = {An empirical investigation into a large-scale Java open source code repository},
	booktitle = {Proceedings of the 2010 ACM-IEEE International Symposium on Empirical Software Engineering and Measurement},
	series = {ESEM '10},
	year = {2010},
	isbn = {978-1-4503-0039-1},
	location = {Bolzano-Bozen, Italy},
	pages = {11:1--11:10},
	articleno = {11},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1852786.1852801},
	doi = {10.1145/1852786.1852801},
	acmid = {1852801},
	publisher = {ACM},
	address = {New York, NY, USA}
} 

@inproceedings{Dagenais:2010:MNS:1806799.1806842,
	author = {Dagenais, Barth{\'e}l{\'e}my and Ossher, Harold and Bellamy, Rachel K. E. and Robillard, Martin P. and de Vries, Jacqueline P.},
	title = {Moving into a new software project landscape},
	booktitle = {Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering - Volume 1},
	series = {ICSE '10},
	year = {2010},
	isbn = {978-1-60558-719-6},
	location = {Cape Town, South Africa},
	pages = {275--284},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1806799.1806842},
	doi = {10.1145/1806799.1806842},
	acmid = {1806842},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@article{vonKrogh20031217,
	title = "Community, joining, and specialization in open source software innovation: a case study",
	journal = "Research Policy",
	volume = "32",
	number = "7",
	pages = "1217 - 1241",
	year = "2003",
	note = "<ce:title>Open Source Software Development</ce:title>",
	issn = "0048-7333",
	doi = "10.1016/S0048-7333(03)00050-7",
	url = "http://www.sciencedirect.com/science/article/pii/S0048733303000507",
	author = "Georg von Krogh and Sebastian Spaeth and Karim R Lakhani",
	keywords = "Open source software",
	keywords = "Innovation",
	keywords = "Community",
	keywords = "Collective action",
	keywords = "Virtual teams"
}
@inproceedings{Schweikhardt:1982:PEB:800071.802260,
	author = {Schweikhardt, Waltraud},
	title = {A Programming Environment for Blind APL-programmers},
	booktitle = {Proceedings of the International Conference on APL},
	series = {APL '82},
	year = {1982},
	isbn = {0-89791-078-8},
	location = {Heidelberg, Germany},
	pages = {325--331},
	numpages = {7},
	url = {http://doi.acm.org/10.1145/800071.802260},
	doi = {10.1145/800071.802260},
	acmid = {802260},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Sanchez:2006:AAP:2097931.2098146,
	author = {S\'{a}nchez, Jaime and Aguayo, Fernando},
	title = {APL: Audio Programming Language for Blind Learners},
	booktitle = {Proceedings of the 10th International Conference on Computers Helping People with Special Needs},
	series = {ICCHP'06},
	year = {2006},
	isbn = {3-540-36020-4, 978-3-540-36020-9},
	location = {Linz, Austria},
	pages = {1334--1341},
	numpages = {8},
	url = {http://dx.doi.org/10.1007/11788713_192},
	doi = {10.1007/11788713_192},
	acmid = {2098146},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
}

@inproceedings{ComputerWorld2004,
	author = {Hodson, Bernard},
	booktitle = {ComputerWorld Canada},
	title = {Sixties Ushers in Program To Train Blind Programmers},
	year = {2004},
	month = {June}
}

@inproceedings{ComputerWorld1998,
	author = {Alexander, Steve},
	booktitle = {ComputerWorld},
	title = {Blind programmers face an uncertain future},
	year = {1998},
	month = {November}
}

@inproceedings{TechReview2014,
	author = {Staff},
	booktitle = {MIT Technology Review},
	title = {App Turns Smartphone Into Virtual Cane for the Blind},
	year = {2014},
	month = {January}
}

@inproceedings{blum2011s,
	title={What’s around me? Spatialized audio augmented reality for blind users with a smartphone},
	author={Blum, Jeffrey R and Bouchard, Mathieu and Cooperstock, Jeremy R},
	booktitle={International Conference on Mobile and Ubiquitous Systems: Computing, Networking, and Services},
	pages={49--62},
	year={2011},
	organization={Springer}
}

@inproceedings{lopez2011indoor,
	title={Indoor navigation and product recognition for blind people assisted shopping},
	author={L{\'o}pez-de-Ipi{\~n}a, Diego and Lorido, Tania and L{\'o}pez, Unai},
	booktitle={International Workshop on Ambient Assisted Living},
	pages={33--40},
	year={2011},
	organization={Springer}
}

@inproceedings{HigherEd2010,
	author = {Parry, Marc},
	booktitle = {Chronicle of Higher Education},
	title = {Colleges Lock Out Blind Students Online},
	year = {2010},
	month = {December}
}

@inproceedings{ED2014,
	author = {Liana Heitin},
	booktitle = {Education Week},
	title = {Computer Science: Not Just an Elective Anymore},
	year = {2014},
	month = {February}
}

@inproceedings{CT2013,
	author = {Lauren Zumbach},
	booktitle = {Chicago Tribune},
	title = {CPS making computer science core subject},
	year = {2013},
	month = {December}
}

@article{abner2002implementation,
	title={Implementation of Assistive Technology with Students Who Are Visually Impaired: Teachers' Readiness.},
	author={Abner, Gerald H and Lahm, Elizabeth A},
	journal={Journal of Visual Impairment \& Blindness},
	volume={96},
	number={2},
	year={2002}
}

@article{supalo2009using,
	title={Using adaptive tools and techniques to teach a class of students who are blind or low-vision},
	author={Supalo, Cary A and Mallouk, Thomas E and Amorosi, Christeallia and Lanouette, James and Wohlers, H David and McEnnis, Kathleen},
	journal={Journal of Chemical Education},
	volume={86},
	number={5},
	pages={587},
	year={2009},
	publisher={ACS Publications}
}

@inproceedings{AP2008,
	author = {David Crary},
	booktitle = {Associated Press},
	title = {Employer Bias Thwarts Many Blind Workers},
	year = {2008},
	month = {May}
}

@inproceedings{BM2009,
	author = {James Nyman},
	booktitle = {Braille Monitor},
	title = {Unemployment Rates and Reasons},
	year = {2009},
	month = {March}
}

@article{Glinert:1992:CPD:129875.129876,
	author = {Glinert, Ephraim P. and York, Bryant W.},
	title = {Computers and People with Disabilities},
	journal = {Commun. ACM},
	issue_date = {May 1992},
	volume = {35},
	number = {5},
	month = may,
	year = {1992},
	issn = {0001-0782},
	pages = {32--35},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/129875.129876},
	doi = {10.1145/129875.129876},
	acmid = {129876},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Blenkhorn199817,
	title = "Using speech and touch to enable blind people to access schematic diagrams ",
	journal = "Journal of Network and Computer Applications ",
	volume = "21",
	number = "1",
	pages = "17 - 29",
	year = "1998",
	note = "",
	issn = "1084-8045",
	doi = "http://dx.doi.org/10.1006/jnca.1998.0060",
	url = "http://www.sciencedirect.com/science/article/pii/S1084804598900601",
	author = "P. Blenkhorn and D.G. Evans"
}

@misc{ResourcesNIST,
	author = {National Institute of Standards and Technology},
	title = {Multiple Biometric Grand Challenge},
	month = Jan,
	year = {2014},
	note = {http://face.nist.gov/mbgc/}
}

@misc{ResourcesCONDOR,
	author = {University of Notre Dame Department of Computer Science},
	title = {CCL Condor Pool},
	month = Jan,
	year = {2014},
	note = {http://www.cse.nd.edu/~ccl/operations/condor/}
}

@misc{ResourcesNWICG,
	author = {Northwest Indiana Computational Grid},
	title = {High-Capacity Network Connectivity},
	month = Jan,
	year = {2014},
	note = {http://www.nwicgrid.org/}
}

@misc{MS:Blind:Website,
	author = {Microsoft},
	title = {Windows XP Accessibility},
	month = Jan,
	year = {2014},
	note = {http://support.microsoft.com/kb/308978}
}

@inproceedings{Kane:2011:AOI:2047196.2047232,
	author = {Kane, Shaun K. and Morris, Meredith Ringel and Perkins, Annuska Z. and Wigdor, Daniel and Ladner, Richard E. and Wobbrock, Jacob O.},
	title = {Access Overlays: Improving Non-visual Access to Large Touch Screens for Blind Users},
	booktitle = {Proceedings of the 24th Annual ACM Symposium on User Interface Software and Technology},
	series = {UIST '11},
	year = {2011},
	isbn = {978-1-4503-0716-1},
	location = {Santa Barbara, California, USA},
	pages = {273--282},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/2047196.2047232},
	doi = {10.1145/2047196.2047232},
	acmid = {2047232},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {accessibility, blindness, touch screens, visual impairments},
} 

@incollection{Gross09,
	year={2009},
	isbn={978-3-642-03654-5},
	booktitle={Human-Computer Interaction – INTERACT 2009},
	volume={5726},
	series={Lecture Notes in Computer Science},
	editor={Gross, Tom and Gulliksen, Jan and Kotzé, Paula and Oestreicher, Lars and Palanque, Philippe and Prates, RaquelOliveira and Winckler, Marco},
	doi={10.1007/978-3-642-03655-2_41},
	title={What’s Next? A Visual Editor for Correcting Reading Order},
	url={http://dx.doi.org/10.1007/978-3-642-03655-2_41},
	publisher={Springer Berlin Heidelberg},
	keywords={Reading flow; reading order; Web accessibility; ARIA flowto},
	author={Sato, Daisuke and Kobayashi, Masatomo and Takagi, Hironobu and Asakawa, Chieko},
	pages={364-377}
}

@inproceedings{Sanchez:2005:BLP:1056808.1057018,
	author = {S\'{a}nchez, Jaime and Aguayo, Fernando},
	title = {Blind Learners Programming Through Audio},
	booktitle = {CHI '05 Extended Abstracts on Human Factors in Computing Systems},
	series = {CHI EA '05},
	year = {2005},
	isbn = {1-59593-002-7},
	location = {Portland, OR, USA},
	pages = {1769--1772},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1056808.1057018},
	doi = {10.1145/1056808.1057018},
	acmid = {1057018},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {audio-based navigation, blind children, spatialized sound, usability, virtual acoustic environments},
}

@inproceedings{LaToza:2006:MMM:1134285.1134355,
	author = {LaToza, Thomas D. and Venolia, Gina and DeLine, Robert},
	title = {Maintaining mental models: a study of developer work habits},
	booktitle = {Proceedings of the 28th international conference on Software engineering},
	series = {ICSE '06},
	year = {2006},
	isbn = {1-59593-375-1},
	location = {Shanghai, China},
	pages = {492--501},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1134285.1134355},
	doi = {10.1145/1134285.1134355},
	acmid = {1134355},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {agile software development, code duplication, code ownership, communication, debugging, interruptions},
}

@inproceedings{Armaly:ICSE:2014,
	author = {Armaly, Ameer and Ferris, Casey and McMillan, Collin},
	title = {Reusable Execution Replay: Execution Record and Replay for Source Code Reuse},
	booktitle = {Proceedings of the 36th international conference on Software engineering, New Ideas and Emerging Results Track},
	series = {ICSE NIER'14},
	year = {2014},
	location = {Hyderabad, India},
	numpages = {4},
	note = {To appear}
}

@inproceedings{CruzTraceLab2016,
	author = {Cruz, Breno and McBurney, Paul and McMillan, Collin},
	title = {TraceLab Components for Reproducing Source Code Summarization Experiments},
	booktitle = {Proceedings of the 32nd international conference on software maintenance and evolution, artifacts track},
	series = {ICSME'16},
	year = {2016},
	location = {Raleigh, NC, USA}
}

@inproceedings{McBurney:ICPC:2014,
	author = {McBurney, Paul W. and McMillan, Collin},
	title = {Automatic Documentation Generation via Source Code Summarization of Method Context},
	booktitle = {Proceedings of the 22nd international conference on program comprehension},
	series = {ICPC'14},
	year = {2014},
	location = {Hyderabad, India},
	numpages = {12}
}

@inproceedings{McBurney:ICPCERA:2014,
	author = {McBurney, Paul W. and Liu, Cheng and McMillan, Collin and Weninger, Tim},
	title = {Improving Topic Model Source Code Summarization},
	booktitle = {Proceedings of the 22nd international conference on program comprehension},
	series = {ICPC '14},
	year = {2014},
	location = {Hyderabad, India},
	numpages = {12},
	note = {To appear}
}

@ARTICLE{7118751,
	author={P. Rodeghero and C. Liu and P. W. McBurney and C. McMillan},
	journal={IEEE Transactions on Software Engineering},
	title={An Eye-Tracking Study of Java Programmers and Application to Source Code Summarization},
	year={2015},
	volume={41},
	number={11},
	pages={1038-1054},
	keywords={Java;program compilers;source code (software);Java programmer;code generation;eye-tracking study;source code summarization;Documentation;Java;Navigation;Software;Software engineering;XML;Source code summaries;program comprehension},
	doi={10.1109/TSE.2015.2442238},
	ISSN={0098-5589},
	month={Nov},}

@inproceedings{Rodeghero:ICSE:2014,
	author = {Rodeghero, Paige and McMillan, Collin and McBurney, Paul W. and Bosch, Nigel and D'Mello, Sidney},
	title = {Improving Automated Source Code Summarization via an Eye-Tracking Study of Programmers},
	booktitle = {Proceedings of the 36th international conference on Software engineering},
	series = {ICSE '14},
	year = {2014},
	location = {Hyderabad, India},
	numpages = {12},
	note = {To appear}
}

@inproceedings{Khambadkar:2013:GGI:2501988.2502047,
	author = {Khambadkar, Vinitha and Folmer, Eelke},
	title = {GIST: A Gestural Interface for Remote Nonvisual Spatial Perception},
	booktitle = {Proceedings of the 26th Annual ACM Symposium on User Interface Software and Technology},
	series = {UIST '13},
	year = {2013},
	isbn = {978-1-4503-2268-3},
	location = {St. Andrews, Scotland, United Kingdom},
	pages = {301--310},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/2501988.2502047},
	doi = {10.1145/2501988.2502047},
	acmid = {2502047},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {gestures, spatial perception, visual impairment},
}

@inproceedings{Franqueiro:2006:DSL:1168987.1169035,
	author = {Franqueiro, Kenneth G. and Siegfried, Robert M.},
	title = {Designing a Scripting Language to Help the Blind Program Visually},
	booktitle = {Proceedings of the 8th International ACM SIGACCESS Conference on Computers and Accessibility},
	series = {Assets '06},
	year = {2006},
	isbn = {1-59593-290-9},
	location = {Portland, Oregon, USA},
	pages = {241--242},
	numpages = {2},
	url = {http://doi.acm.org/10.1145/1168987.1169035},
	doi = {10.1145/1168987.1169035},
	acmid = {1169035},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {blind programmers, graphical user interfaces, visual basic, visual programming},
}


@inproceedings{Steidl:2013:ICPC,
	author = {Steidl, Daniela and Hummel, Benjamin and Juergens, Elmar},
	title = {Quality Analysis of Source Code Comments},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	year = {2013},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@inproceedings{Smucker:07,
	author = {Smucker, Mark D. and Allan, James and Carterette, Ben},
	title = {A comparison of statistical significance tests for information retrieval evaluation},
	booktitle = {CIKM},
	year = {2007},
	pages = {623--632}
}

@inproceedings{Fagin:2003:CTK:644108.644113,
	author = {Fagin, Ronald and Kumar, Ravi and Sivakumar, D.},
	title = {Comparing top k lists},
	booktitle = {Proceedings of the fourteenth annual ACM-SIAM symposium on Discrete algorithms},
	series = {SODA '03},
	year = {2003},
	isbn = {0-89871-538-5},
	location = {Baltimore, Maryland},
	pages = {28--36},
	numpages = {9},
	url = {http://dl.acm.org/citation.cfm?id=644108.644113},
	acmid = {644113},
	publisher = {Society for Industrial and Applied Mathematics},
	address = {Philadelphia, PA, USA},
}

@article{Bansal:2009:CDP:1480540.1480730,
	author = {Bansal, Mukul S. and Fern\'{a}ndez-Baca, David},
	title = {Computing distances between partial rankings},
	journal = {Inf. Process. Lett.},
	issue_date = {January, 2009},
	volume = {109},
	number = {4},
	month = jan,
	year = {2009},
	issn = {0020-0190},
	pages = {238--241},
	numpages = {4},
	url = {http://dx.doi.org/10.1016/j.ipl.2008.10.010},
	doi = {10.1016/j.ipl.2008.10.010},
	acmid = {1480730},
	publisher = {Elsevier North-Holland, Inc.},
	address = {Amsterdam, The Netherlands, The Netherlands},
	keywords = {Algorithms, Kendall tau distance, Partial rankings, Top-m lists, p-ratings},
}

@article{wolfe1973nonparametric,
	title={Nonparametric statistical methods},
	author={Wolfe, Douglas A and Hollander, Myles},
	journal={Nonparametric statistical methods},
	publisher={John Wiley New York}
}

@article{BBS:209012,
	author = {Rayner,Keith and Pollatsek,Alexander and Reichle,Erik D.},
	title = {Eye movements in reading: Models and data},
	journal = {Behavioral and Brain Sciences},
	volume = {26},
	issue = {04},
	month = {7},
	year = {2003},
	issn = {1469-1825},
	pages = {507--518},
	numpages = {12},
	doi = {10.1017/S0140525X03520106},
	URL = {http://journals.cambridge.org/article_S0140525X03520106},
}

@inproceedings{SaiZhang:2011:ADI:2190078.2190153,
	author = {Sai Zhang and Cheng Zhang and Ernst, Michael D.},
	title = {Automated documentation inference to explain failed tests},
	booktitle = {Proceedings of the 2011 26th IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '11},
	year = {2011},
	isbn = {978-1-4577-1638-6},
	pages = {63--72},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ASE.2011.6100145},
	doi = {10.1109/ASE.2011.6100145},
	acmid = {2190153},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@PhdThesis{MurphyPhd96,
	title = "{Lightweight structural summarization as an aid to software evolution}",
	author = "Gail C. Murphy",
	school = "University of Washington",
	month = "July",
	year = "1996",
}

@inproceedings{Buse:2008:ADI:1390630.1390664,
	author = {Buse, Raymond P.L. and Weimer, Westley R.},
	title = {Automatic documentation inference for exceptions},
	booktitle = {Proceedings of the 2008 international symposium on Software testing and analysis},
	series = {ISSTA '08},
	isbn = {978-1-60558-050-0},
	location = {Seattle, WA, USA},
	pages = {273--282},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1390630.1390664},
	doi = {10.1145/1390630.1390664},
	acmid = {1390664},
	keywords = {documentation inference, exception handling, software documentation},
}

@inproceedings{Buse:2010:ADP:1858996.1859005,
	author = {Buse, Raymond P.L. and Weimer, Westley R.},
	title = {Automatically documenting program changes},
	booktitle = {Proceedings of the IEEE/ACM international conference on Automated software engineering},
	series = {ASE '10},
	isbn = {978-1-4503-0116-9},
	location = {Antwerp, Belgium},
	pages = {33--42},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1858996.1859005},
	doi = {10.1145/1858996.1859005},
	acmid = {1859005},
	keywords = {code summarization, commit messages, differencing},
}

@ARTICLE{6165314,
	author={Miryung Kim and Notkin, D. and Grossman, D. and Wilson, G.},
	journal={IEEE Transactions on Software Engineering},
	title={Identifying and Summarizing Systematic Code Changes via Rule Inference},
	year={2013},
	month={Jan. },
	volume={39},
	number={1},
	pages={45 -62},
	doi={10.1109/TSE.2012.16},
	ISSN={0098-5589},
}

@inproceedings{Aponte:2011:ITL:1987856.1987867,
	author = {Aponte, Jairo and Marcus, Andrian},
	title = {Improving traceability link recovery methods through software artifact summarization},
	booktitle = {Proceedings of the 6th International Workshop on Traceability in Emerging Forms of Software Engineering},
	series = {TEFSE '11},
	year = {2011},
	isbn = {978-1-4503-0589-1},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {46--49},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1987856.1987867},
	doi = {10.1145/1987856.1987867},
	acmid = {1987867},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {information retrieval, program comprehension, summarization, traceability management},
}

@article{Crosby:1990:WRA:77577.77580,
	author = {Crosby, Martha E. and Stelovsky, Jan},
	title = {How Do We Read Algorithms? A Case Study},
	journal = {Computer},
	issue_date = {January 1990},
	volume = {23},
	number = {1},
	month = jan,
	issn = {0018-9162},
	pages = {24--35},
	numpages = {12},
	url = {http://dl.acm.org/citation.cfm?id=77577.77580},
	acmid = {77580},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{Bednarik:2006:EMC:1117309.1117356,
	author = {Bednarik, Roman and Tukiainen, Markku},
	title = {An eye-tracking methodology for characterizing program comprehension processes},
	booktitle = {Proceedings of the 2006 symposium on Eye tracking research \& applications},
	series = {ETRA '06},
	year = {2006},
	isbn = {1-59593-305-0},
	location = {San Diego, California},
	pages = {125--132},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1117309.1117356},
	doi = {10.1145/1117309.1117356},
	acmid = {1117356},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {eye-movement tracking methodology, program comprehension, program visualization, psychology of programming},
} 

@inproceedings{Sharif:2012:ESR:2168556.2168642,
	author = {Sharif, Bonita and Falcone, Michael and Maletic, Jonathan I.},
	title = {An eye-tracking study on the role of scan time in finding source code defects},
	booktitle = {Proceedings of the Symposium on Eye Tracking Research and Applications},
	series = {ETRA '12},
	year = {2012},
	isbn = {978-1-4503-1221-9},
	location = {Santa Barbara, California},
	pages = {381--384},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/2168556.2168642},
	doi = {10.1145/2168556.2168642},
	acmid = {2168642},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {eye-tracking study, software defects, source-code review},
} 

@inproceedings{Sharif:2011:EAU:2117694.2119672,
	author = {Sharif, Bonita},
	title = {Empirical assessment of UML class diagram layouts based on architectural importance},
	booktitle = {Proceedings of the 2011 27th IEEE International Conference on Software Maintenance},
	series = {ICSM '11},
	year = {2011},
	isbn = {978-1-4577-0663-9},
	pages = {544--549},
	numpages = {6},
	url = {http://dx.doi.org/10.1109/ICSM.2011.6080828},
	doi = {10.1109/ICSM.2011.6080828},
	acmid = {2119672},
	address = {Washington, DC, USA},
} 

@inproceedings{Sharif:2010:ELD:1796177.1796642,
	author = {Sharif, Bonita and Maletic, Jonathan I.},
	title = {The Effects of Layout on Detecting the Role of Design Patterns},
	booktitle = {Proceedings of the 2010 23rd IEEE Conference on Software Engineering Education and Training},
	series = {CSEET '10},
	year = {2010},
	isbn = {978-0-7695-4054-2},
	pages = {41--48},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/CSEET.2010.23},
	acmid = {1796642},
	address = {Washington, DC, USA},
} 

@article{Binkley:2013:IIS:2436118.2436136,
	author = {Binkley, Dave and Davis, Marcia and Lawrie, Dawn and Maletic, Jonathan I. and Morrell, Christopher and Sharif, Bonita},
	title = {The impact of identifier style on effort and comprehension},
	journal = {Empirical Softw. Engg.},
	issue_date = {April     2013},
	volume = {18},
	number = {2},
	month = apr,
	year = {2013},
	issn = {1382-3256},
	pages = {219--276},
	numpages = {58},
	url = {http://dx.doi.org/10.1007/s10664-012-9201-4},
	doi = {10.1007/s10664-012-9201-4},
	acmid = {2436136},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Code readability, Coding standards, Eye-tracking study, Identifier names, Identifier styles, Memory, Program comprehension, Text recognition},
} 

@inproceedings{Sharif:2010:ETS:1846454.1847968,
	author = {Sharif, Bonita and Maletic, Jonathan I.},
	title = {An Eye Tracking Study on camelCase and under\_score Identifier Styles},
	booktitle = {Proceedings of the 2010 IEEE 18th International Conference on Program Comprehension},
	series = {ICPC '10},
	year = {2010},
	isbn = {978-0-7695-4113-6},
	pages = {196--205},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICPC.2010.41},
	doi = {10.1109/ICPC.2010.41},
	acmid = {1847968},
	address = {Washington, DC, USA},
	keywords = {identifier styles, eye-tracking study, code readability},
} 

@inproceedings{Bednarik:2008:TED:1344471.1344497,
	author = {Bednarik, Roman and Tukiainen, Markku},
	title = {Temporal eye-tracking data: evolution of debugging strategies with multiple representations},
	booktitle = {Proceedings of the 2008 symposium on Eye tracking research \&\#38; applications},
	series = {ETRA '08},
	year = {2008},
	isbn = {978-1-59593-982-1},
	location = {Savannah, Georgia},
	pages = {99--102},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1344471.1344497},
	doi = {10.1145/1344471.1344497},
	acmid = {1344497},
	address = {New York, NY, USA},
}

@inproceedings{Uwano:2006:AIP:1117309.1117357,
	author = {Uwano, Hidetake and Nakamura, Masahide and Monden, Akito and Matsumoto, Ken-ichi},
	title = {Analyzing individual performance of source code review using reviewers' eye movement},
	booktitle = {Proceedings of the 2006 symposium on Eye tracking research \& applications},
	series = {ETRA '06},
	year = {2006},
	isbn = {1-59593-305-0},
	location = {San Diego, California},
	pages = {133--140},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1117309.1117357},
	doi = {10.1145/1117309.1117357},
	acmid = {1117357},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {computer program, eye movement, human factor, source code review},
} 

@inproceedings{LaToza:2006:MMM:1134285.1134355,
	author = {LaToza, Thomas D. and Venolia, Gina and DeLine, Robert},
	title = {Maintaining mental models: a study of developer work habits},
	booktitle = {Proceedings of the 28th international conference on Software engineering},
	series = {ICSE '06},
	year = {2006},
	isbn = {1-59593-375-1},
	location = {Shanghai, China},
	pages = {492--501},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1134285.1134355},
	doi = {10.1145/1134285.1134355},
	acmid = {1134355},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {agile software development, code duplication, code ownership, communication, debugging, interruptions},
}

@inproceedings{Guzzi:2012:DSK:2337223.2337476,
	author = {Guzzi, Anja},
	title = {Documenting and sharing knowledge about code},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {1535--1538},
	numpages = {4},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337476},
	acmid = {2337476},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@inproceedings{Brandt:2010:EPI:1753326.1753402,
	author = {Brandt, Joel and Dontcheva, Mira and Weskamp, Marcos and Klemmer, Scott R.},
	title = {Example-centric programming: integrating web search into the development environment},
	booktitle = {Proceedings of the 28th international conference on Human factors in computing systems},
	series = {CHI '10},
	year = {2010},
	isbn = {978-1-60558-929-9},
	location = {Atlanta, Georgia, USA},
	pages = {513--522},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1753326.1753402},
	doi = {10.1145/1753326.1753402},
	acmid = {1753402},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {example-centric development},
}

@inproceedings{Kotonya:2008:ORL:1478087.1478113,
	author = {Kotonya, Gerald and Lock, Simon and Mariani, John},
	title = {Opportunistic Reuse: Lessons from Scrapheap Software Development},
	booktitle = {Proceedings of the 11th International Symposium on Component-Based Software Engineering},
	series = {CBSE '08},
	year = {2008},
	isbn = {978-3-540-87890-2},
	location = {Karlsruhe, Germany},
	pages = {302--309},
	numpages = {8},
	url = {http://dx.doi.org/10.1007/978-3-540-87891-9_20},
	doi = {10.1007/978-3-540-87891-9_20},
	acmid = {1478113},
	address = {Berlin, Heidelberg},
}

@ARTICLE{Davison00understandingand,
	author = {Joseph W. Davison and Dennis M. Mancl and William F. Opdyke},
	title = {Understanding and addressing the essential costs of evolving systems},
	journal = {Bell Labs Technical Journal},
	year = {2000},
	pages = {44--54}
}

@inproceedings{Mirghasemi:2011:QMB:2025113.2025184,
	author = {Mirghasemi, Salman and Barton, John J. and Petitpierre, Claude},
	title = {Querypoint: moving backwards on wrong values in the buggy execution},
	booktitle = {Proceedings of the 19th ACM SIGSOFT symposium and the 13th European conference on Foundations of software engineering},
	series = {ESEC/FSE '11},
	isbn = {978-1-4503-0443-6},
	location = {Szeged, Hungary},
	pages = {436--439},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/2025113.2025184},
	doi = {10.1145/2025113.2025184},
	acmid = {2025184},
	address = {New York, NY, USA},
	keywords = {breakpoint, debugging, lastchange, locating defects, logging, querypoint, watchpoint},
}

@article{Douce91,
	author = {Douce, C.},
	title = {Long Term Comprehension of Software Systems: A Methodology for Study},
	journal = {Proc. Psychology of Programming Interest Group},
	year = {2001}
}

@inproceedings{Gonzalez:2004:CCM:985692.985707,
	author = {Gonz\'{a}lez, Victor M. and Mark, Gloria},
	title = {"Constant, constant, multi-tasking craziness": managing multiple working spheres},
	booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
	series = {CHI '04},
	year = {2004},
	isbn = {1-58113-702-8},
	location = {Vienna, Austria},
	pages = {113--120},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/985692.985707},
	doi = {10.1145/985692.985707},
	acmid = {985707},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {attention management, empirical study, information overload, interruptions, personal information management},
} 

@inproceedings{Kramer:2012:BLA:2337223.2337451,
	author = {Kr\"{a}mer, Jan-Peter and Kurz, Joachim and Karrer, Thorsten and Borchers, Jan},
	title = {Blaze},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {1457--1458},
	numpages = {2},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337451},
	acmid = {2337451},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@article{ALTMANN2001189,
	title = "Near-term memory in programming: a simulation-based analysis ",
	journal = "International Journal of Human-Computer Studies ",
	volume = "54",
	number = "2",
	pages = "189 - 210",
	year = "2001",
	note = "",
	issn = "1071-5819",
	doi = "http://dx.doi.org/10.1006/ijhc.2000.0407",
	url = "http://www.sciencedirect.com/science/article/pii/S1071581900904075",
	author = "Erik M. Altmann"
}

@article{Holmes:2013:SPS:2377656.2377657,
	author = {Holmes, Reid and Walker, Robert J.},
	title = {Systematizing pragmatic software reuse},
	journal = {ACM Trans. Softw. Eng. Methodol.},
	issue_date = {November 2012},
	volume = {21},
	number = {4},
	month = feb,
	year = {2013},
	issn = {1049-331X},
	pages = {20:1--20:44},
	articleno = {20},
	numpages = {44},
	url = {http://doi.acm.org/10.1145/2377656.2377657},
	doi = {10.1145/2377656.2377657},
	acmid = {2377657},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Gilligan, Software reuse, lightweight process and tooling, low commitment, planning, pragmatic software reuse, pragmatic-reuse plan enactment, pragmatic-reuse plans, source code investigation, white box reuse},
}

@article{Littman1987341,
	title = "Mental models and software maintenance ",
	journal = "Journal of Systems and Software ",
	volume = "7",
	number = "4",
	pages = "341 - 355",
	year = "1987",
	note = "",
	issn = "0164-1212",
	doi = "http://dx.doi.org/10.1016/0164-1212(87)90033-1",
	url = "http://www.sciencedirect.com/science/article/pii/0164121287900331",
	author = "David C. Littman and Jeannine Pinto and Stanley Letovsky and Elliot Soloway"
}

@article{Ko200541,
	title = "A framework and methodology for studying the causes of software errors in programming systems ",
	journal = "Journal of Visual Languages and Computing ",
	volume = "16",
	number = "1–2",
	pages = "41 - 84",
	year = "2005",
	issn = "1045-926X",
	doi = "http://dx.doi.org/10.1016/j.jvlc.2004.08.003",
	url = "http://www.sciencedirect.com/science/article/pii/S1045926X04000394",
	author = "Andrew J. Ko and Brad A. Myers"
}

@inproceedings{Dearman:2005:ACV:1058432.1059367,
	author = {Dearman, David and Cox, Anthony and Fisher, Maryanne},
	title = {Adding Control-Flow to a Visual Data-Flow Representation},
	booktitle = {Proceedings of the 13th International Workshop on Program Comprehension},
	series = {IWPC '05},
	year = {2005},
	isbn = {0-7695-2254-8},
	pages = {297--306},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/WPC.2005.5},
	doi = {10.1109/WPC.2005.5},
	acmid = {1059367},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Eddy:2013:ICPC,
	author = {Eddy, Brian and Robinson, Jeffrey and Kraft, Nicholas and Carver, Jeffrey},
	title = {Evaluating Source Code Summarization Techniques: Replication and Expansion},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	year = {2013},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@article{Freeman:2003:RDF:903893.903930,
	author = {Freeman, Lee A.},
	title = {A refresher in data flow diagramming: an effective aid for analysts},
	journal = {Commun. ACM},
	issue_date = {September 2003},
	volume = {46},
	number = {9},
	month = sep,
	year = {2003},
	issn = {0001-0782},
	pages = {147--151},
	numpages = {5},
	url = {http://doi.acm.org/10.1145/903893.903930},
	doi = {10.1145/903893.903930},
	acmid = {903930},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@incollection{Anderson:1992,
	year={1992},
	isbn={978-3-540-55606-0},
	booktitle={Intelligent Tutoring Systems},
	volume={608},
	series={Lecture Notes in Computer Science},
	editor={Frasson, Claude and Gauthier, Gilles and McCalla, GordonI.},
	doi={10.1007/3-540-55606-0_68},
	title={The advantages of data flow diagrams for beginning programming},
	url={http://dx.doi.org/10.1007/3-540-55606-0_68},
	publisher={Springer Berlin Heidelberg},
	author={Anjaneyulu, K.S.R. and Anderson, JohnR.},
	pages={585-592}
}

@article{Ko:2006:ESD:1248728.1248780,
	author = {Ko, Andrew J. and Myers, Brad A. and Coblenz, Michael J. and Aung, Htet Htet},
	title = {An Exploratory Study of How Developers Seek, Relate, and Collect Relevant Information during Software Maintenance Tasks},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {December 2006},
	volume = {32},
	number = {12},
	month = dec,
	year = {2006},
	issn = {0098-5589},
	pages = {971--987},
	numpages = {17},
	url = {http://dx.doi.org/10.1109/TSE.2006.116},
	doi = {10.1109/TSE.2006.116},
	acmid = {1248780},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Program investigation, Program investigation, program understanding, program comprehension, empirical software engineering, information foraging, information scent., empirical software engineering, information foraging, information scent., program comprehension, program understanding},
}

@inproceedings{Singer:1997:ESE:782010.782031,
	author = {Singer, Janice and Lethbridge, Timothy and Vinson, Norman and Anquetil, Nicolas},
	title = {An examination of software engineering work practices},
	booktitle = {Proceedings of the 1997 conference of the Centre for Advanced Studies on Collaborative research},
	series = {CASCON '97},
	year = {1997},
	location = {Toronto, Ontario, Canada},
	pages = {21--},
	url = {http://dl.acm.org/citation.cfm?id=782010.782031},
	acmid = {782031},
	publisher = {IBM Press},
}

@article{Lakhotia:1993:USE:177728.177735,
	author = {Lakhotia, Arun},
	title = {Understanding someone else's code: analysis of experiences},
	journal = {J. Syst. Softw.},
	issue_date = {Dec. 1993},
	volume = {23},
	number = {3},
	issn = {0164-1212},
	pages = {269--275},
	numpages = {7},
	url = {http://dx.doi.org/10.1016/0164-1212(93)90101-3},
	doi = {10.1016/0164-1212(93)90101-3},
	acmid = {177735},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
}

@inproceedings{fjeldstadt83,
	author = {Fjeldstad, R. K. and Hamlen, W. T.},
	booktitle = {Proceedings GUIDE 48},
	citeulike-article-id = {6922207},
	keywords = {maintenance},
	location = {Philadelphia, PA},
	month = apr,
	posted-at = {2010-03-27 23:13:35},
	priority = {2},
	title = {{Application Program Maintenance Study: Report to Our Respondents}},
	year = {1983}
}

@inproceedings{Roehm:2012:PDC:2337223.2337254,
	author = {Roehm, Tobias and Tiarks, Rebecca and Koschke, Rainer and Maalej, Walid},
	title = {How do professional developers comprehend software?},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {255--265},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337254},
	acmid = {2337254},
} 

@inproceedings{Stylos:2006:MWT:1174509.1174678,
	author = {Stylos, Jeffrey and Myers, Brad A.},
	title = {Mica: A Web-Search Tool for Finding API Components and Examples},
	booktitle = {Proceedings of the Visual Languages and Human-Centric Computing},
	series = {VLHCC '06},
	year = {2006},
	isbn = {0-7695-2586-5},
	pages = {195--202},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/VLHCC.2006.32},
	doi = {10.1109/VLHCC.2006.32},
	acmid = {1174678},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@ARTICLE{1241364,
	author={Lethbridge, T.C. and Singer, J. and Forward, A.},
	journal={Software, IEEE},
	title={How software engineers use documentation: the state of the practice},
	year={2003},
	volume={20},
	number={6},
	pages={35-39},
	keywords={software engineering;system documentation;decision making;documentation update;documentation use;software engineering;software engineers;software process managers;software process personnel;tool design;Data engineering;Documentation;Humans;Maintenance engineering;Power engineering and energy;Software engineering;Software maintenance;Software systems;Software testing;System testing},
	doi={10.1109/MS.2003.1241364},
	ISSN={0740-7459}
}

@inproceedings{Forward:2002:RSD:585058.585065,
	author = {Forward, Andrew and Lethbridge, Timothy C.},
	title = {The relevance of software documentation, tools and technologies: a survey},
	booktitle = {Proceedings of the 2002 ACM symposium on Document engineering},
	series = {DocEng '02},
	year = {2002},
	isbn = {1-58113-594-7},
	location = {McLean, Virginia, USA},
	pages = {26--33},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/585058.585065},
	doi = {10.1145/585058.585065},
	acmid = {585065},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation relevance, documentation survey, documentation technologies, program comprehension, software documentation, software engineering, software maintenance},
} 

@inproceedings{Gweon:2007:EAT:1308174.1308329,
	author = {Gweon, G. and Bergman, L. and Castelli, V. and Bellamy, R. K. E.},
	title = {Evaluating an Automated Tool to Assist Evolutionary Document Generation},
	booktitle = {Proceedings of the IEEE Symposium on Visual Languages and Human-Centric Computing},
	series = {VLHCC '07},
	year = {2007},
	isbn = {0-7695-2987-9},
	pages = {243--248},
	numpages = {6},
	url = {http://dx.doi.org/10.1109/VLHCC.2007.20},
	doi = {10.1109/VLHCC.2007.20},
	acmid = {1308329},
	address = {Washington, DC, USA},
} 

@inproceedings{Bergman:2005:DSA:1095034.1095067,
	author = {Bergman, Lawrence and Castelli, Vittorio and Lau, Tessa and Oblinger, Daniel},
	title = {DocWizards: a system for authoring follow-me documentation wizards},
	booktitle = {Proceedings of the 18th annual ACM symposium on User interface software and technology},
	series = {UIST '05},
	year = {2005},
	isbn = {1-59593-271-2},
	location = {Seattle, WA, USA},
	pages = {191--200},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1095034.1095067},
	doi = {10.1145/1095034.1095067},
	acmid = {1095067},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation generation, programming-by-demonstration},
} 

@inproceedings{5306335,
	author={Starke, J. and Luce, C. and Sillito, J.},
	booktitle={Software Maintenance, 2009. ICSM 2009. IEEE International Conference on},
	title={Searching and skimming: An exploratory study},
	year={2009},
	pages={157-166},
	keywords={software engineering;program comprehension;software system;source code search tools;Concrete;Data analysis;Information analysis;Java;Laboratories;Navigation;Programming profession;Software design;Software systems;Software tools},
	doi={10.1109/ICSM.2009.5306335},
	ISSN={1063-6773}
}

@inproceedings{Kramer:1999:ADS:318372.318577,
	author = {Kramer, Douglas},
	title = {API documentation from source code comments: a case study of Javadoc},
	booktitle = {Proceedings of the 17th annual international conference on Computer documentation},
	series = {SIGDOC '99},
	year = {1999},
	isbn = {1-58113-072-4},
	location = {New Orleans, Louisiana, USA},
	pages = {147--153},
	numpages = {7},
	url = {http://doi.acm.org/10.1145/318372.318577},
	doi = {10.1145/318372.318577},
	acmid = {318577},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {API documentation, Java platform, Javadoc, doc comments, doclets, documentation comments, generated documentation, source code comments},
} 

@inproceedings{deSouza:2005:SDE:1085313.1085331,
	author = {de Souza, Sergio Cozzetti B. and Anquetil, Nicolas and de Oliveira, K\'{a}thia M.},
	title = {A study of the documentation essential to software maintenance},
	booktitle = {Proceedings of the 23rd annual international conference on Design of communication: documenting \& designing for pervasive information},
	series = {SIGDOC '05},
	year = {2005},
	isbn = {1-59593-175-9},
	location = {Coventry, United Kingdom},
	pages = {68--75},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1085313.1085331},
	doi = {10.1145/1085313.1085331},
	acmid = {1085331},
	address = {New York, NY, USA},
	keywords = {empirical study, program understanding, software maintenance, software system documentation},
}

@article{Kajko-Mattsson:2005:SDP:1032622.1035374,
	author = {Kajko-Mattsson, Mira},
	title = {A Survey of Documentation Practice within Corrective Maintenance},
	journal = {Empirical Softw. Engg.},
	issue_date = {January 2005},
	volume = {10},
	number = {1},
	month = jan,
	year = {2005},
	issn = {1382-3256},
	pages = {31--55},
	numpages = {25},
	url = {http://dx.doi.org/10.1023/B:LIDA.0000048322.42751.ca},
	doi = {10.1023/B:LIDA.0000048322.42751.ca},
	acmid = {1035374},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Corrective maintenance, software process documentation, software system documentation},
}

@inproceedings{Fluri:2007:CCC:1339262.1339530,
	author = {Fluri, Beat and Wursch, Michael and Gall, Harald C.},
	title = {Do Code and Comments Co-Evolve? On the Relation between Source Code and Comment Changes},
	booktitle = {Proceedings of the 14th Working Conference on Reverse Engineering},
	series = {WCRE '07},
	year = {2007},
	isbn = {0-7695-3034-6},
	pages = {70--79},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/WCRE.2007.21},
	doi = {10.1109/WCRE.2007.21},
	acmid = {1339530},
	address = {Washington, DC, USA},
} 

@article{Ibrahim:2012:CCR:2330373.2330435,
	author = {Ibrahim, Walid M. and Bettenburg, Nicolas and Adams, Bram and Hassan, Ahmed E.},
	title = {Controversy Corner: On the relationship between comment update practices and Software Bugs},
	journal = {J. Syst. Softw.},
	issue_date = {October, 2012},
	volume = {85},
	number = {10},
	month = oct,
	year = {2012},
	issn = {0164-1212},
	pages = {2293--2304},
	numpages = {12},
	url = {http://dx.doi.org/10.1016/j.jss.2011.09.019},
	doi = {10.1016/j.jss.2011.09.019},
	acmid = {2330435},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {Code quality, Empirical studies, Software bugs, Software evolution, Source code comments},
}

@inproceedings{Sim:1998:ASC:580914.858229,
	author = {Sim, S. E. and Clarke, C. L. A. and Holt, R. C.},
	title = {Archetypal Source Code Searches: A Survey of Software Developers and Maintainers},
	booktitle = {Proceedings of the 6th International Workshop on Program Comprehension},
	series = {IWPC '98},
	year = {1998},
	isbn = {0-8186-8560-3},
	pages = {180--},
	url = {http://dl.acm.org/citation.cfm?id=580914.858229},
	acmid = {858229},
	address = {Washington, DC, USA},
} 

@article{Sillito:2008:AAQ:1446226.1446241,
	author = {Sillito, Jonathan and Murphy, Gail C. and De Volder, Kris},
	title = {Asking and Answering Questions during a Programming Change Task},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {July 2008},
	volume = {34},
	number = {4},
	issn = {0098-5589},
	pages = {434--451},
	numpages = {18},
	url = {http://dx.doi.org/10.1109/TSE.2008.26},
	doi = {10.1109/TSE.2008.26},
	acmid = {1446241},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Enhancement, Programming Environments/Construction Tools, Software psychology, Software psychology, Programming Environments/Construction Tools, Enhancement},
} 

@inproceedings{Burden:2011:NLG:2095654.2095665,
	author = {Burden, H{\aa}kan and Heldal, Rogardt},
	title = {Natural language generation from class diagrams},
	booktitle = {Proceedings of the 8th International Workshop on Model-Driven Engineering, Verification and Validation},
	series = {MoDeVVa},
	year = {2011},
	isbn = {978-1-4503-0914-1},
	location = {Wellington, New Zealand},
	pages = {8:1--8:8},
	articleno = {8},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/2095654.2095665},
	doi = {10.1145/2095654.2095665},
	acmid = {2095665},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {model transformations, model-driven architecture},
} 

@inproceedings{Mani:2012:AAU:2393596.2393607,
	author = {Mani, Senthil and Catherine, Rose and Sinha, Vibha Singhal and Dubey, Avinava},
	title = {AUSUM: approach for unsupervised bug report summarization},
	booktitle = {Proceedings of the ACM SIGSOFT 20th International Symposium on the Foundations of Software Engineering},
	series = {FSE '12},
	year = {2012},
	isbn = {978-1-4503-1614-9},
	location = {Cary, North Carolina},
	pages = {11:1--11:11},
	articleno = {11},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2393596.2393607},
	doi = {10.1145/2393596.2393607},
	acmid = {2393607},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {bug report, summarization, unsupervised},
} 

@inproceedings{Moreno:2013:ICPC,
	author = {Moreno, Laura and Aponte, Jairo and Sridhara Giriprasad and Marcus, Andrian and Pollock, Lori and Vijay-Shanker, K.},
	title = {Automatic Generation of Natural Language Summaries for Java Classes},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@inproceedings{Sridhara:2011:ADD:1985793.1985808,
	author = {Sridhara, Giriprasad and Pollock, Lori and Vijay-Shanker, K.},
	title = {Automatically detecting and describing high level actions within methods},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {101--110},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985808},
	doi = {10.1145/1985793.1985808},
	acmid = {1985808},
	address = {New York, NY, USA},
	keywords = {documentation, program comprehension},
}

@inproceedings{Sridhara:2010:TAG:1858996.1859006,
	author = {Sridhara, Giriprasad and Hill, Emily and Muppaneni, Divya and Pollock, Lori and Vijay-Shanker, K.},
	title = {Towards automatically generating summary comments for Java methods},
	booktitle = {Proceedings of the IEEE/ACM international conference on Automated software engineering},
	series = {ASE '10},
	year = {2010},
	isbn = {978-1-4503-0116-9},
	location = {Antwerp, Belgium},
	pages = {43--52},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1858996.1859006},
	doi = {10.1145/1858996.1859006},
	acmid = {1859006},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {comment generation, method summarization, natural language program analysis},
} 

@inproceedings{McMillan:2011:PFR:1985793.1985809,
	author = {McMillan, Collin and Grechanik, Mark and Poshyvanyk, Denys and Xie, Qing and Fu, Chen},
	title = {Portfolio: finding relevant functions and their usage},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {111--120},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985809},
	doi = {10.1145/1985793.1985809},
	acmid = {1985809},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {code search, function call graph, pagerank, portfolio, ranking},
} 


@PhdThesis{SridharaPhd12,
	title = "{Automatic Generation of Descriptive Summary Comments for Methods in Object-oriented Programs}",
	author = "Giriprasad Sridhara",
	school = "University of Delaware",
	month = Jan,
}

@inproceedings{Sridhara:2011:GPC:2057176.2057211,
	author = {Sridhara, Giriprasad and Pollock, Lori and Vijay-Shanker, K.},
	title = {Generating Parameter Comments and Integrating with Method Summaries},
	booktitle = {Proceedings of the 2011 IEEE 19th International Conference on Program Comprehension},
	series = {ICPC '11},
	year = {2011},
	isbn = {978-0-7695-4398-7},
	pages = {71--80},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICPC.2011.28},
	doi = {10.1109/ICPC.2011.28},
	acmid = {2057211},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {documentation, software maintenance},
}

@inproceedings{Haiduc:2010:UAT:1919284.1919577,
	author = {Haiduc, Sonia and Aponte, Jairo and Moreno, Laura and Marcus, Andrian},
	title = {On the Use of Automated Text Summarization Techniques for Summarizing Source Code},
	booktitle = {Proceedings of the 2010 17th Working Conference on Reverse Engineering},
	series = {WCRE '10},
	year = {2010},
	isbn = {978-0-7695-4123-5},
	pages = {35--44},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/WCRE.2010.13},
	doi = {10.1109/WCRE.2010.13},
	acmid = {1919577},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {text summarization, program comprehension},
}

@inproceedings{Ying:2013:CFS:2491411.2494587,
	author = {Ying, Annie T. T. and Robillard, Martin P.},
	title = {Code Fragment Summarization},
	booktitle = {Proceedings of the 2013 9th Joint Meeting on Foundations of Software Engineering},
	series = {ESEC/FSE 2013},
	year = {2013},
	isbn = {978-1-4503-2237-9},
	location = {Saint Petersburg, Russia},
	pages = {655--658},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/2491411.2494587},
	doi = {10.1145/2491411.2494587},
	acmid = {2494587},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Machine Learning, source code analysis, summarization},
} 

@article{Dijkstra:1968:LEG:362929.362947,
	author = {Dijkstra, Edsger W.},
	title = {Letters to the editor: go to statement considered harmful},
	journal = {Commun. ACM},
	issue_date = {March 1968},
	volume = {11},
	number = {3},
	month = mar,
	year = {1968},
	issn = {0001-0782},
	pages = {147--148},
	numpages = {2},
	url = {http://doi.acm.org/10.1145/362929.362947},
	doi = {10.1145/362929.362947},
	acmid = {362947},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {alternative clause, branch instruction, conditional clause, go to statement, jump instruction, program intelligibility, program sequencing, repetitive clause},
} 

@book{Campbell-Kelly:2003:ARS:640679,
	author = {Campbell-Kelly, Martin},
	title = {From Airline Reservations to Sonic the Hedgehog (History of Computing Series): A History of the Software Industry},
	year = {2003},
	isbn = {0262033038},
	publisher = {MIT Press},
	address = {Cambridge, MA, USA},
} 

@ARTICLE{1278847,
	author={Mahoney, Michael S.},
	journal={Annals of the History of Computing, IEEE},
	title={Finding a History for Software Engineering},
	year={2004},
	volume={26},
	number={1},
	pages={8-19},
	keywords={history;societies;software engineering;enterprise;industry;professions;software engineering history;Application software;Computer industry;History;Manufacturing;Software engineering},
	doi={10.1109/MAHC.2004.1278847},
	ISSN={1058-6180}
}

@ARTICLE{4617909,
	author={Mahoney, Michael S.},
	journal={Annals of the History of Computing, IEEE},
	title={What Makes the History of Software Hard},
	year={2008},
	volume={30},
	number={3},
	pages={8-18},
	keywords={computer software;history;computational models;historical experience;software history;Biomedical informatics;Computational modeling;History;Humans;Microcomputers;Optical computing;Permission;Photonic integrated circuits;Shape;Software tools},
	doi={10.1109/MAHC.2008.55},
	ISSN={1058-6180}
}

@book{Campbell-Kelly:2013,
	author = {Martin Campbell-Kelly and William Aspray and Nathan Ensmenger and Jeffrey R. Yost},
	title = {Computer: A History of the Information Machine},
	year = {2013},
	publisher = {Westview Press},
	address = {New York, NY, USA}
}

@article{Tzanakis2002,
	year={2002},
	isbn={978-0-7923-6399-6},
	journal={History in Mathematics Education},
	volume={6},
	series={New ICMI Study Series},
	editor={Fauvel, John and Maanen, Jan},
	doi={10.1007/0-306-47220-1_7},
	title={Integrating history of mathematics in the classroom: an analytic survey},
	url={http://dx.doi.org/10.1007/0-306-47220-1_7},
	publisher={Springer Netherlands},
	author={Tzanakis, Constantinos and Arcavi, Abraham and Sa, CarlosCorreia and Isoda, Masami and Lit, Chi-Kai and Niss, Mogens and Carvalho, JoãoPitombeira and Rodriguez, Michel and Siu, Man-Keung},
	pages={201-240}
}

@article{Letovsky1987325,
	title = "Cognitive processes in program comprehension ",
	journal = "Journal of Systems and Software ",
	volume = "7",
	number = "4",
	pages = "325 - 339",
	year = "1987",
	note = "",
	issn = "0164-1212",
	doi = "http://dx.doi.org/10.1016/0164-1212(87)90032-X",
	url = "http://www.sciencedirect.com/science/article/pii/016412128790032X",
	author = "Stanley Letovsky"
}


@article {JOB:JOB87,
	author = {Levesque, Laurie L. and Wilson, Jeanne M. and Wholey, Douglas R.},
	title = {Cognitive divergence and shared mental models in software development project teams},
	journal = {Journal of Organizational Behavior},
	volume = {22},
	number = {2},
	publisher = {John Wiley \& Sons, Ltd.},
	issn = {1099-1379},
	url = {http://dx.doi.org/10.1002/job.87},
	doi = {10.1002/job.87},
	pages = {135--144},
	year = {2001},
}

@article{Ko:2006:ESD:1248728.1248780,
	author = {Ko, Andrew J. and Myers, Brad A. and Coblenz, Michael J. and Aung, Htet Htet},
	title = {An Exploratory Study of How Developers Seek, Relate, and Collect Relevant Information during Software Maintenance Tasks},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {December 2006},
	volume = {32},
	number = {12},
	month = dec,
	year = {2006},
	issn = {0098-5589},
	pages = {971--987},
	numpages = {17},
	url = {http://dx.doi.org/10.1109/TSE.2006.116},
	doi = {10.1109/TSE.2006.116},
	acmid = {1248780},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Program investigation, Program investigation, program understanding, program comprehension, empirical software engineering, information foraging, information scent., empirical software engineering, information foraging, information scent., program comprehension, program understanding},
}

@inproceedings{LaToza:2006:MMM:1134285.1134355,
	author = {LaToza, Thomas D. and Venolia, Gina and DeLine, Robert},
	title = {Maintaining mental models: a study of developer work habits},
	booktitle = {Proceedings of the 28th international conference on Software engineering},
	series = {ICSE '06},
	year = {2006},
	isbn = {1-59593-375-1},
	location = {Shanghai, China},
	pages = {492--501},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1134285.1134355},
	doi = {10.1145/1134285.1134355},
	acmid = {1134355},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {agile software development, code duplication, code ownership, communication, debugging, interruptions},
}

@inproceedings{Singer:1997:ESE:782010.782031,
	author = {Singer, Janice and Lethbridge, Timothy and Vinson, Norman and Anquetil, Nicolas},
	title = {An examination of software engineering work practices},
	booktitle = {Proceedings of the 1997 conference of the Centre for Advanced Studies on Collaborative research},
	series = {CASCON '97},
	year = {1997},
	location = {Toronto, Ontario, Canada},
	pages = {21--},
	url = {http://dl.acm.org/citation.cfm?id=782010.782031},
	acmid = {782031},
	publisher = {IBM Press},
}

@book{Rajlich:2011:SEC:2077657,
	author = {Rajlich, Vaclav},
	title = {Software Engineering: The Current Practice},
	year = {2011},
	isbn = {1439841225, 9781439841228},
	edition = {1st},
	publisher = {Chapman \& Hall/CRC},
}

@book{HCM:2004,
	author = {Atsushi Akera and William Aspray},
	title = {Using History to Teach Computer Science and Related Disciplines},
	year = {2004},
	publisher = {Computing Research Association},
}

@book{NCTM:1980,
	author = {NCTM},
	title = {Agenda for Action},
	year = {1980},
	publisher = {NCTM},
	location = {Reston, Virginia}
}

@book{Black:1962,
	author = {M. Black},
	title = {Models and Metaphors: Studies in Language and Philosophy},
	year = {1962},
	publisher = {Cornell University Press},
	location = {Ithaca, New York}
}

@book{MM:1983,
	author = {P. Johnson-Laird},
	title = {Mental Models},
	year = {1983},
	publisher = {Cambridge University Press},
	location = {Cambridge}
}

@article{Rouse:1986,
	author = {Rouse, W.B. and Morris, N.M.},
	title = {On looking into the black box: prospects and limits in the search for mental models},
	journal = {Psychological Bulletin},
	volume = {100},
	number = {3},
	pages = {349--363},
	year = {1986}
}

@article{Mathieu:2000,
	author = {Mathieu, John E. and Heffner, Tonia S. and Goodwin, Gerald F. and Salas, Eduardo and Cannon-Bowers, Janis A.},
	title = {The Influence of Shared Mental Models on Team Process and Performance},
	journal = {Journal of Applied Psychology},
	volume = {85},
	number = {2},
	pages = {273--283},
	year = {2000}
}

@article{Adelson:1985:RDE:4557.4578,
	author = {Adelson, Beth and Soloway, Elliot},
	title = {The Role of Domain Expenence in Software Design},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {November 1985},
	volume = {11},
	number = {11},
	month = nov,
	year = {1985},
	issn = {0098-5589},
	pages = {1351--1360},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/TSE.1985.231883},
	doi = {10.1109/TSE.1985.231883},
	acmid = {4578},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Artificial intelligence, cognitive models, cognitive science, software design, software design, Artificial intelligence, cognitive models, cognitive science},
} 

@article{doi:10.1080/095006900416839,
	author = {Gobert, Janice D. and Buckley, Barbara C.},
	title = {Introduction to model-based teaching and learning in science education},
	journal = {International Journal of Science Education},
	volume = {22},
	number = {9},
	pages = {891-894},
	year = {2000},
	doi = {10.1080/095006900416839},
}

@article {TEA:TEA3660320508,
	author = {Williamson, Vickie M. and Abraham, Michael R.},
	title = {The effects of computer animation on the particulate mental models of college chemistry students},
	journal = {Journal of Research in Science Teaching},
	volume = {32},
	number = {5},
	publisher = {Wiley Subscription Services, Inc., A Wiley Company},
	issn = {1098-2736},
	url = {http://dx.doi.org/10.1002/tea.3660320508},
	doi = {10.1002/tea.3660320508},
	pages = {521--534},
	year = {1995},
}

@inproceedings{Rajlich:2013:TDS:2486788.2486940,
	author = {Rajlich, V\'{a}clav},
	title = {Teaching developer skills in the first software engineering course},
	booktitle = {Proceedings of the 2013 International Conference on Software Engineering},
	series = {ICSE '13},
	year = {2013},
	isbn = {978-1-4673-3076-3},
	location = {San Francisco, CA, USA},
	pages = {1109--1116},
	numpages = {8},
	url = {http://dl.acm.org/citation.cfm?id=2486788.2486940},
	acmid = {2486940},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@inproceedings{Marmorstein:2011:OSC:1999747.1999823,
	author = {Marmorstein, Robert},
	title = {Open source contribution as an effective software engineering class project},
	booktitle = {Proceedings of the 16th annual joint conference on Innovation and technology in computer science education},
	series = {ITiCSE '11},
	year = {2011},
	isbn = {978-1-4503-0697-3},
	location = {Darmstadt, Germany},
	pages = {268--272},
	numpages = {5},
	url = {http://doi.acm.org/10.1145/1999747.1999823},
	doi = {10.1145/1999747.1999823},
	acmid = {1999823},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {open source, real-world projects, software engineering, software maintenance, team programming},
} 

@book{Papert:1980:MCC:1095592,
	author = {Papert, Seymour},
	title = {Mindstorms: children, computers, and powerful ideas},
	year = {1980},
	isbn = {0-465-04627-4},
	publisher = {Basic Books, Inc.},
	address = {New York, NY, USA},
}

@inproceedings{Allen:2003:PPC:611892.611940,
	author = {Allen, Eric and Cartwright, Robert and Reis, Charles},
	title = {Production programming in the classroom},
	booktitle = {Proceedings of the 34th SIGCSE technical symposium on Computer science education},
	series = {SIGCSE '03},
	year = {2003},
	isbn = {1-58113-648-X},
	location = {Reno, Navada, USA},
	pages = {89--93},
	numpages = {5},
	url = {http://doi.acm.org/10.1145/611892.611940},
	doi = {10.1145/611892.611940},
	acmid = {611940},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {DrJava, JUnit, ant, extreme programming, open source, production programming, software engineering, sourceforge},
}

@book{Hunt:2000:PPJ:320326,
	author = {Hunt, Andrew and Thomas, David},
	title = {The pragmatic programmer: from journeyman to master},
	year = {1999},
	isbn = {0-201-61622-X},
	publisher = {Addison-Wesley Longman Publishing Co., Inc.},
	address = {Boston, MA, USA},
}

@inproceedings{Begel:2008:SNC:1352135.1352218,
	author = {Begel, Andrew and Simon, Beth},
	title = {Struggles of new college graduates in their first software development job},
	booktitle = {Proceedings of the 39th SIGCSE technical symposium on Computer science education},
	series = {SIGCSE '08},
	year = {2008},
	isbn = {978-1-59593-799-5},
	location = {Portland, OR, USA},
	pages = {226--230},
	numpages = {5},
	url = {http://doi.acm.org/10.1145/1352135.1352218},
	doi = {10.1145/1352135.1352218},
	acmid = {1352218},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {computer science education, human aspects of software engineering, software development},
} 

@misc{libdwarf,
	author = {Michael Eager},
	title = {The DWARF Debugging Standard},
	month = apr,
	year = {2012},
	note = {http://www.dwarfstd.org/}
}

@inproceedings{Mockus:2007:LCR:1270231.1270273,
	author = {Mockus, Audris},
	title = {Large-Scale Code Reuse in Open Source Software},
	booktitle = {Proceedings of the First International Workshop on Emerging Trends in FLOSS Research and Development},
	series = {FLOSS '07},
	year = {2007},
	isbn = {0-7695-2961-5},
	pages = {7--},
	url = {http://dx.doi.org/10.1109/FLOSS.2007.10},
	acmid = {1270273},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Krueger:1992:SR:130844.130856,
	author = {Krueger, Charles W.},
	title = {Software reuse},
	journal = {ACM Comput. Surv.},
	issue_date = {June 1992},
	volume = {24},
	number = {2},
	month = jun,
	year = {1992},
	issn = {0360-0300},
	pages = {131--183},
	numpages = {53},
	url = {http://doi.acm.org/10.1145/130844.130856},
	doi = {10.1145/130844.130856},
	acmid = {130856},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {abstraction, cognitive distance, software reuse},
}

@inproceedings{Brechner:2003:TTT:949344.949387,
	author = {Brechner, Eric},
	title = {Things they would not teach me of in college: what Microsoft developers learn later},
	booktitle = {Companion of the 18th annual ACM SIGPLAN conference on Object-oriented programming, systems, languages, and applications},
	series = {OOPSLA '03},
	year = {2003},
	isbn = {1-58113-751-6},
	location = {Anaheim, CA, USA},
	pages = {134--136},
	numpages = {3},
	url = {http://doi.acm.org/10.1145/949344.949387},
	doi = {10.1145/949344.949387},
	acmid = {949387},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {FMEA, accessibility, analysis, cohesion, collaboration, commercial, contracts, coordination, coupling, cryptography, design, diversity, globalization, multidisciplinary, privacy, quality, redundancy, reliability, requirements, security, testability},
} 

@inproceedings{Brannock:2012:RTU:2380552.2380578,
	author = {Brannock, Evelyn and Napier, Nannette},
	title = {Real-world testing: using FOSS for software development courses},
	booktitle = {Proceedings of the 13th annual conference on Information technology education},
	series = {SIGITE '12},
	year = {2012},
	isbn = {978-1-4503-1464-0},
	location = {Calgary, Alberta, Canada},
	pages = {87--88},
	numpages = {2},
	url = {http://doi.acm.org/10.1145/2380552.2380578},
	doi = {10.1145/2380552.2380578},
	acmid = {2380578},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {open source, testing},
} 

@article{Crosby:1990:WRA:77577.77580,
	author = {Crosby, Martha E. and Stelovsky, Jan},
	title = {How Do We Read Algorithms? A Case Study},
	journal = {Computer},
	issue_date = {January 1990},
	volume = {23},
	number = {1},
	month = jan,
	year = {1990},
	issn = {0018-9162},
	pages = {24--35},
	numpages = {12},
	url = {http://dl.acm.org/citation.cfm?id=77577.77580},
	acmid = {77580},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{Sharif:2012:ESR:2168556.2168642,
	author = {Sharif, Bonita and Falcone, Michael and Maletic, Jonathan I.},
	title = {An eye-tracking study on the role of scan time in finding source code defects},
	booktitle = {Proceedings of the Symposium on Eye Tracking Research and Applications},
	series = {ETRA '12},
	year = {2012},
	isbn = {978-1-4503-1221-9},
	location = {Santa Barbara, California},
	pages = {381--384},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/2168556.2168642},
	doi = {10.1145/2168556.2168642},
	acmid = {2168642},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {eye-tracking study, software defects, source-code review},
}

@inproceedings{Roehm:2012:PDC:2337223.2337254,
	author = {Roehm, Tobias and Tiarks, Rebecca and Koschke, Rainer and Maalej, Walid},
	title = {How do professional developers comprehend software?},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {255--265},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337254},
	acmid = {2337254},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@ARTICLE{402076,
	author={von Mayrhauser, A. and Vans, A.M.},
	journal={Computer},
	title={Program comprehension during software maintenance and evolution},
	year={1995},
	volume={28},
	number={8},
	pages={44-55},
	keywords={human factors;large-scale systems;reverse engineering;software maintenance;bottom-up model;code cognition models;data availability;experimental procedures;integrated metamodel;large-scale code;partial understanding;program code understanding;program comprehension models;scalability;software evolution;software maintenance;specialized tasks;top-down model;Application software;Cognition;Cognitive science;Computer architecture;Documentation;Large-scale systems;Programming profession;Round robin;Scalability;Software maintenance},
	doi={10.1109/2.402076},
	ISSN={0018-9162}
}

@article{Littman:1987:MMS:39161.39170,
	author = {Littman, David C. and Pinto, Jeannine and Letovsky, Stanley and Soloway, Elliot},
	title = {Mental models and software maintenance},
	journal = {J. Syst. Softw.},
	issue_date = {December 1, 1987},
	volume = {7},
	number = {4},
	month = dec,
	year = {1987},
	issn = {0164-1212},
	pages = {341--355},
	numpages = {15},
	url = {http://dx.doi.org/10.1016/0164-1212(87)90033-1},
	doi = {10.1016/0164-1212(87)90033-1},
	acmid = {39170},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
}

@book{liu2000smalltalk,
	title={Smalltalk, Objects, and Design},
	author={Liu, C.},
	isbn={9781583484906},
	year={2000},
	publisher={iUniverse}
}

@book{Abadi:1996:TO:547964,
	author = {Abadi, Martin and Cardelli, Luca},
	title = {A  Theory of Objects},
	year = {1996},
	isbn = {0387947752},
	edition = {1st},
	publisher = {Springer-Verlag New York, Inc.},
	address = {Secaucus, NJ, USA},
}

@article{Dekel:2007:NRC:1297105.1297047,
	author = {Dekel, Uri and Herbsleb, James D.},
	title = {Notation and representation in collaborative object-oriented design: an observational study},
	journal = {SIGPLAN Not.},
	issue_date = {October 2007},
	volume = {42},
	number = {10},
	month = oct,
	year = {2007},
	issn = {0362-1340},
	pages = {261--280},
	numpages = {20},
	url = {http://doi.acm.org/10.1145/1297105.1297047},
	doi = {10.1145/1297105.1297047},
	acmid = {1297047},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {OOD, UML, collaborative software design, modeling, notation, representation},
} 

@article{Biggerstaff:1989:DRM:72893.72896,
	author = {Biggerstaff, Ted J.},
	title = {Design Recovery for Maintenance and Reuse},
	journal = {Computer},
	issue_date = {July 1989},
	volume = {22},
	number = {7},
	month = jul,
	year = {1989},
	issn = {0018-9162},
	pages = {36--49},
	numpages = {14},
	url = {http://dx.doi.org/10.1109/2.30731},
	doi = {10.1109/2.30731},
	acmid = {72896},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
} 

@INPROCEEDINGS{Etzkorn95anapproach,
	author = {Letha H. Etzkorn and Carl G. Davis},
	title = {An Approach to Object-oriented Program Understanding},
	booktitle = {Proceedings of the IEEE Third Workshop on Program Comprehension},
	year = {1995},
	pages = {14--15}
}

@book{Kan:2002:MMS:559784,
	author = {Kan, Stephen H.},
	title = {Metrics and Models in Software Quality Engineering},
	year = {2002},
	isbn = {0201729156},
	edition = {2nd},
	publisher = {Addison-Wesley Longman Publishing Co., Inc.},
	address = {Boston, MA, USA},
} 

@article{Gyimothy:2005:EVO:1100866.1100985,
	author = {Gyimothy, Tibor and Ferenc, Rudolf and Siket, Istvan},
	title = {Empirical Validation of Object-Oriented Metrics on Open Source Software for Fault Prediction},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {October 2005},
	volume = {31},
	number = {10},
	month = oct,
	year = {2005},
	issn = {0098-5589},
	pages = {897--910},
	numpages = {14},
	url = {http://dx.doi.org/10.1109/TSE.2005.112},
	doi = {10.1109/TSE.2005.112},
	acmid = {1100985},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Bugzilla, C++, Columbus., Index Terms- Fact extraction, Index Terms- Fact extraction, metrics validation, reverse engineering, open source software, fault-proneness detection, Mozilla, Bugzilla, C++, compiler wrapping, Columbus., Mozilla, compiler wrapping, fault-proneness detection, metrics validation, open source software, reverse engineering},
} 

@article{Chidamber:1994:MSO:630808.631131,
	author = {Chidamber, S. R. and Kemerer, C. F.},
	title = {A Metrics Suite for Object Oriented Design},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {June 1994},
	volume = {20},
	number = {6},
	month = jun,
	year = {1994},
	issn = {0098-5589},
	pages = {476--493},
	numpages = {18},
	url = {http://dx.doi.org/10.1109/32.295895},
	doi = {10.1109/32.295895},
	acmid = {631131},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {automated data collection tool, measurement principles, metrics suite, object oriented design, object oriented programming, object-oriented methods, object-oriented programming, organization, process improvement, software development, software measures, software metrics},
} 

@book{Gamma:1995:DPE:186897,
	author = {Gamma, Erich and Helm, Richard and Johnson, Ralph and Vlissides, John},
	title = {Design patterns: elements of reusable object-oriented software},
	year = {1995},
	isbn = {0-201-63361-2},
	publisher = {Addison-Wesley Longman Publishing Co., Inc.},
	address = {Boston, MA, USA},
}

@book{Cockburn:2002:ASD:502980,
	author = {Cockburn, Alistair},
	title = {Agile software development},
	year = {2002},
	isbn = {0-201-69969-9},
	publisher = {Addison-Wesley Longman Publishing Co., Inc.},
	address = {Boston, MA, USA},
}  

@article{Ponder:1994:PCH:181628.181635,
	author = {Ponder, Carl and Bush, Bill},
	title = {Polymorphism considered harmful},
	journal = {SIGSOFT Softw. Eng. Notes},
	issue_date = {April 1994},
	volume = {19},
	number = {2},
	month = apr,
	year = {1994},
	issn = {0163-5948},
	pages = {35--37},
	numpages = {3},
	url = {http://doi.acm.org/10.1145/181628.181635},
	doi = {10.1145/181628.181635},
	acmid = {181635},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@article{Kurland:LOGO,
	author = {Kurland, D. M. and Pea, R. D.},
	title = {Children's mental models of recursive Logo programs},
	journal = {Journal of Educational Computing Research},
	volume = {1},
	number = {2},
	year = {1985},
	pages = {235--243}
}

@ARTICLE{Johnson88designingreuseable,
	author = {Ralph E. Johnson and Brian Foote},
	title = {Designing reuseable classes},
	journal = {Journal of Object-Oriented Programming},
	year = {1988}
}

@article{Rosson:1996:RUS:234526.234530,
	author = {Rosson, Mary Beth and Carroll, John M.},
	title = {The reuse of uses in Smalltalk programming},
	journal = {ACM Trans. Comput.-Hum. Interact.},
	issue_date = {Sept. 1996},
	volume = {3},
	number = {3},
	month = sep,
	year = {1996},
	issn = {1073-0516},
	pages = {219--253},
	numpages = {35},
	url = {http://doi.acm.org/10.1145/234526.234530},
	doi = {10.1145/234526.234530},
	acmid = {234530},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Smalltalk, debugging into existence, example-based learning, reuse of uses, usage context},
}

@inproceedings{Ko:2004:SLB:1032665.1034570,
	author = {Ko, Andrew J. and Myers, Brad A. and Aung, Htet Htet},
	title = {Six Learning Barriers in End-User Programming Systems},
	booktitle = {Proceedings of the 2004 IEEE Symposium on Visual Languages - Human Centric Computing},
	series = {VLHCC '04},
	year = {2004},
	isbn = {0-7803-8696-5},
	pages = {199--206},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/VLHCC.2004.47},
	doi = {10.1109/VLHCC.2004.47},
	acmid = {1034570},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@article{Corbi:1989:PUC:97118.97124,
	author = {Corbi, T. A.},
	title = {Program understanding: challenge for the 1990's},
	journal = {IBM Syst. J.},
	issue_date = {1989},
	volume = {28},
	number = {2},
	month = jun,
	year = {1989},
	issn = {0018-8670},
	pages = {294--306},
	numpages = {13},
	url = {http://dx.doi.org/10.1147/sj.282.0294},
	doi = {10.1147/sj.282.0294},
	acmid = {97124},
	publisher = {IBM Corp.},
	address = {Riverton, NJ, USA},
} 

@article{Sillito:2008:AAQ:1446226.1446241,
	author = {Sillito, Jonathan and Murphy, Gail C. and De Volder, Kris},
	title = {Asking and Answering Questions during a Programming Change Task},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {July 2008},
	volume = {34},
	number = {4},
	month = jul,
	year = {2008},
	issn = {0098-5589},
	pages = {434--451},
	numpages = {18},
	url = {http://dx.doi.org/10.1109/TSE.2008.26},
	doi = {10.1109/TSE.2008.26},
	acmid = {1446241},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Enhancement, Programming Environments/Construction Tools, Software psychology, Software psychology, Programming Environments/Construction Tools, Enhancement},
}

@inproceedings{Sim:1998:ASC:580914.858229,
	author = {Sim, S. E. and Clarke, C. L. A. and Holt, R. C.},
	title = {Archetypal Source Code Searches: A Survey of Software Developers and Maintainers},
	booktitle = {Proceedings of the 6th International Workshop on Program Comprehension},
	series = {IWPC '98},
	year = {1998},
	isbn = {0-8186-8560-3},
	pages = {180--},
	url = {http://dl.acm.org/citation.cfm?id=580914.858229},
	acmid = {858229},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@ARTICLE{Davison00understandingand,
	author = {Joseph W. Davison and Dennis M. Mancl and William F. Opdyke},
	title = {Understanding and addressing the essential costs of evolving systems},
	journal = {Bell Labs Technical Journal},
	year = {2000},
	pages = {44--54}
}

@inproceedings{Kapser:2006:CCH:1174510.1174714,
	author = {Kapser, Cory and Godfrey, Michael W.},
	title = {``Cloning Considered Harmful'' Considered Harmful},
	booktitle = {Proceedings of the 13th Working Conference on Reverse Engineering},
	series = {WCRE '06},
	year = {2006},
	isbn = {0-7695-2719-1},
	pages = {19--28},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/WCRE.2006.1},
	doi = {10.1109/WCRE.2006.1},
	acmid = {1174714},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{Juergens:2009:CCM:1555001.1555062,
	author = {Juergens, Elmar and Deissenboeck, Florian and Hummel, Benjamin and Wagner, Stefan},
	title = {Do code clones matter?},
	booktitle = {Proceedings of the 31st International Conference on Software Engineering},
	series = {ICSE '09},
	year = {2009},
	isbn = {978-1-4244-3453-4},
	pages = {485--495},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2009.5070547},
	doi = {10.1109/ICSE.2009.5070547},
	acmid = {1555062},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{begel2010codebook,
	title={Codebook: discovering and exploiting relationships in software repositories},
	author={Begel, Andrew and Khoo, Yit Phang and Zimmermann, Thomas},
	booktitle={2010 ACM/IEEE 32nd International Conference on Software Engineering},
	volume={1},
	pages={125--134},
	year={2010},
	organization={IEEE}
}

@inproceedings{weiss2007long,
	title={How long will it take to fix this bug?},
	author={Weiss, Cathrin and Premraj, Rahul and Zimmermann, Thomas and Zeller, Andreas},
	booktitle={Proceedings of the Fourth International Workshop on Mining Software Repositories},
	pages={1},
	year={2007},
	organization={IEEE Computer Society}
}

@inproceedings{dit2011can,
	title={Can better identifier splitting techniques help feature location?},
	author={Dit, Bogdan and Guerrouj, Latifa and Poshyvanyk, Denys and Antoniol, Giuliano},
	booktitle={Program Comprehension (ICPC), 2011 IEEE 19th International Conference on},
	pages={11--20},
	year={2011},
	organization={IEEE}
}

@inproceedings{enslen2009mining,
	title={Mining source code to automatically split identifiers for software analysis},
	author={Enslen, Eric and Hill, Emily and Pollock, Lori and Vijay-Shanker, K},
	booktitle={2009 6th IEEE International Working Conference on Mining Software Repositories},
	pages={71--80},
	year={2009},
	organization={IEEE}
}

@article{Kagdi:2007:STA:1345056.1345057,
	author = {Kagdi, Huzefa and Collard, Michael L. and Maletic, Jonathan I.},
	title = {A survey and taxonomy of approaches for mining software repositories in the context of software evolution},
	journal = {J. Softw. Maint. Evol.},
	issue_date = {March 2007},
	volume = {19},
	number = {2},
	month = mar,
	year = {2007},
	issn = {1532-060X},
	pages = {77--131},
	numpages = {55},
	url = {http://dx.doi.org/10.1002/smr.344},
	doi = {10.1002/smr.344},
	acmid = {1345057},
	publisher = {John Wiley \& Sons, Inc.},
	address = {New York, NY, USA},
	keywords = {mining software repositories, multi-version analysis, software evolution},
} 

@inproceedings{Clause:2007:DGD:1273463.1273490,
	author = {Clause, James and Li, Wanchun and Orso, Alessandro},
	title = {Dytan: a generic dynamic taint analysis framework},
	booktitle = {Proceedings of the 2007 international symposium on Software testing and analysis},
	series = {ISSTA '07},
	year = {2007},
	isbn = {978-1-59593-734-6},
	location = {London, United Kingdom},
	pages = {196--206},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1273463.1273490},
	doi = {10.1145/1273463.1273490},
	acmid = {1273490},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {dynamic tainting, general framework, information flow},
} 

@inproceedings{Chan:2012:SCA:2393596.2393606,
	author = {Chan, Wing-Kwan and Cheng, Hong and Lo, David},
	title = {Searching connected API subgraph via text phrases},
	booktitle = {Proceedings of the ACM SIGSOFT 20th International Symposium on the Foundations of Software Engineering},
	series = {FSE '12},
	year = {2012},
	isbn = {978-1-4503-1614-9},
	location = {Cary, North Carolina},
	pages = {10:1--10:11},
	articleno = {10},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2393596.2393606},
	doi = {10.1145/2393596.2393606},
	acmid = {2393606},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {API graph, API recommendation, subgraph searching},
} 

@article{Shackelford:2006:CCO:1124706.1121482,
	author = {Shackelford, Russell and McGettrick, Andrew and Sloan, Robert and Topi, Heikki and Davies, Gordon and Kamali, Reza and Cross, James and Impagliazzo, John and LeBlanc, Richard and Lunt, Barry},
	title = {Computing Curricula 2005: The Overview Report},
	journal = {SIGCSE Bull.},
	issue_date = {March 2006},
	volume = {38},
	number = {1},
	month = mar,
	year = {2006},
	issn = {0097-8418},
	pages = {456--457},
	numpages = {2},
	url = {http://doi.acm.org/10.1145/1124706.1121482},
	doi = {10.1145/1124706.1121482},
	acmid = {1121482},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {comparison of curriculum, computer engineering curriculum, computer science curriculum, computing curricula, information systems curriculum, information technology curriculum, software engineering curriculum},
} 

@article{10.1109/HICSS.2005.378,
	author = {Georg von Krogh and Sebastian Spaeth and Stefan Haefliger},
	title = {Knowledge Reuse in Open Source Software: An Exploratory Study of 15 Open Source Projects},
	journal ={Hawaii International Conference on System Sciences},
	volume = {7},
	issn = {1530-1605},
	year = {2005},
	pages = {198b},
	doi = {http://doi.ieeecomputersociety.org/10.1109/HICSS.2005.378},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{McMillan:2011:CSA:2117694.2119646,
	author = {McMillan, Collin and Linares-Vasquez, Mario and Poshyvanyk, Denys and Grechanik, Mark},
	title = {Categorizing software applications for maintenance},
	booktitle = {Proceedings of the 2011 27th IEEE International Conference on Software Maintenance},
	series = {ICSM '11},
	year = {2011},
	isbn = {978-1-4577-0663-9},
	pages = {343--352},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICSM.2011.6080801},
	doi = {10.1109/ICSM.2011.6080801},
	acmid = {2119646},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Grechanik:2010:EIL:1852786.1852801,
	author = {Grechanik, Mark and McMillan, Collin and DeFerrari, Luca and Comi, Marco and Crespi, Stefano and Poshyvanyk, Denys and Fu, Chen and Xie, Qing and Ghezzi, Carlo},
	title = {An empirical investigation into a large-scale Java open source code repository},
	booktitle = {Proceedings of the 2010 ACM-IEEE International Symposium on Empirical Software Engineering and Measurement},
	series = {ESEM '10},
	year = {2010},
	isbn = {978-1-4503-0039-1},
	location = {Bolzano-Bozen, Italy},
	pages = {11:1--11:10},
	articleno = {11},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1852786.1852801},
	doi = {10.1145/1852786.1852801},
	acmid = {1852801},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {empirical study, large-scale software, mining software repositories, open source, patterns, practice, software repository},
}

@inproceedings{Agichtein:2006:LUI:1148170.1148175,
	author = {Agichtein, Eugene and Brill, Eric and Dumais, Susan and Ragno, Robert},
	title = {Learning user interaction models for predicting web search result preferences},
	booktitle = {Proceedings of the 29th annual international ACM SIGIR conference on Research and development in information retrieval},
	series = {SIGIR '06},
	year = {2006},
	isbn = {1-59593-369-7},
	location = {Seattle, Washington, USA},
	pages = {3--10},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1148170.1148175},
	doi = {10.1145/1148170.1148175},
	acmid = {1148175},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {interpreting implicit relevance feedback, predicting relevance preferences, user behavior modeling},
} 

@article{Claypool:2001:IUI:613351.613651,
	author = {Claypool, Mark and Brown, David and Le, Phong and Waseda, Makoto},
	title = {Inferring User Interest},
	journal = {IEEE Internet Computing},
	issue_date = {November 2001},
	volume = {5},
	number = {6},
	month = nov,
	year = {2001},
	issn = {1089-7801},
	pages = {32--39},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/4236.968829},
	doi = {10.1109/4236.968829},
	acmid = {613651},
	publisher = {IEEE Educational Activities Department},
	address = {Piscataway, NJ, USA},
} 

@book{IR:08,
	author = {Manning, Christopher D. and Raghavan, Prabhakar and Schtze, Hinrich},
	title = {Introduction to Information Retrieval},
	year = {2008},
	isbn = {0521865719, 9780521865715},
	publisher = {Cambridge University Press},
	address = {New York, NY, USA}
}

@article{Likert1932,
	author = {Likert, R.A.},
	title= {A technique for the measurement of attitudes},
	year = {1932},
	journal = {Archives of Psychology},
	volume = {22},
	number = {140},
	pages = {5-55},
}

@article{Deerwester:jasis1990,
	Author = {S. Deerwester and S. T. Dumais and G. W. Furnas and T. K. Landauer and R. Harshman},
	Date-Added = {2007-08-31 12:57:51 +0200},
	Date-Modified = {2007-08-31 12:57:51 +0200},
	Journal = {Journal of the American Society for Information Science},
	Number = {6},
	Pages = {391-407},
	Title = {Indexing by Latent Semantic Analysis},
	Volume = {41},
	Year = {1990}
}

@inproceedings{Marcus:icse2003,
	Author = {A. Marcus and J. I. Maletic},
	Booktitle = {Proceedings of 25th International Conference on Software Engineering},
	Date-Added = {2007-08-31 12:57:51 +0200},
	Date-Modified = {2010-02-19 22:36:39 +0100},
	Pages = {125-135},
	Title = {Recovering Documentation-to-Source-Code Traceability Links using Latent Semantic Indexing},
	Year = {2003}
}

@book{Baeza-Yates:1999,
	Author = {R. Baeza-Yates and B. Ribeiro-Neto},
	Date-Added = {2007-08-31 12:57:51 +0200},
	Date-Modified = {2007-08-31 12:57:51 +0200},
	Publisher = {Addison-Wesley},
	Title = {Modern Information Retrieval},
	Year = {1999}
}

@article{Landi:1992:USA:161494.161501,
	author = {Landi, William},
	title = {Undecidability of static analysis},
	journal = {ACM Lett. Program. Lang. Syst.},
	issue_date = {Dec. 1992},
	volume = {1},
	number = {4},
	month = dec,
	year = {1992},
	issn = {1057-4514},
	pages = {323--337},
	numpages = {15},
	url = {http://doi.acm.org/10.1145/161494.161501},
	doi = {10.1145/161494.161501},
	acmid = {161501},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {abstract interpretation, alias analysis, data flow analysis, halting problem, static analysis},
}

@inproceedings{Biggerstaff:1993:CAP:257572.257679,
	author = {Biggerstaff, Ted J. and Mitbander, Bharat G. and Webster, Dallas},
	title = {The concept assignment problem in program understanding},
	booktitle = {Proceedings of the 15th international conference on Software Engineering},
	series = {ICSE '93},
	year = {1993},
	isbn = {0-89791-588-7},
	location = {Baltimore, Maryland, United States},
	pages = {482--498},
	numpages = {17},
	url = {http://dl.acm.org/citation.cfm?id=257572.257679},
	acmid = {257679},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
	keywords = {concept recognition, connectionist, domain, knowledge base, plausible reasoning, reverse engineering, slicing},
}

@article{Knight:1998:SQT:590631.590635,
	author = {Knight, John C. and Dunn, Michael F.},
	title = {Software quality through domain-driven certification},
	journal = {Ann. Softw. Eng.},
	issue_date = {1998},
	volume = {5},
	month = jan,
	year = {1998},
	issn = {1022-7091},
	pages = {293--315},
	numpages = {23},
	url = {http://dl.acm.org/citation.cfm?id=590631.590635},
	acmid = {590635},
	publisher = {J. C. Baltzer AG, Science Publishers},
	address = {Red Bank, NJ, USA},
}

@ARTICLE{62928,
	author={Barns, B.H. and Bollinger, T.B.},
	journal={Software, IEEE}, title={Making reuse cost-effective},
	year={1991},
	month={jan. },
	volume={8},
	number={1},
	pages={13 -24},
	keywords={consumer reuse;human problem solving;management;quality-of-investment;reuse investments;software reuse;DP management;software reusability;},
	doi={10.1109/52.62928},
	ISSN={0740-7459},}

@article{Banker:1991:RPI:120901.120908,
	author = {Banker, Rajiv D. and Kauffman, Robert J.},
	title = {Reuse and productivity in integrated computer-aided software engineering: an empirical study},
	journal = {MIS Q.},
	issue_date = {Sept. 1991},
	volume = {15},
	number = {3},
	month = oct,
	year = {1991},
	issn = {0276-7783},
	pages = {375--401},
	numpages = {27},
	url = {http://dx.doi.org/10.2307/249649},
	doi = {10.2307/249649},
	acmid = {120908},
	publisher = {Society for Information Management and The Management Information Systems Research Center},
	address = {Minneapolis, MN, USA},
	keywords = {CASE, ICASE, productivity measurement, reuse, software development, software economics, software engineering},
}

@article{10.1109/TSE.2011.84,
	author = {Collin McMillan and Mark Grechanik and Denys Poshyvanyk and Chen Fu and Qing Xie},
	title = {Exemplar: A Source Code Search Engine For Finding Highly Relevant Applications},
	journal ={IEEE Transactions on Software Engineering},
	volume = {99},
	number = {PrePrints},
	issn = {0098-5589},
	year = {2011},
	doi = {http://doi.ieeecomputersociety.org/10.1109/TSE.2011.84},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{Grechanik:2010:SEF:1806799.1806868,
	author = {Grechanik, Mark and Fu, Chen and Xie, Qing and McMillan, Collin and Poshyvanyk, Denys and Cumby, Chad},
	title = {A search engine for finding highly relevant applications},
	booktitle = {Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering - Volume 1},
	series = {ICSE '10},
	year = {2010},
	isbn = {978-1-60558-719-6},
	location = {Cape Town, South Africa},
	pages = {475--484},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1806799.1806868},
	doi = {10.1145/1806799.1806868},
	acmid = {1806868},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{McMillan:2011:PFR:1985793.1985809,
	author = {McMillan, Collin and Grechanik, Mark and Poshyvanyk, Denys and Xie, Qing and Fu, Chen},
	title = {Portfolio: finding relevant functions and their usage},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {111--120},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985809},
	doi = {10.1145/1985793.1985809},
	acmid = {1985809},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {code search, function call graph, pagerank, portfolio, ranking},
} 

@article{Mario:EMSE:13,
	author = {Mario Linares-Vasquez and Collin McMillan and Denys Poshyvanyk and Mark Grechanik},
	title = {Searching for Relevant Functions and Their Usages in Millions of Lines of Code},
	journal ={Empirical Software Engineering},
	year = {2013},
	publisher = {EMSE},
	note = {To appear},
}

@article{McMillan:Portfolio:TOSEM,
	author = {Collin McMillan and Mark Grechanik and Denys Poshyvanyk and Qing Xie and Chen Fu},
	title = {Searching for Relevant Functions and Their Usages in Millions of Lines of Code},
	journal ={ACM Transactions on Software Engineering and Methodology},
	year = {2012},
	doi = {http://doi.ieeecomputersociety.org/10.1109/TSE.2011.84},
	publisher = {ACM},
	note = {To appear},
}

@article {springerlink:10.1007/s10618-008-0118-x,
	author = {Linstead, Erik and Bajracharya, Sushil and Ngo, Trung and Rigor, Paul and Lopes, Cristina and Baldi, Pierre},
	affiliation = {University of California Donald Bren School of Information and Computer Sciences Irvine USA},
	title = {Sourcerer: mining and searching internet-scale software repositories},
	journal = {Data Mining and Knowledge Discovery},
	publisher = {Springer Netherlands},
	issn = {1384-5810},
	keyword = {Computer Science},
	pages = {300-336},
	volume = {18},
	issue = {2},
	url = {http://dx.doi.org/10.1007/s10618-008-0118-x},
	note = {10.1007/s10618-008-0118-x},
	year = {2009}
}

@inproceedings{CODEFINDER:96,
	author    = {Scott Henninger},
	title     = {Supporting the Construction and Evolution of Component Repositories.},
	booktitle = {ICSE},
	year      = {1996},
	pages     = {279-288},
	ee        = {http://portal.acm.org/citation.cfm?id=227726.227776},
}

@inproceedings{MICA:06,
	author    = {Jeffrey Stylos and
	Brad A. Myers},
	title     = {A Web-Search Tool for Finding \textsc{API} Components and Examples.},
	booktitle = {IEEE Symposium on VL and HCC},
	year      = {2006},
	pages     = {195-202},
}

@inproceedings{CODEBROKER:02,
	author    = {Yunwen Ye and
	Gerhard Fischer},
	title     = {Supporting reuse by delivering task-relevant and personalized
	information.},
	booktitle = {ICSE},
	year      = {2002},
	pages     = {513-523},
	ee        = {http://doi.acm.org/10.1145/581339.581402},
}

@article{HIPIKAT:05,
	author    = {Davor Cubranic and
	Gail C. Murphy and
	Janice Singer and
	Kellogg S. Booth},
	title     = {Hipikat: A Project Memory for Software Development.},
	journal   = {IEEE Trans. Software Eng.},
	volume    = {31},
	number    = {6},
	year      = {2005},
	pages     = {446-465},
	ee        = {http://dx.doi.org/10.1109/TSE.2005.71},
}

@inproceedings{Holmes:2007:SIP:1248820.1248877,
	author = {Holmes, Reid and Walker, Robert J.},
	title = {Supporting the Investigation and Planning of Pragmatic Reuse Tasks},
	booktitle = {Proceedings of the 29th international conference on Software Engineering},
	series = {ICSE '07},
	year = {2007},
	isbn = {0-7695-2828-7},
	pages = {447--457},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/ICSE.2007.83},
	doi = {10.1109/ICSE.2007.83},
	acmid = {1248877},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@inproceedings{STRATHCONA:05,
	author    = {Reid Holmes and
	Robert J. Walker and
	Gail C. Murphy},
	title     = {Strathcona example recommendation tool.},
	booktitle = {ESEC/FSE},
	year      = {2005},
	pages     = {237-240},
	ee        = {http://doi.acm.org/10.1145/1081706.1081744},
}

@article{SPARSJ:05,
	author = {Inoue, Katsuro and Yokomori, Reishi and Yamamoto, Tetsuo and Matsushita, Makoto and Kusumoto, Shinji},
	title = {Ranking Significance of Software Components Based on Use Relations},
	journal = {IEEE Trans. Softw. Eng.},
	volume = {31},
	number = {3},
	year = {2005},
	issn = {0098-5589},
	pages = {213--225},
	doi = {http://dx.doi.org/10.1109/TSE.2005.38},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@inproceedings{McMillan:2012:DSS:2337223.2337267,
	author = {McMillan, Collin and Grechanik, Mark and Poshyvanyk, Denys},
	title = {Detecting similar software applications},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {364--374},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337267},
	acmid = {2337267},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
} 

@inproceedings{SPOTWEB:08,
	author = {Thummalapenta, S. and Tao Xie},
	title = {SpotWeb: Detecting Framework Hotspots and Coldspots via Mining Open Source Code on the Web},
	booktitle = {ASE '08},
	year = {2008},
	isbn = {978-1-4244-2187-9},
	pages = {327--336},
	doi = {http://dx.doi.org/10.1109/ASE.2008.43},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{PROSPECTOR:05,
	author    = {David Mandelin and
	Lin Xu and
	Rastislav Bod\'{\i}k and
	Doug Kimelman},
	title     = {Jungloid mining: helping to navigate the \textsc{API} jungle.},
	booktitle = {PLDI},
	year      = {2005},
	pages     = {48-61},
	ee        = {http://doi.acm.org/10.1145/1065010.1065018},
}

@inproceedings{XSNIPPET:06,
	author    = {Naiyana Sahavechaphan and
	Kajal T. Claypool},
	title     = {\textsc{XS}nippet: mining For sample code.},
	booktitle = {OOPSLA},
	year      = {2006},
	pages     = {413-430},
	ee        = {http://doi.acm.org/10.1145/1167473.1167508},
}

@inproceedings{PARSEWEB:07,
	author = {Thummalapenta, Suresh and Xie, Tao},
	title = {Parseweb: a programmer assistant for reusing open source code on the web},
	booktitle = {ASE '07},
	year = {2007},
	isbn = {978-1-59593-882-4},
	pages = {204--213},
	location = {Atlanta, Georgia, USA},
	doi = {http://doi.acm.org/10.1145/1321631.1321663},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{MURPHY:05,
	author    = {Reid Holmes and
	Gail C. Murphy},
	title     = {Using structural context to recommend source code examples.},
	booktitle = {ICSE},
	year      = {2005},
	pages     = {117-125},
	ee        = {http://doi.acm.org/10.1145/1062455.1062491},
}

@inproceedings{S6:09,
	author    = {Steven P. Reiss},
	title     = {Semantics-based code search},
	booktitle = {ICSE},
	year      = {2009},
	pages     = {243-253},
	ee        = {http://dx.doi.org/10.1109/ICSE.2009.5070525},
}

@article{Hummel:2008:CCP:1439186.1439224,
	author = {Hummel, Oliver and Janjic, Werner and Atkinson, Colin},
	title = {Code Conjurer: Pulling Reusable Software out of Thin Air},
	journal = {IEEE Softw.},
	issue_date = {September 2008},
	volume = {25},
	number = {5},
	month = sep,
	year = {2008},
	issn = {0740-7459},
	pages = {45--52},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/MS.2008.110},
	doi = {10.1109/MS.2008.110},
	acmid = {1439224},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
} 

@article{Frakes:2005:SRR:1083823.1083997,
	author = {Frakes, William B. and Kang, Kyo},
	title = {Software Reuse Research: Status and Future},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {July 2005},
	volume = {31},
	number = {7},
	month = jul,
	year = {2005},
	issn = {0098-5589},
	pages = {529--536},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/TSE.2005.85},
	doi = {10.1109/TSE.2005.85},
	acmid = {1083997},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@BOOK{Arango:DomainAnalysis,
	AUTHOR = "G. Arango and R. Prieto-Diaz",
	TITLE = "Domain Analysis: Acquisition of Reusable Information for Software Construction",
	PUBLISHER ="IEEE Comp. Society Press",
	MONTH = "May",
	YEAR = {1989}
}
@ARTICLE{Frakes:DARE,
	AUTHOR = "W.B. Frakes and R. Prieto-Diaz and C.J. Fox",
	TITLE = "Dare: Domain Analysis and Reuse Environment",
	JOURNAL = "Annals of Software Eng.",
	PUBLISHER ="IEEE Computer Society Press",
	VOLUME = {5},
	YEAR = {1998}
}

@book{Weiss:1999:SPE:317887,
	author = {Weiss, David M. and Lai, Chi Tau Robert},
	title = {Software product-line engineering: a family-based software development process},
	year = {1999},
	isbn = {0-201-69438-7},
	publisher = {Addison-Wesley Longman Publishing Co., Inc.},
	address = {Boston, MA, USA},
}

@ARTICLE{1020288,
	author={Kang, K.C. and Jaejoon Lee and Donohoe, P.},
	journal={Software, IEEE}, title={Feature-oriented product line engineering},
	year={2002},
	month={jul/aug},
	volume={19},
	number={4},
	pages={ 58 - 65},
	keywords={ FORM; commonalities; differences; feature-oriented product line engineering; feature-oriented reuse method; home integration system; software development management; software reusability;},
	doi={10.1109/MS.2002.1020288},
	ISSN={0740-7459},
}

@article{Bajracharya:2012:AMC:2318097.2318150,
	author = {Bajracharya, Sushil Krishna and Lopes, Cristina Videira},
	title = {Analyzing and mining a code search engine usage log},
	journal = {Empirical Softw. Engg.},
	issue_date = {August 2012},
	volume = {17},
	number = {4-5},
	month = aug,
	year = {2012},
	issn = {1382-3256},
	pages = {424--466},
	numpages = {43},
	url = {http://dx.doi.org/10.1007/s10664-010-9144-6},
	doi = {10.1007/s10664-010-9144-6},
	acmid = {2318150},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Code search engine, Mining topics, Usage log analysis},
} 

@inproceedings{Linstead:2007:MCC:1321631.1321709,
	author = {Linstead, Erik and Rigor, Paul and Bajracharya, Sushil and Lopes, Cristina and Baldi, Pierre},
	title = {Mining concepts from code with probabilistic topic models},
	booktitle = {Proceedings of the twenty-second IEEE/ACM international conference on Automated software engineering},
	series = {ASE '07},
	year = {2007},
	isbn = {978-1-59593-882-4},
	location = {Atlanta, Georgia, USA},
	pages = {461--464},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/1321631.1321709},
	doi = {10.1145/1321631.1321709},
	acmid = {1321709},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {mining software, program understanding, topic models},
} 

@inproceedings{McMillan:2012:RSC:2337223.2337323,
	author = {McMillan, Collin and Hariri, Negar and Poshyvanyk, Denys and Cleland-Huang, Jane and Mobasher, Bamshad},
	title = {Recommending source code for use in rapid software prototypes},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {848--858},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337323},
	acmid = {2337323},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@book{Gomaa:2004:DSP:983234,
	author = {Gomaa, Hassan},
	title = {Designing Software Product Lines with UML: From Use Cases to Pattern-Based Software Architectures},
	year = {2004},
	isbn = {0201775956},
	publisher = {Addison Wesley Longman Publishing Co., Inc.},
	address = {Redwood City, CA, USA},
}

@ARTICLE{Niu:Features2,
	AUTHOR="N.Niu and S.Easterbrook",
	TITLE="Extracting and Modeling Product Line Functional Requirements",
	JOURNAL="RE",
	LOCATION="Washington DC",
	YEAR ={2008},
}

@ARTICLE{Moon:Features3,
	AUTHOR="M.Moon and K.Yeom and H.S.Chae",
	TITLE="An approach to developing domain requirements as a core asset based on commonality and variability analysis in a product line",
	JOURNAL="TSE",
	VOLUME={31},
	ISSUE={7},
	YEAR={2005},
}

@inproceedings{Dumitru:11,
	author = {Dumitru, Horatiu and Gibiec, Marek and Hariri, Negar and Cleland-Huang, Jane and Mobasher, Bamshad and Castro-Herrera, Carlos and Mirakhorli, Mehdi},
	title = {On-demand feature recommendations derived from mining public product descriptions},
	booktitle = {ICSE},
	year = {2011},
	pages = {181--190},
}

@article{Holmes:2013:SPS:2377656.2377657,
	author = {Holmes, Reid and Walker, Robert J.},
	title = {Systematizing pragmatic software reuse},
	journal = {ACM Trans. Softw. Eng. Methodol.},
	issue_date = {November 2012},
	volume = {21},
	number = {4},
	month = feb,
	year = {2013},
	issn = {1049-331X},
	pages = {20:1--20:44},
	articleno = {20},
	numpages = {44},
	url = {http://doi.acm.org/10.1145/2377656.2377657},
	doi = {10.1145/2377656.2377657},
	acmid = {2377657},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Gilligan, Software reuse, lightweight process and tooling, low commitment, planning, pragmatic software reuse, pragmatic-reuse plan enactment, pragmatic-reuse plans, source code investigation, white box reuse},
} 

@inproceedings{Holmes:2009:ART:1747491.1747534,
	author = {Holmes, Reid and Ratchford, Tristan and Robillard, Martin P. and Walker, Robert J.},
	title = {Automatically Recommending Triage Decisions for Pragmatic Reuse Tasks},
	booktitle = {Proceedings of the 2009 IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '09},
	year = {2009},
	isbn = {978-0-7695-3891-4},
	pages = {397--408},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/ASE.2009.65},
	doi = {10.1109/ASE.2009.65},
	acmid = {1747534},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {pragmatic software reuse tasks, triage decisions, recommendation systems, structural relevance, cost, source code analysis, retroactive evaluation},
}

@inproceedings{Kotonya:2008:ORL:1478087.1478113,
	author = {Kotonya, Gerald and Lock, Simon and Mariani, John},
	title = {Opportunistic Reuse: Lessons from Scrapheap Software Development},
	booktitle = {Proceedings of the 11th International Symposium on Component-Based Software Engineering},
	series = {CBSE '08},
	year = {2008},
	isbn = {978-3-540-87890-2},
	location = {Karlsruhe, Germany},
	pages = {302--309},
	numpages = {8},
	url = {http://dx.doi.org/10.1007/978-3-540-87891-9_20},
	doi = {10.1007/978-3-540-87891-9_20},
	acmid = {1478113},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
}

@inproceedings{Brandt:2010:EPI:1753326.1753402,
	author = {Brandt, Joel and Dontcheva, Mira and Weskamp, Marcos and Klemmer, Scott R.},
	title = {Example-centric programming: integrating web search into the development environment},
	booktitle = {Proceedings of the 28th international conference on Human factors in computing systems},
	series = {CHI '10},
	year = {2010},
	isbn = {978-1-60558-929-9},
	location = {Atlanta, Georgia, USA},
	pages = {513--522},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1753326.1753402},
	doi = {10.1145/1753326.1753402},
	acmid = {1753402},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {example-centric development},
}

@inproceedings{Hartmann:2010:OPS:1753326.1753478,
	author = {Hartmann, Bj\"{o}rn and MacDougall, Daniel and Brandt, Joel and Klemmer, Scott R.},
	title = {What would other programmers do: suggesting solutions to error messages},
	booktitle = {Proceedings of the 28th international conference on Human factors in computing systems},
	series = {CHI '10},
	year = {2010},
	isbn = {978-1-60558-929-9},
	location = {Atlanta, Georgia, USA},
	pages = {1019--1028},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1753326.1753478},
	doi = {10.1145/1753326.1753478},
	acmid = {1753478},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, recommender systems},
}

@inproceedings{Weiser:1981:PS:800078.802557,
	author = {Weiser, Mark},
	title = {Program slicing},
	booktitle = {Proceedings of the 5th international conference on Software engineering},
	series = {ICSE '81},
	year = {1981},
	isbn = {0-89791-146-6},
	location = {San Diego, California, United States},
	pages = {439--449},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=800078.802557},
	acmid = {802557},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Data flow analysis, Debugging, Human factors, Program maintenance, Program metrics, Software tools},
}

@article{DBLP:journals/tse/Weiser84,
	author    = {Mark Weiser},
	title     = {Program Slicing},
	journal   = {IEEE Trans. Software Eng.},
	volume    = {10},
	number    = {4},
	year      = {1984},
	pages     = {352-357},
	ee        = {http://doi.ieeecomputersociety.org/10.1109/TSE.1984.5010248},
	bibsource = {DBLP, http://dblp.uni-trier.de}
} 

@article{Horwitz:1988:ISU:960116.53994,
	author = {Horwitz, S. and Reps, T. and Binkley, D.},
	title = {Interprocedural slicing using dependence graphs},
	journal = {SIGPLAN Not.},
	issue_date = {July 1988},
	volume = {23},
	number = {7},
	month = jun,
	year = {1988},
	issn = {0362-1340},
	pages = {35--46},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/960116.53994},
	doi = {10.1145/960116.53994},
	acmid = {53994},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Horwitz:1988:ISU:53990.53994,
	author = {Horwitz, S. and Reps, T. and Binkley, D.},
	title = {Interprocedural slicing using dependence graphs},
	booktitle = {Proceedings of the ACM SIGPLAN 1988 conference on Programming Language design and Implementation},
	series = {PLDI '88},
	year = {1988},
	isbn = {0-89791-269-1},
	location = {Atlanta, Georgia, United States},
	pages = {35--46},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/53990.53994},
	doi = {10.1145/53990.53994},
	acmid = {53994},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Malenfant:2001:FAD:846228.848706,
	author = {Malenfant, Bruno},
	title = {Flow Analysis to Detect Blocked Statements},
	booktitle = {Proceedings of the IEEE International Conference on Software Maintenance (ICSM'01)},
	series = {ICSM '01},
	year = {2001},
	isbn = {0-7695-1189-9},
	pages = {62--},
	url = {http://dx.doi.org/10.1109/ICSM.2001.972712},
	doi = {10.1109/ICSM.2001.972712},
	acmid = {848706},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {Blocking analysis, inter-procedural flow analysis, software evaluation},
}

@article{Horwitz:1990:ISU:77606.77608,
	author = {Horwitz, Susan and Reps, Thomas and Binkley, David},
	title = {Interprocedural slicing using dependence graphs},
	journal = {ACM Trans. Program. Lang. Syst.},
	issue_date = {Jan. 1990},
	volume = {12},
	number = {1},
	month = jan,
	year = {1990},
	issn = {0164-0925},
	pages = {26--60},
	numpages = {35},
	url = {http://doi.acm.org/10.1145/77606.77608},
	doi = {10.1145/77606.77608},
	acmid = {77608},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Mock:2005:PSD:1083824.1084006,
	author = {Mock, Markus and Atkinson, Darren C. and Chambers, Craig and Eggers, Susan J.},
	title = {Program Slicing with Dynamic Points-To Sets},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {August 2005},
	volume = {31},
	number = {8},
	month = aug,
	year = {2005},
	issn = {0098-5589},
	pages = {657--678},
	numpages = {22},
	url = {http://dx.doi.org/10.1109/TSE.2005.94},
	doi = {10.1109/TSE.2005.94},
	acmid = {1084006},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Index Terms- Dynamic analysis, Index Terms- Dynamic analysis, points-to analysis, program slicing., points-to analysis, program slicing.},
} 

@inproceedings{Venkatesh:1991:SAP:113445.113455,
	author = {Venkatesh, G. A.},
	title = {The semantic approach to program slicing},
	booktitle = {Proceedings of the ACM SIGPLAN 1991 conference on Programming language design and implementation},
	series = {PLDI '91},
	year = {1991},
	isbn = {0-89791-428-7},
	location = {Toronto, Ontario, Canada},
	pages = {107--119},
	numpages = {13},
	url = {http://doi.acm.org/10.1145/113445.113455},
	doi = {10.1145/113445.113455},
	acmid = {113455},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{Krinke:1998:SST:277631.277638,
	author = {Krinke, Jens},
	title = {Static slicing of threaded programs},
	booktitle = {Proceedings of the 1998 ACM SIGPLAN-SIGSOFT workshop on Program analysis for software tools and engineering},
	series = {PASTE '98},
	year = {1998},
	isbn = {1-58113-055-4},
	location = {Montreal, Quebec, Canada},
	pages = {35--42},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/277631.277638},
	doi = {10.1145/277631.277638},
	acmid = {277638},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Giffhorn:2009:PSC:1530080.1530094,
	author = {Giffhorn, Dennis and Hammer, Christian},
	title = {Precise slicing of concurrent programs},
	journal = {Automated Software Engg.},
	issue_date = {June      2009},
	volume = {16},
	number = {2},
	month = jun,
	year = {2009},
	issn = {0928-8910},
	pages = {197--234},
	numpages = {38},
	url = {http://dx.doi.org/10.1007/s10515-009-0048-x},
	doi = {10.1007/s10515-009-0048-x},
	acmid = {1530094},
	publisher = {Kluwer Academic Publishers},
	address = {Hingham, MA, USA},
	keywords = {Concurrency, Program analysis, Slicing, Threads},
}

@article{Binkley:2007:ESS:1217295.1217297,
	author = {Binkley, David and Gold, Nicolas and Harman, Mark},
	title = {An empirical study of static program slice size},
	journal = {ACM Trans. Softw. Eng. Methodol.},
	issue_date = {April 2007},
	volume = {16},
	number = {2},
	month = apr,
	year = {2007},
	issn = {1049-331X},
	articleno = {8},
	url = {http://doi.acm.org/10.1145/1217295.1217297},
	doi = {10.1145/1217295.1217297},
	acmid = {1217297},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Program slicing, slice size},
} 

@article{Agrawal:1990:DPS:93548.93576,
	author = {Agrawal, Hiralal and Horgan, Joseph R.},
	title = {Dynamic program slicing},
	journal = {SIGPLAN Not.},
	issue_date = {Jun. 1990},
	volume = {25},
	number = {6},
	month = jun,
	year = {1990},
	issn = {0362-1340},
	pages = {246--256},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/93548.93576},
	doi = {10.1145/93548.93576},
	acmid = {93576},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Binkley:2007:ESO:1290520.1290523,
	author = {Binkley, David and Harman, Mark and Krinke, Jens},
	title = {Empirical study of optimization techniques for massive slicing},
	journal = {ACM Trans. Program. Lang. Syst.},
	issue_date = {November 2007},
	volume = {30},
	number = {1},
	month = nov,
	year = {2007},
	issn = {0164-0925},
	articleno = {3},
	url = {http://doi.acm.org/10.1145/1290520.1290523},
	doi = {10.1145/1290520.1290523},
	acmid = {1290523},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Slicing, empirical study, internal representation, performance enhancement},
}

@article{Krinke:2006:ECP:1167771.1167775,
	author = {Krinke, Jens},
	title = {Effects of context on program slicing},
	journal = {J. Syst. Softw.},
	issue_date = {September 2006},
	volume = {79},
	number = {9},
	month = sep,
	year = {2006},
	issn = {0164-1212},
	pages = {1249--1260},
	numpages = {12},
	url = {http://dx.doi.org/10.1016/j.jss.2006.02.040},
	doi = {10.1016/j.jss.2006.02.040},
	acmid = {1167775},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {program analysis, program slicing},
}

@article{Canfora1998595,
	title = "Conditioned program slicing",
	journal = "Information and Software Technology",
	volume = "40",
	number = "11–12",
	pages = "595 - 607",
	year = "1998",
	note = "",
	issn = "0950-5849",
	doi = "10.1016/S0950-5849(98)00086-X",
	url = "http://www.sciencedirect.com/science/article/pii/S095058499800086X",
	author = "Gerardo Canfora and Aniello Cimitile and Andrea De Lucia",
}

@article{Korel:1997:CDP:249578.249587,
	author = {Korel, Bogdan},
	title = {Computation of Dynamic Program Slices for Unstructured Programs},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {January 1997},
	volume = {23},
	number = {1},
	month = jan,
	year = {1997},
	issn = {0098-5589},
	pages = {17--34},
	numpages = {18},
	url = {http://dx.doi.org/10.1109/32.581327},
	doi = {10.1109/32.581327},
	acmid = {249587},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Program slicing, dynamic program slicing, removable block, control dependence, data dependence, execution trace, unstructured program, debugging.},
} 

@article{DBLP:journals/infsof/KorelR98,
	author    = {Bogdan Korel and
	Juergen Rilling},
	title     = {Dynamic program slicing methods},
	journal   = {Information {\&} Software Technology},
	volume    = {40},
	number    = {11-12},
	year      = {1998},
	pages     = {647-659},
	ee        = {http://dx.doi.org/10.1016/S0950-5849(98)00089-5},
	bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{Xu:2005:BSP:1050849.1050865,
	author = {Xu, Baowen and Qian, Ju and Zhang, Xiaofang and Wu, Zhongqiang and Chen, Lin},
	title = {A brief survey of program slicing},
	journal = {SIGSOFT Softw. Eng. Notes},
	issue_date = {March 2005},
	volume = {30},
	number = {2},
	month = mar,
	year = {2005},
	issn = {0163-5948},
	pages = {1--36},
	numpages = {36},
	url = {http://doi.acm.org/10.1145/1050849.1050865},
	doi = {10.1145/1050849.1050865},
	acmid = {1050865},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, dependence analysis, pointer analysis, program analysis, program slicing},
}

@techreport{
	yiji_2012_tr,
	author = "Yiji Zhang and Raul Santelices",
	institution = "University of Notre Dame Computer Science Department",
	title = "Predicting Runtime Data Dependences for Slice Inspection Prioritization",
	number = "2012-02",
	month = "July",
	year = "2012"
}

@inproceedings{Zhang:2006:PDS:1133981.1134002,
	author = {Zhang, Xiangyu and Gupta, Neelam and Gupta, Rajiv},
	title = {Pruning dynamic slices with confidence},
	booktitle = {Proceedings of the 2006 ACM SIGPLAN conference on Programming language design and implementation},
	series = {PLDI '06},
	year = {2006},
	isbn = {1-59593-320-4},
	location = {Ottawa, Ontario, Canada},
	pages = {169--180},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1133981.1134002},
	doi = {10.1145/1133981.1134002},
	acmid = {1134002},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {data and control dependences, debugging, dynamic slicing},
}

@inproceedings{Sridharan:2007:TS:1250734.1250748,
	author = {Sridharan, Manu and Fink, Stephen J. and Bodik, Rastislav},
	title = {Thin slicing},
	booktitle = {Proceedings of the 2007 ACM SIGPLAN conference on Programming language design and implementation},
	series = {PLDI '07},
	year = {2007},
	isbn = {978-1-59593-633-2},
	location = {San Diego, California, USA},
	pages = {112--122},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1250734.1250748},
	doi = {10.1145/1250734.1250748},
	acmid = {1250748},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, program understanding, slicing},
}

@article{Gallagher:1991:UPS:126244.126248,
	author = {Gallagher, Keith Brian and Lyle, James R.},
	title = {Using Program Slicing in Software Maintenance},
	journal = {IEEE Trans. Softw. Eng.},
	issue_date = {August 1991},
	volume = {17},
	number = {8},
	month = aug,
	year = {1991},
	issn = {0098-5589},
	pages = {751--761},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/32.83912},
	doi = {10.1109/32.83912},
	acmid = {126248},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {line number, linear time, program slice, program slicing, program testing, semantically consistent changes, set inclusion, single variable decomposition slices, slice-based decomposition, software maintenance, software maintenance problem, unmodified components},
}

@inproceedings{Robillard:2002:CGF:581339.581390,
	author = {Robillard, Martin P. and Murphy, Gail C.},
	title = {Concern graphs: finding and describing concerns using structural program dependencies},
	booktitle = {Proceedings of the 24th International Conference on Software Engineering},
	series = {ICSE '02},
	year = {2002},
	isbn = {1-58113-472-X},
	location = {Orlando, Florida},
	pages = {406--416},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/581339.581390},
	doi = {10.1145/581339.581390},
	acmid = {581390},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Mund:2006:EID:1150566.1150570,
	author = {Mund, G. B. and Mall, Rajib},
	title = {An efficient interprocedural dynamic slicing method},
	journal = {J. Syst. Softw.},
	issue_date = {June 2006},
	volume = {79},
	number = {6},
	month = jun,
	year = {2006},
	issn = {0164-1212},
	pages = {791--806},
	numpages = {16},
	url = {http://dx.doi.org/10.1016/j.jss.2005.07.024},
	doi = {10.1016/j.jss.2005.07.024},
	acmid = {1150570},
	publisher = {Elsevier Science Inc.},
	address = {New York, NY, USA},
	keywords = {Control dependence graph, Control flow graph, Dynamic slicing, Program debugging, Program dependence graph, Program slicing, Static slicing},
}

@inproceedings{Dunn:1993:ADR:257572.257660,
	author = {Dunn, Michael F. and Knight, John C.},
	title = {Automating the detection of reusable parts in existing software},
	booktitle = {Proceedings of the 15th international conference on Software Engineering},
	series = {ICSE '93},
	year = {1993},
	isbn = {0-89791-588-7},
	location = {Baltimore, Maryland, United States},
	pages = {381--390},
	numpages = {10},
	url = {http://dl.acm.org/citation.cfm?id=257572.257660},
	acmid = {257660},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
	keywords = {Prolog, expert system, reengineering, reusable components, software reuse},
}

@article{Zhang:2010:BAH:1944279.1944280,
	author = {Zhang, Lu and Luo, Jing and Li, He and Sun, Jiasu and Mei, Hong},
	title = {A biting-down approach to hierarchical decomposition of object-oriented systems based on structure analysis},
	journal = {J. Softw. Maint. Evol.},
	issue_date = {December 2010},
	volume = {22},
	number = {8},
	month = dec,
	year = {2010},
	issn = {1532-060X},
	pages = {567--596},
	numpages = {30},
	url = {http://dx.doi.org/10.1002/smr.417},
	doi = {10.1002/smr.417},
	acmid = {1944280},
	publisher = {John Wiley \& Sons, Inc.},
	address = {New York, NY, USA},
	keywords = {architecture recovery, hierarchical system decomposition, software clustering},
}

@article{Caldiera:1991:IQR:103293.103294,
	author = {Caldiera, Gianluigi and Basili, Victor R.},
	title = {Identifying and Qualifying Reusable Software Components},
	journal = {Computer},
	issue_date = {February 1991},
	volume = {24},
	number = {2},
	month = feb,
	year = {1991},
	issn = {0018-9162},
	pages = {61--70},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/2.67210},
	doi = {10.1109/2.67210},
	acmid = {103294},
	publisher = {IEEE Computer Society Press},
	address = {Los Alamitos, CA, USA},
}

@inproceedings{Schach:1995:MTC:315891.316024,
	author = {Schach, Stephen R. and Yang, Xuefeng},
	title = {Metrics for targeting candidates for reuse: an experimental approach},
	booktitle = {Proceedings of the 1995 ACM symposium on Applied computing},
	series = {SAC '95},
	year = {1995},
	isbn = {0-89791-658-1},
	location = {Nashville, Tennessee, United States},
	pages = {379--383},
	numpages = {5},
	url = {http://doi.acm.org/10.1145/315891.316024},
	doi = {10.1145/315891.316024},
	acmid = {316024},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {accidental reuse, experimentation, reusability, software metrics},
}

@article{Roemer:2012:RPS:2133375.2133377,
	author = {Roemer, Ryan and Buchanan, Erik and Shacham, Hovav and Savage, Stefan},
	title = {Return-Oriented Programming: Systems, Languages, and Applications},
	journal = {ACM Trans. Inf. Syst. Secur.},
	issue_date = {March 2012},
	volume = {15},
	number = {1},
	month = mar,
	year = {2012},
	issn = {1094-9224},
	pages = {2:1--2:34},
	articleno = {2},
	numpages = {34},
	url = {http://doi.acm.org/10.1145/2133375.2133377},
	doi = {10.1145/2133375.2133377},
	acmid = {2133377},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {NX, RISC, Return-oriented programming, SPARC, W-xor-X, attacks, control flow integrity, memory safety, return-into-libc, x86},
}

@inproceedings{Checkoway:2010:RPW:1866307.1866370,
	author = {Checkoway, Stephen and Davi, Lucas and Dmitrienko, Alexandra and Sadeghi, Ahmad-Reza and Shacham, Hovav and Winandy, Marcel},
	title = {Return-oriented programming without returns},
	booktitle = {Proceedings of the 17th ACM conference on Computer and communications security},
	series = {CCS '10},
	year = {2010},
	isbn = {978-1-4503-0245-6},
	location = {Chicago, Illinois, USA},
	pages = {559--572},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/1866307.1866370},
	doi = {10.1145/1866307.1866370},
	acmid = {1866370},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {arm, return-oriented programming, x86},
}

@inproceedings{Chen:2010:EDR:1940366.1940380,
	author = {Chen, Ping and Xing, Xiao and Han, Hao and Mao, Bing and Xie, Li},
	title = {Efficient detection of the return-oriented programming malicious code},
	booktitle = {Proceedings of the 6th international conference on Information systems security},
	series = {ICISS'10},
	year = {2010},
	isbn = {3-642-17713-1, 978-3-642-17713-2},
	location = {Gandhinagar, India},
	pages = {140--155},
	numpages = {16},
	url = {http://dl.acm.org/citation.cfm?id=1940366.1940380},
	acmid = {1940380},
	publisher = {Springer-Verlag},
	address = {Berlin, Heidelberg},
}

@inproceedings{Bletsch:2011:JPN:1966913.1966919,
	author = {Bletsch, Tyler and Jiang, Xuxian and Freeh, Vince W. and Liang, Zhenkai},
	title = {Jump-oriented programming: a new class of code-reuse attack},
	booktitle = {Proceedings of the 6th ACM Symposium on Information, Computer and Communications Security},
	series = {ASIACCS '11},
	year = {2011},
	isbn = {978-1-4503-0564-8},
	location = {Hong Kong, China},
	pages = {30--40},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1966913.1966919},
	doi = {10.1145/1966913.1966919},
	acmid = {1966919},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@INPROCEEDINGS{mohan12woot,
	author = "Vishwath Mohan and Kevin W. Hamlen",
	title = "{Frankenstein}: Stitching Malware from Benign Binaries",
	booktitle = "Proceedings of the 6th USENIX Workshop on Offensive Technologies (WOOT)",
	address = "Bellevue, Washington",
	month = "August",
	year = 2012,
}

@article{Il68,
	added-at = {2006-11-21T05:45:44.000+0100},
	author = {McIlroy, M. D.},
	biburl = {http://www.bibsonomy.org/bibtex/2bdd8dc73582a1061c5353c143b85bb9e/berger},
	chapter = 14,
	interhash = {f27eb07f75ede5abc8af427c9d186453},
	intrahash = {bdd8dc73582a1061c5353c143b85bb9e},
	journal = {Proc. NATO Conf. on Software Engineering, Garmisch, Germany},
	keywords = {Software-Engineering},
	publisher = {Springer-Verlag},
	timestamp = {2006-11-21T05:45:44.000+0100},
	title = {Mass-produced software components},
	year = 1968
}

@INPROCEEDINGS{Howison04theperils,
	author = {James Howison and Kevin Crowston},
	title = {The perils and pitfalls of mining SourceForge},
	booktitle = {In Proceedings of the International Workshop on Mining Software Repositories (MSR 2004},
	year = {2004},
	pages = {7--11}
}

@article{Dunlap:2002:REI:844128.844148,
	author = {Dunlap, George W. and King, Samuel T. and Cinar, Sukru and Basrai, Murtaza A. and Chen, Peter M.},
	title = {ReVirt: enabling intrusion analysis through virtual-machine logging and replay},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {Winter 2002},
	volume = {36},
	number = {SI},
	month = dec,
	year = {2002},
	issn = {0163-5980},
	pages = {211--224},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/844128.844148},
	doi = {10.1145/844128.844148},
	acmid = {844148},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@misc{GDB:Website,
	author = {GNU},
	title = {The GNU Project Debugger},
	month = sep,
	year = {2012},
	note = {http://www.gnu.org/software/gdb/}
}

@article{LeBlanc:1987:DPP:32387.32396,
	author = {LeBlanc, T. J. and Mellor-Crummey, J. M.},
	title = {Debugging Parallel Programs with Instant Replay},
	journal = {IEEE Trans. Comput.},
	issue_date = {April 1987},
	volume = {36},
	number = {4},
	month = apr,
	year = {1987},
	issn = {0018-9340},
	pages = {471--482},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/TC.1987.1676929},
	doi = {10.1109/TC.1987.1676929},
	acmid = {32396},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {CREW protocols, distributed debugging, execution replay, parallel programming, program instrumentation, shared objects, shared objects, CREW protocols, distributed debugging, execution replay, parallel programming, program instrumentation},
}

@inproceedings{Balzer:1969:EED:1476793.1476881,
	author = {Balzer, R. M.},
	title = {EXDAMS: extendable debugging and monitoring system},
	booktitle = {Proceedings of the May 14-16, 1969, spring joint computer conference},
	series = {AFIPS '69 (Spring)},
	year = {1969},
	location = {Boston, Massachusetts},
	pages = {567--580},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/1476793.1476881},
	doi = {10.1145/1476793.1476881},
	acmid = {1476881},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Bacon:1991:HRM:122759.122777,
	author = {Bacon, David F. and Goldstein, Seth Copen},
	title = {Hardware-assisted replay of multiprocessor programs},
	booktitle = {Proceedings of the 1991 ACM/ONR workshop on Parallel and distributed debugging},
	series = {PADD '91},
	year = {1991},
	isbn = {0-89791-457-0},
	location = {Santa Cruz, California, United States},
	pages = {194--206},
	numpages = {13},
	url = {http://doi.acm.org/10.1145/122759.122777},
	doi = {10.1145/122759.122777},
	acmid = {122777},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Devietti:2009:DDS:1508244.1508255,
	author = {Devietti, Joseph and Lucia, Brandon and Ceze, Luis and Oskin, Mark},
	title = {DMP: deterministic shared memory multiprocessing},
	booktitle = {Proceedings of the 14th international conference on Architectural support for programming languages and operating systems},
	series = {ASPLOS '09},
	year = {2009},
	isbn = {978-1-60558-406-5},
	location = {Washington, DC, USA},
	pages = {85--96},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1508244.1508255},
	doi = {10.1145/1508244.1508255},
	acmid = {1508255},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, determinism, multicores, parallel programming},
}

@inproceedings{Hower:2008:REE:1381306.1382144,
	author = {Hower, Derek R. and Hill, Mark D.},
	title = {Rerun: Exploiting Episodes for Lightweight Memory Race Recording},
	booktitle = {Proceedings of the 35th Annual International Symposium on Computer Architecture},
	series = {ISCA '08},
	year = {2008},
	isbn = {978-0-7695-3174-8},
	pages = {265--276},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/ISCA.2008.26},
	doi = {10.1109/ISCA.2008.26},
	acmid = {1382144},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {Multicore, Determinism, Race Recording},
}

@inproceedings{Montesinos:2008:DRD:1381306.1382146,
	author = {Montesinos, Pablo and Ceze, Luis and Torrellas, Josep},
	title = {DeLorean: Recording and Deterministically Replaying Shared-Memory Multiprocessor Execution Ef?ciently},
	booktitle = {Proceedings of the 35th Annual International Symposium on Computer Architecture},
	series = {ISCA '08},
	year = {2008},
	isbn = {978-0-7695-3174-8},
	pages = {289--300},
	numpages = {12},
	url = {http://dx.doi.org/10.1109/ISCA.2008.36},
	doi = {10.1109/ISCA.2008.36},
	acmid = {1382146},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Montesinos:2009:CSI:1508244.1508254,
	author = {Montesinos, Pablo and Hicks, Matthew and King, Samuel T. and Torrellas, Josep},
	title = {Capo: a software-hardware interface for practical deterministic multiprocessor replay},
	booktitle = {Proceedings of the 14th international conference on Architectural support for programming languages and operating systems},
	series = {ASPLOS '09},
	year = {2009},
	isbn = {978-1-60558-406-5},
	location = {Washington, DC, USA},
	pages = {73--84},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1508244.1508254},
	doi = {10.1145/1508244.1508254},
	acmid = {1508254},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {capo, capoone, deterministic replay, replay sphere},
}

@article{Narayanasamy:2006:RSM:1168917.1168886,
	author = {Narayanasamy, Satish and Pereira, Cristiano and Calder, Brad},
	title = {Recording shared memory dependencies using strata},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {December 2006},
	volume = {40},
	number = {5},
	month = oct,
	year = {2006},
	issn = {0163-5980},
	pages = {229--240},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1168917.1168886},
	doi = {10.1145/1168917.1168886},
	acmid = {1168886},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, dependencies, logging, replay, shared memory, strata},
}

@article{Narayanasamy:2005:BCR:1080695.1069994,
	author = {Narayanasamy, Satish and Pokam, Gilles and Calder, Brad},
	title = {BugNet: Continuously Recording Program Execution for Deterministic Replay Debugging},
	journal = {SIGARCH Comput. Archit. News},
	issue_date = {May 2005},
	volume = {33},
	number = {2},
	month = may,
	year = {2005},
	issn = {0163-5964},
	pages = {284--295},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1080695.1069994},
	doi = {10.1145/1080695.1069994},
	acmid = {1069994},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Olszewski:2009:KED:1508284.1508256,
	author = {Olszewski, Marek and Ansel, Jason and Amarasinghe, Saman},
	title = {Kendo: efficient deterministic multithreading in software},
	journal = {SIGPLAN Not.},
	issue_date = {March 2009},
	volume = {44},
	number = {3},
	month = mar,
	year = {2009},
	issn = {0362-1340},
	pages = {97--108},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1508284.1508256},
	doi = {10.1145/1508284.1508256},
	acmid = {1508256},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, determinism, deterministic multithreading, multicore, parallel programming},
}

@article{Bressoud:1996:HFT:225535.225538,
	author = {Bressoud, Thomas C. and Schneider, Fred B.},
	title = {Hypervisor-based fault tolerance},
	journal = {ACM Trans. Comput. Syst.},
	issue_date = {Feb. 1996},
	volume = {14},
	number = {1},
	month = feb,
	year = {1996},
	issn = {0734-2071},
	pages = {80--107},
	numpages = {28},
	url = {http://doi.acm.org/10.1145/225535.225538},
	doi = {10.1145/225535.225538},
	acmid = {225538},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {fault-tolerant computing system, primary/backup approach, virtual-machine manager},
}

@inproceedings{Dunlap:2008:ERM:1346256.1346273,
	author = {Dunlap, George W. and Lucchetti, Dominic G. and Fetterman, Michael A. and Chen, Peter M.},
	title = {Execution replay of multiprocessor virtual machines},
	booktitle = {Proceedings of the fourth ACM SIGPLAN/SIGOPS international conference on Virtual execution environments},
	series = {VEE '08},
	year = {2008},
	isbn = {978-1-59593-796-4},
	location = {Seattle, WA, USA},
	pages = {121--130},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1346256.1346273},
	doi = {10.1145/1346256.1346273},
	acmid = {1346273},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {ReVirt, Xen, determinism, direct memory access, execution replay, hardware page protections, multiprocessors, multithreading, virtual machines},
}

@article{Chow:2010:MRC:1837854.1736002,
	author = {Chow, Jim and Lucchetti, Dominic and Garfinkel, Tal and Lefebvre, Geoffrey and Gardner, Ryan and Mason, Joshua and Small, Sam and Chen, Peter M.},
	title = {Multi-stage replay with crosscut},
	journal = {SIGPLAN Not.},
	issue_date = {July 2010},
	volume = {45},
	number = {7},
	month = mar,
	year = {2010},
	issn = {0362-1340},
	pages = {13--24},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1837854.1736002},
	doi = {10.1145/1837854.1736002},
	acmid = {1736002},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {design, experimentation, performance, replay, security, virtual machines},
}

@inproceedings{Geels:2006:RDD:1267359.1267386,
	author = {Geels, Dennis and Altekar, Gautam and Shenker, Scott and Stoica, Ion},
	title = {Replay debugging for distributed applications},
	booktitle = {Proceedings of the annual conference on USENIX '06 Annual Technical Conference},
	series = {ATEC '06},
	year = {2006},
	location = {Boston, MA},
	pages = {27--27},
	numpages = {1},
	url = {http://dl.acm.org/citation.cfm?id=1267359.1267386},
	acmid = {1267386},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
}

@inproceedings{Guo:2008:RAK:1855741.1855755,
	author = {Guo, Zhenyu and Wang, Xi and Tang, Jian and Liu, Xuezheng and Xu, Zhilei and Wu, Ming and Kaashoek, M. Frans and Zhang, Zheng},
	title = {R2: an application-level kernel for record and replay},
	booktitle = {Proceedings of the 8th USENIX conference on Operating systems design and implementation},
	series = {OSDI'08},
	year = {2008},
	location = {San Diego, California},
	pages = {193--208},
	numpages = {16},
	url = {http://dl.acm.org/citation.cfm?id=1855741.1855755},
	acmid = {1855755},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
}

@inproceedings{Saito:2005:JUL:1085130.1085139,
	author = {Saito, Yasushi},
	title = {Jockey: a user-space library for record-replay debugging},
	booktitle = {Proceedings of the sixth international symposium on Automated analysis-driven debugging},
	series = {AADEBUG'05},
	year = {2005},
	isbn = {1-59593-050-7},
	location = {Monterey, California, USA},
	pages = {69--76},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1085130.1085139},
	doi = {10.1145/1085130.1085139},
	acmid = {1085139},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Linux, checkpointing, debugging, execution record and replay, jockey, keywords, x86},
}

@inproceedings{Choi:1998:DRJ:281035.281041,
	author = {Choi, Jong-Deok and Srinivasan, Harini},
	title = {Deterministic replay of Java multithreaded applications},
	booktitle = {Proceedings of the SIGMETRICS symposium on Parallel and distributed tools},
	series = {SPDT '98},
	year = {1998},
	isbn = {1-58113-001-5},
	location = {Welches, Oregon, United States},
	pages = {48--59},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/281035.281041},
	doi = {10.1145/281035.281041},
	acmid = {281041},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Russinovich:1996:RCN:249069.231432,
	author = {Russinovich, Mark and Cogswell, Bryce},
	title = {Replay for concurrent non-deterministic shared-memory applications},
	journal = {SIGPLAN Not.},
	issue_date = {May 1996},
	volume = {31},
	number = {5},
	month = may,
	year = {1996},
	issn = {0362-1340},
	pages = {258--266},
	numpages = {9},
	url = {http://doi.acm.org/10.1145/249069.231432},
	doi = {10.1145/249069.231432},
	acmid = {231432},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {instruction counter, non-determinism, repeatable execution, shared memory},
}

@inproceedings{Bergheaud:2007:FTM:1270387.1270855,
	author = {Bergheaud, Philippe and Subhraveti, Dinesh and Vertes, Marc},
	title = {Fault Tolerance in Multiprocessor Systems Via Application Cloning},
	booktitle = {Proceedings of the 27th International Conference on Distributed Computing Systems},
	series = {ICDCS '07},
	year = {2007},
	isbn = {0-7695-2837-3},
	pages = {21--},
	url = {http://dx.doi.org/10.1109/ICDCS.2007.111},
	doi = {10.1109/ICDCS.2007.111},
	acmid = {1270855},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Bressoud:1998:TSS:795671.796914,
	author = {Bressoud, T. C.},
	title = {TFT: A Software System for Application-Transparent Fault Tolerance},
	booktitle = {Proceedings of the The Twenty-Eighth Annual International Symposium on Fault-Tolerant Computing},
	series = {FTCS '98},
	year = {1998},
	isbn = {0-8186-8470-4},
	pages = {128--},
	url = {http://dl.acm.org/citation.cfm?id=795671.796914},
	acmid = {796914},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Bressoud:1998:TSS:795671.796914,
	author = {Bressoud, T. C.},
	title = {TFT: A Software System for Application-Transparent Fault Tolerance},
	booktitle = {Proceedings of the The Twenty-Eighth Annual International Symposium on Fault-Tolerant Computing},
	series = {FTCS '98},
	year = {1998},
	isbn = {0-8186-8470-4},
	pages = {128--},
	url = {http://dl.acm.org/citation.cfm?id=795671.796914},
	acmid = {796914},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Srinivasan:2004:FLE:1247415.1247418,
	author = {Srinivasan, Sudarshan M. and Kandula, Srikanth and Andrews, Christopher R. and Zhou, Yuanyuan},
	title = {Flashback: a lightweight extension for rollback and deterministic replay for software debugging},
	booktitle = {Proceedings of the annual conference on USENIX Annual Technical Conference},
	series = {ATEC '04},
	year = {2004},
	location = {Boston, MA},
	pages = {3--3},
	numpages = {1},
	url = {http://dl.acm.org/citation.cfm?id=1247415.1247418},
	acmid = {1247418},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
}

@inproceedings{Thane:2000:UDR:1947412.1947455,
	author = {Thane, Henrik and Hansson, Hans},
	title = {Using deterministic replay for debugging of distributed real-time systems},
	booktitle = {Proceedings of the 12th Euromicro conference on Real-time systems},
	series = {Euromicro-RTS'00},
	year = {2000},
	isbn = {0-7695-0734-4},
	location = {Stockholm, Sweden},
	pages = {265--272},
	numpages = {8},
	url = {http://dl.acm.org/citation.cfm?id=1947412.1947455},
	acmid = {1947455},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {debugging, determinism, distributed real-time systems, monitoring, probe-effect, replay, testing},
} 

@article{Laadan:2010:TLA:1811099.1811057,
	author = {Laadan, Oren and Viennot, Nicolas and Nieh, Jason},
	title = {Transparent, lightweight application execution replay on commodity multiprocessor operating systems},
	journal = {SIGMETRICS Perform. Eval. Rev.},
	issue_date = {June 2010},
	volume = {38},
	number = {1},
	month = jun,
	year = {2010},
	issn = {0163-5999},
	pages = {155--166},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1811099.1811057},
	doi = {10.1145/1811099.1811057},
	acmid = {1811057},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {debugging, fault-tolerance, record-replay, virtualization},
}

@inproceedings{Xu:2003:FDR:859618.859633,
	author = {Xu, Min and Bodik, Rastislav and Hill, Mark D.},
	title = {A "flight data recorder" for enabling full-system multiprocessor deterministic replay},
	booktitle = {Proceedings of the 30th annual international symposium on Computer architecture},
	series = {ISCA '03},
	year = {2003},
	isbn = {0-7695-1945-8},
	location = {San Diego, California},
	pages = {122--135},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/859618.859633},
	doi = {10.1145/859618.859633},
	acmid = {859633},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Subhraveti:2011:RTP:1993744.1993757,
	author = {Subhraveti, Dinesh and Nieh, Jason},
	title = {Record and transplay: partial checkpointing for replay debugging across heterogeneous systems},
	booktitle = {Proceedings of the ACM SIGMETRICS joint international conference on Measurement and modeling of computer systems},
	series = {SIGMETRICS '11},
	year = {2011},
	isbn = {978-1-4503-0814-4},
	location = {San Jose, California, USA},
	pages = {109--120},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1993744.1993757},
	doi = {10.1145/1993744.1993757},
	acmid = {1993757},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {checkpoint-restart, record-replay, virtualization},
}

@article{Min:1991:ECA:106974.106996,
	author = {Min, Sang L. and Choi, Jong-Deok},
	title = {An efficient cache-based access anomaly detection scheme},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {Apr. 1991},
	volume = {25},
	number = {Special Issue},
	month = apr,
	year = {1991},
	issn = {0163-5980},
	pages = {235--244},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/106974.106996},
	doi = {10.1145/106974.106996},
	acmid = {106996},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Pan:1988:SRE:68210.69227,
	author = {Pan, Douglas Z. and Linton, Mark A.},
	title = {Supporting reverse execution for parallel programs},
	booktitle = {Proceedings of the 1988 ACM SIGPLAN and SIGOPS workshop on Parallel and distributed debugging},
	series = {PADD '88},
	year = {1988},
	isbn = {0-89791-296-9},
	location = {Madison, Wisconsin, United States},
	pages = {124--129},
	numpages = {6},
	url = {http://doi.acm.org/10.1145/68210.69227},
	doi = {10.1145/68210.69227},
	acmid = {69227},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Netzer:1993:OTR:174266.174268,
	author = {Netzer, Robert H. B.},
	title = {Optimal tracing and replay for debugging shared-memory parallel programs},
	booktitle = {Proceedings of the 1993 ACM/ONR workshop on Parallel and distributed debugging},
	series = {PADD '93},
	year = {1993},
	isbn = {0-89791-633-6},
	location = {San Diego, California, United States},
	pages = {1--11},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/174266.174268},
	doi = {10.1145/174266.174268},
	acmid = {174268},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Savage:1997:EDD:269005.266641,
	author = {Savage, Stefan and Burrows, Michael and Nelson, Greg and Sobalvarro, Patrick and Anderson, Thomas},
	title = {Eraser: a dynamic data race detector for multi-threaded programs},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {Dec. 1997},
	volume = {31},
	number = {5},
	month = oct,
	year = {1997},
	issn = {0163-5980},
	pages = {27--37},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/269005.266641},
	doi = {10.1145/269005.266641},
	acmid = {266641},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@article{Laadan:2007:DPV:1323293.1294289,
	author = {Laadan, Oren and Baratto, Ricardo A. and Phung, Dan B. and Potter, Shaya and Nieh, Jason},
	title = {DejaView: a personal virtual computer recorder},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {December 2007},
	volume = {41},
	number = {6},
	month = oct,
	year = {2007},
	issn = {0163-5980},
	pages = {279--292},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/1323293.1294289},
	doi = {10.1145/1323293.1294289},
	acmid = {1294289},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {desktop search, virtualization},
}

@inproceedings{Tsankov:2011:EHI:1989760.1990086,
	author = {Tsankov, Petar and Jin, Wei and Orso, Alessandro and Sinha, Saurabh},
	title = {Execution Hijacking: Improving Dynamic Analysis by Flying off Course},
	booktitle = {Proceedings of the 2011 Fourth IEEE International Conference on Software Testing, Verification and Validation},
	series = {ICST '11},
	year = {2011},
	isbn = {978-0-7695-4342-0},
	pages = {200--209},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICST.2011.45},
	doi = {10.1109/ICST.2011.45},
	acmid = {1990086},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@article{Silva:2012:VPS:2187671.2187674,
	author = {Silva, Josep},
	title = {A vocabulary of program slicing-based techniques},
	journal = {ACM Comput. Surv.},
	issue_date = {June 2012},
	volume = {44},
	number = {3},
	month = jun,
	year = {2012},
	issn = {0360-0300},
	pages = {12:1--12:41},
	articleno = {12},
	numpages = {41},
	url = {http://doi.acm.org/10.1145/2187671.2187674},
	doi = {10.1145/2187671.2187674},
	acmid = {2187674},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Program slicing, software engineering},
}

@inproceedings{LeVasseur:2004:SAR:1133572.1133617,
	author = {LeVasseur, Joshua and Uhlig, Volkmar},
	title = {A sledgehammer approach to reuse of legacy device drivers},
	booktitle = {Proceedings of the 11th workshop on ACM SIGOPS European workshop},
	series = {EW 11},
	year = {2004},
	location = {Leuven, Belgium},
	articleno = {24},
	url = {http://doi.acm.org/10.1145/1133572.1133617},
	doi = {10.1145/1133572.1133617},
	acmid = {1133617},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@inproceedings{Jamrozik:2012:ADS:2351676.2351716,
	author = {Jamrozik, Konrad and Fraser, Gordon and Tillmann, Nikolai and De Halleux, Jonathan},
	title = {Augmented dynamic symbolic execution},
	booktitle = {Proceedings of the 27th IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE 2012},
	year = {2012},
	isbn = {978-1-4503-1204-2},
	location = {Essen, Germany},
	pages = {254--257},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/2351676.2351716},
	doi = {10.1145/2351676.2351716},
	acmid = {2351716},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Test generation, boundary values, dynamic symbolic execution, mutation testing},
}

@inproceedings{Zhang:2010:TGV:1912607.1913317,
	author = {Zhang, Lingming and Xie, Tao and Zhang, Lu and Tillmann, Nikolai and de Halleux, Jonathan and Mei, Hong},
	title = {Test generation via Dynamic Symbolic Execution for mutation testing},
	booktitle = {Proceedings of the 2010 IEEE International Conference on Software Maintenance},
	series = {ICSM '10},
	year = {2010},
	isbn = {978-1-4244-8630-4},
	pages = {1--10},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICSM.2010.5609672},
	doi = {10.1109/ICSM.2010.5609672},
	acmid = {1913317},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Anand:2011:HCE:2190078.2190144,
	author = {Anand, Saswat and Harrold, Mary Jean},
	title = {Heap cloning: Enabling dynamic symbolic execution of java programs},
	booktitle = {Proceedings of the 2011 26th IEEE/ACM International Conference on Automated Software Engineering},
	series = {ASE '11},
	year = {2011},
	isbn = {978-1-4577-1638-6},
	pages = {33--42},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ASE.2011.6100071},
	doi = {10.1109/ASE.2011.6100071},
	acmid = {2190144},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
}

@inproceedings{Sen:2005:CCU:1081706.1081750,
	author = {Sen, Koushik and Marinov, Darko and Agha, Gul},
	title = {CUTE: a concolic unit testing engine for C},
	booktitle = {Proceedings of the 10th European software engineering conference held jointly with 13th ACM SIGSOFT international symposium on Foundations of software engineering},
	series = {ESEC/FSE-13},
	year = {2005},
	isbn = {1-59593-014-0},
	location = {Lisbon, Portugal},
	pages = {263--272},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1081706.1081750},
	doi = {10.1145/1081706.1081750},
	acmid = {1081750},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {concolic testing, data structure testing, explicit path model-checking, random testing, testing C programs, unit testing},
} 

@inproceedings{Godefroid:2005:DDA:1065010.1065036,
	author = {Godefroid, Patrice and Klarlund, Nils and Sen, Koushik},
	title = {DART: directed automated random testing},
	booktitle = {Proceedings of the 2005 ACM SIGPLAN conference on Programming language design and implementation},
	series = {PLDI '05},
	year = {2005},
	isbn = {1-59593-056-6},
	location = {Chicago, IL, USA},
	pages = {213--223},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/1065010.1065036},
	doi = {10.1145/1065010.1065036},
	acmid = {1065036},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {automated test generation, interfaces, program verification, random testing, software testing},
} 

@inproceedings{Rubinov:2012:ATS:2337223.2337438,
	author = {Rubinov, Konstantin and Wuttke, Jochen},
	title = {Augmenting test suites automatically},
	booktitle = {Proceedings of the 2012 International Conference on Software Engineering},
	series = {ICSE 2012},
	year = {2012},
	isbn = {978-1-4673-1067-3},
	location = {Zurich, Switzerland},
	pages = {1433--1434},
	numpages = {2},
	url = {http://dl.acm.org/citation.cfm?id=2337223.2337438},
	acmid = {2337438},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
}

@article{Thummalapenta:2011:SMS:2076021.2048083,
	author = {Thummalapenta, Suresh and Xie, Tao and Tillmann, Nikolai and de Halleux, Jonathan and Su, Zhendong},
	title = {Synthesizing method sequences for high-coverage testing},
	journal = {SIGPLAN Not.},
	issue_date = {October 2011},
	volume = {46},
	number = {10},
	month = oct,
	year = {2011},
	issn = {0362-1340},
	pages = {189--206},
	numpages = {18},
	url = {http://doi.acm.org/10.1145/2076021.2048083},
	doi = {10.1145/2076021.2048083},
	acmid = {2048083},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {object-oriented testing, symbolic execution},
}

@inproceedings{Fraser:2011:ECO:1989760.1990074,
	author = {Fraser, Gordon and Zeller, Andreas},
	title = {Exploiting Common Object Usage in Test Case Generation},
	booktitle = {Proceedings of the 2011 Fourth IEEE International Conference on Software Testing, Verification and Validation},
	series = {ICST '11},
	year = {2011},
	isbn = {978-0-7695-4342-0},
	pages = {80--89},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICST.2011.53},
	doi = {10.1109/ICST.2011.53},
	acmid = {1990074},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {test case generation, specification mining, readability},
}

@inproceedings{Zhang:2011:CSD:2001420.2001463,
	author = {Zhang, Sai and Saff, David and Bu, Yingyi and Ernst, Michael D.},
	title = {Combined static and dynamic automated test generation},
	booktitle = {Proceedings of the 2011 International Symposium on Software Testing and Analysis},
	series = {ISSTA '11},
	year = {2011},
	isbn = {978-1-4503-0562-4},
	location = {Toronto, Ontario, Canada},
	pages = {353--363},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/2001420.2001463},
	doi = {10.1145/2001420.2001463},
	acmid = {2001463},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {automated test generation, dynamic analyses, static},
}



/home/cmc/projects/eyesum/svn/paper/biblio.bib
@article{chawla2002smote,
	title={SMOTE: synthetic minority over-sampling technique},
	author={Chawla, Nitesh V. and Bowyer, Kevin W. and Hall, Lawrence O. and Kegelmeyer, W. Philip},
	journal={Journal of artificial intelligence research},
	volume={16},
	pages={321--357},
	year={2002}
}

@article{batista2004study,
	title={A study of the behavior of several methods for balancing machine learning training data},
	author={Batista, Gustavo EAPA and Prati, Ronaldo C and Monard, Maria Carolina},
	journal={ACM Sigkdd Explorations Newsletter},
	volume={6},
	number={1},
	pages={20--29},
	year={2004},
	publisher={ACM}
}

@article{chawla2004editorial,
	title={Editorial: special issue on learning from imbalanced data sets},
	author={Chawla, Nitesh V and Japkowicz, Nathalie and Kotcz, Aleksander},
	journal={ACM Sigkdd Explorations Newsletter},
	volume={6},
	number={1},
	pages={1--6},
	year={2004},
	publisher={ACM}
}

@article{hearst1998support,
	title={Support vector machines},
	author={Hearst, Marti A. and Dumais, Susan T and Osman, Edgar and Platt, John and Scholkopf, Bernhard},
	journal={IEEE Intelligent Systems and their Applications},
	volume={13},
	number={4},
	pages={18--28},
	year={1998},
	publisher={IEEE}
}

@article{chang2011libsvm,
	title={LIBSVM: a library for support vector machines},
	author={Chang, Chih-Chung and Lin, Chih-Jen},
	journal={ACM Transactions on Intelligent Systems and Technology (TIST)},
	volume={2},
	number={3},
	pages={27},
	year={2011},
	publisher={ACM}
}

@book{hosmer2004applied,
	title={Applied logistic regression},
	author={Hosmer Jr, David W and Lemeshow, Stanley},
	year={2004},
	publisher={John Wiley \& Sons}
}

@article{pedregosa2011scikit,
	title={Scikit-learn: Machine learning in Python},
	author={Pedregosa, Fabian and Varoquaux, Ga{\"e}l and Gramfort, Alexandre and Michel, Vincent and Thirion, Bertrand and Grisel, Olivier and Blondel, Mathieu and Prettenhofer, Peter and Weiss, Ron and Dubourg, Vincent and others},
	journal={Journal of Machine Learning Research},
	volume={12},
	number={Oct},
	pages={2825--2830},
	year={2011}
}

@article{hsu2003practical,
	title={A practical guide to support vector classification},
	author={Hsu, Chih-Wei and Chang, Chih-Chung and Lin, Chih-Jen and others},
	year={2003}
}

@book{ten2007doing,
	title={Doing conversation analysis},
	author={Ten Have, Paul},
	year={2007},
	publisher={Sage}
}

@book{ford2002language,
	title={The language of turn and sequence},
	author={Ford, Cecilia E and Fox, Barbara A and Thompson, Sandra A},
	year={2002},
	publisher={Oxford University Press on Demand}
}

@book{hutchby2008conversation,
	title={Conversation analysis},
	author={Hutchby, Ian and Wooffitt, Robin},
	year={2008},
	publisher={Polity}
}

@book{nishida2007convanalysis,
	title={Conversational Informatics: An Engineering Approach},
	author={Toyoaki Nishida},
	year={2007},
	publisher={Wiley}
}

@book{emanuel2007sequence,
	title={Sequence Organization in Interaction: A Primer in Conversation Analysis I},
	author={Emanuel A.. Schegloff},
	year={2007},
	publisher={Cambridge University Press}
}

@inproceedings{Barzilay:1999:IFC:1034678.1034760,
	author = {Barzilay, Regina and McKeown, Kathleen R. and Elhadad, Michael},
	title = {Information Fusion in the Context of Multi-document Summarization},
	booktitle = {Proceedings of the 37th Annual Meeting of the Association for Computational Linguistics on Computational Linguistics},
	series = {ACL '99},
	year = {1999},
	isbn = {1-55860-609-3},
	location = {College Park, Maryland},
	pages = {550--557},
	numpages = {8},
	url = {http://dx.doi.org/10.3115/1034678.1034760},
	doi = {10.3115/1034678.1034760},
	acmid = {1034760},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
}

@article{gupta2010survey,
	title={A survey of text summarization extractive techniques},
	author={Gupta, Vishal and Lehal, Gurpreet Singh},
	journal={Journal of emerging technologies in web intelligence},
	volume={2},
	number={3},
	pages={258--268},
	year={2010}
}

@inproceedings{Buse:2008:ADI:1390630.1390664,
	author = {Buse, Raymond P.L. and Weimer, Westley R.},
	title = {Automatic documentation inference for exceptions},
	booktitle = {Proceedings of the 2008 international symposium on Software testing and analysis},
	series = {ISSTA '08},
	year = {2008},
	isbn = {978-1-60558-050-0},
	location = {Seattle, WA, USA},
	pages = {273--282},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1390630.1390664},
	doi = {10.1145/1390630.1390664},
	acmid = {1390664},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation inference, exception handling, software documentation},
}

@inproceedings{Sridhara:2010:TAG:1858996.1859006,
	author = {Sridhara, Giriprasad and Hill, Emily and Muppaneni, Divya and Pollock, Lori and Vijay-Shanker, K.},
	title = {Towards automatically generating summary comments for Java methods},
	booktitle = {Proceedings of the IEEE/ACM international conference on Automated software engineering},
	series = {ASE '10},
	year = {2010},
	isbn = {978-1-4503-0116-9},
	location = {Antwerp, Belgium},
	pages = {43--52},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1858996.1859006},
	doi = {10.1145/1858996.1859006},
	acmid = {1859006},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {comment generation, method summarization, natural language program analysis},
}

@inproceedings{Sridhara:2011:GPC:2057176.2057211,
	author = {Sridhara, Giriprasad and Pollock, Lori and Vijay-Shanker, K.},
	title = {Generating Parameter Comments and Integrating with Method Summaries},
	booktitle = {Proceedings of the 2011 IEEE 19th International Conference on Program Comprehension},
	series = {ICPC '11},
	year = {2011},
	isbn = {978-0-7695-4398-7},
	pages = {71--80},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICPC.2011.28},
	doi = {10.1109/ICPC.2011.28},
	acmid = {2057211},
	keywords = {documentation, software maintenance}
} 

@inproceedings{Sridhara:2011:ADD:1985793.1985808,
	author = {Sridhara, Giriprasad and Pollock, Lori and Vijay-Shanker, K.},
	title = {Automatically detecting and describing high level actions within methods},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {101--110},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985808},
	doi = {10.1145/1985793.1985808},
	acmid = {1985808},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation, program comprehension}
} 

@inproceedings{Moreno:2013:ICPC,
	author = {Moreno, Laura and Aponte, Jairo and Sridhara Giriprasad and Marcus, Andrian and Pollock, Lori and Vijay-Shanker, K.},
	title = {Automatic Generation of Natural Language Summaries for Java Classes},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	year = {2013},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@article{rau1989information,
	title={Information extraction and text summarization using linguistic knowledge acquisition},
	author={Rau, Lisa F and Jacobs, Paul S and Zernik, Uri},
	journal={Information Processing \& Management},
	volume={25},
	number={4},
	pages={419--428},
	year={1989},
	publisher={Elsevier}
}

@article{radev2002introduction,
	title={Introduction to the special issue on summarization},
	author={Radev, Dragomir R and Hovy, Eduard and McKeown, Kathleen},
	journal={Computational linguistics},
	volume={28},
	number={4},
	pages={399--408},
	year={2002},
	publisher={MIT Press}
}

@inproceedings{goldstein1999summarizing,
	title={Summarizing text documents: sentence selection and evaluation metrics},
	author={Goldstein, Jade and Kantrowitz, Mark and Mittal, Vibhu and Carbonell, Jaime},
	booktitle={Proceedings of the 22nd annual international ACM SIGIR conference on Research and development in information retrieval},
	pages={121--128},
	year={1999},
	organization={ACM}
}

@inproceedings{haiduc2010use,
	title={On the use of automated text summarization techniques for summarizing source code},
	author={Haiduc, Sonia and Aponte, Jairo and Moreno, Laura and Marcus, Andrian},
	booktitle={2010 17th Working Conference on Reverse Engineering},
	pages={35--44},
	year={2010},
	organization={IEEE}
}

@article{mcburney2016automatic,
	title={Automatic Source Code Summarization of Context for Java Methods},
	author={McBurney, Paul W and McMillan, Collin},
	journal={IEEE Transactions on Software Engineering},
	volume={42},
	number={2},
	pages={103--119},
	year={2016},
	publisher={IEEE}
}

@article{rastkar2014automatic,
	title={Automatic summarization of bug reports},
	author={Rastkar, Sarah and Murphy, Gail C and Murray, Gabriel},
	journal={IEEE Transactions on Software Engineering},
	volume={40},
	number={4},
	pages={366--380},
	year={2014},
	publisher={IEEE}
}

@book{cohn2004user,
	title={User stories applied: For agile software development},
	author={Cohn, Mike},
	year={2004},
	publisher={Addison-Wesley Professional}
}

@article{beck2001manifesto,
	title={Manifesto for agile software development},
	author={Beck, Kent and Beedle, Mike and Van Bennekum, Arie and Cockburn, Alistair and Cunningham, Ward and Fowler, Martin and Grenning, James and Highsmith, Jim and Hunt, Andrew and Jeffries, Ron and others},
	year={2001}
}

@book{robertson2012mastering,
	title={Mastering the requirements process: Getting requirements right},
	author={Robertson, Suzanne and Robertson, James},
	year={2012},
	publisher={Addison-wesley}
}

@inproceedings{murray2008summarizing,
	title={Summarizing spoken and written conversations},
	author={Murray, Gabriel and Carenini, Giuseppe},
	booktitle={Proceedings of the Conference on Empirical Methods in Natural Language Processing},
	pages={773--782},
	year={2008},
	organization={Association for Computational Linguistics}
}

@inproceedings{klimt2004enron,
	title={The enron corpus: A new dataset for email classification research},
	author={Klimt, Bryan and Yang, Yiming},
	booktitle={European Conference on Machine Learning},
	pages={217--226},
	year={2004},
	organization={Springer}
}

@inproceedings{mccowan2005ami,
	title={The AMI meeting corpus},
	author={McCowan, Iain and Carletta, Jean and Kraaij, W and Ashby, S and Bourban, S and Flynn, M and Guillemot, M and Hain, T and Kadlec, J and Karaiskos, V and others},
	booktitle={Proceedings of the 5th International Conference on Methods and Techniques in Behavioral Research},
	volume={88},
	year={2005}
}

@inproceedings{rastkar2010summarizing,
	title={Summarizing software artifacts: a case study of bug reports},
	author={Rastkar, Sarah and Murphy, Gail C and Murray, Gabriel},
	booktitle={Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering-Volume 1},
	pages={505--514},
	year={2010},
	organization={ACM}
}

@inproceedings{bird2006mining,
	title={Mining email social networks},
	author={Bird, Christian and Gourley, Alex and Devanbu, Prem and Gertz, Michael and Swaminathan, Anand},
	booktitle={Proceedings of the 2006 international workshop on Mining software repositories},
	pages={137--143},
	year={2006},
	organization={ACM}
}

@inproceedings{Bird:2008:LSS:1453101.1453107,
	author = {Bird, Christian and Pattison, David and D'Souza, Raissa and Filkov, Vladimir and Devanbu, Premkumar},
	title = {Latent Social Structure in Open Source Projects},
	booktitle = {Proceedings of the 16th ACM SIGSOFT International Symposium on Foundations of Software Engineering},
	series = {SIGSOFT '08/FSE-16},
	year = {2008},
	isbn = {978-1-59593-995-1},
	location = {Atlanta, Georgia},
	pages = {24--35},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1453101.1453107},
	doi = {10.1145/1453101.1453107},
	acmid = {1453107},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {collaboration, open source software, social networks}
} 

@article{10.1109/TSE.2005.72,
	author = {Thomas Zimmermann and Peter Weissgerber and Stephan Diehl and Andreas Zeller},
	title = {Mining Version Histories to Guide Software Changes},
	journal ={IEEE Transactions on Software Engineering},
	volume = {31},
	number = {6},
	issn = {0098-5589},
	year = {2005},
	pages = {429-445},
	doi = {http://doi.ieeecomputersociety.org/10.1109/TSE.2005.72},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
}

@article{Anvik:2011:REB:2000791.2000794,
	author = {Anvik, John and Murphy, Gail C.},
	title = {Reducing the Effort of Bug Report Triage: Recommenders for Development-oriented Decisions},
	journal = {ACM Trans. Softw. Eng. Methodol.},
	issue_date = {August 2011},
	volume = {20},
	number = {3},
	month = aug,
	year = {2011},
	issn = {1049-331X},
	pages = {10:1--10:35},
	articleno = {10},
	numpages = {35},
	url = {http://doi.acm.org/10.1145/2000791.2000794},
	doi = {10.1145/2000791.2000794},
	acmid = {2000794},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Bug report triage, configuration assistance, machine learning, recommendation, task assignment}
} 

@online{MSR16,
	author = {MSR 2016},
	title = {International Conference on Mining Software Repositories},
	year = 2016,
	url = {http://2016.msrconf.org/},
	urldate = {2016-06-01}
}

@inproceedings{menzies2012goldfish,
	title={Goldfish bowl panel: Software development analytics},
	author={Menzies, Tim and Zimmermann, Thomas},
	booktitle={Software Engineering (ICSE), 2012 34th International Conference on},
	pages={1032--1033},
	year={2012},
	organization={IEEE}
}

@article{sharp2016role,
	title={The role of ethnographic studies in empirical software engineering},
	author={Sharp, Helen and Dittrich, Yvonne and de Souza, Cleidson},
	journal={IEEE Transactions on Software Engineering},
	pages={in--press},
	year={2016}
}

@article{storey2009software,
	title={How software developers use tagging to support reminding and refinding},
	author={Storey, Margaret-Anne and Ryall, Jody and Singer, Janice and Myers, Dorothy and Cheng, Li-Te and Muller, Michael},
	journal={Software Engineering, IEEE Transactions on},
	volume={35},
	number={4},
	pages={470--483},
	year={2009},
	publisher={IEEE}
}

@article{madey2002open,
	title={The open source software development phenomenon: An analysis based on social network theory},
	author={Madey, Gregory and Freeh, Vincent and Tynan, Renee},
	journal={AMCIS 2002 Proceedings},
	pages={247},
	year={2002}
}

@article{barua2014developers,
	title={What are developers talking about? an analysis of topics and trends in stack overflow},
	author={Barua, Anton and Thomas, Stephen W and Hassan, Ahmed E},
	journal={Empirical Software Engineering},
	volume={19},
	number={3},
	pages={619--654},
	year={2014},
	publisher={Springer}
}

@article{lanubile2010collaboration,
	title={Collaboration tools for global software engineering},
	author={Lanubile, Filippo and Ebert, Christof and Prikladnicki, Rafael and Vizca{\'\i}no, Aurora},
	journal={IEEE software},
	volume={27},
	number={2},
	pages={52},
	year={2010},
	publisher={IEEE Computer Society}
}

@article{mangano2015software,
	title={How Software Designers Interact with Sketches at the Whiteboard},
	author={Mangano, Nicolas and LaToza, Thomas D and Petre, Marian and Van Der Hoek, Andre},
	journal={Software Engineering, IEEE Transactions on},
	volume={41},
	number={2},
	pages={135--156},
	year={2015},
	publisher={IEEE}
}

@inproceedings{roehm2012professional,
	title={How do professional developers comprehend software?},
	author={Roehm, Tobias and Tiarks, Rebecca and Koschke, Rainer and Maalej, Walid},
	booktitle={Proceedings of the 34th International Conference on Software Engineering},
	pages={255--265},
	year={2012},
	organization={IEEE Press}
}

@article{andres2002comparison,
	title={A comparison of face-to-face and virtual software development teams},
	author={Andres, Hayward P},
	journal={Team Performance Management: An International Journal},
	volume={8},
	number={1/2},
	pages={39--48},
	year={2002},
	publisher={MCB UP Ltd}
}

@article{crowston2007role,
	title={The role of face-to-face meetings in technology-supported self-organizing distributed teams},
	author={Crowston, Kevin and Howison, James and Masango, Chengetai and Eseryel, U Yeliz},
	journal={Professional Communication, IEEE Transactions on},
	volume={50},
	number={3},
	pages={185--203},
	year={2007},
	publisher={IEEE}
}

@article{kraut1995coordination,
	title={Coordination in software development},
	author={Kraut, Robert E and Streeter, Lynn A},
	journal={Communications of the ACM},
	volume={38},
	number={3},
	pages={69--82},
	year={1995},
	publisher={Association for Computing Machinery, Inc.}
}

@inproceedings{rigby2007can,
	title={What can oss mailing lists tell us? a preliminary psychometric text analysis of the apache developer mailing list},
	author={Rigby, Peter C and Hassan, Ahmed E},
	booktitle={Proceedings of the Fourth International Workshop on Mining Software Repositories},
	pages={23},
	year={2007},
	organization={IEEE Computer Society}
}

@ARTICLE{7447797,
	author={T. Lee and J. Nam and D. Han and S. Kim and H. In},
	journal={IEEE Transactions on Software Engineering},
	title={Developer Micro Interaction Metrics for Software Defect Prediction},
	year={2016},
	volume={PP},
	number={99},
	pages={1-1},
	keywords={Complexity theory;Quality assurance;Software metrics;Software quality;Defect prediction;Mylyn;developer interaction;software metrics;software quality},
	doi={10.1109/TSE.2016.2550458},
	ISSN={0098-5589},
	month={},}

@book{Rijsbergen:fscore,
	author = {Rijsbergen, C. J. Van},
	title = {Information Retrieval},
	year = {1979},
	isbn = {0408709294},
	edition = {2nd},
	publisher = {Butterworth-Heinemann},
	address = {Newton, MA, USA}
} 

@inproceedings{caruana2006empirical,
	author = {Caruana, Rich and Niculescu-Mizil, Alexandru},
	title = {An Empirical Comparison of Supervised Learning Algorithms},
	booktitle = {Proceedings of the 23rd International Conference on Machine Learning},
	series = {ICML '06},
	year = {2006},
	isbn = {1-59593-383-2},
	location = {Pittsburgh, Pennsylvania, USA},
	pages = {161--168},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1143844.1143865},
	doi = {10.1145/1143844.1143865},
	acmid = {1143865},
	publisher = {ACM},
	address = {New York, NY, USA}
} 

@inproceedings{carenini2008summarizing,
	title={Summarizing Emails with Conversational Cohesion and Subjectivity.},
	author={Carenini, Giuseppe and Ng, Raymond T and Zhou, Xiaodong},
	year={2008}
}

@inproceedings{Buse:2008:MSR:1390630.1390647,
	author = {Buse, Raymond P.L. and Weimer, Westley R.},
	title = {A Metric for Software Readability},
	booktitle = {Proceedings of the 2008 International Symposium on Software Testing and Analysis},
	series = {ISSTA '08},
	year = {2008},
	isbn = {978-1-60558-050-0},
	location = {Seattle, WA, USA},
	pages = {121--130},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1390630.1390647},
	doi = {10.1145/1390630.1390647},
	acmid = {1390647},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {FindBugs, code metrics, machine learning, program understanding, software maintenance, software readability}
} 

@article{moreno2012analysis,
	title={On the analysis of human and automatic summaries of source code},
	author={Moreno, Laura and Aponte, Jairo},
	journal={CLEI Electronic Journal},
	volume={15},
	number={2},
	pages={2--2},
	year={2012},
	publisher={Centro Latinoamericano de Estudios en Inform{\'a}tica}
}

@inproceedings{Moreno:2014:SCS:2591062.2591096,
	author = {Moreno, Laura},
	title = {Summarization of Complex Software Artifacts},
	booktitle = {Companion Proceedings of the 36th International Conference on Software Engineering},
	series = {ICSE Companion 2014},
	year = {2014},
	isbn = {978-1-4503-2768-8},
	location = {Hyderabad, India},
	pages = {654--657},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/2591062.2591096},
	doi = {10.1145/2591062.2591096},
	acmid = {2591096},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Software Documentation, Source code, Summarization}
} 
@article{chawla2002smote,
	title={SMOTE: synthetic minority over-sampling technique},
	author={Chawla, Nitesh V. and Bowyer, Kevin W. and Hall, Lawrence O. and Kegelmeyer, W. Philip},
	journal={Journal of artificial intelligence research},
	volume={16},
	pages={321--357},
	year={2002}
}

@article{batista2004study,
	title={A study of the behavior of several methods for balancing machine learning training data},
	author={Batista, Gustavo EAPA and Prati, Ronaldo C and Monard, Maria Carolina},
	journal={ACM Sigkdd Explorations Newsletter},
	volume={6},
	number={1},
	pages={20--29},
	year={2004},
	publisher={ACM}
}

@article{chawla2004editorial,
	title={Editorial: special issue on learning from imbalanced data sets},
	author={Chawla, Nitesh V and Japkowicz, Nathalie and Kotcz, Aleksander},
	journal={ACM Sigkdd Explorations Newsletter},
	volume={6},
	number={1},
	pages={1--6},
	year={2004},
	publisher={ACM}
}

@article{hearst1998support,
	title={Support vector machines},
	author={Hearst, Marti A. and Dumais, Susan T and Osman, Edgar and Platt, John and Scholkopf, Bernhard},
	journal={IEEE Intelligent Systems and their Applications},
	volume={13},
	number={4},
	pages={18--28},
	year={1998},
	publisher={IEEE}
}

@article{chang2011libsvm,
	title={LIBSVM: a library for support vector machines},
	author={Chang, Chih-Chung and Lin, Chih-Jen},
	journal={ACM Transactions on Intelligent Systems and Technology (TIST)},
	volume={2},
	number={3},
	pages={27},
	year={2011},
	publisher={ACM}
}

@book{hosmer2004applied,
	title={Applied logistic regression},
	author={Hosmer Jr, David W and Lemeshow, Stanley},
	year={2004},
	publisher={John Wiley \& Sons}
}

@article{pedregosa2011scikit,
	title={Scikit-learn: Machine learning in Python},
	author={Pedregosa, Fabian and Varoquaux, Ga{\"e}l and Gramfort, Alexandre and Michel, Vincent and Thirion, Bertrand and Grisel, Olivier and Blondel, Mathieu and Prettenhofer, Peter and Weiss, Ron and Dubourg, Vincent and others},
	journal={Journal of Machine Learning Research},
	volume={12},
	number={Oct},
	pages={2825--2830},
	year={2011}
}

@article{hsu2003practical,
	title={A practical guide to support vector classification},
	author={Hsu, Chih-Wei and Chang, Chih-Chung and Lin, Chih-Jen and others},
	year={2003}
}

@book{ten2007doing,
	title={Doing conversation analysis},
	author={Ten Have, Paul},
	year={2007},
	publisher={Sage}
}

@book{ford2002language,
	title={The language of turn and sequence},
	author={Ford, Cecilia E and Fox, Barbara A and Thompson, Sandra A},
	year={2002},
	publisher={Oxford University Press on Demand}
}

@book{hutchby2008conversation,
	title={Conversation analysis},
	author={Hutchby, Ian and Wooffitt, Robin},
	year={2008},
	publisher={Polity}
}

@book{nishida2007convanalysis,
	title={Conversational Informatics: An Engineering Approach},
	author={Toyoaki Nishida},
	year={2007},
	publisher={Wiley}
}

@book{emanuel2007sequence,
	title={Sequence Organization in Interaction: A Primer in Conversation Analysis I},
	author={Emanuel A.. Schegloff},
	year={2007},
	publisher={Cambridge University Press}
}

@inproceedings{Barzilay:1999:IFC:1034678.1034760,
	author = {Barzilay, Regina and McKeown, Kathleen R. and Elhadad, Michael},
	title = {Information Fusion in the Context of Multi-document Summarization},
	booktitle = {Proceedings of the 37th Annual Meeting of the Association for Computational Linguistics on Computational Linguistics},
	series = {ACL '99},
	year = {1999},
	isbn = {1-55860-609-3},
	location = {College Park, Maryland},
	pages = {550--557},
	numpages = {8},
	url = {http://dx.doi.org/10.3115/1034678.1034760},
	doi = {10.3115/1034678.1034760},
	acmid = {1034760},
	publisher = {Association for Computational Linguistics},
	address = {Stroudsburg, PA, USA},
}

@article{gupta2010survey,
	title={A survey of text summarization extractive techniques},
	author={Gupta, Vishal and Lehal, Gurpreet Singh},
	journal={Journal of emerging technologies in web intelligence},
	volume={2},
	number={3},
	pages={258--268},
	year={2010}
}

@inproceedings{Buse:2008:ADI:1390630.1390664,
	author = {Buse, Raymond P.L. and Weimer, Westley R.},
	title = {Automatic documentation inference for exceptions},
	booktitle = {Proceedings of the 2008 international symposium on Software testing and analysis},
	series = {ISSTA '08},
	year = {2008},
	isbn = {978-1-60558-050-0},
	location = {Seattle, WA, USA},
	pages = {273--282},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1390630.1390664},
	doi = {10.1145/1390630.1390664},
	acmid = {1390664},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation inference, exception handling, software documentation},
}

@inproceedings{Sridhara:2010:TAG:1858996.1859006,
	author = {Sridhara, Giriprasad and Hill, Emily and Muppaneni, Divya and Pollock, Lori and Vijay-Shanker, K.},
	title = {Towards automatically generating summary comments for Java methods},
	booktitle = {Proceedings of the IEEE/ACM international conference on Automated software engineering},
	series = {ASE '10},
	year = {2010},
	isbn = {978-1-4503-0116-9},
	location = {Antwerp, Belgium},
	pages = {43--52},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1858996.1859006},
	doi = {10.1145/1858996.1859006},
	acmid = {1859006},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {comment generation, method summarization, natural language program analysis},
}

@inproceedings{Sridhara:2011:GPC:2057176.2057211,
	author = {Sridhara, Giriprasad and Pollock, Lori and Vijay-Shanker, K.},
	title = {Generating Parameter Comments and Integrating with Method Summaries},
	booktitle = {Proceedings of the 2011 IEEE 19th International Conference on Program Comprehension},
	series = {ICPC '11},
	year = {2011},
	isbn = {978-0-7695-4398-7},
	pages = {71--80},
	numpages = {10},
	url = {http://dx.doi.org/10.1109/ICPC.2011.28},
	doi = {10.1109/ICPC.2011.28},
	acmid = {2057211},
	keywords = {documentation, software maintenance}
} 

@inproceedings{Sridhara:2011:ADD:1985793.1985808,
	author = {Sridhara, Giriprasad and Pollock, Lori and Vijay-Shanker, K.},
	title = {Automatically detecting and describing high level actions within methods},
	booktitle = {Proceedings of the 33rd International Conference on Software Engineering},
	series = {ICSE '11},
	year = {2011},
	isbn = {978-1-4503-0445-0},
	location = {Waikiki, Honolulu, HI, USA},
	pages = {101--110},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1985793.1985808},
	doi = {10.1145/1985793.1985808},
	acmid = {1985808},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {documentation, program comprehension}
} 

@inproceedings{Moreno:2013:ICPC,
	author = {Moreno, Laura and Aponte, Jairo and Sridhara Giriprasad and Marcus, Andrian and Pollock, Lori and Vijay-Shanker, K.},
	title = {Automatic Generation of Natural Language Summaries for Java Classes},
	booktitle = {Proceedings of the 21st International Conference on Program Comprehension},
	series = {ICPC '13},
	year = {2013},
	location = {San Francisco, CA, USA},
	numpages = {10}
}

@article{rau1989information,
	title={Information extraction and text summarization using linguistic knowledge acquisition},
	author={Rau, Lisa F and Jacobs, Paul S and Zernik, Uri},
	journal={Information Processing \& Management},
	volume={25},
	number={4},
	pages={419--428},
	year={1989},
	publisher={Elsevier}
}

@article{radev2002introduction,
	title={Introduction to the special issue on summarization},
	author={Radev, Dragomir R and Hovy, Eduard and McKeown, Kathleen},
	journal={Computational linguistics},
	volume={28},
	number={4},
	pages={399--408},
	year={2002},
	publisher={MIT Press}
}

@inproceedings{goldstein1999summarizing,
	title={Summarizing text documents: sentence selection and evaluation metrics},
	author={Goldstein, Jade and Kantrowitz, Mark and Mittal, Vibhu and Carbonell, Jaime},
	booktitle={Proceedings of the 22nd annual international ACM SIGIR conference on Research and development in information retrieval},
	pages={121--128},
	year={1999},
	organization={ACM}
}

@inproceedings{haiduc2010use,
	title={On the use of automated text summarization techniques for summarizing source code},
	author={Haiduc, Sonia and Aponte, Jairo and Moreno, Laura and Marcus, Andrian},
	booktitle={2010 17th Working Conference on Reverse Engineering},
	pages={35--44},
	year={2010},
	organization={IEEE}
}

@article{mcburney2016automatic,
	title={Automatic Source Code Summarization of Context for Java Methods},
	author={McBurney, Paul W and McMillan, Collin},
	journal={IEEE Transactions on Software Engineering},
	volume={42},
	number={2},
	pages={103--119},
	year={2016},
	publisher={IEEE}
}

@article{rastkar2014automatic,
	title={Automatic summarization of bug reports},
	author={Rastkar, Sarah and Murphy, Gail C and Murray, Gabriel},
	journal={IEEE Transactions on Software Engineering},
	volume={40},
	number={4},
	pages={366--380},
	year={2014},
	publisher={IEEE}
}

@book{cohn2004user,
	title={User stories applied: For agile software development},
	author={Cohn, Mike},
	year={2004},
	publisher={Addison-Wesley Professional}
}

@article{beck2001manifesto,
	title={Manifesto for agile software development},
	author={Beck, Kent and Beedle, Mike and Van Bennekum, Arie and Cockburn, Alistair and Cunningham, Ward and Fowler, Martin and Grenning, James and Highsmith, Jim and Hunt, Andrew and Jeffries, Ron and others},
	year={2001}
}

@book{robertson2012mastering,
	title={Mastering the requirements process: Getting requirements right},
	author={Robertson, Suzanne and Robertson, James},
	year={2012},
	publisher={Addison-wesley}
}

@inproceedings{murray2008summarizing,
	title={Summarizing spoken and written conversations},
	author={Murray, Gabriel and Carenini, Giuseppe},
	booktitle={Proceedings of the Conference on Empirical Methods in Natural Language Processing},
	pages={773--782},
	year={2008},
	organization={Association for Computational Linguistics}
}

@inproceedings{klimt2004enron,
	title={The enron corpus: A new dataset for email classification research},
	author={Klimt, Bryan and Yang, Yiming},
	booktitle={European Conference on Machine Learning},
	pages={217--226},
	year={2004},
	organization={Springer}
}

@inproceedings{mccowan2005ami,
	title={The AMI meeting corpus},
	author={McCowan, Iain and Carletta, Jean and Kraaij, W and Ashby, S and Bourban, S and Flynn, M and Guillemot, M and Hain, T and Kadlec, J and Karaiskos, V and others},
	booktitle={Proceedings of the 5th International Conference on Methods and Techniques in Behavioral Research},
	volume={88},
	year={2005}
}

@inproceedings{rastkar2010summarizing,
	title={Summarizing software artifacts: a case study of bug reports},
	author={Rastkar, Sarah and Murphy, Gail C and Murray, Gabriel},
	booktitle={Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering-Volume 1},
	pages={505--514},
	year={2010},
	organization={ACM}
}

@inproceedings{bird2006mining,
	title={Mining email social networks},
	author={Bird, Christian and Gourley, Alex and Devanbu, Prem and Gertz, Michael and Swaminathan, Anand},
	booktitle={Proceedings of the 2006 international workshop on Mining software repositories},
	pages={137--143},
	year={2006},
	organization={ACM}
}

@inproceedings{Bird:2008:LSS:1453101.1453107,
	author = {Bird, Christian and Pattison, David and D'Souza, Raissa and Filkov, Vladimir and Devanbu, Premkumar},
	title = {Latent Social Structure in Open Source Projects},
	booktitle = {Proceedings of the 16th ACM SIGSOFT International Symposium on Foundations of Software Engineering},
	series = {SIGSOFT '08/FSE-16},
	year = {2008},
	isbn = {978-1-59593-995-1},
	location = {Atlanta, Georgia},
	pages = {24--35},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1453101.1453107},
	doi = {10.1145/1453101.1453107},
	acmid = {1453107},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {collaboration, open source software, social networks}
} 

@article{10.1109/TSE.2005.72,
	author = {Thomas Zimmermann and Peter Weissgerber and Stephan Diehl and Andreas Zeller},
	title = {Mining Version Histories to Guide Software Changes},
	journal ={IEEE Transactions on Software Engineering},
	volume = {31},
	number = {6},
	issn = {0098-5589},
	year = {2005},
	pages = {429-445},
	doi = {http://doi.ieeecomputersociety.org/10.1109/TSE.2005.72},
	publisher = {IEEE Computer Society},
	address = {Los Alamitos, CA, USA},
}

@article{Anvik:2011:REB:2000791.2000794,
	author = {Anvik, John and Murphy, Gail C.},
	title = {Reducing the Effort of Bug Report Triage: Recommenders for Development-oriented Decisions},
	journal = {ACM Trans. Softw. Eng. Methodol.},
	issue_date = {August 2011},
	volume = {20},
	number = {3},
	month = aug,
	year = {2011},
	issn = {1049-331X},
	pages = {10:1--10:35},
	articleno = {10},
	numpages = {35},
	url = {http://doi.acm.org/10.1145/2000791.2000794},
	doi = {10.1145/2000791.2000794},
	acmid = {2000794},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Bug report triage, configuration assistance, machine learning, recommendation, task assignment}
} 

@online{MSR16,
	author = {MSR 2016},
	title = {International Conference on Mining Software Repositories},
	year = 2016,
	url = {http://2016.msrconf.org/},
	urldate = {2016-06-01}
}

@inproceedings{menzies2012goldfish,
	title={Goldfish bowl panel: Software development analytics},
	author={Menzies, Tim and Zimmermann, Thomas},
	booktitle={Software Engineering (ICSE), 2012 34th International Conference on},
	pages={1032--1033},
	year={2012},
	organization={IEEE}
}

@article{sharp2016role,
	title={The role of ethnographic studies in empirical software engineering},
	author={Sharp, Helen and Dittrich, Yvonne and de Souza, Cleidson},
	journal={IEEE Transactions on Software Engineering},
	pages={in--press},
	year={2016}
}

@article{storey2009software,
	title={How software developers use tagging to support reminding and refinding},
	author={Storey, Margaret-Anne and Ryall, Jody and Singer, Janice and Myers, Dorothy and Cheng, Li-Te and Muller, Michael},
	journal={Software Engineering, IEEE Transactions on},
	volume={35},
	number={4},
	pages={470--483},
	year={2009},
	publisher={IEEE}
}

@article{madey2002open,
	title={The open source software development phenomenon: An analysis based on social network theory},
	author={Madey, Gregory and Freeh, Vincent and Tynan, Renee},
	journal={AMCIS 2002 Proceedings},
	pages={247},
	year={2002}
}

@article{barua2014developers,
	title={What are developers talking about? an analysis of topics and trends in stack overflow},
	author={Barua, Anton and Thomas, Stephen W and Hassan, Ahmed E},
	journal={Empirical Software Engineering},
	volume={19},
	number={3},
	pages={619--654},
	year={2014},
	publisher={Springer}
}

@article{lanubile2010collaboration,
	title={Collaboration tools for global software engineering},
	author={Lanubile, Filippo and Ebert, Christof and Prikladnicki, Rafael and Vizca{\'\i}no, Aurora},
	journal={IEEE software},
	volume={27},
	number={2},
	pages={52},
	year={2010},
	publisher={IEEE Computer Society}
}

@article{mangano2015software,
	title={How Software Designers Interact with Sketches at the Whiteboard},
	author={Mangano, Nicolas and LaToza, Thomas D and Petre, Marian and Van Der Hoek, Andre},
	journal={Software Engineering, IEEE Transactions on},
	volume={41},
	number={2},
	pages={135--156},
	year={2015},
	publisher={IEEE}
}

@inproceedings{roehm2012professional,
	title={How do professional developers comprehend software?},
	author={Roehm, Tobias and Tiarks, Rebecca and Koschke, Rainer and Maalej, Walid},
	booktitle={Proceedings of the 34th International Conference on Software Engineering},
	pages={255--265},
	year={2012},
	organization={IEEE Press}
}

@article{andres2002comparison,
	title={A comparison of face-to-face and virtual software development teams},
	author={Andres, Hayward P},
	journal={Team Performance Management: An International Journal},
	volume={8},
	number={1/2},
	pages={39--48},
	year={2002},
	publisher={MCB UP Ltd}
}

@article{crowston2007role,
	title={The role of face-to-face meetings in technology-supported self-organizing distributed teams},
	author={Crowston, Kevin and Howison, James and Masango, Chengetai and Eseryel, U Yeliz},
	journal={Professional Communication, IEEE Transactions on},
	volume={50},
	number={3},
	pages={185--203},
	year={2007},
	publisher={IEEE}
}

@article{kraut1995coordination,
	title={Coordination in software development},
	author={Kraut, Robert E and Streeter, Lynn A},
	journal={Communications of the ACM},
	volume={38},
	number={3},
	pages={69--82},
	year={1995},
	publisher={Association for Computing Machinery, Inc.}
}

@inproceedings{rigby2007can,
	title={What can oss mailing lists tell us? a preliminary psychometric text analysis of the apache developer mailing list},
	author={Rigby, Peter C and Hassan, Ahmed E},
	booktitle={Proceedings of the Fourth International Workshop on Mining Software Repositories},
	pages={23},
	year={2007},
	organization={IEEE Computer Society}
}

@ARTICLE{7447797,
	author={T. Lee and J. Nam and D. Han and S. Kim and H. In},
	journal={IEEE Transactions on Software Engineering},
	title={Developer Micro Interaction Metrics for Software Defect Prediction},
	year={2016},
	volume={PP},
	number={99},
	pages={1-1},
	keywords={Complexity theory;Quality assurance;Software metrics;Software quality;Defect prediction;Mylyn;developer interaction;software metrics;software quality},
	doi={10.1109/TSE.2016.2550458},
	ISSN={0098-5589},
	month={},}

@book{Rijsbergen:fscore,
	author = {Rijsbergen, C. J. Van},
	title = {Information Retrieval},
	year = {1979},
	isbn = {0408709294},
	edition = {2nd},
	publisher = {Butterworth-Heinemann},
	address = {Newton, MA, USA}
} 

@inproceedings{caruana2006empirical,
	author = {Caruana, Rich and Niculescu-Mizil, Alexandru},
	title = {An Empirical Comparison of Supervised Learning Algorithms},
	booktitle = {Proceedings of the 23rd International Conference on Machine Learning},
	series = {ICML '06},
	year = {2006},
	isbn = {1-59593-383-2},
	location = {Pittsburgh, Pennsylvania, USA},
	pages = {161--168},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1143844.1143865},
	doi = {10.1145/1143844.1143865},
	acmid = {1143865},
	publisher = {ACM},
	address = {New York, NY, USA}
} 

@inproceedings{carenini2008summarizing,
	title={Summarizing Emails with Conversational Cohesion and Subjectivity.},
	author={Carenini, Giuseppe and Ng, Raymond T and Zhou, Xiaodong},
	year={2008}
}

@inproceedings{Buse:2008:MSR:1390630.1390647,
	author = {Buse, Raymond P.L. and Weimer, Westley R.},
	title = {A Metric for Software Readability},
	booktitle = {Proceedings of the 2008 International Symposium on Software Testing and Analysis},
	series = {ISSTA '08},
	year = {2008},
	isbn = {978-1-60558-050-0},
	location = {Seattle, WA, USA},
	pages = {121--130},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1390630.1390647},
	doi = {10.1145/1390630.1390647},
	acmid = {1390647},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {FindBugs, code metrics, machine learning, program understanding, software maintenance, software readability}
} 

@article{moreno2012analysis,
	title={On the analysis of human and automatic summaries of source code},
	author={Moreno, Laura and Aponte, Jairo},
	journal={CLEI Electronic Journal},
	volume={15},
	number={2},
	pages={2--2},
	year={2012},
	publisher={Centro Latinoamericano de Estudios en Inform{\'a}tica}
}

@inproceedings{Moreno:2014:SCS:2591062.2591096,
	author = {Moreno, Laura},
	title = {Summarization of Complex Software Artifacts},
	booktitle = {Companion Proceedings of the 36th International Conference on Software Engineering},
	series = {ICSE Companion 2014},
	year = {2014},
	isbn = {978-1-4503-2768-8},
	location = {Hyderabad, India},
	pages = {654--657},
	numpages = {4},
	url = {http://doi.acm.org/10.1145/2591062.2591096},
	doi = {10.1145/2591062.2591096},
	acmid = {2591096},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Software Documentation, Source code, Summarization}
} 

@inproceedings{lee2009snackbot,
	title={The snackbot: documenting the design of a robot for long-term human-robot interaction},
	author={Lee, Min Kyung and Forlizzi, Jodi and Rybski, Paul E and Crabbe, Frederick and Chung, Wayne and Finkle, Josh and Glaser, Eric and Kiesler, Sara},
	booktitle={Proceedings of the 4th ACM/IEEE international conference on Human robot interaction},
	pages={7--14},
	year={2009},
	organization={ACM}
}

@article{carletta1996assessing,
	title={Assessing agreement on classification tasks: the kappa statistic},
	author={Carletta, Jean},
	journal={Computational linguistics},
	volume={22},
	number={2},
	pages={249--254},
	year={1996},
	publisher={MIT Press}
}

@article{krippendorff2004reliability,
	title={Reliability in content analysis},
	author={Krippendorff, Klaus},
	journal={Human communication research},
	volume={30},
	number={3},
	pages={411--433},
	year={2004},
	publisher={Wiley Online Library}
}

@article{craggs2005evaluating,
	title={Evaluating discourse and dialogue coding schemes},
	author={Craggs, Richard and Wood, Mary McGee},
	journal={Computational Linguistics},
	volume={31},
	number={3},
	pages={289--296},
	year={2005},
	publisher={MIT Press}
}

@article{hsieh2005three,
	title={Three approaches to qualitative content analysis},
	author={Hsieh, Hsiu-Fang and Shannon, Sarah E},
	journal={Qualitative health research},
	volume={15},
	number={9},
	pages={1277--1288},
	year={2005},
	publisher={Sage publications Sage CA: Thousand Oaks, CA}
}

@article{kelley1984iterative,
	title={An iterative design methodology for user-friendly natural language office information applications},
	author={Kelley, John F},
	journal={ACM Transactions on Information Systems (TOIS)},
	volume={2},
	number={1},
	pages={26--41},
	year={1984},
	publisher={ACM}
}

@inproceedings{Weiser:1981:PS:800078.802557,
	author = {Weiser, Mark},
	title = {Program Slicing},
	booktitle = {Proceedings of the 5th International Conference on Software Engineering},
	series = {ICSE '81},
	year = {1981},
	isbn = {0-89791-146-6},
	location = {San Diego, California, USA},
	pages = {439--449},
	numpages = {11},
	url = {http://dl.acm.org/citation.cfm?id=800078.802557},
	acmid = {802557},
	publisher = {IEEE Press},
	address = {Piscataway, NJ, USA},
	keywords = {Data flow analysis, Debugging, Human factors, Program maintenance, Program metrics, Software tools},
} 

@inproceedings{Klemmer:2000:SWO:354401.354406,
	author = {Klemmer, Scott R. and Sinha, Anoop K. and Chen, Jack and Landay, James A. and Aboobaker, Nadeem and Wang, Annie},
	title = {Suede: A Wizard of Oz Prototyping Tool for Speech User Interfaces},
	booktitle = {Proceedings of the 13th Annual ACM Symposium on User Interface Software and Technology},
	series = {UIST '00},
	year = {2000},
	isbn = {1-58113-212-3},
	location = {San Diego, California, USA},
	pages = {1--10},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/354401.354406},
	doi = {10.1145/354401.354406},
	acmid = {354406},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Wizard of Oz, design, design tools, informal user interfaces, low-fidelity, prototyping, speech user interfaces},
} 

@inproceedings{Lu:2011:PWO:1957656.1957729,
	author = {Lu, David V. and Smart, William D.},
	title = {Polonius: A Wizard of Oz Interface for HRI Experiments},
	booktitle = {Proceedings of the 6th International Conference on Human-robot Interaction},
	series = {HRI '11},
	year = {2011},
	isbn = {978-1-4503-0561-7},
	location = {Lausanne, Switzerland},
	pages = {197--198},
	numpages = {2},
	url = {http://doi.acm.org/10.1145/1957656.1957729},
	doi = {10.1145/1957656.1957729},
	acmid = {1957729},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {graphical user interface, human-robot interaction},
} 

@article{fraser1991simulating,
	title={Simulating speech systems},
	author={Fraser, Norman M and Gilbert, G Nigel},
	journal={Computer Speech \& Language},
	volume={5},
	number={1},
	pages={81--99},
	year={1991},
	publisher={Elsevier}
}

@Inbook{Easterbrook2008,
	author="Easterbrook, Steve
	and Singer, Janice
	and Storey, Margaret-Anne
	and Damian, Daniela",
	editor="Shull, Forrest
	and Singer, Janice
	and Sj{\o}berg, Dag I. K.",
	title="Selecting Empirical Methods for Software Engineering Research",
	bookTitle="Guide to Advanced Empirical Software Engineering",
	year="2008",
	publisher="Springer London",
	address="London",
	pages="285--311",
	abstract="Selecting a research method for empirical software engineering research is problematic because the benefits and challenges to using each method are not yet well catalogued. Therefore, this chapter describes a number of empirical methods available. It examines the goals of each and analyzes the types of questions each best addresses. Theoretical stances behind the methods, practical considerations in the application of the methods and data collection are also briefly reviewed. Taken together, this information provides a suitable basis for both understanding and selecting from the variety of methods applicable to empirical software engineering.",
	isbn="978-1-84800-044-5",
	doi="10.1007/978-1-84800-044-5_11",
	url="https://doi.org/10.1007/978-1-84800-044-5_11"
}



@inproceedings{murphy2019developers,
	title={Do developers discover new tools on the toilet?},
	author={Murphy-Hill, Emerson and Smith, Edward K and Sadowski, Caitlin and Jaspan, Ciera and Winter, Collin and Jorde, Matthew and Knight, Andrea and Trenk, Andrew and Gross, Steve},
	booktitle={Proceedings of the 41st International Conference on Software Engineering},
	pages={465--475},
	year={2019},
	organization={IEEE Press}
}

@article{DYBA2008833,
	title = "Empirical studies of agile software development: A systematic review",
	journal = "Information and Software Technology",
	volume = "50",
	number = "9",
	pages = "833 - 859",
	year = "2008",
	issn = "0950-5849",
	doi = "https://doi.org/10.1016/j.infsof.2008.01.006",
	url = "http://www.sciencedirect.com/science/article/pii/S0950584908000256",
	author = "Tore Dybå and Torgeir Dingsøyr",
	keywords = "Empirical software engineering, Evidence-based software engineering, Systematic review, Research synthesis, Agile software development, XP, Extreme programming, Scrum",
	abstract = "Agile software development represents a major departure from traditional, plan-based approaches to software engineering. A systematic review of empirical studies of agile software development up to and including 2005 was conducted. The search strategy identified 1996 studies, of which 36 were identified as empirical studies. The studies were grouped into four themes: introduction and adoption, human and social factors, perceptions on agile methods, and comparative studies. The review investigates what is currently known about the benefits and limitations of, and the strength of evidence for, agile methods. Implications for research and practice are presented. The main implication for research is a need for more and better empirical studies of agile software development within a common research agenda. For the industrial readership, the review provides a map of findings, according to topic, that can be compared for relevance to their own settings and situations."
}

@inproceedings{Perry:2000:ESS:336512.336586,
	author = {Perry, Dewayne E. and Porter, Adam A. and Votta, Lawrence G.},
	title = {Empirical Studies of Software Engineering: A Roadmap},
	booktitle = {Proceedings of the Conference on The Future of Software Engineering},
	series = {ICSE '00},
	year = {2000},
	isbn = {1-58113-253-0},
	location = {Limerick, Ireland},
	pages = {345--355},
	numpages = {11},
	url = {http://doi.acm.org/10.1145/336512.336586},
	doi = {10.1145/336512.336586},
	acmid = {336586},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {empirical studies, software engineering},
} 


@ARTICLE{1702275, 
	author={H. F. {Li} and W. K. {Cheung}}, 
	journal={IEEE Transactions on Software Engineering}, 
	title={An Empirical Study of Software Metrics}, 
	year={1987}, 
	volume={SE-13}, 
	number={6}, 
	pages={697-708}, 
	keywords={Control complexity;cross correlation;empirical study;Halstead's software science;hybrid metrics;software metric;Software metrics;Software measurement;Volume measurement;Size measurement;Software maintenance;Costs;Size control;Databases;Flow graphs;Testing;Control complexity;cross correlation;empirical study;Halstead's software science;hybrid metrics;software metric}, 
	doi={10.1109/TSE.1987.233475}, 
	ISSN={0098-5589}, 
	month={June},}

@ARTICLE{87283, 
	author={M. {van Genuchten}}, 
	journal={IEEE Transactions on Software Engineering}, 
	title={Why is software late? An empirical study of reasons for delay in software development}, 
	year={1991}, 
	volume={17}, 
	number={6}, 
	pages={582-590}, 
	keywords={project engineering;software engineering;software development;development activities;classification;delay enabled actions;Delay;Programming;Software engineering;Project management;Job shop scheduling;Software measurement;Software development management;Engineering management;Management information systems;Automation}, 
	doi={10.1109/32.87283}, 
	ISSN={0098-5589}, 
	month={June},}


@ARTICLE{799955, 
	author={C. B. {Seaman}}, 
	journal={IEEE Transactions on Software Engineering}, 
	title={Qualitative methods in empirical studies of software engineering}, 
	year={1999}, 
	volume={25}, 
	number={4}, 
	pages={557-572}, 
	keywords={user interfaces;human factors;software development management;project management;qualitative methods;empirical studies;software engineering;research community;human aspects;software development;research questions;research methods;nontechnical aspects;qualitative research methods;human behaviour;data collection;quantitative methods;real software engineering studies;Software engineering;Humans;Programming;Data analysis;Design for experiments;Laboratories;Computer industry;Software development management;Design methodology}, 
	doi={10.1109/32.799955}, 
	ISSN={0098-5589}, 
	month={July},}

@ARTICLE{1027796, 
	author={B. A. {Kitchenham} and S. L. {Pfleeger} and L. M. {Pickard} and P. W. {Jones} and D. C. {Hoaglin} and K. {El Emam} and J. {Rosenberg}}, 
	journal={IEEE Transactions on Software Engineering}, 
	title={Preliminary guidelines for empirical research in software engineering}, 
	year={2002}, 
	volume={28}, 
	number={8}, 
	pages={721-734}, 
	keywords={software engineering;software engineering;software researchers;Guidelines;Software engineering;Computer Society;Statistics;Computer science;Data analysis;Software standards;Laboratories;Software performance;Surgery}, 
	doi={10.1109/TSE.2002.1027796}, 
	ISSN={0098-5589}, 
	month={Aug},}

@article{popescu2005dialogue,
	title={Dialogue acts: One or more dimensions},
	author={Popescu-Belis, Andrei},
	journal={ISSCO WorkingPaper},
	volume={62},
	year={2005}
}

@article{TRAINS,
	author = { JAMES F.   ALLEN  and  LENHART K.   SCHUBERT  and  GEORGE   FERGUSON  and  PETER   HEEMAN  and  CHUNG   HEE   HWANG  and  TSUNEAKI   KATO  and  MARC   LIGHT  and  NATHANIEL   MARTIN  and  BRADFORD   MILLER  and  MASSIMO   POESIO  and  DAVID R.   TRAUM },
	title = {The TRAINS project: a case study in building a conversational planning agent},
	journal = {Journal of Experimental \& Theoretical Artificial Intelligence},
	volume = {7},
	number = {1},
	pages = {7-48},
	year  = {1995},
	publisher = {Taylor & Francis},
	doi = {10.1080/09528139508953799},
	
	URL = { 
	https://doi.org/10.1080/09528139508953799
	},
	eprint = { 
	https://doi.org/10.1080/09528139508953799
	}
}

@inproceedings{zarisheva2015dialog,
	title={Dialog act annotation for Twitter conversations},
	author={Zarisheva, Elina and Scheffler, Tatjana},
	booktitle={Proceedings of the 16th Annual Meeting of the Special Interest Group on Discourse and Dialogue},
	pages={114--123},
	year={2015}
}

@inproceedings{ohtake2009annotating,
	title={Annotating dialogue acts to construct dialogue systems for consulting},
	author={Ohtake, Kiyonori and Misu, Teruhisa and Hori, Chiori and Kashioka, Hideki and Nakamura, Satoshi},
	booktitle={Proceedings of the 7th Workshop on Asian Language Resources},
	pages={32--39},
	year={2009},
	organization={Association for Computational Linguistics}
}

@article{DIT,
	author = {Bunt, Harry},
	year = {2009},
	month = {01},
	pages = {},
	title = {The DIT++ taxanomy for functional dialogue markup},
	journal = {Journal of Philosophical Logic}
}

@inproceedings{Agrawal:1994:FAM:645920.672836,
	author = {Agrawal, Rakesh and Srikant, Ramakrishnan},
	title = {Fast Algorithms for Mining Association Rules in Large Databases},
	booktitle = {Proceedings of the 20th International Conference on Very Large Data Bases},
	series = {VLDB '94},
	year = {1994},
	isbn = {1-55860-153-8},
	pages = {487--499},
	numpages = {13},
	url = {http://dl.acm.org/citation.cfm?id=645920.672836},
	acmid = {672836},
	publisher = {Morgan Kaufmann Publishers Inc.},
	address = {San Francisco, CA, USA},
} 

@article{Zaki:2001:SEA:599609.599626,
	author = {Zaki, Mohammed J.},
	title = {SPADE: An Efficient Algorithm for Mining Frequent Sequences},
	journal = {Mach. Learn.},
	issue_date = {January-February 2001},
	volume = {42},
	number = {1-2},
	month = jan,
	year = {2001},
	issn = {0885-6125},
	pages = {31--60},
	numpages = {30},
	url = {http://dl.acm.org/citation.cfm?id=599609.599626},
	acmid = {599626},
	publisher = {Kluwer Academic Publishers},
	address = {Norwell, MA, USA},
	keywords = {data mining, frequent patterns, knowledge discovery, sequence mining, sequential patterns},
} 

@inbook{ISOStandard2017,
	author = {Bunt, Harry and Petukhova, Volha and Traum, David and Alexandersson, Jan},
	year = {2017},
	month = {11},
	pages = {109-135},
	title = {Dialogue Act Annotation with the ISO 24617-2 Standard},
	isbn = {978-3-319-42814-7},
	doi = {10.1007/978-3-319-42816-1_6}
}

@inproceedings{Core1997CodingDW,
	title={Coding Dialogs with the DAMSL Annotation Scheme},
	author={Mark G. Core and James F. Allen},
	year={1997}
}

@inproceedings{chowdhury-etal-2016-transfer,
	title = "Transfer of Corpus-Specific Dialogue Act Annotation to {ISO} Standard: Is it worth it?",
	author = "Chowdhury, Shammur Absar  and
	Stepanov, Evgeny  and
	Riccardi, Giuseppe",
	booktitle = "Proceedings of the Tenth International Conference on Language Resources and Evaluation ({LREC} 2016)",
	month = may,
	year = "2016",
	address = "Portoro{\v{z}}, Slovenia",
	publisher = "European Language Resources Association (ELRA)",
	url = "https://www.aclweb.org/anthology/L16-1020",
	pages = "132--135",
	abstract = "Spoken conversation corpora often adapt existing Dialogue Act (DA) annotation specifications, such as DAMSL, DIT++, etc., to task specific needs, yielding incompatible annotations; thus, limiting corpora re-usability. Recently accepted ISO standard for DA annotation {--} Dialogue Act Markup Language (DiAML) {--} is designed as domain and application independent. Moreover, the clear separation of dialogue dimensions and communicative functions, coupled with the hierarchical organization of the latter, allows for classification at different levels of granularity. However, re-annotating existing corpora with the new scheme might require significant effort. In this paper we test the utility of the ISO standard through comparative evaluation of the corpus-specific legacy and the semi-automatically transferred DiAML DA annotations on supervised dialogue act classification task. To test the domain independence of the resulting annotations, we perform cross-domain and data aggregation evaluation. Compared to the legacy annotation scheme, on the Italian LUNA Human-Human corpus, the DiAML annotation scheme exhibits better cross-domain and data aggregation classification performance, while maintaining comparable in-domain performance.",
}

@article{doi:10.1162/089120100561737,
	author = {Stolcke, Andreas and Ries, Klaus and Coccaro, Noah and Shriberg, Elizabeth and Bates, Rebecca and Jurafsky, Daniel and Taylor, Paul and Martin, Rachel and Ess-Dykema, Carol Van and Meteer, Marie},
	title = {Dialogue Act Modeling for Automatic Tagging and Recognition of Conversational Speech},
	journal = {Computational Linguistics},
	volume = {26},
	number = {3},
	pages = {339-373},
	year = {2000},
	doi = {10.1162/089120100561737},
	
	URL = { 
	https://doi.org/10.1162/089120100561737
	
	},
	eprint = { 
	https://doi.org/10.1162/089120100561737
	
	}
	,
	abstract = { We describe a statistical approach for modeling dialogue acts in conversational speech, i.e., speech-act-like units such as STATEMENT, Question, BACKCHANNEL, Agreement, Disagreement, and Apology. Our model detects and predicts dialogue acts based on lexical, collocational, and prosodic cues, as well as on the discourse coherence of the dialogue act sequence. The dialogue model is based on treating the discourse structure of a conversation as a hidden Markov model and the individual dialogue acts as observations emanating from the model states. Constraints on the likely sequence of dialogue acts are modeled via a dialogue act n-gram. The statistical dialogue grammar is combined with word n-grams, decision trees, and neural networks modeling the idiosyncratic lexical and prosodic manifestations of each dialogue act. We develop a probabilistic integration of speech recognition with dialogue modeling, to improve both speech recognition and dialogue act classification accuracy. Models are trained and evaluated using a large hand-labeled database of 1,155 conversations from the Switchboard corpus of spontaneous human-to-human telephone speech. We achieved good dialogue act labeling accuracy (65\% based on errorful, automatically recognized words and prosody, and 71\% based on word transcripts, compared to a chance baseline accuracy of 35\% and human accuracy of 84\%) and a small reduction in word recognition error. }
}

@inproceedings{rieser2005corpus,
	title={A corpus collection and annotation framework for learning multimodal clarification strategies},
	author={Rieser, Verena and Kruijff-Korbayov{\'a}, Ivana and Lemon, Oliver},
	booktitle={6th SIGdial Workshop on DISCOURSE and DIALOGUE},
	year={2005}
}

@inproceedings{bertomeu2006contextual,
	title={Contextual phenomena and thematic relations in database QA dialogues: results from a Wizard-of-Oz experiment},
	author={Bertomeu, N{\'u}ria and Uszkoreit, Hans and Frank, Anette and Krieger, Hans-Ulrich and J{\"o}rg, Brigitte},
	booktitle={Proceedings of the Interactive Question Answering Workshop at HLT-NAACL 2006},
	pages={1--8},
	year={2006}
}


@inproceedings{benzmuller2006corpus,
	title={A corpus of tutorial dialogs on theorem proving; the influence of the presentation of the study-material},
	author={Benzm{\"u}ller, Christoph and Horacek, Helmut and Lesourd, Henri and Kruijff-Korbayov{\'a}, Ivana and Schiller, Marvin and Wolska, Magdalena},
	booktitle={Proceedings of the Fifth International Conference on Language Resources and Evaluation (LREC’06)},
	year={2006}
}

@inproceedings{pineda2002dime,
	title={The DIME project},
	author={Pineda, Luis Alberto and Mass{\'e}, Antonio and Meza, Ivan and Salas, Miguel and Schwarz, Eric and Uraga, Esmeralda and Villase{\~n}or, Luis},
	booktitle={Mexican International Conference on Artificial Intelligence},
	pages={166--175},
	year={2002},
	organization={Springer}
}

@article{georgila2010match,
	title={The MATCH corpus: a corpus of older and younger users’ interactions with spoken dialogue systems},
	author={Georgila, Kallirroi and Wolters, Maria and Moore, Johanna D and Logie, Robert H},
	journal={Language Resources and Evaluation},
	volume={44},
	number={3},
	pages={221--261},
	year={2010},
	publisher={Springer}
}

@article{frames,
	author    = {Layla El Asri and
	Hannes Schulz and
	Shikhar Sharma and
	Jeremie Zumer and
	Justin Harris and
	Emery Fine and
	Rahul Mehrotra and
	Kaheer Suleman},
	title     = {Frames: {A} Corpus for Adding Memory to Goal-Oriented Dialogue Systems},
	journal   = {CoRR},
	volume    = {abs/1704.00057},
	year      = {2017},
	url       = {http://arxiv.org/abs/1704.00057},
	archivePrefix = {arXiv},
	eprint    = {1704.00057},
	timestamp = {Mon, 13 Aug 2018 16:48:29 +0200},
	biburl    = {https://dblp.org/rec/bib/journals/corr/AsriSSZHFMS17},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{multiwoz,
	author    = {Pawel Budzianowski and
	Tsung{-}Hsien Wen and
	Bo{-}Hsiang Tseng and
	I{\~{n}}igo Casanueva and
	Stefan Ultes and
	Osman Ramadan and
	Milica Gasic},
	title     = {MultiWOZ - {A} Large-Scale Multi-Domain Wizard-of-Oz Dataset for Task-Oriented
	Dialogue Modelling},
	journal   = {CoRR},
	volume    = {abs/1810.00278},
	year      = {2018},
	url       = {http://arxiv.org/abs/1810.00278},
	archivePrefix = {arXiv},
	eprint    = {1810.00278},
	timestamp = {Tue, 30 Oct 2018 10:49:09 +0100},
	biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1810-00278},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@INPROCEEDINGS{1374824, 
	author={A. {Green} and H. {Huttenrauch} and K. S. {Eklundh}}, 
	booktitle={RO-MAN 2004. 13th IEEE International Workshop on Robot and Human Interactive Communication (IEEE Catalog No.04TH8759)}, 
	title={Applying the Wizard-of-Oz framework to cooperative service discovery and configuration}, 
	year={2004}, 
	volume={}, 
	number={}, 
	pages={575-580}, 
	keywords={service robots;interactive systems;cooperative systems;mobile robots;man-machine systems;Wizard-of-Oz framework;cooperative service discovery;cooperative service configuration;service robotics scenario;multimodal dialogue;dialogue production tool;joystick navigation tool;home tour scenario;simulation tools;Cognitive robotics;Virtual prototyping;Face;Laboratories;Collaboration;Production;Navigation;Service robots;Humans;Interactive systems}, 
	doi={10.1109/ROMAN.2004.1374824}, 
	ISSN={}, 
	month={Sep.},}

@article{negotiationannotation,
	author = {Tenbrink, Thora and Eberhard, Kathleen and Shi, Hui and Kübler, Sandra and Scheutz, Matthias},
	year = {2013},
	month = {01},
	pages = {185–214},
	title = {Annotation of negotiation processes in joint action dialogues},
	volume = {4},
	journal = {Dialogue \& Discourse},
	doi = {10.5087/dad.2013.209}
}

@inproceedings{Lala:2016:MIA:2993148.2998528,
	author = {Lala, Divesh and Milhorat, Pierrick and Inoue, Koji and Zhao, Tianyu and Kawahara, Tatsuya},
	title = {Multimodal Interaction with the Autonomous Android ERICA},
	booktitle = {Proceedings of the 18th ACM International Conference on Multimodal Interaction},
	series = {ICMI '16},
	year = {2016},
	isbn = {978-1-4503-4556-9},
	location = {Tokyo, Japan},
	pages = {417--418},
	numpages = {2},
	url = {http://doi.acm.org/10.1145/2993148.2998528},
	doi = {10.1145/2993148.2998528},
	acmid = {2998528},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {gaze behavior, human-robot interaction, speech},
}

@inproceedings{cahn1999psychological,
	title={A psychological model of grounding and repair in dialog},
	author={Cahn, Janet E and Brennan, Susan E},
	booktitle={Proc. Fall 1999 AAAI Symposium on Psychological Models of Communication in Collaborative Systems},
	year={1999}
}

@article{clark1989contributing,
	title={Contributing to discourse},
	author={Clark, Herbert H and Schaefer, Edward F},
	journal={Cognitive science},
	volume={13},
	number={2},
	pages={259--294},
	year={1989},
	publisher={Elsevier}
}

@article{white2018skill,
	title={Skill discovery in virtual assistants},
	author={White, Ryen W},
	journal={Communications of the ACM},
	volume={61},
	number={11},
	pages={106--113},
	year={2018},
	publisher={ACM}
}

@inproceedings{kang2018data,
	title={Data Collection for Dialogue System: A Startup Perspective},
	author={Kang, Yiping and Zhang, Yunqi and Kummerfeld, Jonathan K and Tang, Lingjia and Mars, Jason},
	booktitle={Proceedings of the 2018 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 3 (Industry Papers)},
	volume={3},
	pages={33--40},
	year={2018}
}

@inproceedings{gangadharaiah2018we,
	title={What we need to learn if we want to do and not just talk},
	author={Gangadharaiah, Rashmi and Narayanaswamy, Balakrishnan and Elkan, Charles},
	booktitle={Proceedings of the 2018 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 3 (Industry Papers)},
	volume={3},
	pages={25--32},
	year={2018}
}

@article{tenbrink2013annotation,
	title={Annotation of negotiation processes in joint-action dialogues},
	author={Tenbrink, Thora and Eberhard, Kathleen and Shi, Hui and Kuebler, Sandra and Scheutz, Matthias},
	journal={Dialogue \& Discourse},
	volume={4},
	number={2},
	pages={185--214},
	year={2013}
}

@article{bach1979linguistic,
	title={Linguistic Communication and Speech Acts},
	author={Bach, K and Harnish, R},
	year={1979}
}

@inproceedings{mccowan2005ami,
	title={The AMI meeting corpus},
	author={McCowan, Iain and Carletta, Jean and Kraaij, W and Ashby, S and Bourban, S and Flynn, M and Guillemot, M and Hain, T and Kadlec, J and Karaiskos, V and others},
	booktitle={Proceedings of the 5th International Conference on Methods and Techniques in Behavioral Research},
	volume={88},
	pages={100},
	year={2005}
}

@inproceedings{kumar2018dialogue,
	title={Dialogue act sequence labeling using hierarchical encoder with crf},
	author={Kumar, Harshit and Agarwal, Arvind and Dasgupta, Riddhiman and Joshi, Sachindra},
	booktitle={Thirty-Second AAAI Conference on Artificial Intelligence},
	year={2018}
}

@inproceedings{chen2018dialogue,
	title={Dialogue act recognition via crf-attentive structured network},
	author={Chen, Zheqian and Yang, Rongqin and Zhao, Zhou and Cai, Deng and He, Xiaofei},
	booktitle={The 41st International ACM SIGIR Conference on Research \& Development in Information Retrieval},
	pages={225--234},
	year={2018},
	organization={ACM}
}

@article{riek2012wizard,
	title={Wizard of oz studies in hri: a systematic review and new reporting guidelines},
	author={Riek, Laurel D},
	journal={Journal of Human-Robot Interaction},
	volume={1},
	number={1},
	pages={119--136},
	year={2012},
	publisher={Journal of Human-Robot Interaction Steering Committee}
}

@article{hajdinjak2006paradise,
	title={The PARADISE evaluation framework: Issues and findings},
	author={Hajdinjak, Melita and Miheli{\v{c}}, France},
	journal={Computational Linguistics},
	volume={32},
	number={2},
	pages={263--272},
	year={2006},
	publisher={MIT Press}
}

@inproceedings{benzmuller2003wizard,
	title={A Wizard-of-Oz experiment for tutorial dialogues in mathematics},
	author={Benzm{\"u}ller, Christoph and Fiedler, Armin and Gabsdil, Malte and Horacek, Helmut and Kruijff-korbayov{\'a}, Ivana and Pinkal, Manfred and Siekmann, J{\"o}rg and Tsovaltzi, Dimitra and Vo, Bao Quoc and Wolska, Magdalena},
	booktitle={In Proceedings of the AIED Workshop on Advanced Technologies for Mathematics Education},
	year={2003},
	organization={Citeseer}
}

@inproceedings{schatzmann2007agenda,
	title={Agenda-based user simulation for bootstrapping a POMDP dialogue system},
	author={Schatzmann, Jost and Thomson, Blaise and Weilhammer, Karl and Ye, Hui and Young, Steve},
	booktitle={Human Language Technologies 2007: The Conference of the North American Chapter of the Association for Computational Linguistics; Companion Volume, Short Papers},
	pages={149--152},
	year={2007},
	organization={Association for Computational Linguistics}
}

@inproceedings{kruijff2006sammie,
	title={The SAMMIE Corpus of Multimodal Dialogues with an MP3 Player.},
	author={Kruijff-Korbayov{\'a}, Ivana and Becker, Tilman and Blaylock, Nate and Gerstenberger, Ciprian and Kaisser, Michael and Poller, Peter and Rieser, Verena and Schehl, Jan},
	booktitle={LREC},
	pages={2018--2023},
	year={2006}
}

@article{ullerwizard,
	title={A Wizard-of-Oz Experiment for Tutorial Dialogues in Mathematics},
	author={ULLER, Christoph BENZM and FIEDLER, Armin and GABSDIL, Malte and HORACEK, Helmut and PINKAL, Manfred and SIEKMANN, J{\"o}rg and TSOVALTZI, Dimitra and Bao Quoc, VO and WOLSKA, Magdalena}
}

@article{dahlback1993wizard,
	title={Wizard of Oz studies—why and how},
	author={Dahlb{\"a}ck, Nils and J{\"o}nsson, Arne and Ahrenberg, Lars},
	journal={Knowledge-based systems},
	volume={6},
	number={4},
	pages={258--266},
	year={1993},
	publisher={Elsevier}
}

@article{robillard2009makes,
	title={What makes APIs hard to learn? Answers from developers},
	author={Robillard, Martin P},
	journal={IEEE software},
	volume={26},
	number={6},
	pages={27--34},
	year={2009}
}

@book{rieser2011reinforcement,
	title={Reinforcement learning for adaptive dialogue systems: a data-driven methodology for dialogue management and natural language generation},
	author={Rieser, Verena and Lemon, Oliver},
	year={2011},
	publisher={Springer Science \& Business Media}
}

@inproceedings{Howison:2011:SSP:1958824.1958904,
	author = {Howison, James and Herbsleb, James D.},
	title = {Scientific Software Production: Incentives and Collaboration},
	booktitle = {Proceedings of the ACM 2011 Conference on Computer Supported Cooperative Work},
	series = {CSCW '11},
	year = {2011},
	isbn = {978-1-4503-0556-3},
	location = {Hangzhou, China},
	pages = {513--522},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1958824.1958904},
	doi = {10.1145/1958824.1958904},
	acmid = {1958904},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {scholarly publishing, scientific software, software development, software ecosystem},
} 

@inproceedings{arnaoudova2015use,
	title={The use of text retrieval and natural language processing in software engineering},
	author={Arnaoudova, Venera and Haiduc, Sonia and Marcus, Andrian and Antoniol, Giuliano},
	booktitle={Proceedings of the 37th International Conference on Software Engineering-Volume 2},
	pages={949--950},
	year={2015},
	organization={IEEE Press}
}

@inproceedings{bradley2018context,
	title={Context-aware conversational developer assistants},
	author={Bradley, Nick C and Fritz, Thomas and Holmes, Reid},
	booktitle={Proceedings of the 40th International Conference on Software Engineering},
	pages={993--1003},
	year={2018},
	organization={ACM}
}

@article{pruski2015tiqi,
	title={TiQi: answering unstructured natural language trace queries},
	author={Pruski, Piotr and Lohar, Sugandha and Goss, William and Rasin, Alexander and Cleland-Huang, Jane},
	journal={Requirements Engineering},
	volume={20},
	number={3},
	pages={215--232},
	year={2015},
	publisher={Springer}
}

@inproceedings{ko2004designing,
	title={Designing the whyline: a debugging interface for asking questions about program behavior},
	author={Ko, Andrew J and Myers, Brad A},
	booktitle={Proceedings of the SIGCHI conference on Human factors in computing systems},
	pages={151--158},
	year={2004},
	organization={ACM}
}

@inproceedings{tian2017apibot,
	title={APIBot: Question answering bot for API documentation},
	author={Tian, Yuan and Thung, Ferdian and Sharma, Abhishek and Lo, David},
	booktitle={2017 32nd IEEE/ACM International Conference on Automated Software Engineering (ASE)},
	pages={153--158},
	year={2017},
	organization={IEEE}
}

@article{robillard2011field,
	title={A field study of API learning obstacles},
	author={Robillard, Martin P and Deline, Robert},
	journal={Empirical Software Engineering},
	volume={16},
	number={6},
	pages={703--732},
	year={2011},
	publisher={Springer}
}

@article{monperrus2012should,
	title={What should developers be aware of? An empirical study on the directives of API documentation},
	author={Monperrus, Martin and Eichberg, Michael and Tekes, Elif and Mezini, Mira},
	journal={Empirical Software Engineering},
	volume={17},
	number={6},
	pages={703--737},
	year={2012},
	publisher={Springer}
}

@article{maalej2014comprehension,
	title={On the comprehension of program comprehension},
	author={Maalej, Walid and Tiarks, Rebecca and Roehm, Tobias and Koschke, Rainer},
	journal={ACM Transactions on Software Engineering and Methodology (TOSEM)},
	volume={23},
	number={4},
	pages={31},
	year={2014},
	publisher={ACM}
}

@inproceedings{head2018not,
	title={When not to comment: questions and tradeoffs with API documentation for C++ projects},
	author={Head, Andrew and Sadowski, Caitlin and Murphy-Hill, Emerson and Knight, Andrea},
	booktitle={Proceedings of the 40th International Conference on Software Engineering},
	pages={643--653},
	year={2018},
	organization={ACM}
}

@inproceedings{aghajani2018large,
	title={A large-scale empirical study on linguistic antipatterns affecting apis},
	author={Aghajani, Emad and Nagy, Csaba and Bavota, Gabriele and Lanza, Michele},
	booktitle={2018 IEEE International Conference on Software Maintenance and Evolution (ICSME)},
	pages={25--35},
	year={2018},
	organization={IEEE}
}

@ARTICLE{1041053, 
	author={G. {Antoniol} and G. {Canfora} and G. {Casazza} and A. {De Lucia} and E. {Merlo}}, 
	journal={IEEE Transactions on Software Engineering}, 
	title={Recovering traceability links between code and documentation}, 
	year={2002}, 
	volume={28}, 
	number={10}, 
	pages={970-983}, 
	keywords={system documentation;information retrieval;object-oriented programming;natural languages;probability;software system documentation;information retrieval;object orientation;traceability;program comprehension;traceability link recovery;source code;free text documents;vector space;Documentation;Programming profession;Information retrieval;Natural languages;Context modeling;Information resources;Writing;Java;Inspection;Mathematics}, 
	doi={10.1109/TSE.2002.1041053}, 
	ISSN={0098-5589}, 
	month={Oct},}

@article {Sparrow776,
	author = {Sparrow, Betsy and Liu, Jenny and Wegner, Daniel M.},
	title = {Google Effects on Memory: Cognitive Consequences of Having Information at Our Fingertips},
	volume = {333},
	number = {6043},
	pages = {776--778},
	year = {2011},
	doi = {10.1126/science.1207745},
	publisher = {American Association for the Advancement of Science},
	abstract = {The advent of the Internet, with sophisticated algorithmic search engines, has made accessing information as easy as lifting a finger. No longer do we have to make costly efforts to find the things we want. We can {\textquotedblleft}Google{\textquotedblright} the old classmate, find articles online, or look up the actor who was on the tip of our tongue. The results of four studies suggest that when faced with difficult questions, people are primed to think about computers and that when people expect to have future access to information, they have lower rates of recall of the information itself and enhanced recall instead for where to access it. The Internet has become a primary form of external or transactive memory, where information is stored collectively outside ourselves.},
	issn = {0036-8075},
	URL = {https://science.sciencemag.org/content/333/6043/776},
	eprint = {https://science.sciencemag.org/content/333/6043/776.full.pdf},
	journal = {Science}
}


@article{Xu2018Graph2SeqGT,
	title={Graph2Seq: Graph to Sequence Learning with Attention-based Neural Networks},
	author={Kun Xu and Lingfei Wu and Zhiguo Wang and Yansong Feng and Vadim Sheinin},
	journal={ArXiv},
	year={2018},
	volume={abs/1804.00823}
}

@article{krippendorff2011agreement,
	title={Agreement and information in the reliability of coding},
	author={Krippendorff, Klaus},
	journal={Communication Methods and Measures},
	volume={5},
	number={2},
	pages={93--112},
	year={2011},
	publisher={Taylor \& Francis}
}

@article{BENGTSSON20168,
	title = "How to plan and perform a qualitative study using content analysis",
	journal = "NursingPlus Open",
	volume = "2",
	pages = "8 - 14",
	year = "2016",
	issn = "2352-9008",
	doi = "https://doi.org/10.1016/j.npls.2016.01.001",
	url = "http://www.sciencedirect.com/science/article/pii/S2352900816000029",
	author = "Mariette Bengtsson",
	keywords = "Content analysis, Credibility, Qualitative design, Research process",
	abstract = "This paper describes the research process – from planning to presentation, with the emphasis on credibility throughout the whole process – when the methodology of qualitative content analysis is chosen in a qualitative study. The groundwork for the credibility initiates when the planning of the study begins. External and internal resources have to be identified, and the researcher must consider his or her experience of the phenomenon to be studied in order to minimize any bias of his/her own influence. The purpose of content analysis is to organize and elicit meaning from the data collected and to draw realistic conclusions from it. The researcher must choose whether the analysis should be of a broad surface structure (a manifest analysis) or of a deep structure (a latent analysis). Four distinct main stages are described in this paper: the decontextualisation, the recontextualisation, the categorization, and the compilation. This description of qualitative content analysis offers one approach that shows how the general principles of the method can be used."
}

@article{spooren2010coding,
	title={Coding coherence relations: Reliability and validity},
	author={Spooren, Wilbert and Degand, Liesbeth},
	journal={Corpus linguistics and linguistic theory},
	volume={6},
	number={2},
	pages={241--266},
	year={2010},
	publisher={Walter de Gruyter GmbH \& Co. KG}
}

@article{meng2018application,
	title={Application programming interface documentation: what do software developers want?},
	author={Meng, Michael and Steinhardt, Stephanie and Schubert, Andreas},
	journal={Journal of Technical Writing and Communication},
	volume={48},
	number={3},
	pages={295--330},
	year={2018},
	publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{racz20144fx,
	title={4FX: Light verb constructions in a multilingual parallel corpus},
	author={R{\'a}cz, Anita and Nagy, T and Vincze, Veronika and others},
	year={2014},
	publisher={ELRA}
}

@inproceedings{schloder2015clarifying,
	title={Clarifying intentions in dialogue: A corpus study},
	author={Schl{\"o}der, Julian J and Fern{\'a}ndez, Raquel},
	booktitle={Proceedings of the 11th International Conference on Computational Semantics},
	pages={46--51},
	year={2015}
}

@article{maalej2013patterns,
	title={Patterns of knowledge in API reference documentation},
	author={Maalej, Walid and Robillard, Martin P},
	journal={IEEE Transactions on Software Engineering},
	volume={39},
	number={9},
	pages={1264--1282},
	year={2013},
	publisher={IEEE}
}

@article{downe1992content,
	title={Content analysis: method, applications, and issues},
	author={Downe-Wamboldt, Barbara},
	journal={Health care for women international},
	volume={13},
	number={3},
	pages={313--321},
	year={1992},
	publisher={Taylor \& Francis}
}

@article{witte2008text,
	title={Text mining and software engineering: an integrated source code and document analysis approach},
	author={Witte, Ren{\'e} and Li, Qiangqiang and Zhang, Yonggang and Rilling, Juergen},
	journal={IET software},
	volume={2},
	number={1},
	pages={3--16},
	year={2008},
	publisher={IET}
}

@inproceedings{wiebe2005creating,
	title={Creating subjective and objective sentence classifiers from unannotated texts},
	author={Wiebe, Janyce and Riloff, Ellen},
	booktitle={International conference on intelligent text processing and computational linguistics},
	pages={486--497},
	year={2005},
	organization={Springer}
}

@misc{chollet2015keras,
  title={Keras},
  author={Chollet, Fran\c{c}ois and others},
  year={2015},
  publisher={GitHub},
  howpublished={\url{https://github.com/fchollet/keras}},
}

@inproceedings{stoyanov2008topic,
	title={Topic identification for fine-grained opinion analysis},
	author={Stoyanov, Veselin and Cardie, Claire},
	booktitle={Proceedings of the 22nd International Conference on Computational Linguistics-Volume 1},
	pages={817--824},
	year={2008},
	organization={Association for Computational Linguistics}
}

@inproceedings{wood2018detecting,
	title={Detecting Speech Act Types in Developer Question/Answer Conversations During Bug Repair},
	author={Wood, Andrew and Rodeghero, Paige and Armaly, Ameer and McMillan, Collin},
	booktitle={Proc. of the 26th ACM Symposium on the Foundations of Software Engineering},
	year={2018}
}

@article{serban2015survey,
	title={A survey of available corpora for building data-driven dialogue systems},
	author={Serban, Iulian Vlad and Lowe, Ryan and Henderson, Peter and Charlin, Laurent and Pineau, Joelle},
	journal={arXiv preprint arXiv:1512.05742},
	year={2015}
}

@misc{brown2017conversational,
	title={Conversational virtual healthcare assistant},
	author={Brown, Fred A and Lawrence, Mitchell G and Morrison, Victor O'Brien},
	year={2017},
	month=nov # "~21",
	publisher={Google Patents},
	note={US Patent 9,824,188}
}

@inproceedings{lv2015virtual,
	title={Virtual reality assistant technology for learning primary geography},
	author={Lv, Zhihan and Li, Xiaoming},
	booktitle={International Conference on Web-Based Learning},
	pages={31--40},
	year={2015},
	organization={Springer}
}

@inproceedings{robillard2017demand,
	title={On-demand developer documentation},
	author={Robillard, Martin P and Marcus, Andrian and Treude, Christoph and Bavota, Gabriele and Chaparro, Oscar and Ernst, Neil and Gerosa, Marco Aur{\'e}lio and Godfrey, Michael and Lanza, Michele and Linares-V{\'a}squez, Mario and others},
	booktitle={Software Maintenance and Evolution (ICSME), 2017 IEEE International Conference on},
	pages={479--483},
	year={2017},
	organization={IEEE}
}

@inproceedings{boehm2006view,
	title={A view of 20th and 21st century software engineering},
	author={Boehm, Barry},
	booktitle={Proceedings of the 28th international conference on Software engineering},
	pages={12--29},
	year={2006},
	organization={ACM}
}

 @inproceedings{wan2018reinforcement,
 author = {Wan, Yao and Zhao, Zhou and Yang, Min and Xu, Guandong and Ying, Haochao and Wu, Jian and Yu, Philip S.},
 title = {Improving Automatic Source Code Summarization via Deep Reinforcement Learning},
 year = {2018},
 isbn = {9781450359375},
 publisher = {Association for Computing Machinery},
 address = {New York, NY, USA},
 url = {https://doi.org/10.1145/3238147.3238206},
 doi = {10.1145/3238147.3238206},
 booktitle = {Proceedings of the 33rd ACM/IEEE International Conference on Automated Software Engineering},
 pages = {397–407},
 numpages = {11},
 keywords = {deep learning, reinforcement learning, Code summarization, comment generation},
 location = {Montpellier, France},
 series = {ASE 2018}
}



@inproceedings{lewis2017deal,
	title={Deal or No Deal? End-to-End Learning of Negotiation Dialogues},
	author={Lewis, Mike and Yarats, Denis and Dauphin, Yann and Parikh, Devi and Batra, Dhruv},
	booktitle={Proceedings of the 2017 Conference on Empirical Methods in Natural Language Processing},
	pages={2443--2453},
	year={2017}
}

@article{chen2019sequencer,
	title={Sequencer: Sequence-to-sequence learning for end-to-end program repair},
	author={Chen, Zimin and Kommrusch, Steve James and Tufano, Michele and Pouchet, Louis-No{\"e}l and Poshyvanyk, Denys and Monperrus, Martin},
	journal={IEEE Transactions on Software Engineering},
	year={2019},
	publisher={IEEE}
}

@inproceedings{hayati2018retrieval,
	title={Retrieval-Based Neural Code Generation},
	author={Hayati, Shirley Anugrah and Olivier, Raphael and Avvaru, Pravalika and Yin, Pengcheng and Tomasic, Anthony and Neubig, Graham},
	booktitle={Proceedings of the 2018 Conference on Empirical Methods in Natural Language Processing},
	pages={925--930},
	year={2018}
}

@inproceedings{lin2019task,
	title={Task-Oriented Conversation Generation Using Heterogeneous Memory Networks},
	author={Lin, Zehao and Huang, Xinjing and Ji, Feng and Chen, Haiqing and Zhang, Ying},
	booktitle={Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing},
	year={2019}
}

@inproceedings{li2016deep,
	title={Deep Reinforcement Learning for Dialogue Generation},
	author={Li, Jiwei and Monroe, Will and Ritter, Alan and Jurafsky, Dan and Galley, Michel and Gao, Jianfeng},
	booktitle={Proceedings of the 2016 Conference on Empirical Methods in Natural Language Processing},
	pages={1192--1202},
	year={2016}
}

@inproceedings{he2018decoupling,
	title={Decoupling Strategy and Generation in Negotiation Dialogues},
	author={He, He and Chen, Derek and Balakrishnan, Anusha and Liang, Percy},
	booktitle={Proceedings of the 2018 Conference on Empirical Methods in Natural Language Processing},
	pages={2333--2343},
	year={2018}
}

@inproceedings{schmidt2018industrial,
	title={Industrial Virtual Assistants: Challenges and Opportunities},
	author={Schmidt, Benedikt and Borrison, Reuben and Cohen, Andrew and Dix, Marcel and G{\"a}rtler, Marco and Hollender, Martin and Kl{\"o}pper, Benjamin and Maczey, Sylvia and Siddharthan, Shunmuga},
	booktitle={Proceedings of the 2018 ACM International Joint Conference and 2018 International Symposium on Pervasive and Ubiquitous Computing and Wearable Computers},
	pages={794--801},
	year={2018},
	organization={ACM}
}

@inproceedings{whittaker2002fish,
	title={Fish or Fowl: A Wizard of Oz Evaluation of Dialogue Strategies in the Restaurant Domain.},
	author={Whittaker, Steve and Walker, Marilyn A and Moore, Johanna D},
	booktitle={LREC},
	year={2002}
}

@article{fernandes2019structured,
  author    = {Patrick Fernandes and
               Miltiadis Allamanis and
               Marc Brockschmidt},
  title     = {Structured Neural Summarization},
  journal   = {CoRR},
  volume    = {abs/1811.01824},
  year      = {2018},
  url       = {http://arxiv.org/abs/1811.01824},
  archivePrefix = {arXiv},
  eprint    = {1811.01824},
  timestamp = {Thu, 22 Nov 2018 17:58:30 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1811-01824},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@ARTICLE{doshi2017interpretableml,
       author = {{Doshi-Velez}, Finale and {Kim}, Been},
        title = "{Towards A Rigorous Science of Interpretable Machine Learning}",
      journal = {arXiv e-prints},
     keywords = {Statistics - Machine Learning, Computer Science - Artificial Intelligence, Computer Science - Machine Learning},
         year = "2017",
        month = "Feb",
          eid = {arXiv:1702.08608},
        pages = {arXiv:1702.08608},
archivePrefix = {arXiv},
       eprint = {1702.08608},
 primaryClass = {stat.ML},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017arXiv170208608D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{rueden2019informed,
    title={Informed Machine Learning - Towards a Taxonomy of Explicit Integration of Knowledge into Machine Learning},
    author={Laura von Rueden and Sebastian Mayer and Jochen Garcke and Christian Bauckhage and Jannis Schuecker},
    year={2019},
    eprint={1903.12394},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@INPROCEEDINGS{leclair2018codecat,
author={A. {LeClair} and Z. {Eberhart} and C. {McMillan}},
booktitle={2018 IEEE International Conference on Software Maintenance and Evolution (ICSME)},
title={Adapting Neural Text Classification for Improved Software Categorization},
year={2018},
volume={},
number={},
pages={461-472},
keywords={pattern classification;public domain software;software maintenance;text analysis;Debian end-user programs;maintenance tasks;feature elicitation;NLP domain;neural classification algorithm;software classification techniques;neural text classification technique;software categorization;source code classification;C/C++ libraries;Task analysis;Computer architecture;Software maintenance;Classification algorithms;Software algorithms;Vocabulary;source code categorization;neural classification;deep learning in software engineering},
doi={10.1109/ICSME.2018.00056},
ISSN={2576-3148},
month={Sep.},}

@INPROCEEDINGS{howard2013mappings,
author={M. J. {Howard} and S. {Gupta} and L. {Pollock} and K. {Vijay-Shanker}},
booktitle={2013 10th Working Conference on Mining Software Repositories (MSR)},
title={Automatically mining software-based, semantically-similar words from comment-code mappings},
year={2013},
volume={},
number={},
pages={377-386},
keywords={data mining;natural language processing;software maintenance;software tools;text analysis;software development tools;software maintenance tools;natural language words;software artifacts;textual artifact representation;synonyms;vocabulary mismatch;automatic mining software-based semantically-similar word mining;natural language documents;comment-code word mapping;WordNet;computer science;software traceability;Software;Context;Semantics;Computer science;Data mining;Tagging;Maintenance engineering},
doi={10.1109/MSR.2013.6624052},
ISSN={2160-1852},
month={May},}

@article{Arras2017explainabletext,
   title={“What is relevant in a text document?”: An interpretable machine learning approach},
   volume={12},
   ISSN={1932-6203},
   url={http://dx.doi.org/10.1371/journal.pone.0181142},
   DOI={10.1371/journal.pone.0181142},
   number={8},
   journal={PLOS ONE},
   publisher={Public Library of Science (PLoS)},
   author={Arras, Leila and Horn, Franziska and Montavon, Grégoire and Müller, Klaus-Robert and Samek, Wojciech},
   editor={Sidorov, GrigoriEditor},
   year={2017},
   month={Aug},
   pages={e0181142}
}

@article{gu2016copy,
   title={Incorporating Copying Mechanism in Sequence-to-Sequence Learning},
   url={http://dx.doi.org/10.18653/v1/P16-1154},
   DOI={10.18653/v1/p16-1154},
   journal={Proceedings of the 54th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
   publisher={Association for Computational Linguistics},
   author={Gu, Jiatao and Lu, Zhengdong and Li, Hang and Li, Victor O.K.},
   year={2016}
}


@misc{roscher2019explainable,
    title={Explainable Machine Learning for Scientific Insights and Discoveries},
    author={Ribana Roscher and Bastian Bohn and Marco F. Duarte and Jochen Garcke},
    year={2019},
    eprint={1905.08883},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}
@article{doran2017explainable,
  author    = {Derek Doran and
               Sarah Schulz and
               Tarek R. Besold},
  title     = {What Does Explainable {AI} Really Mean? {A} New Conceptualization
               of Perspectives},
  journal   = {CoRR},
  volume    = {abs/1710.00794},
  year      = {2017},
  url       = {http://arxiv.org/abs/1710.00794},
  archivePrefix = {arXiv},
  eprint    = {1710.00794},
  timestamp = {Mon, 13 Aug 2018 16:48:14 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1710-00794},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{MILLER2019explainai,
title = "Explanation in artificial intelligence: Insights from the social sciences",
journal = "Artificial Intelligence",
volume = "267",
pages = "1 - 38",
year = "2019",
issn = "0004-3702",
doi = "https://doi.org/10.1016/j.artint.2018.07.007",
url = "http://www.sciencedirect.com/science/article/pii/S0004370218305988",
author = "Tim Miller",
keywords = "Explanation, Explainability, Interpretability, Explainable AI, Transparency",
abstract = "There has been a recent resurgence in the area of explainable artificial intelligence as researchers and practitioners seek to provide more transparency to their algorithms. Much of this research is focused on explicitly explaining decisions or actions to a human observer, and it should not be controversial to say that looking at how humans explain to each other can serve as a useful starting point for explanation in artificial intelligence. However, it is fair to say that most work in explainable artificial intelligence uses only the researchers' intuition of what constitutes a ‘good’ explanation. There exist vast and valuable bodies of research in philosophy, psychology, and cognitive science of how people define, generate, select, evaluate, and present explanations, which argues that people employ certain cognitive biases and social expectations to the explanation process. This paper argues that the field of explainable artificial intelligence can build on this existing research, and reviews relevant papers from philosophy, cognitive psychology/science, and social psychology, which study these topics. It draws out some important findings, and discusses ways that these can be infused with work on explainable artificial intelligence."
}


@misc{tensorflow2015whitepaper,
title={ {TensorFlow}: Large-Scale Machine Learning on Heterogeneous Systems},
url={https://www.tensorflow.org/},
note={Software available from tensorflow.org},
author={
    Mart\'{\i}n~Abadi and
    Ashish~Agarwal and
    Paul~Barham and
    Eugene~Brevdo and
    Zhifeng~Chen and
    Craig~Citro and
    Greg~S.~Corrado and
    Andy~Davis and
    Jeffrey~Dean and
    Matthieu~Devin and
    Sanjay~Ghemawat and
    Ian~Goodfellow and
    Andrew~Harp and
    Geoffrey~Irving and
    Michael~Isard and
    Yangqing Jia and
    Rafal~Jozefowicz and
    Lukasz~Kaiser and
    Manjunath~Kudlur and
    Josh~Levenberg and
    Dandelion~Man\'{e} and
    Rajat~Monga and
    Sherry~Moore and
    Derek~Murray and
    Chris~Olah and
    Mike~Schuster and
    Jonathon~Shlens and
    Benoit~Steiner and
    Ilya~Sutskever and
    Kunal~Talwar and
    Paul~Tucker and
    Vincent~Vanhoucke and
    Vijay~Vasudevan and
    Fernanda~Vi\'{e}gas and
    Oriol~Vinyals and
    Pete~Warden and
    Martin~Wattenberg and
    Martin~Wicke and
    Yuan~Yu and
    Xiaoqiang~Zheng},
  year={2015},
}
